Large Scale Earth's Bow Shock with Northern IMF as simulated by PIC code in parallel with MHD model

In this paper, we propose a 3D kinetic model (Particle-in-Cell PIC ) for the description of the large scale Earth's bow shock. The proposed version is stable and does not require huge or extensive computer resources. Because PIC simulations work with scaled plasma and field parameters, we also propose to validate our code by comparing its results with the available MHD simulations under same scaled Solar wind ( SW ) and ( IMF ) conditions. We report new results from the two models. In both codes the Earth's bow shock position is found to be ~14.8 RE along the Sun-Earth line, and ~ 29 RE on the dusk side. Those findings are consistent with past in situ observations. Both simulations reproduce the theoretical jump conditions at the shock. However, the PIC code density and temperature distributions are inflated and slightly shifted sunward when compared to the MHD results. Kinetic electron motions and reflected ions upstream may cause this sunward shift. Species distributions in the foreshock region are depicted within the transition of the shock (measured ~2 c/{\omega}pi for {\Theta}Bn =90o and MMS =4.7 ) and in the downstream. The size of the foot jump in the magnetic field at the shock is measured to be (1.7 c/{\omega}pi ). In the foreshocked region, the thermal velocity is found equal to 213 km.sec-1 at 15 RE and is equal to 63 km.sec-1at 12 RE (Magnetosheath region). Despite the large cell size of the current version of the PIC code, it is powerful to retain macrostructure of planets magnetospheres in very short time, thus it can be used for a pedagogical test purposes. It is also likely complementary with MHD to deepen our understanding of the large scale magnetosphere

==> baraka <==
% This file was created with JabRef 2.10.
% Encoding: UTF8


@Article{Oieroset2001,
  Title                    = {{In situ detection of collisionless reconnection in the Earth's magnetotail}},
  Author                   = {{\O}ieroset, M and Phan, T D and Fujimoto, M and Lin, R P and Lepping, R P},
  Journal                  = {Nature},
  Year                     = {2001},
  Number                   = {6845},
  Pages                    = {414--417},
  Volume                   = {412},

  __markedentry            = {[suleimanbaraka:6]},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/{\O}ieroset et al/Nature/Phan et al. - 2001 - In situ detection of collisionless reconnection in the Earth ' s magnetotail.pdf:pdf},
  Owner                    = {suleimanbaraka},
  Publisher                = {Nature Publishing Group},
  Timestamp                = {2016.02.23}
}

@Article{Abbot2003,
  Title                    = {Seasonal and interannual variability of {North} {American} isoprene emissions as determined by formaldehyde column measurements from space},
  Author                   = {Abbot, Dorian S. and Palmer, Paul I. and Martin, Randall V. and Chance, Kelly V. and Jacob, Daniel J. and Guenther, Alex},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2003},
  Number                   = {17},
  Volume                   = {30},

  Doi                      = {10.1029/2003GL017336/full},
  Urldate                  = {2014-11-13}
}

@Article{Abe1993,
  Title                    = {{EXOS} {D} ({Akebono}) suprathermal mass spectrometer observations of the polar wind},
  Author                   = {Abe, T. and Whalen, B. A. and Yau, A. W. and Horita, R. E. and Watanabe, S. and Sagawa, E.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1993},

  Month                    = jul,
  Pages                    = {11191},
  Volume                   = {98},

  Doi                      = {10.1029/92JA01971}
}

@Article{Abe1993a,
  Title                    = {{EXOS} {D} ({Akebono}) suprathermal mass spectrometer observations of the polar wind},
  Author                   = {Abe, T and Whalen, BA and Yau, AW},
  Journal                  = {{\textbackslash}ldots Sp. Phys. (1978 {\textbackslash}ldots},
  Year                     = {1993},

  Doi                      = {10.1029/92JA01971/full}
}

@Article{Abe2004,
  Title                    = {Long-term variation of the polar wind velocity and its implication for the ion acceleration process: {Akebono}/suprathermal ion mass spectrometer observations},
  Author                   = {Abe, Takumi and Yau, Andrew W and Watanabe, Shigeto and Yamada, Manabu and Sagawa, Eiichi},
  Journal                  = {J. Geophys. Res. Sp. Phys.},
  Year                     = {2004},
  Number                   = {A9},
  Volume                   = {109}
}

@Article{Achilleos2006,
  Title                    = {Orientation, location, and velocity of {Saturn}'s bow shock: {Initial} results from the {Cassini} spacecraft},
  Author                   = {Achilleos, N and Bertucci, C and Russell, CT and Hospodarsky, GB and Rymer, AM and Arridge, CS and Burton, ME and Dougherty, MK and Hendricks, S and Smith, EJ and {others}},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2006},
  Number                   = {A3},
  Volume                   = {111}
}

@InProceedings{Adamson2012,
  Title                    = {3-{D} mesoscale {MHD} simulations of magnetospheric cusp-like configurations: cusp diamagnetic cavities and boundary structure},
  Author                   = {Adamson, E. and Otto, A. and Nykyri, K.},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2012},
  Pages                    = {325--341},
  Publisher                = {Copernicus GmbH},
  Volume                   = {30},

  Shorttitle               = {3-{D} mesoscale {MHD} simulations of magnetospheric cusp-like configurations},
  Url                      = {http://www.ann-geophys.net/30/325/2012/},
  Urldate                  = {2014-10-22}
}

@Article{Akasofu1980,
  Title                    = {The solar wind-magnetosphere energy coupling and magnetospheric disturbances},
  Author                   = {Akasofu, S-I},
  Journal                  = {Planetary and space science},
  Year                     = {1980},
  Number                   = {5},
  Pages                    = {495--509},
  Volume                   = {28}
}

@Article{Alexandrova2006,
  Title                    = {Alfvén vortex filaments observed in magnetosheath downstream of a quasi-perpendicular bow shock},
  Author                   = {Alexandrova, O and Mangeney, A and Maksimovic, M and Cornilleau-Wehrlin, N and Bosqued, J-M and André, Mats},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2006},
  Number                   = {A12},
  Volume                   = {111}
}

@Article{Alexandrova2004,
  Title                    = {Cluster observations of finite amplitude {Alfvén} waves and small-scale magnetic filaments downstream of a quasi-perpendicular shock},
  Author                   = {Alexandrova, O and Mangeney, A and Maksimovic, M and Lacombe, C and Cornilleau-Wehrlin, N and Lucek, EA and Décréau, PME and Bosqued, J-M and Travnicek, P and Fazakerley, AN},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2004},
  Number                   = {A5},
  Volume                   = {109}
}

@Article{Alexeev1998,
  Title                    = {Concerning the location of magnetopause merging as a function of the magnetopause current strength},
  Author                   = {Alexeev, I. I. and Sibeck, D. G. and Bobrovnikov, S. Y.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1998},
  Pages                    = {6675--6684},
  Volume                   = {103},

  Abstract                 = {We start from an assumption that merging occurs in regions of the magnetopause where current strengths are greater than some threshold value which corresponds to the total jump in the field across the magnetopause greater than 50 nT. Because time and cost constraints preclude running numerical simulations for a wide variety of interplanetary magnetic field (IMF) orientations to determine these locations, we adopt an analytical model based on previously derived formulations for magnetospheric and magnetosheath magnetic fields. The magnetospheric magnetic field is confined within a paraboloid. The magnetosheath magnetic field is derived from that in the solar wind and lies between the magnetopause and a paraboloid bow shock. We allow a slight diffusion of the magnetosheath magnetic field into the magnetosphere. The results of the model show that during periods of due southward IMF orientation, merging occurs (as expected) in a wide region centered on the subsolar magnetopause. During periods of northward IMF, connection continues near the subsolar point but also poleward of the cusps. Magnetic energy is only released to the plasma in the latter regions. During periods of strongly northward IMF (B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater}=0), reconnection ceases on the subsolar magnetopause but continues poleward of the cusp. If the IMF points northward but B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater} is nonzero, reconnection continues near the subsolar point and poleward of the cusps. During periods of sunward IMF orientation, merging nearly ceases on the northern hemisphere (except in the vicinity of the subsolar point) but continues outside the southern lobes. Dawnward and duskward IMF orientations produce tilted patches of enhanced current densities in the subsolar region. We compare the results of our model with previous predictions of the “component” and “antiparallel” merging models.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Current systems Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetospheric configuration and dynamics Space Plasma Physics: Magnetic reconnection},
  Url                      = {http://adsabs.harvard.edu/abs/1998JGR...103.6675A}
}

@Article{Andr,
  Title                    = {The {ULF} wave foreshock boundary {Cluster} observations},
  Author                   = {Andr, Nahuel},
  Number                   = {Cp 1428},
  Pages                    = {1--12},
  Volume                   = {47890179},

  Keywords                 = {cluster spacecraft, earth, interplanetary magnetic field, particle accel-, s foreshock, ulf waves}
}

@Article{Andre1998,
  Title                    = {Ion energization mechanisms at 1700 km in the auroral region},
  Author                   = {André, M. and Norqvist, P. and Andersson, L. and Eliasson, L. and Eriksson, A. I. and Blomberg, L. and Erlandson, R. E. and Waldemark, J.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1998},

  Month                    = mar,
  Pages                    = {4199--4222},
  Volume                   = {103},

  Doi                      = {10.1029/97JA00855},
  Keywords                 = {Ionosphere: Ionosphere/magnetosphere interactions, Ionosphere: Particle acceleration, Magnetospheric Physics: Auroral phenomena, Space Plasma Physics: Wave/particle interactions}
}

@Article{Andre1997,
  Title                    = {Theories and {Observations} of {Ion} {Energization} and {Outflow} in the {High} {Latitude} {Magnetosphere}},
  Author                   = {Andre, M. and Yau, A.},
  Journal                  = {ßr},
  Year                     = {1997},

  Month                    = apr,
  Pages                    = {27--48},
  Volume                   = {80},

  Doi                      = {10.1023/A:1004921619885}
}

@Article{Andre1997a,
  Title                    = {Theories and {Observations} of {Ion} {Energization} and {Outflow} in the {High} {Latitude} {Magnetosphere}},
  Author                   = {Andre, M. and Yau, A.},
  Journal                  = {√ür},
  Year                     = {1997},

  Month                    = apr,
  Pages                    = {27--48},
  Volume                   = {80},

  Doi                      = {10.1023/A:1004921619885}
}

@Article{Andres2013,
  Title                    = {Effects of electron inertia in collisionless magnetic reconnection},
  Author                   = {Andrés, Nahuel and Martin, Luis and Dmitruk, Pablo and Gómez, Daniel},
  Journal                  = {arXiv preprint arXiv:1312.2437},
  Year                     = {2013},

  Url                      = {http://arxiv.org/abs/1312.2437},
  Urldate                  = {2014-05-31}
}

@Article{Andr√©1998,
  Title                    = {Ion energization mechanisms at 1700 km in the auroral region},
  Author                   = {Andr√©, M. and Norqvist, P. and Andersson, L. and Eliasson, L. and Eriksson, A. I. and Blomberg, L. and Erlandson, R. E. and Waldemark, J.},
  Journal                  = {{\textbackslash}textbackslashjgr},
  Year                     = {1998},

  Month                    = mar,
  Pages                    = {4199--4222},
  Volume                   = {103},

  Doi                      = {10.1029/97JA00855},
  Keywords                 = {Ionosphere: Ionosphere/magnetosphere interactions, Ionosphere: Particle acceleration, Magnetospheric Physics: Auroral phenomena, Space Plasma Physics: Wave/particle interactions}
}

@Article{Angelopoulos2008a,
  Title                    = {Tail {Reconnection} {Triggering} {Substorm} {Onset}},
  Author                   = {Angelopoulos, Vassilis and McFadden, James P. and Larson, Davin and Carlson, Charles W. and Mende, Stephen B. and Frey, Harald and Phan, Tai and Sibeck, David G. and Glassmeier, Karl-Heinz and Auster, Uli and Donovan, Eric and Mann, Ian R. and Rae, I. Jonathan and Russell, Christopher T. and Runov, Andrei and Zhou, Xu-Zhi and Kepko, Larry},
  Journal                  = {Science},
  Year                     = {2008},
  Pages                    = {931--},
  Volume                   = {321},

  Abstract                 = {Magnetospheric substorms explosively release solar wind energy previously stored in Earth’s magnetotail, encompassing the entire magnetosphere and producing spectacular auroral displays. It has been unclear whether a substorm is triggered by a disruption of the electrical current flowing across the near-Earth magnetotail, at 10 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} (R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}: Earth radius, or 6374 kilometers), or by the process of magnetic reconnection typically seen farther out in the magnetotail, at 20 to 30 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}. We report on simultaneous measurements in the magnetotail at multiple distances, at the time of substorm onset. Reconnection was observed at 20 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}, at least 1.5 minutes before auroral intensification, at least 2 minutes before substorm expansion, and about 3 minutes before near-Earth current disruption. These results demonstrate that substorms are likely initiated by tail reconnection.},
  ISSN                     = {0036-8075},
  Url                      = {http://adsabs.harvard.edu/abs/2008Sci...321..931A}
}

@Article{Angelopoulos2008,
  Title                    = {{Tail reconnection triggering substorm onset.}},
  Author                   = {Angelopoulos, Vassilis and McFadden, James P and Larson, Davin and Carlson, Charles W and Mende, Stephen B and Frey, Harald and Phan, T. D. and Sibeck, David G and Glassmeier, Karl-Heinz and Auster, Uli and Donovan, Eric and Mann, Ian R and Rae, I Jonathan and Russell, Christopher T and Runov, Andrei and Zhou, Xu-Zhi and Kepko, Larry},
  Journal                  = {Science},
  Year                     = {2008},
  Number                   = {5891},
  Pages                    = {931--5},
  Volume                   = {321},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {Magnetospheric substorms explosively release solar wind energy previously stored in Earth's magnetotail, encompassing the entire magnetosphere and producing spectacular auroral displays. It has been unclear whether a substorm is triggered by a disruption of the electrical current flowing across the near-Earth magnetotail, at approximately 10 R(E) (R(E): Earth radius, or 6374 kilometers), or by the process of magnetic reconnection typically seen farther out in the magnetotail, at approximately 20 to 30 R(E). We report on simultaneous measurements in the magnetotail at multiple distances, at the time of substorm onset. Reconnection was observed at 20 R(E), at least 1.5 minutes before auroral intensification, at least 2 minutes before substorm expansion, and about 3 minutes before near-Earth current disruption. These results demonstrate that substorms are likely initiated by tail reconnection.},
  Doi                      = {10.1126/science.1160495},
  ISBN                     = {1095-9203 (Electronic)$\backslash$r0036-8075 (Linking)},
  ISSN                     = {1095-9203},
  Owner                    = {suleimanbaraka},
  Pmid                     = {18653845},
  Timestamp                = {2016.02.23},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/18653845}
}

@Article{Angelopoulos2008b,
  Title                    = {First {Results} from the {THEMIS} {Mission}},
  Author                   = {Angelopoulos, V. and Sibeck, D. and Carlson, C. W. and McFadden, J. P. and Larson, D. and Lin, R. P. and Bonnell, J. W. and Mozer, F. S. and Ergun, R. and Cully, C. and Glassmeier, K. H. and Auster, U. and Roux, A. and Lecontel, O. and Frey, S. and Phan, T. and Mende, S. and Frey, H. and Donovan, E. and Russell, C. T. and Strangeway, R. and Liu, J. and Mann, I. and Rae, J. and Raeder, J. and Li, X. and Liu, W. and Singer, H. J. and Sergeev, V. A. and Apatenkov, S. and Parks, G. and Fillingim, M. and Sigwarth, J.},
  Journal                  = {Space Science Reviews},
  Year                     = {2008},
  Pages                    = {453--476},
  Volume                   = {141},

  Abstract                 = {THEMIS was launched on February 17, 2007 to determine the trigger and large-scale evolution of substorms. During the first seven months of the mission the five satellites coasted near their injection orbit to avoid differential precession in anticipation of orbit placement, which started in September 2007 and led to a commencement of the baseline mission in December 2007. During the coast phase the probes were put into a string-of-pearls configuration at 100 s of km to 2 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} along-track separations, which provided a unique view of the magnetosphere and enabled an unprecedented dataset in anticipation of the first tail season. In this paper we describe the first THEMIS substorm observations, captured during instrument commissioning on March 23, 2007. THEMIS measured the rapid expansion of the plasma sheet at a speed that is commensurate with the simultaneous expansion of the auroras on the ground. These are the first unequivocal observations of the rapid westward expansion process in space and on the ground. Aided by the remote sensing technique at energetic particle boundaries and combined with ancillary measurements and MHD simulations, they allow determination and mapping of space currents. These measurements show the power of the THEMIS instrumentation in the tail and the radiation belts. We also present THEMIS Flux Transfer Events (FTE) observations at the magnetopause, which demonstrate the importance of multi-point observations there and the quality of the THEMIS instrumentation in that region of space.},
  ISSN                     = {0038-6308},
  Url                      = {http://adsabs.harvard.edu/abs/2008SSRv..141..453A}
}

@Article{Antiochos2012,
  Title                    = {The {Structure} and {Dynamics} of the {Corona}{\textbackslash}{mdashHeliosphere} {Connection}},
  Author                   = {Antiochos, S. K. and Linker, J. A. and Lionello, R. and Mikić, Z. and Titov, V. and Zurbuchen, T. H.},
  Journal                  = {ßr},
  Year                     = {2012},

  Month                    = nov,
  Pages                    = {169--185},
  Volume                   = {172},

  Doi                      = {10.1007/s11214-011-9795-7},
  Keywords                 = {Sun: corona, Sun: solar wind}
}

@Article{Appleton1932,
  Title                    = {Suggested {Wireless} {Observations} during the {Solar} {Eclipse} of {August} 31, 1932},
  Author                   = {Appleton, E. V. and Chapman, S.},
  Journal                  = {{\textbackslash}nat},
  Year                     = {1932},

  Month                    = may,
  Pages                    = {757--758},
  Volume                   = {129},

  Doi                      = {10.1038/129757a0}
}

@Article{Archer2013,
  Title                    = {Magnetospheric response to magnetosheath pressure pulses: {A} low-pass filter effect},
  Author                   = {Archer, M. O. and Horbury, T. S. and Eastwood, J. P. and Weygand, J. M. and Yeoman, T. K.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = sep,
  Pages                    = {5454--5466},
  Volume                   = {118},

  Doi                      = {10.1002/jgra.50519},
  Keywords                 = {magnetosheath, magnetosphere, pressure, TCV, ULF, waves}
}

@Article{Archer2014,
  Title                    = {Global impacts of a {Foreshock} {Bubble}: {Magnetosheath}, magnetopause and ground-based observations},
  Author                   = {Archer, M O and Turner, D L and Eastwood, J P and Schwartz, S J and Horbury, T S},
  Year                     = {2014},
  Pages                    = {1--24},

  Keywords                 = {dynamics, foreshock, magnetosphere, pressure, transient}
}

@InProceedings{Arndt2000,
  Title                    = {X-{Ray} and {Gamma} {Ray} {Measurements} of the 15 {November} 1991 {Solar} {Flare}},
  Author                   = {Arndt, Martina B and Connors, Alanna and McConnell, Mark and Ryan, James M and Suleiman, Raid and Young, C Alex and Bennett, Kevin and Rank, Gerhard and Schönfelder, Volker},
  Booktitle                = {High {Energy} {Solar} {Physics} {Workshop}-{Anticipating} {Hess}!},
  Year                     = {2000},
  Pages                    = {451},
  Volume                   = {206}
}

@Article{Artemyev2012,
  Title                    = {Kinetic {Structure} of {Current} {Sheets} in the {Earth} {Magnetotail}},
  Author                   = {Artemyev, Anton and Zelenyi, Lev},
  Journal                  = {Space Sci. Rev.},
  Year                     = {2012},

  Month                    = dec,
  Number                   = {2-4},
  Pages                    = {419--440},
  Volume                   = {178},

  Doi                      = {10.1007/s11214-012-9954-5},
  ISSN                     = {0038-6308},
  Keywords                 = {current sheets, earth magnetotail, kinetic models},
  Url                      = {http://link.springer.com/10.1007/s11214-012-9954-5}
}

@InProceedings{Arvelius2005,
  Title                    = {Statistics of high-altitude and high-latitude {O}{\textless} sup{\textgreater}+{\textless}/sup{\textgreater} ion outflows observed by {Cluster}/{CIS}},
  Author                   = {Arvelius, S and Yamauchi, M and Nilsson, H and Lundin, R and Hobara, Y and Reme, H and Bavassano-Cattaneo, M B and Paschmann, G and Korth, A and Kistler, L M and {Others}},
  Booktitle                = {Ann. {Geophys}.},
  Year                     = {2005},
  Pages                    = {1909--1916},
  Volume                   = {23}
}

@Article{Arvelius2005a,
  Title                    = {Statistics of high-altitude and high-latitude {O}$^{\textrm{+\$}}$ ion outflows observed by {Cluster}/{CIS}},
  Author                   = {Arvelius, S. and Yamauchi, M. and Nilsson, H. and Lundin, R. and Hobara, Y. and Rème, H. and Bavassano-Cattaneo, M. B. and Paschmann, G. and Korth, A. and Kistler, L. M. and Parks, G. K.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2005},

  Month                    = jul,
  Pages                    = {1909--1916},
  Volume                   = {23},

  Doi                      = {10.5194/angeo-23-1909-2005}
}

@Article{Arvelius2005b,
  Title                    = {Statistics of high-altitude and high-latitude {O}$^{\textrm{+\$}}$\$ ion outflows observed by {Cluster}/{CIS}},
  Author                   = {Arvelius, S. and Yamauchi, M. and Nilsson, H. and Lundin, R. and Hobara, Y. and R√®me, H. and Bavassano-Cattaneo, M. B. and Paschmann, G. and Korth, A. and Kistler, L. M. and Parks, G. K.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2005},

  Month                    = jul,
  Pages                    = {1909--1916},
  Volume                   = {23},

  Doi                      = {10.5194/angeo-23-1909-2005}
}

@Article{Asbridge1968,
  Title                    = {Outward flow of protons from the earth's bow shock},
  Author                   = {Asbridge, JR and Bame, SJ and Strong, IB},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1968},
  Number                   = {17},
  Pages                    = {5777--5782},
  Volume                   = {73}
}

@Article{Asplund2009,
  Title                    = {The {Chemical} {Composition} of the {Sun}},
  Author                   = {Asplund, M. and Grevesse, N. and Sauval, A. J. and Scott, P.},
  Journal                  = {{\textbackslash}araa},
  Year                     = {2009},

  Month                    = sep,
  Pages                    = {481--522},
  Volume                   = {47},

  Doi                      = {10.1146/annurev.astro.46.060407.145222}
}

@Article{Aubry1970,
  Title                    = {Inward motion of the magnetopause before a substorm},
  Author                   = {Aubry, Michel P and Russell, Christopher T and Kivelson, Margaret G},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1970},
  Number                   = {34},
  Pages                    = {7018--7031},
  Volume                   = {75}
}

@Article{Aubry1970a,
  Title                    = {Inward motion of the magnetopause before a substorm},
  Author                   = {Aubry, M. P. and Russell, C. T. and Kivelson, M. G.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1970},
  Pages                    = {7018},
  Volume                   = {75},

  Abstract                 = {On March 27, 1968, the UCLA magnetometer on board the inbound Ogo 5 satellite recorded an inward motion of the magnetopause by about 2 RE in two hours. It is shown that this inward motion was associated with a reversal of the vertical component of the interplanetary field from northward to southward, the solar wind momentum flux remaining constant. The inward shift did not produce any compression of the magnetospheric cavity, which implies a transfer of magnetic flux from the dayside magnetosphere to the tail: the Imp 4 satellite saw the magnetic tail field increasing at the end of this interval and later the substorm-associated collapse of this field. The substorm was also recorded on the ground. It is emphasized that the position of the magnetopause after the inward shift cannot be explained in terms of the available numerical models.},
  Doi                      = {10.1029/JA075i034p07018},
  Keywords                 = {Particles and Fields in the Earth's Magnetosphere: Magnetic storms, Particles and Fields in the Earth's Magnetosphere: Magnetosheath}
}

@Article{Aunai2013,
  Title                    = {Electron nongyrotropy in the context of collisionless magnetic reconnection},
  Author                   = {Aunai, Nicolas and Hesse, Michael and Kuznetsova, Maria},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2013},
  Number                   = {9},
  Pages                    = {092903},
  Volume                   = {20},

  Url                      = {http://scitation.aip.org/content/aip/journal/pop/20/9/10.1063/1.4820953},
  Urldate                  = {2014-05-31}
}

@Article{Axford1962,
  Title                    = {The interaction between the solar wind and the earth's magnetosphere},
  Author                   = {Axford, WI},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1962},
  Number                   = {10},
  Pages                    = {3791--3796},
  Volume                   = {67}
}

@InCollection{Baker2005,
  Title                    = {Specifying and forecasting space weather threats to human technology},
  Author                   = {Baker, Daniel N},
  Booktitle                = {Effects of {Space} {Weather} on {Technology} {Infrastructure}},
  Publisher                = {Springer},
  Year                     = {2005},
  Pages                    = {1--25}
}

@Article{Baker2002,
  Title                    = {How to cope with space weather},
  Author                   = {Baker, Daniel N},
  Journal                  = {Science},
  Year                     = {2002},
  Number                   = {5586},
  Pages                    = {1486--1487},
  Volume                   = {297},

  Url                      = {http://www.sciencemag.org/content/297/5586/1486.short}
}

@Article{Baker1995,
  Title                    = {Lidar-measured winds from space: a key component for weather and climate prediction},
  Author                   = {Baker, Wayman E and Emmitt, George D and Robertson, Franklin and Atlas, Robert M and Molinari, John E and Bowdle, David A and Paegle, Jan and Hardesty, R Michael and Post, Madison J and Menzies, Robert T and {others}},
  Journal                  = {Bull. Amer. Meteor. Soc.},
  Year                     = {1995},
  Number                   = {6},
  Pages                    = {869--888},
  Volume                   = {76},

  Url                      = {http://journals.ametsoc.org/doi/abs/10.1175/1520-0477(1995)076%3C0869:LMWFSA%3E2.0.CO%3B2}
}

@Article{Balch2008,
  Title                    = {Updated verification of the {Space} {Weather} {Prediction} {Center}'s solar energetic particle prediction model},
  Author                   = {Balch, Christopher C},
  Journal                  = {Space Weather},
  Year                     = {2008},
  Number                   = {1},
  Volume                   = {6}
}

@Article{,
  Title                    = {Quasi-perpendicular shock structure and processes},
  Author                   = {Bale, SD and Balikhin, MA and Horbury, TS and Krasnoselskikh, VV and Kucharek, H and Möbius, E and Walker, SN and Balogh, A and Burgess, D and Lembège, Bertrand and {others}},
  Journal                  = {Space science reviews},
  Year                     = {2005},
  Number                   = {1-4},
  Pages                    = {161--203},
  Volume                   = {118}
}

@Article{Bale2003,
  Title                    = {Density-{Transition} {Scale} at {Quasiperpendicular} {Collisionless} {Shocks}},
  Author                   = {Bale, S. and Mozer, F. and Horbury, T.},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2003},

  Month                    = dec,
  Number                   = {26},
  Pages                    = {265004},
  Volume                   = {91},

  Doi                      = {10.1103/PhysRevLett.91.265004},
  ISSN                     = {0031-9007},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.91.265004}
}

@Article{Bale2008,
  Title                    = {Direct measurement of the cross-shock electric potential at low plasma \$\${\textbackslash}backslash\$ beta \$, quasi-perpendicular bow shocks},
  Author                   = {Bale, SD and Mozer, FS and Krasnoselskikh, VV},
  Journal                  = {arXiv preprint arXiv:0809.2435},
  Year                     = {2008}
}

@Article{Bale2005,
  Title                    = {Chapter 5 {Quasi}-perpendicular {Shock} {Structure} and {Processes}},
  Author                   = {Bale, S D and Balikhin, M A and Horbury, T S and Krasnoselskikh, V V and Kucharek, H and Walker, S N and Balogh, A and Burgess, D and Lemb, B and Lucek, E A and Scholer, M and Schwartz, S J and Thomsen, M F},
  Year                     = {2005},
  Pages                    = {161--203},

  Doi                      = {10.1007/s11214-005-3827-0}
}

@Article{Bale2003a,
  Title                    = {Density-{Transition} {Scale} at {Quasiperpendicular} {Collisionless} {Shocks}},
  Author                   = {Bale, S D and Mozer, F S},
  Year                     = {2003},
  Number                   = {December},
  Pages                    = {1--4},

  Doi                      = {10.1103/PhysRevLett.91.265004}
}

@Article{Balikhin2009,
  Title                    = {{THEMIS observations of mirror structures: Magnetic holes and instability threshold}},
  Author                   = {Balikhin, M. A. and Sagdeev, R. Z. and Walker, S. N. and Pokhotelov, O. A. and Sibeck, D. G. and Beloff, N. and Dudnikova, G.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2009},
  Number                   = {3},
  Volume                   = {36},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {Nonpropagating mirror-mode structures are commonly observed in many regions of natural plasma such as solar wind, planetary magnetosheaths, in cometary plasma, Io wake, terrestrial ring current and even on the outskirts of solar system. Mirror structures are typically observed in the shape of magnetic holes or peaks. Fast survey mode plasma data from the THEMIS satellites are used to solve the puzzle of how mirror structures in the form of dips can be observed in the regions of mirror stable plasma. THEMIS data also show that for mirror structures with spatial scales that considerably exceed ion Larmor radius the perpendicular temperature anticorrelates with the strength of the magnetic field. This contradiction with the conservation of adiabatic invariants is explained by the role of trapped particles. Citation: Balikhin, M. A., R. Z. Sagdeev, S. N. Walker, O. A. Pokhotelov, D. G. Sibeck, N. Beloff, and G. Dudnikova (2009), THEMIS observations of mirror structures: Magnetic holes and instability threshold, Geophys. Res. Lett., 36, L03105, doi:10.1029/ 2008GL036923.},
  Doi                      = {10.1029/2008GL036923},
  ISBN                     = {00948276},
  ISSN                     = {00948276},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Balikhin2009a,
  Title                    = {{THEMIS} observations of mirror structures: {Magnetic} holes and instability threshold},
  Author                   = {Balikhin, M. A. and Sagdeev, R. Z. and Walker, S. N. and Pokhotelov, O. A. and Sibeck, D. G. and Beloff, N. and Dudnikova, G.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2009},
  Pages                    = {3105},
  Volume                   = {36},

  Abstract                 = {Nonpropagating mirror-mode structures are commonly observed in many regions of natural plasma such as solar wind, planetary magnetosheaths, in cometary plasma, Io wake, terrestrial ring current and even on the outskirts of solar system. Mirror structures are typically observed in the shape of magnetic holes or peaks. Fast survey mode plasma data from the THEMIS satellites are used to solve the puzzle of how mirror structures in the form of dips can be observed in the regions of mirror stable plasma. THEMIS data also show that for mirror structures with spatial scales that considerably exceed ion Larmor radius the perpendicular temperature anticorrelates with the strength of the magnetic field. This contradiction with the conservation of adiabatic invariants is explained by the role of trapped particles.},
  ISSN                     = {0094-8276},
  Keywords                 = {Space Plasma Physics: Kinetic waves and instabilities Magnetospheric Physics: Plasma waves and instabilities (2471) Magnetospheric Physics: Magnetosheath Radio Science: Nonlinear phenomena (4400 7839) Space Plasma Physics: Wave/particle interactions (2483 6984)},
  Url                      = {http://adsabs.harvard.edu/abs/2009GeoRL..36.3105B}
}

@Article{Balikhin2012,
  Title                    = {Magnetic holes in the vicinity of dipolarization fronts: {Mirror} or tearing structures?},
  Author                   = {Balikhin, M. A. and Sibeck, D. G. and Runov, A. and Walker, S. N.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2012},
  Pages                    = {8229},
  Volume                   = {117},

  Abstract                 = {Magnetic holes filled with isotropic energetic electrons (up to a few 10{\textless}SUP{\textgreater}5{\textless}/SUP{\textgreater} eV) have been observed by THEMIS in the vicinity of dipolarization fronts. These structures can partially contribute to the initial seed population of energetic electrons within the magnetosphere; therefore finding their nature is important for understanding of the population of high energy electrons within the magnetosphere. Previously, these structures have been interpreted as the result of the mirror instability due to the similarity in their appearance with mirror dips observed in the terrestrial magnetosheath and solar wind. The THEMIS data shown here prove that the measured properties of these structures contradict to the interpretation as mirror waves. In the present study it is shown that these waves do not exhibit the effects on the ion population that are expected due to mirror wave structures. However, they do have a pronounced effect on the high energy electron population. The evolution of the high energy electron population within these structures is investigated. It is then argued that the tearing instability can be responsible for their generation.},
  ISSN                     = {0148-0227},
  Keywords                 = {dipolarization Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Magnetotail Magnetospheric Physics: Plasma waves and instabilities (2471) Space Plasma Physics: Kinetic waves and instabilities Space Plasma Physics: Plasma energization},
  Url                      = {http://adsabs.harvard.edu/abs/2012JGRA..117.8229B}
}

@InProceedings{Balogh2001,
  Title                    = {The {Cluster} magnetic field investigation: {Overview} of in-flight performance and initial results},
  Author                   = {Balogh, A and Carr, CM and Acuna, MH and Dunlop, MW and Beek, TJ and Brown, P and Fornacon, K-H and Georgescu, E and Glassmeier, K-H and Harris, J and {others}},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2001},
  Pages                    = {1207--1217},
  Volume                   = {19}
}

@InCollection{Balogh1997,
  Title                    = {The {Cluster} magnetic field investigation},
  Author                   = {Balogh, A and Dunlop, MW and Cowley, SWH and Southwood, DJ and Thomlinson, JG and Glassmeier, KH and Musmann, G and Lühr, H and Buchert, S and Acuna, MH and {others}},
  Booktitle                = {The {Cluster} and {Phoenix} {Missions}},
  Publisher                = {Springer},
  Year                     = {1997},
  Pages                    = {65--91}
}

@Article{Balogh1997a,
  Title                    = {The {Cluster} {Magnetic} {Field} {Investigation}},
  Author                   = {Balogh, A. and Dunlop, M. W. and Cowley, S. W. H. and Southwood, D. J. and Thomlinson, J. G. and Glassmeier, K. H. and Musmann, G. and Luhr, H. and Buchert, S. and Acuna, M. H. and Fairfield, D. H. and Slavin, J. A. and Riedler, W. and Schwingenschuh, K. and Kivelson, M. G.},
  Journal                  = {ßr},
  Year                     = {1997},

  Month                    = jan,
  Pages                    = {65--91},
  Volume                   = {79},

  Doi                      = {10.1023/A:1004970907748}
}

@Article{Balogh1997b,
  Title                    = {The {Cluster} {Magnetic} {Field} {Investigation}},
  Author                   = {Balogh, A. and Dunlop, M. W. and Cowley, S. W. H. and Southwood, D. J. and Thomlinson, J. G. and Glassmeier, K. H. and Musmann, G. and Luhr, H. and Buchert, S. and Acuna, M. H. and Fairfield, D. H. and Slavin, J. A. and Riedler, W. and Schwingenschuh, K. and Kivelson, M. G.},
  Journal                  = {√ür},
  Year                     = {1997},

  Month                    = jan,
  Pages                    = {65--91},
  Volume                   = {79},

  Doi                      = {10.1023/A:1004970907748}
}

@InCollection{Balogh2005,
  Title                    = {Cluster at the bow shock: {Introduction}},
  Author                   = {Balogh, A and Schwartz, SJ and Bale, SD and Balikhin, MA and Burgess, D and Horbury, TS and Krasnoselskikh, VV and Kucharek, H and Lembege, B and Lucek, EA and {others}},
  Booktitle                = {Outer {Magnetospheric} {Boundaries}: {Cluster} {Results}},
  Publisher                = {Springer},
  Year                     = {2005},
  Pages                    = {155--160}
}

@InCollection{Balogh2013,
  Title                    = {Planetary {Bow} {Shocks}},
  Author                   = {Balogh, André and Treumann, Rudolf A},
  Booktitle                = {Physics of {Collisionless} {Shocks}},
  Publisher                = {Springer},
  Year                     = {2013},
  Pages                    = {411--461}
}

@Article{Balogh2004,
  Title                    = {The bimodal galaxy color distribution: dependence on luminosity and environment},
  Author                   = {Balogh, Michael L and Baldry, Ivan K and Nichol, Robert and Miller, Chris and Bower, Richard and Glazebrook, Karl},
  Journal                  = {The Astrophysical Journal Letters},
  Year                     = {2004},
  Number                   = {2},
  Pages                    = {L101},
  Volume                   = {615}
}

@Article{Balogh2001a,
  Title                    = {Revisiting the cosmic cooling crisis},
  Author                   = {Balogh, Michael L and Pearce, Frazer R and Bower, Richard G and Kay, Scott T},
  Journal                  = {Monthly Notices of the Royal Astronomical Society},
  Year                     = {2001},
  Number                   = {4},
  Pages                    = {1228--1234},
  Volume                   = {326}
}

@InProceedings{Barak,
  Title                    = {Ion to {Electron} {Mass} {Ratio} {Impact} on {MP} {Position}, {Three} {Parametric} {Case} {Studies}.},
  Author                   = {{Barak}},

  Address                  = {Montreal Canada},
  Editor                   = {Assembly, AGU Joint},
  Pages                    = {SPA34B--0364},
  Publisher                = {AGU}
}

@PhdThesis{Baraka2007,
  Title                    = {Etude de l'interactionentre le vent solaire et la magnetosphere de la {Terre}: {Modele} theorique et {Application} sur l'analyse de donnees de l'evenement du {Halloween} d'octobre 2003},
  Author                   = {Baraka, Suleiman},
  School                   = {Université Pierre et Marie Curie-Paris VI},
  Year                     = {2007},

  Url                      = {https://tel.archives-ouvertes.fr/tel-00138416/en/}
}

@InProceedings{Baraka2006,
  Title                    = {Sensitivity of the {Earth} {Magnetosphere} to the {Solar} {Wind} {Activity}: 3D {Macroparticle} {Model}},
  Author                   = {Baraka, SM and Ben Jaffel, L},
  Booktitle                = {{AGU} {Spring} {Meeting} {Abstracts}},
  Year                     = {2006},
  Pages                    = {03},
  Volume                   = {1},

  Url                      = {http://adsabs.harvard.edu/abs/2006AGUSMSM42A..03B}
}

@Article{Baraka2011,
  Title                    = {Impact of solar wind depression on the dayside magnetosphere under northward interplanetary magnetic field},
  Author                   = {Baraka, S. and Ben-Jaffel, L.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2011},

  Month                    = jan,
  Pages                    = {31--46},
  Volume                   = {29},

  Doi                      = {10.5194/angeo-29-31-2011}
}

@InProceedings{Baraka2011a,
  Title                    = {{PIC} {EM} {Relativistic} code is used to simulate the {Earth} bow shock},
  Author                   = {Baraka, SM and Ben-Jaffel, L},
  Booktitle                = {{AGU} {Fall} {Meeting} {Abstracts}},
  Year                     = {2011},
  Pages                    = {2032},
  Volume                   = {1},

  Url                      = {http://adsabs.harvard.edu/abs/2011AGUFMSM23A2032B}
}

@Article{Baraka2011b,
  Title                    = {Impact of solar wind depression on the dayside magnetosphere under northward interplanetary magnetic field},
  Author                   = {Baraka, S. and Ben-Jaffel, L.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2011},

  Month                    = jan,
  Pages                    = {31--46},
  Volume                   = {29},

  Doi                      = {10.5194/angeo-29-31-2011}
}

@Article{Baraka2010,
  Title                    = {Impact of solar wind depression on the dayside magnetosphere under northward interplanetary magnetic field},
  Author                   = {Baraka, Suleiman and Ben-Jaffel, Lotfi},
  Journal                  = {arXiv preprint arXiv:1012.5722},
  Year                     = {2010},

  Url                      = {http://arxiv.org/abs/1012.5722}
}

@Article{Baraka2007a,
  Title                    = {Sensitivity of the {Earth}√î√∏Œ©s magnetosphere to solar wind activity: {Three}-dimensional macroparticle model},
  Author                   = {Baraka, Suleiman and Ben-Jaffel, L},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2007},
  Number                   = {A6},
  Volume                   = {112}
}

@Article{Baraka2007b,
  Title                    = {Sensitivity of the {Earth}'s magnetosphere to solar wind activity: {Three}-dimensional macroparticle model},
  Author                   = {Baraka, S. and Ben-Jaffel, L.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2007},

  Month                    = jun,
  Pages                    = {6212},
  Volume                   = {112},

  Doi                      = {10.1029/2006JA011946},
  Keywords                 = {7835), Air pocket effect in solar wind flow, bow shock, dayside magnetopause boundary, Magnetic reconnection, magnetosphere expansion/recovery phase, Magnetospheric Physics: Magnetic reconnection (7526, Magnetospheric Physics: Magnetopause and boundary layers, Magnetospheric Physics: Magnetosphere: inner, Magnetospheric Physics: Magnetosphere: outer, Magnetospheric Physics: Plasma sheet, Magnetospheric Physics: Solar wind/magnetosphere interactions, particle in cell code, southward IMF}
}

@Article{Baraka2007c,
  Title                    = {Sensitivity of the {Earth}'s magnetosphere to solar wind activity: {Three}-dimensional macroparticle model},
  Author                   = {Baraka, S. and Ben-Jaffel, L.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2007},

  Month                    = jun,
  Pages                    = {A06212},
  Volume                   = {112},

  Doi                      = {10.1029/2006JA011946},
  Keywords                 = {7835), Air pocket effect in solar wind flow, bow shock, dayside magnetopause boundary, Magnetic reconnection, magnetosphere expansion/recovery phase, Magnetospheric Physics: Magnetic reconnection (7526, Magnetospheric Physics: Magnetopause and boundary layers, Magnetospheric Physics: Magnetosphere: inner, Magnetospheric Physics: Magnetosphere: outer, Magnetospheric Physics: Plasma sheet, Magnetospheric Physics: Solar wind/magnetosphere interactions, particle in cell code, southward IMF}
}

@InProceedings{Baraka2012,
  Title                    = {Particle-{In}-{Cell} {PIC} 3D and {MHD} simulations of the {Earth}'s {Bow} show.},
  Author                   = {Baraka, S. and Jaffel, L.},
  Booktitle                = {{EGU} {General} {Assembly} {Conference} {Abstracts}},
  Year                     = {2012},
  Editor                   = {Abbasi, A. and Giesen, N.},
  Month                    = apr,
  Pages                    = {6477},
  Series                   = {{EGU} {General} {Assembly} {Conference} {Abstracts}},
  Volume                   = {14},

  Abstract                 = {Particles-In-Cell (PIC) and magnetohydrodynamics (MHD) 3D models are used to simulate Earth's magnetosphere under similar solar wind (SW) and north interplanetary magnetic field (IMF) conditions. The bow shock's position is found by both codes at a distance of ∼14.8 RE along the Sun-Earth line, and ∼29 RE on the dusk side, consistent with past in situ observations. Based on our comparison, running PIC and MHD models under similar input SW parameters elucidates the strengths and drawbacks of these approaches and demonstrates the use of both models in a complementary, rather than competitive, manner for a better understanding of magnetospheres.}
}

@InProceedings{Baraka2014,
  Title                    = {3D {Simulation} of {Eareth}'s magentosphere by {Particle}-{In}-{Cell} and magnetohydrodynamics models: parameteric study},
  Author                   = {Baraka, SM and Jaffel, LB},
  Booktitle                = {{AGU} {Fall} {Meeting} {Abstracts}},
  Year                     = {2014},
  Pages                    = {4222},
  Volume                   = {1}
}

@InProceedings{Baraka2013,
  Title                    = {The unusual event of {Jan} 21st 2005 observed by {Cluster} spacecracts is considered for comparison by {PIC} {EM} {Relativistic} code simulation},
  Author                   = {Baraka, SM and Jaffel, LB and Dandouras, IS},
  Booktitle                = {{AGU} {Fall} {Meeting} {Abstracts}},
  Year                     = {2013},
  Pages                    = {2236},
  Volume                   = {1}
}

@Article{Baraka2006a,
  Title                    = {Sensitivity of the {Earth} {Magnetosphere} to the {Solar} {Wind} {Activity}: 3D {Macroparticle} {Model}},
  Author                   = {Baraka, S. M. and Ben Jaffel, L.},
  Journal                  = {AGU Spring Meeting Abstracts},
  Year                     = {2006},

  Month                    = may,
  Pages                    = {A3},

  Abstract                 = {A new approach is proposed to study the sensitivity of the Earth Magnetosphere to the variability of the Solar Wind bulk velocity. A numerical particles in cell (PIC) method initially proposed by Buneman (1993) has been adopted and modified to carry out the study. Space was stretched as cubic boxes of dimension 155x105x105 Re filled with 2 million of Solar Wind particles, with Earth is located at 60x52x53 Re. The magnetic field of Earth was hypothetically set to zero, and then switched on. The formation of the magnetospheric cavity and its elongation around the planet was observed to evolve with time until a steady state topology of the system is attained with the classical structure of a magnetosphere. We also found that the cavity is repopulated by clouds of particles from the Solar Wind, producing the current sheet– a thin plasma sheet that stands at the equatorial plane. The study was carried out with the very basic elements of the interaction processes as described by Maxwell and Lorentz equations. IMF was then included as a steady southward magnetic field. Drift velocity of the Solar Wind was changed to simulate compression/depression of the system. 3-D analysis of the response of the magnetosphere dayside to that variation was studied, and the corresponding relaxation time of the magnetopause interface was measured. In response to the Solar Wind drift velocity imposed drop-off, a ∼ 15 Re gap in the incoming Solar Wind plasma appeared moving toward Earth. As soon as the gap hit the initial shock of the steady magnetosphere, a reconnection between the Earth magnetic field and IMF was noticed at the dayside magnetopause when IMF was included. Injection of nightside of the magnetosphere by energetic particles due to magnetic erosion and reconnection is observed. During the expansion phase of the disturbance, the outer boundary of the dayside magnetopause broke up during the absence of the IMF as it responded to the reduction of the ram pressure, whilst sustained its bullet shape with a thin layer of plasma walling its boundary when a southward IMF was included. The expansion/contraction of the magnetopause nose position side was almost linear in the absence of IMF but shrank when IMF was included. Thanks to the complete view provided by the PIC code on particles and fields present in the system, a simple statistical and time analysis is presented aimed to explain the forces and physics processes in play during the travel of the depression gap through the simulation box. The system recovered to its initial state on the dayside soon after the impulse disturbance was beyond the Earth position},
  Keywords                 = {2724 Magnetopause and boundary layers, 2730 Magnetosphere: inner, 2731 Magnetosphere: outer, 2764 Plasma sheet, 2784 Solar wind/magnetosphere interactions}
}

@Article{Baraka2006b,
  Title                    = {Sensitivity of the {Earth} {Magnetosphere} to the {Solar} {Wind} {Activity}: 3D {Macroparticle} {Model}},
  Author                   = {Baraka, S. M. and Ben Jaffel, L.},
  Journal                  = {AGU Spring Meeting Abstracts},
  Year                     = {2006},

  Month                    = may,

  Keywords                 = {2724 Magnetopause and boundary layers, 2730 Magnetosphere: inner, 2731 Magnetosphere: outer, 2764 Plasma sheet, 2784 Solar wind/magnetosphere interactions}
}

@Article{Baraka2011c,
  Title                    = {{PIC} {EM} {Relativistic} code is used to simulate the {Earth} bow shock},
  Author                   = {Baraka, S. M. and Ben-Jaffel, L.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2011},

  Month                    = dec,
  Pages                    = {A2032},

  Abstract                 = {The Earth bow shock is created by the supersonic solar wind flowing onto the geomagnetic field. The front of this shock is curved, standing around the Earth from the dayside. The bow shock is of great interest in space plasma investigation as it contains important physics ranging from kinetic to global scales. Interaction of the supersonic solar wind with Earth magnetosphere (magnetopause) creates fast mode magnetosonic waves that travel back upstream, combine and steepen to form the bow shock wave. The distance to the bow shock is then the sum of the magnetopause distance and the magnetosheath thickness. [Merka and Szabo and references therein] It has been established been well established that the bow shock (and the magnetopause) scales with the solar wind ram pressure Psw[Binsack and Vasyliunas, 1968; Formisano, 1979] . We are trying though to simulate the position of the bow shock by using a modified Tristan PIC EM Relativistic Code. By doing so, we will help the science community to use our model to better understand the shock physics in our geospace.},
  Keywords                 = {2724 MAGNETOSPHERIC PHYSICS / Magnetopause and boundary layers, 2728 MAGNETOSPHERIC PHYSICS / Magnetosheath, 2784 MAGNETOSPHERIC PHYSICS / Solar wind/magnetosphere interactions}
}

@Article{Baraka2011d,
  Title                    = {{PIC} {EM} {Relativistic} code is used to simulate the {Earth} bow shock},
  Author                   = {Baraka, S. M. and Ben-Jaffel, L.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2011},

  Month                    = dec,

  Keywords                 = {2724 MAGNETOSPHERIC PHYSICS / Magnetopause and boundary layers, 2728 MAGNETOSPHERIC PHYSICS / Magnetosheath, 2784 MAGNETOSPHERIC PHYSICS / Solar wind/magnetosphere interactions}
}

@Article{Baraka2014a,
  Title                    = {Earth's {Magnetosphere} 3D {Simulation} by {Coupling} {Particle}-{In}-{Cell} and {Magnetohydrodynamics} {Models}: {Parametric} {Study}},
  Author                   = {Baraka, S. M. and Ben-Jaffel, L. B.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2014},

  Month                    = dec,
  Pages                    = {A4222},

  Abstract                 = {We use particle-in-cell PIC 3D Electromagnetic, relativistic global code to address large-scale problems in magnetosphere electrodynamics. Terrestrial bow shock is simulated as an example. 3D Magnetohydrodynamics model ,MHD GUMICS in CCMC project, have been used in parallel with PIC under same scaled Solar wind (SW) and IMF conditions. We report new results from the coupling between the two models. Further investigations are required for confirmations of these results. In both codes the Earth's bow shock position is found at ∼14.8 RE along the Sun-Earth line, and ∼29 RE on the dusk side which is consistent with past in situ observation. Both simulations reproduce the theoretical jump conditions at the shock. However, PIC code density and temperature distributions are inflated and slightly shifted sunward when compared to MHD results. Reflected ions upstream of the bow shock may cause this sunward shift for density and temperature. Distribution of reflected ions and electrons are shown in the foreshock region, within the transition of the shock and in the downstream. The current version of PIC code can be run under modest computing facilities and resources. Additionally, existing MHD simulations should be useful to calibrate scaled properties of plasma resulting from PIC simulations for comparison with observations. Similarities and drawbacks of the results obtained by the two models are listed. The ultimate goal of using these different models in a complimentary manner rather than competitive is to better understand the macrostructure of the magnetosphere},
  Keywords                 = {2723 Magnetic reconnection, 2724 Magnetopause and boundary layers, 2728 Magnetosheath, 2784 Solar wind/magnetosphere interactions}
}

@Article{Baraka2014b,
  Title                    = {Earth's {Magnetosphere} 3D {Simulation} by {Coupling} {Particle}-{In}-{Cell} and {Magnetohydrodynamics} {Models}: {Parametric} {Study}},
  Author                   = {Baraka, S. M. and Ben-Jaffel, L. B.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2014},

  Month                    = dec,

  Keywords                 = {2723 Magnetic reconnection, 2724 Magnetopause and boundary layers, 2728 Magnetosheath, 2784 Solar wind/magnetosphere interactions}
}

@Article{Baraka2013a,
  Title                    = {The unusual event of {Jan} 21st 2005 observed by {Cluster} spacecracts is considered for comparison by {PIC} {EM} {Relativistic} code simulation},
  Author                   = {Baraka, S. M. and Jaffel, L. B. and Dandouras, I. S.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2013},

  Month                    = dec,

  Keywords                 = {2724 MAGNETOSPHERIC PHYSICS Magnetopause and boundary layers, 5443 PLANETARY SCIENCES: SOLID SURFACE PLANETS Magnetospheres}
}

@Article{Baraka2013b,
  Title                    = {The unusual event of {Jan} 21st 2005 observed by {Cluster} spacecracts is considered for comparison by {PIC} {EM} {Relativistic} code simulation},
  Author                   = {Baraka, S. M. and Jaffel, L. B. and Dandouras, I. S.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2013},

  Month                    = dec,
  Pages                    = {B2236},

  Abstract                 = {The unusual event of Jan 21st 2005 observed by Cluster spacecrafts and other space instruments, has been considered for comparison with numerical simulations using a PIC EM Relativistic code for several solar wind plasma conditions. From the comparison using the results obtained so far, we could learn that the main difficulty of the simulation of strong events measured in situ is to properly define/find the undisturbed SW boundary conditions. The second lesson is that it is difficult for the strong and sharp jumps observed in the plasma properties to obtain a clear steady state of the magnetosphere that could be compared instantaneously with in situ measurements. We will show a detailed comparison of the plasma density, velocity components, and magnetic field components along the CL trajectory to the measured in situ data, stressing the added-value of using a PIC code to enrich our diagnostic about very short-term magnetospheric events.},
  Keywords                 = {2724 MAGNETOSPHERIC PHYSICS Magnetopause and boundary layers, 5443 PLANETARY SCIENCES: SOLID SURFACE PLANETS Magnetospheres}
}

@Article{Barakat1994,
  Title                    = {The effect of wave√î√∏Œ©particle interactions on the polar wind: {Preliminary} results},
  Author                   = {Barakat, AR and Barghouthi, IA},
  Journal                  = {Planetary and Space Science},
  Year                     = {1994},
  Number                   = {11},
  Pages                    = {987--992},
  Volume                   = {42}
}

@Article{Barakat1994a,
  Title                    = {The effect of wave-particle interactions on the polar wind {O}+},
  Author                   = {Barakat, AR and Barghouthi, IA},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1994},
  Number                   = {21},
  Pages                    = {2279--2282},
  Volume                   = {21}
}

@Article{Barakat1995,
  Title                    = {Double-hump {H}+ velocity distribution in the polar wind},
  Author                   = {Barakat, AR and Barghouthi, IA and Schunk, RW},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1995},
  Number                   = {14},
  Pages                    = {1857--1860},
  Volume                   = {22}
}

@Article{Barakat1990,
  Title                    = {Monte {Carlo} study of the escape of a minor species},
  Author                   = {Barakat, AR and Lemaire, J},
  Journal                  = {Physical Review A},
  Year                     = {1990},
  Number                   = {6},
  Pages                    = {3291},
  Volume                   = {42}
}

@Article{Barakat2001,
  Title                    = {Effects of wave–particle interactions on the dynamic behavior of the generalized polar wind},
  Author                   = {Barakat, AR and Schunk, RW},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2001},
  Number                   = {1},
  Pages                    = {75--83},
  Volume                   = {63}
}

@Article{Barakat1982,
  Title                    = {Transport equations for multicomponent anisotropic space plasmas: {A} review},
  Author                   = {Barakat, AR and Schunk, RW},
  Journal                  = {Plasma Physics},
  Year                     = {1982},
  Number                   = {4},
  Pages                    = {389--389},
  Volume                   = {24},

  Annote                   = {Added to JabRef: 2015.04.18}
}

@Article{Barakat2003,
  Title                    = {Seasonal and solar activity dependence of the generalized polar wind with low-altitude auroral ion energization},
  Author                   = {Barakat, AR and Schunk, RW and Demars, HG},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2003},
  Number                   = {A11},
  Volume                   = {108}
}

@Article{Barakat1987,
  Title                    = {Ion escape fluxes from the terrestrial high-latitude ionosphere},
  Author                   = {Barakat, AR and Schunk, RW and Moore, TE and Waite, JH},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1987},
  Number                   = {A11},
  Pages                    = {12255--12266},
  Volume                   = {92},

  Annote                   = {Added to JabRef: 2015.04.18}
}

@Article{Barakat1983,
  Title                    = {Monte {Carlo} {Calculations} of the {O}+ velocity distributions in the auroral ionosphere},
  Author                   = {Barakat, AR and Schunk, RW and St-Maurice, JP},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1983},
  Pages                    = {3237--3241},
  Volume                   = {88}
}

@Article{Barghouthi2008,
  Title                    = {A {Monte} {Carlo} study for ion outflows at high altitude and high latitude: {Barghouthi} model},
  Author                   = {Barghouthi, IA},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2008},
  Number                   = {A8},
  Volume                   = {113}
}

@Article{Barghouthi2005,
  Title                    = {O+ ion temperature partition coefficients β and β : {The} {Effect} of {O}+–{O}+ {Coulomb} self-collisions},
  Author                   = {Barghouthi, IA},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2005},
  Number                   = {A6},
  Volume                   = {110}
}

@Article{Barghouthi1997,
  Title                    = {Effects of wave‚Äö√Ñ√∂‚àö√ë‚àö‚Ñ¢particle interactions on {H}+ and {O}+ outflow at high latitude: {A} comparative study},
  Author                   = {Barghouthi, IA},
  Journal                  = {{\textbackslash}ldots Geophys. Res. Sp. Phys. (1978 {\textbackslash}ldots},
  Year                     = {1997},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/96JA03293/full}
}

@Article{Barghouthi1997a,
  Title                    = {Effects of wave-particle interactions on {H}+ and {O}+ outflow at high latitude: {A} comparative study},
  Author                   = {Barghouthi, IA},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1997},
  Number                   = {A10},
  Pages                    = {22065--22075},
  Volume                   = {102}
}

@Article{Barghouthi2012,
  Title                    = {Comparison between the simulation results of {Barghouthi} model for ion outflows in the polar wind and auroral regions},
  Author                   = {Barghouthi, Imad A and Nilsson, Hans and Ghithan, Sharif},
  Journal                  = {Journal of the Association of Arab Universities for Basic and Applied Sciences},
  Year                     = {2012},
  Number                   = {1},
  Pages                    = {1--10},
  Volume                   = {12}
}

@Article{Barghouthi2003,
  Title                    = {Monte {Carlo} simulation of {Boltzmann} equation in space plasma at high latitudes},
  Author                   = {Barghouthi, Imad A and Qatanani, Naji A and Allan, Fathi M},
  Journal                  = {Monte Carlo Methods and Applications mcma},
  Year                     = {2003},
  Number                   = {3},
  Pages                    = {201--217},
  Volume                   = {9}
}

@Article{Barghouthi2006,
  Title                    = {Monte {Carlo} modeling of toroidal ion distributions and ion temperatures at high altitudes equatorward of the cusp: {Effect} of finite gyroradius},
  Author                   = {Barghouthi, IA and Atout, MA},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2006},
  Number                   = {A3},
  Volume                   = {111}
}

@Article{Barghouthi1995,
  Title                    = {Comparison between the wave-particle interaction in the polar wind and in the auroral region, {Phys}},
  Author                   = {Barghouthi, IA and Barakat, AR},
  Journal                  = {Space Plasmas},
  Year                     = {1995},
  Pages                    = {445--450},
  Volume                   = {13}
}

@Article{Barghouthi1998,
  Title                    = {The effects of altitude-dependent wave particle interactions on the polar wind plasma},
  Author                   = {Barghouthi, IA and Barakat, AR and Persoon, AM},
  Journal                  = {Astrophysics and space science},
  Year                     = {1998},
  Number                   = {2},
  Pages                    = {117--140},
  Volume                   = {259}
}

@InProceedings{Barghouthi1994,
  Title                    = {A {Monte} {Carlo} simulation of the effect of ion self-collisions on the ion velocity distribution function in the high-latitude {F}-region},
  Author                   = {Barghouthi, IA and Barakat, AR and Schunk, RW},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {1994},
  Pages                    = {1076--1084},
  Publisher                = {Springer},
  Volume                   = {12}
}

@Article{Barghouthi1993,
  Title                    = {Monte {Carlo} study of the transition region in the polar wind: {An} improved collision model},
  Author                   = {Barghouthi, IA and Barakat, AR and Schunk, RW},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1993},
  Number                   = {A10},
  Pages                    = {17583--17591},
  Volume                   = {98}
}

@Article{Barghouthi2008a,
  Title                    = {The effect of altitude-and velocity-dependent wave–particle interactions on the {H}{\textless} sup{\textgreater}+{\textless}/sup{\textgreater} and {O}{\textless} sup{\textgreater}+{\textless}/sup{\textgreater} outflows in the auroral region},
  Author                   = {Barghouthi, IA and Doudin, NM},
  Journal                  = {J. Atmos. {\textbackslash}ldots},
  Year                     = {2008},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S1364682608000096}
}

@Article{Barghouthi2007,
  Title                    = {High-altitude and high-latitude {O}+ and {H}+ outflows: the effect of finite electromagnetic turbulence wavelength},
  Author                   = {Barghouthi, IA and Doudin, NM},
  Journal                  = {Ann. {\textbackslash}ldots},
  Year                     = {2007},

  Url                      = {http://www.ann-geophys.net/25/2195/2007/angeo-25-2195-2007.pdf}
}

@Article{Barghouthi2008b,
  Title                    = {The effect of altitude-and velocity-dependent wave–particle interactions on the {H}+ and {O}+ outflows in the auroral region},
  Author                   = {Barghouthi, IA and Doudin, NM and Saleh, AA and Pierrard, V},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2008},
  Number                   = {8},
  Pages                    = {1159--1169},
  Volume                   = {70}
}

@InProceedings{Barghouthi2007a,
  Title                    = {High-altitude and high-latitude {O}+ and {H}+ outflows: the effect of finite electromagnetic turbulence wavelength},
  Author                   = {Barghouthi, IA and Doudin, NM and Saleh, AA and Pierrard, V},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2007},
  Pages                    = {2195--2202},
  Volume                   = {25}
}

@Article{Barghouthi2011,
  Title                    = {A comparison study between observations and simulation results of {Barghouthi} model for {O}+ and {H}+ outflows in the polar wind},
  Author                   = {Barghouthi, IA and Ghithan, SH and Nilsson, H},
  Journal                  = {Annales Geophysicae-Atmospheres Hydrospheresand Space Sciences},
  Year                     = {2011},
  Number                   = {11},
  Pages                    = {2061},
  Volume                   = {29}
}

@InProceedings{Barghouthi2014,
  Title                    = {O+ and {H}+ ion heat fluxes at high altitudes and high latitudes},
  Author                   = {Barghouthi, IA and Nilsson, H and Ghithan, SH},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2014},
  Pages                    = {1043--1057},
  Publisher                = {Copernicus GmbH},
  Volume                   = {32}
}

@Article{Barghouthi2012a,
  Title                    = {Comparison between the simulation results of {Barghouthi} model for ion outflows in the polar wind and auroral regions},
  Author                   = {Barghouthi, IA and Nilsson, H and Ghithan, S},
  Journal                  = {J. Assoc. Arab {\textbackslash}ldots},
  Year                     = {2012},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S1815385212000375}
}

@Article{Barghouthi2001,
  Title                    = {A {Monte} {Carlo} simulation of the {H}+ polar wind: {Effect} of velocity distributions with {Kappa} suprathermal tails},
  Author                   = {Barghouthi, IA and Pierrard, V and Barakat, AR and Lemaire, J},
  Journal                  = {Astrophysics and Space Science},
  Year                     = {2001},
  Number                   = {3},
  Pages                    = {427--436},
  Volume                   = {277}
}

@Article{Barkley2008,
  Title                    = {Net ecosystem fluxes of isoprene over tropical {South} {America} inferred from {Global} {Ozone} {Monitoring} {Experiment} ({GOME}) observations of {HCHO} columns},
  Author                   = {Barkley, Michael P. and Palmer, Paul I. and Kuhn, Uwe and Kesselmeier, Juergen and Chance, Kelly and Kurosu, Thomas P. and Martin, Randall V. and Helmig, Detlev and Guenther, Alex},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2008},
  Number                   = {D20},
  Volume                   = {113},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2008JD009863/full},
  Urldate                  = {2014-11-13}
}

@Article{Barnes1983,
  Title                    = {Implicit particle simulation of magnetized plasmas},
  Author                   = {Barnes, DC and Kamimura, T and Leboeuf, J-N and Tajima, T},
  Journal                  = {J. Comput. Phys.},
  Year                     = {1983},
  Number                   = {3},
  Pages                    = {480--502},
  Volume                   = {52}
}

@Article{Basu2008,
  Title                    = {Helioseismology and solar abundances},
  Author                   = {Basu, S. and Antia, H. M.},
  Journal                  = {{\textbackslash}physrep},
  Year                     = {2008},

  Month                    = mar,
  Pages                    = {217--283},
  Volume                   = {457},

  Doi                      = {10.1016/j.physrep.2007.12.002}
}

@Article{Basu2001,
  Title                    = {Response of the equatorial ionosphere in the {South} {Atlantic} {Region} to the {Great} {Magnetic} {Storm} of {July} 15, 2000},
  Author                   = {Basu, S. and Basu, S. and Groves, K. M. and Yeh, H.-C. and Su, S.-Y. and Rich, F. J. and Sultan, P. J. and Keskinen, M. J.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {2001},
  Pages                    = {3577--3580},
  Volume                   = {28},

  Doi                      = {10.1029/2001GL013259},
  Keywords                 = {Ionosphere: Equatorial ionosphere, Ionosphere: Ionospheric dynamics, Ionosphere: Ionospheric irregularities}
}

@Article{Bauer2000,
  Title                    = {Dual spacecraft determinations of magnetopause motion},
  Author                   = {Bauer, TM and Dunlop, MW and Ö Sonnerup, BU and Sckopke, N and Fazakerley, AN and Khrabrov, AV},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2000},
  Number                   = {13},
  Pages                    = {1835--1838},
  Volume                   = {27}
}

@Article{Baumann2013,
  Title                    = {Kinetic {Modeling} of {Particle} {Acceleration} in a {Solar} {Null}-point {Reconnection} {Region}},
  Author                   = {Baumann, G. and Haugbølle, Troels and Nordlund, {\textbackslash}textbackslashAA},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2013},
  Number                   = {2},
  Pages                    = {93},
  Volume                   = {771},

  Url                      = {http://iopscience.iop.org/0004-637X/771/2/93},
  Urldate                  = {2014-05-31}
}

@Article{Baumjohann1989,
  Title                    = {Average plasma properties in the central plasma sheet},
  Author                   = {Baumjohann, W and Paschmann, G and Cattell, CA},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1989},
  Number                   = {A6},
  Pages                    = {6597--6606},
  Volume                   = {94}
}

@InProceedings{Bednarz1995,
  Title                    = {{GOME} {Global} {Ozone} {Monitoring} {Experiment} users manual},
  Author                   = {Bednarz, Floyd},
  Booktitle                = {{ESA} {Special} {Publication}},
  Year                     = {1995},
  Volume                   = {1182},

  Url                      = {http://adsabs.harvard.edu/abs/1995ESASP1182.....B},
  Urldate                  = {2014-11-13}
}

@Article{Begue1999,
  Title                    = {Two-dimensional {Vlasov} simulation of {Raman} scattering and plasma beatwave acceleration on parallel computers},
  Author                   = {Begue, ML and Ghizzo, A and Bertrand, P},
  Journal                  = {J. Comput. Phys.},
  Year                     = {1999},
  Number                   = {2},
  Pages                    = {458--478},
  Volume                   = {151},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S0021999199961934}
}

@Article{Behannon1983,
  Title                    = {Structure and dynamics of {Saturn}'s outer magnetosphere and boundary regions},
  Author                   = {Behannon, KW and Lepping, RP and Ness, NF},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1983},
  Number                   = {A11},
  Pages                    = {8791--8800},
  Volume                   = {88}
}

@Article{Bemporad2003,
  Title                    = {Temporal {Evolution} of a {Streamer} {Complex}: {Coronal} and in {Situ} {Plasma} {Parameters}},
  Author                   = {Bemporad, A. and Poletto, G. and Suess, S. T. and Ko, Y. K. and Parenti, S. and Riley, P. and Romoli, M. and Zurbuchen, T. Z.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2003},

  Month                    = aug,
  Pages                    = {1146--1163},
  Volume                   = {593},

  Doi                      = {10.1086/376605},
  Keywords                 = {Sun: abundances, Sun: corona, Sun: solar wind, Sun: UV Radiation}
}

@Book{BenJaffel1996,
  Title                    = {The {Abundance} and {Distribution} of {Deuterium} on {Saturn}},
  Author                   = {Ben Jaffel, L.},
  Year                     = {1996},
  Month                    = jul,
  Note                     = {Published: HST Proposal},

  Abstract                 = {We propose to obtain high resolution profiles of the D Lymanalpha line emitted by the limb of the upper atmosphere Saturn,using the GHRS Echelle A and the LSA. Ourtechnique consists in a radial drift of the LSA slit acrossthe limb of the planet. This is much like the very efficientoccultation technique although we record reflected instead oftransmitted light. As the deuterium emission is opticallythin, the analysis of the resulting profiles will provide,through our photochemistry models and radiative transfercalculations, the possibility for the first time to retrievethe deuterium scale height and abundance at least in four locationsof the upper atmosphere of Saturn. Scale heights at differentlocations derived from the D Ly-alpha emission, and the analysis of theH Ly-alpha profile, obtained with each limb observation, will accuratelyprovide the H total column density. A precise estimate of theD/H ratio will therefore be inferred. Recently, wesuccessfully applied the technique to observe the limb ofJupiter with the medium resolution grating G160M. The inferredD/H ratio ∼ 6+/- 1 * 10{\textasciicircum}-5 seems to support the measurementsmade through HD/H2 rather than CH3D/CH4. The uncertainty onthis value could be reduced if high resolution observationswith Echelle A are conducted. This should confirm the newlyderived ratio and check the D/H ratio for Saturn.Ultimately, this will help to refine the scenario on theformation and the evolution our Solar System 4.5 billionsyears ago.}
}

@Book{BenJaffel1992,
  Title                    = {Abundance and {Distribution} of {Atomic} {Deuterium} in the {Jovian} {Upper} {Atmosphere} {Through} {D}-{Lyman} {Alpha} {Profile} {Analysis} at {Planetary} {Limb} - {Cyc} 3 {Med}},
  Author                   = {Ben Jaffel, L.},
  Year                     = {1992},
  Month                    = jun,
  Note                     = {Published: HST Proposal},

  Abstract                 = {The purpose of this proposal is to obtain middle and high resolution profiles of the D Lyman alpha line emitted by the Jovian upper atmosphere near the planet approaching limb, with the G160M grating and the LSA.The analysis of the profiles resulting from the limb scan, will provide, through our radiative transfer calculations and photochemistry models, the possibility for the first time to retrieve the abundance and the scale height of the deuterium at least in two locations of the upper atmosphere of Jupiter. On the other hand, continuous observations of Jupiter's H Lyman alpha emission since 1969, are slowly providing more precise evaluation of the [H] total content above the methane level. Recent IUE data, and short-term observation with the GHRS, are now providing this parameter with higher precision. A precise estimate of the D/H ratio will therefore be inferred. Contrary to Infra-red measurements where the chemical isotopic fractionation introduces a large uncertainty, the present method will provide a direct measure of the D/H ratio.}
}

@InProceedings{BenJaffel1998,
  Title                    = {The {Lyman} α {Bulge} of {Jupiter} {\textbackslash}amp the {Auroral}-{Equatorial} {Regions} {Coupling}},
  Author                   = {Ben Jaffel, L. and Ballester, G. and Clarke, J. T. and Emerich, C. and Gladstone, R. and Rego, D.},
  Booktitle                = {Ultraviolet {Astrophysics} {Beyond} the {IUE} {Final} {Archive}},
  Year                     = {1998},
  Editor                   = {Wamsteker, W. and Gonzalez Riestra, R. and Harris, B.},
  Pages                    = {53},
  Series                   = {{ESA} {Special} {Publication}},
  Volume                   = {413}
}

@Article{BenJaffel2005,
  Title                    = {H {Lyman}-{Alpha} {Disc} {Emission} from the {Upper} atmosphere of {Jupiter}: {New} {Radiation} {Transfer} {Diagnosis}},
  Author                   = {Ben Jaffel, L. and Clarke, J. T.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2005},

  Month                    = dec,
  Pages                    = {A94},

  Abstract                 = {The properties of the upper atmosphere of Jupiter have been of much interest with the still unresolved issue of the H Ly-alpha bulge, suprathermal hydrogen, and coronal Ly-alpha emissions as revealed by recent high-resolution observations made by the Hubble Space Telescope Imaging Spectrometer (STIS). To help understand these questions better, we have performed a theoretical study of Jupiter's upper atmosphere using its reflected solar Ly-alpha. This uses the adding-doubling radiation transfer method in which we take into account the curvature effect of the planetary atmosphere. Our goal is to test the sensitivity of the Jovian Ly-alpha emission line in relation to H column density, eddy diffusion coefficient, frequency redistribution function for photon scattering, the temperature vertical profile, and a hot atomic H layer embedded into the top of the atmosphere. Beyond reasserting finding of earlier studies, particularly the Ly-a center-to-limb (CTL) brightening, self-reversed line profile at disk center, and wide line profile on the planetary limb, we focus in this study on developing new diagnosis tools, to attain more confidently the unknown structure of Jupiter's thermosphere. First, using the brightness distribution for specific wavelength bands as proposed by Ben Jaffel et al., A{\textbackslash}ampA, 204, 319, 1988, we show how to derive the thickness of the atomic H layer above the homopause level by a new technique that uses the spatial gap that separates the optical limb positions of respectively the line core and line wing. We also propose to derive the eddy diffusion coefficient at the homopause level, using the Q ratio between the limb peak brightness and the intensity from other regions over the planetary disc. This new technique only requires low-resolution observations and does not depend on the absolute calibration of the corresponding instrument. Finally, the relationship between the intensity of a specific wavelength range of the emission line and the temperature gradient in the thermosphere is demonstrated, allowing a new tool to access that fundamental property. Quick comparisons with some existing data show the strength of the proposed approach and opens new horizons to use strong resonant emission line at high resolution as a diagnostic for the state and structure of planetary upper atmospheres.},
  Keywords                 = {0300 ATMOSPHERIC COMPOSITION AND STRUCTURE, 0350 Pressure, 0360 Radiation: transmission and scattering, 6200 PLANETARY SCIENCES: SOLAR SYSTEM OBJECTS, 7549 Ultraviolet emissions, and temperature, density}
}

@Article{BenJaffel1993,
  Title                    = {The {Lyman} alpha bulge of {Jupiter} - {Effects} of non-thermal velocity field},
  Author                   = {Ben Jaffel, L. and Clarke, J. T. and Prange, R. and Gladstone, G. R. and Vidal-Madjar, A.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {1993},

  Month                    = apr,
  Pages                    = {747--750},
  Volume                   = {20},

  Abstract                 = {We outline for the first time the effect of such nonthermal line broadening processes as turbulence, random waves, convection, etc., on the shape and intensity of the H Ly-alpha line resonance scattered from the atmosphere of Jupiter. We show how a nonthermal velocity field confined to the bulge region, in the upper atmosphere of Jupiter, may account for most of the H Ly-alpha bulge features. Both the shape and the brightness of the Ly-alpha line from the bulge region as reported by the IUE instrument and the Voyager UV Spectrometer can be recovered assuming resonant scattering with a total atomic hydrogen of about 4 x 10 exp 17/sq cm, and a nonthermal component H of about 2 x 10 exp 15/sq cm above the thermopause.},
  Doi                      = {10.1029/92GL02488},
  Keywords                 = {Atmospheric Scattering, Atmospheric Turbulence, Jupiter (Planet), Lyman Alpha Radiation, Radiative Transfer, Resonance Scattering, Spectral Line Width, Turbulence Models, Ultraviolet Astronomy, Ultraviolet Spectrometers, Velocity Distribution}
}

@Article{BenJaffel1993a,
  Title                    = {The {Lyman} alpha bulge of {Jupiter}: {Effects} of non-thermal velocity field},
  Author                   = {Ben Jaffel, Lotfi and Clarke, John T and Prangé, Renée and Gladstone, G Randall and Vidal-Madjar, Alfred},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1993},
  Number                   = {8},
  Pages                    = {747--750},
  Volume                   = {20}
}

@Article{BenJaffel2007,
  Title                    = {The {H} {Lyman}- α emission line from the upper atmosphere of {Jupiter}: {Parametric} radiative transfer study and comparison with data},
  Author                   = {Ben Jaffel, L. and Kim, Y. J. and Clarke, J.},
  Journal                  = {ıcarus},
  Year                     = {2007},

  Month                    = oct,
  Pages                    = {504--527},
  Volume                   = {190},

  Abstract                 = {This study uses the adding-doubling radiative transfer method in which we take into account the curvature effect of the planetary atmosphere in order to test the sensitivity of the jovian Ly- α emission line in relation to H column density, eddy diffusion coefficient, frequency redistribution function for photon scattering, temperature vertical profile, and an added hot atomic H layer on the top of the atmosphere. We also focus here on developing new diagnostic tools that will help us to obtain more confidently the underlying thermospheric structure of Jupiter. First, using the brightness distribution for specific wavelength bands as proposed by Ben Jaffel et al. [Ben Jaffel, L., Magnan, C., Vidal-Madjar, A., 1988. Astron. Astrophys. 204, 319-326], we show that the spatial thickness of the atomic H layer above the homopause level can be measured directly as the separation between the vertical positions of respectively the line core and line wing optical limbs. This thickness also constrains the [H] column and the value K of the eddy diffusion coefficient at the homopause level at the disc location under consideration. We also propose to refine the value of K and [H], respectively, at a specific planetary latitude, using the Q ratio of the limb peak brightness to the intensity from other regions over the planetary disc. Finally, the relationship between the disc brightness distribution from specific wavelength bands of the emission line and the temperature gradient in the thermosphere is demonstrated, thus providing an accurate tool to access this key information from high resolution observations. Quick, preliminary comparisons with some existing HTS/STIS data show the H layer thickness at auroral latitudes ( {\textbackslash}tilde1700 km) is much smaller than at equatorial latitudes ( {\textbackslash}tilde3900 km). These results strongly support the existence of a gradient in both H density and K versus latitude, with higher values of K at high latitudes and higher values of the H density at the equatorial regions. Such a small H layer thickness at auroral latitudes is consistent with a high mixing in the atmosphere that brings the hydrocarbons upwards, reducing consequently the column of hydrogen that scatters photons. These preliminary results show the strength of the proposed approach and open new horizons to use strong resonant emission lines at high resolution as a diagnostic for the state and structure of planetary upper atmospheres.},
  Doi                      = {10.1016/j.icarus.2007.03.013}
}

@Article{BenJaffel1995,
  Title                    = {Dark {Auroral} {Oval} on {Saturn} {Discovered} in {Hubble} {Space} {Telescope} {Ultraviolet} {Images}},
  Author                   = {Ben Jaffel, L. and Leers, V. and Sandel, B. R.},
  Journal                  = {Science},
  Year                     = {1995},

  Month                    = aug,
  Pages                    = {951--953},
  Volume                   = {269},

  Abstract                 = {Hubble Space Telescope ultraviolet images of Saturn obtained with the Faint Object Camera near 220 nanometers reveal a dark oval encircling the north magnetic pole of the planet. The opacity has an equivalent width of ∼11{\textasciicircum}circ in latitude and is centered around ∼79{\textasciicircum}circN. The oval shape of the dark structure and its coincidence with the aurora detected by the Voyager Ultraviolet Spectrometer suggest that the aerosol formation is related to the auroral activity.},
  Doi                      = {10.1126/science.269.5226.951}
}

@Article{BenJaffel1988,
  Title                    = {The {Lyman} alpha albedo of {Jupiter}},
  Author                   = {Ben Jaffel, L and Magnan, C and Vidal-Madjar, A},
  Journal                  = {Astronomy and Astrophysics},
  Year                     = {1988},
  Pages                    = {319--326},
  Volume                   = {204}
}

@Article{BenJaffel1991,
  Title                    = {A model for the disc {Lyman} alpha emission of {Uranus}},
  Author                   = {Ben Jaffel, L. and Prange, R. and Emerich, C. and Vidal-Madjar, A. and McConnell, J. C.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1991},

  Month                    = jun,
  Pages                    = {9781--9791},
  Volume                   = {96},

  Abstract                 = {A new efficient radiative transfer algorithm for nonhomogeneous model atmospheres has been applied to the Uranian atmosphere. The contribution of the scatter solar Lyman-alpha to the Uranain emission is of the order of 300 R, and the Rayleigh contribution may reach 450 R for small values of the eddy diffusion coefficient (EDC). The total solar contribution may then reach about 750 R for a solar flux of 2.5 x 10 to the 11th photons/sq cm/s/A. A level of up to 400 R is confirmed in some directions for the interstellar wind contribution. The values of the atmospheric EDC necessary to mimic the observations are 50-100 sq cm/s. A small additional source located on the dayside Uranian atmosphere seems necessary correctly to fit the shape of the limb to limb intensity variation, especially near the limbs. Its contribution to the emergent intensity would range from 100 to 500 R.},
  Doi                      = {10.1029/91JA00349},
  Keywords                 = {Flyby Missions, Lyman Alpha Radiation, Planetary Limb, Planetary Radiation, Radiative Transfer, Resonance Scattering, Ultraviolet Spectrometers, Uranus (Planet), Voyager 2 Spacecraft}
}

@Article{BenJaffel1995a,
  Title                    = {New analysis of the {Voyager} {UVS} {H} {Lyman}-alpha emission of {Saturn}},
  Author                   = {Ben Jaffel, L. and Prange, R. and Sandel, B. R. and Yelle, R. V. and Emerich, C. and Feng, D. and Hall, D. T.},
  Journal                  = {ıcarus},
  Year                     = {1995},

  Month                    = jan,
  Pages                    = {91--102},
  Volume                   = {113},

  Abstract                 = {The limb to limb Lyman-alpha reflectivities observed with the Voyager ultraviolet spectrometer (UVS) instruments during the fly-by of Saturn are reanalyzed using a revised H Lyman-alpha sensitivity for the Voyager 1 instrument. The new sensitivity reconciles the measured intensities to those of Voyager 2 and gives a coherent set of data. To fit the UV airglow observations, four sources are considered: (1) H resonance and H2 Rayleigh scattering of solar Lyman-alpha radiation, (2) the interplanetary Lyman-alpha radiation, (3) a possible internal source of unknown origin, (4) the possibility of atmospheric turbulence recently proposed to explain the Lyman-alpha bulge of Jupiter. The analysis supports neither a dominant collisional excitation source for the UV emissions nor the presence of strong atmospheric turbulence. The best fit, in terms of brightness but also in terms of shape of the limb to limb profile (that is to say independent on the absolute calibrations), is obtained for pure resonance and Rayleigh scattering of solar and interstellar wind line in an atmosphere enriched in atomic hydrogen up to three times the standard model. Influx of water from the rings of Saturn may provide a means for producing such enhanced H densities in the upper atmosphere.},
  Doi                      = {10.1006/icar.1995.1007},
  Keywords                 = {Airglow, Emission Spectra, Hydrogen, Lyman Alpha Radiation, Radiative Transfer, Rayleigh Scattering, Saturn (Planet), Ultraviolet Spectrometers, Voyager Project}
}

@Article{BenJaffel2011,
  Title                    = {The {Local} {Interstellar} {Medium} {Magnetic} {Field}: {Back} to the {Old} {Times}!},
  Author                   = {Ben Jaffel, L. and Ratkiewicz, R.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2011},

  Month                    = dec,
  Pages                    = {B1965},

  Abstract                 = {The crossing of the solar wind termination shock (TS) by Voyager 1 (V1) {\textbackslash}amp Voyager 2 (V2) spacecrafts respectively at ∼94 AU and ∼84 AU revealed a rather strong asymmetry in the heliosphere that was immediately associated with the imprint of the unknown local interstellar medium magnetic field (LIMF). The observed asymmetry in the TS shape and further in situ measurements made by the Voyager plasma and magnetic field instruments deep in the heliosheath were interpreted as being a result of the unusually strong LIMF level that stands in stark contrast with commonly accepted values 1.8-2.5 μG derived from ground-based observations. In addition, the derived orientation was different from average orientation observed on the ∼100 parsecs scale, requiring a distortion of the far field lines in order to adjust to the solar vicinity region. The Lyman-α emission originating from the neutral hydrogen component was reported to show a distortion in the heliosphere, however, and this distortion should also be used to constrain the LIMF strength and its two orientation angles. In addition, Interstellar Boundary Explorer (IBEX) reported a ribbon-like structure in the spatial distribution of energetic neutrals of heliospheric origin, a structure that may be explained by the presence of an oblique LIMF. Here we show that the asymmetries observed in respectively the Lyman-α emission deep in the heliosphere-in the TS position as measured by V1 and V2-and the Ibex ribbon could be explained with a rather weak 1.8-2.5 μG strength of LIMF and orientation well below the galactic plane. We also show that the magnetohydrodynamic (MHD) modelling of V1 and V2 plasma observations does not lead to unique values of the LIMF strength and orientation as previously claimed. The LIMF derived here is oriented almost orthogonal to the spiral arm that hosts our solar system, which is consistent with previous findings from pulsar rotation, diffuse radio emission, and polarization of starlight observations.},
  Keywords                 = {2126 INTERPLANETARY PHYSICS / Heliosphere/interstellar medium interactions, 2144 INTERPLANETARY PHYSICS / Interstellar gas, 7524 SOLAR PHYSICS, AND ASTRONOMY / Magnetic fields, ASTROPHYSICS}
}

@InProceedings{BenJaffel1992a,
  Title                    = {A {New} {Model} for the {Lyman} α {Bulge} of {Jupiter}},
  Author                   = {Ben Jaffel, L. and Sommeria, J. and Prangé, R.},
  Booktitle                = {{AAS}/{Division} for {Planetary} {Sciences} {Meeting} {Abstracts} \#24},
  Year                     = {1992},
  Month                    = jun,
  Pages                    = {1033},
  Series                   = {Bulletin of the {American} {Astronomical} {Society}},
  Volume                   = {24}
}

@Article{BenJaffel1990,
  Title                    = {A new method for the resolution of the radiative transfer equation in three-dimensional geometry. {I} - {Theory}},
  Author                   = {Ben Jaffel, L. and Vidal-Madjar, A.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {1990},

  Month                    = feb,
  Pages                    = {801--818},
  Volume                   = {350},

  Abstract                 = {A method for solving the three-dimensional equation of transfer for an inhomogeneous static medium is described. The resolution of the three-dimensional transfer equation is important for studying the planetary atmosphere where an accurate model of the radiation field near the terminator region and in the nightside is necessary. The procedure involves: the reduction of the three-dimensional equation to a one-dimensional equation system; the resolution of this system by the discrete ordinate method, and reconstruction of the three-dimensional radiation field. This method considers variations in atmospheric parameters and reflectance at the bottom of the atmosphere relative to spatial and frequency parameters.},
  Doi                      = {10.1086/168432},
  Keywords                 = {Computational Astrophysics, Fourier Series, Planetary Atmospheres, Radiation Distribution, Radiative Transfer, Three Dimensional Models, Transport Properties}
}

@Article{BenJaffel1989,
  Title                    = {New developments in the discrete ordinate method for the resolution of the radiative transfer equation},
  Author                   = {Ben Jaffel, L. and Vidal-Madjar, A.},
  Journal                  = {{\textbackslash}aap},
  Year                     = {1989},

  Month                    = aug,
  Pages                    = {306--312},
  Volume                   = {220},

  Abstract                 = {The application of the discrete ordinate method of solving the radiative transfer equation as developed by Wehrse (1985) and Schmidt and Wehrse (1987) to a resonance line in a planetary atmosphere is discussed. It is shown that the construction of a quasi-analytical solution to the corresponding matrix diagonalization problem reduces the time calculation and permits the use of more dense discrete frequency and angle grids. A comparison with previous work shows that the present method reduces the computation time by more than a factor of 10 and is more appropriate in all cases.},
  Keywords                 = {Albedo, Eigenvalues, Jupiter Atmosphere, Line Spectra, Lyman Alpha Radiation, Planetary Atmospheres, Radiative Transfer, Resonance Lines}
}

@InProceedings{BenJaffel1994,
  Title                    = {{HST}-{GHRS} {Detection} of the {Deuterium} {Lyman} {Alpha} {Emission} at the {Limb} of {Jupiter}},
  Author                   = {Ben Jaffel, L. and Vidal-Madjar, A. and Clarke, J. T. and Emerich, C. and Prangé, R. and Gladstone, R. and McConnell, J. and Noll, K.},
  Booktitle                = {{AAS}/{Division} for {Planetary} {Sciences} {Meeting} {Abstracts} \#26},
  Year                     = {1994},
  Month                    = jun,
  Pages                    = {1100},
  Series                   = {Bulletin of the {American} {Astronomical} {Society}},
  Volume                   = {26}
}

@InProceedings{BenJaffel1998a,
  Title                    = {{GHRS} {Detection} of the {Fossil} {Deuterium} of {Jupiter}},
  Author                   = {Ben Jaffel, L. and Vidal-Madjar, A. and Gladstone, G. R. and McConnell, J. C. and Emerich, C. and Prange, R. and Clarke, J. T.},
  Booktitle                = {The {Scientific} {Impact} of the {Goddard} {High} {Resolution} {Spectrograph}},
  Year                     = {1998},
  Editor                   = {Brandt, J. C. and Ake, T. B. and Petersen, C. C.},
  Pages                    = {366},
  Series                   = {Astronomical {Society} of the {Pacific} {Conference} {Series}},
  Volume                   = {143}
}

@Article{Ben-Jaffel2008,
  Title                    = {Spectral, spatial, and time properties of the hydrogen nebula around exoplanet {HD} 209458b},
  Author                   = {Ben-Jaffel, Lotfi},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2008},
  Number                   = {2},
  Pages                    = {1352},
  Volume                   = {688}
}

@Article{Ben-Jaffel2008a,
  Title                    = {Spectral, {Spatial}, and {Time} {Properties} of the {Hydrogen} {Nebula} around {Exoplanet} {HD} 209458b},
  Author                   = {Ben-Jaffel, L.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2008},

  Month                    = dec,
  Pages                    = {1352--1360},
  Volume                   = {688},

  Abstract                 = {All far-ultraviolet (FUV) observations of HD 209458 tend to support a scenario in which the inflated hydrogen atmosphere of its planetary companion strongly absorbs the stellar Lyα flux during transit. However, it is not clear how the transit absorption depends on the selected wavelength range in the stellar line profile, nor how the atomic hydrogen cloud is distributed spatially around HD 209458b. Here we report a sensitivity study of observed time and spectral variations of the stellar flux. In particular, the sensitivity of the absorption depth during transit to the assumed spectral range in the stellar line profile is shown to be very weak, leading to a transit depth in the range (8.4\%-8.9\%)+/-2.0\% for all possible wavelength ranges, and thereby confirming our initially reported absorption rate. Taking the ratio of the line profile during transit to the unperturbed line profile, we also show that the spectral signature of the absorption by the exoplanetary hydrogen nebula is symmetric and typical of a Lorentzian, optically thick medium. Our results question the adequacy of models that require a huge absorption and/or a strong asymmetry between the blue and red sides of the absorption line during transit, as no such features could be detected in the HST FUV absorption profile. Finally, we show that standard atmospheric models of HD 209458b provide a good fit to the observed absorption profile during transit. Other hybrid models assuming a standard model with a thin layer of superthermal hydrogen on top remain possible.},
  Doi                      = {10.1086/592101},
  Keywords                 = {Line: Profiles, Stars: Individual: Henry Draper Number: HD 209458, Stars: Planetary Systems, Techniques: Spectroscopic, Ultraviolet: Stars}
}

@Article{Ben-Jaffel2007,
  Title                    = {Exoplanet {HD} 209458b: {Inflated} {Hydrogen} {Atmosphere} but {No} {Sign} of {Evaporation}},
  Author                   = {Ben-Jaffel, L.},
  Journal                  = {{\textbackslash}apjl},
  Year                     = {2007},

  Month                    = dec,
  Pages                    = {L61--L64},
  Volume                   = {671},

  Abstract                 = {Many extrasolar planets orbit closely to their parent star. Their existence raises the fundamental problem of loss and gain in their mass. For exoplanet HD 209458b, reports on an unusually extended hydrogen corona and a hot layer in the lower atmosphere seem to support the scenario of atmospheric inflation by the strong stellar irradiation. However, difficulties in reconciling evaporation models with observations call for a reassessment of the problem. Here we use HST archive data to report a new absorption rate of ∼8.9\% +/- 2.1\% by atomic hydrogen during the HD 209458b transit and show that no sign of evaporation could be detected for the exoplanet. We also report evidence of time variability in the HD 209458 Lyα flux, a variability that was not accounted for in previous studies, which corrupted their diagnostics. Mass-loss rates thus far proposed in the literature in the range 5{\textbackslash}times(10$^{\textrm{10\$}}$-10$^{\textrm{11\$}}$) g s$^{\textrm{-1\$}}$ must induce a spectral signature in the Lyα line profile of HD 209458 that cannot be found in the present analysis. Either an unknown compensation effect is hiding the expected spectral feature or else the mass-loss rate of neutrals from HD 209458 is modest.},
  Doi                      = {10.1086/524706},
  Keywords                 = {Line: Profiles, Stars: Individual: Henry Draper Number: HD 209458, Stars: Planetary Systems, Techniques: Spectroscopic, Ultraviolet: Stars}
}

@Article{Ben-Jaffel2007a,
  Title                    = {Exoplanet {HD} 209458b: {Inflated} hydrogen atmosphere but no sign of evaporation},
  Author                   = {Ben-Jaffel, Lotfi},
  Journal                  = {The Astrophysical Journal Letters},
  Year                     = {2007},
  Number                   = {1},
  Pages                    = {L61},
  Volume                   = {671}
}

@Article{Ben-Jaffel2015,
  Title                    = {Helium abundance in giant planets and the local interstellar medium},
  Author                   = {Ben-Jaffel, L. and Abbes, I.},
  Journal                  = {Journal of Physics Conference Series},
  Year                     = {2015},

  Month                    = jan,
  Number                   = {1},
  Pages                    = {012003},
  Volume                   = {577},

  Abstract                 = {The sun and giant planets are generally thought to have the same helium abundance as that in the solar nebula from which they were formed 4.6 billion years ago. In contrast, the interstellar medium reflects current galactic conditions. The departure of current abundances from the primordial and protosolar values may help trace the processes that drive the nucleosynthesis evolution of the galaxy and planetary interior formation and evolution. The Galileo probe measured the He abundance in situ the atmosphere of Jupiter, showing that He is only slightly depleted compared to the solar value. For Saturn, contradictory estimates from past Voyager observations make its He abundance very uncertain. Here, we use He 58.4 nm dayglow measured from the outer planets by the Voyager ultraviolet spectrometers to derive the He abundance in the atmosphere of Jupiter and Saturn. With the He abundance reported here, credible models become possible for the interior of Jupiter, Saturn, and extrasolar planets. We also use the solar He 58.4 nm line measured by the Solar Heliospheric Observatory to derive the He abundance inside the focusing cone. Finally, we compare He abundances derived here with primordial and protosolar values, stressing the unique opportunity offered by inner heliosphere observations and future Voyager in situ local interstellar medium measurements to derive the He abundance in the very interstellar cloud in which we reside.},
  Doi                      = {10.1088/1742-6596/577/1/012003}
}

@Article{Ben-Jaffel2013,
  Title                    = {Hubble {Space} {Telescope} detection of oxygen in the atmosphere of exoplanet {HD} 189733b},
  Author                   = {Ben-Jaffel, Lotfi and Ballester, GE},
  Journal                  = {Astronomy \& Astrophysics},
  Year                     = {2013},
  Pages                    = {A52},
  Volume                   = {553}
}

@Article{Ben-Jaffel2013a,
  Title                    = {Hubble Space Telescope detection of oxygen in the atmosphere of exoplanet HD 189733b},
  Author                   = {Ben-Jaffel, Lotfi and Ballester, GE},
  Journal                  = {Astronomy \& Astrophysics},
  Year                     = {2013},
  Pages                    = {A52},
  Volume                   = {553},

  Owner                    = {suleimanbaraka},
  Publisher                = {EDP Sciences},
  Timestamp                = {2016.02.20}
}

@InProceedings{Ben-Jaffel2010,
  Title                    = {High {Resolution} {Lyman}-α {Mapping} of the {Jovian} {Upper} {Atmopshere} and {Corona}},
  Author                   = {Ben-Jaffel, L. and Ballester, G. and Clarke, J. T. and Vincent, F.},
  Booktitle                = {{AAS}/{Division} for {Planetary} {Sciences} {Meeting} {Abstracts} \#42},
  Year                     = {2010},
  Month                    = oct,
  Pages                    = {1019},
  Series                   = {Bulletin of the {American} {Astronomical} {Society}},
  Volume                   = {42},

  Abstract                 = {Owing to the particular capabilities of the HST/STIS spectro-imaging instrument, Jovian H-Lyman-α line profiles were obtained with unprecedented accuracy on different locations of the planetary disc, using the 52”x0.5{\textbackslash}rdquo long slit in the echelle mode. This mode is allowed by STSCI but not supported for calibration because of potential contamination from adjacent orders. In addition, the telescope pointing to any selected location on the planetary disc is not very accurate for a moving and extended target. The construction of a sophisticated pipeline of calibration was thus necessary to correct for all potential image distortion, signal contamination, and mapping of the slit image over the apparent disc of the planet. These efforts represent the necessary step for checking the serendipitous discovery of supersonic turbulence in the Jovian Lyman-α bulge and the consequent thermospheric circulation proposed in the literature, including strong winds (up to 20 km/s) predicted in the upper layers (altitudes above the 1 nanobar pressure level) of the atmosphere (Sommeria, Ben-Jaffel, and Prangé, Icarus, 118, pp 2-24, 1995). A two-dimensional Lyman-α map of the Jovian atmosphere and its corona, corrected for all potential contamination, will be presented with a preliminary analysis, confirming our previous finding of 60 km/s fast rotating hot hydrogen belt at equatorial latitudes.}
}

@Article{Ben-Jaffel2014,
  Title                    = {Transit of exomoon plasma tori: new diagnosis},
  Author                   = {Ben-Jaffel, Lotfi and Ballester, Gilda E},
  Journal                  = {The Astrophysical Journal Letters},
  Year                     = {2014},
  Number                   = {2},
  Pages                    = {L30},
  Volume                   = {785}
}

@Article{Ben-Jaffel2014a,
  Title                    = {Transit of {Exomoon} {Plasma} {Tori}: {New} {Diagnosis}},
  Author                   = {Ben-Jaffel, L. and Ballester, G. E.},
  Journal                  = {{\textbackslash}apjl},
  Year                     = {2014},

  Month                    = apr,
  Pages                    = {L30},
  Volume                   = {785},

  Abstract                 = {In the solar system, moons largely exceed planets in number. The Kepler database has been shown to be sensitive to exomoon detection down to the mass of Mars, but the first search has been unsuccessful. Here, we use a particles-in-cell code to predict the transit of the plasma torus produced by a satellite. Despite the small size of a moon, the spatial extent of its plasma torus can be large enough to produce substantial transit absorptions. The model is used for the interpretation of Hubble Space Telescope early ingress absorptions apparently observed during the WASP-12 b and HD 189733 b UV transits for which no consistent explanation exists. For HD 189733 b an exomoon transiting ∼16 R$_{\textrm{p}}$ ahead of the planet and loading ∼10$^{\textrm{29\$}}$ C II ions s$^{\textrm{-1\$}}$ into space is required to explain the tentative early ingress absorption observed for C II. For WASP-12b, a moon transiting ∼6 R$_{\textrm{p}}$ ahead from the planet and ejecting ∼10$^{\textrm{28\$}}$ Mg II ions per second is required to explain the NUV early ingress absorption feature. Interestingly, both HD 189733 b and WASP-12b predicted satellites are outside the Hill sphere of their planets, an indication that the moons, if present, were not formed in situ but probably captured later. Finally, our simulations show a strong electromagnetic coupling between the polar regions of planets and the orbital position of the moons, an expected outcome of the unipolar induction DC circuit model. Future observations should test our predictions with a potential opportunity to unambiguously detect the first exomoon plasma torus.},
  Doi                      = {10.1088/2041-8205/785/2/L30},
  Keywords                 = {opacity, planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: detection, plasmas, ultraviolet: planetary systems}
}

@Article{Ben-Jaffel2014b,
  Title                    = {Transit of exomoon plasma tori: new diagnosis},
  Author                   = {Ben-Jaffel, Lotfi and Ballester, Gilda E.},
  Journal                  = {The Astrophysical Journal Letters},
  Year                     = {2014},
  Number                   = {2},
  Pages                    = {L30},
  Volume                   = {785},

  File                     = {[PDF] from arxiv.org:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/76USBVVB/Ben-Jaffel and Ballester - 2014 - Transit of exomoon plasma tori new diagnosis.pdf:application/pdf;Snapshot:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/XUIC4M96/meta\;jsessionid=00A03307AF8FBDAE9FBB739DCFAEDF76.c5.iopscience.cld.iop.html:text/html},
  Shorttitle               = {Transit of exomoon plasma tori},
  Url                      = {http://iopscience.iop.org/2041-8205/785/2/L30},
  Urldate                  = {2015-12-09}
}

@Article{Ben-Jaffel2013b,
  Title                    = {Hubble {Space} {Telescope} detection of oxygen in the atmosphere of exoplanet {HD} 189733b},
  Author                   = {Ben-Jaffel, L. and Ballester, G. E.},
  Journal                  = {{\textbackslash}textbackslashaap},
  Year                     = {2013},

  Month                    = may,
  Pages                    = {A52},
  Volume                   = {553},

  Doi                      = {10.1051/0004-6361/201221014},
  Keywords                 = {planets and satellites: magnetic fields, planet-star interactions, stars: activity, stars: individual: HD 189733, Sun: activity, ultraviolet: general}
}

@InProceedings{Ben-Jaffel1997,
  Title                    = {Production and {Escape} {Rates} of {Titan}'s {Atomic} {Hydrogen}},
  Author                   = {Ben-Jaffel, L. and Deur, A.},
  Booktitle                = {Bulletin of the {American} {Astronomical} {Society}},
  Year                     = {1997},
  Editor                   = {Bietenholz, M. F. and Bartel, N. and Rupen, M. P. and Beasley, A. J. and Graham, D. A. and Altunin, V. I. and Venturi, T. and Umana, G. and Conway, J. E.},
  Month                    = jan,
  Pages                    = {744},
  Series                   = {Bulletin of the {American} {Astronomical} {Society}},
  Volume                   = {29}
}

@InProceedings{Ben-Jaffel2000,
  Title                    = {Hydrocarbon {Distribution} in {Saturn}'s {Upper} {Atmosphere}. {Re}-analysis of {Saturn}'s {Voyager} {UVS} {H}-{Lyman}-alpha and {He} 584 {A} {Airglow}},
  Author                   = {Ben-Jaffel, L. and Feng, D. and Herbert, F.},
  Booktitle                = {{AAS}/{Division} for {Planetary} {Sciences} {Meeting} {Abstracts} \#32},
  Year                     = {2000},
  Month                    = oct,
  Pages                    = {1013},
  Series                   = {Bulletin of the {American} {Astronomical} {Society}},
  Volume                   = {32},

  Abstract                 = {Simultaneous re-analysis of respectively the Voyager 2 UVS stellar Occultation observations obtained during the spacecraft encounter with Saturn and an IUE albedo spectrum of the planet obtained in 1983, provided the height distributions of eleven minor constituents from the top of the troposphere up to the atmospheric homopause region. These constituents are: CH$_{\textrm{4}}$, C$_{\textrm{2}}$H$_{\textrm{2}}$, C$_{\textrm{2}}$H$_{\textrm{4}}$, C$_{\textrm{4}}$H$_{\textrm{2}}$, C$_{\textrm{2}}$H$_{\textrm{6}}$, H$_{\textrm{2}}$O, GeH$_{\textrm{4}}$, PH$_{\textrm{3}}$, AsH$_{\textrm{3}}$, CO$_{\textrm{2}}$, and NH$_{\textrm{3}}$. A thin layer of H$_{\textrm{2}}$O is discovered near altitude 625 km. Our results seem to be consistent with HC abundances recently derived from ISO observations (Feng et al., 2000). We use the derived HC distribution to model the H Lyman-alpha and He 584 A airglow of Saturn observed by Voyager UVS in 1982, with a focus on the helium abundance in the upper atmosphere.}
}

@InProceedings{Ben-Jaffel1998,
  Title                    = {Hydrocarbons {Distribution} in {Saturn}'s {Upper} {Atmosphere}},
  Author                   = {Ben-Jaffel, L. and Feng, D. and Herbert, F. and Hermann, B.},
  Booktitle                = {{AAS}/{Division} for {Planetary} {Sciences} {Meeting} {Abstracts} \#30},
  Year                     = {1998},
  Month                    = sep,
  Pages                    = {1096},
  Series                   = {Bulletin of the {American} {Astronomical} {Society}},
  Volume                   = {30},

  Abstract                 = {We propose a new method that uses occultation observations and solar reflected spectra to derive self-consistently the abundance of several minor constituents in the upper atmosphere of planets. The data analysis process iterates between matrix inversion of occultation data and radiative transfer calculations of the reflected spectra. Simultaneous analysis of respectively the Voyager 2 UVS stellar Occultation observations obtained during the spacecraft encounter with Saturn and an IUE albedo spectrum of the planet obtained in 1983, provided the height distribution of eleven minor constituents from the top of the troposphere up to the atmospheric homopause region. These constituents are: CH\_4, C\_2H\_2, C\_2H\_4, C\_4H\_2, C\_2H\_6, H\_2O, GeH\_4, PH\_3, AsH\_3, CO\_2, and NH\_3. H\_2O appears as a key element of the upper atmosphere of Saturn that strongly influences its chemistry. Our results seem to be consistent with some HC abundances, recently derived from ISO observations.}
}

@Article{Ben-Jaffel2005,
  Title                    = {Predictions on the application of the {Hanle} effect to map the surface magnetic field of {Jupiter}},
  Author                   = {Ben-Jaffel, L. and Harris, W. and Bommier, V. and Roesler, F. and Ballester, G. E. and Jossang, J.},
  Journal                  = {ıcarus},
  Year                     = {2005},

  Month                    = nov,
  Pages                    = {297--311},
  Volume                   = {178},

  Abstract                 = {In this paper we evaluate the possibility of detecting, for the first time, the surface magnetic field of Jupiter ({\textbackslash}tilde1 bar level) by observing the change of linear polarization induced by the Hanle effect on the H Lyman-alpha (Ly α) emission line of the planet. We find that, indeed, the Hanle effect, which results from the interaction between a local magnetic field and the atomic polarization induced by absorption of anisotropic radiation, is sensitive to relatively weak values of the strength of the magnetic fields expected on planets. First, we show that for the Ly α emission backscattered by atomic H in the presence of a magnetic field, the Hanle effect is polarizing. This new result is in total contrast to the depolarizing effect predicted and observed for emission lines scattered at right angles in solar prominences. Additionally, to estimate the polarization rate for the case of Jupiter, we have considered three magnetic field models: a dipole field for reference, an O based model [Connerney, J.E.P., 1981. The magnetic field of Jupiter{\textbackslash}mdashA generalized inverse approach. J. Geophys. Res. 86, 7679-7693], and finally, an O based model [Khurana, K.K., 1997. Euler potential models of Jupiter's magnetospheric field. J. Geophys. Res. 102, 11295-11306]. In all models, we show that for the jovian backscattered Ly α line, the Hanle effect does enhance the Ly α linear polarization; the polarization rate may exceed 2\% at specific regions of the jovian disc, making detection possible either remotely or from an orbiter around Jupiter. In general, depending on the instrumental sensitivity and the observing strategy used, we show that accurate mapping of the linear polarization rate at the planetary surface (thermosphere) or off-disc (corona) may provide a rather accurate estimate of the jovian total magnetic field strength on large area scales.},
  Doi                      = {10.1016/j.icarus.2005.01.021}
}

@Article{Ben-Jaffel2010a,
  Title                    = {Helium {Abundance} in the {Atmosphere} of {Jupiter} and {Saturn}},
  Author                   = {Ben-Jaffel, L. and Herbert, F.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2010},

  Month                    = dec,
  Pages                    = {A1515},

  Abstract                 = {The Sun and giant planets are generally thought to have the same He abundance as that in the solar nebula from which they were formed. During the Voyagers' deep space cruises, helium abundance derived for the outer planets suggested that processes in the interior of Jupiter and Saturn may have substantially modified the original ratio as observed for the Sun. Galileo probe measured the helium abundance in situ the atmosphere of Jupiter, showing that He is only slightly depleted compared to the solar value, in contradiction with initial Voyager data analysis. For Saturn, contradictory estimates thus far reported from past Voyager observations make its He abundance very uncertain. Here, we use the He first resonance line (584{\textbackslash}AA ) dayglow measured from the outer planets by the Voyager ultraviolet spectrometers (UVS) to derive the helium abundance in the atmosphere of Jupiter and Saturn. The He 584{\textbackslash}AA dayglow corresponds to solar He emission line back-scattered by the upper atmosphere of planets. Our finding is that the [He/H2] mixing ratio is {\textbackslash}tilde 0.16{\textbackslash}plusmn0.03 and {\textbackslash}tilde 0.15{\textbackslash}plusmn0.025 respectively for Jupiter and Saturn. These abundances correspond to a helium mass fraction relative to the total helium and hydrogen Y {\textbackslash}tilde 0.24{\textbackslash}plusmn0.04 for Jupiter and Y {\textbackslash}tilde0.23{\textbackslash}plusmn 0.03 for Saturn.The He abundance derived here for Jupiter and Saturn are consistent with Galileo in situ measurement, suggesting little change in the primordial composition of the giants' interior since their formation from the solar nebula.},
  Keywords                 = {5704 PLANETARY SCIENCES: FLUID PLANETS / Atmospheres, 5724 PLANETARY SCIENCES: FLUID PLANETS / Interiors, 6220 PLANETARY SCIENCES: SOLAR SYSTEM OBJECTS / Jupiter, 6275 PLANETARY SCIENCES: SOLAR SYSTEM OBJECTS / Saturn}
}

@Article{Ben-Jaffel2010b,
  Title                    = {On the existence of energetic atoms in the upper atmosphere of exoplanet {HD}209458b},
  Author                   = {Ben-Jaffel, Lotfi and Hosseini, S Sona},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2010},
  Number                   = {2},
  Pages                    = {1284},
  Volume                   = {709}
}

@Article{Ben-Jaffel2000a,
  Title                    = {Far-{Ultraviolet} {Echoes} from the {Frontier} between the {Solar} {Wind} and the {Local} {Interstellar} {Cloud}},
  Author                   = {Ben-Jaffel, L. and Puyoo, O. and Ratkiewicz, R.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2000},

  Month                    = apr,
  Pages                    = {924--930},
  Volume                   = {533},

  Abstract                 = {We propose that first-order Fermi acceleration of Lyα photons should occur at the interface region between the solar and interstellar winds. In this process, photons are Doppler-shifted toward shorter wavelengths each time they are scattered by hydrogen neutrals that have been decelerated by charge exchange with protons in the transition region wrapping the heliopause. An additional component should therefore appear on the blue side of the line profile of the Lyα sky background emission. Its detection would not only reveal the existence of the heliopause interface but also trace its spatial distribution. We report here Hubble Space Telescope (HST) high-resolution Ly$^{\textrm{-1\$}}$ in the upwind direction. This velocity corresponds to an averaged deceleration along the line of sight of the interstellar hydrogen of 2.8+/-0.5 km s$^{\textrm{-1\$}}$ after crossing the transition region. We show that an extra component, which we interpret to be the spectral signature of the Fermi process in the upwind direction, is present in the blue wing of the Lyα sky line profile. In addition, we interpret here the enigmatic excess in the Lyα sky brightness that was recently detected by Voyager deep in the inner heliosphere as being due to the additional Fermi emission. According to this interpretation, the distribution of this excess emission should also represent the spatial variation of the neutral velocity drop-off across the interface region. In this scope, we show that the region of the heliosphere's nose is ∼12{\textbackslash}deg away from the upwind axis-a good indication that the interstellar magnetic field deviates ∼40{\textbackslash}deg from the interstellar flow direction.},
  Doi                      = {10.1086/308710},
  Keywords                 = {INTERPLANETARY MEDIUM, ISM: ABUNDANCES, ISM: MAGNETIC FIELDS, LINE: FORMATION, Radiative Transfer, ULTRAVIOLET: ISM}
}

@Article{Ben-Jaffel2000b,
  Title                    = {Far-ultraviolet echoes from the frontier between the solar wind and the local interstellar cloud},
  Author                   = {Ben-Jaffel, L and Puyoo, O and Ratkiewicz, R},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2000},
  Number                   = {2},
  Pages                    = {924},
  Volume                   = {533}
}

@Article{Ben-Jaffel2012,
  Title                    = {Uncovering the magnetic environment of our solar system},
  Author                   = {Ben-Jaffel, L. and Ratkiewicz, R.},
  Journal                  = {{\textbackslash}aap},
  Year                     = {2012},

  Month                    = oct,
  Pages                    = {A78},
  Volume                   = {546},

  Abstract                 = {Since its formation 4.6 billion years ago, our solar system has most likely crossed numerous magnetized interstellar clouds and bubbles of different sizes and contents on its path through the Milky Way. Having a reference model for how the heliosphere and interstellar winds interact is critical for understanding our current Galactic environment, and it requires untangling the roles of two major actors: the time-variable solar wind and the local interstellar magnetic field. Numerical simulations predict a distortion of the heliosphere caused by both solar wind anisotropy and interstellar magnetic field orientation. However, model comparison to deep space probes' measurements led to contradictory reports by Voyager 1 and Voyager 2 of both several crossings of the solar wind's termination shock and of the strength of the local interstellar field, with values ranging from 1.8 to 5.7 μG. Here, we show that Voyager 1 and 2 plasma, fields, and Lyman-α sky background measurements, as well as space observations of high-energy particles of heliospheric origin, may all be explained by a rather weak interstellar field 2.2 {\textbackslash}plusmn 0.1 μG pointing from Galactic coordinates (l,b) ∼ (28,52) {\textbackslash}plusmn 3{\textbackslash}deg. For the 2000 epoch Ulysses-based helium parameters assumed thus far, the interstellar bow shock must exist. By contrast, using the 2010 epoch IBEX-based He parameters and a stronger magnetic field leads to a plasma configuration that is not consistent with the Voyagers TS crossings. For the newly proposed interstellar He parameters, more simulations are required before one may determine whether the interstellar bow shock truly does disappear under those assumptions.},
  Doi                      = {10.1051/0004-6361/201219637},
  Keywords                 = {ISM: MAGNETIC FIELDS, magnetohydrodynamics (MHD), solar neighborhood, Solar Wind, Sun: heliosphere}
}

@Article{Ben-Jaffel2010c,
  Title                    = {On the {Existence} of {Energetic} {Atoms} in the {Upper} {Atmosphere} of {Exoplanet} {HD}209458b},
  Author                   = {Ben-Jaffel, L. and Sona Hosseini, S.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2010},

  Month                    = feb,
  Pages                    = {1284--1296},
  Volume                   = {709},

  Abstract                 = {Stellar irradiation and particle forcing strongly affect the immediate environment of extrasolar giant planets orbiting near their parent stars. However, it is not clear how the energy is deposited over the planetary atmosphere, nor how the momentum and energy spaces of the different species that populate the system are modified. Here, we use far-ultraviolet emission spectra from HD209458 in the wavelength range (1180-1710) {\textbackslash}AA to bring new insight to the composition and energetic processes in play in the gas nebula around the transiting planetary companion. In that frame, we consider up-to-date atmospheric models of the giant exoplanet where we implement non-thermal line broadening to simulate the impact on the transit absorption of superthermal atoms (H I, O I, and C II) populating the upper layers of the nebula. Our sensitivity study shows that for all existing models, a significant line broadening is required for O I and probably for C II lines in order to fit the observed transit absorptions. In that frame, we show that O I and C II are preferentially heated compared to the background gas with effective temperatures as large as T $_{\textrm{O I }}$/T$_{\textrm{B}}$ ∼ 10 for O I and T $_{\textrm{C II }}$/T$_{\textrm{B}}$ ∼ 5 for C II. By contrast, the situation is much less clear for H I because several models could fit the Lyα observations including either thermal H I in an atmosphere that has a dayside vertical column [H I] ∼ 1.05 {\textbackslash}times 10$^{\textrm{21\$}}$ cm$^{\textrm{-2\$}}$, or a less extended thermal atmosphere but with hot H I atoms populating the upper layers of the nebula. If the energetic H I atoms are either of stellar origin or populations lost from the planet and energized in the outer layers of the nebula, our finding is that most models should converge toward one hot population that has an H I vertical column in the range [H I]$_{\textrm{hot}}$ ∼ (2-4) {\textbackslash}times 10$^{\textrm{13\$}}$ cm$^{\textrm{-2\$}}$ and an effective temperature in the range T $_{\textrm{H I }}$ ∼ (1-1.3) {\textbackslash}times 10$^{\textrm{6\$}}$ K, but with a bulk velocity that should be rather slow.},
  Doi                      = {10.1088/0004-637X/709/2/1284},
  Keywords                 = {LINE: FORMATION, Line: Profiles, planetary systems, radiation mechanisms: non-thermal, stars: individual: HD209458, Ultraviolet: Stars}
}

@Article{Ben-Jaffel2013c,
  Title                    = {The existence and nature of the interstellar bow shock},
  Author                   = {Ben-Jaffel, Lotfi and Strumik, M and Ratkiewicz, R and Grygorczuk, J},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2013},
  Number                   = {2},
  Pages                    = {130},
  Volume                   = {779}
}

@Article{Ben-Jaffel2013d,
  Title                    = {The {Existence} and {Nature} of the {Interstellar} {Bow} {Shock}},
  Author                   = {Ben-Jaffel, L. and Strumik, M. and Ratkiewicz, R. and Grygorczuk, J.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2013},

  Month                    = dec,
  Pages                    = {130},
  Volume                   = {779},

  Abstract                 = {We report a new diagnosis of two different states of the local interstellar medium (LISM) near our solar system by using a sensitivity study constrained by several distinct and complementary observations of the LISM, solar wind, and inner heliosphere. Assuming the Interstellar Boundary Explorer (IBEX) He flow parameters for the LISM, we obtain a strength of ∼2.7 {\textbackslash}plusmn 0.2 μG and a direction pointing away from galactic coordinates (28, 52) {\textbackslash}plusmn 3{\textbackslash}deg for the interstellar magnetic field as a result of fitting Voyager 1 and Voyager 2 in situ plasma measurements and IBEX energetic neutral atoms ribbon. When using Ulysses parameters for the LISM He flow, we recently reported the same direction but with a strength of 2.2 {\textbackslash}plusmn 0.1 μG. First, we notice that with Ulysses He flow, our solution is in the expected hydrogen deflection plane (HDP). In contrast, for the IBEX He flow, the solution is ∼20{\textbackslash}deg away from the corresponding HDP plane. Second, the long-term monitoring of the interplanetary H I flow speed shows a value of ∼26 km s$^{\textrm{-1\$}}$ measured upwind from the Doppler shift in the strong Lyα sky background emission line. All elements of the diagnosis seem therefore to support Ulysses He flow parameters for the interstellar state. In that frame, we argue that reliable discrimination between superfast, subfast, or superslow states of the interstellar flow should be based on most existing in situ and remote observations used together with global modeling of the heliosphere. For commonly accepted LISM ionization rates, we show that a fast interstellar bow shock should be standing off upstream of the heliopause.},
  Doi                      = {10.1088/0004-637X/779/2/130},
  Keywords                 = {INTERPLANETARY MEDIUM, ISM: MAGNETIC FIELDS, local interstellar matter, shock waves, Solar Wind, Sun: heliosphere}
}

@Article{Ben-Jaffel2014c,
  Title                    = {Helium and {Hydrogen} {Abundances} in the {Heliosphere} and the {Local} {Interstellar} {Medium}},
  Author                   = {Ben-Jaffel, L. B. and Vincent, F. E.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2014},

  Month                    = dec,
  Pages                    = {B4051},

  Abstract                 = {The sun is generally thought to have the same helium abundance as that in the solar nebula from which it was formed 4.6 billion years ago. In contrast, the interstellar medium reflects current galactic conditions. The departure of current abundances from the primordial and protosolar values may help trace the processes that drive the nucleosynthesis evolution of the galaxy. Here, we use the solar He 58.4 nm line measured by the Solar Heliospheric Observatory (SOHO) to derive the He abundance inside the focusing cone. We also use Hubble Space Telescope, SOHO, and Voyager observations to constrain the properties of the interplanetary hydrogen flow, particularly at the heliospheric interface. Finally, we compare H and He abundances derived here with primordial and protosolar values, stressing the unique opportunity offered by inner heliosphere observations and future Voyager in situ local interstellar medium measurements to derive the He abundance in the very interstellar cloud in which we reside.},
  Keywords                 = {2104 Cosmic rays, 2124 Heliopause and solar wind termination, 2126 Heliosphere/interstellar medium interactions, 7845 Particle acceleration, INTERPLANETARY PHYSICS, Space Plasma Physics}
}

@InProceedings{Berchem2013,
  Title                    = {Plasma transport at the dayside magnetopause: observations and large-scale modeling},
  Author                   = {Berchem, Jean and Richard, Robert and Escoubet, C. Philippe and Pitout, Frederic and Taylor, Matthew G. and Laasko, Harri and Masson, Arnaud and Dandouras, Iannis and Reme, Henri},
  Booktitle                = {{EGU} {General} {Assembly} {Conference} {Abstracts}},
  Year                     = {2013},
  Pages                    = {5784},
  Volume                   = {15},

  Shorttitle               = {Plasma transport at the dayside magnetopause},
  Url                      = {http://adsabs.harvard.edu/abs/2013EGUGA..15.5784B},
  Urldate                  = {2014-10-22}
}

@Article{Bhartia,
  Title                    = {{OMI} {Algorithm} {Theoretical} {Basis} {Document} {Volume} {II}},
  Author                   = {Bhartia, Pawan K.},
  Journal                  = {OMI Ozone},

  Url                      = {ftp://snarktoo.gsfc.nasa.gov/pub/ML_climatology/old_climatology/ATBD-OMI-02.pdf},
  Urldate                  = {2014-11-13}
}

@Article{Bhartia2002,
  Title                    = {{OMI} algorithm theoretical basis document, vol. {II}},
  Author                   = {Bhartia, Pawan K},
  Journal                  = {Ozone Monitoring Instrument ozone products, version},
  Year                     = {2002},
  Volume                   = {2}
}

@Article{Bhattacharjee1998,
  Title                    = {Ballooning instability of a thin current sheet in the high-{Lundquist}-number magnetotail},
  Author                   = {Bhattacharjee, A and Ma, ZW and Wang, Xiaogang},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1998},
  Number                   = {6},
  Pages                    = {861--864},
  Volume                   = {25}
}

@InCollection{Binsack1968,
  Title                    = {Shock and magnetopause boundary observations with {IMP}-2},
  Author                   = {Binsack, Joseph H},
  Booktitle                = {Physics of the {Magnetosphere}},
  Publisher                = {Springer},
  Year                     = {1968},
  Pages                    = {605--621}
}

@Article{Binsack1967,
  Title                    = {Plasmapause observations with the {MIT} experiment on {IMP} 2},
  Author                   = {Binsack, Joseph H},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1967},
  Number                   = {21},
  Pages                    = {5231--5237},
  Volume                   = {72}
}

@Article{Binsack1968a,
  Title                    = {Simultaneous {IMP} 2 and {OGO} 1 observations of bow shock compression},
  Author                   = {Binsack, Joseph H and Vasyliunas, Vytenis M},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1968},
  Number                   = {1},
  Pages                    = {429--433},
  Volume                   = {73}
}

@Article{Birdsall1991,
  Title                    = {Particle-in-cell charged-particle simulations, plus {Monte} {Carlo} collisions with neutral atoms, {PIC}-{MCC}},
  Author                   = {Birdsall, Charles K},
  Journal                  = {Plasma Science, IEEE Transactions on},
  Year                     = {1991},
  Number                   = {2},
  Pages                    = {65--85},
  Volume                   = {19}
}

@Book{Birdsall2005,
  Title                    = {Plasma {Physics} {Via} {Computer} {Simulaition}},
  Author                   = {Birdsall, Charles Kennedy and Langdon, Allan Bruce},
  Publisher                = {CRC Press},
  Year                     = {2005}
}

@Article{Birn2005,
  Title                    = {Three-dimensional magnetotail equilibria with prescribed boundary shapes},
  Author                   = {Birn, Joachim},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2005},
  Number                   = {A7},
  Volume                   = {110}
}

@Article{Birn2001,
  Title                    = {Geospace {Environmental} {Modeling} ({GEM}) magnetic reconnection challenge},
  Author                   = {Birn, J and Drake, JF and Shay, MA and Rogers, BN and Denton, RE and Hesse, M and Kuznetsova, M and Ma, ZW and Bhattacharjee, A and Otto, A and {others}},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2001},
  Number                   = {A3},
  Pages                    = {3715--3719},
  Volume                   = {106}
}

@Article{Birn2005a,
  Title                    = {Forced magnetic reconnection},
  Author                   = {Birn, J and Galsgaard, Klaus and Hesse, M and Hoshino, M and Huba, J and Lapenta, Giovanni and Pritchett, PL and Schindler, K and Yin, L and Büchner, J and {others}},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2005},
  Number                   = {6},
  Pages                    = {L06105},
  Volume                   = {32}
}

@Article{Birn2005b,
  Title                    = {{Forced magnetic reconnection}},
  Author                   = {Birn, J and Galsgaard, Klaus and Hesse, M and Hoshino, M and Huba, J and Lapenta, Giovanni and Pritchett, P L and Schindler, K and Yin, L and B{\"{u}}chner, J and Others},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2005},
  Number                   = {6},
  Pages                    = {L06105},
  Volume                   = {32},

  __markedentry            = {[suleimanbaraka:6]},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Birn et al/Geophysical research letters/Birn et al. - 2005 - Forced magnetic reconnection.pdf:pdf},
  Owner                    = {suleimanbaraka},
  Publisher                = {American Geophysical Union},
  Timestamp                = {2016.02.23}
}

@Article{Birn1998,
  Title                    = {Formation of thin current sheets in space plasmas},
  Author                   = {Birn, Joachim and Hesse, Michael and Schindler, Karl},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1998},
  Number                   = {A4},
  Pages                    = {6843--6852},
  Volume                   = {103}
}

@Article{Birn2011,
  Title                    = {Bursty bulk flows and dipolarization in {MHD} simulations of magnetotail reconnection},
  Author                   = {Birn, J and Nakamura, R and Panov, EV and Hesse, M},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2011},
  Number                   = {A1},
  Volume                   = {116}
}

@Book{Birn2007,
  Title                    = {Reconnection of magnetic fields},
  Author                   = {Birn, Joachim and Priest, Eric R},
  Publisher                = {Cambridge University Press Cambridge},
  Year                     = {2007}
}

@Article{Birn2001a,
  Title                    = {{Geospace Environmental Modeling ( GEM ) Magnetic}},
  Author                   = {Birn, J and Shay, J F Drake M A and Hesse, N Rogersr E Denton M and Kuznetsova, M and Ma, Z W and Bhattacharjee, A and Otto, A and Pritchett, P L},
  Year                     = {2001},
  Pages                    = {3715--3719},
  Volume                   = {106},

  __markedentry            = {[suleimanbaraka:6]},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Birn et al/Unknown/Birn et al. - 2001 - Geospace Environmental Modeling ( GEM ) Magnetic.pdf:pdf},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Bisikalo2013,
  Title                    = {Three-dimensional {Gas} {Dynamic} {Simulation} of the {Interaction} between the {Exoplanet} {WASP}-12b and its {Host} {Star}},
  Author                   = {Bisikalo, D. and Kaygorodov, P. and Ionov, D. and Shematovich, V. and Lammer, H. and Fossati, L.},
  Journal                  = {{\textbackslash}textbackslashapj},
  Year                     = {2013},

  Month                    = feb,
  Pages                    = {19},
  Volume                   = {764},

  Doi                      = {10.1088/0004-637X/764/1/19},
  Keywords                 = {hydrodynamics, planet-star interactions, stars: individual: WASP-12}
}

@Book{Biskamp2005,
  Title                    = {Magnetic reconnection in plasmas},
  Author                   = {Biskamp, Dieter},
  Publisher                = {Cambridge University Press},
  Year                     = {2005},
  Number                   = {3}
}

@Article{Biskamp1973,
  Title                    = {Collisionless shock waves in plasmas},
  Author                   = {Biskamp, D},
  Journal                  = {Nucl. Fusion},
  Year                     = {1973},
  Pages                    = {719--740},
  Volume                   = {13}
}

@Article{Biskamp1972,
  Title                    = {Numerical studies of magnetosonic collisionless shock waves},
  Author                   = {Biskamp, D and Welter, H},
  Journal                  = {Nucl. Fusion},
  Year                     = {1972},
  Number                   = {6},
  Pages                    = {663},
  Volume                   = {12}
}

@Article{Blanco-Cano2006,
  Title                    = {Macrostructure of collisionless bow shocks: 2. {ULF} waves in the foreshock and magnetosheath},
  Author                   = {Blanco-Cano, X and Omidi, N and Russell, CT},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2006},
  Number                   = {A10},
  Volume                   = {111}
}

@InProceedings{Blelly1992,
  Title                    = {Observations of the structure and vertical transport of the polar upper ionosphere with the {EISCAT} {VHF} radar. {I}: {Is} {EISCAT} able to determine {O}+ and {H}+ polar wind characteristic? {A} simulation study},
  Author                   = {Blelly, Pierre-Louis and Barakat, Abdullah R and Fontanari, Jean and Alcayde, Denis and Blanc, Michel and Wu, Jian and Lathuillere, C},
  Booktitle                = {Annales geophysicae},
  Year                     = {1992},
  Pages                    = {367--374},
  Publisher                = {Copernicus},
  Volume                   = {10}
}

@Book{Board2007,
  Title                    = {Earth {Science} and {Applications} from {Space}:: {National} {Imperatives} for the {Next} {Decade} and {Beyond}},
  Author                   = {Board, Space Studies and {others}},
  Publisher                = {National Academies Press},
  Year                     = {2007},

  Shorttitle               = {Earth {Science} and {Applications} from {Space}},
  Url                      = {http://books.google.com/books?hl=en&lr=&id=5rXB3qvv8RoC&oi=fnd&pg=PA1&dq=%5B12%5D%09National+Research+Council,+Earth+Science+and+Applications+from+Space:+National+Imperatives+for+the+Next+Decade+and+Beyond,+the+National+Academy+of+Sciences,+Washington,+D.C.,+2007&ots=98dXyFeQ2t&sig=DmHGg2RMV4mHiK3ZP4d_YtgDezw},
  Urldate                  = {2014-11-13}
}

@Article{Boardsen2009,
  Title                    = {Narrow-band ultra-low-frequency wave observations by {MESSENGER} during its {January} 2008 flyby through {Mercury}'s magnetosphere},
  Author                   = {Boardsen, S. A. and Anderson, B. J. and Acuña, M. H. and Slavin, J. A. and Korth, H. and Solomon, S. C.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {2009},

  Month                    = jan,
  Pages                    = {1104},
  Volume                   = {36},

  Doi                      = {10.1029/2008GL036034},
  Keywords                 = {2752, 6050), Planetary Sciences: Solar System Objects: Mercury, Radio Science: Waves in plasma (7867), Space Plasma Physics: Kinetic waves and instabilities, Space Plasma Physics: MHD waves and instabilities (2149}
}

@Article{Bochsler2007,
  Title                    = {Solar abundances of oxygen and neon derived from solar wind observations},
  Author                   = {Bochsler, P.},
  Journal                  = {{\textbackslash}aap},
  Year                     = {2007},

  Month                    = aug,
  Pages                    = {315--319},
  Volume                   = {471},

  Doi                      = {10.1051/0004-6361:20077772},
  Keywords                 = {Sun: abundances, Sun: corona, Sun: photosphere, Sun: solar wind}
}

@Article{Bochsler1986,
  Title                    = {Abundances of carbon, oxygen, and neon in the solar wind during the period from {August} 1978 to {June} 1982},
  Author                   = {Bochsler, P. and Geiss, J. and Kunz, S.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {1986},

  Month                    = jan,
  Pages                    = {177--201},
  Volume                   = {103},

  Doi                      = {10.1007/BF00154867},
  Keywords                 = {Abundance, Carbon, Heavy Ions, International Sun Earth Explorer 3, Mass Spectra, Neon, Oxygen, Solar Wind}
}

@Article{Bodmer2000,
  Title                    = {Influence of {Coulomb} collisions on isotopic and elemental fractionation in the solar wind acceleration process},
  Author                   = {Bodmer, R. and Bochsler, P.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {2000},

  Month                    = jan,
  Pages                    = {47--60},
  Volume                   = {105},

  Doi                      = {10.1029/1999JA900434},
  Keywords                 = {Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Sources of the solar wind, Magnetospheric Physics: Plasma sheet, Space Plasma Physics: Numerical simulation studies}
}

@Article{Boeke2011,
  Title                    = {Formaldehyde columns from the {Ozone} {Monitoring} {Instrument}: {Urban} versus background levels and evaluation using aircraft data and a global model},
  Author                   = {Boeke, Nicholas L. and Marshall, Julian D. and Alvarez, Sergio and Chance, Kelly V. and Fried, Alan and Kurosu, Thomas P. and Rappengl‚Äö√†√∂¬¨‚à´ck, Bernhard and Richter, Dirk and Walega, James and Weibring, Petter and {others}},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2011},
  Number                   = {D5},
  Volume                   = {116},

  Shorttitle               = {Formaldehyde columns from the {Ozone} {Monitoring} {Instrument}},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2010JD014870/full},
  Urldate                  = {2014-11-13}
}

@Article{Boersma2004,
  Title                    = {Error analysis for tropospheric {NO}2 retrieval from space},
  Author                   = {Boersma, K. F. and Eskes, H. J. and Brinksma, E. J.},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2004},
  Number                   = {D4},
  Volume                   = {109},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2003JD003962/full},
  Urldate                  = {2014-11-13}
}

@InProceedings{Bogdan2008,
  Title                    = {The {Space} {Weather} {Prediction} {Center}: {Changing} {To} {Be} {Ready} {For} {Cycle} 24},
  Author                   = {Bogdan, Tom and Murtagh, Bill and Kunches, Joseph},
  Booktitle                = {37th {COSPAR} {Scientific} {Assembly}},
  Year                     = {2008},
  Pages                    = {338},
  Volume                   = {37},

  Url                      = {http://adsabs.harvard.edu/abs/2008cosp...37..338B}
}

@Article{Bogdanova2004,
  Title                    = {Correlation between suprathermal electron bursts, broadband extremely low frequency waves, and local ion heating in the midaltitude cleft/low-latitude boundary layer observed by {Cluster}},
  Author                   = {Bogdanova, Y. V. and Fazakerley, A. N. and Owen, C. J. and Klecker, B. and Cornilleau-Wehrlin, N. and Grison, B. and André, M. and Cargill, P. and RèMe, H. and Bosqued, J. M. and Kistler, L. M. and Balogh, A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = dec,
  Number                   = {A18},
  Pages                    = {12226},
  Volume                   = {109},

  Doi                      = {10.1029/2004JA010554},
  Keywords                 = {and boundary layers, cleft electron observations, cusp, dayside ion outflow, ion heating in the cleft/cusp, Magnetospheric Physics: Magnetopause, Magnetospheric Physics: Magnetosphere/ionosphere interactions, Space Plasma Physics: Charged particle motion and acceleration, Space Plasma Physics: Wave/particle interactions, wave/particle interaction}
}

@Article{Bogdanova2004a,
  Title                    = {Correlation between suprathermal electron bursts, broadband extremely low frequency waves, and local ion heating in the midaltitude cleft/low-latitude boundary layer observed by {Cluster}},
  Author                   = {Bogdanova, Y. V. and Fazakerley, A. N. and Owen, C. J. and Klecker, B. and Cornilleau-Wehrlin, N. and Grison, B. and Andr√©, M. and Cargill, P. and R√®Me, H. and Bosqued, J. M. and Kistler, L. M. and Balogh, A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = dec,
  Number                   = {A18},
  Pages                    = {12226},
  Volume                   = {109},

  Doi                      = {10.1029/2004JA010554},
  Keywords                 = {and boundary layers, cleft electron observations, cusp, dayside ion outflow, ion heating in the cleft/cusp, Magnetospheric Physics: Magnetopause, Magnetospheric Physics: Magnetosphere/ionosphere interactions, Space Plasma Physics: Charged particle motion and acceleration, Space Plasma Physics: Wave/particle interactions, wave/particle interaction}
}

@Article{Bonifazi1981,
  Title                    = {Reflected and diffuse ions backstreaming from the {Earth}'s bow shock 2. {Origin}},
  Author                   = {Bonifazi, C and Moreno, G},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1981},
  Number                   = {A6},
  Pages                    = {4405--4413},
  Volume                   = {86}
}

@Article{Book1995,
  Title                    = {Plasma transport through the magnetopause by turbulent interchange processes},
  Author                   = {Book, David L. and Sibeck, David G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1995},
  Pages                    = {9567--9574},
  Volume                   = {100},

  Abstract                 = {The turbulent motion of the plasma compressed behind the Earth's bow shock can cause magnetospheric field lines at the magnetopause to develop localized regions or negative curvature. These regions are unstable with respect to interchange, which can lead to significant transport of mass and energy across the magnetopause. The rate at which magnetosheath plasma crosses the magnetopause is estimated to be of order 10{\textless}SUP{\textgreater}2{\textless}/SUP{\textgreater}{\textless}SUP{\textgreater}6{\textless}/SUP{\textgreater} s{\textless}SUP{\textgreater}-{\textless}/SUP{\textgreater}{\textless}SUP{\textgreater}1{\textless}/SUP{\textgreater}, which is consistent with estimates based on observations.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Solar wind plasma Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Magnetospheric configuration and dynamics},
  Url                      = {http://adsabs.harvard.edu/abs/1995JGR...100.9567B}
}

@InProceedings{Boris1970,
  Title                    = {Relativistic plasma simulation-optimization of a hybrid code},
  Author                   = {Boris, JP},
  Booktitle                = {Proc. {Fourth} {Conf}. {Num}. {Sim}. {Plasmas}, {Naval} {Res}. {Lab}, {Wash}. {DC}},
  Year                     = {1970},
  Pages                    = {3--67}
}

@Article{Borodkova1998,
  Title                    = {Fast {Deformation} of {Dayside} {Magnetopause}},
  Author                   = {Borodkova, N. L. and Sibeck, D. G. and Zastenker, G. N. and Romanov, S. A. and Sauvaud, J.-A.},
  Journal                  = {Cosmic Research},
  Year                     = {1998},
  Pages                    = {245},
  Volume                   = {36},

  Abstract                 = {Not Available},
  ISSN                     = {0023-4206},
  Url                      = {http://adsabs.harvard.edu/abs/1998CosRe..36..245B}
}

@Article{Borodkova1995,
  Title                    = {A case and statistical study of transient magnetic field events at geosynchronous orbit and their solar wind origin},
  Author                   = {Borodkova, N. L. and Zastenker, G. N. and Sibeck, D. G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1995},
  Pages                    = {5643--5656},
  Volume                   = {100},

  Abstract                 = {We present a statisical survey of Prognoz 10 solar wind observations at the times of transient (step function and impulsive) variations in the dayside magnetospheric magnetic field strength measured by the GOES 5 and 6 geosynchronous satellites. The results indicate that 51\% of the magnetospheric events can be associated with corresponding variations in the solar wind dynamic pressure. A further 17\% of the events can be associated with fluctuations in the interplanetary magnetic field orientation in the sense previously associated with foreshock pressure pulses. We find no tendency for impulsive events at dayside geosynchronous orbit to be associated with north/south fluctuations in the interplanetary magnetic field (IMF) orientation, nor for the events to occur primarily during intervals of southward IMF. The success rate for associating transient events at dayside geosynchronous orbit with solar wind features decreases as Prognoz 10 moves farther from the Earth-Sun line. The observations indicate that variations in the solar wind dynamic pressure and foreshock pressure pulses associated with variations in the IMF cone angle are the predominant causes of large-amplitude transient events observed at dayside geosynchronous orbit.},
  ISSN                     = {0148-0227},
  Keywords                 = {Case Histories Earth Magnetosphere Geomagnetism Geosynchronous Orbits Magnetic Flux Solar Terrestrial Interactions Solar Wind Statistical Analysis Transient Response Goes 5 Goes 6 Magnetometers Plasma Diagnostics Prognoz Satellites Step Functions Temporal Resolution},
  Url                      = {http://adsabs.harvard.edu/abs/1995JGR...100.5643B}
}

@Article{Borovsky2013,
  Title                    = {Estimating the effects of ionospheric plasma on solar wind/magnetosphere coupling via mass loading of dayside reconnection: {Ion}-plasma-sheet oxygen, plasmaspheric drainage plumes, and the plasma cloak},
  Author                   = {Borovsky, Joseph E. and Denton, Michael H. and Denton, Richard E. and Jordanova, Vania K. and Krall, Jonathan},
  Journal                  = {Journal of Geophysical Research: Space Physics},
  Year                     = {2013},
  Number                   = {9},
  Pages                    = {5695--5719},
  Volume                   = {118},

  Shorttitle               = {Estimating the effects of ionospheric plasma on solar wind/magnetosphere coupling via mass loading of dayside reconnection},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1002/jgra.50527/full},
  Urldate                  = {2014-05-31}
}

@Article{Boteler1999,
  Title                    = {August 4, 1972 revisited: {A} new look at the geomagnetic disturbance that caused the {L}4 cable system outage},
  Author                   = {Boteler, D. H. and van Beek, G. J.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {1999},
  Pages                    = {577--580},
  Volume                   = {26},

  Doi                      = {10.1029/1999GL900035},
  Keywords                 = {magnetospheric physics, Magnetospheric Physics: Solar wind/magnetosphere interactions}
}

@Book{Bothmer2007,
  Title                    = {Introduction},
  Author                   = {Bothmer, Volker and Daglis, Ioannis A},
  Publisher                = {Springer},
  Year                     = {2007}
}

@Article{Boudouridis2003,
  Title                    = {Effect of solar wind pressure pulses on the size and strength of the auroral oval},
  Author                   = {Boudouridis, A. and Zesta, E. and Lyons, R. and Anderson, P. C. and Lummerzheim, D.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2003},

  Month                    = apr,
  Pages                    = {8012},
  Volume                   = {108},

  Abstract                 = {It has recently been found that solar wind dynamic pressure changes can dramatically affect the precipitation of magnetospheric particles on the high-latitude ionosphere. We have examined the effect of large solar wind dynamic pressure increases on the location, size, and intensity of the auroral oval using particle precipitation data from Defense Meteorological Satellite Program (DMSP) spacecraft. Three events have been selected for study during the time period after 1997 when four DMSP spacecraft (F11-F14) were simultaneously operational. Interplanetary magnetic field (IMF) orientation is different from event to event. For each event, we determine equatorward and poleward boundaries of the auroral oval before and after an increase in solar wind pressure. Also, using measured integral fluxes, we construct precipitating particle energy input maps for the auroral oval. All cases studied show a significant change of the auroral oval location, size, and intensity in response to the solar wind pressure pulse. Most prominent are an increase of the auroral zone width and a decrease of the polar cap size when the solar wind dynamic pressure increases under steady southward IMF conditions. An increase in total precipitating particle energy flux is also observed. A smaller response is seen when the IMF Bz has a simultaneous northward turning and when it is nearly zero before the pressure enhancement. Our results also point to significant differences between the auroral precipitation response to solar wind pressure changes and its response to isolated substorms, the former inducing a global auroral reaction while the latter is related to more localized premidnight disturbances. Auroral UV observations from the Polar spacecraft during our events are found to give results consistent with the results we get from the precipitating particle observations.},
  Doi                      = {10.1029/2002JA009373},
  Keywords                 = {Magnetospheric Physics: Auroral phenomena (2407), Magnetospheric Physics: Energetic particles, Magnetospheric Physics: Polar cap phenomena, Magnetospheric Physics: Solar wind/magnetosphere interactions, precipitating}
}

@Article{Bouhram2004,
  Title                    = {Multipoint analysis of the spatio-temporal coherence of dayside {O}+ outflows with {Cluster}},
  Author                   = {Bouhram, M. and Klecker, B. and Paschmann, G. and Rème, H. and Blagau, A. and Kistler, L. and Puhl-Quinn, P. and Sauvaud, J.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2004},

  Month                    = jul,
  Pages                    = {2507--2514},
  Volume                   = {22},

  Doi                      = {10.5194/angeo-22-2507-2004}
}

@Article{Bouhram2004a,
  Title                    = {Multipoint analysis of the spatio-temporal coherence of dayside {O}+ outflows with {Cluster}},
  Author                   = {Bouhram, M. and Klecker, B. and Paschmann, G. and R√®me, H. and Blagau, A. and Kistler, L. and Puhl-Quinn, P. and Sauvaud, J.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2004},

  Month                    = jul,
  Pages                    = {2507--2514},
  Volume                   = {22},

  Doi                      = {10.5194/angeo-22-2507-2004}
}

@Article{Bouhram2003,
  Title                    = {Modeling transverse heating and outflow of ionospheric ions from the dayside cusp/cleft. 1 {A} parametric study},
  Author                   = {Bouhram, M and Malingre, M and Jasperse, JR and Dubouloz, N},
  Year                     = {2003},

  Url                      = {http://oai.dtic.mil/oai/oai?verb=getRecord&metadataPrefix=html&identifier=ADA423203}
}

@InProceedings{Brackbill2012,
  Title                    = {Magnetic {Reconnection} {Scaling} from {Kinetic} {Simulations}},
  Author                   = {Brackbill, Jeremiah},
  Booktitle                = {{APS} {Meeting} {Abstracts}},
  Year                     = {2012},
  Pages                    = {8053P},
  Volume                   = {1},

  Url                      = {http://adsabs.harvard.edu/abs/2012APS..DPPCP8053B},
  Urldate                  = {2014-05-31}
}

@Article{Brackbill1982,
  Title                    = {An implicit method for electromagnetic plasma simulation in two dimensions},
  Author                   = {Brackbill, JU and Forslund, DW},
  Journal                  = {J. Comput. Phys.},
  Year                     = {1982},
  Number                   = {2},
  Pages                    = {271--308},
  Volume                   = {46}
}

@Article{Brackbill1993,
  Title                    = {Electron kinetic effects in switch-off slow shocks},
  Author                   = {Brackbill, JU and Vu, HX},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1993},
  Number                   = {19},
  Pages                    = {2015--2018},
  Volume                   = {20}
}

@Article{Brackbill2011,
  Title                    = {A comparison of fluid and kinetic models of steady magnetic reconnection},
  Author                   = {Brackbill, J. U.},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2011},
  Number                   = {3},
  Pages                    = {032309},
  Volume                   = {18},

  Url                      = {http://scitation.aip.org/content/aip/journal/pop/18/3/10.1063/1.3568828},
  Urldate                  = {2014-05-31}
}

@Article{Branduardi-Raymont2012,
  Title                    = {{AXIOM}: advanced {X}-ray imaging of the magnetosphere},
  Author                   = {Branduardi-Raymont, Graziella and Sembay, Steve F. and Eastwood, Jonathan P. and Sibeck, David G. and Abbey, Tony A. and Brown, Patrick and Carter, Jenny A. and Carr, Chris M. and Forsyth, Colin and Kataria, Dhiren and Kemble, Steve and Milan, Steve E. and Owen, Chris J. and Peacocke, Lisa and Read, Andy M. and Coates, Andrew J. and Collier, Michael R. and Cowley, Stan W. H. and Fazakerley, Andrew N. and Fraser, George W. and Jones, Geraint H. and Lallement, Rosine and Lester, Mark and Porter, F. Scott and Yeoman, Tim K.},
  Journal                  = {Experimental Astronomy},
  Year                     = {2012},
  Pages                    = {403--443},
  Volume                   = {33},

  Abstract                 = {Planetary plasma and magnetic field environments can be studied in two complementary ways—by in situ measurements, or by remote sensing. While the former provide precise information about plasma behaviour, instabilities and dynamics on local scales, the latter offers the global view necessary to understand the overall interaction of the magnetospheric plasma with the solar wind. Some parts of the Earth's magnetosphere have been remotely sensed, but the majority remains unexplored by this type of measurements. Here we propose a novel and more elegant approach employing remote X-ray imaging techniques, which are now possible thanks to the relatively recent discovery of solar wind charge exchange X-ray emissions in the vicinity of the Earth's magnetosphere. In this article we describe how an appropriately designed and located X-ray telescope, supported by simultaneous in situ measurements of the solar wind, can be used to image the dayside magnetosphere, magnetosheath and bow shock, with a temporal and spatial resolution sufficient to address several key outstanding questions concerning how the solar wind interacts with the Earth's magnetosphere on a global level. Global images of the dayside magnetospheric boundaries require vantage points well outside the magnetosphere. Our studies have led us to propose `AXIOM: Advanced X-ray Imaging of the Magnetosphere', a concept mission using a Vega launcher with a LISA Pathfinder-type Propulsion Module to place the spacecraft in a Lissajous orbit around the Earth-Moon L1 point. The model payload consists of an X-ray Wide Field Imager, capable of both imaging and spectroscopy, and an in situ plasma and magnetic field measurement package. This package comprises a Proton-Alpha Sensor, designed to measure the bulk properties of the solar wind, an Ion Composition Analyser, to characterise the minor ion populations in the solar wind that cause charge exchange emission, and a Magnetometer, designed to measure the strength and direction of the solar wind magnetic field. We also show simulations that demonstrate how the proposed X-ray telescope design is capable of imaging the predicted emission from the dayside magnetosphere with the sensitivity and cadence required to achieve the science goals of the mission.},
  ISSN                     = {0922-6435},
  Keywords                 = {X-rays Space telescope Space plasma instrumentation Magnetometer Techniques Imaging Spectroscopy Plasma and field analysers},
  Url                      = {http://adsabs.harvard.edu/abs/2012ExA....33..403B}
}

@Article{Brassard2010,
  Title                    = {{Can quantum-mechanical description of physical reality be considered correct?}},
  Author                   = {Brassard, Gilles and M{\'{e}}thot, A. Allan},
  Journal                  = {Found. Phys.},
  Year                     = {2010},
  Number                   = {4},
  Volume                   = {40},

  __markedentry            = {[suleimanbaraka:]},
  Archiveprefix            = {arXiv},
  Arxivid                  = {quant-ph/0701001},
  Doi                      = {10.1007/s10701-010-9411-9},
  Eprint                   = {0701001},
  ISBN                     = {0031-899X$\backslash$r1536-6065},
  ISSN                     = {00159018},
  Owner                    = {suleimanbaraka},
  Pmid                     = {201519800010},
  Primaryclass             = {quant-ph},
  Timestamp                = {2016.02.23}
}

@InCollection{Brekke2005,
  Title                    = {Space weather effects on {SOHO} and its space weather warning capabilities},
  Author                   = {Brekke, P and Chaloupy, M and Fleck, B and Haugan, SV and van Overbeek, T and Schweitzer, H},
  Booktitle                = {Effects of {Space} {Weather} on {Technology} {Infrastructure}},
  Publisher                = {Springer},
  Year                     = {2005},
  Pages                    = {109--122},

  Url                      = {http://link.springer.com/chapter/10.1007/1-4020-2754-0_6}
}

@Article{Bristow1995,
  Title                    = {Observations of convection vortices in the afternoon sector using the {SuperDARN} {HF} radars},
  Author                   = {Bristow, W. A. and Sibeck, D. G. and Jacquey, C. and Greenwald, R. A. and Sofko, G. J. and Mukai, T. and Yamamoto, T. and Kokubun, S. and Hughes, T. J. and Hughes, W. J. and Engebretson, M. J.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1995},
  Pages                    = {19743--19756},
  Volume                   = {100},

  Abstract                 = {Observation of convection vortices using the new SuperDARN HF radars are presented. The velocity field derived from the overlapping fields of view of the new HF radars at Kapuskasing, Ontario, and Saskatoon, Saskatchewan, Canada, often image the portion of the convection pattern near the convection reversal boundary. Observations from near the convection reversal boundary in the afternoon sector of October 22, 1993, showed two convection vortices evolving within the field of view of both radars. The first vortex appeared at about 2120 UT and the second at about 2145 UT: 1446 MLT and 1512 MLT, respectively. The vortices were roughly 900 km in diameter and moved tailward with a velocity of about 600 m/s. At the times the vortices were observed by the radars, ground-based magnetometers of the CANOPUS and MACCS chains show transient deflections of near 100 nT, and the GOES 6 and GOES 7 satellite magnetometers showed significant decreases in the magnetospheric magnetic field strength. Data from the Geotail satellite magnetometer lagged by an appropriate time interval indicated that there were southward turnings of the interplanetary magnetic field that coincided with the decreases of magnetospheric magnetic field strength. The observations differ in many respects from previously published vortex observations. It is theorized that the vortices were caused by the Kelvin-Helmholtz instability at the inner edge of the low-latitude boundary layer.},
  ISSN                     = {0148-0227},
  Keywords                 = {Ionosphere: Ionosphere/magnetosphere interactions Ionosphere: Ionospheric dynamics Magnetospheric Physics: Magnetosphere/ionosphere interactions Magnetospheric Physics: Magnetopause cusp and boundary layers},
  Url                      = {http://adsabs.harvard.edu/abs/1995JGR...10019743B}
}

@Article{Brittnacher1995,
  Title                    = {A new approach to the linear theory of single-species tearing in two-dimensional quasi-neutral sheets},
  Author                   = {Brittnacher, M and Quest, KB and Karimabadi, H},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1995},
  Number                   = {A3},
  Pages                    = {3551--3562},
  Volume                   = {100}
}

@Article{Brown1976,
  Title                    = {A model of {Jupiter}'s sulfur nebula},
  Author                   = {Brown, R. A.},
  Journal                  = {{\textbackslash}textbackslashapjl},
  Year                     = {1976},

  Month                    = jun,
  Pages                    = {L179--L183},
  Volume                   = {206},

  Doi                      = {10.1086/182162},
  Keywords                 = {Atmospheric Composition, Atmospheric Models, Atmospheric Radiation, Electron Density (Concentration), Electron Energy, Electron Impact, Forbidden Bands, Io, Jupiter Atmosphere, Jupiter (Planet), Nebulae, Sulfur}
}

@Book{Buechner2003,
  Title                    = {Space plasma simulation},
  Author                   = {Büchner, Jörg and Dum, Christian and Scholer, Manfred},
  Publisher                = {Springer},
  Year                     = {2003},
  Volume                   = {615}
}

@InProceedings{Buechner1996,
  Title                    = {Three-dimensional collisionless reconnection through thin current sheets-theory and self-consistent simulations},
  Author                   = {Büchner, Jörg and Kuska, J-P},
  Booktitle                = {International {Conference} on {Substorms}},
  Year                     = {1996},
  Pages                    = {373},
  Volume                   = {389}
}

@Article{Buneman,
  Title                    = {{TRISTAN}: {The} 3-{D} {EM} {Particle} {Code}, {Computer} {Space} {Plasma} {Physics}: {Simulation} {Techniques} and {Software} {H}},
  Author                   = {Buneman, O},
  Journal                  = {Space Plasmas},
  Volume                   = {67}
}

@Article{Bunemana,
  Title                    = {{TRISTAN}: {The} 3-{D}, {EM} particle code, {Computer} {Space} {Plasma} {Physics}, {Simulation} {Techniques} and {Software} {H}},
  Author                   = {Buneman, O},
  Journal                  = {Matsumoto, Y. Omura},
  Volume                   = {67}
}

@Article{Buneman1993,
  Title                    = {Computer space plasma physics},
  Author                   = {Buneman, O},
  Journal                  = {Simulation Techniques and Software},
  Year                     = {1993},
  Pages                    = {67}
}

@Article{Buneman1993a,
  Title                    = {{TRISTAN}: {The} 3-{D}, {EM} {Particle} {Code}},
  Author                   = {Buneman, Oscar},
  Journal                  = {Computer Space Plasma Physics, Simulation Techniques and Software},
  Year                     = {1993},
  Pages                    = {67}
}

@Article{Buneman1980,
  Title                    = {Principles and capabilities of 3-{D}, {EM} particle simulations},
  Author                   = {Buneman, O and Barnes, CW and Green, JC and Nielsen, DE},
  Journal                  = {J. Comput. Phys.},
  Year                     = {1980},
  Number                   = {1},
  Pages                    = {1--44},
  Volume                   = {38}
}

@Article{Buneman1992,
  Title                    = {Solar wind-magnetosphere interaction as simulated by a 3-{D} {EM} particle code},
  Author                   = {Buneman, Oscar and Neubert, Torsten and Nishikawa, K-I},
  Journal                  = {Plasma Science, IEEE Transactions on},
  Year                     = {1992},
  Number                   = {6},
  Pages                    = {810--816},
  Volume                   = {20}
}

@Article{Buneman1992a,
  Title                    = {Solar wind-magnetosphere interaction as simulated by a 3-{D} {EM} particle code},
  Author                   = {Buneman, O. and Neubert, T. and Nishikawa, K.-I.},
  Journal                  = {IEEE},
  Year                     = {1992},

  Month                    = dec,
  Pages                    = {810--816},
  Volume                   = {20},

  Doi                      = {10.1109/27.199533},
  Keywords                 = {Computerized Simulation, Earth Magnetosphere, Flux Transfer Events, Lorentz Transformations, Magnetic Field Reconnection, Particle Motion, Solar Terrestrial Interactions, Solar Wind, Three Dimensional Models}
}

@Article{Buneman1995,
  Title                    = {Solar {Wind}-{Magnetosphere} {Interaction} as {Simulated} by a 3D, {Em} {Particle} {Code}},
  Author                   = {Buneman, Oscar and Nishikawa, Ken-Ichi and Neubert, Torsten},
  Journal                  = {Space Plasmas: Coupling Between Small and Medium Scale Processes},
  Year                     = {1995},
  Pages                    = {347--356}
}

@Article{Buneman1995a,
  Title                    = {Solar {Wind}-{Magnetosphere} {Interaction} as {Simulated} by a 3D, {EM} {Particle} {Code}},
  Author                   = {Buneman, O. and Nishikawa, K.-I. and Neubert, T.},
  Journal                  = {Washington DC American Geophysical Union Geophysical Monograph Series},
  Year                     = {1995},
  Pages                    = {347},
  Volume                   = {86},

  Abstract                 = {Not Available}
}

@Article{Burch2005,
  Title                    = {Magnetospheric imaging: {Promise} to reality},
  Author                   = {Burch, J. L.},
  Journal                  = {Rev. Geophys.},
  Year                     = {2005},

  Month                    = sep,
  Pages                    = {3001},
  Volume                   = {43},

  Abstract                 = {Measurements of the plasmas, energetic particles, and electric and magnetic fields within the Earth's magnetosphere have been made with ever greater coverage and precision throughout the past 46 years; but until recently, no images of this important environment were available. However, for 2 decades or more, theoretical estimates, data from sounding rockets, and background signals from orbiting instruments designed for in situ ion measurements accumulated to show that most of the plasmas contained in the inner magnetosphere could be imaged if new instruments designed for the purpose could be placed in a suitable high-altitude orbit. With the launch of the NASA IMAGE satellite in March 2000 the promise of magnetospheric imaging began to be realized. IMAGE provides nearly continuous imaging of the inner magnetosphere on a nominal timescale of 2 min. The discoveries made by IMAGE during its first 5 years of operation are reviewed in this paper.},
  Doi                      = {10.1029/2004RG000160},
  Keywords                 = {inner magnetosphere dynamics, magnetic storms, Magnetospheric Physics: Auroral phenomena (2407), Magnetospheric Physics: Magnetic storms and substorms (7954), Magnetospheric Physics: Magnetosphere: inner, Magnetospheric Physics: Plasmasphere, Magnetospheric Physics: Ring current, neutral atom imaging, ultraviolet imaging}
}

@Article{Burgess2006,
  Title                    = {Interpreting multipoint observations of substructure at the quasi-perpendicular bow shock: {Simulations}},
  Author                   = {Burgess, D},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2006},
  Number                   = {A10},
  Volume                   = {111}
}

@Article{Burgess1997,
  Title                    = {What do we really know about upstream waves?},
  Author                   = {Burgess, D},
  Journal                  = {Advances in Space Research},
  Year                     = {1997},
  Number                   = {4},
  Pages                    = {673--682},
  Volume                   = {20}
}

@Article{Burgess1989,
  Title                    = {Cyclic behavior at quasi-parallel collisionless shocks},
  Author                   = {Burgess, D},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1989},
  Number                   = {5},
  Pages                    = {345--348},
  Volume                   = {16}
}

@Article{Burgess2012,
  Title                    = {Ion {Acceleration} at the {Earth}'s {Bow} {Shock}},
  Author                   = {Burgess, D. and Möbius, E. and Scholer, M.},
  Journal                  = {Space Sci. Rev.},
  Year                     = {2012},

  Month                    = nov,
  Pages                    = {5--47},
  Volume                   = {173},

  Doi                      = {10.1007/s11214-012-9901-5},
  Keywords                 = {bow shock, Collisionless shock, ion acceleration, Particle Acceleration, Space plasma}
}

@Article{Burkhart1990,
  Title                    = {Magnetic reconnection in collisionless plasmas: {Prescribed} fields},
  Author                   = {Burkhart, GR and Drake, JF and Chen, J},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1990},
  Number                   = {A11},
  Pages                    = {18833--18848},
  Volume                   = {95}
}

@Article{Burkhart1990a,
  Title                    = {{Magnetic reconnection in collisionless plasmas: Prescribed fields}},
  Author                   = {Burkhart, G R and Drake, J F and Chen, J},
  Journal                  = {J. Geophys. Res. Sp. Phys.},
  Year                     = {1990},
  Number                   = {A11},
  Pages                    = {18833--18848},
  Volume                   = {95},

  __markedentry            = {[suleimanbaraka:6]},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Burkhart, Drake, Chen/Journal of Geophysical Research Space Physics (1978--2012)/Burkhart, Drake, Chen - 1990 - Magnetic reconnection in collisionless plasmas Prescribed fields.pdf:pdf},
  Owner                    = {suleimanbaraka},
  Publisher                = {Wiley Online Library},
  Timestamp                = {2016.02.23}
}

@Article{Burlaga1998,
  Title                    = {A magnetic cloud containing prominence material - {January} 1997},
  Author                   = {Burlaga, L. and Fitzenreiter, R. and Lepping, R. and Ogilvie, K. and Szabo, A. and Lazarus, A. and Steinberg, J. and Gloeckler, G. and Howard, R. and Michels, D. and Farrugia, C. and Lin, R. P. and Larson, D. E.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1998},

  Month                    = jan,
  Pages                    = {277},
  Volume                   = {103},

  Doi                      = {10.1029/97JA02768},
  Keywords                 = {Coronal Mass Ejection, Force-Free Magnetic Fields, Helium Ions, Hydrogen Ions, Interplanetary Magnetic Fields, Magnetic Clouds, Magnetic Field Configurations, Plasma Composition, Soho Mission, Solar Instruments, Solar Prominences, Solar Wind}
}

@Article{Burlaga1981,
  Title                    = {Magnetic loop behind an interplanetary shock - {Voyager}, {Helios}, and {IMP} 8 observations},
  Author                   = {Burlaga, L. and Sittler, E. and Mariani, F. and Schwenn, R.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1981},

  Month                    = aug,
  Pages                    = {6673--6684},
  Volume                   = {86},

  Doi                      = {10.1029/JA086iA08p06673},
  Keywords                 = {Cosmic Plasma, Explorer 50 Satellite, Flow Velocity, Helios Satellites, Interplanetary Magnetic Fields, Loops, Magnetic Clouds, Magnetic Field Configurations, Magnetohydrodynamic Flow, Plasma Density, Plasma Sheaths, Plasma Temperature, Plasma Turbulence, Pressure Distribution, Satellite Observation, Shock Discontinuity, shock waves, Voyager Project}
}

@Article{Burlaga1982,
  Title                    = {Magnetic clouds - {Voyager} observations between 2 and 4 {AU}},
  Author                   = {Burlaga, L. F. and Behannon, K. W.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {1982},

  Month                    = nov,
  Pages                    = {181--192},
  Volume                   = {81},

  Doi                      = {10.1007/BF00151989},
  Keywords                 = {Dynamic Characteristics, Dynamic Stability, Interplanetary Magnetic Fields, Loops, Magnetic Clouds, Magnetohydrodynamic Flow, Solar Wind, Solar Wind Velocity}
}

@Article{Burlaga1987,
  Title                    = {Compound streams, magnetic clouds, and major geomagnetic storms},
  Author                   = {Burlaga, L. F. and Behannon, K. W. and Klein, L. W.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1987},

  Month                    = jun,
  Pages                    = {5725--5734},
  Volume                   = {92},

  Doi                      = {10.1029/JA092iA06p05725},
  Keywords                 = {Ejecta, Geomagnetism, INTERPLANETARY MEDIUM, Magnetic Clouds, magnetic storms, Plasma Clouds, Satellite Sounding, Solar Flares, Solar Terrestrial Interactions, Solar Wind}
}

@Article{Bust2007,
  Title                    = {Four-dimensional {GPS} imaging of space weather storms},
  Author                   = {Bust, GS and Crowley, G and Garner, TW and Gaussiran, TL and Meggs, Robert W and Mitchell, Cathryn N and Spencer, Paul SJ and Yin, Ping and Zapfe, Bettina},
  Journal                  = {Space Weather},
  Year                     = {2007},
  Number                   = {2},
  Volume                   = {5}
}

@Article{Byhring2011,
  Title                    = {The {Helium} {Abundance} in {Polar} {Coronal} {Holes} and the {Fast} {Solar} {Wind}},
  Author                   = {Byhring, H. S.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2011},

  Month                    = sep,
  Pages                    = {172},
  Volume                   = {738},

  Doi                      = {10.1088/0004-637X/738/2/172},
  Keywords                 = {Sun: abundances, Sun: chromosphere, Sun: corona, Sun: heliosphere}
}

@Article{Bykov2011,
  Title                    = {Fundamentals of collisionless shocks for astrophysical application, 2. Relativistic shocks},
  Author                   = {Bykov, AM and Treumann, RA},
  Journal                  = {The Astronomy and Astrophysics Review},
  Year                     = {2011},
  Number                   = {1},
  Pages                    = {1--67},
  Volume                   = {19},

  Owner                    = {suleimanbaraka},
  Publisher                = {Springer},
  Timestamp                = {2016.02.20}
}

@Article{Bykov2012,
  Title                    = {Twinkling pulsar wind nebulae in the synchrotron cut-off regime and the γ-ray flares in the {Crab} {Nebula}},
  Author                   = {Bykov, A. M. and Pavlov, G. G. and Artemyev, A. V. and Uvarov, Y. A.},
  Journal                  = {{\textbackslash}mnras},
  Year                     = {2012},

  Month                    = mar,
  Pages                    = {L67--L71},
  Volume                   = {421},

  Doi                      = {10.1111/j.1745-3933.2011.01208.x},
  Keywords                 = {ISM: supernova remnants, shock waves, supernovae: individual: Crab Nebula, turbulence}
}

@Article{Boe2013,
  Title                    = {Effect of {Coulomb} {Collisions} on the {Gravitational} {Settling} of {Low} and {High} {First} {Ionization} {Potential} {Elements}},
  Author                   = {Bø, I. M. T. and Esser, R. and Lie-Svendsen, Ø.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2013},

  Month                    = may,
  Pages                    = {60},
  Volume                   = {769},

  Doi                      = {10.1088/0004-637X/769/1/60},
  Keywords                 = {Sun: abundances, Sun: chromosphere, Sun: corona}
}

@Article{Blecki2002,
  Title                    = {Preface},
  Author                   = {Bł ęcki, Jan and Sibeck, David G.},
  Journal                  = {Advances in Space Research},
  Year                     = {2002},
  Pages                    = {1619--1619},
  Volume                   = {30},

  Abstract                 = {Not Available},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/2002AdSpR..30.1619B}
}

@Article{Caffau2011,
  Title                    = {Solar {Chemical} {Abundances} {Determined} with a {CO}5BOLD 3D {Model} {Atmosphere}},
  Author                   = {Caffau, E. and Ludwig, H.-G. and Steffen, M. and Freytag, B. and Bonifacio, P.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {2011},

  Month                    = feb,
  Pages                    = {255--269},
  Volume                   = {268},

  Doi                      = {10.1007/s11207-010-9541-4},
  Keywords                 = {Convection, hydrodynamics, LINE: FORMATION, Radiative Transfer, Sun: abundances, Sun: photosphere}
}

@Article{Cahill1973,
  Title                    = {Magnetic storm inflation in the evening sector},
  Author                   = {Cahill, LJ},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1973},
  Number                   = {22},
  Pages                    = {4724--4730},
  Volume                   = {78}
}

@Article{Cahill1967,
  Title                    = {The boundary of the geomagnetic field, {August} to {November}, 1961},
  Author                   = {Cahill, LJ and Patel, VL},
  Journal                  = {Planetary and Space Science},
  Year                     = {1967},
  Number                   = {6},
  Pages                    = {997--1033},
  Volume                   = {15}
}

@Article{Cahill1966,
  Title                    = {Inflation of the inner magnetosphere during a magnetic storm},
  Author                   = {Cahill, Laurence J},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1966},
  Number                   = {19},
  Pages                    = {4505--4519},
  Volume                   = {71}
}

@Article{Cahill1959,
  Title                    = {Investigation of the equatorial electrojet by rocket magnetometer},
  Author                   = {Cahill, Laurence J},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1959},
  Number                   = {5},
  Pages                    = {489--503},
  Volume                   = {64}
}

@Article{Cahill1963,
  Title                    = {The {Boundary} of the {Geomagnetic} {Field}},
  Author                   = {Cahill, L. J. and Amazeen, P. G.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1963},

  Month                    = apr,
  Pages                    = {1835--1843},
  Volume                   = {68},

  Abstract                 = {Not Available},
  Doi                      = {10.1029/JZ068i007p01835}
}

@Article{Cai2015,
  Title                    = {Cusp dynamics under northward IMF using three-dimensional global particle-in-cell simulations},
  Author                   = {Cai, Dongsheng and Esmaeili, Amin and Lemb{\`e}ge, Bertrand and Nishikawa, K-I},
  Journal                  = {Journal of Geophysical Research: Space Physics},
  Year                     = {2015},
  Number                   = {10},
  Pages                    = {8368--8386},
  Volume                   = {120},

  Owner                    = {suleimanbaraka},
  Publisher                = {Wiley Online Library},
  Timestamp                = {2016.02.21}
}

@InCollection{Cai2003,
  Title                    = {Parallel 3-D electromagnetic particle code using high performance FORTRAN: Parallel TRISTAN},
  Author                   = {Cai, Dongsheng and Li, Yaoting and Nishikawa, Ken-Ichi and Xiao, Chijie and Yan, Xiaoyang and Pu, Zuying},
  Booktitle                = {Space Plasma Simulation},
  Publisher                = {Springer},
  Year                     = {2003},
  Pages                    = {25--53},

  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.21}
}

@Article{Cai2006,
  Title                    = {Particle entry into the inner magnetosphere during duskward {IMF} {By}: {Global} three-dimensional electromagnetic full particle simulations},
  Author                   = {Cai, D and Yan, XY and Nishikawa, K-I and Lembège, Bertrand},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2006},
  Number                   = {12},
  Volume                   = {33}
}

@Article{Cai2006a,
  Title                    = {Particle entry into the inner magnetosphere during duskward {IMF} {B}$_{\textrm{y}}$: {Global} three-dimensional electromagnetic full particle simulations},
  Author                   = {Cai, D. and Yan, X. Y. and Nishikawa, K.-I. and Lembege, B.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {2006},

  Month                    = jun,
  Pages                    = {12101},
  Volume                   = {33},

  Abstract                 = {The change of the interplanetary magnetic field (IMF) direction from northward to duskward has an important impact on the inner magnetosphere. This impact is analyzed with the help of a new parallel version of the global three-dimensional full particle simulation code. For northward IMF, bands of weak magnetic field (sash) form poleward of the cusp at high latitudes in each hemisphere. These sashes move to the equator (within opposite quadrants) as the IMF rotates duskward and merge into one another to form the characteristic “Crosstail-S” within the neutral sheet of the magnetotail. These macroscopic magnetic patterns (sashes and Crosstail-S) evidenced herein are in a good agreement with results of previous 3D MHD simulations and experimental observations. Moreover, the analysis of particle fluxes shows that “sashes” and “Crosstail-S” act as magnetic groove to facilitate the entry and injection of magnetosheath particles into the inner magnetosphere. Injected particles are accelerated after the IMF changes its direction from northward to duskward.},
  Doi                      = {10.1029/2005GL023520},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers, Magnetospheric Physics: Magnetospheric configuration and dynamics, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Solar wind/magnetosphere interactions, Magnetospheric Physics: Substorms}
}

@Article{Cai2012,
  Title                    = {Characterization and correction of {Global} {Ozone} {Monitoring} {Experiment} 2 ultraviolet measurements and application to ozone profile retrievals},
  Author                   = {Cai, Zhaonan and Liu, Yi and Liu, Xiong and Chance, Kelly and Nowlan, Caroline R and Lang, Ruediger and Munro, Rosemary and Suleiman, Raid},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984–2012)},
  Year                     = {2012},
  Number                   = {D7},
  Volume                   = {117}
}

@InProceedings{Cairns2012,
  Title                    = {Dynamically important wave-particle interactions in solar wind - magnetosphere - ionosphere coupling: {A} review},
  Author                   = {Cairns, I.},
  Booktitle                = {39th {COSPAR} {Scientific} {Assembly}},
  Year                     = {2012},
  Month                    = jul,
  Pages                    = {272},
  Series                   = {{COSPAR} {Meeting}},
  Volume                   = {39}
}

@Article{Cairns1995,
  Title                    = {Unusual locations of {Earth}'s bow shock on {September} 24–25, 1987: {Mach} number effects},
  Author                   = {Cairns, Iver H and Fairfield, Donald H and Anderson, Roger R and Carlton, Victoria EH and Paularena, Karolen I and Lazarus, Alan J},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1995},
  Number                   = {A1},
  Pages                    = {47--62},
  Volume                   = {100}
}

@Article{Cairns1994,
  Title                    = {Towards an {MHD} theory for the standoff distance of {Earth}'s bow shock},
  Author                   = {Cairns, Iver H and Grabbe, Crockett L},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1994},
  Number                   = {25},
  Pages                    = {2781--2784},
  Volume                   = {21}
}

@Article{Calisesi2005,
  Title                    = {Regridding of remote soundings: {Formulation} and application to ozone profile comparison},
  Author                   = {Calisesi, Yasmine and Soebijanta, Vincent T. and van Oss, Roeland},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2005},
  Number                   = {D23},
  Volume                   = {110},

  Shorttitle               = {Regridding of remote soundings},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2005JD006122/full},
  Urldate                  = {2014-11-13}
}

@InCollection{Cannon2005,
  Title                    = {The effects of space weather on radio systems},
  Author                   = {Cannon, PS and Angling, MJ and Heaton, JAT and Rogers, NC and Shukla, AK},
  Booktitle                = {Effects of {Space} {Weather} on {Technology} {Infrastructure}},
  Publisher                = {Springer},
  Year                     = {2005},
  Pages                    = {185--201},

  Url                      = {http://link.springer.com/chapter/10.1007/1-4020-2754-0_10}
}

@Article{Carmichael2008,
  Title                    = {Predicting air quality: {Improvements} through advanced methods to integrate models and measurements},
  Author                   = {Carmichael, Gregory R and Sandu, Adrian and Chai, Tianfeng and Daescu, Dacian N and Constantinescu, Emil M and Tang, Youhua},
  Journal                  = {J. Comput. Phys.},
  Year                     = {2008},
  Number                   = {7},
  Pages                    = {3540--3571},
  Volume                   = {227}
}

@Article{Carpenter2002,
  Title                    = {Small-scale field-aligned plasmaspheric density structures inferred from the {Radio} {Plasma} {Imager} on {IMAGE}},
  Author                   = {Carpenter, Don L. and Spasojević, M. A. and Bell, Timothy F. and Inan, Umran S. and Reinisch, Bodo W. and Galkin, I. A. and Benson, Robert F. and Green, J. L. and Fung, Shing F. and Boardsen, S. A.},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2002},
  Number                   = {A9},
  Pages                    = {SMP--22},
  Volume                   = {107},

  File                     = {[HTML] from wiley.com:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/9AET6SRK/full.html:text/html},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2001JA009199/full},
  Urldate                  = {2015-12-09}
}

@Article{Cattell2003,
  Title                    = {Large amplitude solitary waves in and near the {Earth}? s magnetosphere, magnetopause and bow shock: {Polar} and {Cluster} observations},
  Author                   = {Cattell, C and Neiman, C and Dombeck, J and Crumley, J and Wygant, J and Kletzing, CA and Peterson, WK and Mozer, FS and André, Mats and {others}},
  Journal                  = {Nonlinear Processes in Geophysics},
  Year                     = {2003},
  Number                   = {1/2},
  Pages                    = {13--26},
  Volume                   = {10}
}

@Misc{CHNM,
  Title                    = {Zotero {Quick} {Start} {Guide}},

  Author                   = {{Center for History and New Media}},

  Annote                   = {Welcome to Zotero!View the Quick Start Guide to learn how to begin collecting, managing, citing, and sharing your research sources.Thanks for installing Zotero.},
  Url                      = {http://zotero.org/support/quick_start_guide}
}

@Book{CHNMa,
  Title                    = {Zotero {Quick} {Start} {Guide}},
  Author                   = {{Center for History and New Media}},

  Annote                   = {Welcome to Zotero!View the Quick Start Guide to learn how to begin collecting, managing, citing, and sharing your research sources.Thanks for installing Zotero.},
  Url                      = {http://zotero.org/support/quick_start_guide}
}

@Book{CHNMb,
  Title                    = {Zotero {Quick} {Start} {Guide}},
  Author                   = {{Center for History and New Media}},

  Annote                   = {Welcome to Zotero!View the Quick Start Guide to learn how to begin collecting, managing, citing, and sharing your research sources.Thanks for installing Zotero.},
  Url                      = {http://zotero.org/support/quick_start_guide}
}

@Article{Cerruti2008,
  Title                    = {Effect of intense {December} 2006 solar radio bursts on {GPS} receivers},
  Author                   = {Cerruti, Alessandro P and Kintner, Paul M and Gary, Dale E and Mannucci, Anthony J and Meyer, Robert F and Doherty, Patricia and Coster, Anthea J},
  Journal                  = {Space Weather},
  Year                     = {2008},
  Number                   = {10},
  Volume                   = {6}
}

@InCollection{Chance2006,
  Title                    = {Spectroscopic measurements of tropospheric composition from satellite measurements in the ultraviolet and visible: steps toward continuous pollution monitoring from space},
  Author                   = {Chance, Kelly},
  Booktitle                = {Remote {Sensing} of the {Atmosphere} for {Environmental} {Security}},
  Publisher                = {Springer},
  Year                     = {2006},
  Pages                    = {1--25},

  Shorttitle               = {Spectroscopic measurements of tropospheric composition from satellite measurements in the ultraviolet and visible},
  Url                      = {http://link.springer.com/chapter/10.1007/978-1-4020-5090-9_1},
  Urldate                  = {2014-11-13}
}

@Article{Chance2002,
  Title                    = {{OMI} algorithm theoretical basis document, volume {IV}: {OMI} trace gas algorithms},
  Author                   = {Chance, K.},
  Journal                  = {Accessed on},
  Year                     = {2002},
  Number                   = {10},
  Pages                    = {2009},
  Volume                   = {12},

  Shorttitle               = {{OMI} algorithm theoretical basis document, volume {IV}}
}

@Article{Chance1998,
  Title                    = {Analysis of {BrO} measurements from the global ozone monitoring experiment},
  Author                   = {Chance, Kelly},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1998},
  Number                   = {17},
  Pages                    = {3335--3338},
  Volume                   = {25},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/98GL52359/full},
  Urldate                  = {2014-11-13}
}

@Article{Chance2005,
  Title                    = {Undersampling correction for array detector-based satellite spectrometers},
  Author                   = {Chance, Kelly and Kurosu, Thomas P. and Sioris, Christopher E.},
  Journal                  = {Appl. Opt.},
  Year                     = {2005},
  Number                   = {7},
  Pages                    = {1296--1304},
  Volume                   = {44},

  Url                      = {http://www.opticsinfobase.org/abstract.cfm?uri=AO-44-7-1296},
  Urldate                  = {2014-11-13}
}

@InProceedings{Chance2013,
  Title                    = {Tropospheric emissions: monitoring of pollution ({TEMPO})},
  Author                   = {Chance, Kelly and Liu, Xiong and Suleiman, Raid M and Flittner, David E and Al-Saadi, Jassim and Janz, Scott J},
  Booktitle                = {{SPIE} {Optical} {Engineering}+ {Applications}},
  Year                     = {2013},
  Pages                    = {88660D--88660D},
  Publisher                = {International Society for Optics and Photonics}
}

@Article{Chance2000,
  Title                    = {Satellite observations of formaldehyde over {North} {America} from {GOME}},
  Author                   = {Chance, Kelly and Palmer, Paul I. and Spurr, Robert JD and Martin, Randall V. and Kurosu, Thomas P. and Jacob, Daniel J.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2000},
  Number                   = {21},
  Pages                    = {3461--3464},
  Volume                   = {27},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2000GL011857/full},
  Urldate                  = {2014-11-13}
}

@InProceedings{Chance1991,
  Title                    = {Retrieval and molecule sensitivity studies for the global ozone monitoring experiment and the scanning imaging absorption spectrometer for atmospheric chartography},
  Author                   = {Chance, Kelly V. and Burrows, John P. and Schneider, Wolfgang},
  Booktitle                = {Orlando'91, {Orlando}, {FL}},
  Year                     = {1991},
  Pages                    = {151--165},
  Publisher                = {International Society for Optics and Photonics},

  Url                      = {http://proceedings.spiedigitallibrary.org/proceeding.aspx?articleid=965179},
  Urldate                  = {2014-11-13}
}

@Article{Chandler1991,
  Title                    = {Observations of polar ion outflows},
  Author                   = {Chandler, MO},
  Journal                  = {J. Geophys. {\textbackslash}ldots},
  Year                     = {1991},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/90JA02180/full}
}

@Article{Chandran2011,
  Title                    = {Incorporating {Kinetic} {Physics} into a {Two}-fluid {Solar}-wind {Model} with {Temperature} {Anisotropy} and {Low}-frequency {Alfvén}-wave {Turbulence}},
  Author                   = {Chandran, B. D. G. and Dennis, T. J. and Quataert, E. and Bale, S. D.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2011},

  Month                    = dec,
  Pages                    = {197},
  Volume                   = {743},

  Doi                      = {10.1088/0004-637X/743/2/197},
  Keywords                 = {Solar Wind, Sun: corona, turbulence, waves}
}

@Article{Chang2000,
  Title                    = {Energetic magnetosheath ions connected to the {Earth}'s bow shock: {Possible} source of cusp energetic ions},
  Author                   = {Chang, S-W and Scudder, JD and Fennell, JF and Friedel, R and Lepping, RP and Russell, CT and Trattner, KJ and Fuselier, SA and Peterson, WK and Spence, Harlan E},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2000},
  Number                   = {A3},
  Pages                    = {5471--5488},
  Volume                   = {105}
}

@Article{Chang1998,
  Title                    = {Cusp energetic ions: {A} bow shock source},
  Author                   = {Chang, S-W and Scudder, JD and Fuselier, SA and Fennell, JF and Trattner, KJ and Pickett, JS and Spence, Harlan E and Menietti, JD and Peterson, WK and Lepping, RP and {others}},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1998},
  Number                   = {19},
  Pages                    = {3729--3732},
  Volume                   = {25}
}

@Article{Chang1986,
  Title                    = {Transverse acceleration of oxygen ions by electromagnetic ion cyclotron resonance with broad band left‚Äö√Ñ√∂‚àö√ë‚àö‚Ñ¢hand polarized waves},
  Author                   = {Chang, T and Crew, GB},
  Journal                  = {Geophys. {\textbackslash}ldots},
  Year                     = {1986},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/GL013i007p00636/full}
}

@Article{Chang1986a,
  Title                    = {Transverse acceleration of oxygen ions by electromagnetic ion cyclotron resonance with broad band left-hand polarized waves},
  Author                   = {Chang, T. and Crew, G. B. and Hershkowitz, N. and Jasperse, J. R. and Retterer, J. M.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {1986},

  Month                    = jul,
  Pages                    = {636--639},
  Volume                   = {13},

  Doi                      = {10.1029/GL013i007p00636},
  Keywords                 = {Broadband, Cyclotron Resonance, Electric Fields, Ion Accelerators, Ion Cyclotron Radiation, Oxygen Ions, Particle Acceleration, Plasma Layers, Polarized Electromagnetic Radiation}
}

@Article{Chang1986b,
  Title                    = {Transverse acceleration of oxygen ions by electromagnetic ion cyclotron resonance with broad band left-hand polarized waves},
  Author                   = {Chang, T. and Crew, G. B. and Hershkowitz, N. and Jasperse, J. R. and Retterer, J. M.},
  Journal                  = {{\textbackslash}textbackslashgrl},
  Year                     = {1986},

  Month                    = jul,
  Pages                    = {636--639},
  Volume                   = {13},

  Doi                      = {10.1029/GL013i007p00636},
  Keywords                 = {Broadband, Cyclotron Resonance, Electric Fields, Ion Accelerators, Ion Cyclotron Radiation, Oxygen Ions, Particle Acceleration, Plasma Layers, Polarized Electromagnetic Radiation}
}

@InProceedings{Chao2002,
  Title                    = {Models for the size and shape of the {Earth}'s magnetopause and bow shock},
  Author                   = {Chao, JK and Wu, DJ and Lin, C-H and Yang, Y-H and Wang, XY and Kessel, M and Chen, SH and Lepping, RP},
  Booktitle                = {Cospar {Colloquia} series},
  Year                     = {2002},
  Pages                    = {127--135},
  Publisher                = {Elsevier},
  Volume                   = {12}
}

@Article{Chapman2004,
  Title                    = {{MHD} simulations of {Earth}'s bow shock: {Interplanetary} magnetic field orientation effects on shape and position},
  Author                   = {Chapman, JF and Cairns, Iver H and Lyon, JG and Boshuizen, Christopher R},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2004},
  Number                   = {A4},
  Volume                   = {109}
}

@Article{Chapman1932,
  Title                    = {The {Lunar} {Diurnal} {Variation} of {Atmospheric} {Temperature} at {Batavia}, 1866-1928},
  Author                   = {Chapman, S.},
  Journal                  = {Royal Society of London Proceedings Series A},
  Year                     = {1932},

  Month                    = jul,
  Pages                    = {1--24},
  Volume                   = {137},

  Doi                      = {10.1098/rspa.1932.0117}
}

@Article{Chapman1932a,
  Title                    = {The influence of a solar eclipse upon upper atmospheric ionization},
  Author                   = {Chapman, S.},
  Journal                  = {{\textbackslash}mnras},
  Year                     = {1932},

  Month                    = mar,
  Pages                    = {413},
  Volume                   = {92}
}

@Article{Chapman1930,
  Title                    = {On {Solar} {Ultra}-{Violet} {Radiation} as the {Cause} of {Aurora} and {Magnetic} {Storms}.},
  Author                   = {Chapman, S.},
  Journal                  = {Geophysical Journal},
  Year                     = {1930},

  Month                    = apr,
  Pages                    = {296--300},
  Volume                   = {2},

  Doi                      = {10.1111/j.1365-246X.1930.tb05414.x}
}

@Article{Chapman1929,
  Title                    = {Solar streams of corpuscles: their geometry, absorption of light, and penetration},
  Author                   = {Chapman, S.},
  Journal                  = {{\textbackslash}mnras},
  Year                     = {1929},

  Month                    = mar,
  Pages                    = {456},
  Volume                   = {89}
}

@Article{Chapman1930a,
  Title                    = {A new theory of magnetic storms},
  Author                   = {Chapman, Sidney and Ferraro, Vincent CA},
  Journal                  = {Nature},
  Year                     = {1930},
  Number                   = {3169},
  Pages                    = {129--130},
  Volume                   = {126},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.22}
}

@Article{Chapman1930b,
  Title                    = {A {New} {Theory} of {Magnetic} {Storms}.},
  Author                   = {Chapman, S. and Ferraro, V. C. A.},
  Journal                  = {{\textbackslash}nat},
  Year                     = {1930},

  Month                    = jul,
  Pages                    = {129--130},
  Volume                   = {126},

  Abstract                 = {AN attempt to infer the course of events when a neutral ionised stream of particles from the sun is directed towards the earth has now led to results which we believe indicate how magnetic storms are produced. A full discussion of the phenomena involves the solution of numerous intricate mathematical problems, many of which have not yet been attacked in detail; but it seems possible to outline the main sequence of events.},
  Doi                      = {10.1038/126129a0}
}

@Article{Chapman1929a,
  Title                    = {The electrical state of solar streams of corpuscles},
  Author                   = {Chapman, S. and Ferraro, V. C. A.},
  Journal                  = {{\textbackslash}mnras},
  Year                     = {1929},

  Month                    = mar,
  Pages                    = {470},
  Volume                   = {89}
}

@Article{Chappell1988,
  Title                    = {The terrestrial plasma source - {A} new perspective in solar-terrestrial processes from {Dynamics} {Explorer}},
  Author                   = {Chappell, C. R.},
  Journal                  = {Reviews of Geophysics},
  Year                     = {1988},

  Month                    = may,
  Pages                    = {229--248},
  Volume                   = {26},

  Doi                      = {10.1029/RG026i002p00229},
  Keywords                 = {Auroral Zones, Dynamics Explorer Satellites, Magnetosphere-Ionosphere Coupling, Polar Caps, Solar Terrestrial Interactions, Solar Wind, Space Plasmas}
}

@Article{Chappell1988a,
  Title                    = {The terrestrial plasma source - {A} new perspective in solar-terrestrial processes from {Dynamics} {Explorer}},
  Author                   = {Chappell, C. R.},
  Journal                  = {Reviews of Geophysics},
  Year                     = {1988},

  Month                    = may,
  Pages                    = {229--248},
  Volume                   = {26},

  Doi                      = {10.1029/RG026i002p00229},
  Keywords                 = {Auroral Zones, Dynamics Explorer Satellites, Magnetosphere-Ionosphere Coupling, Polar Caps, Solar Terrestrial Interactions, Solar Wind, Space Plasmas}
}

@Article{Chaston2004,
  Title                    = {Auroral ion acceleration in dispersive {Alfvén} waves},
  Author                   = {Chaston, C. C. and Bonnell, J. W. and Carlson, C. W. and McFadden, J. P. and Ergun, R. E. and Strangeway, R. J. and Lund, E. J.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = apr,
  Pages                    = {4205},
  Volume                   = {109},

  Doi                      = {10.1029/2003JA010053},
  Keywords                 = {Alfvén waves, aurora, ion acceleration, ion heating, Ionosphere: Ionosphere/magnetosphere interactions (2736), Ionosphere: Particle acceleration, Ionosphere: Wave/particle interactions, ionospheric Alfvén resonator, kinetic effects, Magnetospheric Physics: Auroral phenomena (2407), Magnetospheric Physics: Magnetosphere interactions with satellites and rings}
}

@Article{Chaston2004a,
  Title                    = {Auroral ion acceleration in dispersive {Alfv}√©n waves},
  Author                   = {Chaston, C. C. and Bonnell, J. W. and Carlson, C. W. and McFadden, J. P. and Ergun, R. E. and Strangeway, R. J. and Lund, E. J.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = apr,
  Pages                    = {4205},
  Volume                   = {109},

  Doi                      = {10.1029/2003JA010053},
  Keywords                 = {Alfv√©n waves, aurora, ion acceleration, ion heating, Ionosphere: Ionosphere/magnetosphere interactions (2736), Ionosphere: Particle acceleration, Ionosphere: Wave/particle interactions, ionospheric Alfv√©n resonator, kinetic effects, Magnetospheric Physics: Auroral phenomena (2407), Magnetospheric Physics: Magnetosphere interactions with satellites and rings}
}

@Article{Che2014,
  Title                    = {the {Origin} of {Non}-{Maxwellian} {Solar} {Wind} {Electron} {Velocity} {Distribution} {Function}: {Connection} {To} {Nanoflares} in the {Solar} {Corona}},
  Author                   = {Che, H. and Goldstein, M. L.},
  Journal                  = {Astrophys. J.},
  Year                     = {2014},
  Number                   = {2},
  Pages                    = {L38},
  Volume                   = {795},

  Doi                      = {10.1088/2041-8205/795/2/L38},
  ISSN                     = {2041-8213},
  Keywords                 = {acceleration of particles, color figure, corona, instabilities, online-only material, scattering, Solar Wind, sun, turbulence},
  Url                      = {http://stacks.iop.org/2041-8205/795/i=2/a=L38?key=crossref.a370b5e1ab245f2584f3367e17bdb74a}
}

@Book{Chen1984,
  Title                    = {Introduction to plasma physics and controlled fusion},
  Author                   = {Chen, Francis F. and Chen, Francis F.},
  Publisher                = {Plenum Press},
  Year                     = {1984},

  Address                  = {New York},
  Edition                  = {2nd ed},

  Annote                   = {Rev. ed. of: Introduction to plasma physics. 1974 Includes index},
  ISBN                     = {0-306-41332-9},
  Keywords                 = {Plasma (Ionized gases)}
}

@Article{Chen1993,
  Title                    = {Anomalous aspects of magnetosheath flow and of the shape and oscillations of the magnetopause during an interval of strongly northward interplanetary magnetic field},
  Author                   = {Chen, Sheng-Hsien and Kivelson, Margaret G and Gosling, Jack T and Walker, Raymond J and Lazarus, Allan J},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1993},
  Number                   = {A4},
  Pages                    = {5727--5742},
  Volume                   = {98},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/92JA02263/full}
}

@Article{Chen2003,
  Title                    = {Formation of {Minor}-{Ion} {Charge} {States} in the {Fast} {Solar} {Wind}: {Roles} of {Differential} {Flow} {Speeds} of {Ions} of the {Same} {Element}},
  Author                   = {Chen, Y. and Esser, R. and Hu, Y.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2003},

  Month                    = jan,
  Pages                    = {467--474},
  Volume                   = {582},

  Doi                      = {10.1086/344642},
  Keywords                 = {Atomic Processes, Magnetohydrodynamics: MHD, Sun: corona, Sun: solar wind}
}

@Article{Chen2002,
  Title                    = {A theoretical model for {O}$^{\textrm{5+\$}}$ ({O}$^{\textrm{7+\$}}$) ions in the fast solar wind},
  Author                   = {Chen, Y. and Esser, R. and Hu, Y. Q.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2002},

  Month                    = nov,
  Pages                    = {1368},
  Volume                   = {107},

  Doi                      = {10.1029/2002JA009341},
  Keywords                 = {and Astronomy: Coronal holes, and Astronomy: General or miscellaneous, ASTROPHYSICS, Interplanetary Physics: Solar wind plasma, Solar Physics, Space Plasma Physics: Ionization processes, Space Plasma Physics: Numerical simulation studies}
}

@Article{Chisham2000,
  Title                    = {Multisatellite observations of large magnetic depressions in the solar wind},
  Author                   = {Chisham, G and Schwartz, SJ and Burgess, D and Bale, SD and Dunlop, MW and Russell, CT},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2000},
  Number                   = {A2},
  Pages                    = {2325--2335},
  Volume                   = {105}
}

@Article{Choi2011,
  Title                    = {Analysis of {GEO} spacecraft anomalies: {Space} weather relationships},
  Author                   = {Choi, Ho-Sung and Lee, Jaejin and Cho, Kyung-Suk and Kwak, Young-Sil and Cho, Il-Hyun and Park, Young-Deuk and Kim, Yeon-Han and Baker, Daniel N and Reeves, Geoffrey D and Lee, Dong-Kyu},
  Journal                  = {Space Weather},
  Year                     = {2011},
  Number                   = {6},
  Volume                   = {9}
}

@Article{Christensen2009,
  Title                    = {Energy flux determines magnetic field strength of planets and stars},
  Author                   = {Christensen, U. R. and Holzwarth, V. and Reiners, A.},
  Journal                  = {{\textbackslash}textbackslashnat},
  Year                     = {2009},

  Month                    = jan,
  Pages                    = {167--169},
  Volume                   = {457},

  Doi                      = {10.1038/nature07626}
}

@Article{Chuang2011,
  Title                    = {General formulation for acoustic solitons in three-component nonthermal plasmas},
  Author                   = {Chuang, S-H and Hau, L-N},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2011},
  Number                   = {6},
  Pages                    = {063702},
  Volume                   = {18}
}

@Article{Clarke2002,
  Title                    = {Ultraviolet emissions from the magnetic footprints of {Io}, {Ganymede} and {Europa} on {Jupiter}},
  Author                   = {Clarke, J. T. and Ajello, J. and Ballester, G. and Ben Jaffel, L. and Connerney, J. and G√©rard, J.-C. and Gladstone, G. R. and Grodent, D. and Pryor, W. and Trauger, J. and Waite, J. H.},
  Journal                  = {{\textbackslash}textbackslashnat},
  Year                     = {2002},

  Month                    = feb,
  Pages                    = {997--1000},
  Volume                   = {415}
}

@Article{Cliver2006,
  Title                    = {The 1859 space weather event: {Then} and now},
  Author                   = {Cliver, EW},
  Journal                  = {Advances in Space Research},
  Year                     = {2006},
  Number                   = {2},
  Pages                    = {119--129},
  Volume                   = {38},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S0273117705010215}
}

@Article{Cohen2011,
  Title                    = {The {Dynamics} of {Stellar} {Coronae} {Harboring} {Hot} {Jupiters}. {I}. {A} {Time}-dependent {Magnetohydrodynamic} {Simulation} of the {Interplanetary} {Environment} in the {HD} 189733 {Planetary} {System}},
  Author                   = {Cohen, O. and Kashyap, V. L. and Drake, J. J. and Sokolov, I. V. and Garraffo, C. and Gombosi, T. I.},
  Journal                  = {{\textbackslash}textbackslashapj},
  Year                     = {2011},

  Month                    = may,
  Pages                    = {67},
  Volume                   = {733},

  Doi                      = {10.1088/0004-637X/733/1/67},
  Keywords                 = {planet-star interactions, stars: coronae, stars: magnetic field}
}

@Article{Colak2009,
  Title                    = {Automated {Solar} {Activity} {Prediction}: {A} hybrid computer platform using machine learning and solar imaging for automated prediction of solar flares},
  Author                   = {Colak, T and Qahwaji, R},
  Journal                  = {Space Weather},
  Year                     = {2009},
  Number                   = {6},
  Volume                   = {7}
}

@Article{Cole1976,
  Title                    = {Effects of crossed magnetic and /spatially dependent/ electric fields on charged particle motion},
  Author                   = {Cole, K. D.},
  Journal                  = {{\textbackslash}textbackslashplanss},
  Year                     = {1976},

  Month                    = may,
  Pages                    = {515--518},
  Volume                   = {24},

  Doi                      = {10.1016/0032-0633(76)90096-9},
  Keywords                 = {Charged Particles, Earth Magnetosphere, Electric Fields, Gyration, Gyrofrequency, Magnetic Effects, Particle Acceleration, Particle Motion, Plasma-Particle Interactions, Spatial Dependencies}
}

@Article{Cole1976a,
  Title                    = {Effects of crossed magnetic and /spatially dependent/ electric fields on charged particle motion},
  Author                   = {Cole, K. D.},
  Journal                  = {{\textbackslash}planss},
  Year                     = {1976},

  Month                    = may,
  Pages                    = {515--518},
  Volume                   = {24},

  Doi                      = {10.1016/0032-0633(76)90096-9},
  Keywords                 = {Charged Particles, Earth Magnetosphere, Electric Fields, Gyration, Gyrofrequency, Magnetic Effects, Particle Acceleration, Particle Motion, Plasma-Particle Interactions, Spatial Dependencies}
}

@Article{Collier1996,
  Title                    = {Neon-20, oxygen-16, and helium-4 densities, temperatures, and suprathermal tails in the solar wind determined with {WIND}/{MASS}},
  Author                   = {Collier, M. R. and Hamilton, D. C. and Gloeckler, G. and Bochsler, P. and Sheldon, R. B.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {1996},
  Pages                    = {1191--1194},
  Volume                   = {23},

  Doi                      = {10.1029/96GL00621},
  Keywords                 = {Interplanetary Physics: Solar wind plasma}
}

@Article{Collier2012,
  Title                    = {Prototyping a global soft {X}-ray imaging instrument for heliophysics, planetary science, and astrophysics science},
  Author                   = {Collier, M. R. and Porter, F. S. and Sibeck, D. G. and Carter, J. A. and Chiao, M. P. and Chornay, D. J. and Cravens, T. and Galeazzi, M. and Keller, J. W. and Koutroumpa, D. and Kuntz, K. and Read, A. M. and Robertson, I. P. and Sembay, S. and Snowden, S. and Thomas, N.},
  Journal                  = {Astronomische Nachrichten},
  Year                     = {2012},
  Pages                    = {378},
  Volume                   = {333},

  Abstract                 = {We describe current progress in the development of a prototype wide field-of-view soft X-ray imager that employs Lobster-eye optics and targets heliophysics, planetary, and astrophysics science. The prototype will provide proof-of-concept for a future flight instrument capable of imaging the entire dayside magnetosheath from outside the magnetosphere. Such an instrument was proposed for the ESA AXIOM mission.},
  ISSN                     = {0004-6337},
  Keywords                 = {interplanetary medium solar-terrestrial relations solar wind X-rays: diffuse background},
  Url                      = {http://adsabs.harvard.edu/abs/2012AN....333..378C}
}

@Article{Collier2014,
  Title                    = {On lunar exospheric column densities and solar wind access beyond the terminator from {ROSAT} soft {X}-ray observations of solar wind charge exchange},
  Author                   = {Collier, Michael R. and Snowden, S. L. and Sarantos, M. and Benna, M. and Carter, J. A. and Cravens, T. E. and Farrell, W. M. and Fatemi, S. and Hills, H. Kent and Hodges, R. R. and Holmström, M. and Kuntz, K. D. and Porter, F. Scott and Read, A. and Robertson, I. P. and Sembay, S. F. and Sibeck, D. G. and Stubbs, T. J. and Travnicek, P. and Walsh, B. M.},
  Journal                  = {Journal of Geophysical Research (Planets)},
  Year                     = {2014},
  Pages                    = {1459--1478},
  Volume                   = {119},

  Abstract                 = {We analyze the Röntgen satellite (ROSAT) position sensitive proportional counter soft X-ray image of the Moon taken on 29 June 1990 by examining the radial profile of the surface brightness in three wedges: two 19° wedges (one north and one south) 13-32° off the terminator toward the dark side and one wedge 38° wide centered on the antisolar direction. The radial profiles of both the north and the south wedges show significant limb brightening that is absent in the 38° wide antisolar wedge. An analysis of the soft X-ray intensity increase associated with the limb brightening shows that its magnitude is consistent with that expected due to solar wind charge exchange (SWCX) with the tenuous lunar atmosphere based on lunar exospheric models and hybrid simulation results of solar wind access beyond the terminator. Soft X-ray imaging thus can independently infer the total lunar limb column density including all species, a property that before now has not been measured, and provide a large-scale picture of the solar wind-lunar interaction. Because the SWCX signal appears to be dominated by exospheric species arising from solar wind implantation, this technique can also determine how the exosphere varies with solar wind conditions. Now, along with Mars, Venus, and Earth, the Moon represents another solar system body at which SWCX has been observed.},
  ISSN                     = {0148-0227},
  Keywords                 = {SWCX ROSAT PSPC Moon HPC2N},
  Url                      = {http://adsabs.harvard.edu/abs/2014JGRE..119.1459C}
}

@Article{Collinson2012,
  Title                    = {Hot flow anomalies at {Venus}},
  Author                   = {Collinson, G. A. and Sibeck, D. G. and Masters, A. and Shane, N. and Slavin, J. A. and Coates, A. J. and Zhang, T. L. and Sarantos, M. and Boardsen, S. and Moore, T. E. and Barabash, S.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2012},
  Pages                    = {4204},
  Volume                   = {117},

  Abstract                 = {We present a multi-instrument study of a hot flow anomaly (HFA) observed by the Venus Express spacecraft in the Venusian foreshock, on 22 March 2008, incorporating both Venus Express Magnetometer and Analyzer of Space Plasmas and Energetic Atoms (ASPERA) plasma observations. Centered on an interplanetary magnetic field discontinuity with inward convective motional electric fields on both sides, with a decreased core field strength, ion observations consistent with a flow deflection, and bounded by compressive heated edges, the properties of this event are consistent with those of HFAs observed at other planets within the solar system.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Planetary bow shocks Magnetospheric Physics: Planetary magnetospheres (5443 5737 6033) Magnetospheric Physics: Solar wind interactions with unmagnetized bodies Planetary Sciences: Solid Surface Planets: Interactions with particles and fields Planetary Sciences: Solar System Objects: Venus},
  Url                      = {http://adsabs.harvard.edu/abs/2012JGRA..117.4204C}
}

@Article{Collinson2014,
  Title                    = {{A survey of hot flow anomalies at Venus}},
  Author                   = {Collinson, G. A. and Sibeck, D. G. and Masters, A. and Shane, N. and Zhang, T. L. and Fedorov, A. and Barabash, S. and Coates, A. J. and Moore, T. E. and Slavin, J. A. and Uritsky, V. M. and Boardsen, S. and Sarantos, M.},
  Journal                  = {J. Geophys. Res. A Sp. Phys.},
  Year                     = {2014},
  Number                   = {2},
  Pages                    = {978--991},
  Volume                   = {119},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {We present a multi-instrument study of a hot flow anomaly (HFA) observed by the Venus Express spacecraft in the Venusian foreshock, on 22 March 2008, incorporating both Venus Express Magnetometer and Analyzer of Space Plasmas and Energetic Atoms (ASPERA) plasma observations. Centered on an interplanetary magnetic field discontinuity with inward convective motional electric fields on both sides, with a decreased core field strength, ion observations consistent with a flow deflection, and bounded by compressive heated edges, the properties of this event are consistent with those of HFAs observed at other planets within the solar system.},
  Doi                      = {10.1002/2013JA018863},
  ISBN                     = {0148-0227},
  ISSN                     = {21699402},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Collinson2014a,
  Title                    = {A survey of hot flow anomalies at {Venus}},
  Author                   = {Collinson, G. A. and Sibeck, D. G. and Masters, A. and Shane, N. and Zhang, T. L. and Fedorov, A. and Barabash, S. and Coates, A. J. and Moore, T. E. and Slavin, J. A. and Uritsky, V. M. and Boardsen, S. and Sarantos, M.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2014},
  Pages                    = {978--991},
  Volume                   = {119},

  Abstract                 = {We present the first survey of hot flow anomalies (HFAs) at the bow shock of Venus, expanding on our recent initial case study. A 3.06 sol (774 Earth day) survey of Venus Express magnetometer, ion spectrometer, and electron spectrometer data was undertaken in order to identify Cytherian HFAs. Seven events were discovered, corresponding to a statistical frequency ≈1.2±0.8 per day, approximately the same rate as at the Earth. All seven HFAs were centered on a discontinuity in the solar wind, with inward pointing motional electric fields on at least one side, and exhibited electron and ion perturbations consistent with heating. For one event the calculation of continuous electron moments is possible, revealing that electron temperature increased from ≈2×10{\textless}SUP{\textgreater}5{\textless}/SUP{\textgreater} K to 8×10{\textless}SUP{\textgreater}5{\textless}/SUP{\textgreater} K in the HFA core (comparable to terrestrial and Kronian HFA observations), and density increased from ≈1 cm{\textless}SUP{\textgreater}-3{\textless}/SUP{\textgreater} to 2→2.5 cm{\textless}SUP{\textgreater}-3{\textless}/SUP{\textgreater} in the bounding compression regions. Cytherian HFAs were found to be physically smaller (0.4→1.7 Venus radii (R{\textless}SUB{\textgreater}V{\textless}/SUB{\textgreater})) than their terrestrial or Kronian counterparts, although are much larger when compared to the overall size of the system (≈130\% of the subsolar bow shock distance), and occur very close (1.5→3.0R{\textless}SUB{\textgreater}V{\textless}/SUB{\textgreater}) to the planet. Thus, we hypothesize that HFAs have a much more dominant role in the dynamics of the induced magnetosphere of Venus relative to the magnetospheres of magnetized planets.},
  ISSN                     = {0148-0227},
  Keywords                 = {Venus hot flow anomaly bow shock Venus Express},
  Url                      = {http://adsabs.harvard.edu/abs/2014JGRA..119..978C}
}

@Article{Collinson2012a,
  Title                    = {Short large-amplitude magnetic structures ({SLAMS}) at {Venus}},
  Author                   = {Collinson, G. A. and Wilson, L. B., III and Sibeck, D. G. and Shane, N. and Zhang, T. L. and Moore, T. E. and Coates, A. J. and Barabash, S.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2012},
  Pages                    = {10221},
  Volume                   = {117},

  Abstract                 = {We present the first observation of magnetic fluctuations consistent with short large-amplitude magnetic structures (SLAMS) in the foreshock of the planet Venus. Three monolithic magnetic field spikes were observed by the Venus Express on 11 April 2009. The structures were ˜1.5-11 s in duration, had magnetic compression ratios between ˜3 and 6, and exhibited elliptical polarization. These characteristics are consistent with the SLAMS observed at Earth, Jupiter, and Comet Giacobini-Zinner, and thus we hypothesize that it is possible SLAMS may be found at any celestial body with a foreshock.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Planetary bow shocks Magnetospheric Physics: Plasma waves and instabilities (2471) Magnetospheric Physics: Solar wind interactions with unmagnetized bodies Planetary Sciences: Solar System Objects: Extra-solar planets Space Plasma Physics: Wave/wave interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2012JGRA..11710221C}
}

@InCollection{Cornilleau-Wehrlin1997,
  Title                    = {The {Cluster} spatio-temporal analysis of field fluctuations ({STAFF}) experiment},
  Author                   = {Cornilleau-Wehrlin, Nicole and Chauveau, P and Louis, S and Meyer, A and Nappa, JM and Perraut, S and Rezeau, L and Robert, P and Roux, A and De Villedary, C and {others}},
  Booktitle                = {The {Cluster} and {Phoenix} {Missions}},
  Publisher                = {Springer},
  Year                     = {1997},
  Pages                    = {107--136}
}

@Article{Crank1947,
  Title                    = {A practical method for numerical evaluation of solutions of partial differential equations of the heat-conduction type},
  Author                   = {Crank, John and Nicolson, Phyllis},
  Journal                  = {P. Camb. Philos. Soc.},
  Year                     = {1947},
  Pages                    = {50--64},
  Volume                   = {43}
}

@Article{Cranmer2009,
  Title                    = {Coronal {Holes}},
  Author                   = {Cranmer, S. R.},
  Journal                  = {Living Reviews in Solar Physics},
  Year                     = {2009},

  Month                    = sep,
  Pages                    = {3},
  Volume                   = {6},

  Doi                      = {10.12942/lrsp-2009-3},
  Keywords                 = {Alfven waves, corona, Coronal heating, Coronal holes, Cyclotron Resonance, Kinetic and MHD theory, Magnetohydrodynamics, Magnetohydrodynamic waves, Plasma heating, Solar cycle, Solar Wind, Solar wind plasma, Solar wind turbulence, Space Plasmas, Stellar winds, sun, turbulence, UV radiation, Wave-particle interactions, Waves and instabilities}
}

@Article{Cranmer2002,
  Title                    = {Coronal {Holes} and the {High}-{Speed} {Solar} {Wind}},
  Author                   = {Cranmer, S. R.},
  Journal                  = {ßr},
  Year                     = {2002},

  Month                    = aug,
  Pages                    = {229--294},
  Volume                   = {101}
}

@Article{Cranmer2007,
  Title                    = {Self-consistent {Coronal} {Heating} and {Solar} {Wind} {Acceleration} from {Anisotropic} {Magnetohydrodynamic} {Turbulence}},
  Author                   = {Cranmer, S. R. and van Ballegooijen, A. A. and Edgar, R. J.},
  Journal                  = {{\textbackslash}apjs},
  Year                     = {2007},

  Month                    = aug,
  Pages                    = {520--551},
  Volume                   = {171},

  Doi                      = {10.1086/518001},
  Keywords                 = {Magnetohydrodynamics: MHD, Sun: Atmospheric Motions, Sun: corona, Sun: solar wind, turbulence, waves}
}

@Article{Cranmer1999,
  Title                    = {Spectroscopic {Constraints} on {Models} of {Ion} {Cyclotron} {Resonance} {Heating} in the {Polar} {Solar} {Corona} and {High}-{Speed} {Solar} {Wind}},
  Author                   = {Cranmer, S. R. and Field, G. B. and Kohl, J. L.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {1999},

  Month                    = jun,
  Pages                    = {937--947},
  Volume                   = {518},

  Doi                      = {10.1086/307330},
  Keywords                 = {Line: Profiles, plasmas, Sun: corona, Sun: solar wind, Sun: UV Radiation, waves}
}

@Article{Cravens2004,
  Title                    = {Physics of solar system plasmas},
  Author                   = {Cravens, Thomas E},
  Journal                  = {Physics of Solar System Plasmas, by Thomas E. Cravens, pp. 495. ISBN 0521611946. Cambridge, UK: Cambridge University Press, November 2004.},
  Year                     = {2004},
  Volume                   = {1}
}

@Article{Crooker1993,
  Title                    = {Multiple heliospheric current sheets and coronal streamer belt dynamics},
  Author                   = {Crooker, NU and Siscoe, GL and Shodhan, S and Webb, DF and Gosling, JT and Smith, E Jr},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1993},
  Number                   = {A6},
  Pages                    = {9371--9381},
  Volume                   = {98}
}

@Article{Crosby2006,
  Title                    = {Overview of a graduate course delivered in {Turkey}, emphasizing solar-terrestrial physics and space weather},
  Author                   = {Crosby, NB and Rycroft, MJ and Tulunay, Y},
  Journal                  = {Surveys in geophysics},
  Year                     = {2006},
  Number                   = {3},
  Pages                    = {319--364},
  Volume                   = {27},

  Url                      = {http://link.springer.com/article/10.1007/s10712-005-6204-3}
}

@Article{Cummings1968,
  Title                    = {Magnetic fields in the magnetopause and vicinity at synchronous altitude},
  Author                   = {Cummings, WD and Coleman, PJ},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1968},
  Number                   = {17},
  Pages                    = {5699--5718},
  Volume                   = {73}
}

@Article{Curier2008,
  Title                    = {Retrieval of aerosol optical properties from {OMI} radiances using a multiwavelength algorithm: {Application} to western {Europe}},
  Author                   = {Curier, R. L. and Veefkind, J. P. and Braak, R. and Veihelmann, B. and Torres, O. and De Leeuw, G.},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2008},
  Number                   = {D17},
  Volume                   = {113},

  Shorttitle               = {Retrieval of aerosol optical properties from {OMI} radiances using a multiwavelength algorithm},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2007JD008738/full},
  Urldate                  = {2014-11-13}
}

@Book{Daglis2001,
  Title                    = {Space storms and space weather hazards},
  Author                   = {Daglis, Ioannis A},
  Publisher                = {Springer Science \& Business Media},
  Year                     = {2001},
  Number                   = {5-6},
  Volume                   = {64}
}

@Article{DalPino2012,
  Title                    = {Magnetic flux transport by turbulent reconnection in astrophysical flows},
  Author                   = {Dal Pino, EM de Gouveia and Leão, M. R. M. and Santos-Lima, R. and Guerrero, G. and Kowal, G. and Lazarian, A.},
  Journal                  = {Phys. Scr.},
  Year                     = {2012},
  Number                   = {1},
  Pages                    = {018401},
  Volume                   = {86},

  Url                      = {http://iopscience.iop.org/1402-4896/86/1/018401},
  Urldate                  = {2014-05-31}
}

@Article{Dandouras2013,
  Title                    = {Detection of a plasmaspheric wind in the {Earth}’s magnetosphere by the {Cluster} spacecraft},
  Author                   = {Dandouras, Iannis},
  Journal                  = {Ann. Geophys},
  Year                     = {2013},
  Pages                    = {1143--1153},
  Volume                   = {31},

  File                     = {[PDF] from aeronomie.be:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/5XK3VDDD/Dandouras - 2013 - Detection of a plasmaspheric wind in the Earth’s m.pdf:application/pdf},
  Url                      = {http://plasmasphere.aeronomie.be/pdf/Dandouras_2013_AnnGeo_31_1143.pdf},
  Urldate                  = {2015-12-09}
}

@Article{Dandouras2009,
  Title                    = {Energetic ion dynamics of the inner magnetosphere revealed in coordinated {Cluster}-{Double} {Star} observations},
  Author                   = {Dandouras, Iannis and Cao, Jinbin and Vallat, Claire},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2009},

  Month                    = jan,
  Number                   = {A1},
  Pages                    = {A01S90},
  Volume                   = {114},

  Doi                      = {10.1029/2007JA012757},
  ISSN                     = {0148-0227},
  Keywords                 = {doi:10.102, http://dx.doi.org/10.1029/2007JA012757, like structures},
  Url                      = {http://doi.wiley.com/10.1029/2007JA012757}
}

@Article{Dandouras2009a,
  Title                    = {Magnetosphere response to the 2005 and 2006 extreme solar events as observed by the {Cluster} and {Double} {Star} spacecraft},
  Author                   = {Dandouras, Iannis S and Rème, Henri and Cao, Jinbin and Escoubet, Philippe},
  Journal                  = {Advances in Space Research},
  Year                     = {2009},
  Number                   = {4},
  Pages                    = {618--623},
  Volume                   = {43},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S0273117708005346}
}

@InProceedings{Darrouzet2004,
  Title                    = {Density structures inside the plasmasphere: {Cluster} observations},
  Author                   = {Darrouzet, F. and Décréau, P. M. E. and De Keyser, J. and Masson, A. and Gallagher, D. L. and Santolik, O. and Sandel, B. R. and Trotignon, J. G. and Rauch, J. L. and Le Guirriec, E. and {others}},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2004},
  Pages                    = {2577--2585},
  Volume                   = {22},

  File                     = {[PDF] from archives-ouvertes.fr:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/6QGQ95FF/Darrouzet et al. - 2004 - Density structures inside the plasmasphere Cluste.pdf:application/pdf;Snapshot:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/BM3N25ND/hal-00329350.html:text/html},
  Shorttitle               = {Density structures inside the plasmasphere},
  Url                      = {https://hal.archives-ouvertes.fr/hal-00329350/},
  Urldate                  = {2015-12-09}
}

@InProceedings{Darrouzet2004a,
  Title                    = {Density structures inside the plasmasphere: {Cluster} observations},
  Author                   = {Darrouzet, F. and Décréau, P. M. E. and De Keyser, J. and Masson, A. and Gallagher, D. L. and Santolik, O. and Sandel, B. R. and Trotignon, J. G. and Rauch, J. L. and Le Guirriec, E. and {others}},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2004},
  Pages                    = {2577--2585},
  Volume                   = {22},

  File                     = {[PDF] from archives-ouvertes.fr:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/DHI4EJWW/Darrouzet et al. - 2004 - Density structures inside the plasmasphere Cluste.pdf:application/pdf;Snapshot:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/HDWTH26Q/hal-00329350.html:text/html},
  Shorttitle               = {Density structures inside the plasmasphere},
  Url                      = {https://hal.archives-ouvertes.fr/hal-00329350/},
  Urldate                  = {2015-12-09}
}

@Article{Dasso2006,
  Title                    = {A new model-independent method to compute magnetic helicity in magnetic clouds},
  Author                   = {Dasso, S. and Mandrini, C. H. and Démoulin, P. and Luoni, M. L.},
  Journal                  = {{\textbackslash}aap},
  Year                     = {2006},

  Month                    = aug,
  Pages                    = {349--359},
  Volume                   = {455},

  Doi                      = {10.1051/0004-6361:20064806},
  Keywords                 = {INTERPLANETARY MEDIUM, Sun: coronal mass ejections (CMEs), Sun: magnetic fields}
}

@Article{Daughton2003,
  Title                    = {Electromagnetic properties of the lower-hybrid drift instability in a thin current sheet},
  Author                   = {Daughton, William},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2003},
  Number                   = {8},
  Pages                    = {3103--3119},
  Volume                   = {10}
}

@Article{Daughton2005,
  Title                    = {Kinetic theory of collisionless tearing at the magnetopause},
  Author                   = {Daughton, W. and Karimabadi, H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2005},

  Month                    = mar,
  Pages                    = {3217},
  Volume                   = {110},

  Abstract                 = {This paper is the first in a series of three with the aim of addressing one of the controversial issues at the magnetopause, namely the location where reconnection first occurs during periods of a large interplanetary magnetic field By. In this first paper, the linear properties of the collisionless tearing mode are reexamined as a function of the guide field By using a formally exact approach for computing the nonlocal Vlasov stability of a current layer. Three distinct parameter regimes are identified depending on the degree to which electron orbits are modified by the guide field in the central region of the current layer. In the limit of both weak and strong guide field, the fastest-growing tearing mode has a wave vector kx perpendicular to the direction of the current, in agreement with previous theoretical treatments. However, for intermediate values of the guide field where the electrons begin to transition to magnetized orbits, the fastest-growing modes have a finite wave vector ky in the direction of the current. In this newly discovered regime, the so-called drift tearing modes have finite real frequency and propagate in the direction of the electron diamagnetic drift with growth rates 10-50\% larger than the conventional tearing instability. Maximum growth occurs for a propagation angle in the range θ = tan-1(ky/kx) ≈ 6-10°. These new predictions are confirmed using fully kinetic particle-in-cell simulations. The structure of the out-of-plane magnetic field perturbation predicted by nonlocal Vlasov theory is examined as a function of guide field. In the limit of a neutral sheet, the quadrupole structure has a characteristic scale near the electron meandering width and shows significant differences with the predictions of linear Hall MHD. The addition of a guide field strongly distorts the quadrupole structure and compresses the spatial extent. In the strong guide field limit, the width of the out-of-plane magnetic field perturbation is reduced to the electron gyroscale in the guide field. During the onset phase, these structures represent a distinct signature of the collisionless tearing mode that is significantly different than the typical ion-scale quadrupole pattern from fast reconnection. Finally, we note that the tearing mode maintains a significant growth rate over a large range of guide field so that component merging cannot be ruled out based on linear theory.},
  Doi                      = {10.1029/2004JA010751},
  Keywords                 = {7835), guide field, kinetic, linear theory, Magnetospheric Physics: Magnetic reconnection (7526, Magnetospheric Physics: Magnetopause and boundary layers, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Plasma waves and instabilities (2471), reconnection, Space Plasma Physics: Kinetic waves and instabilities, tearing}
}

@Article{Daughton2011,
  Title                    = {Role of electron physics in the development of turbulent magnetic reconnection in collisionless plasmas},
  Author                   = {Daughton, W. and Roytershteyn, V. and Karimabadi, H. and Yin, L. and Albright, B. J. and Bergen, B. and Bowers, K. J.},
  Journal                  = {Nature Physics},
  Year                     = {2011},
  Number                   = {7},
  Pages                    = {539--542},
  Volume                   = {7},

  Url                      = {http://www.nature.com/nphys/journal/v7/n7/abs/nphys1965.html},
  Urldate                  = {2014-05-31}
}

@Article{Dayeh2009,
  Title                    = {Composition and spectral properties of the 1 {AU} quiet-time suprathermal ion population during solar cycle 23},
  Author                   = {Dayeh, MA and Desai, MI and Dwyer, JR and Rassoul, HK and Mason, GM and Mazur, JE},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2009},
  Number                   = {2},
  Pages                    = {1588},
  Volume                   = {693}
}

@InProceedings{Dayeh2009a,
  Title                    = {Proton intensity gradients and radiation dose equivalents in the inner heliosphere: {Modeling} and {Prediction}},
  Author                   = {Dayeh, MA and Desai, MI and Kozarev, KA and Schwadron, NA and Townsend, LW and Pourarsalan, M and Zeitlin, CJ and Hatcher, RD},
  Booktitle                = {{AGU} {Fall} {Meeting} {Abstracts}},
  Year                     = {2009},
  Pages                    = {1492},
  Volume                   = {1}
}

@InProceedings{Dayeh2012,
  Title                    = {Latitudinal variation of heliospheric {ENAs} and their correlation with solar wind observations},
  Author                   = {Dayeh, MA and McComas, DJ and Allegrini, F and Desai, MI and Ebert, RW and Livadiotis, G and Schwadron, NA},
  Booktitle                = {{AGU} {Fall} {Meeting} {Abstracts}},
  Year                     = {2012},
  Pages                    = {2209},
  Volume                   = {1}
}

@Article{Dayeh2011,
  Title                    = {Spectral properties of regions and structures in the {Interstellar} {Boundary} {Explorer} ({IBEX}) sky maps},
  Author                   = {Dayeh, MA and McComas, DJ and Livadiotis, G and Ebert, RW and Funsten, HO and Janzen, P and Reisenfeld, DB and Schwadron, NA},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2011},
  Number                   = {1},
  Pages                    = {29},
  Volume                   = {734}
}

@Article{DeSterck1998,
  Title                    = {Complex magnetohydrodynamic bow shock topology in field-aligned low-β flow around a perfectly conducting cylinder},
  Author                   = {De Sterck, H. and Low, B. C. and Poedts, S.},
  Journal                  = {Phys. Plasmas},
  Year                     = {1998},
  Number                   = {11},
  Pages                    = {4015},
  Volume                   = {5},

  Doi                      = {10.1063/1.873124},
  ISSN                     = {1070664X},
  Url                      = {http://scitation.aip.org/content/aip/journal/pop/5/11/10.1063/1.873124}
}

@Article{Demoulin2008,
  Title                    = {A review of the quantitative links between {CMEs} and magnetic clouds},
  Author                   = {Démoulin, P.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2008},

  Month                    = oct,
  Pages                    = {3113--3125},
  Volume                   = {26},

  Doi                      = {10.5194/angeo-26-3113-2008}
}

@Article{Dere2007,
  Title                    = {Ionization rate coefficients for the elements hydrogen through zinc},
  Author                   = {Dere, K. P.},
  Journal                  = {{\textbackslash}aap},
  Year                     = {2007},

  Month                    = may,
  Pages                    = {771--792},
  Volume                   = {466},

  Doi                      = {10.1051/0004-6361:20066728},
  Keywords                 = {atomic data, Atomic Processes, plasmas}
}

@Article{Dere1997,
  Title                    = {{CHIANTI} - an atomic database for emission lines},
  Author                   = {Dere, K. P. and Landi, E. and Mason, H. E. and Monsignori Fossi, B. C. and Young, P. R.},
  Journal                  = {{\textbackslash}aaps},
  Year                     = {1997},

  Month                    = oct,
  Pages                    = {149--173},
  Volume                   = {125},

  Doi                      = {10.1051/aas:1997368},
  Keywords                 = {ASTRONOMICAL DATA BASES: MISCELLANEOUS, atomic data, STARS: ATMOSPHERE, SUN: ATMOSPHERE, ultraviolet: general}
}

@Article{Dere2009,
  Title                    = {{CHIANTI} - an atomic database for emission lines. {IX}. {Ionization} rates, recombination rates, ionization equilibria for the elements hydrogen through zinc and updated atomic data},
  Author                   = {Dere, K. P. and Landi, E. and Young, P. R. and Del Zanna, G. and Landini, M. and Mason, H. E.},
  Journal                  = {{\textbackslash}aap},
  Year                     = {2009},

  Month                    = may,
  Pages                    = {915--929},
  Volume                   = {498},

  Doi                      = {10.1051/0004-6361/200911712},
  Keywords                 = {atomic data, Atomic Processes, plasmas, radiation mechanisms: thermal}
}

@Article{Dimmock2012,
  Title                    = {A statistical study of the cross-shock electric potential at low {Mach} number, quasi-perpendicular bow shock crossings using {Cluster} data},
  Author                   = {Dimmock, AP and Balikhin, MA and Krasnoselskikh, VV and Walker, SN and Bale, SD and Hobara, Y},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2012},
  Number                   = {A2},
  Volume                   = {117}
}

@Article{Divin2012,
  Title                    = {Scaling of the inner electron diffusion region in collisionless magnetic reconnection},
  Author                   = {Divin, Andrey and Lapenta, Giovanni and Markidis, Stefano and Semenov, V. S. and Erkaev, N. V. and Korovinskiy, D. B. and Biernat, H. K.},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2012},
  Number                   = {A6},
  Volume                   = {117},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2011JA017464/full},
  Urldate                  = {2014-05-31}
}

@Article{Dmitriev2003,
  Title                    = {Comparative study of bow shock models using {Wind} and {Geotail} observations},
  Author                   = {Dmitriev, AV and Chao, JK and Wu, DJ},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2003},
  Number                   = {A12},
  Pages                    = {1464},
  Volume                   = {108}
}

@Article{Dmitriev2005,
  Title                    = {Interplanetary sources of space weather disturbances in 1997 to 2000},
  Author                   = {Dmitriev, AV and Crosby, NB and Chao, J-K},
  Journal                  = {Space Weather},
  Year                     = {2005},
  Number                   = {3},
  Volume                   = {3}
}

@Article{Domingo1996,
  Title                    = {The first results from {SOHO}.},
  Author                   = {Domingo, V and Fleck, B and Poland, A},
  Journal                  = {ESA bulletin},
  Year                     = {1996},
  Pages                    = {7--24},
  Volume                   = {87}
}

@Article{Domingos2006,
  Title                    = {Stable satellites around extrasolar giant planets},
  Author                   = {Domingos, R. C. and Winter, O. C. and Yokoyama, T.},
  Journal                  = {{\textbackslash}textbackslashmnras},
  Year                     = {2006},

  Month                    = dec,
  Pages                    = {1227--1234},
  Volume                   = {373},

  Doi                      = {10.1111/j.1365-2966.2006.11104.x},
  Keywords                 = {celestial mechanics, planetary systems, planets and satellites: general}
}

@Article{Drake2014,
  Title                    = {The {Onset} of {Ion} {Heating} {During} {Magnetic} {Reconnection} with a {Strong} {Guide} {Field}},
  Author                   = {Drake, J. F. and Swisdak, M.},
  Journal                  = {arXiv preprint arXiv:1404.7795},
  Year                     = {2014},

  Url                      = {http://arxiv.org/abs/1404.7795},
  Urldate                  = {2014-05-31}
}

@Article{Drake2011,
  Title                    = {Neon {Insights} from {Old} {Solar} {X}-{Rays}: {A} {Plasma} {Temperature} {Dependence} of the {Coronal} {Neon} {Content}},
  Author                   = {Drake, J. J.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2011},

  Month                    = dec,
  Pages                    = {22},
  Volume                   = {743},

  Doi                      = {10.1088/0004-637X/743/1/22},
  Keywords                 = {Sun: abundances, Sun: activity, Sun: corona, X-rays: stars}
}

@Article{Drake2005,
  Title                    = {The `solar model problem' solved by the abundance of neon in nearby stars},
  Author                   = {Drake, J. J. and Testa, P.},
  Journal                  = {{\textbackslash}nat},
  Year                     = {2005},

  Month                    = jul,
  Pages                    = {525--528},
  Volume                   = {436},

  Doi                      = {10.1038/nature03803}
}

@Article{Dubinin2005,
  Title                    = {Differential ion streaming in the solar wind as an equilibrium state},
  Author                   = {Dubinin, E. and Sauer, K. and McKenzie, J. F.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2005},

  Month                    = jul,
  Pages                    = {7101},
  Volume                   = {110},

  Doi                      = {10.1029/2004JA010826},
  Keywords                 = {6050, 7836), alpha particles, Interplanetary Physics: Interplanetary magnetic fields, Interplanetary Physics: MHD waves and turbulence (2752, Interplanetary Physics: Plasma waves and turbulence, Interplanetary Physics: Solar wind plasma, Solar Wind, waves}
}

@Article{Dubinin2004,
  Title                    = {Nonlinear stationary waves and solitons in ion beam-plasma configuration},
  Author                   = {Dubinin, E. and Sauer, K. and McKenzie, J. F.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = feb,
  Pages                    = {2208},
  Volume                   = {109},

  Doi                      = {10.1029/2003JA010283},
  Keywords                 = {beam solitons, foreshock, gyrating ions, Interplanetary Physics: MHD waves and turbulence, Interplanetary Physics: Planetary bow shocks, Interplanetary Physics: Plasma waves and turbulence, Ionosphere: Wave/particle interactions, Ionosphere: Wave propagation (6934), nonlinear waves}
}

@Article{Dubovik2008,
  Title                    = {Retrieving global aerosol sources from satellites using inverse modeling},
  Author                   = {Dubovik, O. and Lapyonok, T. and Kaufman, Y. J. and Chin, M. and Ginoux, P. and Kahn, R. A. and Sinyuk, A.},
  Journal                  = {Atmos. Chem. Phys.},
  Year                     = {2008},
  Number                   = {2},
  Pages                    = {209--250},
  Volume                   = {8},

  Url                      = {http://www.atmos-chem-phys.net/8/209/2008/acp-8-209-2008.html},
  Urldate                  = {2014-11-13}
}

@Article{DudokdeWit2013,
  Title                    = {Methods for {Characterising} {Microphysical} {Processes} in {Plasmas}},
  Author                   = {Dudok de Wit, T. and Alexandrova, O. and Furno, I. and Sorriso-Valvo, L. and Zimbardo, G.},
  Journal                  = {Space Sci. Rev.},
  Year                     = {2013},

  Month                    = may,
  Number                   = {2-4},
  Pages                    = {665--693},
  Volume                   = {178},

  Doi                      = {10.1007/s11214-013-9974-9},
  ISSN                     = {0038-6308},
  Url                      = {http://link.springer.com/10.1007/s11214-013-9974-9}
}

@Article{Dungey1962,
  Title                    = {The interplanetary field and auroral theory},
  Author                   = {Dungey, JW},
  Journal                  = {Journal of the Physical Society of Japan Supplement},
  Year                     = {1962},
  Pages                    = {15},
  Volume                   = {17},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.22}
}

@Article{Dunlop2011,
  Title                    = {{Extended magnetic reconnection across the dayside magnetopause}},
  Author                   = {Dunlop, M. W. and Zhang, Q. H. and Bogdanova, Y. V. and Lockwood, M. and Pu, Z. and Hasegawa, H. and Wang, J. and Taylor, M. G G T and Berchem, J. and Lavraud, B. and Eastwood, J. and Volwerk, M. and Shen, C. and Shi, J. K. and Constantinescu, D. and Frey, H. and Fazakerley, A. N. and Sibeck, D. and Escoubet, P. and Wild, J. A. and Liu, Z. X.},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2011},
  Number                   = {2},
  Volume                   = {107},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {The extent of where magnetic reconnection (MR), the dominant process responsible for energy and plasma transport into the magnetosphere, operates across Earth's dayside magnetopause has previously been only indirectly shown by observations. We report the first direct evidence of X-line structure resulting from the operation of MR at each of two widely separated locations along the tilted, subsolar line of maximum current on Earth's magnetopause, confirming the operation of MR at two or more sites across the extended region where MR is expected to occur. The evidence results from in-situ observations of the associated ion and electron plasma distributions, present within each magnetic X-line structure, taken by two spacecraft passing through the active MR regions simultaneously.},
  Doi                      = {10.1103/PhysRevLett.107.025004},
  ISSN                     = {00319007},
  Owner                    = {suleimanbaraka},
  Pmid                     = {21797615},
  Timestamp                = {2016.02.23}
}

@Article{Duston1977,
  Title                    = {Energetic properties of interplanetary plasma at the earth's orbit following the {August} 4, 1972 flare},
  Author                   = {Duston, C. and Bosqued, J. M. and Cambou, F. and Temnyi, V. V. and Zastenker, G. N. and Vaisberg, O. L. and Eroshenko, E. G.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {1977},

  Month                    = feb,
  Pages                    = {217--229},
  Volume                   = {51},

  Doi                      = {10.1007/BF00240459},
  Keywords                 = {Interplanetary Magnetic Fields, Meteorological Satellites, Pioneer 9 Space Probe, Plasma Density, Plasma Dynamics, Shock Wave Propagation, Solar Activity Effects, Solar Flares, Solar Wind}
}

@Article{Dzifcakova2010,
  Title                    = {The {Diagnostics} of the κ-{Distributions} from {EUV} {Spectra}},
  Author                   = {Dzifčáková, E. and Kulinová, A.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {2010},

  Month                    = may,
  Pages                    = {25--41},
  Volume                   = {263},

  Doi                      = {10.1007/s11207-010-9539-y},
  Keywords                 = {Non-thermal distributions, Plasma diagnostics, Sun: EUV spectra}
}

@Article{Eastman1979,
  Title                    = {Characteristics of the magnetospheric boundary layer and magnetopause layer as observed by {IMP} 6},
  Author                   = {Eastman, TE and Hones, EW},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1979},
  Number                   = {A5},
  Pages                    = {2019--2028},
  Volume                   = {84}
}

@Article{Eastwood2005a,
  Title                    = {The foreshock},
  Author                   = {Eastwood, JP and Lucek, EA and Mazelle, C and Meziane, K and Narita, Y and Pickett, J and Treumann, RA},
  Journal                  = {Space science reviews},
  Year                     = {2005},
  Number                   = {1-4},
  Pages                    = {41--94},
  Volume                   = {118}
}

@InCollection{Eastwood2005b,
  Title                    = {The foreshock},
  Author                   = {Eastwood, JP and Lucek, EA and Mazelle, C and Meziane, K and Narita, Y and Pickett, J and Treumann, RA},
  Booktitle                = {Outer {Magnetospheric} {Boundaries}: {Cluster} {Results}},
  Publisher                = {Springer},
  Year                     = {2005},
  Pages                    = {41--94}
}

@Article{Eastwood2008,
  Title                    = {The science of space weather},
  Author                   = {Eastwood, Jonathan P},
  Journal                  = {Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
  Year                     = {2008},
  Number                   = {1884},
  Pages                    = {4489--4500},
  Volume                   = {366}
}

@Article{Eastwood2005c,
  Title                    = {Quasi-monochromatic {ULF} foreshock waves as observed by the four-spacecraft {Cluster} mission: 2. {Oblique} propagation},
  Author                   = {Eastwood, J. P. and Balogh, A. and Lucek, E. A. and Mazelle, C. and Dandouras, I.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2005},

  Month                    = nov,
  Number                   = {A9},
  Pages                    = {11220},
  Volume                   = {110},

  Doi                      = {10.1029/2004JA010618},
  Keywords                 = {6944), 6984), Interplanetary Physics: Instruments and techniques, Interplanetary Physics: Planetary bow shocks, ion beam instabilities, multispacecraft analysis, nonlinear interaction, Space Plasma Physics: Kinetic waves and instabilities, Space Plasma Physics: Nonlinear phenomena (4400, Space Plasma Physics: Wave/particle interactions (2483, terrestrial foreshock, ultra-low-frequency waves}
}

@Article{Eastwood2012,
  Title                    = {Survival of flux transfer event ({FTE}) flux ropes far along the tail magnetopause},
  Author                   = {Eastwood, J. P. and Phan, T. D. and Fear, R. C. and Sibeck, D. G. and Angelopoulos, V. and ØIeroset, M. and Shay, M. A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2012},
  Pages                    = {8222},
  Volume                   = {117},

  Abstract                 = {During intervals of southward IMF, magnetic reconnection can result in the formation of flux transfer events (FTEs) on the dayside magnetopause which travel along the magnetopause in the anti-sunward direction. Of particular interest is their fate and the role they play transporting solar wind plasma into the magnetosphere. We present the discovery of FTEs far along the distant tail magnetopause (x = -67 Earth radii) using data from ARTEMIS on the dusk flank magnetopause under southward/duskward IMF conditions. The identification of several events is further supported by excellent fits to a force-free flux rope model. The axis of each structure is principally north-south, i.e., perpendicular to the Sun-Earth line. Simultaneous observations by THEMIS on the dayside magnetopause indicate that FTEs are being produced there, although perhaps 2-4 times smaller in size. The convection time from the dayside magnetopause to ARTEMIS is 30 min, and the FTEs have a flux content comparable to those typically observed on the dayside magnetopause, indicating that these features are in quasi-equilibrium as they are convected downtail. By considering the relative orientations of the FTEs observed by THEMIS and ARTEMIS, the magnetic field geometry is consistent with the FTEs being produced on the dayside magnetopause along an extended X-line in the presence of IMF B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater} and bending as they are convected to the flanks.},
  ISSN                     = {0148-0227},
  Keywords                 = {ARTEMIS FTE THEMIS flux rope flux transfer event reconnection Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Solar wind/magnetosphere interactions Space Plasma Physics: Magnetic reconnection (2723 7526) Space Plasma Physics: Transport processes},
  Url                      = {http://adsabs.harvard.edu/abs/2012JGRA..117.8222E}
}

@Article{Eastwood2008a,
  Title                    = {{THEMIS} observations of a hot flow anomaly: {Solar} wind, magnetosheath, and ground-based measurements},
  Author                   = {Eastwood, J. P. and Sibeck, D. G. and Angelopoulos, V. and Phan, T. D. and Bale, S. D. and McFadden, J. P. and Cully, C. M. and Mende, S. B. and Larson, D. and Frey, S. and Carlson, C. W. and Glassmeier, K.-H. and Auster, H. U. and Roux, A. and Le Contel, O.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2008},
  Volume                   = {35},

  Abstract                 = {The THEMIS spacecraft encountered a Hot Flow Anomaly (HFA) on the dusk flank of the Earth's bow shock on 4 July 2007, observing it on both sides of the shock. Meanwhile, the THEMIS ground magnetometers traced the progress of the associated Magnetic Impulse Event along the dawn flank of the magnetosphere, providing a unique opportunity to study the transmission of the HFA through the shock and the subsequent downstream response. THEMIS-A, in the solar wind, observed classic HFA signatures. Isotropic electron distributions inside the upstream HFA are attributed to the action of the electron firehose instability. THEMIS-E, just downstream, observed a much more complex disturbance with the pressure perturbation decoupled from the underlying discontinuity. Simple calculations show that the pressure perturbation would be capable of significantly changing the magnetopause location, which is confirmed by the ground-based observations.},
  ISSN                     = {0094-8276},
  Keywords                 = {Space Plasma Physics: Shock waves (4455) Magnetospheric Physics: Solar wind/magnetosphere interactions Space Plasma Physics: Discontinuities (2109) Magnetospheric Physics: Magnetospheric configuration and dynamics},
  Url                      = {http://adsabs.harvard.edu/abs/2008GeoRL..3517S03E}
}

@Article{Eastwood2005,
  Title                    = {{Observations of multiple X-line structure in the Earth's magnetotail current sheet: A Cluster case study}},
  Author                   = {Eastwood, Jonathan P. and Sibeck, D. G. and Slavin, J. A. and Goldstein, M. L. and Lavraud, B. and Sitnov, M. and Imber, S. and Balogh, A. and Lucek, E. A. and Dandouras, I.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2005},
  Number                   = {11},
  Pages                    = {1--4},
  Volume                   = {32},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {Observations of the Earth's magnetotail made by the four Cluster spacecraft on October 2 2003 are presented. Multi-spacecraft analysis is used to show that the variations in field and flow observed in the vicinity of the magnetotail current sheet are most consistent with a series of two active reconnection sites bounding an Earthward moving flux rope. We demonstrate that a single spacecraft analysis of the same data leads to the incorrect conclusion that a single X-line is moving tailward. The implications of this in relation to the interpretation of single spacecraft observations are outlined. These results show that reconnection can occur simultaneously at different points in the near-Earth magnetotail current sheet, providing (further) important experimental validation of multiple X - line reconnection theories on the mesoscale (tens of ion inertial length) level.},
  Doi                      = {10.1029/2005GL022509},
  ISSN                     = {00948276},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Eastwood2005d,
  Title                    = {Observations of multiple {X}-line structure in the {Earth}'s magnetotail current sheet: {A} {Cluster} case study},
  Author                   = {Eastwood, J. P. and Sibeck, D. G. and Slavin, J. A. and Goldstein, M. L. and Lavraud, B. and Sitnov, M. and Imber, S. and Balogh, A. and Lucek, E. A. and Dandouras, I.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2005},
  Pages                    = {11105},
  Volume                   = {32},

  Abstract                 = {Observations of the Earth's magnetotail made by the four Cluster spacecraft on October 2 2003 are presented. Multi-spacecraft analysis is used to show that the variations in field and flow observed in the vicinity of the magnetotail current sheet are most consistent with a series of two active reconnection sites bounding an Earthward moving flux rope. We demonstrate that a single spacecraft analysis of the same data leads to the incorrect conclusion that a single X-line is moving tailward. The implications of this in relation to the interpretation of single spacecraft observations are outlined. These results show that reconnection can occur simultaneously at different points in the near-Earth magnetotail current sheet, providing (further) important experimental validation of multiple X - line reconnection theories on the mesoscale (tens of ion inertial length) level.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Magnetotail Magnetospheric Physics: Plasma sheet},
  Url                      = {http://adsabs.harvard.edu/abs/2005GeoRL..3211105E}
}

@InProceedings{Ebert2012,
  Title                    = {Multipoint {Analysis} of a {Corotating} {Interaction} {Region} and its {Associated} {Energetic} {Particles} at {STEREO}-{A}, {STEREO}-{B}, and {ACE}: {Observations} and {Modeling}},
  Author                   = {Ebert, RW and Dayeh, MA and Desai, MI and Li, G and Mason, GM},
  Booktitle                = {{AGU} {Fall} {Meeting} {Abstracts}},
  Year                     = {2012},
  Pages                    = {03},
  Volume                   = {1}
}

@Article{Echer2006,
  Title                    = {On the geomagnetic effects of solar wind interplanetary magnetic structures},
  Author                   = {Echer, E and Gonzalez, WD and Alves, MV},
  Journal                  = {Space Weather},
  Year                     = {2006},
  Number                   = {6},
  Volume                   = {4}
}

@Article{Echer2005,
  Title                    = {Introduction to space weather},
  Author                   = {Echer, E and Gonzalez, WD and Guarnieri, FL and Lago, A Dal and Vieira, LEA},
  Journal                  = {Advances in Space Research},
  Year                     = {2005},
  Number                   = {5},
  Pages                    = {855--865},
  Volume                   = {35},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S0273117705004709}
}

@Article{Eckart2012,
  Title                    = {Flare emission from {Sagittarius} {A}*},
  Author                   = {Eckart, A. and García-Marín, M. and Vogel, S. N. and Teuben, P. and Morris, M. R. and Baganoff, F. and Dexter, J. and Schödel, R. and Witzel, G. and Valencia-S, M. and Karas, V. and Kunneriath, D. and Bremer, M. and Straubmeier, C. and Moser, L. and Sabha, N. and Buchholz, R. and Zamaninasab, M. and Mužić, K. and Moultaka, J. and Zensus, J. A.},
  Journal                  = {Journal of Physics Conference Series},
  Year                     = {2012},

  Month                    = jul,
  Number                   = {1},
  Pages                    = {012022},
  Volume                   = {372},

  Doi                      = {10.1088/1742-6596/372/1/012022}
}

@Article{Edmondson2013,
  Title                    = {Analysis of {High} {Cadence} {In} {Situ} {Solar} {Wind} {Ionic} {Composition} {Data} {Using} {Wavelet} {Power} {Spectra} {Confidence} {Levels}},
  Author                   = {Edmondson, J. K. and Lynch, B. J. and Lepri, S. T. and Zurbuchen, T. H.},
  Journal                  = {{\textbackslash}apjs},
  Year                     = {2013},

  Month                    = dec,
  Pages                    = {35},
  Volume                   = {209},

  Doi                      = {10.1088/0067-0049/209/2/35},
  Keywords                 = {methods: analytical, methods: data analysis, methods: statistical, Solar Wind, Sun: corona, Sun: heliosphere}
}

@Article{Egedal2012,
  Title                    = {Large-scale electron acceleration by parallel electric fields during magnetic reconnection},
  Author                   = {Egedal, Jan and Daughton, W. and Le, A.},
  Journal                  = {Nature Physics},
  Year                     = {2012},
  Number                   = {4},
  Pages                    = {321--324},
  Volume                   = {8},

  Url                      = {http://www.nature.com/nphys/journal/v8/n4/abs/nphys2249.html},
  Urldate                  = {2014-05-31}
}

@Article{Egedal2013,
  Title                    = {A review of pressure anisotropy caused by electron trapping in collisionless plasma, and its implications for magnetic reconnection},
  Author                   = {Egedal, Jan and Le, Ari and Daughton, William},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2013},
  Number                   = {6},
  Pages                    = {061201},
  Volume                   = {20},

  Url                      = {http://scitation.aip.org/content/aip/journal/pop/20/6/10.1063/1.4811092},
  Urldate                  = {2014-05-31}
}

@Article{Eliasson2007,
  Title                    = {Simulation study of magnetic holes at the {Earth}'s collisionless bow shock},
  Author                   = {Eliasson, B and Shukla, P K},
  Journal                  = {New Journal of Physics},
  Year                     = {2007},

  Month                    = jun,
  Number                   = {6},
  Pages                    = {168--168},
  Volume                   = {9},

  Doi                      = {10.1088/1367-2630/9/6/168},
  ISSN                     = {1367-2630},
  Url                      = {http://stacks.iop.org/1367-2630/9/i=6/a=168?key=crossref.f6b620a7d7b6e7fd61bd09ecff3622f1}
}

@Article{Eliasson2006,
  Title                    = {Theoretical and simulation studies of relativistic ion holes in astrophysical plasmas},
  Author                   = {Eliasson, B. and Shukla, P. K. and Dieckmann, M. E.},
  Journal                  = {New Journal of Physics},
  Year                     = {2006},

  Month                    = apr,
  Pages                    = {55},
  Volume                   = {8},

  Doi                      = {10.1088/1367-2630/8/4/055}
}

@Article{Ellison1993,
  Title                    = {Simulations of particle acceleration in parallel shocks: {Direct} comparison between {Monte} {Carlo} and one-dimensional hybrid codes},
  Author                   = {Ellison, Donald C and Giacalone, J and Burgess, D and Schwartz, SJ},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1993},
  Number                   = {A12},
  Pages                    = {21085--21093},
  Volume                   = {98}
}

@Article{Engebretson2013,
  Title                    = {Multi-instrument observations from {Svalbard} of a traveling convection vortex, electromagnetic ion cyclotron wave burst, and proton precipitation associated with a bow shock instability},
  Author                   = {Engebretson, M. J. and Yeoman, T. K. and Oksavik, K. and SøRaas, F. and Sigernes, F. and Moen, J. I. and Johnsen, M. G. and Pilipenko, V. A. and Posch, J. L. and Lessard, M. R. and Lavraud, B. and Hartinger, M. D. and Clausen, L. B. N. and Raita, T. and Stolle, C.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = jun,
  Pages                    = {2975--2997},
  Volume                   = {118},

  Doi                      = {10.1002/jgra.50291},
  Keywords                 = {bow shock, Electromagnetic ion cyclotron waves, Traveling convection vortices}
}

@Article{Engwall2009,
  Title                    = {Statistics of the cold hidden component of ionospheric outflow determined from 5 to 19 {RE} in the {Earth}'s magnetotail},
  Author                   = {Engwall, E and Eriksson, AI and Cully, CM},
  Journal                  = {Ann. {\textbackslash}ldots},
  Year                     = {2009},

  Url                      = {http://www.diva-portal.org/smash/record.jsf?pid=diva2:210740}
}

@Book{Engwall2008,
  Title                    = {Thousands of tons from the atmosphere lost into space annually},
  Author                   = {Engwall, Erik, Anders Eriksson, Mats Andr‚àö√†},
  Year                     = {2008},
  Note                     = {Published: Swedish Institute of Space Physics},

  Url                      = {http://www.irf.se/Topical/Press/?dbfile=Thousands%20of%20tons%20from%20the%20atmosphere%20lost%20into%20space%20annually&dbsec=P4}
}

@InProceedings{Escoubet1999,
  Title                    = {Introduction the cluster mission},
  Author                   = {Escoubet, CP and Fehringer, M and Goldstein, M},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {1999},
  Pages                    = {1197--1200},
  Publisher                = {Copernicus GmbH},
  Volume                   = {19},

  Url                      = {http://www.ann-geophys.net/19/1197/2001/}
}

@Article{Escoubet2000,
  Title                    = {Cluster {II}: {Plasma} measurements in three dimensions},
  Author                   = {Escoubet, CP and Schmidt, R},
  Journal                  = {Advances in Space Research},
  Year                     = {2000},
  Number                   = {7},
  Pages                    = {1305--1314},
  Volume                   = {25}
}

@InCollection{Escoubet1997,
  Title                    = {Cluster-{Science} and mission overview},
  Author                   = {Escoubet, CP and Schmidt, R and Goldstein, ML},
  Booktitle                = {The {Cluster} and {Phoenix} {Missions}},
  Publisher                = {Springer},
  Year                     = {1997},
  Pages                    = {11--32},

  Url                      = {http://link.springer.com/chapter/10.1007/978-94-011-5666-0_1}
}

@Book{Escoubet1997a,
  Title                    = {The {Cluster} and {PHOENIX} missions},
  Author                   = {Escoubet, C. P. and Russell, C. T. and Schmidt, R.},
  Year                     = {1997}
}

@Book{Escoubet1997b,
  Title                    = {The {Cluster} and {PHOENIX} missions},
  Author                   = {Escoubet, C. P. and Russell, C. T. and Schmidt, R.},
  Year                     = {1997}
}

@Article{Esser2002,
  Title                    = {Constraints on ion outflow speeds and electron distribution function in the corona derived from sumer electron temperatures and {SWICS} ion fractions},
  Author                   = {Esser, R. and Edgar, R. J.},
  Journal                  = {Advances in Space Research},
  Year                     = {2002},
  Pages                    = {481--486},
  Volume                   = {30},

  Doi                      = {10.1016/S0273-1177(02)00321-6}
}

@Article{Esser2001,
  Title                    = {Differential {Flow} {Speeds} of {Ions} of the {Same} {Element}: {Effects} on {Solar} {Wind} {Ionization} {Fractions}},
  Author                   = {Esser, R. and Edgar, R. J.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2001},

  Month                    = dec,
  Pages                    = {1055--1062},
  Volume                   = {563},

  Doi                      = {10.1086/323987},
  Keywords                 = {Sun: Particle Emission, Sun: solar wind}
}

@Article{Esser2000,
  Title                    = {Reconciling {Spectroscopic} {Electron} {Temperature} {Measurements} in the {Solar} {Corona} with {In} {Situ} {Charge} {State} {Observations}},
  Author                   = {Esser, R. and Edgar, R. J.},
  Journal                  = {{\textbackslash}apjl},
  Year                     = {2000},

  Month                    = mar,
  Pages                    = {L71--L74},
  Volume                   = {532},

  Doi                      = {10.1086/312548},
  Keywords                 = {SUN: ATMOSPHERE, Sun: corona, Sun: solar wind}
}

@Article{Esser1998,
  Title                    = {High {Minor} {Ion} {Outflow} {Speeds} in the {Inner} {Corona} and {Observed} {Ion} {Charge} {States} in {Interplanetary} {Space}},
  Author                   = {Esser, R. and Edgar, R. J. and Brickhouse, N. S.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {1998},

  Month                    = may,
  Pages                    = {448--457},
  Volume                   = {498},

  Doi                      = {10.1086/305516},
  Keywords                 = {INTERPLANETARY MEDIUM, Sun: corona, Sun: Particle Emission}
}

@Article{Fairfield1990,
  Title                    = {Upstream pressure variations associated with the bow shock and their effects on the magnetosphere},
  Author                   = {Fairfield, DH and Baumjohann, W and Paschmann, G and Lühr, H and Sibeck, DG},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1990},
  Number                   = {A4},
  Pages                    = {3773--3786},
  Volume                   = {95}
}

@Article{Fairfield1971,
  Title                    = {Average and unusual locations of the {Earth}'s magnetopause and bow shock},
  Author                   = {Fairfield, Donald H},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1971},
  Number                   = {28},
  Pages                    = {6700--6716},
  Volume                   = {76}
}

@Article{Fares2010,
  Title                    = {Searching for star-planet interactions within the magnetosphere of {HD}189733},
  Author                   = {Fares, R. and Donati, J.-F. and Moutou, C. and Jardine, M. M. and Grie{\textbackslash}textbackslashs smeier, J.-M. and Zarka, P. and Shkolnik, E. L. and Bohlender, D. and Catala, C. and Collier Cameron, A.},
  Journal                  = {{\textbackslash}textbackslashmnras},
  Year                     = {2010},

  Month                    = jul,
  Pages                    = {409--419},
  Volume                   = {406},

  Doi                      = {10.1111/j.1365-2966.2010.16715.x},
  Keywords                 = {planetary systems, stars: activity, stars: individual: HD189733, stars: magnetic field}
}

@Article{Farris1991,
  Title                    = {The thickness of the magnetosheath: {Constraints} on the polytropic index},
  Author                   = {Farris, MH and Petrinec, SM and Russell, CT},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1991},
  Number                   = {10},
  Pages                    = {1821--1824},
  Volume                   = {18}
}

@Article{Farrugia2011,
  Title                    = {“{Crater}” flux transfer events: {Highroad} to the {X} line?},
  Author                   = {Farrugia, C. J. and Chen, Li-Jen and Torbert, R. B. and Southwood, D. J. and Cowley, S. W. H. and Vrublevskis, A. and Mouikis, C. and Vaivads, A. and André, M. and Décréau, P. and Vaith, H. and Owen, C. J. and Sibeck, D. J. and Lucek, E. and Smith, C. W.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2011},
  Pages                    = {2204},
  Volume                   = {116},

  Abstract                 = {We examine Cluster observations of a so-called magnetosphere “crater FTE,” employing data from five instruments (FGM, CIS, EDI, EFW, and WHISPER), some at the highest resolution. The aim of doing this is to deepen our understanding of the reconnection nature of these events by applying recent advances in the theory of collisionless reconnection and in detailed observational work. Our data support the hypothesis of a stratified structure with regions which we show to be spatial structures. We support the bulge-like topology of the core region (R3) made up of plasma jetting transverse to reconnected field lines. We document encounters with a magnetic separatrix as a thin layer embedded in the region (R2) just outside the bulge, where the speed of the protons flowing approximately parallel to the field maximizes: (1) short (fraction of a sec) bursts of enhanced electric field strengths (up to ˜30 mV/m) and (2) electrons flowing against the field toward the X line at approximately the same time as the bursts of intense electric fields. R2 also contains a density decrease concomitant with an enhanced magnetic field strength. At its interface with the core region, R3, electric field activity ceases abruptly. The accelerated plasma flow profile has a catenary shape consisting of beams parallel to the field in R2 close to the R2/R3 boundary and slower jets moving across the magnetic field within the bulge region. We detail commonalities our observations of crater FTEs have with reconnection structures in other scenarios. We suggest that in view of these properties and their frequency of occurrence, crater FTEs are ideal places to study processes at the separatrices, key regions in magnetic reconnection. This is a good preparation for the MMS mission.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Magnetic storms and substorms (4305 7954) Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2011JGRA..116.2204F}
}

@Article{Fazakerley1995,
  Title                    = {Observations of upstream ions, solar wind ions and electromagnetic waves in the {Earth}'s foreshock},
  Author                   = {Fazakerley, AN and Coates, AJ and Dunlop, MW},
  Journal                  = {Advances in Space Research},
  Year                     = {1995},
  Number                   = {8},
  Pages                    = {103--106},
  Volume                   = {15}
}

@Article{Fear2010,
  Title                    = {Asymmetry in the bipolar signatures of flux transfer events},
  Author                   = {Fear, R. C. and Milan, S. E. and Raeder, J. and Sibeck, D. G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2010},
  Pages                    = {11217},
  Volume                   = {115},

  Abstract                 = {Several conceptual models have been proposed for the formation of flux transfer events (FTEs), including models based on reconnection at a single reconnection line (X line) and at multiple X lines. Two-dimensional magnetohydrodynamic models have previously been used to simulate both scenarios and have found a tendency for FTEs generated by single X line reconnection to exhibit an asymmetry in the bipolar B{\textless}SUB{\textgreater}N{\textless}/SUB{\textgreater} signature that is the major in situ signature of FTE structures, with the leading peak being substantially smaller than the trailing peak. On the other hand, simulated FTEs generated by multiple X line reconnection led to more symmetric signatures. We present a comparison of these simulation results with observations made at the Earth's magnetopause by the Cluster spacecraft, using a data set of 213 FTEs which were observed by all four spacecraft in 2002/2003 at the high-latitude magnetopause near local noon and at low latitudes on the flanks, and 36 FTEs which were observed by one or more Cluster spacecraft near the subsolar point in 2007 and 2008. A tendency is found for the B{\textless}SUB{\textgreater}N{\textless}/SUB{\textgreater} signatures to be asymmetric but with the leading peak larger in amplitude than the trailing peak, opposite to the prediction made by the 2-D single X line simulations. This tendency is weaker in the subsolar FTEs. Therefore, the observations are not consistent with 2-D MHD simulations of single X line reconnection. The signatures observed near the subsolar point are more consistent with those predicted by 2-D simulations of multiple X line reconnection, although the multiple X line simulation studies did not report any net asymmetry. We propose that the observed asymmetry can be explained by a compression of magnetic flux ahead of the propagating FTE structure and a rarefaction behind it. The weaker tendency nearer the subsolar point is consistent with a weaker compression and rarefaction due to lower FTE velocities.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Magnetosphere: outer flux transfer event magnetic reconnection magnetopause},
  Url                      = {http://adsabs.harvard.edu/abs/2010JGRA..11511217F}
}

@Article{Feldman1996,
  Title                    = {{HST} {Observation} of {Mg} $^{\textrm{+\$}}$\$in {Outburst} from {Comet} {D}/{Shoemaker}-{Levy} 9},
  Author                   = {Feldman, P. D. and Weaver, H. A. and Boice, D. C. and Stern, S. A.},
  Journal                  = {ƒ±carus},
  Year                     = {1996},

  Month                    = jun,
  Pages                    = {442--449},
  Volume                   = {121},

  Doi                      = {10.1006/icar.1996.0099}
}

@Article{Feldman1998,
  Title                    = {{FIP} {Effect} in the {Solar} {Upper} {Atmosphere}: {Spectroscopic} {Results}},
  Author                   = {Feldman, U.},
  Journal                  = {ßr},
  Year                     = {1998},

  Month                    = may,
  Pages                    = {227--240},
  Volume                   = {85},

  Doi                      = {10.1023/A:1005146332450},
  Keywords                 = {Solar Wind, sun}
}

@Article{Feldman2000,
  Title                    = {Element {Abundances} in the {Upper} {Atmospheres} of the {Sun} and {Stars}: {Update} of {Observational} {Results}},
  Author                   = {Feldman, U. and Laming, J. M.},
  Journal                  = {{\textbackslash}physscr},
  Year                     = {2000},

  Month                    = feb,
  Pages                    = {222},
  Volume                   = {61},

  Doi                      = {10.1238/Physica.Regular.061a00222}
}

@Article{Feldman2007,
  Title                    = {Diagnostics of {Suprathermal} {Electrons} in {Active}-{Region} {Plasmas} {Using} {He}-like {UV} {Lines}},
  Author                   = {Feldman, U. and Landi, E. and Doschek, G. A.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2007},

  Month                    = may,
  Pages                    = {1674--1682},
  Volume                   = {660},

  Doi                      = {10.1086/513729},
  Keywords                 = {plasmas, Sun: corona}
}

@Article{Feldman2005,
  Title                    = {On the sources of fast and slow solar wind},
  Author                   = {Feldman, Uri and Landi, E. and Schwadron, Nathan A.},
  Journal                  = {{\textbackslash}jgrs},
  Year                     = {2005},

  Month                    = jul,
  Number                   = {A9},
  Pages                    = {7109--+},
  Volume                   = {110},

  Doi                      = {10.1029/2004JA010918}
}

@Article{Feldman2005a,
  Title                    = {On the sources of fast and slow solar wind},
  Author                   = {Feldman, U. and Landi, E. and Schwadron, N. A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2005},

  Month                    = jul,
  Pages                    = {7109},
  Volume                   = {110},

  Doi                      = {10.1029/2004JA010918},
  Keywords                 = {and Astronomy: Chromosphere, and Astronomy: Corona, and Astronomy: Coronal holes, and Astronomy: Transition region, ASTROPHYSICS, Interplanetary Physics: Solar wind sources, Solar Physics, Solar Wind, solar wind origin}
}

@Article{Feldman2007a,
  Title                    = {Spectroscopic {Measurement} of {Coronal} {Compositions}},
  Author                   = {Feldman, U. and Widing, K. G.},
  Journal                  = {ßr},
  Year                     = {2007},

  Month                    = jun,
  Pages                    = {115--126},
  Volume                   = {130},

  Doi                      = {10.1007/s11214-007-9157-7},
  Keywords                 = {Solar Wind, sun}
}

@Article{Feynman2000,
  Title                    = {On space weather consequences and predictions},
  Author                   = {Feynman, Joan and Gabriel, SB},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2000},
  Number                   = {A5},
  Pages                    = {10543--10564},
  Volume                   = {105},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/1999JA000141/full}
}

@Article{Fidell1970,
  Title                    = {Sensory {Function} in {Multimodal} {Signal} {Detection}},
  Author                   = {Fidell, S.},
  Journal                  = {Acoustical Society of America Journal},
  Year                     = {1970},
  Pages                    = {1009},
  Volume                   = {47},

  Doi                      = {10.1121/1.1912000}
}

@Article{Filbert1979,
  Title                    = {Electrostatic noise at the plasma frequency beyond the earth's bow shock},
  Author                   = {Filbert, P. C. and Kellogg, P. J.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1979},

  Month                    = apr,
  Pages                    = {1369--1381},
  Volume                   = {84},

  Doi                      = {10.1029/JA084iA04p01369},
  Keywords                 = {Bow Waves, Cosmic Noise, Earth (Planet), Electrostatic Waves, High Energy Electrons, Interplanetary Magnetic Fields, Plasma Frequencies, shock waves, Solar Wind}
}

@Article{Filbert1979a,
  Title                    = {Electrostatic noise at the plasma frequency beyond the {Earth}'s bow shock},
  Author                   = {Filbert, Paul C and Kellogg, Paul J},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1979},
  Number                   = {A4},
  Pages                    = {1369--1381},
  Volume                   = {84}
}

@Article{Fishman2008,
  Title                    = {Remote sensing of tropospheric pollution from space},
  Author                   = {Fishman, Jack and Al-Saadi, Jassim A. and Creilson, John K. and Bowman, Kevin W. and Burrows, John P. and Richter, Andreas and Chance, Kelly V. and Edwards, David P. and Martin, Randall V. and Morris, Gary A. and {others}},
  Journal                  = {Bull. Amer. Meteor. Soc.},
  Year                     = {2008},
  Number                   = {6},
  Pages                    = {805--821},
  Volume                   = {89},

  Url                      = {http://journals.ametsoc.org/doi/abs/10.1175/2008BAMS2526.1},
  Urldate                  = {2014-11-13}
}

@Article{Fishman2012,
  Title                    = {The {United} {States}' next generation of atmospheric composition and coastal ecosystem measurements: {NASA}'s {Geostationary} {Coastal} and {Air} {Pollution} {Events} ({GEO}-{CAPE}) {Mission}},
  Author                   = {Fishman, J. and Iraci, L. T. and Al-Saadi, J. and Chance, K. and Chavez, Francisco and Chin, M. and Coble, P. and Davis, C. and DiGiacomo, P. M. and Edwards, D. and {others}},
  Journal                  = {Bull. Amer. Meteor. Soc.},
  Year                     = {2012},
  Number                   = {10},
  Pages                    = {1547--1566},
  Volume                   = {93},

  Shorttitle               = {The {United} {States}' next generation of atmospheric composition and coastal ecosystem measurements},
  Url                      = {http://journals.ametsoc.org/doi/abs/10.1175/BAMS-D-11-00201.1},
  Urldate                  = {2014-11-13}
}

@Article{Fisk2003,
  Title                    = {Acceleration of the solar wind as a result of the reconnection of open magnetic flux with coronal loops},
  Author                   = {Fisk, L. A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2003},

  Month                    = apr,
  Pages                    = {1157},
  Volume                   = {108},

  Doi                      = {10.1029/2002JA009284},
  Keywords                 = {and Astronomy: Corona, ASTROPHYSICS, coronal loops, Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Sources of the solar wind, reconnection, Solar Physics, Solar Wind, solar wind charge states, Space Plasma Physics: Magnetic reconnection}
}

@Article{Fisk2001,
  Title                    = {Origin of the {Solar} {Wind}: {Theory}},
  Author                   = {Fisk, L. A. and Schwadron, N. A.},
  Journal                  = {ßr},
  Year                     = {2001},

  Month                    = may,
  Pages                    = {21--33},
  Volume                   = {97}
}

@Article{Fisk1999,
  Title                    = {Acceleration of the fast solar wind by the emergence of new magnetic flux},
  Author                   = {Fisk, L. A. and Schwadron, N. A. and Zurbuchen, T. H.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1999},

  Month                    = sep,
  Pages                    = {19765--19772},
  Volume                   = {104},

  Doi                      = {10.1029/1999JA900256},
  Keywords                 = {Interplanetary Physics: MHD waves and turbulence, Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Sources of the solar wind}
}

@Article{Fisk1998,
  Title                    = {On the {Slow} {Solar} {Wind}},
  Author                   = {Fisk, Lennard A. and Schwadron, Nathan A. and Zurbuchen, Thomas H.},
  Journal                  = {ßr},
  Year                     = {1998},

  Month                    = jul,
  Pages                    = {51--60},
  Volume                   = {86},

  Doi                      = {10.1023/A:1005015527146}
}

@Article{Fisk1999a,
  Title                    = {Coronal {Hole} {Boundaries} and their {Interactions} with {Adjacent} {Regions}},
  Author                   = {Fisk, Lennard A. and Zurbuchen, Thomas H. and Schwadron, Nathan A.},
  Journal                  = {ßr},
  Year                     = {1999},

  Month                    = jan,
  Pages                    = {43--54},
  Volume                   = {87},

  Doi                      = {10.1023/A:1005153730158},
  Keywords                 = {Coronal holes, Solar Wind, Ulysses}
}

@Article{Fitzenreiter1984,
  Title                    = {Detection of bump-on-tail reduced electron velocity distributions at the electron foreshock boundary},
  Author                   = {Fitzenreiter, R. J. and Klimas, A. J. and Scudder, J. D.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {1984},

  Month                    = may,
  Pages                    = {496--499},
  Volume                   = {11},

  Doi                      = {10.1029/GL011i005p00496},
  Keywords                 = {Boundaries, Earth Magnetosphere, Electron Beams, Electron Energy, International Sun Earth Explorer 1, Magnetic Fields, Magnetohydrodynamic Stability, Plasma Waves, Shock Layers, Solar Wind, Velocity Distribution}
}

@Article{Fitzenreiter1984a,
  Title                    = {Detection of bump-on-tail reduced electron velocity distributions at the electron foreshock boundary},
  Author                   = {Fitzenreiter, Richard J and Klimas, Alexander J and Scudder, Jack D},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1984},
  Number                   = {5},
  Pages                    = {496--499},
  Volume                   = {11}
}

@InProceedings{Fontaine2015,
  Title                    = {Multipoint observations and simulation of the effects of {Earth}'s bow shock on magnetic clouds' structure and geoeffectiveness},
  Author                   = {Fontaine, Dominique and Turc, Lucile and Savoini, Philippe},
  Booktitle                = {{EGU} {General} {Assembly} {Conference} {Abstracts}},
  Year                     = {2015},
  Pages                    = {5908},
  Volume                   = {17},

  File                     = {Snapshot:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/T9I3CGF2/2015EGUGA..17.html:text/html},
  Url                      = {http://adsabs.harvard.edu/abs/2015EGUGA..17.5908F},
  Urldate                  = {2016-01-11}
}

@Article{Forbes1984,
  Title                    = {Astrophysical {Plasmas}. ({Book} {Reviews}: {Magnetic} {Reconnection} in {Space} and {Laboratory} {Plasmas})},
  Author                   = {Forbes, T. G.},
  Journal                  = {Science},
  Year                     = {1984},

  Month                    = dec,
  Pages                    = {1311},
  Volume                   = {226},

  Abstract                 = {Not Available}
}

@Article{Formats2014,
  Title                    = {Journal of {Geophysical} {Research} {Space} {Physics}},
  Author                   = {Formats, Ff},
  Journal                  = {Ann Arbor},
  Year                     = {2014},
  Pages                    = {751--760},

  Doi                      = {10.1002/2013JA019193.Received},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1002/jgra.50671/abstract}
}

@Article{Formisano1982,
  Title                    = {Measurement of the potential drop across the earth's collisionless bow shock},
  Author                   = {Formisano, V},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1982},
  Number                   = {9},
  Pages                    = {1033--1036},
  Volume                   = {9}
}

@Article{Formisano1979,
  Title                    = {Orientation and shape of the {Earth}'s bow shock in three dimensions},
  Author                   = {Formisano, V},
  Journal                  = {Planetary and Space Science},
  Year                     = {1979},
  Number                   = {9},
  Pages                    = {1151--1161},
  Volume                   = {27}
}

@Article{Formisano1971,
  Title                    = {Observations of {Earth}'s bow shock for low {Mach} numbers},
  Author                   = {Formisano, V and Hedgecock, PC and Moreno, G and Sear, J and Bollea, D},
  Journal                  = {Planetary and Space Science},
  Year                     = {1971},
  Number                   = {11},
  Pages                    = {1519--1531},
  Volume                   = {19}
}

@Article{Forslund1985,
  Title                    = {Fundamentals of plasma simulation},
  Author                   = {Forslund, David W},
  Journal                  = {Space Science Reviews},
  Year                     = {1985},
  Number                   = {1-2},
  Pages                    = {3--16},
  Volume                   = {42}
}

@Article{Fossati2010,
  Title                    = {Metals in the {Exosphere} of the {Highly} {Irradiated} {Planet} {WASP}-12b},
  Author                   = {Fossati, L. and Haswell, C. A. and Froning, C. S. and Hebb, L. and Holmes, S. and Kolb, U. and Helling, C. and Carter, A. and Wheatley, P. and Collier Cameron, A. and Loeillet, B. and Pollacco, D. and Street, R. and Stempels, H. C. and Simpson, E. and Udry, S. and Joshi, Y. C. and West, R. G. and Skillen, I. and Wilson, D.},
  Journal                  = {{\textbackslash}textbackslashapjl},
  Year                     = {2010},

  Month                    = may,
  Pages                    = {L222--L227},
  Volume                   = {714},

  Doi                      = {10.1088/2041-8205/714/2/L222},
  Keywords                 = {stars: individual: WASP-12}
}

@Article{Foster2014,
  Title                    = {{Storm time observations of plasmasphere erosion flux in the magnetosphere and ionosphere}},
  Author                   = {Foster, J. C. and Erickson, P. J. and Coster, A. J. and Thaller, S. and Tao, J. and Wygant, J. R. and Bonnell, J. W.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2014},
  Number                   = {3},
  Volume                   = {41},

  __markedentry            = {[suleimanbaraka:]},
  Doi                      = {10.1002/2013GL059124},
  ISSN                     = {19448007},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Foullon2007,
  Title                    = {Multi-{Spacecraft} {Study} of the 21 {January} 2005 {ICME}. {Evidence} of {Current} {Sheet} {Substructure} {Near} the {Periphery} of a {Strongly} {Expanding}, {Fast} {Magnetic} {Cloud}},
  Author                   = {Foullon, C. and Owen, C. J. and Dasso, S. and Green, L. M. and Dandouras, I. and Elliott, H. A. and Fazakerley, A. N. and Bogdanova, Y. V. and Crooker, N. U.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {2007},

  Month                    = aug,
  Pages                    = {139--165},
  Volume                   = {244},

  Doi                      = {10.1007/s11207-007-0355-y}
}

@Article{Friedman1981,
  Title                    = {A direct method for implicit particle-in-cell simulation},
  Author                   = {Friedman, A and Langdon, AB and Cohen, BI},
  Year                     = {1981}
}

@Article{Fu2012,
  Title                    = {Electric structure of dipolarization front at sub-proton scale},
  Author                   = {Fu, Huishan S and Khotyaintsev, Yuri V and Vaivads, Andris and André, Mats and Huang, SY},
  Journal                  = {Geophysical Research Letters},
  Year                     = {2012},
  Number                   = {6},
  Volume                   = {39}
}

@Article{Fu2009,
  Title                    = {{GEOPHYSICS}, {ASTRONOMY}, {AND} {ASTROPHYSICS}: {ULF} {Waves} {Associated} with {Solar} {Wind} {Deceleration} in the {Earth}'s {Foreshock}},
  Author                   = {Fu, H.-S. and Cao, J.-B. and Yang, B. and Lucek, E. and Rème, H. and Dandouras, I.},
  Journal                  = {Chinese Physics Letters},
  Year                     = {2009},

  Month                    = nov,
  Number                   = {11},
  Pages                    = {119402},
  Volume                   = {26},

  Doi                      = {10.1088/0256-307X/26/11/119402}
}

@Article{Fujimoto2012,
  Title                    = {Plasmoid-induced turbulence in collisionless magnetic reconnection},
  Author                   = {Fujimoto, Keizo and Sydora, Richard D.},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2012},
  Number                   = {26},
  Pages                    = {265004},
  Volume                   = {109},

  Url                      = {http://prl.aps.org/abstract/PRL/v109/i26/e265004},
  Urldate                  = {2014-05-31}
}

@Article{Fuselier1995,
  Title                    = {Ion distributions in the {Earth}'s foreshock upstream from the bow shock},
  Author                   = {Fuselier, SA},
  Journal                  = {Advances in Space Research},
  Year                     = {1995},
  Number                   = {8},
  Pages                    = {43--52},
  Volume                   = {15}
}

@Article{Fuselier1994,
  Title                    = {Suprathermal ions upstream and downstream from the {Earth}'s bow shock},
  Author                   = {Fuselier, Stephen A},
  Journal                  = {Solar wind sources of magnetospheric ultra-low-frequency waves},
  Year                     = {1994},
  Pages                    = {107--119}
}

@Article{Fuselier1984,
  Title                    = {Short wavelength ion waves upstream of the {Earth}'s bow shock},
  Author                   = {Fuselier, Stephen A and Gurnett, DA},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1984},
  Number                   = {A1},
  Pages                    = {91--103},
  Volume                   = {89}
}

@Article{Fuselier1985,
  Title                    = {The downshift of electron plasma oscillations in the electron foreshock region},
  Author                   = {Fuselier, Stephen A and Gurnett, Donald A and Fitzenreiter, RJ},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1985},
  Number                   = {A5},
  Pages                    = {3935--3946},
  Volume                   = {90}
}

@Article{Fuselier2012,
  Title                    = {Dayside magnetic topology at the {Earth}'s magnetopause for northward {IMF}},
  Author                   = {Fuselier, S. A. and Trattner, K. J. and Petrinec, S. M. and Lavraud, B.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2012},

  Month                    = aug,
  Pages                    = {8235},
  Volume                   = {117},

  Doi                      = {10.1029/2012JA017852},
  Keywords                 = {7526), 7835), Magnetospheric Physics: Cusp, Magnetospheric Physics: Magnetic reconnection (7526, Magnetospheric Physics: Magnetopause and boundary layers, Space Plasma Physics: Magnetic reconnection (2723, Space Plasma Physics: Particle acceleration}
}

@Article{Fuselier2009,
  Title                    = {Width and variation of the {ENA} flux ribbon observed by the {Interstellar} {Boundary} {Explorer}},
  Author                   = {Fuselier, SA and Allegrini, F and Funsten, HO and Ghielmetti, AG and Heirtzler, D and Kucharek, H and Lennartsson, OW and McComas, DJ and Möbius, E and Moore, TE and {others}},
  Journal                  = {Science},
  Year                     = {2009},
  Number                   = {5955},
  Pages                    = {962--964},
  Volume                   = {326}
}

@Article{Fuselier1997,
  Title                    = {Electron and ion signatures of field line topology at the low-shear magnetopause},
  Author                   = {Fuselier, SA and Anderson, BJ and Onsager, TG},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1997},
  Number                   = {A3},
  Pages                    = {4847--4863},
  Volume                   = {102}
}

@Article{Fuselier1995a,
  Title                    = {Particle signatures of magnetic topology at the magnetopause: {AMPTE}/{CCE} observations},
  Author                   = {Fuselier, SA and Anderson, BJ and Onsager, TG},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1995},
  Number                   = {A7},
  Pages                    = {11805--11821},
  Volume                   = {100}
}

@Article{Fuselier1991,
  Title                    = {Ion reflection and transmission during reconnection at the {Earth}'s subsolar magnetopause},
  Author                   = {Fuselier, SA and Klumpar, DM and Shelley, EG},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1991},
  Number                   = {2},
  Pages                    = {139--142},
  Volume                   = {18}
}

@Article{Fuselier2011,
  Title                    = {Properties of near-{Earth} magnetic reconnection from in-situ observations},
  Author                   = {Fuselier, SA and Lewis, WS},
  Journal                  = {Space science reviews},
  Year                     = {2011},
  Number                   = {1-4},
  Pages                    = {95--121},
  Volume                   = {160}
}

@Article{Fuselier1986,
  Title                    = {Gyrating and intermediate ion distributions upstream from the {Earth}'s bow shock},
  Author                   = {Fuselier, SA and Thomsen, MF and Gosling, JT and Bame, SJ and Russell, CT},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1986},
  Number                   = {A1},
  Pages                    = {91--99},
  Volume                   = {91}
}

@Article{Fuselier1995b,
  Title                    = {Suprathermal {He}2+ in the {Earth}'s foreshock region},
  Author                   = {Fuselier, SA and Thomsen, MF and Ipavich, FM and Schmidt, WKH},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1995},
  Number                   = {A9},
  Pages                    = {17107--17116},
  Volume                   = {100}
}

@Article{Gaimard1998,
  Title                    = {On the improvement of analytical calculations of collisional auroral ion velocity distributions using recent {Monte} {Carlo} results},
  Author                   = {Gaimard, P and St-Maurice, J-P and Lathuillere, C and Hubert, D},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1998},
  Number                   = {A3},
  Pages                    = {4079--4095},
  Volume                   = {103}
}

@Article{Galsgaard2000,
  Title                    = {Dynamical investigation of three-dimensional reconnection in quasi-separatrix layers in a boundary-driven magnetic field},
  Author                   = {Galsgaard, Klaus},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2000},
  Number                   = {A3},
  Pages                    = {5119--5134},
  Volume                   = {105}
}

@Article{Gardner2002,
  Title                    = {{UV} radiometric calibration of {UVCS}},
  Author                   = {Gardner, LARRY D and Smith, PETER L and Kohl, JOHN L and ATKINS, NIGEL and CIARAVELLA, ANGELA and MIRALLES, MARI PAZ and PANASYUK, ALEXANDER and RAYMOND, JOHN C and STRACHAN JR, LEONARD and SULEIMAN, RAID M and {others}},
  Journal                  = {The Radiometric Calibration of SOHO},
  Year                     = {2002},
  Pages                    = {161--180}
}

@Article{Gargate2012,
  Title                    = {{Ion Acceleration in Non-Relativistic Astrophysical Shocks}},
  Author                   = {Gargat{\'{e}}, L. and Spitkovsky, a.},
  Journal                  = {Astrophys. J.},
  Year                     = {2012},

  Month                    = {jan},
  Number                   = {1},
  Pages                    = {67},
  Volume                   = {744},

  __markedentry            = {[suleimanbaraka:6]},
  Doi                      = {10.1088/0004-637X/744/1/67},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Gargat{\'{e}}, Spitkovsky/The Astrophysical Journal/Gargat{\'{e}}, Spitkovsky - 2012 - Ion Acceleration in Non-Relativistic Astrophysical Shocks.pdf:pdf},
  ISSN                     = {0004-637X},
  Keywords                 = {color figures,cosmic rays,ism,online-only material,shock waves,supernova remnants},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23},
  Url                      = {http://stacks.iop.org/0004-637X/744/i=1/a=67?key=crossref.6ad2eab41de7e83eb6b3287f10d75eb9}
}

@Article{Geiss1982,
  Title                    = {Processes affecting abundances in the solar wind},
  Author                   = {Geiss, J.},
  Journal                  = {ßr},
  Year                     = {1982},

  Month                    = mar,
  Pages                    = {201--217},
  Volume                   = {33},

  Doi                      = {10.1007/BF00213254},
  Keywords                 = {Abundance, Coronal holes, Cosmochemistry, Fractionation, Helium Isotopes, Hydrogen, Ionization, Solar Corona, Solar Wind}
}

@Article{Geiss1995,
  Title                    = {Origin of the {Solar} {Wind} {From} {Composition} {Data}},
  Author                   = {Geiss, Johannes and Gloeckler, George and von Steiger, Rudolf},
  Journal                  = {ßr},
  Year                     = {1995},

  Month                    = apr,
  Pages                    = {49--60},
  Volume                   = {72},

  Doi                      = {10.1007/BF00768753}
}

@Article{Genestre,
  Title                    = {Empirical modeling of magnetotail reconnec1on},
  Author                   = {Genestre-, Kevin J and Fuselier, Stephen A and Goldstein, Jerry and Nagai, Tsugunobu and Eastwood, Jonathan P},
  Pages                    = {10000},

  Doi                      = {10.1002/2013JA019125.0}
}

@Article{Genestreti2014,
  Title                    = {The location and rate of occurrence of near-{Earth} magnetotail reconnection as observed by {Cluster} and {Geotail}},
  Author                   = {Genestreti, K.J. and Fuselier, S.a. and Goldstein, J. and Nagai, T. and Eastwood, J.P.},
  Journal                  = {J. Atmos. Solar-Terrestrial Phys.},
  Year                     = {2014},
  Pages                    = {98--109},
  Volume                   = {121},

  Doi                      = {10.1016/j.jastp.2014.10.005},
  ISSN                     = {13646826},
  Keywords                 = {Magnetic reconnection, magnetotail, MMS},
  Url                      = {http://linkinghub.elsevier.com/retrieve/pii/S1364682614002338}
}

@Article{Gershman1978,
  Title                    = {Applicability of the electrostatic approach to the analysis of the penetration of electric fields in the near-earth plasma along geomagnetic lines of force},
  Author                   = {Gershman, B. N. and Samsonov, A. V.},
  Journal                  = {Geomagnetism and Aeronomy},
  Year                     = {1978},

  Month                    = dec,
  Pages                    = {503--506},
  Volume                   = {18},

  Keywords                 = {Current Density, Electric Fields, Electrostatics, Geomagnetism, Hall Effect, Ionospheric Disturbances, Lines Of Force, Magnetospheric Instability}
}

@Article{Gershman1971,
  Title                    = {On small-scale electrostatic fields in the ionosphere.},
  Author                   = {Gershman, B. N. and Samsonov, A. V.},
  Journal                  = {Akademiia Nauk SSSR Doklady},
  Year                     = {1971},
  Pages                    = {73--75},
  Volume                   = {199}
}

@Article{Giacalone1992,
  Title                    = {Shock drift acceleration of energetic protons at a planetary bow shock},
  Author                   = {Giacalone, Joe},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1992},
  Number                   = {A6},
  Pages                    = {8307--8318},
  Volume                   = {97}
}

@Article{Giagkiozis2011,
  Title                    = {Dynamics of ion sound waves in the front of the terrestrial bow shock.},
  Author                   = {Giagkiozis, I and Walker, SN and Balikhin, MA},
  Journal                  = {Annales Geophysicae (09927689)},
  Year                     = {2011},
  Number                   = {5},
  Volume                   = {29}
}

@Article{Gibson1998,
  Title                    = {A {Time}-{Dependent} {Three}-{Dimensional} {Magnetohydrodynamic} {Model} of the {Coronal} {Mass} {Ejection}},
  Author                   = {Gibson, S. E. and Low, B. C.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {1998},

  Month                    = jan,
  Pages                    = {460--473},
  Volume                   = {493},

  Doi                      = {10.1086/305107},
  Keywords                 = {Magnetohydrodynamics: MHD, Sun: corona, Sun: Particle Emission}
}

@Article{Giordano2013,
  Title                    = {{UVCS}/{SoHO} catalog of coronal mass ejections from 1996 to 2005: spectroscopic proprieties},
  Author                   = {Giordano, Silvio and Ciaravella, Angela and Raymond, JC and Ko, Y-K and Suleiman, Raid},
  Journal                  = {Journal of Geophysical Research: Space Physics},
  Year                     = {2013},
  Number                   = {3},
  Pages                    = {967--981},
  Volume                   = {118}
}

@Article{Gjerloev2007,
  Title                    = {Observations of {Pi}2 pulsations by the {Wallops} {HF} radar in association with substorm expansion},
  Author                   = {Gjerloev, J. W. and Greenwald, R. A. and Waters, C. L. and Takahashi, K. and Sibeck, D. and Oksavik, K. and Barnes, R. and Baker, J. and Ruohoniemi, J. M.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2007},
  Pages                    = {20103},
  Volume                   = {34},

  Abstract                 = {We report the first sub-auroral Pi2 pulsations observations by a SuperDARN type HF radar. The Wallops radar LOS measurements obtained at ionospheric altitudes, 56° magnetic latitude, 23 hour magnetic local time, are shown to be highly correlated with ground magnetic field perturbations obtained at Ottawa. The period of the Pi2 pulsations is 118 s and the m-number is 2.3. The availability of both ionospheric LOS measurements and ground based magnetic field perturbations enable us to constrain the properties of the wave. A predominantly shear Alfven mode wave is able to explain both the amplitude and phase relations of our observations. Although the solar wind dynamic pressure is fairly stable the IMF Bz is highly variable thereby preventing an unambiguous identification of a solar wind trigger. Rather, magnetotail observations of a clear dipolarization and an intensification of the auroral westward electrojet producing a modest ground magnetic bay indicate that the wave is associated with the onset of a weak substorm.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: MHD waves and instabilities (2149 6050 7836) Ionosphere: Plasma waves and instabilities (2772) Magnetospheric Physics: Substorms Ionosphere: Midlatitude ionosphere Ionosphere: Instruments and techniques},
  Url                      = {http://adsabs.harvard.edu/abs/2007GeoRL..3420103G}
}

@Article{Glassmeier,
  Title                    = {{THEMIS} {ESA} {First} {Science} {Results} and {Performance} {Issues} {JP} {McFadden}, {CW} {Carlson}, {D}. {Larson}, {J}. {Bonnell}, {F}. {Mozer}, {V}. {Angelopoulos}, {K}.-{H}.},
  Author                   = {Glassmeier, U. Auster},

  File                     = {[PDF] from ucla.edu:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/RDA4EP4P/Glassmeier - THEMIS ESA First Science Results and Performance I.pdf:application/pdf},
  Url                      = {http://www-spc.igpp.ucla.edu/personnel/russell/ESS265/McFadden_etal_SSR_ESA_First_Results_submitted.pdf},
  Urldate                  = {2015-12-09}
}

@Article{Gloeckler1998,
  Title                    = {Investigation of the composition of solar and interstellar matter using solar wind and pickup ion measurements with {SWICS} and {SWIMS} on the {ACE} spacecraft},
  Author                   = {Gloeckler, G. and Cain, J. and Ipavich, F. M. and Tums, E. O. and Bedini, P. and Fisk, L. A. and Zurbuchen, T. H. and Bochsler, P. and Fischer, J. and Wimmer-Schweingruber, R. F. and Geiss, J. and Kallenbach, R.},
  Journal                  = {ßr},
  Year                     = {1998},

  Month                    = jul,
  Pages                    = {497--539},
  Volume                   = {86},

  Doi                      = {10.1023/A:1005036131689}
}

@InProceedings{Gloeckler2001,
  Title                    = {Composition of the {Local} {Interstellar} {Cloud} from {Observations} of {Interstellar} {Pickup} {Ions}},
  Author                   = {Gloeckler, George and Geiss, Johannes},
  Booktitle                = {Joint {SOHO}/{ACE} workshop ”{Solar} and {Galactic} {Composition}”},
  Year                     = {2001},
  Editor                   = {Wimmer-Schweingruber, R. F.},
  Pages                    = {281--289},
  Series                   = {American {Institute} of {Physics} {Conference} {Series}},
  Volume                   = {598}
}

@Article{Gloeckler2007,
  Title                    = {The {Composition} of the {Solar} {Wind} in {Polar} {Coronal} {Holes}},
  Author                   = {Gloeckler, G. and Geiss, J.},
  Journal                  = {ßr},
  Year                     = {2007},

  Month                    = jun,
  Pages                    = {139--152},
  Volume                   = {130},

  Doi                      = {10.1007/s11214-007-9189-z},
  Keywords                 = {Sun: elemental composition, Sun: isotopic abundance ratios, Sun: solar wind}
}

@Article{Gloeckler1998a,
  Title                    = {Interstellar and {Inner} {Source} {Pickup} {Ions} {Observed} with {SWICS} on {ULYSSES}},
  Author                   = {Gloeckler, George and Geiss, Johannes},
  Journal                  = {ßr},
  Year                     = {1998},

  Month                    = jul,
  Pages                    = {127--159},
  Volume                   = {86},

  Doi                      = {10.1023/A:1005019628054}
}

@Article{Gloeckler1992,
  Title                    = {The {Solar} {Wind} {Ion} {Composition} {Spectrometer}},
  Author                   = {Gloeckler, G. and Geiss, J. and Balsiger, H. and Bedini, P. and Cain, J. C. and Fischer, J. and Fisk, L. A. and Galvin, A. B. and Gliem, F. and Hamilton, D. C. and Hollweg, J. V. and Ipavich, F. M. and Joos, R. and Livi, S. and Lundgren, R. A. and Mall, U. and McKenzie, J. F. and Ogilvie, K. W. and Ottens, F. and Rieck, W. and Tums, E. O. and von Steiger, R. and Weiss, W. and Wilken, B.},
  Journal                  = {{\textbackslash}aaps},
  Year                     = {1992},

  Month                    = jan,
  Pages                    = {267--289},
  Volume                   = {92},

  Keywords                 = {Hydrogen Ions, INTERPLANETARY MEDIUM, Ion Charge, Ion Temperature, Mass Spectrometers, Metal Ions, Plasma Composition, Satellite-Borne Instruments, Solar Protons, Solar Wind Velocity, Ulysses Mission}
}

@Article{Gloeckler2003,
  Title                    = {Implications of the observed anticorrelation between solar wind speed and coronal electron temperature},
  Author                   = {Gloeckler, George and Zurbuchen, Thomas H. and Geiss, Johannes},
  Journal                  = {{\textbackslash}jgrs},
  Year                     = {2003},

  Month                    = apr,
  Pages                    = {1158--+},
  Volume                   = {108},

  Doi                      = {10.1029/2002JA009286},
  Keywords                 = {Interplanetary Physics: Solar cycle variations (7536), Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Sources of the solar wind, Space Plasma Physics: Magnetic reconnection}
}

@Article{Goldman2011,
  Title                    = {Jet deflection by very weak guide fields during magnetic reconnection},
  Author                   = {Goldman, M. V. and Lapenta, Giovanni and Newman, D. L. and Markidis, Stefano and Che, Haihong},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2011},
  Number                   = {13},
  Pages                    = {135001},
  Volume                   = {107},

  Url                      = {http://prl.aps.org/abstract/PRL/v107/i13/e135001},
  Urldate                  = {2014-05-31}
}

@InProceedings{Goldman2010,
  Title                    = {Bipolar-field electrostatic turbulence during magnetic reconnection},
  Author                   = {Goldman, Martin V. and Newman, David L. and Lapenta, Giovanni and Divin, Andre and Markidis, Stefano and Che, Haihong},
  Booktitle                = {{EGU} {General} {Assembly} {Conference} {Abstracts}},
  Year                     = {2010},
  Pages                    = {6173},
  Volume                   = {12},

  Url                      = {http://adsabs.harvard.edu/abs/2010EGUGA..12.6173G},
  Urldate                  = {2014-05-31}
}

@Article{Gombosi2000,
  Title                    = {Global {MHD} modeling of space weather},
  Author                   = {Gombosi, TI and Zeeuw, DL De and Groth, CPT},
  Journal                  = {IEEE Trans, Plasma Sci., {\textbackslash}ldots},
  Year                     = {2000},

  Url                      = {http://scholar.google.com/scholar?hl=en&q=T.+I.+Gombosi%2C+D.+L.+De+Zeeuw%2C+C.+P.+T.+Groth%2C+K.+G.+Powell%2C+A.+J.+Ridley%2C+and+P.+Song%2C+%E2%80%9CGlobal+MHD+modeling+of+space+weather%2C%E2%80%9D+IEEE+Trans.+Plasma+Sci.%2C+2000&btnG=&as_sdt=1%2C5&as_sdtp=#0}
}

@Book{Gombosi1998,
  Title                    = {Physics of the {Space} {Environment}},
  Author                   = {Gombosi, Tamas I.},
  Publisher                = {Cambridge University Press},
  Year                     = {1998},

  Address                  = {Cambridge, UK}
}

@Article{Gomez2003,
  Title                    = {Galaxy star formation as a function of environment in the early data release of the sloan digital sky survey},
  Author                   = {Gomez, Percy L and Nichol, Robert C and Miller, Christopher J and Balogh, Michael L and Goto, Tomotsugu and Zabludoff, Ann I and Romer, A Kathy and Bernardi, Mariangela and Sheth, Ravi and Hopkins, Andrew M and {others}},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2003},
  Number                   = {1},
  Pages                    = {210},
  Volume                   = {584}
}

@Article{Gonzalez1994,
  Title                    = {What is a geomagnetic storm?},
  Author                   = {Gonzalez, WD and Joselyn, JA and Kamide, Y and Kroehl, HW and Rostoker, G and Tsurutani, BT and Vasyliunas, VM},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1994},
  Number                   = {A4},
  Pages                    = {5771--5792},
  Volume                   = {99}
}

@Article{Gonzalez2011,
  Title                    = {Preface for the {ILWS} special issue of {JASTP}},
  Author                   = {Gonzalez, Walter D. and Sibeck, David G. and Spann, James F.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2011},
  Pages                    = {1293--1293},
  Volume                   = {73},

  Abstract                 = {Not Available},
  ISSN                     = {1364-6826},
  Url                      = {http://adsabs.harvard.edu/abs/2011JASTP..73.1293G}
}

@Book{Goodman2006,
  Title                    = {Space weather \& telecommunications},
  Author                   = {Goodman, John M},
  Publisher                = {Springer},
  Year                     = {2006},
  Volume                   = {782}
}

@Article{Goodrich1984,
  Title                    = {The adiabatic energy change of plasma electrons and the frame dependence of the cross-shock potential at collisionless magnetosonic shock waves},
  Author                   = {Goodrich, CC and Scudder, JD},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1984},
  Number                   = {A8},
  Pages                    = {6654--6662},
  Volume                   = {89}
}

@Article{Gopalswamy2005,
  Title                    = {Introduction to violent {Sun}-{Earth} connection events of {October}-{November} 2003},
  Author                   = {Gopalswamy, N. and Barbieri, L. and Cliver, E. W. and Lu, G. and Plunkett, S. P. and Skoug, R. M.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2005},

  Month                    = sep,
  Pages                    = {9},
  Volume                   = {110},

  Abstract                 = {The solar-terrestrial events of late October and early November 2003, popularly referred to as the Halloween storms, represent the best observed cases of extreme space weather activity observed to date and have generated research covering multiple aspects of solar eruptions and their space weather effects. In the following article, which serves as an abstract for this collective research, we present highlights taken from 61 of the 74 papers from the Journal of Geophysical Research, Geophysical Research Letters, and Space Weather which are linked under this special issue. (An overview of the 13 associated papers published in Geophysics Research Letters is given in the work of Gopalswamy et al. (2005a)).},
  Doi                      = {10.1029/2005JA011268},
  Keywords                 = {and magnetic clouds, coronal mass ejections, driver gases, geomagnetic storms, Interplanetary Physics: Coronal mass ejections (7513), Interplanetary Physics: Ejecta, Interplanetary Physics: Energetic particles (7514), Interplanetary Physics: Solar wind plasma, interplanetary shocks, Ionosphere: Ionospheric dynamics, solar energetic particles, Solar Flares, superstorms}
}

@Article{Gopalswamy1998,
  Title                    = {On the relationship between coronal mass ejections and magnetic clouds},
  Author                   = {Gopalswamy, N. and Hanaoka, Y. and Kosugi, T. and Lepping, R. P. and Steinberg, J. T. and Plunkett, S. and Howard, R. A. and Thompson, B. J. and Gurman, J. and Ho, G. and Nitta, N. and Hudson, H. S.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {1998},
  Pages                    = {2485--2488},
  Volume                   = {25},

  Doi                      = {10.1029/98GL50757},
  Keywords                 = {and Astronomy, and Astronomy: Coronal holes, and Astronomy: Magnetic fields, and Astronomy: Radio emissions, ASTROPHYSICS, Solar Physics}
}

@Article{Gordon1999,
  Title                    = {Coupled hydromagnetic wave excitation and ion acceleration at interplanetary traveling shocks and {Earth}'s bow shock revisited},
  Author                   = {Gordon, BE and Lee, MA and Möbius, E and Trattner, KJ},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1999},
  Number                   = {A12},
  Pages                    = {28263--28277},
  Volume                   = {104}
}

@Article{Gosling1997,
  Title                    = {Coronal mass ejections: {An} overview},
  Author                   = {Gosling, JT},
  Journal                  = {Geophysical Monograph Series},
  Year                     = {1997},
  Pages                    = {9--16},
  Volume                   = {99}
}

@Article{Gosling1976,
  Title                    = {Solar wind speed variations: 1962–1974},
  Author                   = {Gosling, JT and Asbridge, JR and Bame, SJ and Feldman, WC},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1976},
  Number                   = {28},
  Pages                    = {5061--5070},
  Volume                   = {81}
}

@Article{Gosling1978,
  Title                    = {Observations of two distinct populations of bow shock ions in the upstream solar wind},
  Author                   = {Gosling, JT and Asbridge, JR and Bame, SJ and Paschmann, G and Sckopke, N},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1978},
  Number                   = {11},
  Pages                    = {957--960},
  Volume                   = {5}
}

@Article{Gosling1968,
  Title                    = {Satellite observations of interplanetary shock waves},
  Author                   = {Gosling, JT and Asbridge, JR and Bame, S Jo and Hundhausen, AJ and Strong, IB},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1968},
  Number                   = {1},
  Pages                    = {43--50},
  Volume                   = {73}
}

@Article{Gosling1994,
  Title                    = {The speeds of coronal mass ejections in the solar wind at mid heliographic latitudes: {Ulysses}},
  Author                   = {Gosling, JT and Bame, SJ and McComas, DJ and Phillips, JL and Goldstein, BE and Neugebauer, M},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1994},
  Number                   = {12},
  Pages                    = {1109--1112},
  Volume                   = {21}
}

@Article{Gosling1995,
  Title                    = {Three-dimensional magnetic reconnection and the magnetic topology of coronal mass ejection events},
  Author                   = {Gosling, JT and Birn, J and Hesse, M},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1995},
  Number                   = {8},
  Pages                    = {869--872},
  Volume                   = {22}
}

@Article{Gosling1976a,
  Title                    = {The speeds of coronal mass ejection events},
  Author                   = {Gosling, JT and Hildner, E and MacQueen, RM and Munro, RH and Poland, AI and Ross, CL},
  Journal                  = {Solar Physics},
  Year                     = {1976},
  Number                   = {2},
  Pages                    = {389--397},
  Volume                   = {48}
}

@Article{Gosling1974,
  Title                    = {Mass ejections from the {Sun}: {A} view from {Skylab}},
  Author                   = {Gosling, JT and Hildner, E and MacQueen, RM and Munro, RH and Poland, AI and Ross, CL},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1974},
  Number                   = {31},
  Pages                    = {4581--4587},
  Volume                   = {79}
}

@Article{Gosling1976b,
  Title                    = {Solar wind stream evolution at large heliocentric distances: {Experimental} demonstration and the test of a model},
  Author                   = {Gosling, JT and Hundhausen, AJ and Bame, SJ},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1976},
  Number                   = {13},
  Pages                    = {2111--2122},
  Volume                   = {81}
}

@Article{Gosling1994a,
  Title                    = {A new class of forward-reverse shock pairs in the solar wind},
  Author                   = {Gosling, JT and McComas, DJ and Phillips, JL and Weiss, LA and Pizzo, VJ and Goldstein, BE and Forsyth, RJ},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1994},
  Number                   = {21},
  Pages                    = {2271--2274},
  Volume                   = {21}
}

@Article{Gosling2005,
  Title                    = {Direct evidence for magnetic reconnection in the solar wind near 1 {AU}},
  Author                   = {Gosling, JT and Skoug, RM and McComas, DJ and Smith, CW},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2005},
  Number                   = {A1},
  Volume                   = {110}
}

@Article{Gosling1996,
  Title                    = {Corotating and {Transient} {Solar} {Wind} {Flows} in {Three} {Dimensions}},
  Author                   = {Gosling, J. T.},
  Journal                  = {{\textbackslash}araa},
  Year                     = {1996},
  Pages                    = {35--74},
  Volume                   = {34},

  Abstract                 = {Two types of flows dominate the large-scale structure of the solar wind: corotating flows and transient disturbances. Corotating flows are associated with spatial variability in the coronal expansion and solar rotation, whereas transient disturbances are associated with episodic ejections of material into interplanetary space from coronal regions not previously participating in the solar wind expansion. Ulysses' recent epic journey over the poles of the Sun has provided new insights on the three-dimensional nature of both corotating flows and transient disturbances in the solar wind and their evolution with heliocentric distance and latitude. This paper provides a simple physical description of the origins and dynamics of both of these types of solar wind flows, highlighting new understanding gained from the unique Ulysses high-latitude observations.},
  Doi                      = {10.1146/annurev.astro.34.1.35}
}

@Article{Gosling1990,
  Title                    = {Coronal mass ejections and magnetic flux ropes in interplanetary space},
  Author                   = {Gosling, Jo T},
  Journal                  = {Geophysical Monograph Series},
  Year                     = {1990},
  Pages                    = {343--364},
  Volume                   = {58}
}

@Article{Gosling1990a,
  Title                    = {Coronal mass ejections and magnetic flux ropes in interplanetary space},
  Author                   = {Gosling, Jo T},
  Journal                  = {Physics of Magnetic Flux Ropes},
  Year                     = {1990},
  Pages                    = {343--364}
}

@Article{Gosling1987,
  Title                    = {Bidirectional solar wind electron heat flux events},
  Author                   = {Gosling, John T and Baker, DN and Bame, SJ and Feldman, WC and Zwickl, RD and Smith, EJ},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1987},
  Number                   = {A8},
  Pages                    = {8519--8535},
  Volume                   = {92}
}

@Article{Gosling1995a,
  Title                    = {Three-dimensional magnetic reconnection and the magnetic topology of coronal mass ejection events},
  Author                   = {Gosling, J. T. and Birn, J. and Hesse, M.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {1995},

  Month                    = apr,
  Pages                    = {869--872},
  Volume                   = {22}
}

@Article{Gosling1991,
  Title                    = {Geomagnetic activity associated with earth passage of interplanetary shock disturbances and coronal mass ejections},
  Author                   = {Gosling, J. T. and McComas, D. J. and Phillips, J. L. and Bame, S. J.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1991},

  Month                    = may,
  Pages                    = {7831--7839},
  Volume                   = {96},

  Abstract                 = {Coronal mass ejection events (CMEs) are important occasional sources of plasma and magnetic field in the solar wind at 1 AU, accounting for approximately 10 percent of all solar wind measurements in the ecliptic plane during the last solar activity maximum. Using a recently appreciated capability for distinguishing CMEs in solar wind data in the form of counterstreaming solar wind electron events, this paper explores the overall effectiveness of shock wave disturbances and CMFs in general in stimulating geomagnetic activity. The study is confined to the interval from mid-August 1978 through mid-October 1982, spanning the last solar activity maximum, when ISEE 3 was in orbit about the L1 Lagrange point 220 Re upstream from earth. It is found that all but one of the 37 largest geomagnetic storms in that era were associated with earth passage of CMEs and/or shock disturbances, with the large majority of these storms (27 out of 37) being associated with interplanetary events where earth encountered both a shock and the CME driving the shock (shock/CME events). Although CMEs and/or shock disturbances were increasingly the cause of geomagnetic activity as the level of geomagnetic activity increased, many smaller geomagnetic disturbances were unrelated to these events.},
  Doi                      = {10.1029/91JA00316},
  Keywords                 = {Interplanetary Magnetic Fields, magnetic storms, Magnetoactivity, shock waves, Solar Activity Effects, Solar Corona, Solar Electrons, Solar Wind, Stellar Mass Ejection}
}

@Article{Gosling2008,
  Title                    = {Bifurcated current sheets produced by magnetic reconnection in the solar wind},
  Author                   = {Gosling, J. T. and Szabo, A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2008},

  Month                    = oct,
  Number                   = {A12},
  Pages                    = {10103},
  Volume                   = {113},

  Doi                      = {10.1029/2008JA013473},
  Keywords                 = {7526), and magnetic clouds, bifurcated current sheets, driver gases, Interplanetary Physics: Ejecta, Interplanetary Physics: Interplanetary magnetic fields, Interplanetary Physics: Solar wind plasma, reconnection, Space Plasma Physics: Discontinuities (2109), Space Plasma Physics: Magnetic reconnection (2723}
}

@Article{Gosling1991a,
  Title                    = {Observations of reconnection of interplanetary and lobe magnetic field lines at the high-latitude magnetopause},
  Author                   = {Gosling, J. T. and Thomsen, M. F. and Bame, S. J. and Elphic, R. C. and Russell, C. T.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1991},

  Month                    = aug,
  Pages                    = {14097},
  Volume                   = {96},

  Abstract                 = {Results are presented of ISEE 2 observations of plasma accelerations obtained at the high-latitude (lobe) magnetopause at a time when the local magnetosheath and magnetospheric magnetic fields were nearly oppositely directed and the flow speed in the magnetosheath, V(s), was nearly equal to the local Alfven speed, V(A). The observations provide direct evidence for the rereconnection of the open field lines of the tail lobes with the IMF, when the magnetic field shear is large. It is pointed out, however, that, since V(s) was almost equal to V(A), it is unlikely that the rereconnection is associated with the strong sunward convection in the polar cap.},
  Doi                      = {10.1029/91JA01139},
  Keywords                 = {Geomagnetism, International Sun Earth Explorers, Interplanetary Magnetic Fields, Ion Distribution, Lines Of Force, Magnetic Field Reconnection, Magnetopause, magnetosheath, Plasma Acceleration, Satellite Observation, Solar Terrestrial Interactions}
}

@InProceedings{Granko2012,
  Title                    = {Influence of a quasi-radial {IMF} on the magnetopause position},
  Author                   = {Granko, G. and Safrankova, J. and Nemecek, Z. and Jelinek, K. and Samsonov, A.},
  Booktitle                = {{EGU} {General} {Assembly} {Conference} {Abstracts}},
  Year                     = {2012},
  Editor                   = {Abbasi, A. and Giesen, N.},
  Month                    = apr,
  Pages                    = {1684},
  Series                   = {{EGU} {General} {Assembly} {Conference} {Abstracts}},
  Volume                   = {14}
}

@InProceedings{Granko2013,
  Title                    = {Pressure balance of extreme magnetopause locations},
  Author                   = {Granko, G. and Safrankova, J. and Nemecek, Z. and Jelinek, K. and Samsonov, A.},
  Booktitle                = {{EGU} {General} {Assembly} {Conference} {Abstracts}},
  Year                     = {2013},
  Month                    = apr,
  Pages                    = {5572},
  Series                   = {{EGU} {General} {Assembly} {Conference} {Abstracts}},
  Volume                   = {15}
}

@Article{Grechnev2008,
  Title                    = {An {Extreme} {Solar} {Event} of 20 {January} 2005: {Properties} of the {Flare} and the {Origin} of {Energetic} {Particles}},
  Author                   = {Grechnev, V. V. and Kurt, V. G. and Chertok, I. M. and Uralov, A. M. and Nakajima, H. and Altyntsev, A. T. and Belov, A. V. and Yushkov, B. Y. and Kuznetsov, S. N. and Kashapova, L. K. and Meshalkina, N. S. and Prestage, N. P.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {2008},

  Month                    = oct,
  Pages                    = {149--177},
  Volume                   = {252},

  Doi                      = {10.1007/s11207-008-9245-1},
  Keywords                 = {coronal mass ejections, Cosmic rays, Energetic particles, Flares, Particle Acceleration, Radio bursts, X-ray bursts}
}

@InProceedings{Grevesse2013,
  Title                    = {Why {GN}93 should not be used anymore},
  Author                   = {Grevesse, N. and Asplund, M. and Sauval, J. and Scott, P.},
  Booktitle                = {European {Physical} {Journal} {Web} of {Conferences}},
  Year                     = {2013},
  Month                    = mar,
  Pages                    = {1004},
  Series                   = {European {Physical} {Journal} {Web} of {Conferences}},
  Volume                   = {43},

  Doi                      = {10.1051/epjconf/20134301004}
}

@Article{Grevesse1998,
  Title                    = {Standard {Solar} {Composition}},
  Author                   = {Grevesse, N. and Sauval, A. J.},
  Journal                  = {ßr},
  Year                     = {1998},

  Month                    = may,
  Pages                    = {161--174},
  Volume                   = {85},

  Doi                      = {10.1023/A:1005161325181},
  Keywords                 = {Meteorites: abundances, Solar spectroscopy, Sun: abundances}
}

@Article{Groth2000,
  Title                    = {Global three-dimensional {MHD} simulation of a space weather event: {CME} formation, interplanetary propagation, and interaction with the magnetosphere},
  Author                   = {Groth, Clinton and De Zeeuw, Darren L and Gombosi, Tamas I and Powell, Kenneth G},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2000},
  Number                   = {A11},
  Pages                    = {25053--25078},
  Volume                   = {105}
}

@Article{Gruesbeck2012,
  Title                    = {Two-plasma {Model} for {Low} {Charge} {State} {Interplanetary} {Coronal} {Mass} {Ejection} {Observations}},
  Author                   = {Gruesbeck, J. R. and Lepri, S. T. and Zurbuchen, T. H.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2012},

  Month                    = dec,
  Pages                    = {141},
  Volume                   = {760},

  Doi                      = {10.1088/0004-637X/760/2/141},
  Keywords                 = {Atomic Processes, plasmas, prominences, Solar Wind, Sun: coronal mass ejections: CMEs, Sun: filaments}
}

@Article{Gruesbeck2011,
  Title                    = {Constraints on {Coronal} {Mass} {Ejection} {Evolution} from in {Situ} {Observations} of {Ionic} {Charge} {States}},
  Author                   = {Gruesbeck, J. R. and Lepri, S. T. and Zurbuchen, T. H. and Antiochos, S. K.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2011},

  Month                    = apr,
  Pages                    = {103},
  Volume                   = {730},

  Doi                      = {10.1088/0004-637X/730/2/103},
  Keywords                 = {Atomic Processes, plasmas, Solar Wind, Sun: coronal mass ejections: CMEs}
}

@Article{Gurgiolo1985,
  Title                    = {Comment composition of the polar wind‚Äö√Ñ√∂‚àö√ë‚àö‚Ñ¢not just {H}+ and {He}+},
  Author                   = {Gurgiolo, C and Burch, JL},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1985},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/GL012i001p00069/full}
}

@Article{Gurgiolo1982,
  Title                    = {{DE}-1 observations of the polar {windŸèÿüÔøΩA} heated and an unheated component},
  Author                   = {Gurgiolo, C and Burch, JL},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1982},
  Number                   = {9},
  Pages                    = {945--948},
  Volume                   = {9},

  Annote                   = {Added to JabRef: 2015.04.18}
}

@Book{Gurnett2005,
  Title                    = {Introduction to plasma physics: with space and laboratory applications},
  Author                   = {Gurnett, Donald A and Bhattacharjee, Amitava},
  Publisher                = {Cambridge university press},
  Year                     = {2005}
}

@Article{Gustafsson2001,
  Title                    = {First results of electric field and density observations by {Cluster} {EFW} based on initial months of operation},
  Author                   = {Gustafsson, G. and André, M. and Carozzi, T. and Eriksson, A. I. and Fälthammar, C.-G. and Grard, R. and Holmgren, G. and Holtet, J. A. and Ivchenko, N. and Karlsson, T. and Khotyaintsev, Y. and Klimov, S. and Laakso, H. and Lindqvist, P.-A. and Lybekk, B. and Marklund, G. and Mozer, F. and Mursula, K. and Pedersen, A. and Popielawska, B. and Savin, S. and Stasiewicz, K. and Tanskanen, P. and Vaivads, A. and Wahlund, J.-E.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2001},

  Month                    = oct,
  Pages                    = {1219--1240},
  Volume                   = {19},

  Doi                      = {10.5194/angeo-19-1219-2001}
}

@Article{Gustafsson2001a,
  Title                    = {First results of electric field and density observations by {Cluster} {EFW} based on initial months of operation},
  Author                   = {Gustafsson, G. and Andr√©, M. and Carozzi, T. and Eriksson, A. I. and F√§lthammar, C.-G. and Grard, R. and Holmgren, G. and Holtet, J. A. and Ivchenko, N. and Karlsson, T. and Khotyaintsev, Y. and Klimov, S. and Laakso, H. and Lindqvist, P.-A. and Lybekk, B. and Marklund, G. and Mozer, F. and Mursula, K. and Pedersen, A. and Popielawska, B. and Savin, S. and Stasiewicz, K. and Tanskanen, P. and Vaivads, A. and Wahlund, J.-E.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2001},

  Month                    = oct,
  Pages                    = {1219--1240},
  Volume                   = {19},

  Doi                      = {10.5194/angeo-19-1219-2001}
}

@Article{Guzdar2001,
  Title                    = {Three-dimensional {MHD} simulations of the steady state magnetosphere with northward interplanetary magnetic field},
  Author                   = {Guzdar, PN and Shao, X and Goodrich, CC and Papadopoulos, K and Wiltberger, MJ and Lyon, JG},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2001},
  Number                   = {A1},
  Pages                    = {275--287},
  Volume                   = {106}
}

@Article{Guzewich2013,
  Title                    = {High-altitude dust layers on {Mars}: {Observations} with the {Thermal} {Emission} {Spectrometer}},
  Author                   = {Guzewich, Scott D and Talaat, Elsayed R and Toigo, Anthony D and Waugh, Darryn W and McConnochie, Timothy H},
  Journal                  = {Journal of Geophysical Research: Planets},
  Year                     = {2013},
  Number                   = {6},
  Pages                    = {1177--1194},
  Volume                   = {118}
}

@InProceedings{Haaland2004,
  Title                    = {Four-spacecraft determination of magnetopause orientation, motion and thickness: comparison with results from single-spacecraft methods},
  Author                   = {Haaland, SE and Sonnerup, BU Ö and Dunlop, MW and Balogh, A and Georgescu, E and Hasegawa, H and Klecker, B and Paschmann, G and Puhl-Quinn, P and Reme, H and {others}},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2004},
  Pages                    = {1347--1365},
  Volume                   = {22}
}

@Article{Habbal2011,
  Title                    = {Thermodynamics of the {Solar} {Corona} and {Evolution} of the {Solar} {Magnetic} {Field} as {Inferred} from the {Total} {Solar} {Eclipse} {Observations} of 2010 {July} 11},
  Author                   = {Habbal, S. R. and Druckmüller, M. and Morgan, H. and Ding, A. and Johnson, J. and Druckmüllerová, H. and Daw, A. and Arndt, M. B. and Dietzel, M. and Saken, J.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2011},

  Month                    = jun,
  Pages                    = {120},
  Volume                   = {734},

  Doi                      = {10.1088/0004-637X/734/2/120},
  Keywords                 = {eclipses, Solar Wind, Sun: corona}
}

@Article{,
  Title                    = {Shock front nonstationarity of supercritical perpendicular shocks},
  Author                   = {Hada, Tohru and Oonishi, Makiko and Lembège, Bertrand and Savoini, Philippe},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2003},
  Number                   = {A6},
  Volume                   = {108}
}

@Article{Halekas2011,
  Title                    = {First {Results} from {ARTEMIS}, a {New} {Two}-{Spacecraft} {Lunar} {Mission}: {Counter}-{Streaming} {Plasma} {Populations} in the {Lunar} {Wake}},
  Author                   = {Halekas, J. S. and Angelopoulos, V. and Sibeck, D. G. and Khurana, K. K. and Russell, C. T. and Delory, G. T. and Farrell, W. M. and McFadden, J. P. and Bonnell, J. W. and Larson, D. and Ergun, R. E. and Plaschke, F. and Glassmeier, K. H.},
  Journal                  = {Space Science Reviews},
  Year                     = {2011},
  Pages                    = {93--107},
  Volume                   = {165},

  Abstract                 = {We present observations from the first passage through the lunar plasma wake by one of two spacecraft comprising ARTEMIS (Acceleration, Reconnection, Turbulence, and Electrodynamics of the Moon's Interaction with the Sun), a new lunar mission that re-tasks two of five probes from the THEMIS magnetospheric mission. On Feb 13, 2010, ARTEMIS probe P1 passed through the wake at ˜3.5 lunar radii downstream from the Moon, in a region between those explored by Wind and the Lunar Prospector, Kaguya, Chandrayaan, and Chang'E missions. ARTEMIS observed interpenetrating proton, alpha particle, and electron populations refilling the wake along magnetic field lines from both flanks. The characteristics of these distributions match expectations from self-similar models of plasma expansion into vacuum, with an asymmetric character likely driven by a combination of a tilted interplanetary magnetic field and an anisotropic incident solar wind electron population. On this flyby, ARTEMIS provided unprecedented measurements of the interpenetrating beams of both electrons and ions naturally produced by the filtration and acceleration effects of electric fields set up during the refilling process. ARTEMIS also measured electrostatic oscillations closely correlated with counter-streaming electron beams in the wake, as previously hypothesized but never before directly measured. These observations demonstrate the capability of the comprehensively instrumented ARTEMIS spacecraft and the potential for new lunar science from this unique two spacecraft constellation.},
  ISSN                     = {0038-6308},
  Keywords                 = {Moon Lunar wake Counter-streaming distributions},
  Url                      = {http://adsabs.harvard.edu/abs/2011SSRv..165...93H}
}

@Article{Hall1991,
  Title                    = {Electrons in the boundary layers near the dayside magnetopause},
  Author                   = {Hall, Donald Sydney and Chaloner, CP and Bryant, DA and Lepine, DR and Tritakis, VP},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1991},
  Number                   = {A5},
  Pages                    = {7869--7891},
  Volume                   = {96}
}

@Article{Hall1991a,
  Title                    = {Electrons in the boundary layers near the dayside magnetopause},
  Author                   = {Hall, D. S. and Chaloner, C. P. and Bryant, D. A. and Lepine, D. R. and Tritakis, V. P.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1991},

  Month                    = may,
  Pages                    = {7869--7891},
  Volume                   = {96},

  Abstract                 = {Entry of heated solar wind plasma into the magnetosphere is examined using electron distributions measured by AMPTE UKS and HEOS 2. In particular, the angular structure of the electron distributions is studied within the transition region separating the magnetosheath from the inner magnetosphere. The measurements suggest that electrons in the outer part of the transition region originate in the magnetosheath, while the population closer to the earth consists of electrons from the magnetosphere combined with an energized magnetosheath component. This energized component contains 'counterstreaming' electrons, which are confirmed to directions closely parallel and antiparallel to the magnetic field direction. The possibilities, that the energization of the counterstreaming electrons is cumulatively gained from either waves, electric fields perpendicular to the magnetic field, or quasi-Fermi acceleration, are discussed. It is not possible to identify the topology of the magnetic fields of the outer part of the region, but there is strong evidence that the inner part is on closed magnetic field lines, which map to the dayside auroal zone. The outer part of the transition region is a plasma depletion/magnetic field compression layer. The structure of the transition region is smaller to that surrounding flux transfer events, which leads to the deduction that the plasma and field signatures of flux transfer events may be the result of displacement of the transition region earthward. Cases where the displacement is such that the field maximum of the depletion/compression region is encountered may well explain 'crater' flux transfer event signatures.},
  Doi                      = {10.1029/90JA02137},
  Keywords                 = {Ampte (Satellites), Atmospheric Boundary Layer, Daytime, Heos Satellites, Magnetopause, Magnetospheric Electron Density, Solar Wind}
}

@Article{Hamza2011,
  Title                    = {On turbulence in the quasi-perpendicular bow shock},
  Author                   = {Hamza, AM and Meziane, K},
  Journal                  = {Planetary and Space Science},
  Year                     = {2011},
  Number                   = {7},
  Pages                    = {475--481},
  Volume                   = {59}
}

@Article{Hamza2006,
  Title                    = {Oblique propagation and nonlinear wave particle processes},
  Author                   = {Hamza, AM and Meziane, K and Mazelle, C},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2006},
  Number                   = {A4},
  Volume                   = {111}
}

@Article{Hamza2011a,
  Title                    = {On turbulence in the quasi-perpendicular bow shock},
  Author                   = {Hamza, A. M. and Meziane, K.},
  Journal                  = {{\textbackslash}planss},
  Year                     = {2011},

  Month                    = may,
  Pages                    = {475--481},
  Volume                   = {59},

  Doi                      = {10.1016/j.pss.2010.03.013}
}

@Article{Hamza2014,
  Title                    = {Relaxation currents in poly-4-vinylphenol dielectrics: {Trapping} and macroscopic polarization},
  Author                   = {Hamza, A. M. and Myung-Whun, K. and Bu, S. D. and Seo, J. M. and Lee, J.-K.},
  Journal                  = {Thin Solid Films},
  Year                     = {2014},

  Month                    = jan,
  Pages                    = {710--714},
  Volume                   = {550},

  Doi                      = {10.1016/j.tsf.2013.10.042}
}

@Book{Hanslmeier2010,
  Title                    = {The sun and space weather},
  Author                   = {Hanslmeier, Arnold},
  Publisher                = {Springer},
  Year                     = {2010}
}

@Article{Hansteen1995,
  Title                    = {Coronal heating, densities, and temperatures and solar wind acceleration},
  Author                   = {Hansteen, V. H. and Leer, E.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1995},

  Month                    = nov,
  Pages                    = {21577--21594},
  Volume                   = {100},

  Doi                      = {10.1029/95JA02300},
  Keywords                 = {and Astronomy, and Astronomy: Chromosphere, and Astronomy: Corona, ASTROPHYSICS, Solar Physics}
}

@Article{Hardee2014,
  Title                    = {Radiation from {Particles} {Accelerated} in {Relativistic} {Jet} {Shocks} and {Shear}-flows},
  Author                   = {Hardee, P},
  Year                     = {2014},
  Pages                    = {20--24}
}

@Article{Harnett2003,
  Title                    = {2.5-{D} fluid simulations of the solar wind interacting with multiple dipoles on the surface of the {Moon}},
  Author                   = {Harnett, Erika M and Winglee, Robert M},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2003},
  Number                   = {A2},
  Volume                   = {108}
}

@Article{Hartinger2013,
  Title                    = {The role of transient ion foreshock phenomena in driving {Pc}5 {ULF} wave activity},
  Author                   = {Hartinger, M. D. and Turner, D. L. and Plaschke, F. and Angelopoulos, V. and Singer, H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = jan,
  Pages                    = {299--312},
  Volume                   = {118},

  Doi                      = {10.1029/2012JA018349},
  Keywords                 = {cone angle, foreshock bubble, ion foreshock, Kelvin-Helmholtz instability, Pc5, ULF}
}

@Article{Hasegawa2006,
  Title                    = {Single-spacecraft detection of rolled-up {Kelvin}-{Helmholtz} vortices at the flank magnetopause},
  Author                   = {Hasegawa, H and Fujimoto, M and Takagi, K and Saito, Y and Mukai, T and Rème, H},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2006},
  Number                   = {A9},
  Volume                   = {111}
}

@Article{Hasegawa2015,
  Title                    = {Dual-spacecraft reconstruction of a three-dimensional magnetic flux rope at the {Earth}'s magnetopause},
  Author                   = {Hasegawa, H. and Sonnerup, B. U. Ö. and Eriksson, S. and Nakamura, T. K. M. and Kawano, H.},
  Journal                  = {Ann. Geophys.},
  Year                     = {2015},
  Number                   = {2},
  Pages                    = {169--184},
  Volume                   = {33},

  Doi                      = {10.5194/angeo-33-169-2015},
  ISSN                     = {1432-0576},
  Keywords                 = {and boundary layers, connection, instruments and techniques, magnetic re-, magnetopause cusp, magnetospheric physics, Space Plasma Physics},
  Url                      = {http://www.ann-geophys.net/33/169/2015/}
}

@Article{Haswell2012,
  Title                    = {Near-ultraviolet {Absorption}, {Chromospheric} {Activity}, and {Star}-{Planet} {Interactions} in the {WASP}-12 system},
  Author                   = {Haswell, C. A. and Fossati, L. and Ayres, T. and France, K. and Froning, C. S. and Holmes, S. and Kolb, U. C. and Busuttil, R. and Street, R. A. and Hebb, L. and Collier Cameron, A. and Enoch, B. and Burwitz, V. and Rodriguez, J. and West, R. G. and Pollacco, D. and Wheatley, P. J. and Carter, A.},
  Journal                  = {{\textbackslash}textbackslashapj},
  Year                     = {2012},

  Month                    = nov,
  Pages                    = {79},
  Volume                   = {760},

  Doi                      = {10.1088/0004-637X/760/1/79},
  Keywords                 = {planetary systems, planets and satellites: atmospheres, planets and satellites: composition, planets and satellites: individual: WASP-12 b HD189733 b, planets and satellites: physical evolution, planet-star interactions, stars: activity, stars: chromospheres, stars: individual: WASP-12 HD189733}
}

@Book{Heikkila2011,
  Title                    = {Earth's {Magnetosphere}: {Formed} by the {Low}-latitude {Boundary} {Layer}},
  Author                   = {Heikkila, Walter J},
  Publisher                = {Elsevier},
  Year                     = {2011}
}

@Book{Heikkila2011a,
  Title                    = {Earth's magnetosphere: created by the low latitude boundary layer},
  Author                   = {Heikkila, Walter J.},
  Publisher                = {Elsevier Science},
  Year                     = {2011},

  Address                  = {Amsterdam},

  ISBN                     = {978-0-444-52864-3 0-444-52864-4 978-0-444-52864-3},
  Keywords                 = {Magnetosph√§re, magnetosphere},
  Language                 = {eng},
  Shorttitle               = {Earth's magnetosphere}
}

@Book{Helliwell1965,
  Title                    = {Whistlers and {Related} {Ionospheric} {Phenomena}},
  Author                   = {Helliwell, R. A.},
  Year                     = {1965}
}

@Article{Henon1970,
  Title                    = {Numerical exploration of the restricted problem. {VI}. {Hill}'s case: {Non}-periodic orbits.},
  Author                   = {Henon, M.},
  Journal                  = {{\textbackslash}textbackslashaap},
  Year                     = {1970},

  Month                    = nov,
  Pages                    = {24--36},
  Volume                   = {9}
}

@Article{Hesse2014,
  Title                    = {Theory and {Modeling} for the {Magnetospheric} {Multiscale} {Mission}},
  Author                   = {Hesse, M. and Aunai, N. and Birn, J. and Cassak, P. and Denton, R. E. and Drake, J. F. and Gombosi, T. and Hoshino, M. and Matthaeus, W. and Sibeck, D. and Zenitani, S.},
  Journal                  = {Space Science Reviews},
  Year                     = {2014},
  Pages                    = {62},

  Abstract                 = {The Magnetospheric Multiscale (MMS) mission will provide measurement capabilities, which will exceed those of earlier and even contemporary missions by orders of magnitude. MMS will, for the first time, be able to measure directly and with sufficient resolution key features of the magnetic reconnection process, down to the critical electron scales, which need to be resolved to understand how reconnection works. Owing to the complexity and extremely high spatial resolution required, no prior measurements exist, which could be employed to guide the definition of measurement requirements, and consequently set essential parameters for mission planning and execution. Insight into expected details of the reconnection process could hence only been obtained from theory and modern kinetic modeling. This situation was recognized early on by MMS leadership, which supported the formation of a fully integrated Theory and Modeling Team (TMT). The TMT participated in all aspects of mission planning, from the proposal stage to individual aspects of instrument performance characteristics. It provided and continues to provide to the mission the latest insights regarding the kinetic physics of magnetic reconnection, as well as associated particle acceleration and turbulence, assuring that, to the best of modern knowledge, the mission is prepared to resolve the inner workings of the magnetic reconnection process. The present paper provides a summary of key recent results or reconnection research by TMT members.},
  ISSN                     = {0038-6308},
  Keywords                 = {Magnetic reconnection Magnetospheric multiscale Particle acceleration Dissipation Turbulence Plasma theory},
  Url                      = {http://adsabs.harvard.edu/abs/2014SSRv..tmp...62H}
}

@Article{Hesse2014a,
  Title                    = {On the electron diffusion region in planar, asymmetric, systems},
  Author                   = {Hesse, Michael and Aunai, Nicolas and Sibeck, David and Birn, Joachim},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2014},
  Pages                    = {8673--8680},
  Volume                   = {41},

  Abstract                 = {Particle-in-cell simulations and analytical theory are employed to study the electron diffusion region in asymmetric reconnection, which is taking place in planar configurations without a guide field. The analysis presented here focuses on the nature of the local reconnection electric field and on differences from symmetric configurations. Further emphasis is on the complex structure of the electron distribution in the diffusion region, which is generated by the mixing of particles from different sources. We find that the electric field component that is directly responsible for flux transport is provided not by electron pressure-based, "quasi-viscous," terms but by inertial terms. The quasi-viscous component is shown to be critical in that it is necessary to sustain the required overall electric field pattern in the immediate neighborhood of the reconnection X line.},
  ISSN                     = {0094-8276},
  Keywords                 = {reconnection diffusion electron magnetopause},
  Url                      = {http://adsabs.harvard.edu/abs/2014GeoRL..41.8673H}
}

@Article{Hesse2013,
  Title                    = {Aspects of collisionless magnetic reconnection in asymmetric systems},
  Author                   = {Hesse, Michael and Aunai, Nicolas and Zenitani, Seiji and Kuznetsova, Masha and Birn, Joachim},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2013},
  Number                   = {6},
  Pages                    = {061210},
  Volume                   = {20},

  Url                      = {http://scitation.aip.org/content/aip/journal/pop/20/6/10.1063/1.4811467},
  Urldate                  = {2014-05-31}
}

@Article{Hesse2011,
  Title                    = {The diffusion region in collisionless magnetic reconnection},
  Author                   = {Hesse, Michael and Neukirch, Thomas and Schindler, Karl and Kuznetsova, Masha and Zenitani, Seiji},
  Journal                  = {Space science reviews},
  Year                     = {2011},
  Number                   = {1-4},
  Pages                    = {3--23},
  Volume                   = {160},

  Url                      = {http://link.springer.com/article/10.1007/s11214-010-9740-1},
  Urldate                  = {2014-05-31}
}

@Article{Hesse1996,
  Title                    = {Hybrid {Modeling} of the {Formation} of {Thin} {Current} {Sheets} in {Magnetotail} {Configurations}.},
  Author                   = {Hesse, Michael and Winske, Dan and Kuznetsova, Masha and Birn, Joachim and Schindler, Karl},
  Journal                  = {Journal of geomagnetism and geoelectricity},
  Year                     = {1996},
  Number                   = {5/6},
  Pages                    = {749--763},
  Volume                   = {48}
}

@Article{Hesse1995,
  Title                    = {Hybrid modeling of collisionless reconnection in two-dimensional current sheets: {Simulations}},
  Author                   = {Hesse, Michael and Winske, Dan and Kuznetsova, Masha M},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1995},
  Number                   = {A11},
  Pages                    = {21815--21825},
  Volume                   = {100}
}

@Article{Hewett1988,
  Title                    = {New regimes of magnetic reconnection in collisionless plasmas},
  Author                   = {Hewett, Dennis W and Frances, Gregory E and Max, Claire E},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {1988},
  Number                   = {7},
  Pages                    = {893},
  Volume                   = {61}
}

@Article{Hobara2008,
  Title                    = {Cluster observations of electrostatic solitary waves near the {Earth}'s bow shock},
  Author                   = {Hobara, Y and Walker, SN and Balikhin, M and Pokhotelov, OA and Gedalin, M and Krasnoselskikh, V and Hayakawa, M and André, Mats and Dunlop, M and Rème, H and {others}},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2008},
  Number                   = {A5},
  Volume                   = {113}
}

@Article{Holst2014,
  Title                    = {Alfvén {Wave} {Solar} {Model} ({AWSoM}): {Coronal} {Heating}},
  Author                   = {van der Holst, B. and Sokolov, I. V. and Meng, X. and Jin, M. and Manchester, IV, W. B. and Tóth, G. and Gombosi, T. I.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2014},

  Month                    = feb,
  Pages                    = {81},
  Volume                   = {782},

  Doi                      = {10.1088/0004-637X/782/2/81},
  Keywords                 = {INTERPLANETARY MEDIUM, Magnetohydrodynamics: MHD, methods: numerical, Solar Wind, Sun: corona, waves}
}

@Article{Hones1984,
  Title                    = {Magnetic reconnection in space and laboratory plasmas},
  Author                   = {Hones, Edward W},
  Journal                  = {Eos, Transactions American Geophysical Union},
  Year                     = {1984},
  Number                   = {18},
  Pages                    = {340--341},
  Volume                   = {65}
}

@Article{Hong2012,
  Title                    = {Generation of kinetic {Alfvén} waves by beam-plasma interaction in non-uniform plasma},
  Author                   = {Hong, M. H. and Lin, Y. and Wang, X. Y.},
  Journal                  = {Phys. Plasmas},
  Year                     = {2012},

  Month                    = jul,
  Number                   = {7},
  Pages                    = {072903},
  Volume                   = {19},

  Doi                      = {10.1063/1.4736988},
  Keywords                 = {Atomic molecular ion and heavy-particle collisions, boundary layer effects, Hybrid methods, Magnetohydrodynamic waves, Microinstabilities, Particle beam interactions in plasmas, plasma Alfven waves, plasma-beam interactions, plasma boundary layers, plasma instability, Plasma-material interactions, plasma simulation}
}

@Article{Hoppe1982,
  Title                    = {Particle acceleration at planetary bow shock waves},
  Author                   = {Hoppe, MM and Russell, CT},
  Year                     = {1982}
}

@Article{Hoppe1981,
  Title                    = {On the nature of {ULF} waves upstream of planetary bow shocks},
  Author                   = {Hoppe, M and Russell, CT},
  Journal                  = {Advances in Space Research},
  Year                     = {1981},
  Number                   = {1},
  Pages                    = {327--332},
  Volume                   = {1}
}

@Article{Horne2007,
  Title                    = {Plasma astrophysics: acceleration of killer electrons},
  Author                   = {Horne, Richard Bertram},
  Journal                  = {Nature Physics},
  Year                     = {2007},
  Number                   = {9},
  Pages                    = {590--591},
  Volume                   = {3}
}

@Article{Howard2005,
  Title                    = {Statistical survey of earthbound interplanetary shocks, associated coronal mass ejections and their space weather consequences},
  Author                   = {Howard, TA and Tappin, SJ},
  Journal                  = {ASTRONOMY AND ASTROPHYSICS-BERLIN THEN LES ULIS-},
  Year                     = {2005},
  Number                   = {1},
  Pages                    = {373},
  Volume                   = {440}
}

@Article{Howard2006,
  Title                    = {Tracking halo coronal mass ejections from 0–1 {AU} and space weather forecasting using the {Solar} {Mass} {Ejection} {Imager} ({SMEI})},
  Author                   = {Howard, TA and Webb, DF and Tappin, SJ and Mizuno, DR and Johnston, JC},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2006},
  Number                   = {A4},
  Volume                   = {111}
}

@Article{Howe1972,
  Title                    = {Explorer 33 and 35 plasma observations of magnetosheath flow},
  Author                   = {Howe, Herbert C and Binsack, Joseph H},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1972},
  Number                   = {19},
  Pages                    = {3334--3344},
  Volume                   = {77}
}

@Article{Huang1983,
  Title                    = {The gravitational escape/capture of planetary satellites},
  Author                   = {Huang, T.-Y. and Innanen, K. A.},
  Journal                  = {{\textbackslash}textbackslashaj},
  Year                     = {1983},

  Month                    = oct,
  Pages                    = {1537--1548},
  Volume                   = {88},

  Doi                      = {10.1086/113444},
  Keywords                 = {CALCULATIONS, CAPTURE, Capture Effect, DATA, DIAGRAMS, DISTRIBUTION, dynamics, ECCENTRICITY, Eccentric Orbits, ESCAPE, Escape Velocity, GEOMETRY, GRAVITY EFFECTS, Jupiter Satellites, Orbit Calculation, ORBITS, ORIGIN, PARAMETERS, PARENT BODIES, Planetary Gravitation, Planetary Orbits, PLANETS, RADII, REGIONS, RETROGRADE MOTION, SA‚Ñ°LITES, Three Body Problem}
}

@Article{Huber1996,
  Title                    = {The history of thge {SOHO} mission.},
  Author                   = {Huber, MCE and Bonnet, RM and Dale, DC and Arduini, M and Fröhlich, C and Domingo, V and Whitcomb, G},
  Journal                  = {ESA Bulletin},
  Year                     = {1996},
  Pages                    = {25--35},
  Volume                   = {86}
}

@InProceedings{Hubert1990,
  Title                    = {Comparison of {Monte} {Carlo} simulations and polynomial expansions of auroral non-{Maxwellian} distributions. {I}-{The} 3-{D} representation. {II}-{The} 1-{D} representation},
  Author                   = {Hubert, D and Barakat, AR},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {1990},
  Pages                    = {687--704},
  Volume                   = {8}
}

@Article{Hubert2011,
  Title                    = {Comment on {\textbackslash}{ldquoSlow}-mode shock candidate in the {Jovian} magnetosheath{\textbackslash}rdquo by {Z}. {Bebesi}, {K}. {Szego}, {A}. {Balogh}, {N}. {Krupp}, {G}. {Erdos}, {A}.{M}. {Rymer}, {G}.{R}. {Lewis}, {W}.{S}. {Kurth}, {D}.{T}. {Young}, {M}.{K}. {Dhougherty}},
  Author                   = {Hubert, D. and Samsonov, A.},
  Journal                  = {{\textbackslash}planss},
  Year                     = {2011},

  Month                    = apr,
  Pages                    = {443--444},
  Volume                   = {59},

  Doi                      = {10.1016/j.pss.2010.10.004}
}

@Article{Hubert2005,
  Title                    = {Reply to the comment by {P}. {Song} et al. on “{Steady} state slow shock inside the {Earth}'s magnetosheath: {To} be or not to be? 1. {The} original observations revisited” by {D}. {Hubert} and {A}. {Samsonov}},
  Author                   = {Hubert, D. and Samsonov, A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2005},

  Month                    = nov,
  Number                   = {A9},
  Pages                    = {11211},
  Volume                   = {110},

  Doi                      = {10.1029/2005JA011224},
  Keywords                 = {3-D MHD simulation, discontinuity, magnetosheath, Magnetospheric Physics: Magnetosheath, Magnetospheric Physics: Plasma convection (2463), Magnetospheric Physics: Solar wind/magnetosphere interactions, multiple time convection, slow mode transition}
}

@Article{Hubert2004,
  Title                    = {Steady state slow shock inside the {Earth}'s magnetosheath: {To} be or not to be? 1. {The} original observations revisited},
  Author                   = {Hubert, D. and Samsonov, A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = jan,
  Pages                    = {1217},
  Volume                   = {109},

  Doi                      = {10.1029/2003JA010008},
  Keywords                 = {Convection, discontinuity, diversion, magnetosheath, Magnetospheric Physics: Magnetosheath, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Solar wind/magnetosphere interactions, MHD, Space Plasma Physics: Discontinuities, transition}
}

@Article{Huddleston1998,
  Title                    = {Location and shape of the {Jovian} magnetopause and bow shock},
  Author                   = {Huddleston, DE and Russell, CT and Kivelson, MG and Khurana, KK and Bennett, L},
  Journal                  = {Journal of Geophysical Research: Planets (1991–2012)},
  Year                     = {1998},
  Number                   = {E9},
  Pages                    = {20075--20082},
  Volume                   = {103}
}

@Article{Huddleston2000,
  Title                    = {Toroidal ion distributions observed at high altitudes equatorward of the cusp},
  Author                   = {Huddleston, MM and Pollock, CJ},
  Journal                  = {Geophys. {\textbackslash}ldots},
  Year                     = {2000},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/1999GL010712/full}
}

@Article{Hudman2010,
  Title                    = {Interannual variability in soil nitric oxide emissions over the {United} {States} as viewed from space},
  Author                   = {Hudman, Rynda C. and Russell, A. R. and Valin, L. C. and Cohen, R. C.},
  Journal                  = {Atmos. Chem. Phys},
  Year                     = {2010},
  Number                   = {20},
  Pages                    = {9943--9952},
  Volume                   = {10},

  Url                      = {http://atmos-chem-phys-discuss.net/10/13029/2010/acpd-10-13029-2010.pdf},
  Urldate                  = {2014-11-13}
}

@Article{Hughes1995,
  Title                    = {The magnetopause, magnetotail, and magnetic reconnection},
  Author                   = {Hughes, WJ},
  Journal                  = {Introduction to Space Physics},
  Year                     = {1995},
  Pages                    = {227--287}
}

@Article{Hultqvist1999,
  Title                    = {Chapter 7-{Contributions} of {Different} {Source} and {Loss} {Processes} to the {Plasma} {Content} of the {Magnetosphere}},
  Author                   = {Hultqvist, B. and André, M. and Christon, S. P. and Paschmann, G. and Sibeck, D. G.},
  Journal                  = {Space Science Reviews},
  Year                     = {1999},
  Pages                    = {355--372},
  Volume                   = {88},

  Abstract                 = {Not Available},
  ISSN                     = {0038-6308},
  Url                      = {http://adsabs.harvard.edu/abs/1999SSRv...88..355H}
}

@Article{Hultqvist2005,
  Title                    = {Space {Plasma} {Physics}},
  Author                   = {Hultqvist, B. and Paschmann, G. and Sibeck, D. and Terasawa, T. and Treumann, R. A. and Zelenyi, L.},
  Journal                  = {ISSI Scientific Reports Series},
  Year                     = {2005},
  Pages                    = {113},
  Volume                   = {3},

  Abstract                 = {Not Available},
  Url                      = {http://adsabs.harvard.edu/abs/2005ISSIR...3..113H}
}

@Article{Hundhausen1973,
  Title                    = {Nonlinear model of high-speed solar wind streams},
  Author                   = {Hundhausen, AJ},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1973},
  Number                   = {10},
  Pages                    = {1528--1542},
  Volume                   = {78}
}

@Article{Hundhausen1976,
  Title                    = {Solar wind structure at large heliocentric distances: {An} interpretation of {Pioneer} 10 observations},
  Author                   = {Hundhausen, AJ and Gosling, JT},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1976},
  Number                   = {7},
  Pages                    = {1436--1440},
  Volume                   = {81}
}

@Article{Hundhausen1972,
  Title                    = {Coronal expansion and solar wind},
  Author                   = {Hundhausen, Arthur J},
  Journal                  = {Coronal Expansion and Solar Wind, XII, 238 pp. 101 figs.. Springer-Verlag Berlin Heidelberg New York. Also Physics and Chemistry in Space, volume 5},
  Year                     = {1972},
  Volume                   = {1}
}

@Article{Hundhausen1968,
  Title                    = {Ionization state of the interplanetary plasma},
  Author                   = {Hundhausen, A. J. and Gilbert, H. E. and Bame, S. J.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1968},

  Month                    = sep,
  Pages                    = {5485--5493},
  Volume                   = {73},

  Doi                      = {10.1029/JA073i017p05485},
  Keywords                 = {Particles and Fields in Interplanetary Space: Solar-wind plasma, Solar Physics and Astrophysics: Corona}
}

@Article{Hundhausen1968a,
  Title                    = {The {State} of {Ionization} of {Oxygen} in the {Solar} {Wind}},
  Author                   = {Hundhausen, A. J. and Gilbert, H. E. and Bame, S. J.},
  Journal                  = {{\textbackslash}apjl},
  Year                     = {1968},

  Month                    = apr,
  Pages                    = {L3},
  Volume                   = {152},

  Doi                      = {10.1086/180165}
}

@Article{Hwang2012,
  Title                    = {The first in situ observation of {Kelvin}-{Helmholtz} waves at high-latitude magnetopause during strongly dawnward interplanetary magnetic field conditions},
  Author                   = {Hwang, K.-J. and Goldstein, M. L. and Kuznetsova, M. M. and Wang, Y. and ViñAs, A. F. and Sibeck, D. G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2012},
  Pages                    = {8233},
  Volume                   = {117},

  Abstract                 = {We report the first in situ observation of high-latitude magnetopause (near the northern duskward cusp) Kelvin-Helmholtz waves (KHW) by Cluster on January 12, 2003, under strongly dawnward interplanetary magnetic field (IMF) conditions. The fluctuations unstable to Kelvin-Helmholtz instability (KHI) are found to propagate mostly tailward, i.e., along the direction almost 90° to both the magnetosheath and geomagnetic fields, which lowers the threshold of the KHI. The magnetic configuration across the boundary layer near the northern duskward cusp region during dawnward IMF is similar to that in the low-latitude boundary layer under northward IMF, in that (1) both magnetosheath and magnetospheric fields across the local boundary layer constitute the lowest magnetic shear and (2) the tailward propagation of the KHW is perpendicular to both fields. Approximately 3-hour-long periods of the KHW during dawnward IMF are followed by the rapid expansion of the dayside magnetosphere associated with the passage of an IMF discontinuity that characterizes an abrupt change in IMF cone angle,ϕ = acos{\textless}mfenced open="(" close=")"{\textgreater}{\textless}mfrac{\textgreater}Bx{\textless}mfenced open="{\textbar}" close="{\textbar}"{\textgreater}B{\textless}/mfenced{\textgreater}{\textless}/mfrac{\textgreater}{\textless}/mfenced{\textgreater}, from ˜90° to ˜10°. Cluster, which was on its outbound trajectory, continued observing the boundary waves at the northern evening-side magnetopause during sunward IMF conditions following the passage of the IMF discontinuity. By comparing the signatures of boundary fluctuations before and after the IMF discontinuity, we report that the frequencies of the most unstable KH modes increased after the discontinuity passed. This result demonstrates that differences in IMF orientations (especially inϕ) are associated with the properties of KHW at the high-latitude magnetopause due to variations in thickness of the boundary layer, and/or width of the KH-unstable band on the surface of the dayside magnetopause.},
  ISSN                     = {0148-0227},
  Keywords                 = {Kelvin-Helmholtz instability dayside magnetopause solar wind magnetosphere interaction Magnetospheric Physics: Cusp Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: MHD waves and instabilities (2149 6050 7836) Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2012JGRA..117.8233H}
}

@Article{Imada2008,
  Title                    = {The dawn-dusk asymmetry of energetic electron in the {Earth}'s magnetotail: {Observation} and transport models},
  Author                   = {Imada, S. and Hoshino, M. and Mukai, T.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2008},

  Month                    = nov,
  Number                   = {A12},
  Pages                    = {11201},
  Volume                   = {113},

  Abstract                 = {We have studied the dawn-dusk asymmetry of the energetic/thermal particle in the plasma sheet using the Geotail data. We found the species- and energy-dependent dawn-dusk asymmetries in the plasma sheet. The dawn-dusk asymmetries have some typical structures, and we used a finite width two-dimensional model of the magnetotail to explain their characteristics. The characteristics and assumptions of our model can be summarized as follows: (1) the magnetotail convection is steady (both of magnetic field and electric field is steady), (2) the directions of electric fields are duskward, (3) the directions of magnetic fields are northward, (4) the magnetic field gradient is constant for earthward (constant for other directions), (5) the width of the magnetotail is constant in the entire plasma sheet (40 RE), (6) the plasma source region is steady at XGSM ˜ -100 RE, (7) the magnetic moment μ is conserved during transport, and (8) the particle spatial diffusion takes place only for dawn-dusk direction. In this model, we found that the energetic electrons cannot be provided sufficiently at the dusk flank with the simple adiabatic process (no spatial diffusion). Furthermore we applied the Bohm-type diffusion to the model and found that the observed asymmetries are well reproduced in the case that the diffusion coefficient is equal to 0.006/0.03v⊥rg for electron/ion.},
  Doi                      = {10.1029/2008JA013610},
  Keywords                 = {7835), dawn-dusk asymmetry, Energetic particle, Magnetospheric Physics: Energetic particles: trapped, Magnetospheric Physics: Magnetic reconnection (7526, Magnetospheric Physics: Magnetotail, Magnetospheric Physics: Plasma convection (2463), Magnetospheric Physics: Plasma sheet, transport}
}

@Book{Intriligator,
  Title                    = {Space weather prediction system and method},
  Author                   = {Intriligator, Devrie S and Intriligator, James M},
  Month                    = aug
}

@Article{Ioffe2006,
  Title                    = {Resonance radiative decays as a tool for its parity determination},
  Author                   = {Ioffe, B. L. and Samsonov, A. V.},
  Journal                  = {Phys. Lett. B},
  Year                     = {2006},

  Month                    = feb,
  Pages                    = {298--300},
  Volume                   = {633},

  Doi                      = {10.1016/j.physletb.2005.12.006},
  Keywords                 = {Parity, Pentaquark, Radiative decay}
}

@Article{Ioffe2000,
  Title                    = {Correlation {Function} for {Topological} {Charge} {Densities} within the {Instanton} {Model} in {QCD}},
  Author                   = {Ioffe, B. L. and Samsonov, A. V.},
  Journal                  = {Phys. At. Nucl.},
  Year                     = {2000},

  Month                    = aug,
  Pages                    = {1448--1454},
  Volume                   = {63},

  Doi                      = {10.1134/1.1307466}
}

@Article{Ipavich1998,
  Title                    = {Solar wind measurements with {SOHO}: {The} {CELIAS}/{MTOF} proton monitor},
  Author                   = {Ipavich, F. M. and Galvin, A. B. and Lasley, S. E. and Paquette, J. A. and Hefti, S. and Reiche, K.-U. and Coplan, M. A. and Gloeckler, G. and Bochsler, P. and Hovestadt, D. and Grünwaldt, H. and Hilchenbach, M. and Gliem, F. and Axford, W. I. and Balsiger, H. and Bürgi, A. and Geiss, J. and Hsieh, K. C. and Kallenbach, R. and Klecker, B. and Lee, M. A. and Managadze, Georgy G. and Marsch, E. and Möbius, E. and Neugebauer, M. and Scholer, M. and Verigin, M. I. and Wilken, B. and Wurz, P.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1998},

  Month                    = aug,
  Pages                    = {17205--17214},
  Volume                   = {103},

  Doi                      = {10.1029/97JA02770},
  Keywords                 = {and magnetic clouds, driver gases, Interplanetary Physics: Ejecta, Interplanetary Physics: Pickup ions, Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Sources of the solar wind}
}

@Article{Ipavich1978,
  Title                    = {Measurements of pulse-height defect in {Au}-{Si} detectors for {H}, {He}, {C}, {N}, {O}, {Ne}, {Ar}, {Kr} from about 2 to 400 {keV}/nucleon},
  Author                   = {Ipavich, F. M. and Lundgren, R. A. and Lambird, B. A. and Gloeckler, G.},
  Journal                  = {Nuclear Instruments and Methods},
  Year                     = {1978},

  Month                    = aug,
  Pages                    = {291--294},
  Volume                   = {154},

  Doi                      = {10.1016/0029-554X(78)90412-3},
  Keywords                 = {Crystals, Electron Accelerators, Energy Dissipation, Gas Detectors, Gold, Heavy Ions, Ion Beams, Ionic Collisions, Nucleons, Particle Energy, Pulse Amplitude, Silicon Junctions, Solid-Solid Interfaces, Solid State Devices, Van De Graaff Accelerators}
}

@Article{Iucci2005,
  Title                    = {Space weather conditions and spacecraft anomalies in different orbits},
  Author                   = {Iucci, N and Levitin, AE and Belov, AV and Eroshenko, EA and Ptitsyna, NG and Villoresi, G and Chizhenkov, GV and Dorman, LI and Gromova, LI and Parisi, M and {others}},
  Journal                  = {Space Weather},
  Year                     = {2005},
  Number                   = {1},
  Volume                   = {3}
}

@Article{Ivanenko1990,
  Title                    = {Energy {Spectrum} and {Cosmic} {Ray} {Composition} in the {Region} of {Energies} {Higher} than 1 {TeV} {Investigated} {Onboard} the ”{Cosmos}-1543” and ”{Cosmos}-1713” {Satellites}},
  Author                   = {Ivanenko, P. I. and Rapoport, D. I. and Shestoperov, Y. V. and Basina, V. Y. and Vakulov, V. P. and Vasiliev, Y. Y. and Golinskaya, M. R. and Gordeev, P. Y. and Grigorieva, B. L. and Kazakova, E. A. and Kozlov, D. V. and Kumpan, P. I. and Mischenko, G. L. and Nikanorov, M. V. and Papina, P. L. and Platonov, V. V. and Samsonov, A. G. and Smolensky, G. L. and Sobinyakov, A. V. and Tambovtsev, E. G. and Trigubov, V. Y. and Fateeva, M. I. and Fedorov, N. A. and Hein, A. L. and Chikova, O. L. and Shiryaeva, Y. V. and Yakovlev, M. B. and Yashin, V. I.},
  Journal                  = {International Cosmic Ray Conference},
  Year                     = {1990},
  Pages                    = {77},
  Volume                   = {3}
}

@Article{Ivchenko2000,
  Title                    = {{A statistical study of the magnetosphere boundary crossing by the Geotail satellite}},
  Author                   = {Ivchenko, N. V. and Sibeck, D. G. and Takahashi, K. and Kokubun, S.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2000},
  Number                   = {18},
  Pages                    = {2881--2884},
  Volume                   = {27},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {Geotail magnetometer observations from 1995-97 were used to identify 1369 dayside magnetospheric boundary crossings. Statistical properties of this set of multiple crossings are presented and discussed in terms of models for magnetopause motion. Our results indicate that equatorial boundary crossings are caused by north-south aligned ridges propagating azimuthally around the magnetosphere. Perpendicular orientations of the magnetospheric and magnetosheath magnetic fields inhibit the boundary motion. For the garden hose orientations of the interplanetary magnetic field (IMF), magnetospheric boundary motion is favoured in the dawn sector, while orthospiral orientations favour motion in the dusk sector. These results suggest that pressure pulses generated at the quasi-parallel bow shock drive the boundary motion.},
  Doi                      = {10.1029/2000GL000020},
  ISSN                     = {00948276},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Ivchenko2000a,
  Title                    = {A statistical study of the magnetosphere boundary crossings by the {Geotail} satellite},
  Author                   = {Ivchenko, N. V. and Sibeck, D. G. and Takahashi, K. and Kokubun, S.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2000},
  Pages                    = {2881--2884},
  Volume                   = {27},

  Abstract                 = {Geotail magnetometer observations from 1995-97 were used to identify 1369 dayside magnetospheric boundary crossings. Statistical properties of this set of multiple crossings are presented and discussed in terms of models for magnetopause motion. Our results indicate that equatorial boundary crossings are caused by north-south aligned ridges propagating azimuthally around the magnetosphere. Perpendicular orientations of the magnetospheric and magnetosheath magnetic fields inhibit the boundary motion. For the garden hose orientations of the interplanetary magnetic field (IMF), magnetospheric boundary motion is favoured in the dawn sector, while orthospiral orientations favour motion in the dusk sector. These results suggest that pressure pulses generated at the quasi-parallel bow shock drive the boundary motion.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2000GeoRL..27.2881I}
}

@InProceedings{Iyemori1996,
  Title                    = {Decay of the {Dst} field of geomagnetic disturbance after substorm onset and its implication to storm-substorm relation},
  Author                   = {Iyemori, T and Rao, DRK},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {1996},
  Pages                    = {608--618},
  Publisher                = {Springer},
  Volume                   = {14}
}

@Article{Jaafari2008,
  Title                    = {Simulation of the formation of {O}$^{\textrm{+\$}}$ density troughs at 6000 km altitude in the polar cap ionosphere-magnetosphere region},
  Author                   = {Jaafari, F. and Horwitz, J. L. and Zeng, W.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2008},

  Month                    = jul,
  Pages                    = {7207},
  Volume                   = {113},

  Doi                      = {10.1029/2007JA012690},
  Keywords                 = {auroral effects, Ionosphere: Particle precipitation, Ionosphere: Polar cap ionosphere, Ionosphere: Wave/particle interactions (7867), Magnetospheric Physics: Magnetosphere: inner, Magnetospheric Physics: Magnetosphere/ionosphere interactions (2431), O$^{\textrm{+\$}}$ density trough}
}

@Book{Jackson1999,
  Title                    = {Classical {Electrodynamics}},
  Author                   = {Jackson, J. D.},
  Publisher                = {John Wiley \& Sons},
  Year                     = {1999},

  Address                  = {United States of America},
  Edition                  = {3rd}
}

@Article{Jacobsen2009,
  Title                    = {{THEMIS} observations of extreme magnetopause motion caused by a hot flow anomaly},
  Author                   = {Jacobsen, K. S. and Phan, T. D. and Eastwood, J. P. and Sibeck, D. G. and Moen, J. I. and Angelopoulos, V. and McFadden, J. P. and Engebretson, M. J. and Provan, G. and Larson, D. and Fornaçon, K.-H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2009},
  Pages                    = {8210},
  Volume                   = {114},

  Abstract                 = {On 30 October 2007, the five THEMIS spacecraft observed the cause and consequence of extreme motion of the dawn flank magnetopause, displacing the magnetopause outward by at least 4.8 R {\textless}SUB{\textgreater} E {\textless}/SUB{\textgreater} in 59 s, with flow speeds in the direction normal to the model magnetopause reaching 800 km/s. While the THEMIS A, C, D, and E observations allowed the determination of the velocity, size, and shape of a large bulge moving tailward along the magnetopause at a speed of 355 km/s, THEMIS B observed the signatures of a hot flow anomaly (HFA) upstream of the bow shock at the same time, indicating that the pressure perturbation generated by the HFA may be the source of the fast compression and expansion of the magnetosphere. The transient deformation of the magnetopause generated field-aligned currents and created traveling convection vortices which were detected by ground magnetometers. This event demonstrates that kinetic (non-MHD) effects at the bow shock can have global consequences on the magnetosphere.},
  ISSN                     = {0148-0227},
  Keywords                 = {Geochemistry: Composition of the moon Geochemistry: Composition of the moon Geochemistry: Composition of the moon (2431) Geochemistry: Composition of the moon},
  Url                      = {http://adsabs.harvard.edu/abs/2009JGRA..114.8210J}
}

@Article{Jaegle2005,
  Title                    = {Global partitioning of {NO} x sources using satellite observations: {Relative} roles of fossil fuel combustion, biomass burning and soil emissions},
  Author                   = {Jaeglè, Lyatt and Steinberger, Linda and Martin, Randall V. and Chance, Kelly},
  Journal                  = {Faraday Discuss.},
  Year                     = {2005},
  Pages                    = {407--423},
  Volume                   = {130},

  Shorttitle               = {Global partitioning of {NO} x sources using satellite observations},
  Url                      = {http://pubs.rsc.org/en/content/articlehtml/2005/fd/b502128f},
  Urldate                  = {2014-11-13}
}

@Article{Jaffel1992,
  Title                    = {La bosse {Lyman} alpha de {Jupiter}.},
  Author                   = {Jaffel, L. B.},
  Journal                  = {L'Astronomie},
  Year                     = {1992},

  Month                    = dec,
  Pages                    = {17--20},
  Volume                   = {106}
}

@InProceedings{Jaffel1991,
  Title                    = {The {Lyman} {Alpha} {Bulge} of {Jupiter}: {Effects} of {Non}-{Thermal} {Velocity} {Field}},
  Author                   = {Jaffel, L. B. and Clarke, J. T. and Gladstone, G. R. and Prangé, R. and Sandel, B. R. and Vidal-Madjar, A. and Yelle, R. V.},
  Booktitle                = {Bulletin of the {American} {Astronomical} {Society}},
  Year                     = {1991},
  Month                    = jun,
  Pages                    = {1135},
  Series                   = {Bulletin of the {American} {Astronomical} {Society}},
  Volume                   = {23}
}

@Article{Jaffel1993,
  Title                    = {The {Lyman} alpha bulge of {Jupiter}: {Effects} of non-thermal velocity field},
  Author                   = {Jaffel, L. B. and Clarke, J. T. and Prangé, R. and Gladstone, G. R. and Vidal-Madjar, A.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {1993},

  Month                    = apr,
  Pages                    = {747--750},
  Volume                   = {20},

  Abstract                 = {In this preliminary study, we outline for the first time the effect of non-thermal line broadening processes (turbulence, random waves, convection) on the shape and intensity of the H Ly-α line resonance scattered from the atmosphere of Jupiter and we show how a non-thermal velocity field, confined to the bulge region, in the upper atmosphere of Jupiter, may account for most of the H Ly-α bulge features. Both the shape and the brightness of the Ly-α line from the bulge region as reported by the IUE instrument and the Voyager UV Spectrometer can be recovered assuming resonant scattering with a total atomic hydrogen [H]∼4{\textbackslash}times10$^{\textrm{17\$}}$ cm$^{\textrm{-2\$}}$, and a non-thermal component [H]∼2{\textbackslash}times10$^{\textrm{15\$}}$ cm$^{\textrm{-2\$}}$ above the thermopause.}
}

@InProceedings{Jaffel1991a,
  Title                    = {A {New} {Model} for the {Disc} {Lyman} {Alpha} {Emission} of {Saturn}},
  Author                   = {Jaffel, L. B. and Feng, D. and Yelle, R. V. and Hall, D. T. and Herbert, F.},
  Booktitle                = {Bulletin of the {American} {Astronomical} {Society}},
  Year                     = {1991},
  Month                    = jun,
  Pages                    = {1148},
  Series                   = {Bulletin of the {American} {Astronomical} {Society}},
  Volume                   = {23}
}

@Article{Jaffel1995,
  Title                    = {Dark auroral oval on {Saturn} discovered in {Hubble} {Space} {Telescope} ultraviolet images},
  Author                   = {Jaffel, L Ben and Leers, Véronique and Sandel, Bill R},
  Journal                  = {SCIENCE-NEW YORK THEN WASHINGTON-},
  Year                     = {1995},
  Pages                    = {951--951}
}

@Article{Jaffel1988,
  Title                    = {The {Lyman} alpha albedo of {Jupiter}.},
  Author                   = {Jaffel, L. B. and Magnan, C. and Vidal-Madjar, A.},
  Journal                  = {{\textbackslash}aap},
  Year                     = {1988},

  Month                    = oct,
  Pages                    = {319--326},
  Volume                   = {204},

  Abstract                 = {The formation of the Lyα line in the Jovian atmosphere is treated by the method of addition of layers. Coherent, complete and partial redistribution functions are considered. Planetary center to limb reflectivities and emergent line profiles are computed and comparisons with previous work are done. A local minimum of the reflectivity is shown to appear near the planetary limb in some cases.},
  Keywords                 = {Albedo:Jupiter, Jupiter:Albedo, Jupiter:Lyman Alpha, Lyman Alpha:Jupiter}
}

@Article{Jaffel1995a,
  Title                    = {New analysis of the {Voyager} {UVS} {H} {Lyman}-α emission of {Saturn}},
  Author                   = {Jaffel, L Ben and Prangé, R and Sandel, BR and Yelle, RV and Emerich, C and Feng, D and Hall, DT},
  Journal                  = {Icarus},
  Year                     = {1995},
  Number                   = {1},
  Pages                    = {91--102},
  Volume                   = {113}
}

@InProceedings{Jaffel1992a,
  Title                    = {A new model for the {Lyman} alpha bulge of {Jupiter}.},
  Author                   = {Jaffel, L. B. and Sommeria, J. and Prangé, R.},
  Booktitle                = {Bulletin of the {American} {Astronomical} {Society}},
  Year                     = {1992},
  Month                    = jun,
  Pages                    = {1033--1034},
  Series                   = {Bulletin of the {American} {Astronomical} {Society}},
  Volume                   = {24}
}

@InProceedings{Jaffel1994,
  Title                    = {{HST}-{GHRS} detection of the deuterium {Lyman} alpha emission at the limb of {Jupiter}.},
  Author                   = {Jaffel, L. B. and Vidal-Madjar, A. and Clarke, J. T. and Emerich, C. and Prangé, R. and Gladstone, R. and McConnell, J. and Noll, K.},
  Booktitle                = {Bulletin of the {American} {Astronomical} {Society}},
  Year                     = {1994},
  Month                    = jun,
  Pages                    = {1100},
  Series                   = {Bulletin of the {American} {Astronomical} {Society}},
  Volume                   = {26},

  Keywords                 = {Jupiter Atmosphere: Lyman Alpha}
}

@InProceedings{Jaffel1990,
  Title                    = {Analysis of {Triton}'s {Lyman} {Alpha} {Emissions}},
  Author                   = {Jaffel, L. B. and Yelle, R. V.},
  Booktitle                = {Bulletin of the {American} {Astronomical} {Society}},
  Year                     = {1990},
  Month                    = jun,
  Pages                    = {1127},
  Series                   = {Bulletin of the {American} {Astronomical} {Society}},
  Volume                   = {22}
}

@Article{Jakowski2006,
  Title                    = {On developing a new ionospheric perturbation index for space weather operations},
  Author                   = {Jakowski, N and Stankov, SM and Schlueter, S and Klaehn, D},
  Journal                  = {Advances in Space Research},
  Year                     = {2006},
  Number                   = {11},
  Pages                    = {2596--2600},
  Volume                   = {38},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S0273117705009567}
}

@Book{Janhunen2000,
  Title                    = {Grand {Unified} {Ionosphere}-{Magnetosphere} {Coupling} {Simuation}},
  Author                   = {Janhunen, Pekka},
  Year                     = {2000},

  Url                      = {http://gumics.fmi.fi/en/index.html}
}

@Article{Janhunen2012,
  Title                    = {The {GUMICS}-4 global {MHD} magnetosphere–ionosphere coupling simulation},
  Author                   = {Janhunen, P and Palmroth, M and Laitinen, T and Honkonen, I and Juusola, L and Facsko, G and Pulkkinen, TI},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2012},
  Pages                    = {48--59},
  Volume                   = {80}
}

@Article{Jao2014,
  Title                    = {Fluid aspects of electron streaming instability in electron-ion plasmas},
  Author                   = {Jao, C-S and Hau, L-N},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2014},
  Number                   = {2},
  Pages                    = {022103},
  Volume                   = {21}
}

@Article{Jara-Almonte2014,
  Title                    = {Debye scale turbulence within the electron diffusion layer during magnetic reconnection},
  Author                   = {Jara-Almonte, J. and Daughton, W. and Ji, H.},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2014},
  Number                   = {3},
  Pages                    = {032114},
  Volume                   = {21},

  Url                      = {http://scitation.aip.org/content/aip/journal/pop/21/3/10.1063/1.4867868},
  Urldate                  = {2014-05-31}
}

@Article{Jelinek2012,
  Title                    = {A new approach to magnetopause and bow shock modeling based on automated region identification},
  Author                   = {Jelínek, K and Němeček, Z and Šafránková, J},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2012},
  Number                   = {A5},
  Volume                   = {117}
}

@InProceedings{Jelinek2014,
  Title                    = {Magnetosheath parameter profiles under different magnetic field orientations},
  Author                   = {Jelinek, K. and Nemecek, Z. and Safrankova, J. and Samsonov, A.},
  Booktitle                = {40th {COSPAR} {Scientific} {Assembly}},
  Year                     = {2014},
  Pages                    = {1330},
  Series                   = {{COSPAR} {Meeting}},
  Volume                   = {40}
}

@Article{Jelinek2010,
  Title                    = {Thin magnetosheath as a consequence of the magnetopause deformation: {THEMIS} observations},
  Author                   = {Jelínek, K. and Němeček, Z. and Šafránková, J. and Shue, J.-H. and Suvorova, A. V. and Sibeck, D. G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2010},
  Pages                    = {10203},
  Volume                   = {115},

  Abstract                 = {This paper presents a simultaneous observation of the bow shock and magnetopause by THEMIS probes that allows determination of the actual magnetosheath thickness at the subsolar point. Moreover, Geotail located at the dusk dayside magnetosheath registered a brief excursion to the magnetosphere in this time. The spacecraft configuration reveals a significant deformation of the magnetopause surface that locally decreases its curvature radius. The highly curved magnetopause results in the decrease of the magnetosheath thickness to about half of its standard value in a particular observation point. The observed phenomenon is attributed to a rotation of the interplanetary magnetic field (IMF). Although it is generally expected that the bow shock and magnetopause move in accord, being driven mainly by the solar wind dynamic pressure, we suggest that the local and transient thinning of the magnetosheath can result from different responses of its boundaries to a sudden change of the pressure and/or IMF orientation.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2010JGRA..11510203J}
}

@Book{Jenkins2009,
  Title                    = {The {Sun} and {How} to {Observe} {It}},
  Author                   = {Jenkins, Jamey L.},
  Publisher                = {Springer},
  Year                     = {2009},

  Address                  = {New York, NY},
  Edition                  = {1. ed},

  Annote                   = {Includes bibliographical references and index},
  ISBN                     = {978-0-387-09498-4 978-0-387-09497-7 978-0-387-09498-4},
  Keywords                 = {Beobachtung, Einf√ºhrung, Sonne, sun, Sun Observers' manuals},
  Language                 = {eng}
}

@Article{Jian2009,
  Title                    = {Ion {Cyclotron} {Waves} in the {Solar} {Wind} {Observed} by {STEREO} {Near} 1 {AU}},
  Author                   = {Jian, L. K. and Russell, C. T. and Luhmann, J. G. and Strangeway, R. J. and Leisner, J. S. and Galvin, A. B.},
  Journal                  = {{\textbackslash}apjl},
  Year                     = {2009},

  Month                    = aug,
  Pages                    = {L105--L109},
  Volume                   = {701},

  Doi                      = {10.1088/0004-637X/701/2/L105},
  Keywords                 = {INTERPLANETARY MEDIUM, Magnetic Fields, Solar Wind, waves}
}

@Article{Jin2012,
  Title                    = {A {Global} {Two}-temperature {Corona} and {Inner} {Heliosphere} {Model}: {A} {Comprehensive} {Validation} {Study}},
  Author                   = {Jin, M. and Manchester, W. B. and van der Holst, B. and Gruesbeck, J. R. and Frazin, R. A. and Landi, E. and Vasquez, A. M. and Lamy, P. L. and Llebaria, A. and Fedorov, A. and Toth, G. and Gombosi, T. I.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2012},

  Month                    = jan,
  Pages                    = {6},
  Volume                   = {745},

  Doi                      = {10.1088/0004-637X/745/1/6},
  Keywords                 = {INTERPLANETARY MEDIUM, Magnetohydrodynamics: MHD, methods: numerical, Solar Wind, Sun: corona}
}

@Article{Jing2014,
  Title                    = {{MHD} simulation of energy transfer across magnetopause during sudden changes of the {IMF} orientation},
  Author                   = {Jing, H. and Lu, J. Y. and Kabin, K. and Zhao, J. S. and Liu, Z.-Q. and Yang, Y. F. and Zhao, M. X. and Wang, M.},
  Journal                  = {Planetary and Space Science},
  Year                     = {2014},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S0032063314000890},
  Urldate                  = {2014-10-22}
}

@Article{Johnstone1997,
  Title                    = {Peace: a {Plasma} {Electron} and {Current} {Experiment}},
  Author                   = {Johnstone, A. D. and Alsop, C. and Burge, S. and Carter, P. J. and Coates, A. J. and Coker, A. J. and Fazakerley, A. N. and Grande, M. and Gowen, R. A. and Gurgiolo, C. and Hancock, B. K. and Narheim, B. and Preece, A. and Sheather, P. H. and Winningham, J. D. and Woodliffe, R. D.},
  Journal                  = {√ür},
  Year                     = {1997},

  Month                    = jan,
  Pages                    = {351--398},
  Volume                   = {79},

  Doi                      = {10.1023/A:1004938001388}
}

@Article{Johnstone1997a,
  Title                    = {Peace: a {Plasma} {Electron} and {Current} {Experiment}},
  Author                   = {Johnstone, A. D. and Alsop, C. and Burge, S. and Carter, P. J. and Coates, A. J. and Coker, A. J. and Fazakerley, A. N. and Grande, M. and Gowen, R. A. and Gurgiolo, C. and Hancock, B. K. and Narheim, B. and Preece, A. and Sheather, P. H. and Winningham, J. D. and Woodliffe, R. D.},
  Journal                  = {ßr},
  Year                     = {1997},

  Month                    = jan,
  Pages                    = {351--398},
  Volume                   = {79},

  Doi                      = {10.1023/A:1004938001388}
}

@Article{Joiner2006,
  Title                    = {First results from the {OMI} rotational {Raman} scattering cloud pressure algorithm},
  Author                   = {Joiner, Joanna and Vasilkov, Alexander P.},
  Journal                  = {Geoscience and Remote Sensing, IEEE Transactions on},
  Year                     = {2006},
  Number                   = {5},
  Pages                    = {1272--1282},
  Volume                   = {44},

  Url                      = {http://ieeexplore.ieee.org/xpls/abs_all.jsp?arnumber=1624606},
  Urldate                  = {2014-11-13}
}

@Article{Jones1991,
  Title                    = {The plasma physics of shock acceleration},
  Author                   = {Jones, Frank C and Ellison, Donald C},
  Journal                  = {Space Science Reviews},
  Year                     = {1991},
  Number                   = {1},
  Pages                    = {259--346},
  Volume                   = {58}
}

@Article{Jones2005,
  Title                    = {Space weather and commercial airlines},
  Author                   = {Jones, JBL and Bentley, RD and Hunter, R and Iles, RHA and Taylor, GC and Thomas, DJ},
  Journal                  = {Advances in Space Research},
  Year                     = {2005},
  Number                   = {12},
  Pages                    = {2258--2267},
  Volume                   = {36},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S0273117705000062}
}

@Article{Jones2007,
  Title                    = {Interaction between coronal mass ejections and the solar wind},
  Author                   = {Jones, R. A. and Breen, A. R. and Fallows, R. A. and Canals, A. and Bisi, M. M. and Lawrence, G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2007},

  Month                    = aug,
  Pages                    = {8107},
  Volume                   = {112},

  Doi                      = {10.1029/2006JA011875},
  Keywords                 = {and Astronomy: Coronal mass ejections (2101), and Astronomy: General or miscellaneous, ASTROPHYSICS, Radio Science: Remote sensing, Solar Physics, Space Plasma Physics: Turbulence (4490)}
}

@Article{Jovanovic2009,
  Title                    = {Kinetic theory for the ion humps at the foot of the {Earth}¬¨¬®‚àö‚â†s bow shock},
  Author                   = {Jovanović, D and Krasnoselskikh, VV},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2009},
  Number                   = {10},
  Pages                    = {102902},
  Volume                   = {16}
}

@InCollection{Kaiser2008,
  Title                    = {The {STEREO} mission: {An} introduction},
  Author                   = {Kaiser, Michael L and Kucera, TA and Davila, JM and Cyr, OC St and Guhathakurta, M and Christian, E},
  Booktitle                = {The {STEREO} {Mission}},
  Publisher                = {Springer},
  Year                     = {2008},
  Pages                    = {5--16},

  Url                      = {http://link.springer.com/chapter/10.1007/978-0-387-09649-0_2}
}

@Article{Kajdic2013,
  Title                    = {Statistical study of foreshock cavitons},
  Author                   = {Kajdič, P. and Blanco-Cano, X. and Omidi, N. and Meziane, K. and Russell, C. T. and Sauvaud, J.-A. and Dandouras, I. and Lavraud, B.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2013},

  Month                    = dec,
  Pages                    = {2163--2178},
  Volume                   = {31},

  Doi                      = {10.5194/angeo-31-2163-2013}
}

@Book{Kallenrode2004,
  Title                    = {Space {Physics} an {Introduction} to {Plasmas} and {Particles} in the {Heliosphere} and {Magnetospheres}},
  Author                   = {Kallenrode, May-Britt},
  Publisher                = {Springer Berlin Heidelberg},
  Year                     = {2004},

  Address                  = {Berlin, Heidelberg},

  Abstract                 = {Space is a large natural plasma laboratory offering a wealth of phenomena which range from the simple to the highly complex and non-linear. This book begins with an introduction to basic principles such as single-particle motion, magnetohydrodynamics and plasma waves. It incorporates these concepts into an analysis of complex phenomena including the sun and solar activity, shocks, interplanetary space and magnetospheres, and finally the interaction between these entities in solar-terrestrial relationships. In all these subfields of space research, special attention is paid to energetic particles. The book concludes with a brief chapter on instrumentation. In this third edition, numerous examples have been added to illustrate the basic concepts and aid the reader in applying such concepts to real world physics. In addition, recent observations (ACE, TRACE, Wind) have been included. The chapter on solar-terrestrial relationships has been expanded to introduce the current research topic of Space Weather.},
  ISBN                     = {978-3-662-09959-9 3-662-09959-4},
  Language                 = {English},
  Url                      = {http://dx.doi.org/10.1007/978-3-662-09959-9},
  Urldate                  = {2015-04-18}
}

@Article{Kaltenegger2010,
  Title                    = {Detecting {Volcanism} on {Extrasolar} {Planets}},
  Author                   = {Kaltenegger, L. and Henning, W. G. and Sasselov, D. D.},
  Journal                  = {{\textbackslash}textbackslashaj},
  Year                     = {2010},

  Month                    = nov,
  Pages                    = {1370--1380},
  Volume                   = {140},

  Doi                      = {10.1088/0004-6256/140/5/1370},
  Keywords                 = {astrobiology, earth, methods: observational, planets and satellites: atmospheres, planets and satellites: detection, planets and satellites: tectonics, Techniques: Spectroscopic}
}

@Book{Kappenman2010,
  Title                    = {Geomagnetic storms and their impacts on the {US} power grid},
  Author                   = {Kappenman, John},
  Publisher                = {Citeseer},
  Year                     = {2010}
}

@InCollection{Kappenman2001,
  Title                    = {An introduction to power grid impacts and vulnerabilities from space weather},
  Author                   = {Kappenman, John G},
  Booktitle                = {Space {Storms} and {Space} {Weather} {Hazards}},
  Publisher                = {Springer},
  Year                     = {2001},
  Pages                    = {335--361},

  Url                      = {http://link.springer.com/chapter/10.1007/978-94-010-0983-6_13}
}

@Article{Karachik2011,
  Title                    = {Solar {Wind} and {Coronal} {Bright} {Points} inside {Coronal} {Holes}},
  Author                   = {Karachik, N. V. and Pevtsov, A. A.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2011},

  Month                    = jul,
  Pages                    = {47},
  Volume                   = {735},

  Doi                      = {10.1088/0004-637X/735/1/47},
  Keywords                 = {Solar Wind, Sun: corona}
}

@Article{Karimabadi2013,
  Title                    = {Recent {Evolution} in the {Theory} of {Magnetic} {Reconnection} and {Its} {Connection} with {Turbulence}},
  Author                   = {Karimabadi, Homa and Roytershteyn, Vadim and Daughton, William and Liu, Yi-Hsin},
  Journal                  = {Space Sci. Rev.},
  Year                     = {2013},

  Month                    = sep,
  Number                   = {2-4},
  Pages                    = {307--323},
  Volume                   = {178},

  Doi                      = {10.1007/s11214-013-0021-7},
  ISSN                     = {0038-6308},
  Keywords                 = {magnetic, reconnection, turbulence},
  Url                      = {http://link.springer.com/10.1007/s11214-013-0021-7}
}

@Article{Karpen2008,
  Title                    = {Condensation {Formation} by {Impulsive} {Heating} in {Prominences}},
  Author                   = {Karpen, J. T. and Antiochos, S. K.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2008},

  Month                    = mar,
  Pages                    = {658--671},
  Volume                   = {676},

  Doi                      = {10.1086/526335},
  Keywords                 = {Sun: corona, Sun: magnetic fields, Sun: Prominences}
}

@Article{Kataoka2005,
  Title                    = {Magnetosheath variations during the storm main phase on 20 {November} 2003: {Evidence} for solar wind density control of energy transfer to the magnetosphere},
  Author                   = {Kataoka, R. and Fairfield, D. H. and Sibeck, D. G. and Rastätter, L. and Fok, M.-C. and Nagatsuma, T. and Ebihara, Y.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2005},
  Pages                    = {21108},
  Volume                   = {32},

  Abstract                 = {Energy transfer from the solar wind into the magnetosphere and ionosphere is controlled by the southward magnetic field in the magnetosheath which under normal high Mach number conditions is about four times the solar wind southward field. In a low Mach number regime, however, the magnetosheath compression is diminished by a low solar wind density when the magnetic field remains steady. When magnetic clouds with extremely strong magnetic field cause severe geomagnetic storms under such low Mach number conditions, the density control of the energy transfer is expected to be important in understanding ring current evolution. Here we show evidence for such a density effect using in-situ observation by the GOES and Cluster spacecraft in the magnetosheath during the main phase of the super storm on 20 November 2003. Results from a global magnetohydrodynamic (MHD) simulation with an embedded ring current model also support this density effect.},
  ISSN                     = {0094-8276},
  Keywords                 = {Interplanetary Physics: Ejecta driver gases and magnetic clouds Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Numerical modeling Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetic storms and substorms (7954)},
  Url                      = {http://adsabs.harvard.edu/abs/2005GeoRL..3221108K}
}

@Article{Kaufmann1969,
  Title                    = {Explorer 12 magnetopause observations: {Large}-scale nonuniform motion},
  Author                   = {Kaufmann, Richard L and Konradi, Andrei},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1969},
  Number                   = {14},
  Pages                    = {3609--3627},
  Volume                   = {74}
}

@Article{Kaymaz2001,
  Title                    = {Correlating near-{Earth} interplanetary magnetic fields: {Foreshock} effects},
  Author                   = {Kaymaz, Zerefsan and Sibeck, David G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2001},
  Pages                    = {18599--18614},
  Volume                   = {106},

  Abstract                 = {Interplanetary magnetic field (IMF) observations by ISEE 1 and IMP 8 were correlated to reveal the effects of upstream waves on IMF predictions. Past studies using spacecraft just outside the Earth's bow shock and far upstream at the L1 libration point attributed frequently poor ({\textless}=0.5) correlation coefficients to short IMF scale lengths and difficulties in estimating time delays. We find that the correlation coefficients for two near-Earth spacecraft are actually worse than those for a spacecraft at the L1 point and one just outside the bow shock: 48\% of the near-Earth correlation coefficients for the IMF magnitude are poor ({\textless}0.5), and only 17\% are good ({\textgreater}0.8). We attribute the poor result to two causes: (1) high-frequency waves and diamagnetic effects in the foreshock and (2) intervals of low IMF variance. Of these two, high-frequency waves account for 80\% of the cases with poor correlation, and the intervals of nearly constant IMF account for the remaining 20\% of the cases. While correlation coefficients do not increase with solar wind density while both spacecraft are in the solar wind, they do increase when one or both spacecraft lie within the foreshock. We argue that foreshock waves and intervals of low IMF variance must also have reduced correlation coefficients in previous IMF correlation studies. While the significance of the foreshock waves on the solar wind input into the magnetosphere deserves further study, there is no obstacle to predicting solar wind input into the magnetosphere during intervals with poor correlation coefficients but low IMF variance.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Discontinuities Interplanetary Physics: Planetary bow shocks},
  Url                      = {http://adsabs.harvard.edu/abs/2001JGR...10618599K}
}

@Article{Kazadzis2009,
  Title                    = {Ozone {Monitoring} {Instrument} spectral {UV} irradiance products: comparison with ground based measurements at an urban environment},
  Author                   = {Kazadzis, S. and Bais, A. and Arola, A. and Krotkov, N. and Kouremeti, N. and Meleti, C.},
  Journal                  = {Atmos. Chem. Phys.},
  Year                     = {2009},
  Number                   = {2},
  Pages                    = {585--594},
  Volume                   = {9},

  Shorttitle               = {Ozone {Monitoring} {Instrument} spectral {UV} irradiance products},
  Url                      = {http://www.atmos-chem-phys.net/9/585/2009/},
  Urldate                  = {2014-11-13}
}

@Article{Keika2009,
  Title                    = {Deformation and evolution of solar wind discontinuities through their interactions with the {Earth}'s bow shock},
  Author                   = {Keika, K. and Nakamura, R. and Baumjohann, W. and Angelopoulos, V. and Kabin, K. and Glassmeier, K. H. and Sibeck, D. G. and Magnes, W. and Auster, H. U. and Fornaçon, K. H. and McFadden, J. P. and Carlson, C. W. and Lucek, E. A. and Carr, C. M. and Dandouras, I. and Rankin, R.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2009},
  Volume                   = {114},

  Abstract                 = {The present study examines the interaction of solar wind discontinuities with the Earth's bow shock, using multipoint observations in the magnetosheath by Time History of Events and Macroscale Interactions During Substorms (THEMIS), Cluster, and Double Star TC1. We focus on the deformation and evolution of two discontinuities observed on 21 June 2007, one of which involves a density increase and a magnetic field decrease, while the other is accompanied by a density decrease and a magnetic field increase. In the magnetosheath, the discontinuities are deformed into a concave shape; that is, the normal is inclined toward dusk (dawn) on the dawnside (duskside). The density-increase (-decrease) discontinuity is being compressed (expanded) as it propagates in the magnetosheath. We conclude that the compression (expansion) is due to antisunward (sunward) motion of the bow shock which is initiated or enhanced by the impact of the discontinuity on the bow shock. The steepening of B {\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} reversal followed by an overshoot of the total magnetic field, which appears at the trailing edge of the density-decrease discontinuity, is also discussed.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Interplanetary Physics: Planetary bow shocks Magnetospheric Physics: Magnetosheath Interplanetary Physics: Interplanetary shocks},
  Url                      = {http://adsabs.harvard.edu/abs/2009JGRA..114.0C26K}
}

@Article{Kellogg1962,
  Title                    = {Flow of plasma around the earth},
  Author                   = {Kellogg, Paul J},
  Journal                  = {Journal of Geophysical Research},
  Year                     = {1962},
  Number                   = {10},
  Pages                    = {3805--3811},
  Volume                   = {67},

  Owner                    = {suleimanbaraka},
  Publisher                = {Wiley Online Library},
  Timestamp                = {2016.02.20}
}

@Article{Kessel1996,
  Title                    = {Evidence of high-latitude reconnecting during northward {IMF}: {Hawkeye} observations},
  Author                   = {Kessel, RL and Chen, S-H and Green, JL and Fung, SF and Boardsen, SA and Tan, LC and Eastman, TE and Craven, JD and Frank, LA},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1996},
  Number                   = {5},
  Pages                    = {583--586},
  Volume                   = {23}
}

@Article{Khazanov2015,
  Title                    = {Superthermal electron magnetosphere-ionosphere coupling in the diffuse aurora in the presence of {ECH} waves},
  Author                   = {Khazanov, G. V. and Tripathi, A. K. and Singhal, R. P. and Himwich, E. W. and Glocer, A. and Sibeck, D. G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2015},
  Pages                    = {445--459},
  Volume                   = {120},

  Abstract                 = {There are two main theories for the origin of the diffuse auroral electron precipitation: first, pitch angle scattering by electrostatic electron cyclotron harmonic (ECH) waves, and second, by whistler mode waves. Precipitating electrons initially injected from the plasma sheet to the loss cone via wave-particle interaction processes degrade in the atmosphere toward lower energies and produce secondary electrons via impact ionization of the neutral atmosphere. These secondary electrons can escape back to the magnetosphere, become trapped on closed magnetic field lines, and deposit their energy back to the inner magnetosphere. ECH and whistler mode waves can also move electrons in the opposite direction, from the loss cone into the trap zone, if the source of such electrons exists in conjugate ionospheres located at the same field lines as the trapped magnetospheric electron population. Such a situation exists in the simulation scenario of superthermal electron energy interplay in the region of diffuse aurora presented and discussed by Khazanov et al. (2014) and will be quantified in this paper by taking into account the interaction of secondary electrons with ECH waves.},
  ISSN                     = {0148-0227},
  Keywords                 = {magnetosphere-ionosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2015JGRA..120..445K}
}

@Article{Khodachenko2012,
  Title                    = {Magnetospheres of ‚Äù{Hot} {Jupiters}‚Äù: {The} {Importance} of {Magnetodisks} in {Shaping} a {Magnetospheric} {Obstacle}},
  Author                   = {Khodachenko, M. L. and Alexeev, I. and Belenkaya, E. and Lammer, H. and Grie{\textbackslash}textbackslashs smeier, J.-M. and Leitzinger, M. and Odert, P. and Zaqarashvili, T. and Rucker, H. O.},
  Journal                  = {{\textbackslash}textbackslashapj},
  Year                     = {2012},

  Month                    = jan,
  Pages                    = {70},
  Volume                   = {744},

  Doi                      = {10.1088/0004-637X/744/1/70},
  Keywords                 = {planets and satellites: magnetic fields, planets and satellites: physical evolution, planets and satellites: rings, planet-star interactions}
}

@Article{Khotyaintsev2004,
  Title                    = {Transient reconnection in the cusp during strongly negative {IMF} {B}$_{\textrm{y}}$\$},
  Author                   = {Khotyaintsev, Y. and Buchert, S. and Stasiewicz, K. and Vaivads, A. and Savin, S. and Papitashvili, V. O. and Farrugia, C. J. and Popielawska, B. and Tung, Y.-K.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = apr,
  Pages                    = {4204},
  Volume                   = {109},

  Doi                      = {10.1029/2003JA009908},
  Keywords                 = {and boundary layers, cusp, Ionosphere: Ionospheric dynamics, Magnetopause, Magnetospheric Physics: Magnetopause, Magnetospheric Physics: Magnetosphere/ionosphere interactions, Magnetospheric Physics: Magnetospheric configuration and dynamics, reconnection}
}

@Article{Khotyaintsev2004a,
  Title                    = {Transient reconnection in the cusp during strongly negative {IMF} {B}$_{\textrm{y}}$},
  Author                   = {Khotyaintsev, Y. and Buchert, S. and Stasiewicz, K. and Vaivads, A. and Savin, S. and Papitashvili, V. O. and Farrugia, C. J. and Popielawska, B. and Tung, Y.-K.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = apr,
  Pages                    = {4204},
  Volume                   = {109},

  Doi                      = {10.1029/2003JA009908},
  Keywords                 = {and boundary layers, cusp, Ionosphere: Ionospheric dynamics, Magnetopause, Magnetospheric Physics: Magnetopause, Magnetospheric Physics: Magnetosphere/ionosphere interactions, Magnetospheric Physics: Magnetospheric configuration and dynamics, reconnection}
}

@Article{Khotyaintsev2006,
  Title                    = {Formation of {Inner} {Structure} of a {Reconnection} {Separatrix} {Region}},
  Author                   = {Khotyaintsev, Y. V. and Vaivads, A. and Retinò, A. and André, M. and Owen, C. J. and Nilsson, H.},
  Journal                  = {Physical Review Letters},
  Year                     = {2006},

  Month                    = nov,
  Number                   = {20},
  Pages                    = {205003},
  Volume                   = {97},

  Doi                      = {10.1103/PhysRevLett.97.205003},
  Keywords                 = {Ionosphere/magnetosphere interactions, Magnetic reconnection, Magnetopause}
}

@Article{Khotyaintsev2006a,
  Title                    = {Formation of {Inner} {Structure} of a {Reconnection} {Separatrix} {Region}},
  Author                   = {Khotyaintsev, Y. V. and Vaivads, A. and Retin√≤, A. and Andr√©, M. and Owen, C. J. and Nilsson, H.},
  Journal                  = {Physical Review Letters},
  Year                     = {2006},

  Month                    = nov,
  Number                   = {20},
  Pages                    = {205003},
  Volume                   = {97},

  Doi                      = {10.1103/PhysRevLett.97.205003},
  Keywords                 = {Ionosphere/magnetosphere interactions, Magnetic reconnection, Magnetopause}
}

@Article{Killen2001,
  Title                    = {Evidence for space weather at {Mercury}},
  Author                   = {Killen, RM and Potter, AE and Reiff, P and Sarantos, M and Jackson, BV and Hick, P and Giles, B},
  Journal                  = {Journal of Geophysical Research: Planets (1991–2012)},
  Year                     = {2001},
  Number                   = {E9},
  Pages                    = {20509--20525},
  Volume                   = {106},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2000JE001401/full}
}

@Article{Kim2011,
  Title                    = {Evaluations of {NOx} and highly reactive {VOC} emission inventories in {Texas} and their implications for ozone plume simulations during the {Texas} {Air} {Quality} {Study} 2006},
  Author                   = {Kim, S. W. and McKeen, S. A. and Frost, G. J. and Lee, S. H. and Trainer, M. and Richter, A. and Angevine, W. M. and Atlas, E. and Bianco, L. and Boersma, K. F. and {others}},
  Journal                  = {Atmos. Chem. Phys.},
  Year                     = {2011},
  Number                   = {22},
  Pages                    = {11361--11386},
  Volume                   = {11},

  Url                      = {http://publications.lib.chalmers.se/publication/156532-evaluations-of-nox-and-highly-reactive-voc-emission-inventories-in-texas-and-their-implications-for},
  Urldate                  = {2014-11-13}
}

@Article{Kim2006,
  Title                    = {Satellite-observed {US} power plant {NOx} emission reductions and their impact on air quality},
  Author                   = {Kim, S-W and Heckel, Andreas and McKeen, SA and Frost, GJ and Hsie, E-Y and Trainer, MK and Richter, Andreas and Burrows, JP and Peckham, SE and Grell, GA},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2006},
  Number                   = {22},
  Volume                   = {33}
}

@TechReport{King1977,
  Title                    = {Interplanetary medium data book, appendix},
  Author                   = {King, Joseph H},
  Institution              = {National Aeronautics and Space Administration, Greenbelt, Md.(USA). Goddard Space Flight Center},
  Year                     = {1977}
}

@Article{Kipping2011,
  Title                    = {{LUNA}: an algorithm for generating dynamic planet-moon transits},
  Author                   = {Kipping, D. M.},
  Journal                  = {{\textbackslash}textbackslashmnras},
  Year                     = {2011},

  Month                    = sep,
  Pages                    = {689--709},
  Volume                   = {416},

  Doi                      = {10.1111/j.1365-2966.2011.19086.x},
  Keywords                 = {eclipses, methods: analytical, planetary systems, planets and satellites: general, TECHNIQUES: PHOTOMETRIC}
}

@Book{Kivelson1995,
  Title                    = {Introduction to space physics},
  Author                   = {Kivelson, Margaret G and Russell, Christopher T},
  Publisher                = {Cambridge university press},
  Year                     = {1995}
}

@Article{Klimov2002,
  Title                    = {Interball-1 and {MIR} orbital station coordinated magnetic field and energetic particles measurements},
  Author                   = {Klimov, SI and Grushin, VA and Lissakov, Yu V and Nozdrachev, MN and Petrukovich, AA and Grachev, EA and Grigoryan, OR and Lysakov, DS and Schwingenschuh, K and Auster, HU and {others}},
  Journal                  = {Advances in Space Research},
  Year                     = {2002},
  Number                   = {7},
  Pages                    = {1847--1853},
  Volume                   = {30}
}

@Article{Knizhnik2011,
  Title                    = {The acceleration of ions in solar flares during magnetic reconnection},
  Author                   = {Knizhnik, Kalman and Swisdak, Marc and Drake, James F.},
  Journal                  = {The Astrophysical Journal Letters},
  Year                     = {2011},
  Number                   = {2},
  Pages                    = {L35},
  Volume                   = {743},

  Url                      = {http://iopscience.iop.org/2041-8205/743/2/L35},
  Urldate                  = {2014-05-31}
}

@Article{Ko1997,
  Title                    = {An {Empirical} {Study} of the {Electron} {Temperature} and {Heavy} {Ion} {Velocities} in the {South} {Polar} {Coronal} {Hole}},
  Author                   = {Ko, Y.-K. and Fisk, L. A. and Geiss, J. and Gloeckler, G. and Guhathakurta, M.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {1997},

  Month                    = apr,
  Pages                    = {345--361},
  Volume                   = {171}
}

@Article{Ko1996,
  Title                    = {Limitations on suprathermal tails of electrons in the lower solar corona},
  Author                   = {Ko, Y.-K. and Fisk, L. A. and Gloeckler, G. and Geiss, J.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {1996},
  Pages                    = {2785--2788},
  Volume                   = {23},

  Doi                      = {10.1029/96GL02449},
  Keywords                 = {and Astronomy: Corona, ASTROPHYSICS, Solar Physics, Space Plasma Physics: Ionization processes}
}

@Article{Ko1998,
  Title                    = {On the differential ion velocity in the inner solar corona and the observed solar wind ionic charge states},
  Author                   = {Ko, Y.-K. and Geiss, J. and Gloeckler, G.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1998},

  Month                    = jul,
  Pages                    = {14539--14546},
  Volume                   = {103},

  Doi                      = {10.1029/98JA00763},
  Keywords                 = {and Astronomy: Coronal holes, ASTROPHYSICS, Solar Physics}
}

@Article{Korotova2004,
  Title                    = {Interplanetary magnetic field control of dayside transient event occurrence and motion in the ionosphere and magnetosphere},
  Author                   = {Korotova, G. and Sibeck, D. and Singer, H. and Rosenberg, T. and Engebretson, M.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2004},
  Pages                    = {4197--4202},
  Volume                   = {22},

  Abstract                 = {The pressure pulse model for dayside transient ionospheric events predicts dawnward moving events at and prior to local noon during periods of spiral interplanetary magnetic field (IMF) orientation, but duskward moving events at and after local noon during rarer periods of orthospiral IMF orientation. We use this model to interpret ground and geosynchronous magnetometer observations of a duskward-moving transient event that occurred on 10 August 1995 during a period of orthospiral IMF orientation. We then survey geosynchronous GOES-8, 9, and 10 magnetometer observations to determine the directions of motion for 67 isolated magnetic impulse events seen in South Pole magnetograms from 1995-1999. The occurrence patterns and directions of motion inferred from both case and statistical studies are consistent with pressure pulse model predictions.},
  ISSN                     = {0992-7689},
  Url                      = {http://adsabs.harvard.edu/abs/2004AnGeo..22.4197K}
}

@Article{Korotova2001,
  Title                    = {Erratum: “{Multipoint} observations of global magnetospheric compressions”},
  Author                   = {Korotova, G. I. and Kivelson, M. G. and Sibeck, D. G. and Potemra, T. A. and Stauning, P.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2001},
  Pages                    = {8491--8491},
  Volume                   = {106},

  Abstract                 = {Not Available},
  ISSN                     = {0148-0227},
  Keywords                 = {Corrections},
  Url                      = {http://adsabs.harvard.edu/abs/2001JGR...106.8491K}
}

@Article{Korotova2000,
  Title                    = {Multipoint observations of global magnetospheric compressions},
  Author                   = {Korotova, G. I. and Kivelson, M. G. and Sibeck, D. G. and Potemra, T. A. and Stauning, P.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2000},
  Pages                    = {23293--23302},
  Volume                   = {105},

  Abstract                 = {The magnetic field experiment on the Viking satellite detected long-period compressional oscillations with amplitudes ranging from 2 to 5 nT and periods ranging from 7 to 23 min on nine Viking orbits covering a wide range of polar and subauroral latitudes during the period from March to August 1986. We present a case study of an event on June 18, 1996, in which similar long-period pulsations were also observed by a global network of more than 50 ground magnetometers and by the GOES-5 and GOES-6 spacecraft. The magnetic field variations throughout the auroral, midlatitude, and equatorial regions, at Viking, GOES-5, and GOES-6 were approximately in phase, whereas the variations at some morningside stations were a half-wave period out of phase. We interpret these long-period oscillations as evidence for periodic compressions and inflations of the magnetosphere driven by solar wind pressure pulses. The relative time delays of the peak variations observed by GOES-5, GOES-6, Viking, and the ground-based stations are consistent with an event originating on the prenoon magnetopause whose signatures spread both poleward and antisunward on both sides of local noon.},
  ISSN                     = {0148-0227},
  Keywords                 = {magnetospheric physics},
  Url                      = {http://adsabs.harvard.edu/abs/2000JGR...10523293K}
}

@Article{Korotova2013,
  Title                    = {{THEMIS} observations of compressional poloidal pulsations in the dawnside magnetosphere: {A} case study},
  Author                   = {Korotova, G. I. and Sibeck, D. G. and Angelopoulos, V. and Walsh, B. M.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},
  Pages                    = {7665--7673},
  Volume                   = {118},

  Abstract                 = {We present results from a case study of compressional poloidal pulsations with periods ranging from 5 to 12 min in the dawn magnetosphere from 1630 to 2000 UT on 27 February 2011. However, we employ THEMIS (Time History of Events and Macroscale Interactions during Substorms) magnetic field, plasma, and energetic particle observations to determine azimuthal wavelengths (7000-27,000 km) and velocities (9-28 km/s) consistent with previous work. We then apply a new method invoking the north to south motion of the THEMIS spacecraft and the fact that the equatorial node exhibited north-south oscillations to derive the meridional structure of the wave in great detail. We determined that the amplitude of the meridional motion of the equatorial node was 0.8 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}, and that the meridional wave length exceeded 3 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}.},
  ISSN                     = {0148-0227},
  Keywords                 = {ulf waves},
  Url                      = {http://adsabs.harvard.edu/abs/2013JGRA..118.7665K}
}

@Article{Korotova1999,
  Title                    = {Tracking transient events through geosynchronous orbit},
  Author                   = {Korotova, G. I. and Sibeck, D. G. and Moretto, T. and Reeves, G. D.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1999},
  Pages                    = {10265--10274},
  Volume                   = {104},

  Abstract                 = {Impulsive events in high-latitude dayside ground magnetograms provide evidence for one or more modes of unsteady solar wind-magnetosphere interaction. We use geosynchronous magnetic field and energetic electron observations to demonstrate that the events correspond to abrupt global variations in both the magnetospheric magnetic field strength and the energetic electron flux and that these variations are particularly marked in the dayside magnetosphere. The multiple spacecraft observations suggest that the events move both dawnward and duskward from a point of origin on the prenoon magnetopause during periods of orthospiral, duskward, and northward interplanetary magnetic field orientation. Event properties are consistent with an interpretation in terms of widespread solar wind pressure fronts striking the bow shock and magnetopause.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetosphere-outer Ionosphere: Auroral ionosphere},
  Url                      = {http://adsabs.harvard.edu/abs/1999JGR...10410265K}
}

@Article{Korotova2012,
  Title                    = {{THEMIS observations of unusual bow shock motion attending a transient magnetospheric event}},
  Author                   = {Korotova, G. I. and Sibeck, D. G. and Omidi, N. and Angelopoulos, V.},
  Journal                  = {J. Geophys. Res. Sp. Phys.},
  Year                     = {2012},
  Number                   = {12},
  Volume                   = {117},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {We present a multipoint case study of solar wind and magnetospheric observations during a transient magnetospheric compression at 23:19 UT on 15 October 2008. We use high time resolution magnetic field and plasma data from the THEMIS and GOES 11/12 spacecraft to show that this transient event corresponded to an abrupt rotation in the IMF orientation, a change in the location of the foreshock, and transient outward bow shock motion. We employ results from a global hybrid code model to reconcile the observations indicating transient inward magnetopause motion with the outward bow shock motion.},
  Doi                      = {10.1029/2012JA017510},
  ISBN                     = {2156-2202},
  ISSN                     = {21699402},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Korotova2012a,
  Title                    = {{THEMIS} observations of unusual bow shock motion attending a transient magnetospheric event},
  Author                   = {Korotova, G. I. and Sibeck, D. G. and Omidi, N. and Angelopoulos, V.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2012},
  Pages                    = {12207},
  Volume                   = {117},

  Abstract                 = {We present a multipoint case study of solar wind and magnetospheric observations during a transient magnetospheric compression at 23:19 UT on 15 October 2008. We use high time resolution magnetic field and plasma data from the THEMIS and GOES 11/12 spacecraft to show that this transient event corresponded to an abrupt rotation in the IMF orientation, a change in the location of the foreshock, and transient outward bow shock motion. We employ results from a global hybrid code model to reconcile the observations indicating transient inward magnetopause motion with the outward bow shock motion.},
  ISSN                     = {0148-0227},
  Keywords                 = {THEMIS bow shock discontinuity transient event Interplanetary Physics: Discontinuities (7811) Interplanetary Physics: Planetary bow shocks Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Solar wind/magnetosphere interactions Space Weather: Models},
  Url                      = {http://adsabs.harvard.edu/abs/2012JGRA..11712207K}
}

@Article{Korotova2008,
  Title                    = {Seasonal dependence of {Interball} flux transfer events},
  Author                   = {Korotova, G. I. and Sibeck, D. G. and Rosenberg, T.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2008},
  Pages                    = {5106},
  Volume                   = {35},

  Abstract                 = {J. Raeder (2006) presented the results of a global magnetohydrodynamic simulation indicating that flux transfer events (FTEs) form solely in the winter hemisphere and move poleward in the direction of the background magnetosheath flow during periods of strongly southward interplanetary magnetic field (IMF) orientation. This paper presents results from a statistical survey of flux transfer FTEs observed on the mid-latitude northern and southern magnetopause by the magnetometer on the Interball-1 spacecraft over the course of its five-year mission from 1995 to 1999. Interball-1 observations confirm that FTEs exhibit a strong tendency to occur in the winter hemisphere.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Interplanetary Physics: Interplanetary magnetic fields},
  Url                      = {http://adsabs.harvard.edu/abs/2008GeoRL..35.5106K}
}

@Article{Korotova2008a,
  Title                    = {Interball observations of multiple flux transfer events},
  Author                   = {Korotova, G. I. and Sibeck, D. G. and Rosenberg, T. and Petrov, V. and Styazhkin, V.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2008},
  Pages                    = {391--398},
  Volume                   = {70},

  Abstract                 = {We present results from a statistical study of multiple flux transfer events (FTEs) observed by the Interball-1 spacecraft during 1995-1999. We identified 21 days on which Interball-1 observed 10 or more FTEs. In a database of 807 FTEs, 319 can be identified as multiple FTEs with recurrence times ranging between 50 s and 20 min. Multiple events occur at both equatorial and high latitudes but are most frequently seen on Interball-1 passes that graze the flanks of the magnetosphere. The peak-to-peak amplitudes of multiple FTE Bn signatures vary from 3 to 20 nT but typically lie in the range from 3 to 9 nT, less than amplitudes typical for the FTE database as a whole. The durations of individual FTEs increase with increasing inter-arrival times during sequences of multiple FTEs. Multiple FTEs show a marked tendency to occur for southward IMF orientations, but no preference for high or low solar wind dynamic pressures or velocity. Since the conditions favoring the occurrence of multiple FTEs are similar to those for FTEs as a whole, we conclude that sequences of multiple FTEs must be the norm during periods of southward IMF orientation.},
  ISSN                     = {1364-6826},
  Keywords                 = {Magnetic reconnection Magnetopause Solar wind Flux transfer events},
  Url                      = {http://adsabs.harvard.edu/abs/2008JASTP..70..391K}
}

@Article{Korotova1997,
  Title                    = {High-latitude ionospheric transient events in a global context},
  Author                   = {Korotova, G. I. and Sibeck, D. G. and Rosenberg, T. J. and Russell, C. T. and Friis-Christensen, E.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1997},
  Pages                    = {17499--17508},
  Volume                   = {102},

  Abstract                 = {This paper presents a comprehensive global study of bow shock motion, magnetosheath dynamic pressure variations, dayside magnetospheric magnetic field perturbations, and cosmic noise absorption events attending a sequence of transient events observed in high-latitude global ground magnetograms on February 14, 1986. ISEE 2 spacecraft observations indicated that most of the transient ground magnetometer events were associated with abrupt inward and outward motions of the dawn bow shock during a prolonged period of strongly northward and orthospiral interplanetary magnetic field orientation. Geosynchronous GOES 5 and 6 magnetometer observations provide evidence for corresponding compressions and expansions, which propagated duskward through the prenoon magnetosphere. The magnetopause moved inward past the CCE spacecraft during some of the compressions. The compressions scattered magnetospheric particles and thereby produced quasi-periodic oscillations in the cosmic noise absorption recorded by high-latitude ground riometers. We infer that (unobserved) strong transient variations in the solar wind dynamic pressure produced the various phenomena and that the ground magnetometer signatures are best explained in terms of the pressure pulse model of Southwood and Kivelson [1990], in which a single sharp change in the solar wind dynamic pressure generates a pair of field-aligned currents.},
  ISSN                     = {0148-0227},
  Keywords                 = {Ionosphere: Ionosphere/magnetosphere interactions Ionosphere: Polar cap ionosphere Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetosheath},
  Url                      = {http://adsabs.harvard.edu/abs/1997JGR...10217499K}
}

@Article{Korotova2002,
  Title                    = {Tracking transient events through geosynchronous orbit and in the high-latitude ionosphere},
  Author                   = {Korotova, G. I. and Sibeck, D. G. and Singer, H. J. and Rosenberg, T. J.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2002},
  Pages                    = {1345},
  Volume                   = {107},

  Abstract                 = {We combine observations from seven satellites and more than 50 ground magnetometers to study a series of impulsive ground magnetometer events that originated in response to sudden solar wind plasma and interplanetary magnetic field variations on an otherwise quiet day. We demonstrate that the events were global and conjugate. We use high time resolution geosynchronous magnetometer data to determine the origin, velocity, and direction of propagation of the transient events in the magnetosphere. We show that the transient events propagated antisunward but that the IMF orientation controlled the direction of their propagation near local noon in the sense predicted by the dynamic pressure pulse model.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetosphere/ionosphere interactions Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetosphere-outer},
  Url                      = {http://adsabs.harvard.edu/abs/2002JGRA..107.1345K}
}

@Article{Korotova2011,
  Title                    = {{THEMIS} observations of a transient event at the magnetopause},
  Author                   = {Korotova, G. I. and Sibeck, D. G. and Weatherwax, A. and Angelopoulos, V. and Styazhkin, V.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2011},
  Pages                    = {7224},
  Volume                   = {116},

  Abstract                 = {This study focuses on Time History of Events and Macroscale Interactions During Substorms (THEMIS) observations of a long-duration transient event in the vicinity of the dayside magnetopause at ˜15:34 UT on 18 July 2008 that was characterized by features typical of a magnetospheric flux transfer event (FTE): a bipolar negative-positive 5-7 nT signature in the Bn component, a positive monopolar variation in the Bl and Bm components, a ˜5-7 nT enhancement in the total magnetic field strength, and a transient density and flow enhancement. The interplanetary magnetic field (IMF) was mostly radial and disturbed during the intervals studied; that is, it was favorable for the repeated formation, disappearance and reformation of the foreshock just upstream from the subsolar bow shock. We show that varying IMF directions and solar wind pressures created significant effects that caused the compressions of the magnetosphere and the bow shock and magnetopause motions and triggered the transient event. Global signatures of magnetic impulse events (MIEs) in ground magnetograms during the period suggest a widespread pressure pulse instead of a localized FTE as the cause of the event in the magnetosphere. The directions of propagation and the flow patterns associated with the event also suggest an interpretation in terms of pressure pulses.},
  ISSN                     = {0148-0227},
  Keywords                 = {Ionosphere: Ionosphere/magnetosphere interactions (2736) Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Magnetosphere/ionosphere interactions (2431)},
  Url                      = {http://adsabs.harvard.edu/abs/2011JGRA..116.7224K}
}

@Article{Koval2005,
  Title                    = {Deformation of interplanetary shock fronts in the magnetosheath},
  Author                   = {Koval, A. and Šafránková, J. and Němeček, Z. and Přech, L. and Samsonov, A. A. and Richardson, J. D.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {2005},

  Month                    = aug,
  Pages                    = {15101},
  Volume                   = {32},

  Doi                      = {10.1029/2005GL023009},
  Keywords                 = {Interplanetary Physics: Interplanetary shocks, Magnetospheric Physics: Magnetosheath, Magnetospheric Physics: Solar wind/magnetosphere interactions}
}

@Article{Koval2006,
  Title                    = {Interplanetary shock in the magnetosheath: {Comparison} of experimental data with {MHD} modeling},
  Author                   = {Koval, A. and Šafránková, J. and Němeček, Z. and Samsonov, A. A. and Přech, L. and Richardson, J. D. and Hayosh, M.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {2006},

  Month                    = jun,
  Pages                    = {11102},
  Volume                   = {33},

  Doi                      = {10.1029/2006GL025707},
  Keywords                 = {Interplanetary Physics: Interplanetary shocks, Magnetospheric Physics: Magnetosheath, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Solar wind/magnetosphere interactions}
}

@Article{Kowal2011,
  Title                    = {Magnetohydrodynamic simulations of reconnection and particle acceleration: three-dimensional effects},
  Author                   = {Kowal, Grzegorz and Dal Pino, EM de Gouveia and Lazarian, A},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2011},
  Number                   = {2},
  Pages                    = {102},
  Volume                   = {735}
}

@Article{Kozyra2013,
  Title                    = {Earth's collision with a solar filament on 21 {January} 2005: {Overview}},
  Author                   = {Kozyra, J. U. and Manchester, W. B. and Escoubet, C. P. and Lepri, S. T. and Liemohn, M. W. and Gonzalez, W. D. and Thomsen, M. W. and Tsurutani, B. T.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = oct,
  Pages                    = {5967--5978},
  Volume                   = {118},

  Doi                      = {10.1002/jgra.50567},
  Keywords                 = {Coronal Mass Ejection, Magnetic reconnection, magnetotail, plasma sheet, solar filament}
}

@InCollection{Krasnoselskikh2014,
  Title                    = {The dynamic quasiperpendicular shock: {Cluster} discoveries},
  Author                   = {Krasnoselskikh, V and Balikhin, M and Walker, SN and Schwartz, S and Sundkvist, D and Lobzin, V and Gedalin, M and Bale, SD and Mozer, F and Soucek, J and {others}},
  Booktitle                = {Microphysics of {Cosmic} {Plasmas}},
  Publisher                = {Springer},
  Year                     = {2014},
  Pages                    = {459--522}
}

@Article{Krasnoselskikh2013,
  Title                    = {The {Dynamic} {Quasiperpendicular} {Shock}: {Cluster} {Discoveries}},
  Author                   = {Krasnoselskikh, V. and Balikhin, M. and Walker, S. N. and Schwartz, S. and Sundkvist, D. and Lobzin, V. and Gedalin, M. and Bale, S. D. and Mozer, F. and Soucek, J. and Hobara, Y. and Comisel, H.},
  Journal                  = {Space Sci. Rev.},
  Year                     = {2013},

  Month                    = mar,
  Number                   = {2-4},
  Pages                    = {535--598},
  Volume                   = {178},

  Doi                      = {10.1007/s11214-013-9972-y},
  ISSN                     = {0038-6308},
  Url                      = {http://link.springer.com/10.1007/s11214-013-9972-y}
}

@Article{Krauss-Varban1995,
  Title                    = {Electron dynamics and whistler waves at quasi-perpendicular shocks},
  Author                   = {Krauss-Varban, D and Pantellini, FGE and Burgess, D},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1995},
  Number                   = {16},
  Pages                    = {2091--2094},
  Volume                   = {22}
}

@Article{Krimigis1992,
  Title                    = {Voyager energetic particle observations at interplanetary shocks and upstream of planetary bow shocks: 1977–1990},
  Author                   = {Krimigis, SM},
  Journal                  = {Space science reviews},
  Year                     = {1992},
  Number                   = {1-2},
  Pages                    = {167--201},
  Volume                   = {59}
}

@InProceedings{Krimigis1986,
  Title                    = {Energetic ions upstream of planetary bow shocks-{Fermi} acceleration or leakage?},
  Author                   = {Krimigis, SM},
  Booktitle                = {Comparative {Study} of {Magnetospheric} {Systems}},
  Year                     = {1986},
  Pages                    = {99--124},
  Volume                   = {1}
}

@Article{Kronberg2011,
  Title                    = {On the origin of the energetic ion events measured upstream of the {Earth}'s bow shock by {STEREO}, {Cluster}, and {Geotail}},
  Author                   = {Kronberg, EA and Bučík, R and Haaland, S and Klecker, B and Keika, K and Desai, MI and Daly, PW and Yamauchi, M and Gómez-Herrero, R and Lui, ATY},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2011},
  Number                   = {A2},
  Volume                   = {116}
}

@Article{Krotkov2008,
  Title                    = {Validation of {SO}2 retrievals from the {Ozone} {Monitoring} {Instrument} over {NE} {China}},
  Author                   = {Krotkov, Nickolay A. and McClure, Brittany and Dickerson, Russell R. and Carn, Simon A. and Li, Can and Bhartia, Pawan K. and Yang, Kai and Krueger, Arlin J. and Li, Zhanqing and Levelt, Pieternel F. and {others}},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2008},
  Number                   = {D16},
  Volume                   = {113},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2007JD008818/full},
  Urldate                  = {2014-11-13}
}

@Article{Ku2000,
  Title                    = {Flux transfer events produced by the onset of merging at multiple {X} lines},
  Author                   = {Ku, Hwar C. and Sibeck, David G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2000},
  Pages                    = {2657--2676},
  Volume                   = {105},

  Abstract                 = {We present two-dimensional magnetohydrodynamic model predictions for the signatures of flux transfer events (FTEs) at the dayside magnetopause produced by the onset of merging along two or more extended X lines. We consider three scenarios: (1) equal merging rates with identical resistivities south (ɛ{\textless}SUB{\textgreater}1{\textless}/SUB{\textgreater}) and north (ɛ{\textless}SUB{\textgreater}2{\textless}/SUB{\textgreater}) of the equator, (2) unequal merging rates with ɛ{\textless}SUB{\textgreater}1{\textless}/SUB{\textgreater}{\textgreater}ɛ{\textless}SUB{\textgreater}2{\textless}/SUB{\textgreater}, and (3) equal merging rates in the presence of a background northward magnetosheath flow velocity (V{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater}=0.15B{\textless}SUB{\textgreater}sph{\textless}/SUB{\textgreater}/{\textless}radical{\textgreater}{\textless}radicand{\textgreater}ρ{\textless}SUB{\textgreater}msh{\textless}/SUB{\textgreater}μ{\textless}SUB{\textgreater}0{\textless}/SUB{\textgreater}{\textless}/radicand{\textgreater}{\textless}/radical{\textgreater}). Realistic ratios of magnetosheath to magnetospheric parameters are chosen to conform with in situ observations and our previous simulations [Ku and Sibeck, 1997, 1998a, b]: ρ{\textless}SUB{\textgreater}msh{\textless}/SUB{\textgreater}/ρ{\textless}SUB{\textgreater}sph{\textless}/SUB{\textgreater}=10, B{\textless}SUB{\textgreater}msh{\textless}/SUB{\textgreater}/B{\textless}SUB{\textgreater}sph{\textless}/SUB{\textgreater}=0.5, and T{\textless}SUB{\textgreater}msh{\textless}/SUB{\textgreater}/T{\textless}SUB{\textgreater}sph{\textless}/SUB{\textgreater}=0.175. In case 1, a stationary magnetic island forms between two bulges accelerating away from the subsolar point. In case 2, the magnetic island formed between the two X lines pursues the bulge created near the line with smaller resistivity. In case 3 the island formed between the two X lines pursues the bulge by moving in the direction of the background flow. All three scenarios produce events with characteristics similar to those in the single X line model: strong asymmetric bipolar magnetic fields and plasma velocities normal to the magnetopause in the magnetosheath and no significant signatures in the magnetosphere (with the magnitude of the trailing pulse exceeding that of the leading edge). However, the islands produced in cases 2 and 3 also generate more symmetric signatures typical of FTEs in both the magnetosheath and magnetosphere. By comparison with observations, the transition parameter plots that we present can be used to discriminate between the merging scenarios.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2000JGR...105.2657K}
}

@Article{Ku1998,
  Title                    = {{Flux transfer events produced by bursty merging at a single X line}},
  Author                   = {Ku, Hwar C. and Sibeck, David G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1998},
  Number                   = {A7},
  Pages                    = {14965},
  Volume                   = {103},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {We present predictions for the signatures of flux transfer events (FTEs) at the dayside magnetopause produced by bursty merging at a single extended X line. In this MHD model, the time-dependent enhanced local resistivity turns on at a low northern latitude for a brief time and then turns off. Realistic ratios of magnetosheath to magnetosphere parameters are chosen to conform with observations and our previous simulations [Ku and Sibeck, 1997, 1998]: $\rho$<SUB>msh</SUB>/$\rho$<SUB>sph</SUB>=10, B<SUB>msh</SUB>/B<SUB>sph</SUB>=0.5, and T<SUB>msh</SUB>/T<SUB>sph</SUB>=0.175. The burst of merging produces FTEs marked by strongly asymmetric bipolar magnetic field and plasma velocities normal to the magnetopause in the magnetosheath and no significant signatures in the magnetosphere, just as in the previously studied case for the step-function onset of merging [Ku and Sibeck, 1997]. However, the simulation produces other FTE signatures that differ strikingly from those generated by the step-function onset of merging. After the resistivity is switched off, one or more secondary reconnection sites appear on the trailing edge of the events. Merging at these sites inflates and propels the main FTE as it moves out of the simulation domain. Merging at these sites also fills a magnetic island with hot tenuous plasma near the subsolar (symmetry) point. Transient magnetic islands form on the trailing edge of the main FTE, but these remain small and may disappear. Scatterplots of various parameters versus the plasma density reveal that steep changes for the temperature kT, magnetic field B<SUB>z</SUB>, and the Alfv{\'{e}}n velocity occur on the magnetosheath side immediately adjacent to the magnetopause and also reflect the fact that the events scarcely deform the magnetopause.},
  Doi                      = {10.1029/98JA01171},
  ISSN                     = {0148-0227},
  Keywords                 = {http://dx.doi.org/10.1029/98JA01171, doi:10.1029/9},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Ku1998a,
  Title                    = {Flux transfer events produced by bursty merging at a single {X} line},
  Author                   = {Ku, Hwar C. and Sibeck, David G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1998},
  Pages                    = {14965--14978},
  Volume                   = {103},

  Abstract                 = {We present predictions for the signatures of flux transfer events (FTEs) at the dayside magnetopause produced by bursty merging at a single extended X line. In this MHD model, the time-dependent enhanced local resistivity turns on at a low northern latitude for a brief time and then turns off. Realistic ratios of magnetosheath to magnetosphere parameters are chosen to conform with observations and our previous simulations [Ku and Sibeck, 1997, 1998]: ρ{\textless}SUB{\textgreater}msh{\textless}/SUB{\textgreater}/ρ{\textless}SUB{\textgreater}sph{\textless}/SUB{\textgreater}=10, B{\textless}SUB{\textgreater}msh{\textless}/SUB{\textgreater}/B{\textless}SUB{\textgreater}sph{\textless}/SUB{\textgreater}=0.5, and T{\textless}SUB{\textgreater}msh{\textless}/SUB{\textgreater}/T{\textless}SUB{\textgreater}sph{\textless}/SUB{\textgreater}=0.175. The burst of merging produces FTEs marked by strongly asymmetric bipolar magnetic field and plasma velocities normal to the magnetopause in the magnetosheath and no significant signatures in the magnetosphere, just as in the previously studied case for the step-function onset of merging [Ku and Sibeck, 1997]. However, the simulation produces other FTE signatures that differ strikingly from those generated by the step-function onset of merging. After the resistivity is switched off, one or more secondary reconnection sites appear on the trailing edge of the events. Merging at these sites inflates and propels the main FTE as it moves out of the simulation domain. Merging at these sites also fills a magnetic island with hot tenuous plasma near the subsolar (symmetry) point. Transient magnetic islands form on the trailing edge of the main FTE, but these remain small and may disappear. Scatterplots of various parameters versus the plasma density reveal that steep changes for the temperature kT, magnetic field B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater}, and the Alfvén velocity occur on the magnetosheath side immediately adjacent to the magnetopause and also reflect the fact that the events scarcely deform the magnetopause.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers},
  Url                      = {http://adsabs.harvard.edu/abs/1998JGR...10314965K}
}

@Article{Ku1998b,
  Title                    = {The effect of magnetosheath plasma flow on flux transfer events produced by the onset of merging at a single {X} line},
  Author                   = {Ku, Hwar C. and Sibeck, David G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1998},
  Pages                    = {6693--6702},
  Volume                   = {103},

  Abstract                 = {We present predictions on the signatures of flux transfer events (FTEs) at the dayside magnetopause by the single X line MHD model based on the subsolar environment: initially in the magnetosheath with background flow northward parallel to the dayside magnetopause. In conformity with our previous investigation [Ku and Sibeck, 1997] we choose realistic parameteres for the simulation with the ratio of ρ{\textless}SUB{\textgreater}msh{\textless}/SUB{\textgreater}/ρ{\textless}SUB{\textgreater}sph{\textless}/SUB{\textgreater}=10, B{\textless}SUB{\textgreater}msh{\textless}/SUB{\textgreater}/B{\textless}SUB{\textgreater}sph{\textless}/SUB{\textgreater}=0.5, and T{\textless}SUB{\textgreater}msh{\textless}/SUB{\textgreater}/T{\textless}SUB{\textgreater}sph{\textless}/SUB{\textgreater}=0.175 along the magnetosheath and magnetospheric sides. The localized resistivity turns on near the low northern latitude of dayside magnetopause, and the initial magnitude of background magnetosheath plasma flow is set 0.15V{\textless}SUB{\textgreater}A0{\textless}/SUB{\textgreater} (B{\textless}SUB{\textgreater}sph{\textless}/SUB{\textgreater}/{\textless}radical{\textgreater}{\textless}radicand{\textgreater}ρ{\textless}SUB{\textgreater}msh{\textless}/SUB{\textgreater}μ{\textless}SUB{\textgreater}0{\textless}/SUB{\textgreater}{\textless}/radicand{\textgreater}{\textless}/radical{\textgreater}), or equivalent to 30\% of magnetosheath Alfvén velocity. Simulation results produce signatures of FTEs similar to the previous case without the background magnetosheath flow [Ku and Sibeck, 1997] but different in some respects. Events moving opposite to this flow slow down but intensify, whereas events moving in the direction of the magnetosheath flow accelerate but weaken. Similarly, the satellite observes no significant signatures of FTEs in the magnetosphere. All the FTEs exhibit asymmetric bipolar magnetic field signatures normal to the magnetopause. Scatterplots versus the plasma density reveal that steep changes for the temperature kT, the magnetic field B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater}, and the Alfvén velocity occur in the magnetospheric side immediately adjacent to the magnetopause.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Storms and substorms Space Plasma Physics: Magnetic reconnection},
  Url                      = {http://adsabs.harvard.edu/abs/1998JGR...103.6693K}
}

@Article{Ku1997,
  Title                    = {Internal structure of flux transfer events produced by the onset of merging at a single {X} line},
  Author                   = {Ku, Hwar C. and Sibeck, David G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1997},
  Pages                    = {2243--2260},
  Volume                   = {102},

  Abstract                 = {We present a new, higher-order, two-dimensional, magnetohydrodynamic model for the detailed internal structure of bubbles produced by the onset of merging along a single subsolar X line. The key feature of the model is to implement a nonlinear filter to postprocess results provided by the pseudospectral element method. The devised nonlinear filter (1) eliminates only the high-frequency oscillations, (2) retains conservation laws, and (3) enforces a total variation diminished criterion to guarantee the elimination of spurious oscillations near discontinuities. For realistic parameters, the model predicts that satellites which remain in the magnetosheath will observe asymmetric bipolar magnetic field signatures normal to the magnetopause, magnetic field strength increases, density and temperature decreases, and velocities opposite the motion of the events. Satellites in the magnetosheath which enter the events observe asymmetric bipolar signatures normal to the magnetopause, magnetic field strength decreases, densities intermediate between those in the magnetosheath and magnetosphere, temperature increases, and velocities in the direction of event motion. Satellites initially located just outside the magnetopause observe greatly depressed densities and enhanced temperatures (but no significant bipolar signatures normal to the magnetopause) followed by velocity jets of magnetosheath-like plasma on northward magnetospheric magnetic field lines. Satellites in the magnetosphere which enter the events observe depressed magnetic field strengths, enhanced densities and temperatures, and accelerated flows surrounding a core region of accelerated magnetosheath-like plasma. Neither they nor satellites which remain in the magnetosphere observe any significant bipolar signatures normal to the nominal magnetopause.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetosheath Space Plasma Physics: Magnetic reconnection Space Plasma Physics: Numerical simulation studies},
  Url                      = {http://adsabs.harvard.edu/abs/1997JGR...102.2243K}
}

@Article{Kudela2005,
  Title                    = {{DOK}-2 ion fluxes upstream from the bow shock: characteristics from 4 years of {Interball}-1 measurements},
  Author                   = {Kudela, K. and Lutsenko, V. N. and Sarris, E. T. and Sibeck, D. G. and Slivka, M.},
  Journal                  = {Planetary and Space Science},
  Year                     = {2005},
  Pages                    = {59--64},
  Volume                   = {53},

  Abstract                 = {The spectrometer DOK-2 on Interball-1 provided energetic (˜20-˜600 keV) ion fluxes and spectra for various geomagnetic and interplanetary conditions during the spacecraft's 5-year mission. From April to July in 1996-2000, the spacecraft's apogee lay upstream from the dayside bow shock. We present observations of the diffusive ion flux in the upstream region as a function of energy, magnetic field connection and distance to the position of a model bow shock, solar wind velocity, and geomagnetic activity for years 1996-1998 and a part of year 1999. Measurements by both ion detectors combined into 14 energy ranges are used for the analysis. Although fluxes of ions with energies up to ˜150 keV depend primarily upon the geometry of the connection to the bow shock, the dependence of fluxes on geomagnetic activity, indicating the important contribution of particles leaking the magnetosphere, increases with the energy.},
  ISSN                     = {0032-0633},
  Url                      = {http://adsabs.harvard.edu/abs/2005P%26SS...53...59K}
}

@Article{Kudela2002,
  Title                    = {Energetic ions upstream of the {Earth}'s bow shock: {INTERBALL}-1 survey},
  Author                   = {Kudela, K. and Lutsenko, V. N. and Sibeck, D. G. and Slivka, M.},
  Journal                  = {Advances in Space Research},
  Year                     = {2002},
  Pages                    = {2731--2736},
  Volume                   = {30},

  Abstract                 = {A statistical survey of energetic ions ({\textgreater} 20 keV) observed by the DOK2 experiment on Interball-1 during foreshock intervals from 1996 to 1998 is presented. Flux levels depend on the connection geometry, with higher values at quasi-parallel shocks, particularly at lower energies. The decrease of flux in diffusive events with distance from the bow shock is consistent with results from earlier surveys performed closer to the bow shock. The energy spectra are softer for quasi-parallel than quasi-perpendicular connections. The reflected ions have musch softer spectra. The cumulative frequencies for flux level occurrence patterns exhibit differences for quasi-parallel and quasi-perpendicular geometries up to approximately 200 keV.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/2002AdSpR..30.2731K}
}

@Article{Kudela2002a,
  Title                    = {Energetic ions and electrons within the magnetosheath and upstream of the bow shock: {Interball}-1 overview},
  Author                   = {Kudela, K. and Lutsenko, V. N. and Sibeck, D. G. and Slivka, M.},
  Journal                  = {Advances in Space Research},
  Year                     = {2002},
  Pages                    = {1685--1692},
  Volume                   = {30},

  Abstract                 = {We present the results of a statistical survey of Interball-1 DOK-2 energetic ( E {\textgreater} 20 keV) ion and electron observations in the solar wind and magnetosheath. Using four years of 2-min averages, we demonstrate the manner by which solar wind parameters control energetic particle fluxes within the foreshock. As the angle between the interplanetary magnetic field (IMF) and the normal to the bow shock decreases, ion flux increase and ion spectra soften. Ion spectra harden for higher solar wind velocities and greater geomagnetic activity. While ion fluxes generally decrease with distance from the magnetopause, the flux of ions also increases when the angle between the IMF and the normal to the bow shock decreases, particularly at low energies.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/2002AdSpR..30.1685K}
}

@Article{Kudela2002b,
  Title                    = {High energy particle dispersion events observed by interball-1 and -2},
  Author                   = {Kudela, K. and Lutsenko, V. N. and Sibeck, D. G. and Slivka, M. and Gretchko, T. V. and Sarris, E. T.},
  Journal                  = {Advances in Space Research},
  Year                     = {2002},
  Pages                    = {2849--2854},
  Volume                   = {30},

  Abstract                 = {Time period from October 1996 until January 1998 was checked on high energy resolution DOK2 energetic particle instrument measurements on Interball-1 and Interball-2 for the ion ({\textgreater} 20 keV) dispersive events (EDIS) with the exclusion of Interball-1 orbit parts in the tail. A variety of energy dispersive events, both in ion and electron spectra with different duration is found in the auroral regions, in the outer magnetosphere and near the cusp. While EDIS were observed in all sectors of MLT, the best conditions for their observation were in the afternoon local time. The characteristics of dispersive events observed by DOK2 are consistent with their explanation by the gradient-curvature drift of particles from the injection point(s) in the night local time sector given in Lutsenko at al., 2000a, b.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/2002AdSpR..30.2849K}
}

@Article{Kudela1998,
  Title                    = {Energetic ions in the magnetosheath: statistical study of spectra and anistropy},
  Author                   = {Kudela, K. and Sibeck, D. G. and Slivka, M. and Lutsenko, V.},
  Journal                  = {Advances in Space Research},
  Year                     = {1998},
  Pages                    = {633--636},
  Volume                   = {21},

  Abstract                 = {Prognoz-10 energetic ion measurements (E {\textgreater} 15 keV) in the magnetosheath (MSH) covered wide range of longitudes and low as well as medium latitudes. From all available 4 energy channel measurements of DOK-1 in MSH the energy spectra in 15-950 keV is shown to be harder close to magnetopause (MP) than deep in MSH. The streaming of ions dawnward and duskward close to MP is not showing any clear pattern in (zy)\_GSE plane. This is consistent with suggestion of patchy structure of merging at MP and leakage of magnetospheric particles to MSH.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/1998AdSpR..21..633K}
}

@Article{Kudela1994,
  Title                    = {Medium energy particle perspective from magnetopause to upstream region: {Prognoz}-10 data},
  Author                   = {Kudela, K. and Sibeck, D. G. and Slivka, M. and Venkatesan, D. and Fischer, S. and Lutsenko, V. N.},
  Journal                  = {Advances in Space Research},
  Year                     = {1994},
  Pages                    = {39--},
  Volume                   = {14},

  Abstract                 = {We present typical examples of Prognoz-10 ion (E greater than 15 keV) and electron (E greater than 30 keV) flux observations as the spacecraft crosses the low and mid-latitude magnetosheath and the foreshock. Both leakage from magnetosphere and bow shock acceleration contribute to magnetosheath populations. A statistical survey using 6 months of measurements reveals that the occurrence of high ion and electron fluxes depends upon K{\textless}SUB{\textgreater}p{\textless}/SUB{\textgreater}. For the same K{\textless}SUB{\textgreater}p{\textless}/SUB{\textgreater}, the probability of high ion occurrence is much higher in the magnetosheath than in the upstream region. In the upstream region, the occurrence of high ion fluxes depends upon the distance to the bow shock and on the angle Theta{\textless}SUB{\textgreater}Bn{\textless}/SUB{\textgreater}.},
  ISSN                     = {0273-1177},
  Keywords                 = {Bow Waves Energetic Particles Magnetopause Magnetosheath Shock Waves Charts Flux (Rate) Geomagnetism Prognoz Satellites Satellite Observation Solar Planetary Interactions Spaceborne Astronomy Tables (Data)},
  Url                      = {http://adsabs.harvard.edu/abs/1994AdSpR..14...39K}
}

@Article{Kudela1994a,
  Title                    = {Prognoz 10 energetic particle data: {Leakage} from the magnetosphere versus bow shock acceleration},
  Author                   = {Kudela, K. and Sibeck, L. D. and Slivka, M.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1994},
  Pages                    = {23461},
  Volume                   = {99},

  Abstract                 = {We present a case study and a statistical survey of Prognoz 10 energetic particle and magnetic field observations from the solar wind to the magnetosphere. The results provide evidence for both Fermi acceleration and leakage from the magnetosphere. Energetic ion (E greater than 15 keV) flux levels upstreams of the bow shock and in the outer magnetosphere generally exceed those in the magnetosheath. Energetic electrons rarely accompany ion fluxes in the outer magnetsheath and upstream of the bow shock, but commonly accompany those in the inner magnetosheath, Upstream flux levels increase as the interplanetary magnetic field (IMF) rotates toward the bow shock normal, consistent with Fermi accleleration. Although the north/south magnetosheath magnetic field orientation has no effect upon energetic particle flux levels in the outer magnetosheath, flux levels in the inner magnetosheath increase during periods of southward IMF. We interpret the results as indicating that Fermi acceleration supplies most of the ions observed in the outer dayside magnetosheath but that leakage from the magnetosphere supplies most of the ions observed in the inner magnetosheath.},
  ISSN                     = {0148-0227},
  Keywords                 = {Bow Waves Electron Flux Density Energetic Particles Interplanetary Magnetic Fields Leakage Magnetosheath Particle Acceleration Shock Waves Earth Magnetosphere Geomagnetism Interplanetary Medium Plasma Sheaths Prognoz Satellites Solar Terrestrial Interactions Solar Wind Spectral Energy Distribution},
  Url                      = {http://adsabs.harvard.edu/abs/1994JGR....9923461K}
}

@Article{Kudela1999,
  Title                    = {Energetic proton fluxes within the magnetosheath and upstream from the bow shock: {Interball}-1 data},
  Author                   = {Kudela, K. and Slivka, M. and Sibeck, D. G. and Lutsenko, V. N. and Sarris, E. T. and Kiraly, P. and Kecskemety, K. and Šafránková, J. and Němeček, Z.},
  Journal                  = {Czechoslovak Journal of Physics},
  Year                     = {1999},
  Pages                    = {591--598},
  Volume                   = {49},

  Abstract                 = {The extensive data set of DOK2 energetic proton measurements indicates a decrease of flux at 22-29 keV within the magnetosheath with distance from the magnetopause. It is consistent with the expectations that the main source of medium energy magnetosheath ions is the magnetosphere. In the region upstream from the bow shock the signatures expected for the preferential acceleration of protons at quasiparallel shocks are found in the survey data too. Thus in addition to the proton leakage from the magnetosphere observed by several experiments, especially in the case studies by multipoint measurements or during the increased geomagnetic activity periods, the influence of bow shock acceleration to the population of medium energy ions in near upstream region is not negligible. To clarify the contributions of the two processes the combination of statistical studies and those based on two point measurements are required.},
  ISSN                     = {0011-4626},
  Keywords                 = {Earth Magnetosphere},
  Url                      = {http://adsabs.harvard.edu/abs/1999CzJPh..49..591K}
}

@Article{Kudela2000,
  Title                    = {Medium {Energy} {Proton} {Fluxes} {Outside} the {Magnetopause}: {Interball}-1 {Data}},
  Author                   = {Kudela, K. and Slivka, M. and Sibeck, D. G. and Lutsenko, V. N. and Sarris, E. T. and Safrankova, J. and Nemecek, Z. and Király, P. and Kecskeméty, K.},
  Journal                  = {Advances in Space Research},
  Year                     = {2000},
  Pages                    = {1517--1522},
  Volume                   = {25},

  Abstract                 = {The extensive data set of the DOK2 energetic proton measurements indicates a decrease of flux at 22 - 29 keV based on the distance from the magnetopause within the magnetosheath. In the region upstream from the bow shock the signatures expected for the preferential acceleration of protons at quasiparallel shocks are found in the data. In addition to the proton leakage from the magnetosphere observed in several experiments, the observations confirm the importance of bow shock acceleration for the population of medium energy protons in the near upstream region.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/2000AdSpR..25.1517K}
}

@InProceedings{Kullen2004,
  Title                    = {Relation of polar auroral arcs to magnetotail twisting and {IMF} rotation: {A} systematic {MHD} simulation study},
  Author                   = {Kullen, Anita and Janhunen, P and {others}},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2004},
  Pages                    = {951--970},
  Volume                   = {22}
}

@Article{Kumar2011,
  Title                    = {{Probing the magnetosphere: An interview with David Sibeck}},
  Author                   = {Kumar, Mohi},
  Journal                  = {Sp. Weather},
  Year                     = {2011},
  Number                   = {3},
  Volume                   = {9},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {David Sibeck is a magnetospheric physicist at NASA Goddard Space Flight Center (GSFC), in Greenbelt, Md. Trained as a meteorologist, he focused on space weather in graduate school and wrote his thesis on the response of the Earth's magnetotail to varying solar wind conditions. After earning a Ph.D. in 1984 from the University of California, Los Angeles (UCLA), he went to work at the Johns Hopkins University Applied Physics Laboratory (APL). In 2002 he shifted to NASA and has been an active member of several missions to better understand the Earth's magnetosphere. In this interview, Space Weather talks to Sibeck about his role in these projects.},
  Doi                      = {10.1029/2011SW000667},
  ISBN                     = {1542-7390},
  ISSN                     = {15427390},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@InProceedings{Kumar2012,
  Title                    = {Charge-to-mass-ratio-dependent ion heating during magnetic reconnection in the {MST} {RFP}},
  Author                   = {Kumar, S. T. A. and Den Hartog, D. J. and Nornberg, M. D. and Almagri, A. F. and Sarff, J. S. and Craig, D.},
  Booktitle                = {{APS} {Meeting} {Abstracts}},
  Year                     = {2012},
  Pages                    = {8152P},
  Volume                   = {1},

  Url                      = {http://adsabs.harvard.edu/abs/2012APS..DPPJP8152K},
  Urldate                  = {2014-05-31}
}

@Article{Kunz1983,
  Title                    = {Determination of solar wind elemental abundances from {M}/{Q} observations during three periods in 1980},
  Author                   = {Kunz, S. and Bochsler, P. and Geiss, J. and Ogilvie, K. W. and Coplan, M. A.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {1983},

  Month                    = oct,
  Pages                    = {359--376},
  Volume                   = {88},

  Doi                      = {10.1007/BF00196199},
  Keywords                 = {Abundance, Helium Ions, International Sun Earth Explorer 3, Ion Temperature, Mass Spectra, Oxygen Ions, Plasma Composition, Positive Ions, Solar Wind}
}

@Article{Kupo1976,
  Title                    = {Detection of ionized sulfur in the {Jovian} magnetosphere},
  Author                   = {Kupo, I. and Mekler, Y. and Eviatar, A.},
  Journal                  = {{\textbackslash}textbackslashapjl},
  Year                     = {1976},

  Month                    = apr,
  Pages                    = {L51--L53},
  Volume                   = {205},

  Doi                      = {10.1086/182088},
  Keywords                 = {Atomic Energy Levels, Atomic Spectra, Electron Density (Concentration), Emission Spectra, Forbidden Bands, Forbidden Transitions, Jupiter Atmosphere, Line Spectra, Planetary Magnetospheres, Sulfur}
}

@Book{Kuznetsova1998,
  Title                    = {The {Community} {Coordinated} {Modeling} {Center}},
  Author                   = {Kuznetsova, Masha},
  Year                     = {1998},

  Abstract                 = {The Community Coordinated Modeling Center (CCMC) is a multi-agency partnership. The CCMC provides, to the international research community, access to modern space science simulations. In addition, the CCMC supports the transition to space weather operations of modern space research models.},
  Url                      = {http://ccmc.gsfc.nasa.gov/about.php}
}

@Article{Kuznetsova2009,
  Title                    = {{Cavities of weak magnetic field strength in the wake of FTEs: Results from global magnetospheric MHD simulations}},
  Author                   = {Kuznetsova, M. M. and Sibeck, D. G. and Hesse, M. and Wang, Y. and Rastaetter, L. and Toth, G. and Ridley, A.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2009},
  Number                   = {10},
  Volume                   = {36},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {We use the global magnetohydrodynamic (MHD) code BATS-R-US to model multipoint observations of Flux Transfer Event (FTE) signatures. Simulations with high spatial and temporal resolution predict that cavities of weak magnetic field strength protruding into the magnetosphere trail FTEs. These predictions are consistent with recently reported multi-point Cluster observations of traveling magnetopause erosion regions (TMERs).},
  Doi                      = {10.1029/2009GL037489},
  ISBN                     = {0094-8276},
  ISSN                     = {00948276},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Kuznetsova2009a,
  Title                    = {Cavities of weak magnetic field strength in the wake of {FTEs}: {Results} from global magnetospheric {MHD} simulations},
  Author                   = {Kuznetsova, M. M. and Sibeck, D. G. and Hesse, M. and Wang, Y. and Rastaetter, L. and Toth, G. and Ridley, A.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2009},
  Pages                    = {10104},
  Volume                   = {36},

  Abstract                 = {We use the global magnetohydrodynamic (MHD) code BATS-R-US to model multipoint observations of Flux Transfer Event (FTE) signatures. Simulations with high spatial and temporal resolution predict that cavities of weak magnetic field strength protruding into the magnetosphere trail FTEs. These predictions are consistent with recently reported multi-point Cluster observations of traveling magnetopause erosion regions (TMERs).},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Numerical modeling Magnetospheric Physics: Magnetic reconnection (7526 7835)},
  Url                      = {http://adsabs.harvard.edu/abs/2009GeoRL..3610104K}
}

@Article{Laakso1998,
  Title                    = {Oscillations of magnetospheric boundaries driven by {IMF} rotations},
  Author                   = {Laakso, H. and Fairfield, D. H. and Collier, M. R. and Opgenoorth, H. and Phan, T.-D. and Sibeck, D. G. and Giles, B. L. and Singer, H. J. and Lepping, R. P. and Lin, R. P. and Mozer, F. S. and Pfaff, R. F. and Tsuruda, K. and Wygant, J. R.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1998},
  Pages                    = {3007--3010},
  Volume                   = {25},

  Abstract                 = {The arrival of the magnetic cloud on January 10, 1997, 01:05 UT, was preceded by a 12-hour interval of increased fluctuations in the IMF orientation, which drove boundary oscillations in the magnetosphere. The GEOTAIL spacecraft, initially located near the dawnside magnetopause, experienced multiple crossings of the magnetopause; at the geosynchronous distance, GOES 9 observed weak perturbations associated with these oscillations. During this time, the POLAR spacecraft encountered the dense high-latitude boundary layer, followed by several rapid encounters with the tenuous lobe. The boundary between the mantle and the lobe was observed to be thin as the crossings lasted only 30 seconds. The source of these boundary oscillations is magnetosheath pressure variations produced by rapid IMF directional changes.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: MHD waves and instabilities Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/1998GeoRL..25.3007L}
}

@Article{Lacombe2006,
  Title                    = {Proton temperature anisotropy in the magnetosheath: comparison of {MHD} modeling with {CLUSTER} data},
  Author                   = {Lacombe, C. and Samsonov, A. and Alexandrova, O. and Maksimovic, M.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2006},

  Month                    = dec,
  Pages                    = {A1450},

  Keywords                 = {2728 Magnetosheath, 2752 MHD waves and instabilities (2149, 2753 Numerical modeling, 2772 Plasma waves and instabilities (2471), 6050, 7829 Kinetic waves and instabilities, 7836)}
}

@Article{Lai2010,
  Title                    = {Mass {Transfer}, {Transiting} {Stream}, and {Magnetopause} in {Close}-in {Exoplanetary} {Systems} with {Applications} to {WASP}-12},
  Author                   = {Lai, D. and Helling, C. and van den Heuvel, E. P. J.},
  Journal                  = {{\textbackslash}textbackslashapj},
  Year                     = {2010},

  Month                    = oct,
  Pages                    = {923--928},
  Volume                   = {721},

  Doi                      = {10.1088/0004-637X/721/2/923},
  Keywords                 = {hydrodynamics, outflows, planetary systems, stars: individual: WASP-12, stars: winds}
}

@Article{Lamarque2002,
  Title                    = {Constraining tropospheric ozone column through data assimilation},
  Author                   = {Lamarque, J-F and Khattatov, BV and Gille, JC},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984–2012)},
  Year                     = {2002},
  Number                   = {D22},
  Pages                    = {ACH--9},
  Volume                   = {107}
}

@Article{Lambour2003,
  Title                    = {Operational impacts of space weather},
  Author                   = {Lambour, RL and Coster, AJ and Clouser, R and Thornton, LE and Sharma, J and Cott, TA},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2003},
  Number                   = {3},
  Volume                   = {30}
}

@Article{Laming2012,
  Title                    = {Non-{WKB} {Models} of the {First} {Ionization} {Potential} {Effect}: {The} {Role} of {Slow} {Mode} {Waves}},
  Author                   = {Laming, J. M.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2012},

  Month                    = jan,
  Pages                    = {115},
  Volume                   = {744},

  Doi                      = {10.1088/0004-637X/744/2/115},
  Keywords                 = {Sun: abundances, Sun: chromosphere, turbulence, waves}
}

@Article{Lamsal2010,
  Title                    = {Indirect validation of tropospheric nitrogen dioxide retrieved from the {OMI} satellite instrument: {Insight} into the seasonal variation of nitrogen oxides at northern midlatitudes},
  Author                   = {Lamsal, L. N. and Martin, R. V. and Van Donkelaar, A. and Celarier, E. A. and Bucsela, E. J. and Boersma, K. F. and Dirksen, R. and Luo, C. and Wang, Y.},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2010},
  Number                   = {D5},
  Volume                   = {115},

  Shorttitle               = {Indirect validation of tropospheric nitrogen dioxide retrieved from the {OMI} satellite instrument},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2009JD013351/full},
  Urldate                  = {2014-11-13}
}

@Article{Landi2008,
  Title                    = {The {Off}-{Disk} {Thermal} {Structure} of a {Polar} {Coronal} {Hole}},
  Author                   = {Landi, E.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2008},

  Month                    = oct,
  Pages                    = {1270--1276},
  Volume                   = {685},

  Doi                      = {10.1086/591225},
  Keywords                 = {Sun: corona, Sun: UV Radiation}
}

@Article{Landi2012,
  Title                    = {Carbon {Ionization} {Stages} as a {Diagnostic} of the {Solar} {Wind}},
  Author                   = {Landi, E. and Alexander, R. L. and Gruesbeck, J. R. and Gilbert, J. A. and Lepri, S. T. and Manchester, W. B. and Zurbuchen, T. H.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2012},

  Month                    = jan,
  Pages                    = {100},
  Volume                   = {744},

  Doi                      = {10.1088/0004-637X/744/2/100},
  Keywords                 = {Atomic Processes, Solar Wind, Sun: corona}
}

@Article{Landi2012a,
  Title                    = {{CHIANTI}{\textbackslash}{mdashAn} {Atomic} {Database} for {Emission} {Lines}. {XII}. {Version} 7 of the {Database}},
  Author                   = {Landi, E. and Del Zanna, G. and Young, P. R. and Dere, K. P. and Mason, H. E.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2012},

  Month                    = jan,
  Pages                    = {99},
  Volume                   = {744},

  Doi                      = {10.1088/0004-637X/744/2/99},
  Keywords                 = {atomic data, Atomic Processes, gamma rays, Sun: UV Radiation, Sun: X-rays, ultraviolet: general, X-rays: general}
}

@Article{Landi2002,
  Title                    = {{CHIANTI}-{An} {Atomic} {Database} for {Emission} {Lines}. {V}. {Comparison} with an {Isothermal} {Spectrum} {Observed} with {SUMER}},
  Author                   = {Landi, E. and Feldman, U. and Dere, K. P.},
  Journal                  = {{\textbackslash}apjs},
  Year                     = {2002},

  Month                    = mar,
  Pages                    = {281--296},
  Volume                   = {139},

  Doi                      = {10.1086/337949},
  Keywords                 = {atomic data, Sun: corona, Sun: UV Radiation}
}

@Article{Landi2012b,
  Title                    = {New {Solar} {Wind} {Diagnostic} {Using} {Both} in {Situ} and {Spectroscopic} {Measurements}},
  Author                   = {Landi, E. and Gruesbeck, J. R. and Lepri, S. T. and Zurbuchen, T. H.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2012},

  Month                    = may,
  Pages                    = {159},
  Volume                   = {750},

  Doi                      = {10.1088/0004-637X/750/2/159},
  Keywords                 = {Solar Wind, Sun: UV Radiation}
}

@Article{Landi2012c,
  Title                    = {Charge {State} {Evolution} in the {Solar} {Wind}. {II}. {Plasma} {Charge} {State} {Composition} in the {Inner} {Corona} and {Accelerating} {Fast} {Solar} {Wind}},
  Author                   = {Landi, E. and Gruesbeck, J. R. and Lepri, S. T. and Zurbuchen, T. H. and Fisk, L. A.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2012},

  Month                    = dec,
  Pages                    = {48},
  Volume                   = {761},

  Doi                      = {10.1088/0004-637X/761/1/48},
  Keywords                 = {Solar Wind, Sun: UV Radiation}
}

@Article{Landi2012d,
  Title                    = {Charge {State} {Evolution} in the {Solar} {Wind}. {Radiative} {Losses} in {Fast} {Solar} {Wind} {Plasmas}},
  Author                   = {Landi, E. and Gruesbeck, J. R. and Lepri, S. T. and Zurbuchen, T. H. and Fisk, L. A.},
  Journal                  = {{\textbackslash}apjl},
  Year                     = {2012},

  Month                    = oct,
  Pages                    = {L21},
  Volume                   = {758},

  Doi                      = {10.1088/2041-8205/758/1/L21},
  Keywords                 = {Solar Wind, Sun: UV Radiation}
}

@Article{Landi2013,
  Title                    = {{CHIANTI}{\textbackslash}{mdashAn} {Atomic} {Database} for {Emission} {Lines}. {XIII}. {Soft} {X}-{Ray} {Improvements} and {Other} {Changes}},
  Author                   = {Landi, E. and Young, P. R. and Dere, K. P. and Del Zanna, G. and Mason, H. E.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2013},

  Month                    = feb,
  Pages                    = {86},
  Volume                   = {763},

  Doi                      = {10.1088/0004-637X/763/2/86},
  Keywords                 = {atomic data, Atomic Processes, gamma rays, Sun: UV Radiation, Sun: X-rays, ultraviolet: general, X-rays: general}
}

@Article{Langdon1983,
  Title                    = {Direct implicit large time-step particle simulation of plasmas},
  Author                   = {Langdon, A Bruce and Cohen, Bruce I and Friedman, Alex},
  Journal                  = {J. Comput. Phys.},
  Year                     = {1983},
  Number                   = {1},
  Pages                    = {107--138},
  Volume                   = {51}
}

@Book{Langois,
  Title                    = {Dipolar {Magnetic} {Field} plot in {Latex}},
  Author                   = {Langois, Cyril},

  Abstract                 = {A 3D plot of a dipolar magnetic field similar to the Earth's one. The field lines are drawn in each longitude plane using the dipolar field equation. Like Earth's field, the north magnetic pole lies close to the south geographic pole and vice-versa.},
  Keywords                 = {dipole field},
  Url                      = {http://www.texample.net/tikz/examples/author/cyril-langlois/}
}

@Article{Lanzerotti2001,
  Title                    = {Space weather effects on technologies},
  Author                   = {Lanzerotti, Louis J},
  Journal                  = {Space Weather},
  Year                     = {2001},
  Pages                    = {11--22},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/GM125p0011/summary?primaryCompoundsResultsPerPage=250}
}

@Article{Lapenta2012,
  Title                    = {Particle simulations of space weather},
  Author                   = {Lapenta, Giovanni},
  Journal                  = {J. Comput. Phys.},
  Year                     = {2012},
  Number                   = {3},
  Pages                    = {795--821},
  Volume                   = {231},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S0021999111001860}
}

@Article{Lapenta1999,
  Title                    = {3D reconnection due to oblique modes: a simulation of {Harris} current sheets},
  Author                   = {Lapenta, Giovanni and Brackbill, JU},
  Journal                  = {Nonlinear Processes in Geophysics},
  Year                     = {1999},
  Number                   = {3/4},
  Pages                    = {151--158},
  Volume                   = {7}
}

@Article{Lapenta2013,
  Title                    = {Propagation speed of rotation signals for field lines undergoing magnetic reconnection},
  Author                   = {Lapenta, Giovanni and Goldman, Martin and Newman, David and Markidis, Stefano},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2013},
  Number                   = {10},
  Pages                    = {102113},
  Volume                   = {20},

  Url                      = {http://scitation.aip.org/content/aip/journal/pop/20/10/10.1063/1.4825132},
  Urldate                  = {2014-05-31}
}

@Article{Lapenta2010,
  Title                    = {Scales of guide field reconnection at the hydrogen mass ratio},
  Author                   = {Lapenta, Giovanni and Markidis, Stefano and Divin, Andrey and Goldman, M. and Newman, D.},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2010},
  Number                   = {8},
  Pages                    = {082106},
  Volume                   = {17},

  Url                      = {http://scitation.aip.org/content/aip/journal/pop/17/8/10.1063/1.3467503},
  Urldate                  = {2014-05-31}
}

@Article{Lapenta2011,
  Title                    = {Bipolar electric field signatures of reconnection separatrices for a hydrogen plasma at realistic guide fields},
  Author                   = {Lapenta, Giovanni and Markidis, Stefano and Divin, A. and Goldman, M. V. and Newman, D. L.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2011},
  Number                   = {17},
  Volume                   = {38},

  Url                      = {http://www.agu.org/pubs/crossref/2011/2011GL048572.shtml},
  Urldate                  = {2014-05-31}
}

@InProceedings{Larionova2006,
  Title                    = {Tagamites of the {Yanis}-{Yarvi} {Crater} ({Karelia}, {Russia}): {An} {Example} of {Non}-{Equilibrated} {Impact} {Melt}?},
  Author                   = {Larionova, Y. and Samsonov, A. and Sizova, E.},
  Booktitle                = {37th {Annual} {Lunar} and {Planetary} {Science} {Conference}},
  Year                     = {2006},
  Editor                   = {Mackwell, S. and Stansbery, E.},
  Month                    = mar,
  Pages                    = {1373},
  Series                   = {Lunar and {Planetary} {Inst}. {Technical} {Report}},
  Volume                   = {37}
}

@InProceedings{Lathuillere1999,
  Title                    = {From the {Sun}‚àö√Æ‚àö‚àè≈í¬©s atmosphere to the {Earth}‚àö√Æ‚àö‚àè≈í¬©s atmosphere: an overview of scientific models available for space weather developments},
  Author                   = {Lathuillere, C and Menvielle, M and Lilensten, J and Amari, T and Radicella, SM},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {1999},
  Pages                    = {1081--1104},
  Publisher                = {Copernicus GmbH},
  Volume                   = {20}
}

@Article{Lavraud2009,
  Title                    = {Tracing solar wind plasma entry into the magnetosphere using ion-to-electron temperature ratio},
  Author                   = {Lavraud, B. and Borovsky, J. E. and Génot, V. and Schwartz, S. J. and Birn, J. and Fazakerley, A. N. and Dunlop, M. W. and Taylor, M. G. G. T. and Hasegawa, H. and Rouillard, A. P. and Berchem, J. and Bogdanova, Y. and Constantinescu, D. and Dandouras, I. and Eastwood, J. P. and Escoubet, C. P. and Frey, H. and Jacquey, C. and Panov, E. and Pu, Z. Y. and Shen, C. and Shi, J. and Sibeck, D. G. and Volwerk, M. and Wild, J. A.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2009},
  Pages                    = {18109},
  Volume                   = {36},

  Abstract                 = {When the solar wind Mach number is low, typically such as in magnetic clouds, the physics of the bow shock leads to a downstream ion-to-electron temperature ratio that can be notably lower than usual. We utilize this property to trace solar wind plasma entry into the magnetosphere by use of Cluster measurements in the vicinity of the dusk magnetopause during the passage of a magnetic cloud at Earth on November 25, 2001. The ion-to-electron temperature ratio was indeed low in the magnetosheath (T{\textless}SUB{\textgreater}i{\textless}/SUB{\textgreater}/T{\textless}SUB{\textgreater}e{\textless}/SUB{\textgreater} ˜ 3). In total, three magnetopause boundary layer intervals are encountered on that day. They all show that the low ion-to-electron temperature ratio can be preserved as the plasma enters the magnetosphere, and both with and without the observation of Kelvin-Helmholtz activity. This suggests that the ion-to-electron temperature ratio in the magnetopause boundary layer, which is usually high, is not prescribed by the heating characteristics of the plasma entry mechanism that formed these boundary layers. In the future, this property may be used to (1) further trace plasma entry into inner regions and (2) determine the preferred entry mechanisms if other theoretical, observational and simulation works can give indications on which mechanisms may alter this ratio.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetosheath Space Plasma Physics: Plasma energization Space Plasma Physics: Transport processes Interplanetary Physics: Coronal mass ejections (7513)},
  Url                      = {http://adsabs.harvard.edu/abs/2009GeoRL..3618109L}
}

@Article{Lavraud2014,
  Title                    = {Geo-effectiveness and radial dependence of magnetic cloud erosion by magnetic reconnection},
  Author                   = {Lavraud, B. and Ruffenach, A. and Rouillard, A. P. and Kajdic, P. and Manchester, W. B. and Lugaz, N.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2014},

  Month                    = jan,
  Pages                    = {26--35},
  Volume                   = {119},

  Doi                      = {10.1002/2013JA019154},
  Keywords                 = {Coronal Mass Ejection, erosion, geo-effectiveness, magnetic cloud, Magnetic reconnection}
}

@InProceedings{Lavraud2006,
  Title                    = {Observation of two distinct cold, dense ion populations at geosynchronous orbit: local time asymmetry, solar wind dependence and origin},
  Author                   = {Lavraud, B and Thomsen, MF and Wing, S and Fujimoto, M and Denton, MH and Borovsky, JE and Aasnes, A and Seki, K and Weygand, JM},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2006},
  Pages                    = {3451--3465},
  Volume                   = {24}
}

@Article{Lavraud2006a,
  Title                    = {Evidence for newly closed magnetosheath field lines at the dayside magnetopause under northward {IMF}},
  Author                   = {Lavraud, B. and Thomsen, M. F. and Lefebvre, B. and Schwartz, S. J. and Seki, K. and Phan, T. D. and Wang, Y. L. and Fazakerley, a. and Rème, H. and Balogh, a.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2006},
  Number                   = {A5},
  Pages                    = {A05211},
  Volume                   = {111},

  Doi                      = {10.1029/2005JA011266},
  ISSN                     = {0148-0227},
  Url                      = {http://doi.wiley.com/10.1029/2005JA011266}
}

@Article{Lazarian2013,
  Title                    = {Reconnection {Diffusion}, {Star} {Formation} and {Numerical} {Simulations}},
  Author                   = {Lazarian, A.},
  Journal                  = {arXiv preprint arXiv:1304.3133},
  Year                     = {2013},

  Url                      = {http://arxiv.org/abs/1304.3133},
  Urldate                  = {2014-05-31}
}

@Article{Lazutin2001,
  Title                    = {Westward traveling surge dynamics and the local structure of an isolated substorm},
  Author                   = {Lazutin, L. and Starkov, G. and Meng, C.-I. and Sibeck, D. G. and Stadsnes, J. and Bjordal, J. and Liou, Kan and Kornilova, T. and Reeves, G.},
  Journal                  = {Advances in Space Research},
  Year                     = {2001},
  Pages                    = {1623--1629},
  Volume                   = {28},

  Abstract                 = {We present a case study of a simple isolated substorm. We compare magnetic field and optical observations at Kola Peninsula with POLAR UVI, POLAR/PIXIE and LANL satellite data to examine the relationshipships between global and local auroral structures and their dynamics. In addition to the active phase of the substorm with a main onset, there are two additional Westward Traveling Surge (WTS) intensifications accompanied by energetic particle acceleration and magnetic field dipolarization in associated local sectors of the magnetosphere. The longitudinal dimensions of the main auroral bulge and the WTS were restricted and in neighboring sectors quite different types of activity were observed. The effects of the fragmentation of the night side auroral magnetosphere into sectors with simultaneous auroral bulge expansion and local growth phase may help explain the temporal structure of multiple-onset substorms. Related problems of the substorm geometry are briefly discussed.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/2001AdSpR..28.1623L}
}

@InProceedings{Le2012,
  Title                    = {Magnetic {Reconnection} {Regimes} at the {Real} {Proton}-to-{Electron} {Mass} {Ratio}},
  Author                   = {Le, A. and Egedal, J. and Daughton, W. and Karimabadi, H.},
  Booktitle                = {{APS} {Meeting} {Abstracts}},
  Year                     = {2012},
  Pages                    = {8031P},
  Volume                   = {1},

  Url                      = {http://adsabs.harvard.edu/abs/2012APS..DPPCP8031L},
  Urldate                  = {2014-05-31}
}

@InProceedings{Le2012a,
  Title                    = {Nonlinear {Pressure} {Anisotropy} {Yielding} {Multiple} {Reconnection} {Regimes}},
  Author                   = {Le, A. and Egedal, J. and Daughton, W. and Karimabadi, H.},
  Booktitle                = {{APS} {Meeting} {Abstracts}},
  Year                     = {2012},
  Pages                    = {9006},
  Volume                   = {1},

  Url                      = {http://adsabs.harvard.edu/abs/2012APS..DPPJM9006L},
  Urldate                  = {2014-05-31}
}

@Article{Le2013,
  Title                    = {Regimes of the electron diffusion region in magnetic reconnection},
  Author                   = {Le, A. and Egedal, J. and Ohia, O. and Daughton, W. and Karimabadi, H. and Lukin, V. S.},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2013},
  Number                   = {13},
  Pages                    = {135004},
  Volume                   = {110},

  Url                      = {http://prl.aps.org/abstract/PRL/v110/i13/e135004},
  Urldate                  = {2014-05-31}
}

@Article{Le2001,
  Title                    = {Polar cusp and vicinity under strongly northward interplanetary magnetic field on {April} 11, 1997: {Observations} and {MHD} simulations},
  Author                   = {Le, G. and Raeder, J. and Russell, C. T. and Lu, G. and Petrinec, S. M. and Mozer, F. S.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2001},

  Month                    = oct,
  Pages                    = {21083--21094},
  Volume                   = {106},

  Doi                      = {10.1029/2000JA900091},
  Keywords                 = {and boundary layers, cusp, Magnetospheric Physics: Magnetopause, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Solar wind/magnetosphere interactions}
}

@Article{Le1996,
  Title                    = {{ISEE} observations of low-latitude boundary layer for northward interplanetary magnetic field: {Implications} for cusp reconnection},
  Author                   = {Le, G and Russell, CT and Gosling, JT and Thomsen, MF},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1996},
  Number                   = {A12},
  Pages                    = {27239--27249},
  Volume                   = {101}
}

@Article{Leao2013,
  Title                    = {The {Collapse} of {Turbulent} {Cores} and {Reconnection} {Diffusion}},
  Author                   = {Leão, M. R. M. and Dal Pino, EM de Gouveia and Santos-Lima, R. and Lazarian, A.},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2013},
  Number                   = {1},
  Pages                    = {46},
  Volume                   = {777},

  Url                      = {http://iopscience.iop.org/0004-637X/777/1/46},
  Urldate                  = {2014-05-31}
}

@Article{Leboeuf1978,
  Title                    = {Global simulation of the time dependent magnetosphere},
  Author                   = {Leboeuf, JN and Tajima, T},
  Journal                  = {Geophys. Res. {\textbackslash}ldots},
  Year                     = {1978},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/GL005i007p00609/full}
}

@Article{Leboeuf1978a,
  Title                    = {Global simulation of the time-dependent magnetosphere},
  Author                   = {Leboeuf, JN and Tajima, T and Kennel, Co F and Dawson, JM},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1978},
  Number                   = {7},
  Pages                    = {609--612},
  Volume                   = {5}
}

@Article{Lee2011,
  Title                    = {{SO}2 emissions and lifetimes: {Estimates} from inverse modeling using in situ and global, space-based ({SCIAMACHY} and {OMI}) observations},
  Author                   = {Lee, Chulkyu and Martin, Randall V. and van Donkelaar, Aaron and Lee, Hanlim and Dickerson, Russell R. and Hains, Jennifer C. and Krotkov, Nickolay and Richter, Andreas and Vinnikov, Konstantine and Schwab, James J.},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2011},
  Number                   = {D6},
  Volume                   = {116},

  Shorttitle               = {{SO}2 emissions and lifetimes},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2010JD014758/full},
  Urldate                  = {2014-11-13}
}

@Article{Lee2009,
  Title                    = {Retrieval of vertical columns of sulfur dioxide from {SCIAMACHY} and {OMI}: {Air} mass factor algorithm development, validation, and error analysis},
  Author                   = {Lee, Chulkyu and Martin, Randall V. and van Donkelaar, Aaron and O'Byrne, Gray and Krotkov, Nickolay and Richter, Andreas and Huey, L. Gregory and Holloway, John S.},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2009},
  Number                   = {D22},
  Volume                   = {114},

  Shorttitle               = {Retrieval of vertical columns of sulfur dioxide from {SCIAMACHY} and {OMI}},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2009JD012123/full},
  Urldate                  = {2014-11-13}
}

@Article{Lee2004,
  Title                    = {Geosynchronous magnetic field response to solar wind dynamic pressure pulse},
  Author                   = {Lee, D-Y and Lyons, LR},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2004},
  Number                   = {A4},
  Volume                   = {109}
}

@Article{Lee2012,
  Title                    = {Drift-mobility characterization of silicon thin-film solar cells using photocapacitance},
  Author                   = {Lee, J.-K. and Hamza, A. M. and Dinca, S. and Long, Q. and Schiff, E. A. and Wang, Q. and Yan, B. and Yang, J. and Guha, S.},
  Journal                  = {Journal of Non Crystalline Solids},
  Year                     = {2012},

  Month                    = sep,
  Pages                    = {2194--2197},
  Volume                   = {358},

  Doi                      = {10.1016/j.jnoncrysol.2012.01.024}
}

@Article{Lee2012a,
  Title                    = {Low {Ionization} {State} {Plasma} in {Coronal} {Mass} {Ejections}},
  Author                   = {Lee, J.-Y. and Raymond, J. C.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2012},

  Month                    = oct,
  Pages                    = {116},
  Volume                   = {758},

  Doi                      = {10.1088/0004-637X/758/2/116},
  Keywords                 = {Sun: activity, Sun: corona, Sun: coronal mass ejections: CMEs, Sun: UV Radiation}
}

@Article{Lee1982,
  Title                    = {Coupled hydromagnetic wave excitation and ion acceleration upstream of the {Earth}'s bow shock},
  Author                   = {Lee, Martin A},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1982},
  Number                   = {A7},
  Pages                    = {5063--5080},
  Volume                   = {87}
}

@Article{Lee2014,
  Title                    = {Plasma and energetic particle behaviors during asymmetric magnetic reconnection at the magnetopause},
  Author                   = {Lee, S. H. and Zhang, H. and Zong, Q.-G. and Otto, A. and Sibeck, D. G. and Wang, Y. and Glassmeier, K.-H. and Daly, P. W. and Rème, H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2014},
  Pages                    = {1658--1672},
  Volume                   = {119},

  Abstract                 = {The factors controlling asymmetric reconnection and the role of the cold plasma population in the reconnection process are two outstanding questions. We present a case study of multipoint Cluster observations demonstrating that the separatrix and flow boundary angles are greater on the magnetosheath than on the magnetospheric side of the magnetopause, probably due to the stronger density than magnetic field asymmetry at this boundary. The motion of cold plasmaspheric ions entering the reconnection region differs from that of warmer magnetosheath and magnetospheric ions. In contrast to the warmer ions, which are probably accelerated by reconnection in the diffusion region near the subsolar magnetopause, the colder ions are simply entrained by E×B drifts at high latitudes on the recently reconnected magnetic field lines. This indicates that plasmaspheric ions can sometimes play only a very limited role in asymmetric reconnection, in contrast to previous simulation studies. Three cold ion populations (probably H{\textless}SUP{\textgreater}+{\textless}/SUP{\textgreater}, He{\textless}SUP{\textgreater}+{\textless}/SUP{\textgreater}, and O{\textless}SUP{\textgreater}+{\textless}/SUP{\textgreater}) appear in the energy spectrum, consistent with ion acceleration to a common velocity.},
  ISSN                     = {0148-0227},
  Keywords                 = {Asymmetric Reconnection Particle acceleration cold ions energetic ions},
  Url                      = {http://adsabs.harvard.edu/abs/2014JGRA..119.1658L}
}

@Article{Lee2015,
  Title                    = {Asymmetric ionospheric outflow observed at the dayside magnetopause},
  Author                   = {Lee, S. H. and Zhang, H. and Zong, Q.-G. and Wang, Y. and Otto, A. and Rème, H. and Glassmeier, K.-H.},
  Journal                  = {Journal of Geophysical Research: Space Physics},
  Year                     = {2015},

  File                     = {[PDF] from researchgate.net:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/PNDSXHAG/Lee et al. - 2015 - Asymmetric ionospheric outflow observed at the day.pdf:application/pdf;Snapshot:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/IMNGCJ63/full.html:text/html},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1002/2014JA020943/full},
  Urldate                  = {2015-12-09}
}

@Article{,
  Title                    = {Electron dynamics and cross-shock potential at the quasi-perpendicular {Earth}'s bow shock},
  Author                   = {Lefebvre, Bertrand and Schwartz, Steven J and Fazakerley, Andrew F and Décréau, Pierrette},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2007},
  Number                   = {A9},
  Volume                   = {112}
}

@Article{Lemaire2007,
  Title                    = {History of kinetic polar wind models and early observations},
  Author                   = {Lemaire, JF and Peterson, WK and Chang, T and Schunk, RW and Barakat, AR and Demars, HG and Khazanov, GV},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2007},
  Number                   = {16},
  Pages                    = {1901--1935},
  Volume                   = {69}
}

@Article{Lembege2003,
  Title                    = {Demagnetization of transmitted electrons through a quasi-perpendicular collisionless shock},
  Author                   = {Lembège, B and Savoini, P and Balikhin, M and Walker, S and Krasnoselskikh, V},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2003},
  Number                   = {A6},
  Volume                   = {108}
}

@Article{Lepping1995,
  Title                    = {The {Wind} {Magnetic} {Field} {Investigation}},
  Author                   = {Lepping, R. P. and Acũna, M. H. and Burlaga, L. F. and Farrell, W. M. and Slavin, J. A. and Schatten, K. H. and Mariani, F. and Ness, N. F. and Neubauer, F. M. and Whang, Y. C. and Byrnes, J. B. and Kennon, R. S. and Panetta, P. V. and Scheifele, J. and Worley, E. M.},
  Journal                  = {ßr},
  Year                     = {1995},

  Month                    = feb,
  Pages                    = {207--229},
  Volume                   = {71},

  Doi                      = {10.1007/BF00751330}
}

@Article{Lepri2010,
  Title                    = {Direct {Observational} {Evidence} of {Filament} {Material} {Within} {Interplanetary} {Coronal} {Mass} {Ejections}},
  Author                   = {Lepri, S. T. and Zurbuchen, T. H.},
  Journal                  = {{\textbackslash}apjl},
  Year                     = {2010},

  Month                    = nov,
  Pages                    = {L22--L27},
  Volume                   = {723},

  Doi                      = {10.1088/2041-8205/723/1/L22},
  Keywords                 = {Atomic Processes, plasmas, Solar Wind, Sun: coronal mass ejections: CMEs}
}

@Article{Leroy1981,
  Title                    = {Simulation of a perpendicular bow shock},
  Author                   = {Leroy, MM and Goodrich, CC and Winske, D and Wu, CS and Papadopoulos, K},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1981},
  Number                   = {12},
  Pages                    = {1269--1272},
  Volume                   = {8}
}

@Article{Leroy1982,
  Title                    = {The structure of perpendicular bow shocks},
  Author                   = {Leroy, MM and Winske, D and Goodrich, CC and Wu, Co S and Papadopoulos, K},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1982},
  Number                   = {A7},
  Pages                    = {5081--5094},
  Volume                   = {87}
}

@Article{Lewis2002,
  Title                    = {The 2dF {Galaxy} {Redshift} {Survey}: the environmental dependence of galaxy star formation rates near clusters},
  Author                   = {Lewis, Ian and Balogh, Michael and De Propris, Roberto and Couch, Warrick and Bower, Richard and Offer, Alison and Bland-Hawthorn, Joss and Baldry, Ivan K and Baugh, Carlton and Bridges, Terry and {others}},
  Journal                  = {Monthly Notices of the Royal Astronomical Society},
  Year                     = {2002},
  Number                   = {3},
  Pages                    = {673--683},
  Volume                   = {334}
}

@Article{Lezniak1968,
  Title                    = {Structure of the magnetopause at 6.6 {RE} in terms of 50-to 150-{keV} electrons},
  Author                   = {Lezniak, TW and Winckler, JR},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1968},
  Number                   = {17},
  Pages                    = {5733--5742},
  Volume                   = {73}
}

@Article{Li2012,
  Title                    = {On the ionospheric source region of cold ion outflow},
  Author                   = {Li, K. and Haaland, S. and Eriksson, Anders and André, Mats and Engwall, E. and Wei, Y. and Kronberg, E. A. and Fränz, M. and Daly, P. W. and Zhao, H. and {others}},
  Journal                  = {Geophysical Research Letters},
  Year                     = {2012},
  Number                   = {18},
  Volume                   = {39},

  File                     = {[HTML] from wiley.com:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/G2ND7379/full.html:text/html},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2012GL053297/full},
  Urldate                  = {2015-12-09}
}

@Article{Li2006,
  Title                    = {Modeling of 1 2 {September} 1859 super magnetic storm},
  Author                   = {Li, X. and Temerin, M. and Tsurutani, B. T. and Alex, S.},
  Journal                  = {Advances in Space Research},
  Year                     = {2006},

  Month                    = jan,
  Pages                    = {273--279},
  Volume                   = {38},

  Doi                      = {10.1016/j.asr.2005.06.070}
}

@Article{Liang2013,
  Title                    = {Relativistic {Positron}-{Electron}-{Ion} {Shear} {Flows} and {Application} to {Gamma}-{Ray} {Bursts}},
  Author                   = {Liang, E. and Fu, W. and Boettcher, M. and Smith, I. and Roustazadeh, P.},
  Journal                  = {{\textbackslash}apjl},
  Year                     = {2013},

  Month                    = dec,
  Pages                    = {L27},
  Volume                   = {779},

  Doi                      = {10.1088/2041-8205/779/2/L27},
  Keywords                 = {gamma-ray burst: general, Magnetic Fields, plasmas, relativistic processes}
}

@Article{Liao2015,
  Title                    = {Acceleration of {O}+ from the cusp to the plasma sheet},
  Author                   = {Liao, J and Kistler, LM and Mouikis, CG and Klecker, B and Dandouras, I},
  Journal                  = {Journal of Geophysical Research: Space Physics},
  Year                     = {2015},
  Number                   = {2},
  Pages                    = {1022--1034},
  Volume                   = {120}
}

@Book{Lilensten2007,
  Title                    = {Space weather: research towards applications in {Europe}},
  Author                   = {Lilensten, Jean},
  Publisher                = {Springer},
  Year                     = {2007},
  Volume                   = {344}
}

@Article{Lin2005,
  Title                    = {Generation of diamagnetic cavities at the bow shock by ion kinetic effects},
  Author                   = {Lin, Y.},
  Journal                  = {Washington DC American Geophysical Union Geophysical Monograph Series},
  Year                     = {2005},
  Pages                    = {31--40},
  Volume                   = {156},

  Doi                      = {10.1029/156GM05}
}

@Article{Lin2003,
  Title                    = {Global-scale simulation of foreshock structures at the quasi-parallel bow shock},
  Author                   = {Lin, Y.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2003},

  Month                    = nov,
  Pages                    = {1390},
  Volume                   = {108},

  Doi                      = {10.1029/2003JA009991},
  Keywords                 = {bow shock, Interplanetary Physics: Planetary bow shocks, Interplanetary Physics: Plasma waves and turbulence, kinetic structure, magnetosheath, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Solar wind/magnetosphere interactions, nonlinear wave-particle interaction, numerical simulation, pressure pulses, Space Plasma Physics: Wave/particle interactions}
}

@Article{Lin2006,
  Title                    = {Formation of dayside low-latitude boundary layer under northward interplanetary magnetic field},
  Author                   = {Lin, Y and Wang, XY},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2006},
  Number                   = {21},
  Volume                   = {33}
}

@Article{Lin2008,
  Title                    = {Modeling {Swarthmore} spheromak reconnection experiment using hybrid code},
  Author                   = {Lin, Y. and Wang, X. Y. and Brown, M. R. and Schaffer, M. J. and Cothran, C. D.},
  Journal                  = {Plasma Physics and Controlled Fusion},
  Year                     = {2008},

  Month                    = jul,
  Number                   = {7},
  Pages                    = {074012},
  Volume                   = {50},

  Doi                      = {10.1088/0741-3335/50/7/074012}
}

@Article{Lindman1975,
  Title                    = {“{Free}-space” boundary conditions for the time dependent wave equation},
  Author                   = {Lindman, EL},
  Journal                  = {J. Comput. Phys.},
  Year                     = {1975},
  Number                   = {1},
  Pages                    = {66--78},
  Volume                   = {18}
}

@Article{Lindstedt2009,
  Title                    = {Separatrix regions of magnetic reconnection at the magnetopause},
  Author                   = {Lindstedt, T. and Khotyaintsev, Y. V. and Vaivads, A. and André, M. and Fear, R. C. and Lavraud, B. and Haaland, S. and Owen, C. J.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2009},

  Month                    = oct,
  Pages                    = {4039--4056},
  Volume                   = {27},

  Doi                      = {10.5194/angeo-27-4039-2009}
}

@Article{Lindstedt2010,
  Title                    = {Oxygen energization by localized perpendicular electric fields at the cusp boundary},
  Author                   = {Lindstedt, T and Khotyaintsev, Yuri V and Vaivads, Andris and André, Mats and Nilsson, H and Waara, M},
  Journal                  = {Geophysical Research Letters},
  Year                     = {2010},
  Number                   = {9},
  Volume                   = {37}
}

@Article{Lindstedt2009a,
  Title                    = {Separatrix regions of magnetic reconnection at the magnetopause},
  Author                   = {Lindstedt, T. and Khotyaintsev, Y. V. and Vaivads, A. and Andr√©, M. and Fear, R. C. and Lavraud, B. and Haaland, S. and Owen, C. J.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2009},

  Month                    = oct,
  Pages                    = {4039--4056},
  Volume                   = {27},

  Doi                      = {10.5194/angeo-27-4039-2009}
}

@Article{Liou2001,
  Title                    = {Observation of {IMF} and seasonal effects in the location of auroral substorm onset},
  Author                   = {Liou, K. and Newell, P. T. and Sibeck, D. G. and Meng, C.-I. and Brittnacher, M. and Parks, G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2001},
  Pages                    = {5799--5810},
  Volume                   = {106},

  Abstract                 = {We use Polar ultraviolet imager (UVI) and Wind observations to study the location of 648 well-defined Northern Hemisphere auroral breakups (substorm onsets) in response to interplanetary magnetic field (IMF) orientation and season. The most likely onset location is at 2230 MLT and 67° Λ{\textless}SUB{\textgreater}m{\textless}/SUB{\textgreater} with half-maximum widths of 3 hours of MLT and 2° Λ{\textless}SUB{\textgreater}m{\textless}/SUB{\textgreater}, respectively. The onset latitude depends primarily on IMF B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater}, but also B{\textless}SUB{\textgreater}x{\textless}/SUB{\textgreater}: the onset latitude decreases for B{\textless}SUB{\textgreater}x{\textless}/SUB{\textgreater}{\textgreater}0 or B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater}{\textless}0 and increases for B{\textless}SUB{\textgreater}x{\textless}/SUB{\textgreater}{\textless}0 or B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater}{\textgreater}0. The onset longitude depends on season and IMF B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater}. In summer, substorms tend to occur in the early evening at 2200 MLT, whereas in winter they tend to occur near midnight at 2300 MLT. The average summer-winter difference in the onset location is 1 hour of MLT. Large B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater} effects on the onset longitude occur only when B{\textless}SUB{\textgreater}x{\textless}/SUB{\textgreater} and B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater} are small. Onset locations shift toward earlier local times for B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater}{\textgreater}0 and toward midnight for B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater}{\textless}0. The average onset local time is earliest (2200 MLT) for B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater}{\textgreater}0 in summer and latest (2330 MLT) for B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater}{\textless}0 in winter. These dependencies coincide with those previously reported for the evening sector ionospheric zonal flow reversal in response to IMF B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater} and season, indicating that auroral breakups are most likely in regions of large velocity shears. A weak dependence of the MLT onset location on the IMF B{\textless}SUB{\textgreater}x{\textless}/SUB{\textgreater} is identified: for B{\textless}SUB{\textgreater}x{\textless}/SUB{\textgreater}{\textgreater}0 the onset location shifts toward dusk when B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater}{\textgreater}0 but toward dawn when B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater}{\textless}0 the sense of this shift reverses for B{\textless}SUB{\textgreater}x{\textless}/SUB{\textgreater}{\textless}0. An implication of the results is that auroral breakup is not conjugate.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Auroral phenomena Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Storms and substorms},
  Url                      = {http://adsabs.harvard.edu/abs/2001JGR...106.5799L}
}

@Article{Liou2014,
  Title                    = {Study of a global auroral {Pc}5 pulsation event with concurrent {ULF} waves},
  Author                   = {Liou, Kan and Sibeck, David G.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2014},
  Pages                    = {6547--6555},
  Volume                   = {41},

  Abstract                 = {We present results from a study of concurrent, periodic variations in auroral luminosity (auroral pulsations) and in magnetospheric plasma/magnetic field data. This event occurred on 10 March 2010 from 13 to 17 UT during an extended southward interplanetary magnetic field and was probably triggered by a slow shock. The auroral pulsations, as measured by the Ultraviolet Imager on board the Polar satellite, were long lasting ( 2.5 h), monochromatic ( 2.5 mHz), large scale, and appeared in the night sector auroral zone with a latitudinal extent comparable to the latitudinal width of the oval. There was no phase shift between the auroral pulsations observed at different local times, indicating a stationary structure. Particle data from the Defense Meteorological Satellite Program Special Sensor Precipitating Electron and Ion Spectrometer indicate that the pulsations were diffuse originating from the central plasma sheet. During this time, Geotail was in the dawn sector plasma sheet and observed a ULF wave with the same frequency as the auroral pulsations last 35 min. The ULF wave had large radial and compressional components, and the plasma density and total magnetic field were anticorrelated. These two observations strongly suggest that the observed ULF wave was associated with an standing ULF poloidal mode. The wave compressional component may be able to change the loss cone, resulting in periodic auroral precipitating.},
  ISSN                     = {0094-8276},
  Keywords                 = {auroral pulsations Pc5 ULF waves Polar UVI Geotail},
  Url                      = {http://adsabs.harvard.edu/abs/2014GeoRL..41.6547L}
}

@Article{Liu2013,
  Title                    = {Magnetic {Reconnection} {Driven} by the {Nernst} {Effect}},
  Author                   = {Liu, Chang and Fox, W. and Bhattacharjee, A. and Joglekar, A. and Thomas, A.},
  Journal                  = {Bulletin of the American Physical Society},
  Year                     = {2013},
  Volume                   = {58},

  Url                      = {http://meetings.aps.org/Meeting/DPP13/Event/201101},
  Urldate                  = {2014-05-31}
}

@Article{Liu2014,
  Title                    = {Thermal and dynamical changes of the zonal mean state of the thermosphere during the 2009 {SSW}: {GAIA} simulations},
  Author                   = {Liu, H. and Miyoshi, Y. and Miyahara, S. and Jin, H. and Fujiwara, H. and Shinagawa, H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2014},

  Month                    = aug,
  Pages                    = {6784--6791},
  Volume                   = {119},

  Doi                      = {10.1002/2014JA020222},
  Keywords                 = {stratosphere sudden warming, thermosphere dynamics, vertical coupling, zonal mean state}
}

@Article{Liu2008,
  Title                    = {{THEMIS} observations of the dayside traveling compression region and flows surrounding flux transfer events},
  Author                   = {Liu, J. and Angelopoulos, V. and Sibeck, D. and Phan, T. and Pu, Z. Y. and McFadden, J. and Glassmeier, K. H. and Auster, H. U.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2008},
  Volume                   = {35},

  Abstract                 = {We present multipoint observations of Flux Transfer Events (FTEs) by the THEMIS spacecraft in a string-of-pearls configuration, at the near-equatorial magnetopause. Common characteristics from a number of cases, examined at various local times, are exemplified here by a case study of FTE trains observed in the pre-noon sector, on Aug. 18, 2007. We show that the magneto-pause-normal flow velocity is consistently towards and away from the magnetopause on the inbound and outbound transit of the FTE, on all spacecraft sufficiently away from the magnetopause. The velocity just outside the FTE at the time of closest proximity to the FTE core is opposite to the FTE direction of motion even when the FTE moves in the same direction as the adjacent sheath. The total pressure inside and just outside the FTE is consistently larger than expected from pressure balance at a nominal (unperturbed) magnetopause and therefore the result of local compression by the passing FTE. The multi-spacecraft observation enables the reconstruction of the Dayside Traveling Compression Region (DTCR), whose result is consistent with previous theoretical results. Semi-periodic compressional velocity oscillations were observed and are likely driven by nearby occurrences of FTE trains, implying recurrent reconnection with a similar periodicity.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2008GeoRL..3517S07L}
}

@Article{Liu2010,
  Title                    = {Ozone profile retrievals from the {Ozone} {Monitoring} {Instrument}},
  Author                   = {Liu, X. and Bhartia, P. K. and Chance, K. and Spurr, R. J. D. and Kurosu, T. P.},
  Journal                  = {Atmos. Chem. Phys.},
  Year                     = {2010},
  Number                   = {5},
  Pages                    = {2521--2537},
  Volume                   = {10},

  Url                      = {http://www.atmos-chem-phys.net/10/2521/2010/},
  Urldate                  = {2014-11-13}
}

@Article{Liu2006,
  Title                    = {First directly retrieved global distribution of tropospheric column ozone from {GOME}: {Comparison} with the {GEOS}-{Chem} model},
  Author                   = {Liu, Xiong and Chance, Kelly and Sioris, Christopher E. and Kurosu, Thomas P. and Spurr, Robert JD and Martin, Randall V. and Fu, Tzung-May and Logan, Jennifer A. and Jacob, Daniel J. and Palmer, Paul I. and {others}},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2006},
  Number                   = {D2},
  Volume                   = {111},

  Shorttitle               = {First directly retrieved global distribution of tropospheric column ozone from {GOME}},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2005JD006564/full},
  Urldate                  = {2014-11-13}
}

@Article{Liu2005,
  Title                    = {Ozone profile and tropospheric ozone retrievals from the {Global} {Ozone} {Monitoring} {Experiment}: {Algorithm} description and validation},
  Author                   = {Liu, X. and Chance, K. and Sioris, C. E. and Spurr, R. J. D. and Kurosu, T. P. and Martin, R. V. and Newchurch, M. J.},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2005},
  Number                   = {D20},
  Volume                   = {110},

  Shorttitle               = {Ozone profile and tropospheric ozone retrievals from the {Global} {Ozone} {Monitoring} {Experiment}},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2005JD006240/full},
  Urldate                  = {2014-11-13}
}

@Article{Liu2007,
  Title                    = {Ion thermalization and wave excitation downstream of {Earth}'s bow shock: {A} theory for {Cluster} observations of {He}2+ acceleration},
  Author                   = {Liu, Yong C-M and Lee, Martin A and Kucharek, Harald and Miao, Bin},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2007},
  Number                   = {A7},
  Volume                   = {112}
}

@Article{Liu2014a,
  Title                    = {Do dispersive waves play a role in collisionless magnetic reconnection?},
  Author                   = {Liu, Yi-Hsin and Daughton, W. and Karimabadi, H. and Li, H. and Gary, S. Peter},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2014},
  Number                   = {2},
  Pages                    = {022113},
  Volume                   = {21},

  Url                      = {http://scitation.aip.org/content/aip/journal/pop/21/2/10.1063/1.4865579},
  Urldate                  = {2014-05-31}
}

@Article{Llama2011,
  Title                    = {The shocking transit of {WASP}-12b: modelling the observed early ingress in the near-ultraviolet},
  Author                   = {Llama, J. and Wood, K. and Jardine, M. and Vidotto, A. A. and Helling, C. and Fossati, L. and Haswell, C. A.},
  Journal                  = {{\textbackslash}textbackslashmnras},
  Year                     = {2011},

  Month                    = sep,
  Pages                    = {L41--L44},
  Volume                   = {416},

  Doi                      = {10.1111/j.1745-3933.2011.01093.x},
  Keywords                 = {outflows, planets and satellites: individual: WASP-12b, planets and satellites: magnetic fields, planet-star interactions, planet{\textbackslash}textbackslashndashstar interactions, stars: coronae, stars: winds}
}

@Article{Lobzin2007,
  Title                    = {Nonstationarity and reformation of high-{Mach}-number quasiperpendicular shocks: {Cluster} observations},
  Author                   = {Lobzin, VV and Krasnoselskikh, VV and Bosqued, J-M and Pincon, J-L and Schwartz, SJ and Dunlop, M},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2007},
  Number                   = {5},
  Volume                   = {34}
}

@InProceedings{Lobzin2008,
  Title                    = {On nonstationarity and rippling of the quasiperpendicular zone of the {Earth} bow shock: {Cluster} observations},
  Author                   = {Lobzin, VV and Krasnoselskikh, VV and Musatenko, K and Dudok de Wit, T},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2008},
  Pages                    = {2899--2910},
  Publisher                = {Copernicus GmbH},
  Volume                   = {26}
}

@Article{Lobzin2005,
  Title                    = {Generation of downshifted oscillations in the electron foreshock: {A} loss-cone instability},
  Author                   = {Lobzin, VV and Krasnoselskikh, VV and Schwartz, SJ and Cairns, Iver and Lefebvre, B and Décréau, P and Fazakerley, A},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2005},
  Number                   = {18},
  Volume                   = {32}
}

@Article{Longmore2005,
  Title                    = {Multi-spacecraft observations at {Earth} ' s bow shock and a survey of the dayside magnetosheath},
  Author                   = {Longmore, Melissa Mary},
  Year                     = {2005}
}

@InProceedings{Lopez2001,
  Title                    = {The {Science} of {Space} {Weather}},
  Author                   = {Lopez, Ramon},
  Booktitle                = {{APS} {Texas} {Sections} {Fall} {Meeting} {Abstracts}},
  Year                     = {2001},
  Pages                    = {3001P},
  Volume                   = {1}
}

@Article{Lopez2011,
  Title                    = {The role of the bow shock in solar wind-magnetosphere coupling},
  Author                   = {Lopez, R. E. and Merkin, V. G. and Lyon, J. G.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2011},

  Month                    = jun,
  Pages                    = {1129--1135},
  Volume                   = {29},

  Doi                      = {10.5194/angeo-29-1129-2011}
}

@Article{Loverich2013,
  Title                    = {{AIR} {FORCE} {RESEARCH} {LABORATORY} {AF} {OFFICE} {OF} {SCIENTIFIC} {RESEARCH} ({AFOSR}) {ARLINGTON}, {VIRGINIA} 22203 {AIR} {FORCE} {MATERIEL} {COMMAND}},
  Author                   = {Loverich, John and Shumlak, Uri},
  Year                     = {2013},

  Url                      = {http://www.dtic.mil/dtic/tr/fulltext/u2/a578555.pdf},
  Urldate                  = {2014-05-31}
}

@Article{Lu2002,
  Title                    = {Solar wind effects on ionospheric convection: a review},
  Author                   = {Lu, G. and Cowley, S. W. H. and Milan, S. E. and Sibeck, D. G. and Greenwald, R. A. and Moretto, T.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2002},
  Pages                    = {145--157},
  Volume                   = {64},

  Abstract                 = {The solar wind, magnetosphere, and ionosphere are intrinsically coupled through magnetic field lines. The electrodynamic state of the high-latitude ionosphere is controlled by several geophysical processes, such as the location and rate of magnetic reconnection at the magnetopause and in the magnetotail, and the energisation and precipitation of solar wind and magnetospheric plasmas. Amongst the most observed ionospheric manifestation of solar wind/magnetospheric processes are the convection bursts associated with the so-called flux transfer events (FTEs), magnetic impulse events (MIEs), and travelling convection vortices (TCVs). Furthermore, the large-scale ionospheric convection configuration has also demonstrated a strong correspondence to variations in the interplanetary medium and substorm activity. This report briefly discusses the progress made over the past decade in studies of these transient convection phenomena and outlines some unsettled questions as well as future research directions.},
  ISSN                     = {1364-6826},
  Url                      = {http://adsabs.harvard.edu/abs/2002JASTP..64..145L}
}

@Article{Lu2011,
  Title                    = {Three dimensional shape of the magnetopause: {Global} {MHD} results},
  Author                   = {Lu, J. Y. and Liu, Z.-Q. and Kabin, K. and Zhao, M. X. and Liu, D. D. and Zhou, Q. and Xiao, Y.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2011},

  Month                    = sep,
  Pages                    = {9237},
  Volume                   = {116},

  Doi                      = {10.1029/2010JA016418},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers, Magnetospheric Physics: Magnetospheric configuration and dynamics, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Solar wind/magnetosphere interactions}
}

@Article{Lu2004,
  Title                    = {Electron velocity distributions during beam-plasma interaction},
  Author                   = {Lu, Q. M. and Wang, S.},
  Journal                  = {Phys. Plasmas},
  Year                     = {2004},

  Month                    = jan,
  Pages                    = {80--89},
  Volume                   = {11},

  Doi                      = {10.1063/1.1631288},
  Keywords                 = {Electromagnetic waves, Magnetohydrodynamic waves, Particle beam interactions in plasmas, Particle-in-cell method}
}

@Article{Lucek2005,
  Title                    = {The {Magnetosheath}},
  Author                   = {Lucek, E. A. and Constantinescu, D. and Goldstein, M. L. and Pickett, J. and Pinçon, J. L. and Sahraoui, F. and Treumann, R. A. and Walker, S. N.},
  Journal                  = {ßr},
  Year                     = {2005},

  Month                    = jun,
  Pages                    = {95--152},
  Volume                   = {118},

  Abstract                 = {Not Available},
  Doi                      = {10.1007/s11214-005-3825-2}
}

@Article{Lucek2005a,
  Title                    = {The magnetosheath},
  Author                   = {Lucek, EA and Constantinescu, D and Goldstein, ML and Pickett, J and Pinçon, JL and Sahraoui, F and Treumann, RA and Walker, SN},
  Journal                  = {Space science reviews},
  Year                     = {2005},
  Number                   = {1-4},
  Pages                    = {95--152},
  Volume                   = {118}
}

@Article{Lucek2004,
  Title                    = {Cluster observations of hot flow anomalies},
  Author                   = {Lucek, EA and Horbury, TS and Balogh, A and Dandouras, I and Rème, H},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2004},
  Number                   = {A6},
  Volume                   = {109}
}

@Article{Lugaz2005,
  Title                    = {The {Evolution} of {Coronal} {Mass} {Ejection} {Density} {Structures}},
  Author                   = {Lugaz, N. and Manchester, IV, W. B. and Gombosi, T. I.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2005},

  Month                    = jul,
  Pages                    = {1019--1030},
  Volume                   = {627},

  Doi                      = {10.1086/430465},
  Keywords                 = {Magnetohydrodynamics: MHD, Sun: coronal mass ejections (CMEs)}
}

@Article{Luhmann2002,
  Title                    = {Solar cycle changes in coronal holes and space weather cycles},
  Author                   = {Luhmann, JG and Li, Y and Arge, CN and Gazis, PR and Ulrich, R},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2002},
  Number                   = {A8},
  Pages                    = {SMP--3},
  Volume                   = {107}
}

@Article{Luhmann2008,
  Title                    = {{STEREO} {IMPACT} {Investigation} {Goals}, {Measurements}, and {Data} {Products} {Overview}},
  Author                   = {Luhmann, J. G. and Curtis, D. W. and Schroeder, P. and McCauley, J. and Lin, R. P. and Larson, D. E. and Bale, S. D. and Sauvaud, J.-A. and Aoustin, C. and Mewaldt, R. A. and Cummings, A. C. and Stone, E. C. and Davis, A. J. and Cook, W. R. and Kecman, B. and Wiedenbeck, M. E. and von Rosenvinge, T. and Acuna, M. H. and Reichenthal, L. S. and Shuman, S. and Wortman, K. A. and Reames, D. V. and Mueller-Mellin, R. and Kunow, H. and Mason, G. M. and Walpole, P. and Korth, A. and Sanderson, T. R. and Russell, C. T. and Gosling, J. T.},
  Journal                  = {ßr},
  Year                     = {2008},

  Month                    = apr,
  Pages                    = {117--184},
  Volume                   = {136},

  Doi                      = {10.1007/s11214-007-9170-x},
  Keywords                 = {Coronal Mass Ejection, interplanetary magnetic field, Multipoint heliospheric measurements, solar energetic particles, Solar wind electrons, STEREO, Suprathermal electrons}
}

@Article{Luhmann2004,
  Title                    = {Coupled model simulation of a {Sun}-to-{Earth} space weather event},
  Author                   = {Luhmann, Janet G and Solomon, Stanley C and Linker, Jon A and Lyon, John G and Mikic, Zoran and Odstrcil, Dusan and Wang, Wenbin and Wiltberger, Michael},
  Journal                  = {Journal of atmospheric and solar-terrestrial physics},
  Year                     = {2004},
  Number                   = {15},
  Pages                    = {1243--1256},
  Volume                   = {66},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S1364682604001361}
}

@Article{Lui2008,
  Title                    = {Determination of the substorm initiation region from a major conjunction interval of {THEMIS} satellites},
  Author                   = {Lui, A. T. Y. and Angelopoulos, V. and Lecontel, O. and Frey, H. and Donovan, E. and Sibeck, D. G. and Liu, W. and Auster, H. U. and Larson, D. and Li, X. and Nosé, M. and Fillingim, M. O.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2008},
  Volume                   = {113},

  Abstract                 = {We investigate in detail the time history of substorm disturbances in the magnetotail observed during a major tail conjunction of Time History of Events and Macroscale Interactions during Substorms (THEMIS) satellites on 29 January 2008, 0700-0900 UT. During this interval, all THEMIS satellites were closely aligned along the tail axis near midnight and were bracketed in local time by GOES 11 and 12. The radial distance covered ranges from the geosynchronous altitude to ˜30 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} in the tail. This interval consists of three activations detected by the THEMIS satellites with good ground all-sky-camera observations of auroral activity. The first activation is a small substorm with spatially limited disturbance in the tail. The onset arc was equatorward of an undisturbed arc. The second activation is a moderate size substorm with the onset arc also being equatorward of an undisturbed arc. The third activation is an intensification of the substorm with its onset indicated by the second activation. The active auroral arc for this intensification was near the poleward boundary of the auroral oval. Analysis of these observations indicates that the first activation is a small substorm initiated in the near-Earth plasma sheet and does not involve magnetic reconnection of open magnetic field lines. Magnetic reconnection on closed field lines can be ruled out for this substorm because it cannot generate the observed high-speed plasma flow. The second and third activations are part of a moderate size substorm initiated also in the near-Earth plasma sheet, with a subsequent substorm intensification involving activity initiated tailward of ˜30 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}. Overall, the time history of substorm activity for these two substorms is consistent with the near-Earth initiation model.},
  ISSN                     = {0148-0227},
  Keywords                 = {substorm onset location},
  Url                      = {http://adsabs.harvard.edu/abs/2008JGRA..113.0C04L}
}

@Article{Lui2008a,
  Title                    = {Reconstruction of a magnetic flux rope from {THEMIS} observations},
  Author                   = {Lui, A. T. Y. and Sibeck, D. G. and Phan, T. and Angelopoulos, V. and McFadden, J. and Carlson, C. and Larson, D. and Bonnell, J. and Glassmeier, K.-H. and Frey, S.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2008},
  Volume                   = {35},

  Abstract                 = {We investigate a magnetic flux rope (MFR) observed by THEMIS near the duskside magnetopause on 20 May 2007 using the reconstruction technique based on solving the Grad-Shafranov equation. The MFR has characteristics distinct from the adjacent magnetosheath and magnetosphere regions. In spite of these differences, the reconstruction result shows that the MFR is connected simultaneously with both the magnetosheath and the magnetosphere in terms of the magnetic vector potential characteristics. This result provides strong evidence that the MFR represents the union of these two regions. It has a small spatial dimension of 0.5 R {\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}, a strong core magnetic field of {\textgreater}50 nT, and an intense axial current density of {\textgreater}40 nA/m{\textless}SUP{\textgreater}2{\textless}/SUP{\textgreater} with non-negligible current densities transverse to its axis.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetotail Magnetospheric Physics: Plasma sheet},
  Url                      = {http://adsabs.harvard.edu/abs/2008GeoRL..3517S05L}
}

@Article{Lui2008b,
  Title                    = {Reconstruction of a flux transfer event based on observations from five {THEMIS} satellites},
  Author                   = {Lui, A. T. Y. and Sibeck, D. G. and Phan, T. and McFadden, J. P. and Angelopoulos, V. and Glassmeier, K.-H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2008},
  Volume                   = {113},

  Abstract                 = {We investigate a flux transfer event (FTE) observed by Time History of Events and Macroscale Interactions during Substorms (THEMIS) near the duskside magnetopause using the reconstruction technique based on solving the Grad-Shafranov equation; see review by Sonnerup et al. (2006). THEMIS D detected the FTE with the largest core magnetic field. THEMIS B and C observed deep troughs in the magnetic field associated with the FTE. THEMIS A and E sensed only slightly altered magnetic field from their surroundings. Two-dimensional reconstruction maps of magnetic field and plasma pressure are generated by combining observations from all five THEMIS satellites. These reconstructed maps show distinct differences between a magnetic island and an FTE in terms of vector potential and the derived plasma parameters. The origin of the magnetic field troughs in the crater FTEs can be traced to intrusions of the magnetosheath plasma around the structure in the reconstruction maps. Furthermore, the resulting maps show also cylindrical asymmetry in these parameters between the magnetosheath and magnetospheric sides of the FTE. This asymmetry and the different impact parameters of these satellites with respect to the FTE center together contribute to the different characteristics of the FTE signatures seen by the five THEMIS satellites.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Numerical modeling flux transfer event Grad-Shafranov reconstruction},
  Url                      = {http://adsabs.harvard.edu/abs/2008JGRA..113.0C01L}
}

@Article{Lundin1989,
  Title                    = {Ionospheric plasma escape by high-altitude electric fields - {Magnetic} moment 'pumping'},
  Author                   = {Lundin, R. and Hultqvist, B.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1989},

  Month                    = jun,
  Pages                    = {6665--6680},
  Volume                   = {94},

  Doi                      = {10.1029/JA094iA06p06665},
  Keywords                 = {Atmospheric Electricity, Earth Magnetosphere, Electric Fields, Ion Beams, Ionospheric Ion Density, Magnetic Moments, Particle Acceleration, Satellite Sounding, Space Plasmas, Viking Spacecraft}
}

@Article{Lundin1989a,
  Title                    = {Ionospheric plasma escape by high-altitude electric fields - {Magnetic} moment 'pumping'},
  Author                   = {Lundin, R. and Hultqvist, B.},
  Journal                  = {{\textbackslash}textbackslashjgr},
  Year                     = {1989},

  Month                    = jun,
  Pages                    = {6665--6680},
  Volume                   = {94},

  Doi                      = {10.1029/JA094iA06p06665},
  Keywords                 = {Atmospheric Electricity, Earth Magnetosphere, Electric Fields, Ion Beams, Ionospheric Ion Density, Magnetic Moments, Particle Acceleration, Satellite Sounding, Space Plasmas, Viking Spacecraft}
}

@Article{Lyatsky1997,
  Title                    = {Central plasma sheet disruption and the formation of dayside poleward moving auroral events},
  Author                   = {Lyatsky, Wladislav and Sibeck, David},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1997},
  Pages                    = {17625--17630},
  Volume                   = {102},

  Abstract                 = {Although most dayside poleward moving auroral forms (PMAFs) seem to be reasonably explained as a result of magnetopause merging, a number of these events can hardly be explained in terms of reconnection. These events seem to appear on closed field lines, and their poleward movement seems to be controlled not only by convection due to the interplanetary magnetic field (IMF) but also to the polarization electric field appearing inside them. This type of PMAF may be observed not only for a negative IMF B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} component but also for the positive B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} and rather small B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater} components when field line merging may be inefficient or may occur on lobe magnetic field lines, and the poleward propagation of these auroral forms may differ from the background magnetospheric convection. These events often appear at the equatorward edge of the red auroral band, and the spike structures in dayside electron precipitations which may be responsible for these auroral forms are often seen simultaneously with the plasma sheet population. Another possible mechanism for dayside poleward moving auroral events in a region of closed field lines is proposed. This mechanism is based on observations indicating that the central plasma sheet can be divided from the low-latitude boundary layer and the magnetopause by a gap. This means that the dayside plasma sheet has an outer boundary inside the magnetosphere which is unstable with respect to the interchange (ballooning) instability. As a result, for some conditions, clouds of warm plasma may break out from the plasma sheet and move poleward because of the polarization electric field. Projection of these plasma sheet clouds on the ionosphere would have many features which are inherent for the dayside auroral events.},
  ISSN                     = {0148-0227},
  Keywords                 = {Ionosphere: Auroral ionosphere Magnetospheric Physics: Auroral phenomena Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Plasma sheet},
  Url                      = {http://adsabs.harvard.edu/abs/1997JGR...10217625L}
}

@Article{Lyatsky1997a,
  Title                    = {Surface waves on the low-latitude boundary layer inner edge and travelling convection vortices},
  Author                   = {Lyatsky, W. B. and Sibeck, D. G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1997},
  Pages                    = {17643--17648},
  Volume                   = {102},

  Abstract                 = {Surface waves on the inner boundary of the low-latitude boundary layer (LLBL) are considered as a possible cause for dayside high-latitude travelling convection vortices (TCVs). A dispersion equation for the surface waves with regard to their attenuation in the ionosphere is deduced. The current system of the surface wave is consistent with a pair of upward and downward field-aligned currents. The wave velocity depends upon the wavelength; taking the latter to be equal to 1000 km in the ionosphere, which is typical for the TCVs, we obtain the velocity of these waves to be to about 50-100 km/s in the magnetosphere, which corresponds to several kilometers per second in the ionosphere. The surface waves on the LLBL inner boundary may be generated by a sharp deflection of this boundary from the equilibrium position. A cause of this may be sudden impulses of the solar wind dynamic pressure or bursty reconnection at the dayside magnetopause. Surface waves may play an important role in the relaxation of the magnetosphere. The velocity of the surface waves on the LLBL inner edge is close to or slightly less than the magnetosheath plasma velocity near the magnetopause; the movement of the magnetosheath plasma along the magnetopause with a speed more than that of the surface waves may favor the formation of impulsive TCVs. It follows from the considered mechanism that the disturbance maximum is to be observed on the LLBL inner edge, and the TCV velocity has to increase with the wavelength that might be verified from experimental data.},
  ISSN                     = {0148-0227},
  Keywords                 = {Ionosphere: Auroral ionosphere Magnetospheric Physics: Current systems Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetospheric configuration and dynamics},
  Url                      = {http://adsabs.harvard.edu/abs/1997JGR...10217643L}
}

@Article{Lynch2011,
  Title                    = {Ionic {Composition} {Structure} of {Coronal} {Mass} {Ejections} in {Axisymmetric} {Magnetohydrodynamic} {Models}},
  Author                   = {Lynch, B. J. and Reinard, A. A. and Mulligan, T. and Reeves, K. K. and Rakowski, C. E. and Allred, J. C. and Li, Y. and Laming, J. M. and MacNeice, P. J. and Linker, J. A.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2011},

  Month                    = oct,
  Pages                    = {112},
  Volume                   = {740},

  Doi                      = {10.1088/0004-637X/740/2/112},
  Keywords                 = {Magnetic reconnection, Magnetohydrodynamics: MHD, Sun: corona, Sun: coronal mass ejections: CMEs, Sun: flares, Sun: heliosphere}
}

@Article{Lyon2004,
  Title                    = {The {Lyon}–{Fedder}–{Mobarry} ({LFM}) global {MHD} magnetospheric simulation code},
  Author                   = {Lyon, JG and Fedder, JA and Mobarry, CM},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2004},
  Number                   = {15},
  Pages                    = {1333--1350},
  Volume                   = {66},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S1364682604001439}
}

@Article{Ma2001,
  Title                    = {Hall magnetohydrodynamic reconnection: {The} geospace environment modeling challenge},
  Author                   = {Ma, ZW and Bhattacharjee, A},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2001},
  Number                   = {A3},
  Pages                    = {3773--3782},
  Volume                   = {106}
}

@Article{Ma1998,
  Title                    = {Sudden enhancement and partial disruption of thin current sheets in the magnetotail due to {Hall} {MHD} effects},
  Author                   = {Ma, ZW and Bhattacharjee, A},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1998},
  Number                   = {17},
  Pages                    = {3277--3280},
  Volume                   = {25}
}

@Article{MacAlester2014,
  Title                    = {Extreme {Space} {Weather} {Impact}: {An} {Emergency} {Management} {Perspective}},
  Author                   = {MacAlester, Mark H and Murtagh, William},
  Journal                  = {Space Weather},
  Year                     = {2014},
  Number                   = {8},
  Pages                    = {530--537},
  Volume                   = {12},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1002/2014SW001095/full}
}

@Article{Mackovjak2013,
  Title                    = {On the {Possibility} to {Diagnose} the {Non}-{Maxwellian} κ-{Distributions} from the {Hinode}/{EIS} {EUV} {Spectra}},
  Author                   = {Mackovjak, Š. and Dzifčáková, E. and Dudík, J.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {2013},

  Month                    = jan,
  Pages                    = {263--281},
  Volume                   = {282},

  Doi                      = {10.1007/s11207-012-0136-0}
}

@Article{Maksimovic2003,
  Title                    = {Bow shock motions observed with {CLUSTER}},
  Author                   = {Maksimovic, M and Bale, SD and Horbury, TS and André, M},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2003},
  Number                   = {7},
  Volume                   = {30}
}

@Article{Malakit2013,
  Title                    = {New electric field in asymmetric magnetic reconnection},
  Author                   = {Malakit, Kittipat and Shay, Michael A. and Cassak, Paul A. and Ruffolo, David},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2013},
  Number                   = {13},
  Pages                    = {135001},
  Volume                   = {111},

  Url                      = {http://prl.aps.org/abstract/PRL/v111/i13/e135001},
  Urldate                  = {2014-05-31}
}

@Article{Manchester2005,
  Title                    = {Coronal {Mass} {Ejection} {Shock} and {Sheath} {Structures} {Relevant} to {Particle} {Acceleration}},
  Author                   = {Manchester, IV, W. B. and Gombosi, T. I. and De Zeeuw, D. L. and Sokolov, I. V. and Roussev, I. I. and Powell, K. G. and Kóta, J. and Tóth, G. and Zurbuchen, T. H.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2005},

  Month                    = apr,
  Pages                    = {1225--1239},
  Volume                   = {622},

  Doi                      = {10.1086/427768},
  Keywords                 = {acceleration of particles, Magnetohydrodynamics: MHD, shock waves, Sun: coronal mass ejections (CMEs)}
}

@Article{Manchester2004,
  Title                    = {Modeling a space weather event from the {Sun} to the {Earth}: {CME} generation and interplanetary propagation},
  Author                   = {Manchester, W. B. and Gombosi, T. I. and Roussev, I. and Ridley, A. and de Zeeuw, D. L. and Sokolov, I. V. and Powell, K. G. and Tóth, G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = feb,
  Pages                    = {2107},
  Volume                   = {109},

  Doi                      = {10.1029/2003JA010150},
  Keywords                 = {and Astronomy: Coronal mass ejections, and Astronomy: Magnetic fields, ASTROPHYSICS, Coronal Mass Ejection, Interplanetary Physics: Interplanetary shocks, Magnetohydrodynamics, Magnetospheric Physics: Solar wind/magnetosphere interactions, Solar Physics, Space Plasma Physics: Shock waves, space weather}
}

@Article{Manchester2004a,
  Title                    = {Three-dimensional {MHD} simulation of a flux rope driven {CME}},
  Author                   = {Manchester, W. B. and Gombosi, T. I. and Roussev, I. and de Zeeuw, D. L. and Sokolov, I. V. and Powell, K. G. and Tóth, G. and Opher, M.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = jan,
  Pages                    = {1102},
  Volume                   = {109},

  Doi                      = {10.1029/2002JA009672},
  Keywords                 = {and Astronomy: Corona, and Astronomy: Coronal mass ejections, and Astronomy: Magnetic fields, and Astronomy: Prominence eruptions, ASTROPHYSICS, Coronal Mass Ejection, Magnetohydrodynamics, Solar Physics, sun}
}

@Article{Manchester2006,
  Title                    = {Modeling the {Sun}-to-{Earth} propagation of a very fast {CME}},
  Author                   = {Manchester, W. B. and Ridley, A. J. and Gombosi, T. I. and Dezeeuw, D. L.},
  Journal                  = {Advances in Space Research},
  Year                     = {2006},

  Month                    = jan,
  Pages                    = {253--262},
  Volume                   = {38},

  Doi                      = {10.1016/j.asr.2005.09.044}
}

@Article{Mann2008,
  Title                    = {The upgraded CARISMA magnetometer array in the THEMIS era},
  Author                   = {Mann, IR and Milling, DK and Rae, IJ and Ozeke, LG and Kale, A and Kale, ZC and Murphy, KR and Parent, A and Usanova, M and Pahud, DM and others},
  Journal                  = {Space Science Reviews},
  Year                     = {2008},
  Number                   = {1-4},
  Pages                    = {413--451},
  Volume                   = {141},

  Owner                    = {suleimanbaraka},
  Publisher                = {Springer},
  Timestamp                = {2016.02.20}
}

@Article{Mao2013,
  Title                    = {Application of {Jitter} {Radiation}: {Gamma}-{Ray} {Burst} {Prompt} {Polarization}},
  Author                   = {Mao, J. and Wang, J.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2013},

  Month                    = oct,
  Pages                    = {17},
  Volume                   = {776},

  Doi                      = {10.1088/0004-637X/776/1/17},
  Keywords                 = {gamma-ray burst: general, radiation mechanisms: non-thermal, shock waves, turbulence}
}

@Article{Maqsood2004,
  Title                    = {An ensemble of neural networks for weather forecasting},
  Author                   = {Maqsood, Imran and Khan, Muhammad Riaz and Abraham, Ajith},
  Journal                  = {Neural Computing \& Applications},
  Year                     = {2004},
  Number                   = {2},
  Pages                    = {112--122},
  Volume                   = {13},

  Url                      = {http://link.springer.com/article/10.1007/s00521-004-0413-4}
}

@InProceedings{Marconi2000,
  Title                    = {The {Evolution} and {Dynamics} of {Quasi}-{Collisional} {Gas} {Tori} ({Case} of the {Triton} {Tori})},
  Author                   = {Marconi, M. L.},
  Booktitle                = {{AAS}/{Division} for {Planetary} {Sciences} {Meeting} {Abstracts} \#32},
  Year                     = {2000},
  Month                    = oct,
  Pages                    = {1084},
  Series                   = {Bulletin of the {American} {Astronomical} {Society}},
  Volume                   = {32}
}

@Article{Markidis2012,
  Title                    = {Collisionless magnetic reconnection in a plasmoid chain.},
  Author                   = {Markidis, Stefano and Henri, Pierre and Lapenta, Giovanni and Divin, Andrey and Goldman, Martin V. and Newman, David and Eriksson, Stefan},
  Journal                  = {Nonlinear Processes in Geophysics},
  Year                     = {2012},
  Number                   = {1},
  Volume                   = {19},

  Url                      = {http://search.ebscohost.com/login.aspx?direct=true&profile=ehost&scope=site&authtype=crawler&jrnl=10235809&AN=74247794&h=QZ%2ByesjAJ%2Bi%2FCOLfLSvy9pACOvlfBPLMAmmAEgqdnK6ZhkRP6j1B9P91iEr2kdQOy%2BnNMvlABf1QPzy7ew8Y6Q%3D%3D&crl=c},
  Urldate                  = {2014-05-31}
}

@Article{Markidis2011,
  Title                    = {Kinetic simulations of magnetic reconnection in presence of a background {O}+ population},
  Author                   = {Markidis, Stefano and Lapenta, Giovanni and Bettarini, Lapo and Goldman, M. and Newman, David and Andersson, Laila},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2011},
  Number                   = {A1},
  Volume                   = {116},

  Url                      = {http://www.agu.org/pubs/crossref/2011/2011JA016429.shtml},
  Urldate                  = {2014-05-31}
}

@Article{Marklund1990,
  Title                    = {Signatures of the high-altitude polar cusp and dayside auroral regions as seen by the {Viking} {Electric} {Field} {Experiment}},
  Author                   = {Marklund, GT and Blomberg, LG and Fälthammar, C-G and Erlandson, RE and Potemra, TA},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1990},
  Number                   = {A5},
  Pages                    = {5767--5780},
  Volume                   = {95}
}

@Article{Martin2002,
  Title                    = {An improved retrieval of tropospheric nitrogen dioxide from {GOME}},
  Author                   = {Martin, Randall V. and Chance, Kelly and Jacob, Daniel J. and Kurosu, Thomas P. and Spurr, Robert JD and Bucsela, Eric and Gleason, James F. and Palmer, Paul I. and Bey, Isabelle and Fiore, Arlene M. and {others}},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2002},
  Number                   = {D20},
  Pages                    = {ACH--9},
  Volume                   = {107},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2001JD001027/full},
  Urldate                  = {2014-11-13}
}

@Article{Martin2006,
  Title                    = {Evaluation of space-based constraints on global nitrogen oxide emissions with regional aircraft measurements over and downwind of eastern {North} {America}},
  Author                   = {Martin, Randall V. and Sioris, Christopher E. and Chance, Kelly and Ryerson, Thomas B. and Bertram, Timothy H. and Wooldridge, Paul J. and Cohen, Ronald C. and Neuman, J. Andy and Swanson, Aaron and Flocke, Frank M.},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2006},
  Number                   = {D15},
  Volume                   = {111},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2005JD006680/full},
  Urldate                  = {2014-11-13}
}

@Book{Massey2012,
  Title                    = {Applied atomic collision physics: {Atmospheric} physics and chemistry},
  Author                   = {Massey, Harrie Stewart Wilson},
  Publisher                = {Elsevier},
  Year                     = {2012},
  Number                   = {1},
  Volume                   = {43}
}

@Article{Matsumoto1993,
  Title                    = {Computer {Space} {Plasma} {Physics}},
  Author                   = {Matsumoto, H and Omura, Y},
  Journal                  = {Terra Sci. Publ., Tokyo},
  Year                     = {1993}
}

@Article{Matsuoka1995,
  Title                    = {Observation and modeling of compressional {Pi} 3 magnetic pulsations},
  Author                   = {Matsuoka, Hitoshi and Takahashi, K. and Yumoto, K. and Anderson, B. J. and Sibeck, D. G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1995},
  Pages                    = {12103},
  Volume                   = {100},

  Abstract                 = {Compressional magnetic pulsations with irregular waveforms and periods longer than 150 s (here termed Pi 3) have been studied by using data from Active Magnetospheric Particle Tracer Explorers Charge Composition Explorer (AMPTE/CCE) and GOES 5 and 6 in the dayside magnetosphere and compared with signatures on the ground at low latitudes by using data from Kakioka station (L = 1.25). On the ground, the pulsations appear in the horizontal component. A study of 17 such concurrent events during a 2-month period in 1986 reveals the following pulsation characteristics. (1) The peak-to-peak amplitudes in space (delta B(sub T)) and on the ground (delta H) are comparable and are in the range of 0.5-7 nT. (2) On the ground the pulsations can be seen at all local times, even at midnight, while at geostationary orbit they are observed only on the dayside with a clear amplitude maximum at noon. (3) The pulsations on the ground lag those observed by CCE near local noon, and the lag increases as the local time separation between CCE and the ground station increases. The time lag is 1-2 min longer when the ground station is on the nightside than when it is on the dayside. (4) The time lag between pulsations observed at geostationary orbit and near noon by CCE varies systematically with local time and is about 2 min per 6 hours of local time separation. These observations indicate that some nightside pulsations in the Pi 3 band have dayside origins. The position dependence of the pulsation amplitude can be explained well by changes in the magnetopause current, which are in turn presumably caused by changes in the solar wind dynamic pressure. The time lags observed in space are consistent with signal propagation in the MHD fast mode, but the variation in space-ground time lags with ground station local time must be attributed to another mechanism.},
  ISSN                     = {0148-0227},
  Keywords                 = {Earth Magnetosphere Geomagnetic Micropulsations Geomagnetism Geophysics Magnetoactivity Ampte (Satellites) Goes 5 Goes 6 Magnetic Signatures Solar Wind},
  Url                      = {http://adsabs.harvard.edu/abs/1995JGR...10012103M}
}

@Article{Mauk2013,
  Title                    = {Science {Objectives} and {Rationale} for the {Radiation} {Belt} {Storm} {Probes} {Mission}},
  Author                   = {Mauk, B. H. and Fox, N. J. and Kanekal, S. G. and Kessel, R. L. and Sibeck, D. G. and Ukhorskiy, A.},
  Journal                  = {Space Science Reviews},
  Year                     = {2013},
  Pages                    = {3--27},
  Volume                   = {179},

  Abstract                 = {The NASA Radiation Belt Storm Probes (RBSP) mission addresses how populations of high energy charged particles are created, vary, and evolve in space environments, and specifically within Earth's magnetically trapped radiation belts. RBSP, with a nominal launch date of August 2012, comprises two spacecraft making in situ measurements for at least 2 years in nearly the same highly elliptical, low inclination orbits (1.1×5.8 RE, 10{\textless}SUP{\textgreater}∘{\textless}/SUP{\textgreater}). The orbits are slightly different so that 1 spacecraft laps the other spacecraft about every 2.5 months, allowing separation of spatial from temporal effects over spatial scales ranging from ˜0.1 to 5 RE. The uniquely comprehensive suite of instruments, identical on the two spacecraft, measures all of the particle (electrons, ions, ion composition), fields ( E and B), and wave distributions ( d E and d B) that are needed to resolve the most critical science questions. Here we summarize the high level science objectives for the RBSP mission, provide historical background on studies of Earth and planetary radiation belts, present examples of the most compelling scientific mysteries of the radiation belts, present the mission design of the RBSP mission that targets these mysteries and objectives, present the observation and measurement requirements for the mission, and introduce the instrumentation that will deliver these measurements. This paper references and is followed by a number of companion papers that describe the details of the RBSP mission, spacecraft, and instruments.},
  ISSN                     = {0038-6308},
  Keywords                 = {Radiation belt Magnetosphere Geomagnetic storms NASA mission},
  Url                      = {http://adsabs.harvard.edu/abs/2013SSRv..179....3M}
}

@Article{Maynard2011,
  Title                    = {Interactions of the heliospheric current and plasma sheets with the bow shock: {Cluster} and {Polar} observations in the magnetosheath},
  Author                   = {Maynard, Nelson C and Farrugia, Charles J and Burke, William J and Ober, Daniel M and Scudder, Jack D and Mozer, Forrest S and Russell, Christopher T and Rème, Henri and Mouikis, Christopher and Siebert, Keith D},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2011},
  Number                   = {A1},
  Volume                   = {116}
}

@Article{Mazelle2010,
  Title                    = {Self-{Reformation} of the {Quasi}-{Perpendicular} {Shock}: {CLUSTER} {Observations}},
  Author                   = {Mazelle, C. and Lembège, B. and Morgenthaler, A. and Meziane, K. and Horbury, T. S. and Génot, V. and Lucek, E. A. and Dandouras, I.},
  Journal                  = {Twelfth International Solar Wind Conference},
  Year                     = {2010},

  Month                    = mar,
  Pages                    = {471--474},
  Volume                   = {1216},

  Doi                      = {10.1063/1.3395905},
  Keywords                 = {artificial, Electric and magnetic fields solar magnetism, Heliopause and solar wind termination, interplanetary shocks, Magnetic Fields, Planetary bow shocks, satellites, shock wave effects, spacecraft, Spacecraft/atmosphere interactions}
}

@Article{Mazelle2003,
  Title                    = {Production of gyrating ions from nonlinear wave–particle interaction upstream from the {Earth}'s bow shock: {A} case study from {Cluster}-{CIS}},
  Author                   = {Mazelle, C and Meziane, K and LeQuéau, D and Wilber, M and Eastwood, JP and Reme, H and Sauvaud, JA and Bosqued, JM and Dandouras, I and McCarthy, M and {others}},
  Journal                  = {Planetary and Space Science},
  Year                     = {2003},
  Number                   = {12},
  Pages                    = {785--795},
  Volume                   = {51}
}

@Article{Mazzotta1998,
  Title                    = {Ionization balance for optically thin plasmas: {Rate} coefficients for all atoms and ions of the elements {H} to {NI}},
  Author                   = {Mazzotta, P. and Mazzitelli, G. and Colafrancesco, S. and Vittorio, N.},
  Journal                  = {{\textbackslash}aaps},
  Year                     = {1998},

  Month                    = dec,
  Pages                    = {403--409},
  Volume                   = {133},

  Doi                      = {10.1051/aas:1998330},
  Keywords                 = {atomic data, plasmas, radiation mechanisms: thermal, X-rays: general}
}

@Article{McComas2000,
  Title                    = {Solar wind observations over {Ulysses}' first full polar orbit},
  Author                   = {McComas, David J. and Barraclough, B. L. and Funsten, H. O. and Gosling, J. T. and Santiago-Muñoz, E. and Skoug, Ruth M. and Goldstein, B. E. and Neugebauer, Marsha and Riley, Pete and Balogh, A.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {2000},

  Month                    = may,
  Pages                    = {10419--10434},
  Volume                   = {105},

  Doi                      = {10.1029/1999JA000383},
  Keywords                 = {Interplanetary Physics: Interplanetary magnetic fields, Interplanetary Physics: Solar cycle variations, Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Sources of the solar wind}
}

@Article{McComas2008,
  Title                    = {Weaker solar wind from the polar coronal holes and the whole {Sun}},
  Author                   = {McComas, D. J. and Ebert, R. W. and Elliott, H. A. and Goldstein, B. E. and Gosling, J. T. and Schwadron, N. A. and Skoug, R. M.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {2008},

  Month                    = sep,
  Pages                    = {18103},
  Volume                   = {35},

  Doi                      = {10.1029/2008GL034896},
  Keywords                 = {Interplanetary Physics: Heliopause and solar wind termination, Interplanetary Physics: Interplanetary magnetic fields, Interplanetary Physics: Solar cycle variations (7536), Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Solar wind sources}
}

@Article{McComas2003,
  Title                    = {The three-dimensional solar wind around solar maximum},
  Author                   = {McComas, D. J. and Elliott, H. A. and Schwadron, N. A. and Gosling, J. T. and Skoug, R. M. and Goldstein, B. E.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {2003},

  Month                    = may,
  Pages                    = {1517},
  Volume                   = {30},

  Doi                      = {10.1029/2003GL017136},
  Keywords                 = {Interplanetary Physics: Corotating streams, Interplanetary Physics: General or miscellaneous, Interplanetary Physics: Interplanetary shocks, Interplanetary Physics: Solar cycle variations (7536), Interplanetary Physics: Solar wind plasma}
}

@Article{McIntosh2011,
  Title                    = {Solar {Cycle} {Variations} in the {Elemental} {Abundance} of {Helium} and {Fractionation} of {Iron} in the {Fast} {Solar} {Wind}: {Indicators} of an {Evolving} {Energetic} {Release} of {Mass} from the {Lower} {Solar} {Atmosphere}},
  Author                   = {McIntosh, S. W. and Kiefer, K. K. and Leamon, R. J. and Kasper, J. C. and Stevens, M. L.},
  Journal                  = {{\textbackslash}apjl},
  Year                     = {2011},

  Month                    = oct,
  Pages                    = {L23},
  Volume                   = {740},

  Doi                      = {10.1088/2041-8205/740/1/L23},
  Keywords                 = {Solar Wind, Sun: chromosphere, Sun: corona, Sun: heliosphere, Sun: surface magnetism, Sun: transition region}
}

@Article{McKee2007,
  Title                    = {{Theory of Star Formation}},
  Author                   = {McKee, C F and Ostriker, E C},
  Journal                  = {Annu. Rev. Astron. Astrophys.},
  Year                     = {2007},
  Volume                   = {45},

  __markedentry            = {[suleimanbaraka:]},
  Archiveprefix            = {arXiv},
  Arxivid                  = {0707.3514},
  Doi                      = {10.1146/annurev.astro.45.051806.110602},
  Eprint                   = {0707.3514},
  ISBN                     = {0066-4146},
  ISSN                     = {0066-4146},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{McPherron1997,
  Title                    = {The role of substorms in the generation of magnetic storms},
  Author                   = {McPherron, RL},
  Journal                  = {Magnetic Storms},
  Year                     = {1997},
  Pages                    = {131--147}
}

@Article{McPherron1988,
  Title                    = {{IMF} control of geomagnetic activity},
  Author                   = {McPherron, RL and Baker, DN and Bargatze, LF and Clauer, CR and Holzer, RE},
  Journal                  = {Advances in Space Research},
  Year                     = {1988},
  Number                   = {9},
  Pages                    = {71--86},
  Volume                   = {8}
}

@Article{McWilliams2004,
  Title                    = {Simultaneous observations of magnetopause flux transfer events and of their associated signatures at ionospheric altitudes},
  Author                   = {McWilliams, K. and Sofko, G. and Yeoman, T. and Milan, S. and Sibeck, D. and Nagai, T. and Mukai, T. and Coleman, I. and Hori, T. and Rich, F.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2004},
  Pages                    = {2181--2199},
  Volume                   = {22},

  Abstract                 = {Available from {\textless}A href="http://www.copernicus.org/site/EGU/annales/22/6/2181.htm?FrameEngine=false;"{\textgreater}http://www.copernicus.org/site/EGU/annales/22/6/2181.htm?FrameEngine=false;{\textless}/A{\textgreater}},
  ISSN                     = {0992-7689},
  Url                      = {http://adsabs.harvard.edu/abs/2004AnGeo..22.2181M}
}

@InCollection{Mende2000,
  Title                    = {Far ultraviolet imaging from the {IMAGE} spacecraft: 1. {System} design},
  Author                   = {Mende, SB and Heetderks, H and Frey, HU and Lampton, M and Geller, SP and Habraken, Serge and Renotte, Etienne and Jamar, Claude and Rochus, Pierre and Spann, J and {others}},
  Booktitle                = {The {Image} {Mission}},
  Publisher                = {Springer},
  Year                     = {2000},
  Pages                    = {243--270}
}

@Article{Mende2009,
  Title                    = {Coordinated observation of the dayside magnetospheric entry and exit of the {THEMIS} satellites with ground-based auroral imaging in {Antarctica}},
  Author                   = {Mende, S. B. and Frey, H. U. and McFadden, J. and Carlson, C. W. and Angelopoulos, V. and Glassmeier, K.-H. and Sibeck, D. G. and Weatherwax, A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2009},
  Volume                   = {114},

  Abstract                 = {Data from the five-satellite Time History of Events and Macroscale Interactions during Substorms (THEMIS) constellation suitably located to study solar wind magnetospheric coupling during the austral winter of 2007 were compared to data from ground-based all-sky imagers (ASIs) at South Pole (74° magnetic latitude) and at AGO-1 (80° magnetic latitude). The THEMIS constellation entered and exited the magnetosphere near magnetic midday on 10 and 12 August 2007, respectively. On 12 August interplanetary magnetic field (IMF) (B {\textless}SUB{\textgreater} z {\textless}/SUB{\textgreater} {\textgreater} 0) the dayside aurora was located more poleward between AGO-1 and South Pole. The THEMIS satellites traversing the magnetopause saw it move in and out several times during the satellite crossings. The inward motion of the magnetopause was sometimes correlated with equatorward expansions of the aurora and sometimes with solar wind pressure pulses as seen by Geotail. The B {\textless}SUB{\textgreater} z {\textless}/SUB{\textgreater} {\textgreater} 0 auroral latitude was consistent with dayside cusp “spot” seen by the IMAGE spacecraft and had been associated with footprints of “steady state” lobe reconnection. The aurora consisted of a continuous stream of poleward moving auroral forms (PMAF) even during a period of slightly B {\textless}SUB{\textgreater} z {\textless}/SUB{\textgreater} {\textgreater} 0 and B {\textless}SUB{\textgreater} y {\textless}/SUB{\textgreater} = 0. On 10 August 2007 IMF B {\textless}SUB{\textgreater} z {\textless}/SUB{\textgreater} {\textless} 0 the dayside aurora was located more equatorward, over South Pole, and the THEMIS satellites crossed the bow shock from the magnetosheath into the solar wind. Negative B {\textless}SUB{\textgreater} z {\textless}/SUB{\textgreater} pulses observed at the satellite were correlated with large poleward expansions of the dayside aurora consistent with reconnection in the subsolar region accompanied by simultaneous plasma density increases at THEMIS B satellite consistent with outward radial motion of the bow shock.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Polar cap phenomena Magnetospheric Physics: Auroral phenomena (2407) Magnetospheric Physics: Magnetic reconnection (7526 7835)},
  Url                      = {http://adsabs.harvard.edu/abs/2009JGRA..114.0C23M}
}

@Article{Meng2012,
  Title                    = {Pressure anisotropy in global magnetospheric simulations: {A} magnetohydrodynamics model},
  Author                   = {Meng, X. and T‚àö‚â•th, G. and Liemohn, M. W. and Gombosi, T. I. and Runov, A.},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978‚Äö√Ñ√¨2012)},
  Year                     = {2012},
  Number                   = {A8},
  Volume                   = {117},

  Shorttitle               = {Pressure anisotropy in global magnetospheric simulations},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2012JA017791/full},
  Urldate                  = {2014-10-22}
}

@Article{Mercas2013,
  Title                    = {Binary {Patterns} in {Binary} {Cube}-{Free} {Words}: {Avoidability} and {Growth}},
  Author                   = {Mercas, R. and Ochem, P. and Samsonov, A. V. and Shur, A. M.},
  Journal                  = {ArXiv e-prints},
  Year                     = {2013},

  Month                    = jan,

  Keywords                 = {68R15, Computer Science - Formal Languages and Automata Theory, Mathematics - Combinatorics}
}

@Article{Merka2003,
  Title                    = {Earth's bow shock and magnetopause in the case of a field-aligned upstream flow: {Observation} and model comparison},
  Author                   = {Merka, J and Szabo, A and Šafránková, J and Němeček, Z},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2003},
  Number                   = {A7},
  Volume                   = {108}
}

@Article{Meziane2014,
  Title                    = {On the shape and motion of the {Earth}'s bow shock},
  Author                   = {Meziane, K and Alrefay, TY and Hamza, AM},
  Journal                  = {Planetary and Space Science},
  Year                     = {2014}
}

@Article{Meziane2014a,
  Title                    = {On the shape and motion of the {Earth} ' s bow shock},
  Author                   = {Meziane, K and Alrefay, T Y and Hamza, A M},
  Journal                  = {Planet. Space Sci.},
  Year                     = {2014},
  Pages                    = {1--9},
  Volume                   = {93-94},

  Doi                      = {10.1016/j.pss.2014.01.006},
  ISSN                     = {0032-0633},
  Keywords                 = {bow shock, interplanetary magnetic field, Magnetohydrodynamics, Solar Wind},
  Url                      = {http://dx.doi.org/10.1016/j.pss.2014.01.006}
}

@Article{Meziane2015,
  Title                    = {The {Earth}'s bow shock velocity distribution function},
  Author                   = {Meziane, K. and Hamza, A. M. and Maksimovic, M. and Alrefay, T. Y.},
  Journal                  = {Journal of Geophysical Research: Space Physics},
  Year                     = {2015},
  Number                   = {2},
  Pages                    = {1229--1237},
  Volume                   = {120},

  File                     = {Snapshot:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/RXK384MW/pdf.html:text/html},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1002/2014JA020772/pdf},
  Urldate                  = {2016-01-11}
}

@Article{Meziane1997,
  Title                    = {Wind observation of gyrating-like ion distributions and low frequency waves upstream from the {Earth}'s bow shock},
  Author                   = {Meziane, K and Mazelle, C and d'Uston, C and Reme, H and Lin, RP and Carlson, CW and Larson, D and McFadden, JP and Ergun, RE and Anderson, KA and {others}},
  Journal                  = {Advances in Space Research},
  Year                     = {1997},
  Number                   = {4},
  Pages                    = {703--706},
  Volume                   = {20}
}

@Article{Meziane2001,
  Title                    = {Three-dimensional observations of gyrating ion distributions far upstream from the {Earth}'s bow shock and their association with low-frequency waves},
  Author                   = {Meziane, K and Mazelle, C and Lin, RP and LeQuéau, D and Larson, DE and Parks, GK and Lepping, RP},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2001},
  Number                   = {A4},
  Pages                    = {5731--5742},
  Volume                   = {106}
}

@Article{Meziane2007,
  Title                    = {Evidence for a high-energy tail associated with foreshock field-aligned beams},
  Author                   = {Meziane, K and Wilber, M and Hamza, AM and Mazelle, C and Parks, GK and Reme, H and Lucek, EA},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2007},
  Number                   = {A1},
  Pages                    = {A01101},
  Volume                   = {112}
}

@Article{Meziane2004,
  Title                    = {Simultaneous observations of field-aligned beams and gyrating ions in the terrestrial foreshock},
  Author                   = {Meziane, K and Wilber, M and Mazelle, C and LeQuéau, D and Kucharek, H and Lucek, EA and Reme, H and Hamza, AM and Sauvaud, JA and Bosqued, JM and {others}},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2004},
  Number                   = {A5},
  Volume                   = {109}
}

@Article{Michel1971,
  Title                    = {Solar wind interaction with planetary atmospheres.},
  Author                   = {Michel, F. C.},
  Journal                  = {Rev. Geophys. Space Phys.},
  Year                     = {1971},
  Pages                    = {427--435},
  Volume                   = {9},

  Abstract                 = {Not Available},
  Doi                      = {10.1029/RG009i002p00427}
}

@Article{Millet2008,
  Title                    = {Spatial distribution of isoprene emissions from {North} {America} derived from formaldehyde column measurements by the {OMI} satellite sensor},
  Author                   = {Millet, Dylan B. and Jacob, Daniel J. and Boersma, K. Folkert and Fu, Tzung-May and Kurosu, Thomas P. and Chance, Kelly and Heald, Colette L. and Guenther, Alex},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2008},
  Number                   = {D2},
  Volume                   = {113},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2007JD008950/full},
  Urldate                  = {2014-11-13}
}

@Book{Miralles2011,
  Title                    = {The {Sun}, the {Solar} {Wind}, and the {Heliosphere}},
  Author                   = {Miralles, M. P. and Sánchez Almeida, J.},
  Year                     = {2011}
}

@Article{Miranda2013,
  Title                    = {Universal scaling laws for fully-developed magnetic field turbulence near and far upstream of the {Earth}¬¨¬®‚àö‚â†s bow shock},
  Author                   = {Miranda, Rodrigo A and Chian, Abraham C-L and Rempel, Erico L},
  Journal                  = {Advances in Space Research},
  Year                     = {2013},
  Number                   = {10},
  Pages                    = {1893--1901},
  Volume                   = {51}
}

@Article{Mishin1993,
  Title                    = {Accelerated motions of the magnetopause as a trigger of the {Kelvin}-{Helmholtz} instability},
  Author                   = {Mishin, VV},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1993},
  Number                   = {A12},
  Pages                    = {21365--21371},
  Volume                   = {98}
}

@Article{Mitchell1987,
  Title                    = {An extended study of the low-latitude boundary layer on the dawn and dusk flanks of the magnetosphere},
  Author                   = {Mitchell, DG and Kutchko, F and Williams, DJ and Eastman, TE and Frank, LA and Russell, CT},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1987},
  Number                   = {A7},
  Pages                    = {7394--7404},
  Volume                   = {92}
}

@Book{Moldwin2008,
  Title                    = {An introduction to space weather},
  Author                   = {Moldwin, Mark},
  Publisher                = {Cambridge University Press},
  Year                     = {2008},

  Address                  = {Cambridge},

  ISBN                     = {978-0-521-86149-6 0-521-86149-7 978-0-521-71112-8 0-521-71112-6},
  Keywords                 = {Space environment}
}

@Article{Moore2010,
  Title                    = {{The birth of topological insulators.}},
  Author                   = {Moore, Joel E},
  Journal                  = {Nature},
  Year                     = {2010},
  Number                   = {7286},
  Volume                   = {464},

  __markedentry            = {[suleimanbaraka:]},
  Archiveprefix            = {arXiv},
  Arxivid                  = {arXiv:1011.5462v1},
  Doi                      = {10.1038/nature08916},
  Eprint                   = {arXiv:1011.5462v1},
  ISBN                     = {1476-4687 (Electronic)$\backslash$n0028-0836 (Linking)},
  ISSN                     = {1476-4687},
  Owner                    = {suleimanbaraka},
  Pmid                     = {20220837},
  Timestamp                = {2016.02.23}
}

@Article{Moore1985,
  Title                    = {Superthermal ion signatures of auroral acceleration processes},
  Author                   = {Moore, TE and Chappell, CR and Lockwood, M and Waite, JH},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1985},
  Number                   = {A2},
  Pages                    = {1611--1618},
  Volume                   = {90},

  Annote                   = {Added to JabRef: 2015.04.18}
}

@Article{Moore1984,
  Title                    = {Superthermal ionospheric outflows},
  Author                   = {Moore, Thomas Earle},
  Journal                  = {Rev. Geophys.},
  Year                     = {1984},
  Number                   = {3},
  Pages                    = {264--274},
  Volume                   = {22},

  Annote                   = {Added to JabRef: 2015.04.18}
}

@Article{Moore1999,
  Title                    = {Chapter 2-{Source} {Processes} in the {High}-{Latitude} {Ionosphere}},
  Author                   = {Moore, T. E. and Lundin, R. and Alcayde, D. and André, M. and Ganguli, S. B. and Temerin, M. and Yau, A.},
  Journal                  = {ßr},
  Year                     = {1999},

  Month                    = apr,
  Pages                    = {7--84},
  Volume                   = {88},

  Doi                      = {10.1023/A:1005299616446}
}

@Article{Moore1999a,
  Title                    = {Chapter 2-{Source} {Processes} in the {High}-{Latitude} {Ionosphere}},
  Author                   = {Moore, T. E. and Lundin, R. and Alcayde, D. and Andr√©, M. and Ganguli, S. B. and Temerin, M. and Yau, A.},
  Journal                  = {√ür},
  Year                     = {1999},

  Month                    = apr,
  Pages                    = {7--84},
  Volume                   = {88},

  Doi                      = {10.1023/A:1005299616446}
}

@Article{Moretto2004,
  Title                    = {Occurrence statistics of magnetic impulsive events},
  Author                   = {Moretto, T. and Sibeck, D. and Watermann, J.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2004},
  Pages                    = {585--602},
  Volume                   = {22},

  Abstract                 = {. In this study, we perform a statistical investigation of magnetic impulse events identified in the Greenland magnetometer stations through the years 1995-2001. We focus on occurrence statistics that can be determined reliably with an automatic event identification procedure. Durin the first two years we observed almost 40\% more events than in the following years. Season is not a significant factor in event occurrence. Event occurrence peaks near 12:00 UT, corresponding to approximately 10:00 magnetic local time (MLT) at the west coast of Greenland. More events occur prior to local noon than after. Event days are not distributed evenly. Large amplitude events, particularly, tend to appear on consecutive days. Events are observed at lower latitudes at earlier local times in a way consistent with the projection of the outer magnetospheric boundary into the ionosphere. Event latitude depends on dipole tilt angle in a manner similar to that reported for the cusp. Events occur during intervals of enhanced Kp. The main reason for this is that the events themselves contribute to the Kp index. Events exhibit a preference for high solar wind velocity. In particular, the large amplitude events occur during high-speed streams. A slight preference for lower density and more radial interplanetary magnetic fields, as compared to the nominal solar wind distribution, is also observed. However, both the nominal solar wind and event distribution exhibit large differences from year to year, indicating that events occur under a broad range of conditions.},
  ISSN                     = {0992-7689},
  Url                      = {http://adsabs.harvard.edu/abs/2004AnGeo..22..585M}
}

@Article{Moritaka2012,
  Title                    = {Momentum transfer of solar wind plasma in a kinetic scale magnetosphere},
  Author                   = {Moritaka, Toseo and Kajimura, Yoshihiro and Usui, Hideyuki and Matsumoto, Masaharu and Matsui, Tatsuki and Shinohara, Iku},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2012},
  Number                   = {3},
  Pages                    = {032111},
  Volume                   = {19},

  Owner                    = {suleimanbaraka},
  Publisher                = {AIP Publishing},
  Timestamp                = {2016.02.21}
}

@InProceedings{Murr2004,
  Title                    = {Scarf award presentation: {Magnetosphere}-ionosphere coupling studies of dayside high-latitude transients},
  Author                   = {Murr, DL},
  Booktitle                = {{AGU} {Fall} {Meeting} {Abstracts}},
  Year                     = {2004},
  Pages                    = {01},
  Volume                   = {1}
}

@Article{Murtagh2007,
  Title                    = {Space {Weather} {Enterprise} {Forum}},
  Author                   = {Murtagh, William J},
  Journal                  = {Space Weather},
  Year                     = {2007},
  Number                   = {1},
  Volume                   = {5},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2006SW000302/full}
}

@Article{Muschietti2006a,
  Title                    = {{Electron cyclotron microinstability in the foot of a perpendicular shock: A self-consistent PIC simulation}},
  Author                   = {Muschietti, L and Lemb{\`{e}}ge, B},
  Journal                  = {Adv. Sp. Res.},
  Year                     = {2006},
  Pages                    = {483--493},
  Volume                   = {37},

  __markedentry            = {[suleimanbaraka:6]},
  Doi                      = {10.1016/j.asr.2005.03.077},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Muschietti, Lemb{\`{e}}ge/Advances in Space Research/Muschietti, Lemb{\`{e}}ge - 2006 - Electron cyclotron microinstability in the foot of a perpendicular shock A self-consistent PIC simulation.pdf:pdf},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Muschietti2013,
  Title                    = {Microturbulence in the electron cyclotron frequency range at perpendicular supercritical shocks},
  Author                   = {Muschietti, L. and LembèGe, B.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = may,
  Pages                    = {2267--2285},
  Volume                   = {118},

  Doi                      = {10.1002/jgra.50224},
  Keywords                 = {Collisionless shocks, numerical simulation, Plasma microinstabilities, Shock foot}
}

@Article{Muschietti2006,
  Title                    = {Electron cyclotron microinstability in the foot of a perpendicular shock: {A} self-consistent {PIC} simulation},
  Author                   = {Muschietti, L. and Lembège, B.},
  Journal                  = {Advances in Space Research},
  Year                     = {2006},
  Pages                    = {483--493},
  Volume                   = {37},

  Doi                      = {10.1016/j.asr.2005.03.077}
}

@Article{Nakamura2004,
  Title                    = {Spatial scale of high-speed flows in the plasma sheet observed by {Cluster}},
  Author                   = {Nakamura, R and Baumjohann, W and Mouikis, C and Kistler, LM and Runov, A and Volwerk, M and Asano, Y and Vörös, Z and Zhang, TL and Klecker, B and {others}},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2004},
  Number                   = {9},
  Volume                   = {31}
}

@InProceedings{Nakamura2005,
  Title                    = {Cluster and {Double} {Star} observations of dipolarization},
  Author                   = {Nakamura, R and Baumjohann, W and Zhang, TL and Carr, CM and Balogh, A and Fornacon, KH and Georgescu, E and Reme, H and Dandouras, I and Takada, T and {others}},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2005},
  Pages                    = {2915--2920},
  Publisher                = {Copernicus GmbH},
  Volume                   = {23}
}

@Article{Namouni2010,
  Title                    = {The {Fate} of {Moons} of {Close}-in {Giant} {Exoplanets}},
  Author                   = {Namouni, F.},
  Journal                  = {{\textbackslash}textbackslashapjl},
  Year                     = {2010},

  Month                    = aug,
  Pages                    = {L145--L147},
  Volume                   = {719},

  Doi                      = {10.1088/2041-8205/719/2/L145},
  Keywords                 = {planetary systems, planets and satellites: formation}
}

@InProceedings{Narita2006,
  Title                    = {Propagation pattern of low frequency waves in the terrestrial magnetosheath},
  Author                   = {Narita, Y and Glassmeier, K-H},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2006},
  Pages                    = {2441--2444},
  Publisher                = {Copernicus GmbH},
  Volume                   = {24}
}

@Article{Nariyuki2007,
  Title                    = {Consequences of finite ion temperature effects on parametric instabilities of circularly polarized {Alfvén} waves},
  Author                   = {Nariyuki, Y. and Hada, T.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2007},

  Month                    = oct,
  Number                   = {A11},
  Pages                    = {10107},
  Volume                   = {112},

  Doi                      = {10.1029/2007JA012373},
  Keywords                 = {2487, 2752, 3280, 3285, 4275, 6050), 6934, 7851, 7852), Alfvén waves, ion kinetics, Nonlinear Geophysics: Nonlinear waves, shock waves, Solar Wind, solitons (0689, Space Plasma Physics: Kinetic and MHD theory, Space Plasma Physics: MHD waves and instabilities (2149, Space Plasma Physics: Wave/wave interactions}
}

@Article{Nariyuki2006,
  Title                    = {Kinetically modified parametric instabilities of circularly polarized {Alfvén} waves: {Ion} kinetic effects},
  Author                   = {Nariyuki, Y. and Hada, T.},
  Journal                  = {Phys. Plasmas},
  Year                     = {2006},

  Month                    = dec,
  Number                   = {12},
  Pages                    = {124501},
  Volume                   = {13},

  Doi                      = {10.1063/1.2399468},
  Keywords                 = {Macroinstabilities, Magnetohydrodynamics, Magnetohydrodynamic waves, Plasma kinetic equations, Transport Properties}
}

@Article{Nariyuki2012,
  Title                    = {Nonlinear dissipation of circularly polarized {Alfvén} waves due to the beam-induced obliquely propagating waves},
  Author                   = {Nariyuki, Y. and Hada, T. and Tsubouchi, K.},
  Journal                  = {Phys. Plasmas},
  Year                     = {2012},

  Month                    = aug,
  Number                   = {8},
  Pages                    = {082317},
  Volume                   = {19},

  Doi                      = {10.1063/1.4748296},
  Keywords                 = {astrophysical plasma, Macroinstabilities, Magnetohydrodynamic waves, Nonlinear phenomena: waves wave propagation and other interactions, numerical analysis, numerical simulation, Particle beam interactions in plasmas, plasma Alfven waves, plasma-beam interactions, plasma instability, plasma nonlinear waves, plasma simulation, Solar Wind, solution of equations, wave propagation}
}

@Article{Nariyuki2007a,
  Title                    = {Parametric instabilities of parallel propagating incoherent {Alfvén} waves in a finite ion beta plasma},
  Author                   = {Nariyuki, Y. and Hada, T. and Tsubouchi, K.},
  Journal                  = {Phys. Plasmas},
  Year                     = {2007},

  Month                    = dec,
  Number                   = {12},
  Pages                    = {122110},
  Volume                   = {14},

  Doi                      = {10.1063/1.2824986},
  Keywords                 = {Macroinstabilities, Magnetohydrodynamics, Magnetohydrodynamic waves, Plasma Turbulence}
}

@Article{Natraj2011,
  Title                    = {Multi-spectral sensitivity studies for the retrieval of tropospheric and lowermost tropospheric ozone from simulated clear-sky {GEO}-{CAPE} measurements},
  Author                   = {Natraj, Vijay and Liu, Xiong and Kulawik, Susan and Chance, Kelly and Chatfield, Robert and Edwards, David P and Eldering, Annmarie and Francis, Gene and Kurosu, Thomas and Pickering, Kenneth and {others}},
  Journal                  = {Atmos. Environ.},
  Year                     = {2011},
  Number                   = {39},
  Pages                    = {7151--7165},
  Volume                   = {45}
}

@Article{Nemecek2011,
  Title                    = {{MHD} analysis of propagation of an interplanetary shock across magnetospheric boundaries},
  Author                   = {Němeček, Z and Šafránková, J and Koval, A and Merka, J and Přech, L},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2011},
  Number                   = {1},
  Pages                    = {20--29},
  Volume                   = {73}
}

@Article{Nemecek1998,
  Title                    = {Transient flux enhancements in the magnetosheath},
  Author                   = {Němeček, Z. and Šafránková, J. and Přech, L. and Sibeck, D. G. and Kokubun, S. and Mukai, T.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1998},
  Pages                    = {1273--1276},
  Volume                   = {25},

  Abstract                 = {This study presents INTERBALL-1, and MAGION-4 observations of transient ion flux variations in the magnetosheath which cannot be related to similar changes in the solar wind observed by WIND and GEOTAIL. The duration of the transient events varies from tens of seconds to a few minutes and their amplitude can exceed background levels by a factor of 2 or more. We use the closely-spaced INTERBALL-1 and MAGION-4 satellites to estimate that the spatial dimensions of the events are on the order of ∼ 1R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}. The interaction of foreshock discontinuities with the bow shock is identified as a possible source of these events.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/1998GeoRL..25.1273N}
}

@Article{Neugebauer2002,
  Title                    = {Sources of the solar wind at solar activity maximum},
  Author                   = {Neugebauer, M. and Liewer, P. C. and Smith, E. J. and Skoug, R. M. and Zurbuchen, T. H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2002},

  Month                    = dec,
  Pages                    = {1488},
  Volume                   = {107},

  Doi                      = {10.1029/2001JA000306},
  Keywords                 = {Coronal holes, Interplanetary Physics: Solar cycle variations (7536), Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Sources of the solar wind, solar active regions, solar wind sources}
}

@Article{Newell1989,
  Title                    = {Some low-altitude cusp dependencies on the interplanetary magnetic field},
  Author                   = {Newell, Patrick T and Meng, Ching-I and Sibeck, David G and Lepping, Ronald},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1989},
  Number                   = {A7},
  Pages                    = {8921--8927},
  Volume                   = {94}
}

@Article{Newell1994,
  Title                    = {Reply to {Lockwood}, {Cowley}, and {Smith}},
  Author                   = {Newell, Patrick T. and Sibeck, David G.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1994},
  Pages                    = {1821--1822},
  Volume                   = {21},

  Abstract                 = {Not Available},
  ISSN                     = {0094-8276},
  Keywords                 = {Ionosphere: Plasma convection},
  Url                      = {http://adsabs.harvard.edu/abs/1994GeoRL..21.1821N}
}

@Article{Newell1993,
  Title                    = {By fluctuations in the magnetosheath and azimuthal flow velocity transients in the dayside ionosphere},
  Author                   = {Newell, Patrick T and Sibeck, David G},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1993},
  Number                   = {16},
  Pages                    = {1719--1722},
  Volume                   = {20}
}

@Article{Newell1993a,
  Title                    = {Upper limits on the contribution of flux transfer events to ionospheric convection},
  Author                   = {Newell, Patrick T. and Sibeck, David G.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1993},
  Pages                    = {2829--2832},
  Volume                   = {20},

  Abstract                 = {The possiblility that merging might largely consist of bursts of subsolar merging repeating every 8 minutes (Flux Transfer Events - FTEs) has been raised. We examined the maximum possible contribution to the cross polar cap potential from FTEs. Assuming each candidate FTE actually transfer flux, we calculate the contribution from: (1) FTEs which fit statistical magnetopause observations; (2) FTEs which fit typical ionospheric observations; (3) The largest reported FTEs in case studies at low and high altitude. We find that FTEs account for less than 10\% of a normal active time polar cap potential (approximately 100 kV); although some individual reported cases could, with optimistic assumptions, account for 20-33\%. Two new limits on the size of FTEs are introduced. The requirement that FTEs form within +/- 6 R(sub e) of the subsolar point limits FTEs to producing about 38 kV average potential. An even more fundamental limit is imposed by coherence; to represent a merging burst which starts and stops in 2 minutes, an FTE size is limited by the fast mode wave velocity. The coherence limit is about 14.5 kV, meaning that larger pulses consist of independenly active merging sites. Simulation results in which bursty merging dominates are reconsidered, and shown to have geometrical assumptions that may be applicable locally, but not globally. A burst of subsolar merging every 8 minutes therefore cannot contribute most of the cross polar cap potential.},
  ISSN                     = {0094-8276},
  Keywords                 = {Flux Transfer Events Magnetohydrodynamic Waves Magnetosphere-Ionosphere Coupling Three Dimensional Models Two Dimensional Models Interplanetary Magnetic Fields Lines Of Force Magnetic Signatures Polar Regions},
  Url                      = {http://adsabs.harvard.edu/abs/1993GeoRL..20.2829N}
}

@Article{Newell1995,
  Title                    = {Penetration of the interplanetary magnetic field {B}(sub y) magnetosheath plasma into the magnetosphere: {Implications} for the predominant magnetopause merging site},
  Author                   = {Newell, Patrick T. and Sibeck, David G. and Meng, Ching-I.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1995},
  Pages                    = {235--243},
  Volume                   = {100},

  Abstract                 = {Magnetosheath plasma peertated into the magnetospere creating the particle cusp, and similarly the interplanetary magnetic field (IMF) B(sub y) component penetrates the magnetopause. We reexamine the phenomenology of such penetration to investigate implications for the magnetopause merging site. Three models are popular: (1) the 'antiparallel' model, in which merging occurs where the local magnetic shear is largest (usually high magnetic latitude); (2) a tilted merging line passing through the subsolar point but extending to very high latitudes; or (3) a tilted merging line passing through the subsolar point in which most merging occurs within a few Earth radii of the equatorial plane and local noon (subsolar merging). It is difficult to distinguish between the first two models, but the third implies some very different predictions. We show that properties of the particle cusp imply that plasma injection into the magnetosphere occurs most often at high magnetic latitudes. In particular, we note the following: (1) The altitude of the merging site inferred from midaltitude cusp ion pitch angle dispersion is typically 8-12 R(sub E). (2) The highest ion energy observable when moving poleward through the cusp drops long before the bulk of the cusp plasma is reached, implying that ions are swimming upstream against the sheath flow shortly after merging. (3) Low-energy ions are less able to enter the winter cusp than the summer cusp. (4) The local time behavior of the cusp as a function of B(sub y) and B(sub z) corroborates predictions of the high-latitude merging models. We also reconsider the penetration of the IMF B(sub y) component onto closed dayside field lines. Our approach, in which closed field lines ove to fill in flux voids created by asymmetric magnetopause flux erosion, shows that strich subsolar merging cannot account for the observations.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Magnetic Fields Magnetohydrodynamic Flow Magnetopause Magnetosheath Plasmas (Physics) Magnetic Dipoles Magnetic Flux Mathematical Models Spectrum Analysis},
  Url                      = {http://adsabs.harvard.edu/abs/1995JGR...100..235N}
}

@Article{Ng2012,
  Title                    = {Phase space structure of the electron diffusion region in reconnection with weak guide fields},
  Author                   = {Ng, J. and Egedal, J. and Le, A. and Daughton, W.},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2012},
  Number                   = {11},
  Pages                    = {112108},
  Volume                   = {19},

  Url                      = {http://scitation.aip.org/content/aip/journal/pop/19/11/10.1063/1.4766895},
  Urldate                  = {2014-05-31}
}

@InCollection{Nilsson2011,
  Title                    = {Heavy ion energization, transport, and loss in the {Earth}√î√∏Œ©s magnetosphere},
  Author                   = {Nilsson, Hans},
  Booktitle                = {The {Dynamic} {Magnetosphere}},
  Publisher                = {Springer},
  Year                     = {2011},
  Pages                    = {315--327}
}

@Article{Nilsson2013,
  Title                    = {{Hot and cold ion outflow: Observations and implications for numerical models}},
  Author                   = {Nilsson, H. and Barghouthi, I. A. and Slapak, R. and Eriksson, A. I. and Andr??, M.},
  Journal                  = {J. Geophys. Res. Sp. Phys.},
  Year                     = {2013},
  Number                   = {1},
  Volume                   = {118},

  __markedentry            = {[suleimanbaraka:]},
  Doi                      = {10.1029/2012JA017975},
  ISSN                     = {21699402},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Nilsson2013a,
  Title                    = {Hot and cold ion outflow: {Observations} and implications for numerical models},
  Author                   = {Nilsson, H and Barghouthi, IA and Slapak, R and Eriksson, Anders I and André, Mats},
  Journal                  = {Journal of Geophysical Research: Space Physics},
  Year                     = {2013},
  Number                   = {1},
  Pages                    = {105--117},
  Volume                   = {118}
}

@Article{Nilsson2012,
  Title                    = {Hot and cold ion outflow: {Spatial} distribution of ion heating},
  Author                   = {Nilsson, H and Barghouthi, IA and Slapak, R and Eriksson, Anders I and André, Mats},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2012},
  Number                   = {A11},
  Volume                   = {117}
}

@Article{Nilsson2004,
  Title                    = {The structure of high altitude {O}+ energization and outflow: a case study},
  Author                   = {Nilsson, H. and Joko, S. and Lundin, R. and Rème, H. and Sauvaud, J. and Dandouras, I. and Balogh, A. and Carr, C. and Kistler, L. and Klecker, B. and Carlson, C. and Bavassano-Cattaneo, M. and Korth, A.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2004},

  Month                    = jul,
  Pages                    = {2497--2506},
  Volume                   = {22},

  Doi                      = {10.5194/angeo-22-2497-2004}
}

@InProceedings{Nilsson2004a,
  Title                    = {The structure of high altitude {O}+ energization and outflow: a case study},
  Author                   = {Nilsson, H and Joko, S and Lundin, R and Reme, H and Sauvaud, J-A and Dandouras, I and Balogh, A and Carr, C and Kistler, LM and Klecker, B and {others}},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2004},
  Pages                    = {2497--2506},
  Volume                   = {22}
}

@Article{Nilsson2004b,
  Title                    = {The structure of high altitude {O}+ energization and outflow: a case study},
  Author                   = {Nilsson, H. and Joko, S. and Lundin, R. and R√®me, H. and Sauvaud, J. and Dandouras, I. and Balogh, A. and Carr, C. and Kistler, L. and Klecker, B. and Carlson, C. and Bavassano-Cattaneo, M. and Korth, A.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2004},

  Month                    = jul,
  Pages                    = {2497--2506},
  Volume                   = {22},

  Doi                      = {10.5194/angeo-22-2497-2004}
}

@Article{Nilsson,
  Title                    = {{EPSC}},
  Author                   = {Nilsson, H and Slapak, R and Stenberg, G and Yamauchi, M and Barabash, S and Lundin, R}
}

@Article{Nilsson2006,
  Title                    = {Characteristics of high altitude oxygen ion energization and outflow as observed by {Cluster}: a statistical study},
  Author                   = {Nilsson, H. and Waara, M. and Arvelius, S. and Marghitu, O. and Bouhram, M. and Hobara, Y. and Yamauchi, M. and Lundin, R. and Rème, H. and Sauvaud, J.-A. and Dandouras, I. and Balogh, A. and Kistler, L. M. and Klecker, B. and Carlson, C. W. and Bavassano-Cattaneo, M. B. and Korth, A.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2006},

  Month                    = may,
  Pages                    = {1099--1112},
  Volume                   = {24},

  Doi                      = {10.5194/angeo-24-1099-2006}
}

@InProceedings{Nilsson2006a,
  Title                    = {Characteristics of high altitude oxygen ion energization and outflow as observed by {Cluster}: a statistical study},
  Author                   = {Nilsson, H and Waara, Martin and Arvelius, S and Marghitu, O and Bouhram, M and Hobara, Y and Yamauchi, M and Lundin, R and Reme, H and Sauvaud, J-A and {others}},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2006},
  Pages                    = {1099--1112},
  Volume                   = {24}
}

@Article{Nilsson2006b,
  Title                    = {Characteristics of high altitude oxygen ion energization and outflow as observed by {Cluster}: a statistical study},
  Author                   = {Nilsson, H. and Waara, M. and Arvelius, S. and Marghitu, O. and Bouhram, M. and Hobara, Y. and Yamauchi, M. and Lundin, R. and R√®me, H. and Sauvaud, J.-A. and Dandouras, I. and Balogh, A. and Kistler, L. M. and Klecker, B. and Carlson, C. W. and Bavassano-Cattaneo, M. B. and Korth, A.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2006},

  Month                    = may,
  Pages                    = {1099--1112},
  Volume                   = {24},

  Doi                      = {10.5194/angeo-24-1099-2006}
}

@InProceedings{Nilsson2008,
  Title                    = {Transients in oxygen outflow above the polar cap as observed by the {Cluster} spacecraft},
  Author                   = {Nilsson, H and Waara, M and Marghitu, O and Yamauchi, M and Lundin, R and Rème, H and Sauvaud, JA and Dandouras, I and Lucek, E and Kistler, LM and {others}},
  Booktitle                = {Annales geophysicae: atmospheres, hydrospheres and space sciences},
  Year                     = {2008},
  Pages                    = {3365},
  Volume                   = {26}
}

@InProceedings{Nilsson2008a,
  Title                    = {An assessment of the role of the centrifugal acceleration mechanism in high altitude polar cap oxygen ion outflow},
  Author                   = {Nilsson, H and Waara, M and Marghitu, O and Yamauchi, M and Lundin, R and Rème, H and Sauvaud, J-A and Dandouras, I and Lucek, E and Kistler, LM and {others}},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2008},
  Pages                    = {145--157},
  Publisher                = {Copernicus GmbH},
  Volume                   = {26}
}

@Article{Nishikawa1998,
  Title                    = {Reconnections at {Near}-{Earth} {Magnetotail} and {Substorms} {Studied} by a 3-{D} {EM} {Particle} {Code}},
  Author                   = {Nishikawa, K-I},
  Journal                  = {Geospace Mass and Energy Flow},
  Year                     = {1998},
  Pages                    = {175--180}
}

@Article{Nishikawa1998a,
  Title                    = {Particle entry through reconnection grooves in the magnetopause with a dawnward {IMF} as simulated by a 3-{D} {EM} {Particle} {Code}},
  Author                   = {Nishikawa, K.-I.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {1998},
  Pages                    = {1609--1612},
  Volume                   = {25},

  Abstract                 = {We report progress in the long-term effort to represent the interaction of the solar wind with the Earth's magnetosphere using a three-dimensional electromagnetic particle code. After a quasi-steady state is established with an unmagnetized solar wind we gradually switch on a northward interplanetary magnetic field (IMF), which causes a magnetic reconnection on the magnetopause tailward of the dayside cusps and makes the magnetosphere dipolarized. In the case that the northward IMF is switched gradually to dawnward, there is no signature of reconnection in the near-Earth magnetotail in contrast to the case with the southward turning. On the contrary analysis of magnetic fields in the magnetopause confirms a signature of magnetic reconnection at both the dawnside and duskside. The plasma sheet in the near-Earth magnetotail clearly thins as in the case of southward turning. Arrival of dawnward IMF to the magnetopause creates a reconnection groove which causes particle entry into the deep region of the magnetosphere via field lines that go near the magnetopause. This deep connection is more fully recognized tailward of Earth. The flank weak-field region joins onto the plasma sheet and the current sheet to form a geometrical feature called the cross-tail S that structurally integrates the magnetopause and the tail interior. This structure might contribute to direct entry between the magnetosheath plasma to plasma sheet, in which the entry process heats the magnetosheath plasma to plasma sheet temperatures. In spite of strong plasma entry into the inner magnetosphere, the dawnward IMF prevents the reconnection in the near-Earth magnetotail due to the penetrated IMF By component. Therefore, the onset of substorms may not take place. However, it is still possible that this particle entry causes pseudo-substorm onsets.},
  Doi                      = {10.1029/98GL01027},
  Keywords                 = {and boundary layers, cusp, Magnetospheric Physics: Magnetopause, Magnetospheric Physics: Magnetospheric configuration and dynamics, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Storms and substorms}
}

@Article{Nishikawa1998b,
  Title                    = {Particle entry through reconnection grooves in the magnetopause with a dawnward {IMF} as simulated by a 3-{D} {EM} {Particle} {Code}},
  Author                   = {Nishikawa, K-I},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1998},
  Number                   = {10},
  Pages                    = {1609--1612},
  Volume                   = {25}
}

@Article{Nishikawa1997,
  Title                    = {Particle entry into the magnetosphere with a southward interplanetary magnetic field studied by a three-dimensional electromagnetic particle code},
  Author                   = {Nishikawa, K-I},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1997},
  Number                   = {A8},
  Pages                    = {17631--17641},
  Volume                   = {102}
}

@InProceedings{Nishikawa2013,
  Title                    = {Radiation from accelerated particles in relativistic jets with shocks, shear-flow, and reconnection},
  Author                   = {Nishikawa, K.-I. and Hardee, P. and Mizuno, Y. and Duţan, I. and Zhang, B. and Medvedev, M. and Choi, E. J. and Min, K. W. and Niemiec, J. and Nordlund, {\textbackslash}textbackslashAAke},
  Booktitle                = {{EPJ} {Web} of {Conferences}},
  Year                     = {2013},
  Pages                    = {02003},
  Publisher                = {EDP Sciences},
  Volume                   = {61},

  Url                      = {http://www.epj-conferences.org/articles/epjconf/abs/2013/22/epjconf_rj2013_02003/epjconf_rj2013_02003.html},
  Urldate                  = {2014-05-31}
}

@Article{Nishikawa2014,
  Title                    = {Particle {Acceleration} and {Magnetic} {Field} {Generation} in {Shear}-{Flows}},
  Author                   = {Nishikawa, K.-I. and Hardee, P. and Mizuno, Y. and Duţan, I. and Zhang, B. and Medvedev, M. and Meli, A. and Choi, E. J. and Min, K. W. and Niemiec, J. and Nordlund, {\textbackslash}AA. and Frederiksen, J. and Sol, H. and Pohl, M. and Hartmann, D. H. and Marscher, A. and Gómez, J. L.},
  Journal                  = {International Journal of Modern Physics Conference Series},
  Year                     = {2014},

  Month                    = oct,
  Pages                    = {60195},
  Volume                   = {28},

  Doi                      = {10.1142/S2010194514601951},
  Keywords                 = {generation of magnetic field, Generation of magnetic fields, Instability of shear flows, Jets, magnets, Particle-in-cell method, radiation}
}

@Article{Nishikawa2013a,
  Title                    = {Magnetic field generation in a jet-sheath plasma via the kinetic {Kelvin}-{Helmholtz} instability},
  Author                   = {Nishikawa, K.-I. and Hardee, P. and Zhang, B. and Duţan, I. and Medvedev, M. and Choi, E. J. and Min, K. W. and Niemiec, J. and Mizuno, Y. and Nordlund, A. and Frederiksen, J. T. and Sol, H. and Pohl, M. and Hartmann, D. H.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2013},

  Month                    = sep,
  Pages                    = {1535--1541},
  Volume                   = {31},

  Doi                      = {10.5194/angeo-31-1535-2013}
}

@InCollection{Nishikawa1995,
  Title                    = {Solar wind-magnetosphere interaction as simulated by a 3-{D} {EM} particle code},
  Author                   = {Nishikawa, Ken-Ichi and Neubert, Torsten and Buneman, Oscar},
  Booktitle                = {Plasma {Astrophysics} and {Cosmology}},
  Publisher                = {Springer},
  Year                     = {1995},
  Pages                    = {265--276}
}

@Article{Nishikawa2000,
  Title                    = {Evolution of thin current sheet with a southward interplanetary magnetic field studied by a three-dimensional electromagnetic particle code},
  Author                   = {Nishikawa, K-I and Ohtani, S},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2000},
  Number                   = {A6},
  Pages                    = {13017--13028},
  Volume                   = {105}
}

@Article{Nocera2011,
  Title                    = {The particle distributions of asymmetric kinetic electrostatic structures},
  Author                   = {Nocera, L and Palumbo, LJ},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2011},
  Number                   = {3},
  Pages                    = {032114},
  Volume                   = {18}
}

@Article{Normals2000,
  Title                    = {Shock and {Discontinuity} {Normals} , {Mach} {Numbers} , and {Related} {Parameters}},
  Author                   = {Normals, Discontinuity and Parameters, Related},
  Year                     = {2000},
  Pages                    = {249--270},
  Volume                   = {001}
}

@Article{Norqvist1998,
  Title                    = {A statistical study of ion energization mechanisms in the auroral region},
  Author                   = {Norqvist, P. and André, M. and Tyrland, M.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1998},

  Month                    = oct,
  Pages                    = {23459--23474},
  Volume                   = {103},

  Doi                      = {10.1029/98JA02076},
  Keywords                 = {Ionosphere: Particle acceleration, Ionosphere: Wave/particle interactions, Space Plasma Physics: Wave/particle interactions}
}

@Article{Norqvist1998a,
  Title                    = {A statistical study of ion energization mechanisms in the auroral region},
  Author                   = {Norqvist, P. and Andr√©, M. and Tyrland, M.},
  Journal                  = {{\textbackslash}textbackslashjgr},
  Year                     = {1998},

  Month                    = oct,
  Pages                    = {23459--23474},
  Volume                   = {103},

  Doi                      = {10.1029/98JA02076},
  Keywords                 = {Ionosphere: Particle acceleration, Ionosphere: Wave/particle interactions, Space Plasma Physics: Wave/particle interactions}
}

@Article{Nowada2009,
  Title                    = {Alfvénic plasma velocity variations observed at the inner edge of the low-latitude boundary layer induced by the magnetosheath mirror mode waves: {A} {THEMIS} observation},
  Author                   = {Nowada, M. and Shue, J.-H. and Lin, C.-H. and Sakurai, T. and Sibeck, D. G. and Angelopoulos, V. and Carlson, C. W. and Auster, H.-U.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2009},
  Pages                    = {7208},
  Volume                   = {114},

  Abstract                 = {With unique simultaneous observations both in the magnetosheath and magnetosphere by the THEMIS probes, Alfvénic variations in the plasma velocity are observed at the inner edge of low-latitude boundary layer (LLBL) and are induced by the mirror mode waves in the magnetosheath near the subsolar magnetopause on 31 July 2007. These Alfvénic variations appeared as the wavy perturbations in the V{\textless}SUB{\textgreater}x{\textless}/SUB{\textgreater} and V{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater} components observed by THEMIS C, D, and E, which had the same periodicity as associated magnetic field variations. Simultaneously, THEMIS B observed the mirror mode waves in the magnetosheath. The periodicities of the magnetic and plasma pressure variations of mirror modes in the magnetosheath were consistent with those of the Alfvénic wavy variations in the LLBL. Therefore, the mirror mode waves can induce the magnetopause undulations, launching Alfvén waves, and resultant Alfvénic variations are observed in the LLBL. Also, in the succeeding magnetosheath interval by THEMIS B, we examined whether the mirror mode waves occurred and associated Alfvénic variations were observed in the LLBL. However, no clear evidence for an existence of the mirror mode waves was obtained, and THEMIS C, D, and E do not also observe associated magnetic field and plasma Alfvénic responses in the LLBL. These results suggest that the Alfvénic variations in the LLBL are strongly related to the mirror mode waves in the magnetosheath. On the basis of these results, we emphasize that the magnetosheath energy is transmitted and transported into the magnetosphere via magnetopause surface waves.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: MHD waves and instabilities (2149 6050 7836) Magnetospheric Physics: Magnetosphere: inner Magnetospheric Physics: Magnetosphere: outer},
  Url                      = {http://adsabs.harvard.edu/abs/2009JGRA..114.7208N}
}

@Article{Nowlan2011,
  Title                    = {Retrievals of sulfur dioxide from {GOME}-2 using an optimal estimation approach: {Algorithm} and initial validation},
  Author                   = {Nowlan, C. R. and Liu, X. and Chance, K. and Cai, Z. and Kurosu, T. P. and Lee, C. and Martin, R. V.},
  Journal                  = {J. Geophys. Res},
  Year                     = {2011},
  Pages                    = {D18301},
  Volume                   = {116},

  Shorttitle               = {Retrievals of sulfur dioxide from {GOME}-2 using an optimal estimation approach},
  Url                      = {http://www.cfa.harvard.edu/atmosphere/publications/nowlan_gome2_so2_optest_jgr2011_inpress.pdf},
  Urldate                  = {2014-11-13}
}

@Article{Numata2013,
  Title                    = {Electron and ion heating during magnetic reconnection in weakly collisional plasmas},
  Author                   = {Numata, Ryusuke and Loureiro, Nuno F.},
  Journal                  = {arXiv preprint arXiv:1311.2728},
  Year                     = {2013},

  Url                      = {http://arxiv.org/abs/1311.2728},
  Urldate                  = {2014-05-31}
}

@Article{Nykyri2013,
  Title                    = {Impact of {MHD} shock physics on magnetosheath asymmetry and {Kelvin}-{Helmholtz} instability},
  Author                   = {Nykyri, K.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = aug,
  Pages                    = {5068--5081},
  Volume                   = {118},

  Doi                      = {10.1002/jgra.50499},
  Keywords                 = {Kelvin-Helmholtz instability, magnetosheath asymmetry, Parker spiral IMF}
}

@Article{Oganesian2001,
  Title                    = {Second moment of quark structure function of the ρ-meson in {QCD} sum rules},
  Author                   = {Oganesian, A. and Samsonov, A.},
  Journal                  = {Journal of High Energy Physics},
  Year                     = {2001},

  Month                    = sep,
  Pages                    = {2},
  Volume                   = {9},

  Doi                      = {10.1088/1126-6708/2001/09/002}
}

@Article{Ogilvie1984,
  Title                    = {Observations of electron beams in the low-latitude boundary layer},
  Author                   = {Ogilvie, KW and Fitzenreiter, RJ and Scudder, JD},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1984},
  Number                   = {A12},
  Pages                    = {10723--10732},
  Volume                   = {89}
}

@Article{Ogino1994,
  Title                    = {A global magnetohydrodynamic simulation of the response of the magnetosphere to a northward turning of the interplanetary magnetic field},
  Author                   = {Ogino, Tatsuki and Walker, Raymond J and Ashour-Abdalla, Maha},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1994},
  Number                   = {A6},
  Pages                    = {11027--11042},
  Volume                   = {99},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/93JA03313/full}
}

@Article{Ohira2013,
  Title                    = {{Simulations of Collisionless Perpendicular Shocks in Partially Ionized Plasmas}},
  Author                   = {Ohira, Yutaka},
  Year                     = {2013},

  Month                    = {may},
  Pages                    = {4},

  __markedentry            = {[suleimanbaraka:6]},
  Abstract                 = {Perpendicular collisionless shocks propagating into partially ionized plasmas are investigated by two-dimensional hybrid particle simulations. It is shown that some neutral particles leak into the upstream region from the downstream region, the leaking neutral particles become pickup ions in the upstream region and modify the shock structure, the pickup ions are preferentially accelerated, and plasma instabilities are excited by the pickup ions in the upstream and downstream regions.},
  Archiveprefix            = {arXiv},
  Arxivid                  = {1305.6696},
  Eprint                   = {1305.6696},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Ohira/Unknown/Ohira - 2013 - Simulations of Collisionless Perpendicular Shocks in Partially Ionized Plasmas.pdf:pdf},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23},
  Url                      = {http://arxiv.org/abs/1305.6696}
}

@Article{Omidi2005,
  Title                    = {Macrostructure of collisionless bow shocks: 1. {Scale} lengths},
  Author                   = {Omidi, N and Blanco-Cano, X and Russell, CT},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2005},
  Number                   = {A12},
  Volume                   = {110}
}

@Article{Omidi2002,
  Title                    = {Hybrid simulations of solar wind interaction with magnetized asteroids: {General} characteristics},
  Author                   = {Omidi, N and Blanco-Cano, X and Russell, CT and Karimabadi, H and Acuna, M},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2002},
  Number                   = {A12},
  Pages                    = {SSH--12},
  Volume                   = {107}
}

@Article{Omidi2010,
  Title                    = {Foreshock bubbles and their global magnetospheric impacts},
  Author                   = {Omidi, N. and Eastwood, J. P. and Sibeck, D. G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2010},
  Pages                    = {6204},
  Volume                   = {115},

  Abstract                 = {We employ 2.5-D electromagnetic, hybrid simulations that treat ions kinetically via particle-in-cell methods and electrons as a massless fluid to study the formation and properties of a new structure named the foreshock bubble upstream from the bow shock. This structure forms due to changes in the interplanetary magnetic field (IMF) associated with solar wind discontinuities and their interaction with the backstreaming ions in the foreshock prior to these discontinuities encountering the bow shock. The leading edge of the foreshock bubble consists of a fast magnetosonic shock and the compressed and heated plasma downstream of the shock. The leading edge surrounds the core which consists of a less-dense and hotter plasma and lower magnetic field strength. Ultra low frequency turbulence is present in both the outer and core regions of the foreshock bubbles. The size of the foreshock bubble transverse to the flow direction scales with the width of the ion foreshock and at Earth corresponds to tens of R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}. The size along the flow depends on the age of the bubble and grows with time. Although they expand sunward, foreshock bubbles are carried antisunward by the solar wind, and for small IMF cone angles (angle between IMF and solar wind flow) when the foreshock lies upstream of the dayside magnetosphere they collide with the bow shock. This collision is shown to have significant magnetospheric impacts. Upon encountering the bow shock, the low pressures within the core of the bubble result in the reversal of the magnetosheath flow from antisunward to sunward direction. This in turn results in the outward motion of the magnetopause and expansion of the dayside magnetosphere. The interaction is found to noticeably impact the density and energy of trapped radiation belt ions and plasma injection into the cusp. Foreshock bubbles are found to be highly effective sites for ion reflection and acceleration to high energies via first- and second-order Fermi acceleration. The interaction of the foreshock bubble with the bow shock results in the release of energetic ions into the magnetosheath. Some of these ions are subsequently injected into the cusp.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Planetary bow shocks Magnetospheric Physics: Solar wind/magnetosphere interactions Interplanetary Physics: Discontinuities (7811) Interplanetary Physics: Energetic particles (7514) Interplanetary Physics: Plasma waves and turbulence},
  Url                      = {http://adsabs.harvard.edu/abs/2010JGRA..115.6204O}
}

@Article{Omidi2009,
  Title                    = {Hybrid simulations of magnetic reconnection initiated in the magnetosheath},
  Author                   = {Omidi, N. and Phan, T. and Sibeck, D. G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2009},
  Pages                    = {2222},
  Volume                   = {114},

  Abstract                 = {Interaction of solar wind tangential discontinuities (TDs) with the bow shock may initiate reconnection in the magnetosheath. We employ 2.5-D electromagnetic, hybrid simulations that treat the ions kinetically via particle-in-cell methods and the electrons as a massless fluid to study this interaction. We present results from eight runs corresponding to TD thicknesses ranging from 10 to 260 ion skin depths and shear angles ranging from 120° to 180°. Our results indicate a transition from time-dependent to steady state reconnection as the thickness of the solar wind TD increases above 30 ion skin depths. As the shear angle in the magnetic field decreases, it takes longer to initiate reconnection, and reconnection jet speeds diminish, suggesting a lower reconnection rate. Implications of these results for magnetic reconnection at currents sheets in general and at the magnetopause in particular are also discussed.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Magnetosheath Interplanetary Physics: Planetary bow shocks Magnetospheric Physics: Numerical modeling Space Plasma Physics: Shock waves (4455)},
  Url                      = {http://adsabs.harvard.edu/abs/2009JGRA..114.2222O}
}

@InProceedings{Omidi2005a,
  Title                    = {Stability of the {Bow} shock and {Formation} of {Hot} {Flow} {Anomalies}},
  Author                   = {Omidi, N and Sibeck, DG},
  Booktitle                = {{AGU} {Spring} {Meeting} {Abstracts}},
  Year                     = {2005},
  Pages                    = {01},
  Volume                   = {1}
}

@Article{Omidi2013,
  Title                    = {Dynamics of the foreshock compressional boundary and its connection to foreshock cavities},
  Author                   = {Omidi, N. and Sibeck, D. and Blanco-Cano, X. and Rojas-Castillo, D. and Turner, D. and Zhang, H. and Kajdič, P.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},
  Pages                    = {823--831},
  Volume                   = {118},

  Abstract                 = {We use several global hybrid (kinetic ions, fluid electrons) simulation runs for steady and time-varying interplanetary magnetic field (IMF) conditions to examine the dynamics of the foreshock compressional boundary (FCB) and its connection to foreshock cavities. The results demonstrate that for steady IMF conditions, the FCB forms and evolves over a long period of time due to the dynamics of the bow shock and ion foreshock. Formation of the FCB is tied to the generation and nonlinear evolution of ULF waves associated with large-amplitude fluctuations in magnetic field and density within the foreshock. As a result, even during steady IMF conditions, the transitions in the magnetic field strength and direction across an FCB evolve. Although the FCB itself is associated with increases in the magnetic field strength and density, these quantities are reduced on the turbulent side of the FCB as compared to the pristine solar wind. Hybrid simulations with time-varying IMF have been performed to examine the relationship between the FCB and foreshock cavities generated under two possible scenarios. In the first scenario, a bundle of field lines connects to an otherwise quasi-perpendicular bow shock and results in the formation of a finite-sized foreshock region that travels with this bundle of field lines as it connects to different parts of the bow shock surface. Two FCBs bound the traveling foreshock region. In the second scenario, solar wind discontinuities cause the IMF cone angle (angle between the IMF and the solar wind flow direction) to vary and thereby modify the foreshock geometry and the position of the FCB. We demonstrate that structures similar to foreshock cavities bounded by FCBs form in both scenarios. We show that the two scenarios cannot be distinguished based on convecting or nonconvecting FCBs. We also demonstrate that depending on spacecraft location and the nature of the solar wind discontinuities, foreshock cavities may be bounded by an FCB on one side and a foreshock bubble on the other.},
  ISSN                     = {0148-0227},
  Keywords                 = {foreshock boundaries foreshock cavities bow shock foreshock bubbles magnetosheath},
  Url                      = {http://adsabs.harvard.edu/abs/2013JGRA..118..823O}
}

@Article{Omidi2014,
  Title                    = {Magnetosheath filamentary structures formed by ion acceleration at the quasi-parallel bow shock},
  Author                   = {Omidi, N. and Sibeck, D. and Gutynska, O. and Trattner, K. J.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2014},
  Pages                    = {2593--2604},
  Volume                   = {119},

  Abstract                 = {Results from 2.5-D electromagnetic hybrid simulations show the formation of field-aligned, filamentary plasma structures in the magnetosheath. They begin at the quasi-parallel bow shock and extend far into the magnetosheath. These structures exhibit anticorrelated, spatial oscillations in plasma density and ion temperature. Closer to the bow shock, magnetic field variations associated with density and temperature oscillations may also be present. Magnetosheath filamentary structures (MFS) form primarily in the quasi-parallel sheath; however, they may extend to the quasi-perpendicular magnetosheath. They occur over a wide range of solar wind Alfvénic Mach numbers and interplanetary magnetic field directions. At lower Mach numbers with lower levels of magnetosheath turbulence, MFS remain highly coherent over large distances. At higher Mach numbers, magnetosheath turbulence decreases the level of coherence. Magnetosheath filamentary structures result from localized ion acceleration at the quasi-parallel bow shock and the injection of energetic ions into the magnetosheath. The localized nature of ion acceleration is tied to the generation of fast magnetosonic waves at and upstream of the quasi-parallel shock. The increased pressure in flux tubes containing the shock accelerated ions results in the depletion of the thermal plasma in these flux tubes and the enhancement of density in flux tubes void of energetic ions. This results in the observed anticorrelation between ion temperature and plasma density.},
  ISSN                     = {0148-0227},
  Keywords                 = {magnetosheath ion acceleration density structures temperature structures Temperature Structures},
  Url                      = {http://adsabs.harvard.edu/abs/2014JGRA..119.2593O}
}

@Article{Omidi2007,
  Title                    = {Formation of hot flow anomalies and solitary shocks},
  Author                   = {Omidi, N. and Sibeck, D. G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2007},
  Pages                    = {1203},
  Volume                   = {112},

  Abstract                 = {Interaction of a tangential discontinuity (TD) with the bow shock is investigated by using electromagnetic, global hybrid simulations in which ions are treated kinetically via particle-in-cell methods and electrons form a massless fluid. On the basis of previous studies, it was expected that the interaction would result in the formation of a hot flow anomaly (HFA) propagating along the curved bow shock surface. The results are unexpected in two major ways. First, the hot flow anomaly is only formed during the interaction of the TD with the quasi-parallel side of the bow shock. The lack of a HFA on the perpendicular side is due to the inability of a large fraction of ions to escape into the solar wind, as is required for an HFA to form. Second, the interaction of the TD with the quasi-perpendicular portion of the bow shock results in a previously unknown, shock structure which we name the "solitary shock." The solitary shock consists of a finite width (a few ion inertial length), fast magnetosonic shock-like structure followed by a relatively less compressed, more turbulent plasma with complex and spatially varying properties in the downstream region. We have determined that the formation of the solitary shock after the passage of the TD is due to the new direction of the interplanetary magnetic field. Further, this is not a transitory phenomena and when the interplanetary magnetic field cone angle is large (˜{\textgreater}50°) a significant portion of the bow shock surface is affected. Solitary shocks form in the regions where the motional electric field in the magnetosheath points away from the shock. We demonstrate that solitary shocks differ from regular quasi-perpendicular shocks due to differences in ion dissipation processes. We also present the results of a detailed survey of the effects of simulation parameters such as cell size, resistivity, system size, and 2.5-dimensional versus three-dimensional domains on the solitary shock solutions.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Planetary bow shocks Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Numerical modeling Interplanetary Physics: Discontinuities (7811) bow shock hot flow anomalies ion dissipation quasi-perpendicular shocks shock interaction with discontinuities solitary shocks},
  Url                      = {http://adsabs.harvard.edu/abs/2007JGRA..112.1203O}
}

@Article{Omidi2007a,
  Title                    = {Flux transfer events in the cusp},
  Author                   = {Omidi, N. and Sibeck, D. G.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2007},
  Pages                    = {4106},
  Volume                   = {34},

  Abstract                 = {We use 2.5-dimensional global hybrid (kinetic ions, fluid electrons) simulations to study the evolution of Flux Transfer Events (FTEs) and their interaction with the cusp during their poleward motion. A southward pointing interplanetary magnetic field is considered. It results in low-latitude, time-dependent reconnection and the formation of multiple FTEs with a variety of sizes ranging from a few hundred to thousands of km. FTEs are found to travel along the magnetopause surface with velocities exceeding the surrounding magnetosheath by 1 local Alfven speed. As a result, a slow mode bow wave and a pile up of plasma and magnetic field precede larger, but not smaller, FTEs. As an FTE encounters the cusp, a secondary magnetic reconnection is initiated which ultimately leads to its disintegration as it moves to higher latitudes. Both the slow mode bow wave and reconnection accelerate plasma into the cusp and enhance the flux of energetic ions in this region. The downward flux of ions at a given energy moves poleward in time, exhibiting characteristics similar to the poleward moving auroral forms previously attributed to FTEs.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Magnetosphere/ionosphere interactions (2431) Magnetospheric Physics: Cusp Magnetospheric Physics: Numerical modeling},
  Url                      = {http://adsabs.harvard.edu/abs/2007GeoRL..34.4106O}
}

@Article{Omidi2009a,
  Title                    = {Foreshock compressional boundary},
  Author                   = {Omidi, N. and Sibeck, D. G. and Blanco-Cano, X.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2009},
  Pages                    = {8205},
  Volume                   = {114},

  Abstract                 = {We employ 2.5-D electromagnetic, hybrid simulations that treat ions kinetically via particle-in-cell methods and electrons as a massless fluid to study the formation and properties of a newly discovered boundary named the foreshock compressional boundary (FCB). This boundary forms in the ion foreshock and is associated with enhanced densities and magnetic field strengths. At times, but not always, the FCB separates the pristine solar wind plasma from the ion foreshock. In this study, we investigate the dependence of FCB characteristics on solar wind Mach number and cone angle (the angle between flow velocity and interplanetary magnetic field). We show that the strength of the foreshock compressional boundary increases with the Mach number. This enhancement is in turn tied to the density and velocity of the backstreaming ions in the foreshock whose interaction with the solar wind results in ULF turbulence which is ultimately responsible for the formation of FCB. During small cone angles the foreshock compressional boundary is symmetric with respect to the radial direction. As the cone angle increases, the FCB becomes less symmetric and eventually is confined to one side of the foreshock. The strength of the FCB also decreases with increasing cone angle but depending on the Mach number can exist for cone angles of 40° and beyond. A recent study that compared data from a global hybrid simulation of the foreshock with Cluster spacecraft observations showed that encounters with foreshock cavities can be interpreted as back and forth motion of a FCB causing spacecraft to move from the solar wind through the FCB into the foreshock and back into solar wind. An example of a FCB observed by the Cluster spacecraft is presented and shown to be in general agreement with model predictions.},
  ISSN                     = {0148-0227},
  Keywords                 = {Geochemistry: Composition of the moon Geochemistry: Composition of the moon Geochemistry: Composition of the moon Geochemistry: Composition of the moon (7811) Geochemistry: Composition of the moon},
  Url                      = {http://adsabs.harvard.edu/abs/2009JGRA..114.8205O}
}

@Article{Omidi2011,
  Title                    = {Hybrid simulations of {EMIC} waves in a dipolar magnetic field},
  Author                   = {Omidi, N. and Thorne, R. and Bortnik, J.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2011},

  Month                    = sep,
  Pages                    = {9231},
  Volume                   = {116},

  Doi                      = {10.1029/2011JA016511},
  Keywords                 = {Magnetospheric Physics: Energetic particles: precipitating, Magnetospheric Physics: Energetic particles: trapped, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Plasma waves and instabilities (2471)}
}

@Article{Omidi1988,
  Title                    = {Subcritcal dispersive shock waves upstream of planetary bow shocks and at comet {Giacobini}-{Zinner}},
  Author                   = {Omidi, N and Winske, D},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1988},
  Number                   = {11},
  Pages                    = {1303--1306},
  Volume                   = {15}
}

@Article{Omidi2014a,
  Title                    = {Parametric dependencies of spontaneous hot flow anomalies},
  Author                   = {Omidi, N. and Zhang, H. and Chu, C. and Sibeck, D. and Turner, D.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2014},
  Pages                    = {9823--9833},
  Volume                   = {119},

  Abstract                 = {Parametric dependencies of spontaneous hot flow anomalies at the quasi-parallel bow shock are investigated using global hybrid (kinetic ions and fluid electron) simulations with a variety of solar wind Mach numbers and directions of the interplanetary magnetic field (IMF). Simulations with solar wind Alfvénic Mach number of 3 and small IMF cone angles (with the flow velocity) show sporadic formation of spontaneous hot flow anomalies (SHFAs). Increasing the Mach number shows the formation of copious number of SHFAs whose properties are examined in this study. It is shown that the duration of SHFAs does not show much variation with Mach number indicating that their size generally increases with Mach number. Additionally, the level of solar wind deceleration associated with SHFAs increases with Mach number as does the core ion temperature. It is also found that the edges of SHFAs are associated with jumps in magnetic field that increase with shock Mach number. The results also show that the rate of SHFA formation increases with increasing Mach number. Simulations with IMF cone angle of 90° show that SHFAs form at the quasi-parallel bow shock provided the shock Alfvén Mach number is {\textgreater}3. This shows that SHFAs may form at all cone angles.},
  ISSN                     = {0148-0227},
  Keywords                 = {quasi-parallel bow shock ion heating ion foreshock nonlinear structures},
  Url                      = {http://adsabs.harvard.edu/abs/2014JGRA..119.9823O}
}

@Article{Omidi2013a,
  Title                    = {Spontaneous hot flow anomalies at quasi-parallel shocks: 2. {Hybrid} simulations},
  Author                   = {Omidi, N. and Zhang, H. and Sibeck, D. and Turner, D.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},
  Pages                    = {173--180},
  Volume                   = {118},

  Abstract                 = {{\textless}title type="main"{\textgreater}Abstract{\textless}p label="1"{\textgreater}Motivated by recent THEMIS observations, this paper uses 2.5-D electromagnetic hybrid simulations to investigate the formation of Spontaneous Hot Flow Anomalies (SHFAs) upstream of quasi-parallel bow shocks during steady solar wind conditions and in the absence of discontinuities. The results show the formation of a large number of structures along and upstream of the quasi-parallel bow shock. Their outer edges exhibit density and magnetic field enhancements, while their cores exhibit drops in density, magnetic field, solar wind velocity, and enhancements in ion temperature. Using virtual spacecraft in the simulation, we show that the signatures of these structures in the time series data are very similar to those of SHFAs seen in THEMIS data and conclude that they correspond to SHFAs. Examination of the simulation data shows that SHFAs form as the result of foreshock cavitons interacting with the bow shock. Foreshock cavitons in turn form due to the nonlinear evolution of ULF waves generated by the interaction of the solar wind with the backstreaming ions. Because foreshock cavitons are an inherent part of the shock dissipation process, the formation of SHFAs is also an inherent part of the dissipation process leading to a highly nonuniform plasma in the quasi-parallel magnetosheath including large-scale density and magnetic field cavities.},
  ISSN                     = {0148-0227},
  Keywords                 = {Bow shock Foreshock Cavitons},
  Url                      = {http://adsabs.harvard.edu/abs/2013JGRA..118..173O}
}

@Article{Omura2011,
  Title                    = {Triggering process of whistler mode chorus emissions in the magnetosphere},
  Author                   = {Omura, Y and Nunn, D},
  Journal                  = {J. Geophys. Res},
  Year                     = {2011},
  Pages                    = {A05205},
  Volume                   = {116}
}

@Article{Onsager2001,
  Title                    = {Reconnection at the high-latitude magnetopause during northward interplanetary magnetic field conditions},
  Author                   = {Onsager, TG and Scudder, JD and Lockwood, M and Russell, CT},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2001},
  Number                   = {A11},
  Pages                    = {25--467},
  Volume                   = {106}
}

@Article{Oran2013,
  Title                    = {A {Global} {Wave}-driven {Magnetohydrodynamic} {Solar} {Model} with a {Unified} {Treatment} of {Open} and {Closed} {Magnetic} {Field} {Topologies}},
  Author                   = {Oran, R. and van der Holst, B. and Landi, E. and Jin, M. and Sokolov, I. V. and Gombosi, T. I.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2013},

  Month                    = dec,
  Pages                    = {176},
  Volume                   = {778},

  Doi                      = {10.1088/0004-637X/778/2/176},
  Keywords                 = {Magnetohydrodynamics: MHD, methods: numerical, Solar Wind, Sun: corona, turbulence}
}

@Article{Osmane2014,
  Title                    = {Relativistic surfatron process for {Landau} resonant electrons in radiation belts},
  Author                   = {Osmane, A. and Hamza, A. M.},
  Journal                  = {Nonlinear Processes in Geophysics},
  Year                     = {2014},

  Month                    = jan,
  Pages                    = {115--125},
  Volume                   = {21},

  Doi                      = {10.5194/npg-21-115-2014}
}

@Article{Ottaviani1999,
  Title                    = {The gyro-radius scaling of ion thermal transport from global numerical simulations of ion temperature gradient driven turbulence},
  Author                   = {Ottaviani, M. and Manfredi, G.},
  Journal                  = {Phys. Plasmas},
  Year                     = {1999},

  Month                    = aug,
  Pages                    = {3267--3275},
  Volume                   = {6},

  Doi                      = {10.1063/1.873567},
  Keywords                 = {plasma simulation, Plasma Turbulence, Stellarators torsatrons heliacs bumpy tori and other toroidal confinement devices, Thermodynamics of plasmas, Tokamaks spherical tokamaks, Transport Properties}
}

@Article{Owen2012,
  Title                    = {{IMPALAS}: {Investigation} of {MagnetoPause} {Activity} using {Longitudinally}-{Aligned} {Satellites}—a mission concept proposed for the {ESA} {M}3 2020/2022 launch},
  Author                   = {Owen, Christopher J. and Amm, Olaf and Bruno, Roberto and Keyser, Johan De and Dunlop, Malcolm W. and Eastwood, Jonathan P. and Fazakerley, Andrew N. and Fontaine, Dominique and Forsyth, Colin and Hasegawa, Hiroshi and Hellinger, Petr and Hercik, David and Jacquey, Christian and Milan, Steven and Raeder, Joachim and Sibeck, David G. and Stverak, Stepan and Travnicek, Pavel and Walsh, Andrew P. and Wild, James A.},
  Journal                  = {Experimental Astronomy},
  Year                     = {2012},
  Pages                    = {365--401},
  Volume                   = {33},

  Abstract                 = {The dayside magnetopause is the primary site of energy transfer from the solar wind into the magnetosphere, and modulates the activity observed within the magnetosphere itself. Specific plasma processes operating on the magnetopause include magnetic reconnection, generation of boundary waves, propagation of pressure-pulse induced deformations of the boundary, formation of boundary layers and generation of Alfvén waves and field-aligned current systems connecting the boundary to the inner magnetosphere and ionosphere. However, many of the details of these processes are not fully understood. For example, magnetic reconnection occurs sporadically, producing flux transfer events, but how and where these arise, and their importance to the global dynamics of the magnetospheric system remain unresolved. Many of these phenomena involve propagation across the magnetopause surface. Measurements at widely-spaced (Δ ˜ 5 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}) intervals along the direction of dayside terrestrial field lines at the magnetopause would be decisive in resolving these issues. We describe a mission carrying a fields and plasmas payload (including magnetometer, ion and electron spectrometer and energetic particle telescopes) on three identical spacecraft in synchronized orbits. These provide the needed separations, with each spacecraft skimming the dayside magnetopause and continuously sampling this boundary for many hours. The orbits are phased such that (i) all three spacecraft maintain common longitude and thus sample along the same magnetopause field line; (ii) the three spacecraft reach local midday when northern European ground-based facilities also lie near local midday, enabling simultaneous sampling of magnetopause field lines and their footprints.},
  ISSN                     = {0922-6435},
  Keywords                 = {Magnetopause Magnetic reconnection Solar wind-magnetosphere coupling Cosmic vision},
  Url                      = {http://adsabs.harvard.edu/abs/2012ExA....33..365O}
}

@Article{Owens2012,
  Title                    = {Implications of {Non}-cylindrical {Flux} {Ropes} for {Magnetic} {Cloud} {Reconstruction} {Techniques} and the {Interpretation} of {Double} {Flux} {Rope} {Events}},
  Author                   = {Owens, M. J. and Démoulin, P. and Savani, N. P. and Lavraud, B. and Ruffenach, A.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {2012},

  Month                    = jun,
  Pages                    = {435--446},
  Volume                   = {278},

  Doi                      = {10.1007/s11207-012-9939-2},
  Keywords                 = {Coronal Mass Ejection, magnetic cloud, Magnetic flux rope, Solar Wind}
}

@Article{Pallocchia2010,
  Title                    = {Interplanetary shock transmitted into the {Earth}'s magnetosheath: {Cluster} and {Double} {Star} observations},
  Author                   = {Pallocchia, G. and Samsonov, A. A. and Bavassano Cattaneo, M. B. and Marcucci, M. F. and Rème, H. and Carr, C. M. and Cao, J. B.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2010},

  Month                    = may,
  Pages                    = {1141--1156},
  Volume                   = {28},

  Doi                      = {10.5194/angeo-28-1141-2010}
}

@Article{Palmer2003,
  Title                    = {Mapping isoprene emissions over {North} {America} using formaldehyde column observations from space},
  Author                   = {Palmer, Paul I. and Jacob, Daniel J. and Fiore, Arlene M. and Martin, Randall V. and Chance, Kelly and Kurosu, Thomas P.},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2003},
  Number                   = {D6},
  Volume                   = {108},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2002JD002153/full},
  Urldate                  = {2014-11-13}
}

@InProceedings{Palmroth2005,
  Title                    = {Assessment of ionospheric {Joule} heating by {GUMICS}-4 {MHD} simulation, {AMIE}, and satellite-based statistics: towards a synthesis},
  Author                   = {Palmroth, M and Janhunen, P and Pulkkinen, TI and Aksnes, A and Lu, G and Østgaard, N and Watermann, J and Reeves, GD and Germany, GA},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2005},
  Pages                    = {2051--2068},
  Publisher                = {Copernicus GmbH},
  Volume                   = {23}
}

@Article{Palmroth2002,
  Title                    = {Stormtime energy transfer in global {MHD} simulation},
  Author                   = {Palmroth, M and Pulkkinen, TI and Janhunen, P and Wu, C-C},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2002},
  Number                   = {A1},
  Pages                    = {SMP24--1},
  Volume                   = {108}
}

@Article{Park2013,
  Title                    = {Particle-in-cell {Simulations} of {Particle} {Energization} via {Shock} {Drift} {Acceleration} from {Low} {Mach} {Number} {Quasi}-perpendicular {Shocks} in {Solar} {Flares}},
  Author                   = {Park, J. and Ren, C. and Workman, J. C. and Blackman, E. G.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2013},

  Month                    = mar,
  Pages                    = {147},
  Volume                   = {765},

  Doi                      = {10.1088/0004-637X/765/2/147},
  Keywords                 = {acceleration of particles, instabilities, methods: numerical, plasmas, shock waves, Sun: flares}
}

@Article{Park2013a,
  Title                    = {Particle-in-cell simulations of particle energization via shock drift acceleration from low {Mach} number quasi-perpendicular shocks in solar flares},
  Author                   = {Park, Jaehong and Ren, Chuang and Workman, Jared C and Blackman, Eric G},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2013},
  Number                   = {2},
  Pages                    = {147},
  Volume                   = {765}
}

@Article{Park2012,
  Title                    = {{Particle-in-cell simulations of particle energization from low Mach number fast mode shocks}},
  Author                   = {Park, Jaehong and Workman, Jared C. and Blackman, Eric G. and Ren, Chuang and Siller, Robert},
  Journal                  = {Phys. Plasmas},
  Year                     = {2012},
  Number                   = {6},
  Pages                    = {062904},
  Volume                   = {19},

  __markedentry            = {[suleimanbaraka:6]},
  Doi                      = {10.1063/1.4729913},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Park et al/Physics of Plasmas/Park et al. - 2012 - Particle-in-cell simulations of particle energization from low Mach number fast mode shocks(2).pdf:pdf},
  ISSN                     = {1070664X},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23},
  Url                      = {http://scitation.aip.org/content/aip/journal/pop/19/6/10.1063/1.4729913}
}

@Article{Parker1965,
  Title                    = {Dynamical theory of the solar wind},
  Author                   = {Parker, EN},
  Journal                  = {Space Science Reviews},
  Year                     = {1965},
  Number                   = {5-6},
  Pages                    = {666--708},
  Volume                   = {4}
}

@Article{Parker1959,
  Title                    = {Extension of the {Solar} {Corona} into {Interplanetary} {Space}},
  Author                   = {Parker, Eugene},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1959},

  Month                    = nov,
  Pages                    = {1675--1681},
  Volume                   = {64}
}

@Book{Parker1963,
  Title                    = {Interplanetary dynamical processes},
  Author                   = {Parker, Eugene Newman},
  Publisher                = {Wiley New York},
  Year                     = {1963}
}

@Article{Parker1958,
  Title                    = {Dynamics of the {Interplanetary} {Gas} and {Magnetic} {Fields}.},
  Author                   = {Parker, Eugene N.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {1958},

  Month                    = nov,
  Pages                    = {664--676},
  Volume                   = {128}
}

@Book{Parker1979,
  Title                    = {Solar system plasma physics},
  Author                   = {Parker, Eugene Newman and Kennel, Charles F and Lanzerotti, Louis J},
  Publisher                = {North-Holland Pub. Co.},
  Year                     = {1979},
  Volume                   = {3}
}

@Article{Parks2004,
  Title                    = {Why space physics needs to go beyond the {MHD} box},
  Author                   = {Parks, George K},
  Journal                  = {Space science reviews},
  Year                     = {2004},
  Number                   = {1-2},
  Pages                    = {97--121},
  Volume                   = {113}
}

@Article{Parks1991,
  Title                    = {Physics of space plasmas-an introduction},
  Author                   = {Parks, George K},
  Journal                  = {Redwood City, CA, Addison-Wesley Publishing Co., 1991, 547 p.},
  Year                     = {1991},
  Volume                   = {1}
}

@Article{Paschmann1986,
  Title                    = {The magnetopause for large magnetic shear: {AMPTE}/{IRM} observations},
  Author                   = {Paschmann, G and Papamastorakis, I and Baumjohann, W and Sckopke, N and Carlson, CW and Sonnerup, BU and Lühr, H},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1986},
  Number                   = {A10},
  Pages                    = {11099--11115},
  Volume                   = {91}
}

@Book{Paschmann2005,
  Title                    = {Outer magnetospheric boundaries: {Cluster} results},
  Author                   = {Paschmann, Götz and Schwartz, SJ and Escoubet, CP and Haaland, S},
  Publisher                = {Springer},
  Year                     = {2005},
  Number                   = {1-4}
}

@Article{Paschmann1981,
  Title                    = {Characteristics of reflected and diffuse ions upstream from the earth's bow shock},
  Author                   = {Paschmann, G and Sckopke, N and Papamastorakis, I and Asbridge, JR and Bame, SJ and Gosling, JT},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1981},
  Number                   = {A6},
  Pages                    = {4355--4364},
  Volume                   = {86}
}

@Article{Paschmann2013,
  Title                    = {In-{Situ} {Observations} of {Reconnection} in {Space}},
  Author                   = {Paschmann, Götz and Ø ieroset, Marit and Phan, Tai},
  Journal                  = {Space Sci. Rev.},
  Year                     = {2013},

  Month                    = feb,
  Number                   = {2-4},
  Pages                    = {385--417},
  Volume                   = {178},

  Doi                      = {10.1007/s11214-012-9957-2},
  ISSN                     = {0038-6308},
  Keywords                 = {current sheets, diffusion region, Magnetic reconnection, magnetosphere},
  Url                      = {http://link.springer.com/10.1007/s11214-012-9957-2}
}

@Article{Pedersen2008,
  Title                    = {Electron density estimations derived from spacecraft potential measurements on {Cluster} in tenuous plasma regions},
  Author                   = {Pedersen, A. and Lybekk, B. and André, M. and Eriksson, A. and Masson, A. and Mozer, F. S. and Lindqvist, P.-A. and DéCréAu, P. M. E. and Dandouras, I. and Sauvaud, J.-A. and Fazakerley, A. and Taylor, M. and Paschmann, G. and Svenes, K. R. and Torkar, K. and Whipple, E.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2008},

  Month                    = jul,
  Pages                    = {7},
  Volume                   = {113},

  Doi                      = {10.1029/2007JA012636},
  Keywords                 = {charging, instruments and techniques, magnetospheric physics, Magnetospheric Physics: Instruments and techniques, Magnetospheric Physics: Magnetosphere: outer, Magnetospheric Physics: Magnetotail, Magnetospheric Physics: Magnetotail boundary layers, magnetotail, spacecraft sheaths, wakes}
}

@Article{Pedersen2008a,
  Title                    = {Electron density estimations derived from spacecraft potential measurements on {Cluster} in tenuous plasma regions},
  Author                   = {Pedersen, A. and Lybekk, B. and Andr√©, M. and Eriksson, A. and Masson, A. and Mozer, F. S. and Lindqvist, P.-A. and D√©Cr√©Au, P. M. E. and Dandouras, I. and Sauvaud, J.-A. and Fazakerley, A. and Taylor, M. and Paschmann, G. and Svenes, K. R. and Torkar, K. and Whipple, E.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2008},

  Month                    = jul,
  Pages                    = {7},
  Volume                   = {113},

  Doi                      = {10.1029/2007JA012636},
  Keywords                 = {charging, instruments and techniques, magnetospheric physics, Magnetospheric Physics: Instruments and techniques, Magnetospheric Physics: Magnetosphere: outer, Magnetospheric Physics: Magnetotail, Magnetospheric Physics: Magnetotail boundary layers, magnetotail, spacecraft sheaths, wakes}
}

@Article{Peredo1995,
  Title                    = {Three-dimensional position and shape of the bow shock and their variation with {Alfvenic}, sonic and magnetosonic {Mach} numbers and interplanetary magnetic field orientation},
  Author                   = {Peredo, M and Slavin, JA and Mazur, E and Curtis, SA},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1995},
  Number                   = {A5},
  Pages                    = {7907--7916},
  Volume                   = {100}
}

@Article{Perrone2013,
  Title                    = {Nonclassical {Transport} and {Particle}-{Field} {Coupling}: from {Laboratory} {Plasmas} to the {Solar} {Wind}},
  Author                   = {Perrone, D. and Dendy, R. O. and Furno, I. and Sanchez, R. and Zimbardo, G. and Bovet, a. and Fasoli, a. and Gustafson, K. and Perri, S. and Ricci, P. and Valentini, F.},
  Journal                  = {Space Sci. Rev.},
  Year                     = {2013},

  Month                    = mar,
  Number                   = {2-4},
  Pages                    = {233--270},
  Volume                   = {178},

  Doi                      = {10.1007/s11214-013-9966-9},
  ISSN                     = {0038-6308},
  Url                      = {http://link.springer.com/10.1007/s11214-013-9966-9}
}

@Article{Peterson2012,
  Title                    = {Sources of plasma in the high altitude cusp},
  Author                   = {Peterson, WK and Trattner, KJ},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2012},
  Pages                    = {1--10},
  Volume                   = {87}
}

@Article{Petri2007,
  Title                    = {{Magnetic reconnection at the termination shock in a striped pulsar wind}},
  Author                   = {Petri, Jerome and Lyubarsky, Yuri},
  Year                     = {2007},

  Month                    = {jul},
  Pages                    = {1961--1967},

  __markedentry            = {[suleimanbaraka:6]},
  Abstract                 = {Most of the rotational luminosity of a pulsar is carried away by a relativistic magnetised wind in which the matter energy flux is negligible compared to the Poynting flux. Near the equatorial plane of an obliquely rotating pulsar magnetosphere, the magnetic field reverses polarity with the pulsar period, forming a wind with oppositely directed field lines. This structure is called a striped wind; dissipation of alternating fields in the striped wind is the object of our study. The aim of this paper is to study the conditions required for magnetic energy release at the termination shock of the striped pulsar wind. Magnetic reconnection is considered via analytical methods and 1D relativistic PIC simulations. An analytical condition on the upstream parameters for partial and full magnetic reconnection is derived from the conservation laws of energy, momentum and particle number density across the relativistic shock. Furthermore, by using a 1D relativistic PIC code, we study in detail the reconnection process at the termination shock. We found a very simple criterion for dissipation of alternating fields at the termination shock, depending on the upstream parameters of the flow. 1D relativistic PIC simulations are in agreement with our criterion. Thus, alternating magnetic fields annihilate easily at relativistic highly magnetised shocks.},
  Archiveprefix            = {arXiv},
  Arxivid                  = {0707.1782},
  Doi                      = {10.1142/S0218271808013637},
  Eprint                   = {0707.1782},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Petri, Lyubarsky/Unknown/Petri, Lyubarsky - 2007 - Magnetic reconnection at the termination shock in a striped pulsar wind.pdf:pdf},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23},
  Url                      = {http://arxiv.org/abs/0707.1782}
}

@Article{Petrinec2012,
  Title                    = {Energetic ions near the dayside magnetopause reconnection site: {Implications} for energization sources},
  Author                   = {Petrinec, S. M. and Trattner, K. J. and Fuselier, S. A. and Phan, T. D. and Angelopoulos, V.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2012},

  Month                    = oct,
  Pages                    = {65--69},
  Volume                   = {87},

  Doi                      = {10.1016/j.jastp.2011.11.011}
}

@Article{Petrukovich2015,
  Title                    = {Current sheets in the Earth magnetotail: Plasma and magnetic field structure with Cluster project observations},
  Author                   = {Petrukovich, Anatoli and Artemyev, Anton and Vasko, Ivan and Nakamura, Rumi and Zelenyi, Lev},
  Journal                  = {Space Science Reviews},
  Year                     = {2015},
  Number                   = {1-4},
  Pages                    = {311--337},
  Volume                   = {188},

  Owner                    = {suleimanbaraka},
  Publisher                = {Springer},
  Timestamp                = {2016.02.20}
}

@InCollection{Phan2005,
  Title                    = {Magnetopause processes},
  Author                   = {Phan, TD and Escoubet, CP and Rezeau, L and Treumann, RA and Vaivads, A and Paschmann, G and Fuselier, SA and Attié, D and Rogers, B and Sonnerup, BU Ö},
  Booktitle                = {Outer {Magnetospheric} {Boundaries}: {Cluster} {Results}},
  Publisher                = {Springer},
  Year                     = {2005},
  Pages                    = {367--424}
}

@Book{Piel2010,
  Title                    = {Plasma physics: an introduction to laboratory, space, and fusion plasmas},
  Author                   = {Piel, Alexander},
  Publisher                = {Springer Science \& Business Media},
  Year                     = {2010}
}

@Article{Pierce2007,
  Title                    = {Chemical data assimilation estimates of continental {US} ozone and nitrogen budgets during the {Intercontinental} {Chemical} {Transport} {Experiment}–{North} {America}},
  Author                   = {Pierce, Robert B and Schaack, Todd and Al-Saadi, Jassim A and Fairlie, T Duncan and Kittaka, Chieko and Lingenfelser, Gretchen and Natarajan, Murali and Olson, Jennifer and Soja, Amber and Zapotocny, Tom and {others}},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984–2012)},
  Year                     = {2007},
  Number                   = {D12},
  Volume                   = {112}
}

@Article{Pierrard2006,
  Title                    = {Effects of wave-particle interactions on double-hump distributions of the {H}+ polar wind},
  Author                   = {Pierrard, V and Barghouthi, IA},
  Journal                  = {Astrophysics and Space Science},
  Year                     = {2006},
  Number                   = {1-4},
  Pages                    = {35--41},
  Volume                   = {302}
}

@Article{Pino2011,
  Title                    = {Magnetic {Flux} {Transport} by turbulent reconnection in astrophysical flows},
  Author                   = {Pino, Elisabete M. and Leão, Márcia RM and Santos-Lima, Reinaldo and Guerrero, Gustavo and Kowal, Grzegorz and Lazarian, Alex},
  Journal                  = {arXiv preprint arXiv:1112.4871},
  Year                     = {2011},

  Url                      = {http://arxiv.org/abs/1112.4871},
  Urldate                  = {2014-05-31}
}

@Article{Pirjola2005,
  Title                    = {Space weather risk},
  Author                   = {Pirjola, Risto and Kauristie, Kirsti and Lappalainen, Hanna and Viljanen, Ari and Pulkkinen, Antti},
  Journal                  = {Space Weather},
  Year                     = {2005},
  Number                   = {2},
  Volume                   = {3}
}

@Article{Pirjola2000,
  Title                    = {Space weather risk in power systems and pipelines},
  Author                   = {Pirjola, R and Viljanen, A and Pulkkinen, A and Amm, O},
  Journal                  = {Physics and Chemistry of the Earth, Part C: Solar, Terrestrial \& Planetary Science},
  Year                     = {2000},
  Number                   = {4},
  Pages                    = {333--337},
  Volume                   = {25},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S1464191700000271}
}

@Article{Plaschke2009,
  Title                    = {{Standing Alfv{\'{e}}n waves at the magnetopause}},
  Author                   = {Plaschke, F. and Glassmeier, K. H. and Auster, H. U. and Constantinescu, O. D. and Magnes, W. and Angelopoulos, V. and Sibeck, D. G. and McFadden, J. P.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2009},
  Number                   = {2},
  Volume                   = {36},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {We present results from a statistical analysis of the oscillatory motion of the magnetopause based on THEMIS spacecraft observations, yielding the first experimental evidence for the existence of standing Alfv{\'{e}}nic surface or Kruskal-Schwarzschild modes at the magnetopause. The magnetopause boundary represents a membrane under tension, which may resonantly interact with magnetospheric cavity or waveguide modes. Ultra-low ``magic'' geomagnetic pulsation frequencies, often observed in ground-based and ionospheric measurements and attributed to these cavity or waveguide modes, agree with the detected magnetopause oscillation frequencies and are reinterpreted in terms of surface mode eigenfrequencies.},
  Doi                      = {10.1029/2008GL036411},
  ISSN                     = {00948276},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Plaschke2009a,
  Title                    = {Standing {Alfvén} waves at the magnetopause},
  Author                   = {Plaschke, F. and Glassmeier, K.-H. and Auster, H. U. and Constantinescu, O. D. and Magnes, W. and Angelopoulos, V. and Sibeck, D. G. and McFadden, J. P.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2009},
  Pages                    = {2104},
  Volume                   = {36},

  Abstract                 = {We present results from a statistical analysis of the oscillatory motion of the magnetopause based on THEMIS spacecraft observations, yielding the first experimental evidence for the existence of standing Alfvénic surface or Kruskal-Schwarzschild modes at the magnetopause. The magnetopause boundary represents a membrane under tension, which may resonantly interact with magnetospheric cavity or waveguide modes. Ultra-low “magic” geomagnetic pulsation frequencies, often observed in ground-based and ionospheric measurements and attributed to these cavity or waveguide modes, agree with the detected magnetopause oscillation frequencies and are reinterpreted in terms of surface mode eigenfrequencies.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Field-aligned currents and current systems (2409) Magnetospheric Physics: MHD waves and instabilities (2149 6050 7836)},
  Url                      = {http://adsabs.harvard.edu/abs/2009GeoRL..36.2104P}
}

@Article{Plaschke2013,
  Title                    = {Anti-sunward high-speed jets in the subsolar magnetosheath},
  Author                   = {Plaschke, F. and Hietala, H. and Angelopoulos, V.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2013},

  Month                    = oct,
  Pages                    = {1877--1889},
  Volume                   = {31},

  Doi                      = {10.5194/angeo-31-1877-2013}
}

@Article{Pohjolainen2007,
  Title                    = {{CME} {Propagation} {Characteristics} from {Radio} {Observations}},
  Author                   = {Pohjolainen, S. and van Driel-Gesztelyi, L. and Culhane, J. L. and Manoharan, P. K. and Elliott, H. A.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {2007},

  Month                    = aug,
  Pages                    = {167--188},
  Volume                   = {244},

  Doi                      = {10.1007/s11207-007-9006-6},
  Keywords                 = {coronal mass ejections, Dynamic spectrum, Initiation and propagation, Interplanetary, Meter-wavelengths and longer, Plasma physics, Radio bursts, Radio scintillation, Type II}
}

@InProceedings{Pokhotelov2013,
  Title                    = {Ion distributions upstream and downstream of the {Earth}'s bow shock: first results from {Vlasiator}},
  Author                   = {Pokhotelov, D and von Alfthan, S and Kempf, Y and Vainio, R and Koskinen, HEJ and Palmroth, M},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2013},
  Pages                    = {2207--2212},
  Publisher                = {Copernicus GmbH},
  Volume                   = {31}
}

@Article{Pokhotelov2013a,
  Title                    = {Ion distributions upstream and downstream of the {Earth}'s bow shock: first results from {Vlasiator}},
  Author                   = {Pokhotelov, D. and von Alfthan, S. and Kempf, Y. and Vainio, R. and Koskinen, H. E. J. and Palmroth, M.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2013},

  Month                    = dec,
  Pages                    = {2207--2212},
  Volume                   = {31},

  Doi                      = {10.5194/angeo-31-2207-2013}
}

@Article{Poletto2002,
  Title                    = {Low-latitude solar wind during the {Fall} 1998 {SOHO}-{Ulysses} quadrature},
  Author                   = {Poletto, G. and Suess, S. T. and Biesecker, D. A. and Esser, R. and Gloeckler, G. and Ko, Y.-K. and Zurbuchen, T. H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2002},

  Month                    = oct,
  Pages                    = {1300},
  Volume                   = {107},

  Doi                      = {10.1029/2001JA000275},
  Keywords                 = {and Astronomy: Corona, and Astronomy: Coronal holes, ASTROPHYSICS, in situ data, Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Sources of the solar wind, low-latitude solar wind, oxygen flow speed, proton flow speed, SOHO-Ulysses quadrature, Solar Physics}
}

@Article{Pollack1954,
  Title                    = {Information of {Elementary} {Multidimensional} {Auditory} {Displays}},
  Author                   = {Pollack, I.},
  Journal                  = {Acoustical Society of America Journal},
  Year                     = {1954},
  Pages                    = {155},
  Volume                   = {26},

  Doi                      = {10.1121/1.1907300}
}

@Article{Posch2013,
  Title                    = {Simultaneous traveling convection vortex events and {Pc}1 wave bursts at cusp latitudes observed in {Arctic} {Canada} and {Svalbard}},
  Author                   = {Posch, J. L. and Engebretson, M. J. and Witte, A. J. and Murr, D. L. and Lessard, M. R. and Johnsen, M. G. and Singer, H. J. and Hartinger, M. D.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = oct,
  Pages                    = {6352--6363},
  Volume                   = {118},

  Doi                      = {10.1002/jgra.50604},
  Keywords                 = {bow shock, Electromagnetic ion cyclotron waves, ion foreshock, proton aurora, Traveling convection vortices}
}

@Article{Pour-Biazar2011,
  Title                    = {Utilization of satellite observation of ozone and aerosols in providing initial and boundary condition for regional air quality studies},
  Author                   = {Pour-Biazar, Arastoo and Khan, Maudood and Wang, Lihua and Park, Yun-Hee and Newchurch, Mike and McNider, Richard T and Liu, Xiong and Byun, Daewon W and Cameron, Robert},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984–2012)},
  Year                     = {2011},
  Number                   = {D18},
  Volume                   = {116}
}

@Article{Powell1999,
  Title                    = {A {Solution}-{Adaptive} {Upwind} {Scheme} for {Ideal} {Magnetohydrodynamics}},
  Author                   = {Powell, K. G. and Roe, P. L. and Linde, T. J. and Gombosi, T. I. and De Zeeuw, D. L.},
  Journal                  = {J. Comput. Phys.},
  Year                     = {1999},

  Month                    = sep,
  Pages                    = {284--309},
  Volume                   = {154},

  Doi                      = {10.1006/jcph.1999.6299}
}

@Article{Prech2009,
  Title                    = {Propagation of {CIR} originated interplanetary shocks across magnetospheric boundaries},
  Author                   = {Prech, L. and Safrankova, J. and Nemecek, Z. and Samsonov, A.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2009},

  Month                    = dec,
  Pages                    = {B1528},

  Keywords                 = {[2139] INTERPLANETARY PHYSICS / Interplanetary shocks, [2154] INTERPLANETARY PHYSICS / Planetary bow shocks, [2724] MAGNETOSPHERIC PHYSICS / Magnetopause and boundary layers, [2728] MAGNETOSPHERIC PHYSICS / Magnetosheath}
}

@Book{Priest2000,
  Title                    = {Magnetic {Reconnection} ({Cambridge}},
  Author                   = {Priest, E and Forbes, T},
  Publisher                = {Cambridge Univ. Press},
  Year                     = {2000}
}

@Article{Pritchett2001,
  Title                    = {Geospace {Environment} {Modeling} magnetic reconnection challenge: {Simulations} with a full particle electromagnetic code},
  Author                   = {Pritchett, PL},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2001},
  Number                   = {A3},
  Pages                    = {3783--3798},
  Volume                   = {106}
}

@Article{Pritchett2001a,
  Title                    = {Collisionless magnetic reconnection in a three-dimensional open system},
  Author                   = {Pritchett, PL},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2001},
  Number                   = {A11},
  Pages                    = {25961--25977},
  Volume                   = {106}
}

@Article{Pritchett1994,
  Title                    = {Convection and the formation of thin current sheets in the near-{Earth} plasma sheet},
  Author                   = {Pritchett, PL and Coroniti, FV},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1994},
  Number                   = {15},
  Pages                    = {1587--1590},
  Volume                   = {21}
}

@Article{Pritchett1992,
  Title                    = {Formation and stability of the self-consistent one-dimensional tail current sheet},
  Author                   = {Pritchett, PL and Coroniti, FV},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1992},
  Number                   = {A11},
  Pages                    = {16773--16787},
  Volume                   = {97}
}

@Article{Pritchett1996,
  Title                    = {Three-dimensional stability of thin quasi-neutral current sheets},
  Author                   = {Pritchett, PL and Coroniti, FV and Decyk, VK},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1996},
  Number                   = {A12},
  Pages                    = {27413--27429},
  Volume                   = {101}
}

@Article{Pritchett2010,
  Title                    = {Onset of magnetic reconnection in the presence of a normal magnetic field: {Realistic} ion to electron mass ratio},
  Author                   = {Pritchett, P. L.},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2010},
  Number                   = {A10},
  Volume                   = {115},

  Shorttitle               = {Onset of magnetic reconnection in the presence of a normal magnetic field},
  Url                      = {http://www.agu.org/pubs/crossref/2010/2010JA015371.shtml},
  Urldate                  = {2014-05-31}
}

@Article{Pritchett2000,
  Title                    = {Particle-in-cell simulations of magnetosphere electrodynamics},
  Author                   = {Pritchett, Philip L},
  Journal                  = {Plasma Science, IEEE Transactions on},
  Year                     = {2000},
  Number                   = {6},
  Pages                    = {1976--1990},
  Volume                   = {28}
}

@Article{Pritchett2000a,
  Title                    = {{Particle-in-cell simulations of magnetosphere electrodynamics}},
  Author                   = {Pritchett, Philip L},
  Journal                  = {Plasma Sci. IEEE Trans.},
  Year                     = {2000},
  Number                   = {6},
  Pages                    = {1976--1990},
  Volume                   = {28},

  __markedentry            = {[suleimanbaraka:6]},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Pritchett/Plasma Science, IEEE Transactions on/Pritchett.pdf:pdf},
  Owner                    = {suleimanbaraka},
  Publisher                = {IEEE},
  Timestamp                = {2016.02.23}
}

@Article{Pritchett2011,
  Title                    = {Rippling mode in the subsolar magnetopause current layer and its influence on three-dimensional magnetic reconnection},
  Author                   = {Pritchett, P. L. and Mozer, F. S.},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2011},
  Number                   = {A4},
  Volume                   = {116}
}

@Article{Pritchett2012,
  Title                    = {Intense perpendicular electric fields associated with three-dimensional magnetic reconnection at the subsolar magnetopause},
  Author                   = {Pritchett, P. L. and Mozer, F. S. and Wilber, M.},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2012},
  Number                   = {A6},
  Volume                   = {117},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2012JA017533/full},
  Urldate                  = {2014-05-31}
}

@InCollection{Pu2005,
  Title                    = {Multiple flux rope events at the high-latitude magnetopause: {Cluster}/rapid observation on 26 {January}, 2001},
  Author                   = {Pu, ZY and Zong, Q-G and Fritz, TA and Xiao, CJ and Huang, ZY and Fu, SY and Shi, QQ and Dunlop, MW and Glassmeier, K-H and Balogh, A and {others}},
  Booktitle                = {The {Magnetospheric} {Cusps}: {Structure} and {Dynamics}},
  Publisher                = {Springer},
  Year                     = {2005},
  Pages                    = {193--214}
}

@Article{Pu2010,
  Title                    = {{THEMIS} observations of substorms on 26 {February} 2008 initiated by magnetotail reconnection},
  Author                   = {Pu, Z. Y. and Chu, X. N. and Cao, X. and Mishin, V. and Angelopoulos, V. and Wang, J. and Wei, Y. and Zong, Q. G. and Fu, S. Y. and Xie, L. and Glassmeier, K.-H. and Frey, H. and Russell, C. T. and Liu, J. and McFadden, J. and Larson, D. and Mende, S. and Mann, I. and Sibeck, D. and Sapronova, L. A. and Tolochko, M. V. and Saifudinova, T. I. and Yao, Z. H. and Wang, X. G. and Xiao, C. J. and Zhou, X. Z. and Reme, H. and Lucek, E.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2010},
  Pages                    = {2212},
  Volume                   = {115},

  Abstract                 = {On 26 February 2008, the THEMIS satellites observed two substorms that occurred at about 0405 and 0455 UT. Angelopoulos et al. (2008) made a comprehensive study of the second event. In this paper we display detailed features of the two substorms with emphasis on the first. In both substorms, a distinct auroral intensification occurred during the earliest stage of onset, about 1 to 2 min after midtail reconnection began. This initial intensification was weak and localized and thus had the signatures of a pseudobreakup. In both substorms, a second, major intensification occurred next in the substorm onset sequence, followed by rapid and extensive poleward expansion. This second intensification had the features of the major expansion onset and was nearly coincident with observations of earthward flows and magnetic dipolarization in the near-Earth tail. During the growth phase of the two substorms, open magnetic flux accumulated in the polar cap; in the expansion/recovery phase the polar cap open flux was quickly reduced. These observations are in agreement with the assertion that tail reconnection initiates the initial pseudobreakup and the ensuing major expansion and releases and transports energy to eventually cause near-Earth dipolarization and the expansion phase onset of these two substorms.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Substorms Magnetospheric Physics: Auroral phenomena (2407) Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Magnetotail Magnetospheric Physics: Plasma sheet},
  Url                      = {http://adsabs.harvard.edu/abs/2010JGRA..115.2212P}
}

@Article{Pucci2010,
  Title                    = {Elemental {Abundances} in the {Fast} {Solar} {Wind} {Emanating} from {Chromospheric} {Funnels}},
  Author                   = {Pucci, S. and Lie-Svendsen, Ø. and Esser, R.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2010},

  Month                    = feb,
  Pages                    = {993--1002},
  Volume                   = {709},

  Doi                      = {10.1088/0004-637X/709/2/993},
  Keywords                 = {Solar Wind, Sun: abundances, Sun: chromosphere}
}

@Article{Puchtel1999,
  Title                    = {Combined mantle plume-island arc model for the formation of the 2.9 {Ga} sumozero-kenozero greenstone belt, {SE} baltic shield: {Isotope} and trace element constraints},
  Author                   = {Puchtel, I. S. and Hofmann, A. W. and Amelin, Y. V. and Garbe-Schönberg, C.-D. and Samsonov, A. V. and Shchipansky, A. A.},
  Journal                  = {{\textbackslash}gca},
  Year                     = {1999},

  Month                    = nov,
  Pages                    = {3579--3595},
  Volume                   = {63},

  Doi                      = {10.1016/S0016-7037(99)00111-8}
}

@Article{Puchtel1998,
  Title                    = {Oceanic plateau model for continental crustal growth in the {Archaean}: {A} case study from the {Kostomuksha} greenstone belt, {NW} {Baltic} {Shield}},
  Author                   = {Puchtel, I. S. and Hofmann, A. W. and Mezger, K. and Jochum, K. P. and Shchipansky, A. A. and Samsonov, A. V.},
  Journal                  = {Earth Planet. Sci. Lett.},
  Year                     = {1998},

  Month                    = feb,
  Pages                    = {57--74},
  Volume                   = {155},

  Doi                      = {10.1016/S0012-821X(97)00202-1},
  Keywords                 = {Archean, isotopes, komatiite, mantle plumes, oceanic crust}
}

@Article{Pudovkin1997,
  Title                    = {The magnetopause erosion and the magnetosheath magnetic field penetration into the dayside magnetosphere},
  Author                   = {Pudovkin, MI and Zaitseva, SA and Besser, BP},
  Journal                  = {Advances in Space Research},
  Year                     = {1997},
  Number                   = {12},
  Pages                    = {1909--1912},
  Volume                   = {19}
}

@Article{Pudovkin2002,
  Title                    = {{MHD}-modelling of the magnetosheath},
  Author                   = {Pudovkin, M. I. and Zaitseva, S. A. and Lebedeva, V. V. and Samsonov, A. A. and Besser, B. P. and Meister, C.-V. and Baumjohann, W.},
  Journal                  = {{\textbackslash}planss},
  Year                     = {2002},

  Month                    = apr,
  Pages                    = {473--488},
  Volume                   = {50},

  Doi                      = {10.1016/S0032-0633(02)00027-2}
}

@Article{Pueschel2011,
  Title                    = {Gyrokinetic simulations of magnetic reconnection},
  Author                   = {Pueschel, M. J. and Jenko, F. and Told, D. and Büchner, J.},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2011},
  Number                   = {11},
  Pages                    = {112102},
  Volume                   = {18},

  Url                      = {http://scitation.aip.org/content/aip/journal/pop/18/11/10.1063/1.3656965},
  Urldate                  = {2014-05-31}
}

@Article{Pulkkinen2001,
  Title                    = {Modelling of space weather effects on pipelines},
  Author                   = {Pulkkinen, Antti and Pirjola, Risto and Boteler, David and Viljanen, Ari and Yegorov, Igor},
  Journal                  = {Journal of Applied Geophysics},
  Year                     = {2001},
  Number                   = {4},
  Pages                    = {233--256},
  Volume                   = {48},

  Url                      = {http://www.sciencedirect.com/science/article/pii/S0926985101001094}
}

@InProceedings{Qing2014,
  Title                    = {Kelvin-{Helmholtz} vortices observed by {Themis} at the dusk side of the magnetopause under southward {IMF}},
  Author                   = {Qing, Yan Guang and McFadden, James and Parks, George and Shen, Chao and Mozer, Forrest and Cai, Chunlin and {others}},
  Booktitle                = {40th {COSPAR} {Scientific} {Assembly}. {Held} 2-10 {August} 2014, in {Moscow}, {Russia}, {Abstract} {D}3. 5-16-14.},
  Year                     = {2014},
  Pages                    = {1091},
  Volume                   = {40},

  Url                      = {http://adsabs.harvard.edu/abs/2014cosp...40E1091Q},
  Urldate                  = {2014-10-22}
}

@Article{Quilis2001,
  Title                    = {Bubbles, feedback and the intracluster medium: three-dimensional hydrodynamic simulations},
  Author                   = {Quilis, Vicent and Bower, Richard G and Balogh, Michael L},
  Journal                  = {Monthly Notices of the Royal Astronomical Society},
  Year                     = {2001},
  Number                   = {4},
  Pages                    = {1091--1097},
  Volume                   = {328}
}

@InCollection{Raeder2009,
  Title                    = {{OpenGGCM} simulations for the {THEMIS} mission},
  Author                   = {Raeder, Joachim and Larson, Douglas and Li, Wenhui and Kepko, Emil L and Fuller-Rowell, Timothy},
  Booktitle                = {The {THEMIS} {Mission}},
  Publisher                = {Springer},
  Year                     = {2009},
  Pages                    = {535--555},

  Url                      = {http://link.springer.com/chapter/10.1007/978-0-387-89820-9_22}
}

@Article{Raeder2001,
  Title                    = {Global simulation of magnetospheric space weather effects of the {Bastille} {Day} storm},
  Author                   = {Raeder, J and Wang, YL and Fuller-Rowell, TJ and Singer, HJ},
  Journal                  = {Solar Physics},
  Year                     = {2001},
  Number                   = {1-2},
  Pages                    = {323--337},
  Volume                   = {204},

  Url                      = {http://link.springer.com/article/10.1023/A:1014228230714}
}

@InProceedings{Raines2005,
  Title                    = {Heavy {Ions} in the {Solar} {Wind}: {A} {New} {Dataset} from {ACE}},
  Author                   = {Raines, J. and Lepri, S. T. and Zurbuchen, T. H. and Gloeckler, G. and Fisk, L. A.},
  Booktitle                = {Solar {Wind} 11/{SOHO} 16, {Connecting} {Sun} and {Heliosphere}},
  Year                     = {2005},
  Editor                   = {Fleck, B. and Zurbuchen, T. H. and Lacoste, H.},
  Month                    = sep,
  Pages                    = {539},
  Series                   = {{ESA} {Special} {Publication}},
  Volume                   = {592}
}

@Article{Rastaetter2012,
  Title                    = {Scientific visualization to study {Flux} {Transfer} {Events} at the {Community} {Coordinated} {Modeling} {Center}},
  Author                   = {Rastätter, Lutz and Kuznetsova, Maria M. and Sibeck, David G. and Berrios, David H.},
  Journal                  = {Advances in Space Research},
  Year                     = {2012},
  Pages                    = {1623--1632},
  Volume                   = {49},

  Abstract                 = {In this paper we present recent additions to the visualization toolset offered by the Community Coordinated Modeling Center (CCMC). Two suites of visualization tools are available that can address different needs during the analysis of model simulations of the magnetosphere that are provided by the CCMC. The online, server-side visualization allows the user to quickly browse through simulation runs and now can create maps of magnetic field line topology in the magnetosphere. The second tool, SWX, can be used on the client computer after data have been downloaded. With this second tool the user can interact directly with the three-dimensional objects that are being rendered. We present results from a simulation of a Flux Transfer Event that was performed at the CCMC using a magnetohydrodynamic model of the Earth's magnetosphere with a high resolution grid focused on the dayside magnetosheath and dayside magnetopause. The simulation shows that the FTE that results from localized magnetic reconnection is a complicated three-dimensional structure that requires modern visualization techniques. Visualization techniques that are presented here allow the researcher to fully appreciate the complexity contained in magnetospheric simulation results.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/2012AdSpR..49.1623R}
}

@Article{Raymond1998,
  Title                    = {Elemental abundances in coronal structures},
  Author                   = {Raymond, John C and Suleiman, Raid and Kohl, John L and Noci, Giancarlo},
  Journal                  = {Space science reviews},
  Year                     = {1998},
  Number                   = {1-2},
  Pages                    = {283--289},
  Volume                   = {85}
}

@Article{Reiff1977,
  Title                    = {Solar wind plasma injection at the dayside magnetospheric cusp},
  Author                   = {Reiff, PH and Hill, TW and Burch, JL},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1977},
  Number                   = {4},
  Pages                    = {479--491},
  Volume                   = {82}
}

@Article{Reiners2010,
  Title                    = {A magnetic field evolution scenario for brown dwarfs and giant planets},
  Author                   = {Reiners, A. and Christensen, U. R.},
  Journal                  = {{\textbackslash}textbackslashaap},
  Year                     = {2010},

  Month                    = nov,
  Pages                    = {A13},
  Volume                   = {522},

  Doi                      = {10.1051/0004-6361/201014251},
  Keywords                 = {brown dwarfs, planets and satellites: magnetic fields, stars: activity, stars: low-mass, stars: magnetic field}
}

@InProceedings{Reme2001,
  Title                    = {First multispacecraft ion measurements in and near the {Earth}'s magnetosphere with the identical {Cluster} ion spectrometry ({CIS}) experiment},
  Author                   = {Reme, H and Aoustin, C and Bosqued, JM and Dandouras, I and Lavraud, B and Sauvaud, JA and Barthe, A and Bouyssou, J and Camus, Th and Coeur-Joly, O and {others}},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2001},
  Pages                    = {1303--1354},
  Volume                   = {19}
}

@Article{Reme1997,
  Title                    = {The {Cluster} {Ion} {Spectrometry} (cis) {Experiment}},
  Author                   = {Reme, H. and Bosqued, J. M. and Sauvaud, J. A. and Cros, A. and Dandouras, J. and Aoustin, C. and Bouyssou, J. and Camus, T. and Cuvilo, J. and Martz, C. and Medale, J. L. and Perrier, H. and Romefort, D. and Rouzaud, J. and D`Uston, C. and Mobius, E. and Crocker, K. and Granoff, M. and Kistler, L. M. and Popecki, M. and Hovestadt, D. and Klecker, B. and Paschmann, G. and Scholer, M. and Carlson, C. W. and Curtis, D. W. and Lin, R. P. and McFadden, J. P. and Formisano, V. and Amata, E. and Bavassano-Cattaneo, M. B. and Baldetti, P. and Belluci, G. and Bruno, R. and Chionchio, G. and di Lellis, A. and Shelley, E. G. and Ghielmetti, A. G. and Lennartsson, W. and Korth, A. and Rosenbauer, H. and Lundin, R. and Olsen, S. and Parks, G. K. and McCarthy, M. and Balsiger, H.},
  Journal                  = {ßr},
  Year                     = {1997},

  Month                    = jan,
  Pages                    = {303--350},
  Volume                   = {79},

  Doi                      = {10.1023/A:1004929816409}
}

@Article{Reme1997a,
  Title                    = {The {Cluster} {Ion} {Spectrometry} (cis) {Experiment}},
  Author                   = {Reme, H. and Bosqued, J. M. and Sauvaud, J. A. and Cros, A. and Dandouras, J. and Aoustin, C. and Bouyssou, J. and Camus, T. and Cuvilo, J. and Martz, C. and Medale, J. L. and Perrier, H. and Romefort, D. and Rouzaud, J. and D`Uston, C. and Mobius, E. and Crocker, K. and Granoff, M. and Kistler, L. M. and Popecki, M. and Hovestadt, D. and Klecker, B. and Paschmann, G. and Scholer, M. and Carlson, C. W. and Curtis, D. W. and Lin, R. P. and McFadden, J. P. and Formisano, V. and Amata, E. and Bavassano-Cattaneo, M. B. and Baldetti, P. and Belluci, G. and Bruno, R. and Chionchio, G. and di Lellis, A. and Shelley, E. G. and Ghielmetti, A. G. and Lennartsson, W. and Korth, A. and Rosenbauer, H. and Lundin, R. and Olsen, S. and Parks, G. K. and McCarthy, M. and Balsiger, H.},
  Journal                  = {√ür},
  Year                     = {1997},

  Month                    = jan,
  Pages                    = {303--350},
  Volume                   = {79},

  Doi                      = {10.1023/A:1004929816409}
}

@Article{Remer2012,
  Title                    = {Retrieving aerosol in a cloudy environment: aerosol availability as a function of spatial and temporal resolution},
  Author                   = {Remer, Lorraine A. and Mattoo, Shana and Levy, Robert C. and Heidinger, Andrew and Pierce, R. Bradley and Chin, Mian},
  Journal                  = {Atmospheric Measurement Techniques Discussions},
  Year                     = {2012},
  Number                   = {1},
  Pages                    = {627--662},
  Volume                   = {5},

  Shorttitle               = {Retrieving aerosol in a cloudy environment},
  Url                      = {http://atmos-meas-tech-discuss.net/5/627/2012/amtd-5-627-2012.pdf},
  Urldate                  = {2014-11-13}
}

@Article{Remya2014,
  Title                    = {Large-{Amplitude}, {Circularly} {Polarized}, {Compressive}, {Obliquely} {Propagating} {Electromagnetic} {Proton} {Cyclotron} {Waves} {Throughout} the {Earth}'{S} {Magnetosheath}: {Low} {Plasma} ‚âà√≠‚àö‚â† {Conditions}},
  Author                   = {Remya, B. and Tsurutani, B. T. and Reddy, R. V. and Lakhina, G. S. and Falkowski, B. J. and Echer, E. and Glassmeier, K.-H.},
  Journal                  = {Astrophys. J.},
  Year                     = {2014},
  Number                   = {1},
  Pages                    = {6},
  Volume                   = {793},

  Doi                      = {10.1088/0004-637X/793/1/6},
  ISSN                     = {1538-4357},
  Keywords                 = {cassini, color figures, data analysis, earth, individual, instabilities, Magnetic Fields, methods, online-only material, planets and satellites, polarization, wind},
  Url                      = {http://stacks.iop.org/0004-637X/793/i=1/a=6?key=crossref.abe04e85aa5a2a7b4f9b407126522d95}
}

@Article{Retterer1987,
  Title                    = {Monte {Carlo} modeling of oxygen-ion conic acceleration by cyclotron resonance with broadband electromagnetic turbulence},
  Author                   = {Retterer, JM and Chang, T and Crew, GB},
  Year                     = {1987},

  Url                      = {http://www.osti.gov/scitech/biblio/6992149}
}

@Article{Ricci2002,
  Title                    = {{GEM} reconnection challenge: {Implicit} kinetic simulations with the physical mass ratio},
  Author                   = {Ricci, Paolo},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2002},
  Number                   = {23},
  Pages                    = {2088},
  Volume                   = {29},

  Doi                      = {10.1029/2002GL015314},
  ISSN                     = {0094-8276},
  Keywords                 = {doi:10.1029/2002GL015314, http://dx.doi.org/10.1029/2002GL015314},
  Url                      = {http://doi.wiley.com/10.1029/2002GL015314}
}

@Article{Ricci2002b,
  Title                    = {{GEM reconnection challenge: Implicit kinetic simulations with the physical mass ratio}},
  Author                   = {Ricci, P and Lapenta, G and Brackbill, J.{\~{}}U.},
  Journal                  = {$\backslash$grl},
  Year                     = {2002},

  Month                    = {dec},
  Pages                    = {2088},
  Volume                   = {29},

  __markedentry            = {[suleimanbaraka:6]},
  Doi                      = {10.1029/2002GL015314},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Ricci, Lapenta, Brackbill/grl/Ricci - 2002 - GEM reconnection challenge Implicit kinetic simulations with the physical mass ratio.pdf:pdf},
  Keywords                 = {Magnetospheric Physics: Plasma sheet,Space Plasma Physics: Magnetic reconnection,Space Plasma Physics: Nonlinear phenomena,Space Plasma Physics: Numerical simulation studie},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Ricci2002a,
  Title                    = {{GEM} reconnection challenge: {Implicit} kinetic simulations with the physical mass ratio},
  Author                   = {Ricci, P. and Lapenta, G. and Brackbill, J. U.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {2002},

  Month                    = dec,
  Pages                    = {2088},
  Volume                   = {29},

  Doi                      = {10.1029/2002GL015314},
  Keywords                 = {Magnetospheric Physics: Plasma sheet, Space Plasma Physics: Magnetic reconnection, Space Plasma Physics: Nonlinear phenomena, Space Plasma Physics: Numerical simulation studies}
}

@Article{Rich1994,
  Title                    = {Large-scale convection patterns observed by {DMSP}},
  Author                   = {Rich, Frederick J and Hairston, Marc},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1994},
  Number                   = {A3},
  Pages                    = {3827--3844},
  Volume                   = {99}
}

@Article{Richardson2010,
  Title                    = {Near-{Earth} {Interplanetary} {Coronal} {Mass} {Ejections} {During} {Solar} {Cycle} 23 (1996 - 2009): {Catalog} and {Summary} of {Properties}},
  Author                   = {Richardson, I. G. and Cane, H. V.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {2010},

  Month                    = jun,
  Pages                    = {189--237},
  Volume                   = {264},

  Doi                      = {10.1007/s11207-010-9568-6},
  Keywords                 = {coronal mass ejections, Interplanetary coronal mass ejections, interplanetary magnetic field, Magnetic Clouds, Solar wind plasma}
}

@Article{Richardson2004,
  Title                    = {Identification of interplanetary coronal mass ejections at 1 {AU} using multiple solar wind plasma composition anomalies},
  Author                   = {Richardson, I. G. and Cane, H. V.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = sep,
  Pages                    = {9104},
  Volume                   = {109},

  Doi                      = {10.1029/2004JA010598},
  Keywords                 = {and magnetic clouds, composition, driver gases, Interplanetary coronal mass ejections, Interplanetary Physics: Ejecta, Interplanetary Physics: Interplanetary magnetic fields, Interplanetary Physics: Solar cycle variations (7536), Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Sources of the solar wind, Solar Wind}
}

@Article{Richardson2008,
  Title                    = {Plasma temperature distributions in the heliosheath},
  Author                   = {Richardson, JD},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2008},
  Number                   = {23},
  Volume                   = {35}
}

@Article{Richer2012,
  Title                    = {A global hybrid model for {Mercury}'s interaction with the solar wind: {Case} study of the dipole representation},
  Author                   = {Richer, E and Modolo, Ronan and Chanteur, GM and Hess, Sebastien and Leblanc, François},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2012},
  Number                   = {A10},
  Volume                   = {117}
}

@Article{Ridley2006,
  Title                    = {The magnetospheric and ionospheric response to a very strong interplanetary shock and coronal mass ejection},
  Author                   = {Ridley, A. J. and De Zeeuw, D. L. and Manchester, W. B. and Hansen, K. C.},
  Journal                  = {Advances in Space Research},
  Year                     = {2006},

  Month                    = jan,
  Pages                    = {263--272},
  Volume                   = {38},

  Doi                      = {10.1016/j.asr.2006.06.010}
}

@Article{Rigby1973,
  Title                    = {The effect of the earth's bow shock and magnetosheath on the interaction of a discontinuity in the solar wind with the magnetosphere},
  Author                   = {Rigby, Barbara J and Mainstone, JS},
  Journal                  = {Planetary and Space Science},
  Year                     = {1973},
  Number                   = {3},
  Pages                    = {499--506},
  Volume                   = {21}
}

@Article{Riley1997a,
  Title                    = {by a fast , high-pressure coronal mass ejection},
  Author                   = {Riley, Pete and Gosling, J T},
  Year                     = {1997},
  Number                   = {97},
  Volume                   = {102},

  __markedentry            = {[suleimanbaraka:6]},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Riley, Gosling/Unknown/Riley, Gosling - 1997 - by a fast , high-pressure coronal mass ejection.pdf:pdf},
  Keywords                 = {http://dx.doi.org/10.1029/97JA01131, doi:10.1029/9},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Riley1997,
  Title                    = {A two-dimensional simulation of the radial and latitudinal evolution of a solar wind disturbance driven by a fast, high-pressure coronal mass ejection},
  Author                   = {Riley, Pete and Gosling, Jo To and Pizzo, VJ},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1997},
  Number                   = {A7},
  Pages                    = {14677--14,685},
  Volume                   = {102},

  Abstract                 = {Page 1. JOURNAL OF GEOPHYSICAL RESEARCH, VOL. 102, NO* A7, PAGES 14,677-14,685,JULY 1, 1997 A two-dimensional simulation of the radial and latitudinal evolution of a solar winddisturbance driven by a fast, high-pressure coronal mass ejection.}
}

@Article{Riley2004,
  Title                    = {Fitting flux ropes to a global {MHD} solution: a comparison of techniques},
  Author                   = {Riley, P. and Linker, J. A. and Lionello, R. and Mikić, Z. and Odstrcil, D. and Hidalgo, M. A. and Cid, C. and Hu, Q. and Lepping, R. P. and Lynch, B. J. and Rees, A.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2004},

  Month                    = oct,
  Pages                    = {1321--1331},
  Volume                   = {66},

  Doi                      = {10.1016/j.jastp.2004.03.019}
}

@InProceedings{Robert2006,
  Title                    = {Study of a flux transfer event with {Cluster} spacecraft},
  Author                   = {Robert, P},
  Booktitle                = {Geophysical {Research} {Abstracts}},
  Year                     = {2006},
  Pages                    = {04123},
  Volume                   = {8}
}

@Article{Robertson2012,
  Title                    = {Solar wind charge exchange during geomagnetic storms},
  Author                   = {Robertson, I. P. and Cravens, T. E. and Sibeck, D. G. and Collier, M. R. and Kuntz, K. D.},
  Journal                  = {Astronomische Nachrichten},
  Year                     = {2012},
  Pages                    = {309},
  Volume                   = {333},

  Abstract                 = {On 2001 March 31 a coronal mass ejection pushed the subsolar magnetopause to the vicinity of geosynchronous orbit at 6.6 R\_E. The NASA/GSFC Community Coordinated Modeling Center (CCMC) employed a global magnetohydrodynamic (MHD) model to simulate the solar wind-magnetosphere interaction during the peak of this geomagnetic storm. Robertson et al. then modeled the expected soft X-ray emission due to solar wind charge exchange with geocoronal neutrals in the dayside cusp and magnetosheath. The locations of the bow shock, magnetopause and cusps were clearly evident in their simulations. Another geomagnetic storm took place on 2000 July 14 (Bastille Day). We again modeled X-ray emission due to solar wind charge exchange, but this time as observed from a moving spacecraft. This paper discusses the impact of spacecraft location on observed X-ray emission and the degree to which the locations of the bow shock and magnetopause can be detected in images.},
  ISSN                     = {0004-6337},
  Keywords                 = {Earth solar-terrestrial relations solar wind X-rays: general},
  Url                      = {http://adsabs.harvard.edu/abs/2012AN....333..309R}
}

@Article{Robrade2008,
  Title                    = {Neon and oxygen in low activity stars: towards a coronal unification with the {Sun}},
  Author                   = {Robrade, J. and Schmitt, J. H. M. M. and Favata, F.},
  Journal                  = {{\textbackslash}aap},
  Year                     = {2008},

  Month                    = aug,
  Pages                    = {995--1002},
  Volume                   = {486},

  Doi                      = {10.1051/0004-6361:200809690},
  Keywords                 = {stars: abundances, stars: activity, stars: coronae, X-rays: stars}
}

@Article{Rodgers2003,
  Title                    = {Intercomparison of remote sounding instruments},
  Author                   = {Rodgers, Clive D. and Connor, Brian J.},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2003},
  Number                   = {D3},
  Volume                   = {108},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2002JD002299/full},
  Urldate                  = {2014-11-13}
}

@Article{Rodriguez2008,
  Title                    = {Magnetic clouds seen at different locations in the heliosphere},
  Author                   = {Rodriguez, L. and Zhukov, A. N. and Dasso, S. and Mandrini, C. H. and Cremades, H. and Cid, C. and Cerrato, Y. and Saiz, E. and Aran, A. and Menvielle, M. and Poedts, S. and Schmieder, B.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2008},

  Month                    = feb,
  Pages                    = {213--229},
  Volume                   = {26},

  Doi                      = {10.5194/angeo-26-213-2008}
}

@Article{Roelof1995,
  Title                    = {Reply},
  Author                   = {Roelof, Edmond C. and Sibeck, David G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1995},
  Pages                    = {1903--1910},
  Volume                   = {100},

  Abstract                 = {Not Available},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Magnetotail Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/1995JGR...100.1903R}
}

@Article{Roelof1994,
  Title                    = {Erratum: “{Magnetopause} shape as a bivariate function of interplanetary magnetic field {Bz} and solar wind dynamic pressure”},
  Author                   = {Roelof, Edmond C. and Sibeck, David G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1994},
  Pages                    = {8787--8788},
  Volume                   = {99},

  Abstract                 = {Not Available},
  ISSN                     = {0148-0227},
  Keywords                 = {Corrections},
  Url                      = {http://adsabs.harvard.edu/abs/1994JGR....99.8787R}
}

@Article{Roelof1993,
  Title                    = {Magnetopause shape as a bivariate function of interplanetary magnetic field {Bz} and solar wind dynamic pressure},
  Author                   = {Roelof, Edmond C and Sibeck, David G},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1993},
  Number                   = {A12},
  Pages                    = {21421--21450},
  Volume                   = {98}
}

@Article{Rojas-Castillo2013,
  Title                    = {Foreshock compressional boundaries observed by {Cluster}},
  Author                   = {Rojas-Castillo, D and Blanco-Cano, X and Kajdič, P and Omidi, N},
  Journal                  = {Journal of Geophysical Research: Space Physics},
  Year                     = {2013}
}

@Article{Ruffenach2012,
  Title                    = {Multispacecraft observation of magnetic cloud erosion by magnetic reconnection during propagation},
  Author                   = {Ruffenach, A. and Lavraud, B. and Owens, M. J. and Sauvaud, J.-A. and Savani, N. P. and Rouillard, A. P. and Démoulin, P. and Foullon, C. and Opitz, A. and Fedorov, A. and Jacquey, C. J. and Génot, V. and Louarn, P. and Luhmann, J. G. and Russell, C. T. and Farrugia, C. J. and Galvin, A. B.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2012},

  Month                    = sep,
  Pages                    = {9101},
  Volume                   = {117},

  Doi                      = {10.1029/2012JA017624},
  Keywords                 = {7513), 7835), and Astronomy: Magnetic reconnection (2723, and magnetic clouds, ASTROPHYSICS, driver gases, Interplanetary Physics: Coronal mass ejections (4305, Interplanetary Physics: Ejecta, Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Solar wind sources, Solar Physics}
}

@Article{Rukolaine2013,
  Title                    = {Local immobilization of particles in mass transfer described by a {Jeffreys}-type equation},
  Author                   = {Rukolaine, S. A. and Samsonov, A. M.},
  Journal                  = {{\textbackslash}pre},
  Year                     = {2013},

  Month                    = dec,
  Number                   = {6},
  Pages                    = {062116},
  Volume                   = {88},

  Doi                      = {10.1103/PhysRevE.88.062116},
  Keywords                 = {Classical statistical mechanics, Classical transport, Diffusion, Stochastic analysis methods}
}

@Article{Rukolaine2012,
  Title                    = {Delayed uncoupled continuous-time random walks do not provide a model for the telegraph equation},
  Author                   = {Rukolaine, S. A. and Samsonov, A. M.},
  Journal                  = {{\textbackslash}pre},
  Year                     = {2012},

  Month                    = feb,
  Number                   = {2},
  Pages                    = {021150},
  Volume                   = {85},

  Doi                      = {10.1103/PhysRevE.85.021150},
  Keywords                 = {Approximations and expansions, Classical transport, Partial differential equations, Random walks and Levy flights}
}

@Article{Runov2003,
  Title                    = {Current sheet structure near magnetic {X}-line observed by {Cluster}},
  Author                   = {Runov, A and Nakamura, R and Baumjohann, W and Treumann, RA and Zhang, TL and Volwerk, M and Vörös, Z and Balogh, A and Gla{\textbackslash}s smeier, K-H and Klecker, B and {others}},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2003},
  Number                   = {11},
  Volume                   = {30}
}

@Article{Runov2003a,
  Title                    = {Cluster observation of a bifurcated current sheet},
  Author                   = {Runov, A and Nakamura, R and Baumjohann, W and Zhang, TL and Volwerk, M and Eichelberger, H-U and Balogh, A},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2003},
  Number                   = {2},
  Volume                   = {30}
}

@Article{Russell1988,
  Title                    = {Multipoint measurements of upstream waves},
  Author                   = {Russell, CT},
  Journal                  = {Advances in Space Research},
  Year                     = {1988},
  Number                   = {9},
  Pages                    = {147--156},
  Volume                   = {8}
}

@Article{Russell1985,
  Title                    = {Planetary bow shocks},
  Author                   = {Russell, CT},
  Journal                  = {Collisionless shocks in the heliosphere: reviews of current research},
  Year                     = {1985},
  Pages                    = {109--130}
}

@Article{Russell1977,
  Title                    = {On the relative locations of the bow shocks of the terrestrial planets},
  Author                   = {Russell, CT},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1977},
  Number                   = {10},
  Pages                    = {387--390},
  Volume                   = {4}
}

@Article{Russell1982,
  Title                    = {Overshoots in planetary bow shocks},
  Author                   = {Russell, CT and Hoppe, MM and Livesey, WA},
  Year                     = {1982}
}

@Article{Safrankova2002,
  Title                    = {{The magnetopause shape and location: a comparison of the Interball and Geotail observations with models}},
  Author                   = {Safr{\'{a}}nkov{\'{a}}, J and Nemecek, Z and Dus{\'{\i}}k, S and Prech, L and Sibeck, D G and Borodkova, N N},
  Journal                  = {Ann. Geophys.},
  Year                     = {2002},
  Pages                    = {301--309},
  Volume                   = {20},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {A number of magnetopause models have been developed in the course of last three decades. We have chosen seven of them and tested them using a fresh set of magnetopause crossings observed by Interball-1, Magion-4, and Geotail satellites. The crossings cover the magnetopause from the subsolar region up to near-Earth tail (XGSE {\~{}} - 20 RE ) and all geomagnetic latitudes. Our study reveals that (1) the difference between investigated models is smaller than the error of prediction caused by the factors not included in models, (2) the dayside magnetopause is indented in the cusp region, (3) the deepness of the indentation can reach {\~{}} 4 RE , and (4) the dimensions of the indentation do not depend on the dipole tilt, whereas its location does.},
  Doi                      = {10.5194/angeo-20-301-2002},
  ISSN                     = {0992-7689},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23},
  Url                      = {http://adsabs.harvard.edu/abs/2002AnGeo..20..301S}
}

@Article{Safrankova2012,
  Title                    = {Asymmetric magnetosphere deformation driven by hot flow anomaly(ies)},
  Author                   = {Šafránková, J. and Goncharov, O. and Němeček, Z. and Přech, L. and Sibeck, D. G.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {2012},

  Month                    = aug,
  Pages                    = {15107},
  Volume                   = {39},

  Doi                      = {10.1029/2012GL052636},
  Keywords                 = {Interplanetary Physics: Interplanetary magnetic fields, Magnetospheric Physics: Magnetospheric configuration and dynamics, Magnetospheric Physics: Solar wind/magnetosphere interactions}
}

@Article{Safrankova2012a,
  Title                    = {Asymmetric magnetosphere deformation driven by hot flow anomaly(ies)},
  Author                   = {Šafránková, J. and Goncharov, O. and Němeček, Z. and Přech, L. and Sibeck, D. G.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2012},
  Pages                    = {15107},
  Volume                   = {39},

  Abstract                 = {We present a case study of a large deformation of the magnetopause on November 26, 2008. The investigation is based on observations of five THEMIS spacecraft located at the dawn flank in the magnetosphere and magnetosheath, on Cluster measurements at the dusk magnetosheath, and is supported by ACE solar wind monitoring. The main revelation of our study is that the interaction of the IMF discontinuity with the bow shock creates either one very elongated hot flow anomaly (HFA) or a pair of them that is (are) simultaneously observed at both flanks. Whereas the dusk HFA is weak and does not cause observable deformation of the magnetopause, the pressure variations connected with the dawn HFA lead to a magnetopause displacement by ≈5 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} outward from its nominal position. This is followed by a rapid inward motion of the magnetopause ≈4 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} inward with respect to the model location. The surface deformation is so large that the outermost THEMIS spacecraft was in the magnetosphere, whereas the spacecraft located 9 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} inbound entered into the magnetosheath at the same time. The whole event lasted about 5 minutes.},
  ISSN                     = {0094-8276},
  Keywords                 = {Interplanetary Physics: Interplanetary magnetic fields Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2012GeoRL..3915107S}
}

@Article{Safrankova2005,
  Title                    = {Interplanetary {Shocks} in the {Magnetosheath}: {Comparison} of {Experimental} {Data} {With} {MHD} {Modeling}},
  Author                   = {Safrankova, J. and Koval, A. and Nemecek, Z. and Prech, L. and Hayosh, M. and Samsonov, A. and Kuznetsova, M.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2005},

  Month                    = dec,
  Pages                    = {A1},

  Keywords                 = {2134 Interplanetary magnetic fields, 2139 Interplanetary shocks, 2164 Solar wind plasma, 2728 Magnetosheath}
}

@Article{Safrankova2002a,
  Title                    = {The magnetopause shape and location: a comparison of the {Interball} and {Geotail} observations with models},
  Author                   = {Safránková, J. and Nemecek, Z. and Dusík, S. and Prech, L. and Sibeck, D. G. and Borodkova, N. N.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2002},
  Pages                    = {301--309},
  Volume                   = {20},

  Abstract                 = {A number of magnetopause models have been developed in the course of last three decades. We have chosen seven of them and tested them using a fresh set of magnetopause crossings observed by Interball-1, Magion-4, and Geotail satellites. The crossings cover the magnetopause from the subsolar region up to near-Earth tail (XGSE - 20 RE ) and all geomagnetic latitudes. Our study reveals that (1) the difference between investigated models is smaller than the error of prediction caused by the factors not included in models, (2) the dayside magnetopause is indented in the cusp region, (3) the deepness of the indentation can reach 4 RE , and (4) the dimensions of the indentation do not depend on the dipole tilt, whereas its location does.},
  ISSN                     = {0992-7689},
  Url                      = {http://adsabs.harvard.edu/abs/2002AnGeo..20..301S}
}

@Article{Safrankova2007,
  Title                    = {Modification of interplanetary shocks near the bow shock and through the magnetosheath},
  Author                   = {Šafránková, J. and Němeček, Z. and Přech, L. and Samsonov, A. A. and Koval, A. and Andréeová, K.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2007},

  Month                    = aug,
  Pages                    = {8212},
  Volume                   = {112},

  Doi                      = {10.1029/2007JA012503},
  Keywords                 = {Interplanetary Physics: Interplanetary shocks, Interplanetary Physics: Planetary bow shocks, Magnetospheric Physics: Magnetosheath, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Solar wind/magnetosphere interactions}
}

@Article{Safrankova2007a,
  Title                    = {Interaction of interplanetary shocks with the bow shock},
  Author                   = {Šafránková, J. and Němeček, Z. and Přech, L. and Samsonov, A. A. and Koval, A. and Andréeová, K.},
  Journal                  = {{\textbackslash}planss},
  Year                     = {2007},

  Month                    = dec,
  Pages                    = {2324--2329},
  Volume                   = {55},

  Doi                      = {10.1016/j.pss.2007.05.012}
}

@Article{Safrankova2007b,
  Title                    = {Interaction of {Interplanetary} {Shocks} {With} the {Bow} {Shock} and {Their} {Propagation} {Within} the {Magnetosheath}},
  Author                   = {Safrankova, J. and Nemecek, Z. and Prech, L. and Samsonov, A. and Koval, A. and Andreeova, K.},
  Journal                  = {AGU Spring Meeting Abstracts},
  Year                     = {2007},

  Month                    = may,
  Pages                    = {B8},

  Keywords                 = {2139 Interplanetary shocks, 2154 Planetary bow shocks, 2728 Magnetosheath, 2753 Numerical modeling, 2784 Solar wind/magnetosphere interactions}
}

@Article{Safrankova2007c,
  Title                    = {Variations of the flank {LLBL} thickness as response to the solar wind dynamic pressure and {IMF} orientation},
  Author                   = {Šafránková, J. and Němeček, Z. and Přech, L. and Šimůnek, J. and Sibeck, D. and Sauvaud, J.-A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2007},
  Pages                    = {7201},
  Volume                   = {112},

  Abstract                 = {Several mechanisms have been discussed as candidates for a formation of the low-latitude boundary layer (LLBL) magnetic reconnection between the magnetospheric and magnetosheath magnetic fields, impulsive penetration of magnetosheath plasma, and viscous/diffusive mixing of plasma populations at the magnetopause. The observed fluctuations of plasma parameters inside the LLBL are attributed either to transient nature of the phenomena forming the layer or to sweeping of deformations of the magnetopause or an inner edge of the LLBL surface along the spacecraft. We are using the Interball-1/Magion-4 satellite pair separated by several thousands of kilometers in order to distinguish between spatial and temporal changes of the LLBL plasma population. Observations of LLBL crossings invoked by sudden changes of upstream conditions show that even during a strongly northward interplanetary magnetic field (IMF), the LLBL is relatively thin and follows the compression of the magnetopause induced by changes of the solar wind dynamic pressure. The thickness of the LLBL increases significantly (from a small fraction of R {\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} to more than 1.4 R {\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}) with increase in upstream density and IMF B {\textless}SUB{\textgreater} Y {\textless}/SUB{\textgreater} component. Our results indicate that the dusk LLBL is supplied by high-latitude reconnection in the Southern (Northern) Hemisphere, when IMF B {\textless}SUB{\textgreater} Y {\textless}/SUB{\textgreater} is negative (positive) and lies on open field lines. The change of IMF B {\textless}SUB{\textgreater} Y {\textless}/SUB{\textgreater} direction leads to brief presence of LLBL plasma outside the magnetopause on magnetosheath field lines. Fluctuations of plasma parameters and magnetic field implicate the presence of surface waves on the inner edge of the LLBL, but no waves were observed on the magnetopause.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetic reconnection (7526 7835) Space Plasma Physics: Transport processes},
  Url                      = {http://adsabs.harvard.edu/abs/2007JGRA..112.7201S}
}

@Article{Safrankova1997,
  Title                    = {Two point observation of magnetopause motion: the interball project},
  Author                   = {Šafránková, J. and Němeček, Z. and Přech, L. and Zastenker, G. and Fedorov, A. and Romanov, Š . and Sibeck, D. and Šimůnek, J.},
  Journal                  = {Advances in Space Research},
  Year                     = {1997},
  Pages                    = {801--807},
  Volume                   = {20},

  Abstract                 = {On August 3, 1995, two satellites of the INTERBALL mission were launched into a highly elliptical dawnside orbit with an apogee near 200 000 km and a perigee of 800 km. The distance separating the satellites varies from one to several thousand km. Both satellites carry sets of Faraday cups which cover a spatial angle approaching nearly 4pi. The cups provide high resolution data (up to 16 Hz for the main satellite and 10 Hz for the subsatellite) which we supplement with magnetic field measurements and observations of the electron/ion energy and angular distributions. The configuration of both satellites allows us to determine small-scale variations of the magnetopause shape and position and to estimate the velocity of the magnetopause motion. A preliminary analysis of the data suggests that the nature of magnetopause motion depends significantly on the geomagnetic latitude. Waxy motion of the magnetopause boundaries seems to be preferred at the low-latitude boundary layer near the equatorial plane whereas a radial expansion/contraction seems to be most common at the high latitude plasma mantle.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/1997AdSpR..20..801S}
}

@Article{Safrankova2000,
  Title                    = {The {Flank} {Magnetopause}: {Interball} {Observations}},
  Author                   = {Šafránková, J. and Němeček, Z. and Santolík, O. and Sibeck, D. G. and Zastenker, G. N. and Skalsky, A.},
  Journal                  = {Advances in Space Research},
  Year                     = {2000},
  Pages                    = {1503--1510},
  Volume                   = {25},

  Abstract                 = {The magnetopause represents a key boundary in the solar wind - magnetosphere coupling. Our analysisof corresponding INTERBALL-1 and MAGION-4 spacecraft observations of the high-latitude and flank magnetopause reveals a variety of transient processes superimposed upon a complicated boundary layer structure. The turbulent motion of the plasma compressed behind the bow shock can cause a local deformation of the magnetopause and its inward motion with respect to the mean position determined from magnetopause models. The presented statistics shows that this process prevails on the dawn magnetopause. The effects of the magnetosheath turbulence are further amplified by reconnection if the magnetic shear is high enough.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/2000AdSpR..25.1503S}
}

@Article{Safrankova1998,
  Title                    = {Two point observation of high-latitude reconnection},
  Author                   = {Šafránková, J. and Němeček, Z. and Sibeck, D. G. and Přech, L. and Měrka, J. and Santolík, O.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1998},
  Pages                    = {4301--4304},
  Volume                   = {25},

  Abstract                 = {Reconnection on the high-latitude magnetopause can produce sunward plasma flow in a portion of the lobes. This plasma should precipitate into the polar cap, poleward of the locations where magnetosheath plasma is normally found. We present two point INTERBALL observations of reconnection which is qualitatively consistent with the antiparallel merging model. Reconnection creates a plasma layer about 1R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} thick adjacent to the magnetopause (MP). Timing considerations suggest tailward motion of the reconnection site with a velocity ˜20 km/s and a reconnection site with dimensions on the order of 1 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/1998GeoRL..25.4301S}
}

@Article{Safrankova2002b,
  Title                    = {The structure of hot flow anomalies in the magnetosheath},
  Author                   = {Šafránková, J. and Přech, L. and Němeček, Z. and Sibeck, D.},
  Journal                  = {Advances in Space Research},
  Year                     = {2002},
  Pages                    = {2737--2744},
  Volume                   = {30},

  Abstract                 = {The interaction of the solar wind with the Earth's magnetosphere creates a population of backstreaming ions. When a tangential discontinuity contacts the bow shock, these ions can be focused to the discontinuity region and create so-called Hot Flow Anomalies (HFAs) - diamagnetic cavities filled with hot, tenuous, and deflected plasma population. These cavities are swept downstream and can be observed in the magnetosheath. We have analyzed INTERBALL-1 and MAGION-4 observations of magnetosheath HFAs with attention to their internal structure. We have found that HFAs often consist of two parts separated by an density enhancement. The particle behaviour can differ in these two parts. We demonstrate this peculiarity and discuss its possible origin.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/2002AdSpR..30.2737S}
}

@Article{Safrankova2000a,
  Title                    = {Magnetosheath response to the interplanetary magnetic field tangential discontinuity},
  Author                   = {Šafránková, J. and Přech, L. and Němeček, Z. and Sibeck, D. G. and Mukai, T.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2000},
  Pages                    = {25113--25122},
  Volume                   = {105},

  Abstract                 = {We present a multipoint observational study of the magnetosheath response to the interplanetary magnetic field tangential discontinuities which form hot flow anomaly-like (HFAs) structures. We identify these structures in the vicinity of the bow shock as well as deeper in the magnetosheath. Two or more points of simultaneous observations allow us to describe the gradual evolution and propagation of these HFAs through the magnetosheath. From tens of events recorded by INTERBALL-1, we present two cases. In the first, GEOTAIL identified HFAs in the solar wind near the bow shock, and INTERBALL-1 and MAGION-4 observed related events in the magnetosheath. During the second interval, all three spacecraft observed the HFA features in the magnetosheath. Our analysis of reported events suggests the negligible evolution of these structures in the magnetosheath. A survey of the INTERBALL-1 data has shown that magnetosheath HFAs are observed predominantly during periods of fast solar wind.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Interplanetary magnetic fields Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Plasma convection Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2000JGR...10525113S}
}

@Article{Saitou2012,
  Title                    = {Bow {Shock} {Formation} in a {Complex} {Plasma}},
  Author                   = {Saitou, Y. and Nakamura, Y. and Kamimura, T. and Ishihara, O.},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2012},

  Month                    = feb,
  Number                   = {6},
  Pages                    = {065004},
  Volume                   = {108},

  Doi                      = {10.1103/PhysRevLett.108.065004},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.108.065004}
}

@Article{Samir1983,
  Title                    = {The expansion of a plasma into a vacuum: {Basic} phenomena and processes and applications to space plasma physics},
  Author                   = {Samir, Uri and Wright, KH and Stone, NH},
  Journal                  = {Rev. Geophys.},
  Year                     = {1983},
  Number                   = {7},
  Pages                    = {1631--1646},
  Volume                   = {21}
}

@Article{Samsonov2006,
  Title                    = {Numerical modelling of the {Earth}{\textbackslash}rsquos magnetosheath for different {IMF} orientations},
  Author                   = {Samsonov, A.},
  Journal                  = {Advances in Space Research},
  Year                     = {2006},

  Month                    = jan,
  Pages                    = {1652--1656},
  Volume                   = {38},

  Doi                      = {10.1016/j.asr.2005.06.009}
}

@Article{Samsonov2004,
  Title                    = {Gluon condensate in charmonium sum rules for the axial-vector current},
  Author                   = {Samsonov, A.},
  Journal                  = {ArXiv High Energy Physics - Phenomenology e-prints},
  Year                     = {2004},

  Month                    = jul,

  Keywords                 = {High Energy Physics - Phenomenology}
}

@Article{Samsonov2003,
  Title                    = {Magnetic moment of the rho-meson in {QCD} sum rules: alpha$_{\textrm{s}}$-corrections},
  Author                   = {Samsonov, A.},
  Journal                  = {Journal of High Energy Physics},
  Year                     = {2003},

  Month                    = dec,
  Pages                    = {61},
  Volume                   = {12},

  Doi                      = {10.1088/1126-6708/2003/12/061},
  Keywords                 = {QCD Sum Rules}
}

@InProceedings{Samsonov2001,
  Title                    = {A self-consistent method to calculate shape of the dayside magnetopause},
  Author                   = {Samsonov, A. A.},
  Booktitle                = {Space {Plasma} {Simulation}},
  Year                     = {2001},
  Editor                   = {Büchner, J. and Dum, C. T. and Scholer, M.},
  Pages                    = {334}
}

@Article{Samsonov2011,
  Title                    = {Propagation of inclined interplanetary shock through the magnetosheath},
  Author                   = {Samsonov, A. A.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2011},

  Month                    = jan,
  Pages                    = {30--39},
  Volume                   = {73},

  Doi                      = {10.1016/j.jastp.2009.10.014}
}

@Article{Samsonov2007,
  Title                    = {Specific features of magnetic barrier formation near the magnetopause},
  Author                   = {Samsonov, A. A.},
  Journal                  = {Geomagnetism and Aeronomy},
  Year                     = {2007},

  Month                    = jun,
  Pages                    = {316--324},
  Volume                   = {47},

  Doi                      = {10.1134/S0016793207030061},
  Keywords                 = {94.30.ch}
}

@InProceedings{Samsonov2001a,
  Title                    = {Application of the {Rusanov} shock-capturing scheme for calculation of temporal variations in the {Earths} magnetosheath},
  Author                   = {Samsonov, A. A. and Hubert, D.},
  Booktitle                = {Space {Plasma} {Simulation}},
  Year                     = {2001},
  Editor                   = {Büchner, J. and Dum, C. T. and Scholer, M.},
  Pages                    = {337}
}

@Article{Samsonov2004a,
  Title                    = {Steady state slow shock inside the {Earth}'s magnetosheath: {To} be or not to be? 2. {Numerical} three-dimensional {MHD} modeling},
  Author                   = {Samsonov, A. A. and Hubert, D.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = jan,
  Pages                    = {1218},
  Volume                   = {109},

  Doi                      = {10.1029/2003JA010006},
  Keywords                 = {magnetosheath, Magnetospheric Physics: Magnetosheath, Magnetospheric Physics: MHD waves and instabilities, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Solar wind/magnetosphere interactions, numerical modeling, slow MHD shock, solar wind discontinuites, solar wind - magnetosphere interactions}
}

@Article{Samsonov2002,
  Title                    = {Temporal variations in the magnetosheath: {Comparison} between {MHD} calculations and observations for one event on {September} 17, 1978},
  Author                   = {Samsonov, A. A. and Hubert, D.},
  Journal                  = {{\textbackslash}planss},
  Year                     = {2002},

  Month                    = apr,
  Pages                    = {619--625},
  Volume                   = {50},

  Doi                      = {10.1016/S0032-0633(02)00041-7}
}

@Article{Samsonov2002a,
  Title                    = {Anisotropic {MHD} model for the magnetosheath of {Saturn}},
  Author                   = {Samsonov, A. A. and Meister, C.-V.},
  Journal                  = {{\textbackslash}planss},
  Year                     = {2002},

  Month                    = apr,
  Pages                    = {519--525},
  Volume                   = {50},

  Doi                      = {10.1016/S0032-0633(02)00030-2}
}

@Article{Samsonov2006a,
  Title                    = {Numerical {MHD} modeling of propagation of interplanetary shock through the magnetosheath},
  Author                   = {Samsonov, A. A. and Němeček, Z. and Šafránková, J.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2006},

  Month                    = aug,
  Pages                    = {8210},
  Volume                   = {111},

  Abstract                 = {Propagation of an interplanetary (IP) shock through the bow shock and magnetosheath is studied using numerical results of a three-dimensional MHD model of the magnetosheath. According to already published theoretical studies, a fast forward shock passing through the bow shock would generate a train of new discontinuities including a slow expansion wave, a contact discontinuity, and a slow reversed shock. We have found that these particular discontinuities propagate with similar velocities and thus they cannot be distinguished in our calculations, and we observe one discontinuity that combines properties of all of them. We suggest that the same would be true for an analysis of experimental data. We have simulated three different ways of the magnetopause response to the IP shock. A comparison of these runs reveals that the magnetopause reaction defines the mode of reflected waves. Assuming a fast earthward motion of the magnetopause, about 240 km s-1 or more, we obtain that a fast rarefaction wave would propagate from the magnetopause toward the bow shock, while a slower magnetopause motion would result in a fast reversed shock. On the other hand, the speed of the IP shock propagation does not depend on the magnetopause response, and all three model runs confirm a deceleration of the modeled IP shock front in the magnetosheath in course of its motion from the subsolar region to the magnetosheath flanks.},
  Doi                      = {10.1029/2005JA011537},
  Keywords                 = {Interplanetary Physics: Interplanetary shocks, Interplanetary Physics: Planetary bow shocks, interplanetary shock, magnetosheath, Magnetospheric Physics: Magnetosheath, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Solar wind/magnetosphere interactions, MHD modeling}
}

@Article{Samsonov2013,
  Title                    = {Why does the total pressure on the subsolar magnetopause differ from the solar wind dynamic pressure?},
  Author                   = {Samsonov, A. A. and Němeček, Z. and Šafránková, J. and Jelínek, K.},
  Journal                  = {Cosmic Research},
  Year                     = {2013},

  Month                    = jan,
  Pages                    = {37--45},
  Volume                   = {51},

  Doi                      = {10.1134/S0010952513010073}
}

@Article{Samsonov2012,
  Title                    = {Why does the subsolar magnetopause move sunward for radial interplanetary magnetic field?},
  Author                   = {Samsonov, A. A. and Němeček, Z. and Šafránková, J. and Jelínek, K.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2012},

  Month                    = may,
  Pages                    = {5221},
  Volume                   = {117},

  Doi                      = {10.1029/2011JA017429},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers, Magnetospheric Physics: Magnetosheath, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Plasma waves and instabilities (2471), Magnetospheric Physics: Solar wind/magnetosphere interactions}
}

@InProceedings{Samsonov2004b,
  Title                    = {Numerical modelling of the solar wind - magnetosphere interaction for different {IMF} orientations},
  Author                   = {Samsonov, A. A. and Pudovkin, M. I.},
  Booktitle                = {35th {COSPAR} {Scientific} {Assembly}},
  Year                     = {2004},
  Editor                   = {Paillé, J.-P.},
  Pages                    = {1060},
  Series                   = {{COSPAR} {Meeting}},
  Volume                   = {35}
}

@Article{Samsonov2000,
  Title                    = {Application of the bounded anisotropy model for the dayside magnetosheath},
  Author                   = {Samsonov, A. A. and Pudovkin, M. I.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {2000},

  Month                    = jun,
  Pages                    = {12859--12868},
  Volume                   = {105},

  Doi                      = {10.1029/2000JA900009},
  Keywords                 = {Magnetospheric Physics: Magnetosheath, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Plasma waves and instabilities, Magnetospheric Physics: Solar wind/magnetosphere interactions}
}

@Article{Samsonov2001b,
  Title                    = {Anisotropic {MHD} model of the dayside magnetosheath downstream of the oblique bow shock},
  Author                   = {Samsonov, A. A. and Pudovkin, M. I. and Gary, S. P. and Hubert, D.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {2001},

  Month                    = oct,
  Pages                    = {21689--21700},
  Volume                   = {106},

  Doi                      = {10.1029/2000JA900150},
  Keywords                 = {Magnetospheric Physics: Magnetosheath, Magnetospheric Physics: MHD waves and instabilities, Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Plasma waves and instabilities}
}

@Article{Samsonov2013a,
  Title                    = {Large-scale flow vortices following a magnetospheric sudden impulse},
  Author                   = {Samsonov, A. A. and Sibeck, D. G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},
  Pages                    = {3055--3064},
  Volume                   = {118},

  Abstract                 = {Global MHD simulations predict the generation of flow vortices on the magnetospheric flanks near the equatorial plane after the impact of solar wind dynamic pressure pulses on the magnetosphere. These vortices are associated with field-aligned currents, having similar senses to those responsible for the main impulse, i.e., the second impulse of the well-known sudden impulse variations at high geomagnetic latitudes. We investigate the evolution of the vortices and show that they result from the interaction of a fast MHD wave and the inner (near-Earth) boundary of numerical models. Near the inner boundary, the Ampere force decelerates plasma flow resulting in two closely related phenomena: the generation of flow vortices and the launch of a reflected fast wave moving sunward. The vortices propagate antisunward and split into several parts during several minutes. The reflected wave interacts with the magnetopause and bow shock and changes its velocity. The interaction between the reflected wave and bow shock results in two new discontinuities moving earthward through the magnetosheath. The first is either a very weak fast rarefaction wave or a weak fast shock, and the second is either a tangential discontinuity or a compound discontinuity with a decrease of the density and magnetic field and an increase of the temperature. We speculate that the inner boundary in simulations may correspond to either the plasmasphere or ionosphere.},
  ISSN                     = {0148-0227},
  Keywords                 = {sudden impulse flow vortices MHD discontinuities},
  Url                      = {http://adsabs.harvard.edu/abs/2013JGRA..118.3055S}
}

@Article{Samsonov2013b,
  Title                    = {Large-scale flow vortices following a magnetospheric sudden impulse},
  Author                   = {Samsonov, A. A. and Sibeck, D. G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = jun,
  Pages                    = {3055--3064},
  Volume                   = {118},

  Doi                      = {10.1002/jgra.50329},
  Keywords                 = {flow vortices, MHD discontinuities, sudden impulse}
}

@Article{Samsonov2007a,
  Title                    = {Magnetospheric {Variations} {Resulting} {From} the {Propagation} of an {Interplanetary} {Shock}},
  Author                   = {Samsonov, A. A. and Sibeck, D. G.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2007},

  Month                    = dec,
  Pages                    = {A315},

  Keywords                 = {2139 Interplanetary shocks, 2736 Magnetosphere/ionosphere interactions (2431), 2740 Magnetospheric configuration and dynamics, 2753 Numerical modeling, 2784 Solar wind/magnetosphere interactions}
}

@Article{Samsonov2010,
  Title                    = {An event of interplanetary shock - magnetosphere interaction: {Comparison} between spacecraft observations and {MHD} modeling},
  Author                   = {Samsonov, A. A. and Sibeck, D. G. and Chen, S. and Singer, H. J. and Biernat, H. K. and Zolotova, N.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2010},

  Month                    = dec,
  Pages                    = {B1799},

  Keywords                 = {[2139] INTERPLANETARY PHYSICS / Interplanetary shocks, [2752] MAGNETOSPHERIC PHYSICS / MHD waves and instabilities, [2753] MAGNETOSPHERIC PHYSICS / Numerical modeling, [2784] MAGNETOSPHERIC PHYSICS / Solar wind/magnetosphere interactions}
}

@Article{Samsonov2007b,
  Title                    = {{MHD} simulation for the interaction of an interplanetary shock with the {Earth}'s magnetosphere},
  Author                   = {Samsonov, A. A. and Sibeck, D. G. and Imber, J.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2007},
  Pages                    = {12220},
  Volume                   = {112},

  Abstract                 = {The global BATS-R-US MHD code is used to simulate the interaction of a moderately strong interplanetary shock with the Earth's magnetosphere. The model predicts the propagation of a transmitted fast shock through the magnetosheath and magnetosphere and the reflection of this shock from the inner numerical boundary. The reflected fast shock propagates sunward through the dayside magnetosphere and magnetosheath. The passage of the transmitted shock causes the bow shock and magnetopause to move inward, while the passage of the reflected fast shock causes these boundaries to move outward, consistent with previously reported in situ observations. A supplementary study employing a one-dimensional MHD model addresses the interaction of the forward fast shock with the plasmapause. This study demonstrates that most of the energy associated with the fast shock energy penetrates into the plasmasphere. Consequently, the transmitted fast wave must reach the ionosphere, produce the well known sudden impulse signatures, and then be reflected due to the shielding effects of ionospheric currents. The predictions of the numerical simulations are consistent with observations of the dayside geosynchronous magnetic field.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Interplanetary Physics: Interplanetary shocks Magnetospheric Physics: Numerical modeling Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetic storms and substorms (7954)},
  Url                      = {http://adsabs.harvard.edu/abs/2007JGRA..11212220S}
}

@Article{Samsonov2014,
  Title                    = {Sudden impulse observations in the dayside magnetosphere by {THEMIS}},
  Author                   = {Samsonov, A. A. and Sibeck, D. G. and Walsh, B. M. and Zolotova, N. V.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2014},
  Pages                    = {9476--9496},
  Volume                   = {119},

  Abstract                 = {We present a study of the magnetospheric response to interplanetary shocks. We show eight events with simultaneous observations of sudden impulses in the dayside magnetosphere and interplanetary shocks in the solar wind. The spacecraft measurements in the equatorial plane, even those very close to the Earth, can be interpreted in terms of the vortices predicted by previous studies employing global MHD models. In fact, these vortices are velocity oscillations with the properties of Alfvén waves. The amplitude and frequency of the oscillations depend on radial distance from the Earth. The amplitude of the velocity perturbations decreases with increase of the density and magnetic field magnitude, but the velocity amplitude shows no dependence on magnitude of the solar wind dynamic pressure change attending the interplanetary shocks. The oscillations are observed both in the outer magnetosphere and the plasmasphere, but they become less sinusoidal near the plasmapause, i.e., in the region with a large-density gradient. The amplitude of the magnetic field enhancement in the sudden impulses also depends on the radial distance. The MHD simulations successfully predict the amplitudes of magnetic field increase and the first cycles of the velocity oscillations in these events.},
  ISSN                     = {0148-0227},
  Keywords                 = {sudden impulse THEMIS interplanetary shock global MHD simulation velocity oscillations},
  Url                      = {http://adsabs.harvard.edu/abs/2014JGRA..119.9476S}
}

@Article{Samsonov2010a,
  Title                    = {Transient changes in magnetospheric-ionospheric currents caused by the passage of an interplanetary shock: {Northward} interplanetary magnetic field case},
  Author                   = {Samsonov, A. A. and Sibeck, D. G. and Yu, Yiqun},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2010},
  Pages                    = {5207},
  Volume                   = {115},

  Abstract                 = {We use results from a global MHD simulation to study the interaction of an interplanetary shock with the Earth's magnetosphere for a northward interplanetary magnetic field orientation. We connect intensifications of the transient northward Bz (NBZ) and Region 1 currents in the ionosphere with the appearance of two strong dynamo regions in the magnetosphere: the first on the high-latitude magnetopause near and behind the cusps and the second near the equatorial plane on the flanks. The ionospheric and magnetospheric transients are well synchronized and move antisunward gradually. According to the results obtained, the source of energy for the transient NBZ current is related to shock-intensified lobe reconnection, while the transient Region 1 current corresponds to the reflected fast shock predicted by Samsonov et al. (2007). We speculate that the electric circuits for the quasi-stationary field-aligned currents are similar to the transient electric circuits obtained in this paper.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Field-aligned currents and current systems (2409) Interplanetary Physics: Interplanetary shocks Magnetospheric Physics: Numerical modeling Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetosphere/ionosphere interactions (2431)},
  Url                      = {http://adsabs.harvard.edu/abs/2010JGRA..115.5207S}
}

@Article{Samsonov2011a,
  Title                    = {Propagation of a sudden impulse through the magnetosphere initiating magnetospheric {Pc}5 pulsations},
  Author                   = {Samsonov, A. A. and Sibeck, D. G. and Zolotova, N. V. and Biernat, H. K. and Chen, S.-H. and Rastaetter, L. and Singer, H. J. and Baumjohann, W.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2011},
  Pages                    = {10216},
  Volume                   = {116},

  Abstract                 = {We compare multipoint observations of an interplanetary shock's interaction with the Earth's magnetosphere on 29 July 2002 with results from global MHD simulations. The sudden impulse associated with the shock's arrival initiates global ultralow-frequency waves with periods from 2 to 5 min. We interpret four cycles of Bz oscillations with T = ˜3 min at Geotail in the postdawn magnetosphere as radial magnetopause oscillations. GOES 8, in the same late morning sector, observed compressional and toroidal waves with the same frequency at the same time. GOES 10, in the early morning sector, observed toroidal waves with a slightly lower period. We suggest that these observations confirm the mode coupling theory. The interplanetary shock initiates compressional magnetospheric waves which, according to our estimates, oscillate between the ionosphere and magnetopause and gradually convert their energy into that of standing Alfven waves. At the same time, Polar in the outer predawn magnetosphere observed strong velocity oscillations and weak magnetic field oscillations with a ˜4 min period. Global MHD models successfully predict these oscillations and connect them to the Kelvin-Helmholtz instability which results in large flow vortices with sizes of about ten Earth radii. However, the global models do not predict the multiple compressional oscillations with the observed periods and therefore cannot readily explain the GOES observations.},
  ISSN                     = {0148-0227},
  Keywords                 = {Kelvin-Helmholtz instability Pc5 waves global MHD models sudden impulse Interplanetary Physics: Interplanetary shocks Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: MHD waves and instabilities (2149 6050 7836) Magnetospheric Physics: Numerical modeling Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2011JGRA..11610216S}
}

@InProceedings{Samsonov2014a,
  Title                    = {Variations of the total pressure through the magnetosheath},
  Author                   = {Samsonov, A. and Jelinek, K. and Nemecek, Z. and Safrankova, J.},
  Booktitle                = {40th {COSPAR} {Scientific} {Assembly}},
  Year                     = {2014},
  Pages                    = {2859},
  Series                   = {{COSPAR} {Meeting}},
  Volume                   = {40}
}

@Article{Samsonov2013c,
  Title                    = {Why does the total pressure on the subsolar magnetopause differ from the solar wind dynamic pressure?},
  Author                   = {Samsonov, AA and Němeček, Z and Šafránková, J and Jelínek, K},
  Journal                  = {Cosmic Research},
  Year                     = {2013},
  Number                   = {1},
  Pages                    = {37--45},
  Volume                   = {51}
}

@Article{Samsonov2004c,
  Title                    = {Why {Does} the {Plasma} {Depletion} {Layer} {Exist} {Near} the {Magnetopause}?},
  Author                   = {Samsonov, A. and Salem, C.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2004},

  Month                    = dec,
  Pages                    = {B367},

  Keywords                 = {2728 Magnetosheath, 2753 Numerical modeling, 2784 Solar wind/magnetosphere interactions, 2799 General or miscellaneous, 7827 Kinetic and MHD theory}
}

@Article{Samsonov1997,
  Title                    = {Comment on “{Pionic} decay of a possible d' dibaryon and the short-range {NN} interaction”},
  Author                   = {Samsonov, A. and Schepkin, M.},
  Journal                  = {ArXiv Nuclear Theory e-prints},
  Year                     = {1997},

  Month                    = dec,

  Keywords                 = {Nuclear Theory}
}

@InProceedings{Samsonov2014b,
  Title                    = {Sudden impulse observations in the dayside magnetosphere by {THEMIS}},
  Author                   = {Samsonov, A. and Sibeck, D. and Angelopoulos, V.},
  Booktitle                = {40th {COSPAR} {Scientific} {Assembly}},
  Year                     = {2014},
  Pages                    = {2858},
  Series                   = {{COSPAR} {Meeting}},
  Volume                   = {40}
}

@Article{Samsonov2006b,
  Title                    = {Modeling the interaction of interplanetary shocks with the {Earth}'s magnetosphere: {The} first three steps},
  Author                   = {Samsonov, A. and Sibeck, D. and Nemecek, Z. and Safrankova, J.},
  Journal                  = {AGU Fall Meeting Abstracts},
  Year                     = {2006},

  Month                    = dec,
  Pages                    = {D2},

  Keywords                 = {2139 Interplanetary shocks, 2154 Planetary bow shocks, 2728 Magnetosheath, 2753 Numerical modeling, 2784 Solar wind/magnetosphere interactions}
}

@Article{Samsonov1981,
  Title                    = {Temporal {Evolution} of the {Energy} {Spectrum} of {Ultrarelativistic} {Electrons} {Under} the {Action} of {Synchrotron} {Losses} and {Turbulent} {Acceleration}},
  Author                   = {Samsonov, A. M. and Fedorenko, V. N.},
  Journal                  = {{\textbackslash}sovast},
  Year                     = {1981},

  Month                    = feb,
  Pages                    = {72--76},
  Volume                   = {25}
}

@InProceedings{Samsonov2008,
  Title                    = {On {Modeling} of {Gene} {Expression} {Patterns} in the {Drosophila} {Embryo} by the {Gene} {Circuit} {Method}},
  Author                   = {Samsonov, A. M. and Gursky, V. V. and Kozlov, K. N. and Reinitz, J.},
  Booktitle                = {Latest {Advances} in {Atomic} {Cluster} {Collisions}: {Structure} and {Dynamics} from the {Nuclear} to the {Biological} {Scale}},
  Year                     = {2008},
  Editor                   = {Connerade, J.-P. and Solov'yov, A.},
  Pages                    = {426}
}

@Article{Samsonov2005,
  Title                    = {Magnetic moment of the ρ meson in {QCD} sum rules},
  Author                   = {Samsonov, A. V.},
  Journal                  = {Phys. At. Nucl.},
  Year                     = {2005},

  Month                    = jan,
  Pages                    = {114--118},
  Volume                   = {68},

  Doi                      = {10.1134/1.1858564}
}

@Article{Samsonov1998,
  Title                    = {Decay constant of eta-meson from {QCD} sum rule},
  Author                   = {Samsonov, A. V.},
  Journal                  = {ArXiv High Energy Physics - Phenomenology e-prints},
  Year                     = {1998},

  Month                    = jul,

  Keywords                 = {High Energy Physics - Phenomenology}
}

@Article{Samsonov1998a,
  Title                    = {{QED} amplitude of the forward scattering of a virtual longitudinal photon},
  Author                   = {Samsonov, A. V.},
  Journal                  = {Phys. At. Nucl.},
  Year                     = {1998},

  Month                    = dec,
  Pages                    = {2119--2122},
  Volume                   = {61}
}

@Article{Samsonov1998b,
  Title                    = {Oceanic plateau model for continental crustal growth in the {Archaean}: {A} case study from the {Kostomuksha} greenstone belt, {NW} {Baltic} {Shield}},
  Author                   = {Samsonov, A. V. and Shchipansky, A. A. and Jochum, K. P. and Mezger, K. and Hofmann, A. W. and Puchtel, I. S.},
  Journal                  = {Earth Planet. Sci. Lett.},
  Year                     = {1998},

  Month                    = feb,
  Pages                    = {57--74},
  Volume                   = {155}
}

@Article{Samsonov2006c,
  Title                    = {Relation of solar wind parameters to high-latitude magnetic pulsations},
  Author                   = {Samsonov, S. N. and Plotnikov, I. Ya. and Sibeck, D. Y. and Watermann, Yu.},
  Journal                  = {Kosmichna Nauka i Tekhnologiya},
  Year                     = {2006},
  Pages                    = {80--84},
  Volume                   = {12},

  Abstract                 = {Magnetometric data of north-American and Greenland station chains are compared with measurements of plasma parameters and magnetic fields aboard the IMP-8, ISEE-1.2, GEOS-5.6 and IRM. For the sign-changeable IMF Bz-component having the oscillation form in the range of 5 to 20 min and with a regular amplitude of about 5 nT on October 29, 1985 the cross-correlation relationship to dayside high-latitude pulsations of the ground magnetic field is revealed. On the three station chains in the near noon sector of 9-15 LT we obtained the latitude-longitudinal distribution of oscillation phases which is the correspondence with the inclined and quasi-field aligned propagation of Alfvén waves in different parts of the magnetosphere. The inclined phase oscillation fronts are formed in the 10-14 LT sector in the region of maximum dispersion of lengths of geomagnetic force lines. It is supposed that in this intermediate region between Alfvén waves falling (running away) on the subauroral ionosphere and Alfvén waves running (falling) from the polar cap at southern (northern) IMF the power-exchangeable process which is typical for the entry layer in the magnetopause takes place. Perhaps, in this case the pulsations penetrating from solar wind into the magnetosphere are the earlier unknown manifestation of the magnetopause reaction to the IMF fluctuations. In the oscillation sense the reaction is reversible when the sign of Bz-component changes in the above-mentioned range of periods.},
  Keywords                 = {Space Technology},
  Url                      = {http://adsabs.harvard.edu/abs/2006KosNT..12a..80S}
}

@Article{Sanny1998,
  Title                    = {A statistical study of the magnetic signatures of {FTEs} near the dayside magnetopause},
  Author                   = {Sanny, J. and Beck, C. and Sibeck, D. G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1998},
  Pages                    = {4683--4692},
  Volume                   = {103},

  Abstract                 = {During magnetopause crossings, the AMPTE CCE satellite frequently observed flux transfer events (FTEs) characterized by fluctuations in the magnetic field strength (B) and bipolar signatures in the field component (B{\textless}SUB{\textgreater}N{\textless}/SUB{\textgreater}) normal to the nominal magnetopause. In this study, we survey 110 events observed from October to December 1984 and during January 1986. Nearly all events exhibited increases in B, and although the majority of events exhibited a symmetric bipolar signature in B{\textless}SUB{\textgreater}N{\textless}/SUB{\textgreater}, a significant number (31 of 110) had asymmetric bipolar signatures in which the trailing pulse was dominant. Most of the asymmetric events were observed near the magnetic equator. This is consistent with an explanation in which FTEs form via merging along a single subsolar X line with strongly asymmetric signatures but that these signatures evolve into the familiar symmetric bipolar form with distance from the merging line.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Solar wind/magnetosphere interactions Space Plasma Physics: Magnetic reconnection},
  Url                      = {http://adsabs.harvard.edu/abs/1998JGR...103.4683S}
}

@Article{Sanny2001,
  Title                    = {A statistical study of transient event motion at geosynchronous orbit},
  Author                   = {Sanny, J. and Berube, D. and Sibeck, D. G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2001},
  Pages                    = {21217--21230},
  Volume                   = {106},

  Abstract                 = {The geosynchronous GOES 5 and GOES 6 satellites frequently observe transient events marked by magnetic field strength increases and bipolar magnetic field signatures lasting several minutes. In this study we report a survey of 87 events observed simultaneously by both GOES spacecraft (for a total of 174 individual observations) from August to December 1984. Events detected in the prenoon sector outnumbered those in the postnoon sector by about a 3 to 1 ratio. The distribution of the events versus local time exhibited a significant prenoon peak like the distribution of magnetic impulse events observed in high-latitude ground magnetometers. A cross-correlation analysis of the two GOES data sets indicated lags that range from 0 to over 2 min, with the majority of the events moving antisunward. The short lags correspond to azimuthal speeds of hundreds of kilometers per second, greater than flow speeds in the magnetosheath, but less than fast mode waves. The short lags may indicate that the events move primarily latitudinally and/or that transient events are seldom localized, but rather occur over extended, if not global, regions. Investigations of event occurrence versus interplanetary magnetic field (IMF) B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater}, event motion versus IMF B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater}, and correspondence between upstream plasma data and the events all indicate that pressure pulses are the likely source of many of the events. About 27\% of the events with simultaneous solar wind data were preceded by sharp reversals in one or more IMF components, and nearly all of this particular group of events occurred in the dawn sector. This suggests that the pressure pulses may be commonly generated in the foreshock/bow shock region, since the prenoon magnetopause lies generally behind the quasi-parallel bow shock where such pulses are thought to be triggered by IMF discontinuities. Finally, several events in the data set were also observed by the AMPTE/CCE. These are presented as case studies.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetosphere/ionosphere interactions Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Solar wind interactions with unmagnetized bodies},
  Url                      = {http://adsabs.harvard.edu/abs/2001JGR...10621217S}
}

@Article{Sanny2007,
  Title                    = {Global profiles of compressional ultralow frequency wave power at geosynchronous orbit and their response to the solar wind},
  Author                   = {Sanny, J. and Judnick, D. and Moldwin, M. B. and Berube, D. and Sibeck, D. G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2007},
  Pages                    = {5224},
  Volume                   = {112},

  Abstract                 = {We investigate the global local-time profiles of compressional wave power in three ultralow frequency (ULF) bands corresponding to Pc3, Pc4, and Pc5 pulsations using magnetic field data from the geosynchronous GOES satellites. The global power profiles of the three frequency bands are studied for low, moderate, and high levels of geomagnetic activity based on the Dst index. We also consider the seasonal variation of the ULF power profiles, as well as the effects of solar wind and interplanetary magnetic field (IMF) parameters. For high geomagnetic activity, we find that the greatest power is associated with compressional Pc5 pulsations in the afternoon sector; for low geomagnetic activity, ULF power levels are consistently highest in the tail region. A summer power minimum in all three frequency bands is observed in our study of seasonal variation, while higher power levels occur around local midnight throughout the year. The enhancement of ULF power by high solar wind velocity and pressure is greater for the lower-frequency waves. Furthermore, solar wind plasma parameters have a significantly greater influence on ULF wave power than IMF parameters like cone angle and northward/southward orientation.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Plasma waves and instabilities (2471) Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetic storms and substorms (7954) ULF waves global power profile solar wind},
  Url                      = {http://adsabs.harvard.edu/abs/2007JGRA..112.5224S}
}

@Article{Sanny1996,
  Title                    = {A statistical study of transient events in the outer dayside magnetosphere},
  Author                   = {Sanny, J. and Sibeck, D. G. and Venturini, C. C. and Russell, C. T.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1996},
  Pages                    = {4939--4952},
  Volume                   = {101},

  Abstract                 = {The AMPTE CCE satellite frequently observed transient (1{\textless}=τ{\textless}=8 min) events marked by magnetic field strength increases and bipolar magnetic field signatures (peak-to-peak amplitudes {\textgreater}=4 nT) while in the outer dayside magnetosphere. We report a survey of 59 prominent events observed from August to November 1984. The bipolar signatures and minimum variance analysis reveal that most events move poleward and antisunward, except in the immediate vicinity of local noon. Here the motion of the events appears to be better governed by the spiral/orthospiral interplanetary magnetic field (IMF) orientation than magnetic curvature forces associated with IMF B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater}. The IMF orientation appears to have little or no influence on event occurrence or orientation. We interpret the events in terms of solar wind/foreshock pressure pulse induced ripples on the magnetopause surface. Our results can be reconciled with those obtained in previous studies which made use of ISEE 1/2, AMPTE IRM, and AMPTE UKS observations if pressure pulses produce large-amplitude events and bursty merging (or reconnection) produces small-amplitude events.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Solar wind/magnetosphere interactions Space Plasma Physics: Magnetic reconnection},
  Url                      = {http://adsabs.harvard.edu/abs/1996JGR...101.4939S}
}

@Article{Sanny2002,
  Title                    = {Quiet time variability of the geosynchronous magnetic field and its response to the solar wind},
  Author                   = {Sanny, J. and Tapia, J. A. and Sibeck, D. G. and Moldwin, M. B.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2002},
  Pages                    = {1443},
  Volume                   = {107},

  Abstract                 = {We present a survey of the variability of the geosynchronous magnetic field strength on the dayside using observations by the GOES satellites over a period exceeding 4 years. Only intervals of reduced geomagnetic activity, as defined by Dst {\textgreater} -20 nT, were considered in this study. The magnetic field strength data were filtered with a passband of 1.7 mHz to 17 mHz (1-10 minutes), a process that eliminates the diurnal variation of the field strength and the effects of most of the higher frequency ({\textgreater}17 mHz) ultralow-frequency (ULF) waves. The geosynchronous field strength appears to exhibit the greatest variability in the prenoon sector for spiral interplanetary magnetic fields (IMF) and in the postnoon sector for orthospiral IMF, suggesting that pressure pulses generated in the foreshock/bow shock region may have a significant influence on the geosynchronous field. The seasonal dependence of the variability was determined to be positively correlated to the seasonal dependence of ground-based observations of magnetic impulse events. The response of the variability of the geosynchronous magnetic field strength around local noon to solar wind parameters was also studied. Here, we observed that the variability was strongly affected by changes in the solar wind dynamic pressure but was seemingly independent of the northward/southward direction of the interplanetary magnetic field. However, for high solar wind dynamic pressures, the variability was found to be greater for northward IMF than for southward IMF.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: MHD waves and instabilities Space Plasma Physics: Magnetic reconnection Magnetospheric Physics: Magnetosphere-outer variability solar wind geosynchronous magnetic field dynamic pressure IMF},
  Url                      = {http://adsabs.harvard.edu/abs/2002JGRA..107.1443S}
}

@Article{Santolik2003,
  Title                    = {Transverse dimensions of chorus in the source region},
  Author                   = {Santolík, O and Gurnett, DA},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2003},
  Number                   = {2},
  Volume                   = {30}
}

@Article{Santos2014,
  Title                    = {Three-dimensional {MHD} simulation of {FTEs} produced by merging at an isolated point in a sheared magnetic field configuration},
  Author                   = {Santos, J. C. and Sibeck, D. G. and Büchner, J. and Gonzalez, W. D. and Ferreira, J. L.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2014},
  Pages                    = {2009--2023},
  Volume                   = {119},

  Abstract                 = {We present predictions for the evolution of FTEs generated by localized bursts of reconnection on a planar magnetopause that separates a magnetosheath region of high densities and weak magnetic field from a magnetospheric region of low densities and strong magnetic field. The magnetic fields present a shear angle of 105 degrees. Reconnection forms a pair of FTEs each crossing the magnetopause in the field reversal region and bulging into the magnetosphere and magnetosheath. At their initial stage they can be characterized as flux tubes since the newly reconnected magnetic field lines are not twisted. Reconnection launches Alfvenic perturbations that propagate along the FTEs generating high-speed jets, which move the pair of FTEs in opposite directions. As the FTE moves, it displaces the ambient magnetic field and plasma producing bipolar magnetic field and plasma velocity signatures normal to the nominal magnetopause in the regions surrounding the FTE. The combination of the ambient plasma with the FTE flows generates a vortical velocity pattern around the reconnected field lines. During its evolution the FTE evolves to a flux rope configuration due to the twist of the magnetic field lines. The alfvenic perturbations propagate faster along the part of the FTE bulging into the magnetosphere than in the magnetosheath, and due to the differences between the plasma and magnetic field properties the perturbations have slightly different signatures in the two regions. As a consequence, the FTEs have different signatures depending on whether the satellite encounters the part bulging into the magnetosphere or into the magnetosheath.},
  ISSN                     = {0148-0227},
  Keywords                 = {flux transfer events magnetic reconnection magnetospheric configuration and dynamics solar wind/magnetosphere interactions numerical modeling},
  Url                      = {http://adsabs.harvard.edu/abs/2014JGRA..119.2009S}
}

@Article{Santos-Lima2012,
  Title                    = {The role of turbulent magnetic reconnection in the formation of rotationally supported protostellar disks},
  Author                   = {Santos-Lima, R. and Dal Pino, EM de Gouveia and Lazarian, A.},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2012},
  Number                   = {1},
  Pages                    = {21},
  Volume                   = {747},

  Url                      = {http://iopscience.iop.org/0004-637X/747/1/21},
  Urldate                  = {2014-05-31}
}

@Article{Sanz-Forcada2011,
  Title                    = {Estimation of the {XUV} radiation onto close planets and their evaporation},
  Author                   = {Sanz-Forcada, J. and Micela, G. and Ribas, I. and Pollock, A. M. T. and Eiroa, C. and Velasco, A. and Solano, E. and Garc√≠a-√Ålvarez, D.},
  Journal                  = {{\textbackslash}textbackslashaap},
  Year                     = {2011},

  Month                    = aug,
  Pages                    = {A6},
  Volume                   = {532},

  Doi                      = {10.1051/0004-6361/201116594},
  Keywords                 = {astrobiology, planetary systems, stars: coronae, X-rays: stars}
}

@Article{Sarafopoulos2000,
  Title                    = {Energetic proton and electron dispersion signatures in the nightside magnetosheath supporting their leakage out of the magnetopause},
  Author                   = {Sarafopoulos, D. V. and Athanasiu, M. A. and Sibeck, D. G. and McEntire, R. W. and Sarris, E. T. and Kokubun, S.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2000},
  Pages                    = {15729--15740},
  Volume                   = {105},

  Abstract                 = {Energetic proton and electron dispersion structures are detected at both the dawn and dusk nightside magnetosheath near the equatorial plane using the Geotail Energetic Particles and Ion Composition instrument data. A common feature of all the exhibited examples is that the vector magnetic field progressively scans from northward to southward through all the latitude angles while remaining almost within a plane intersecting the nightside magnetopause. For such geometries, at the duskside magnetosheath, peaks in the energetic electron flux precede those in the proton, whereas the opposite occurs at the dawnside magnetosheath. The peak fluxes of energetic protons (electrons) are measured at the duskside (dawnside) magnetosheath whenever the vector magnetic field points toward the central dusk (dawn) low-latitude boundary layer (LLBL) region of the magnetosphere. Therefore we infer that the energetic electron (proton) source is essentially spatially limited to the central dawn (dusk) LLBL. We interpret the observed dispersion structures as spatial phenomena: Energetic electrons (protons) leak out from-the equatorial dawn (dusk) LLBL and then are channeled along the draped magnetic field lines over the magnetopause toward spacecraft on the duckside (dawnside). The energetic electrons (protons) are detected in the duskside (dawnside) magnetosheath for a larger range of magnetic field latitude angles. In conclusion, the leakage of energetic particles through the magnetopause seems to be a process of great importance, in parallel with the merging one.},
  ISSN                     = {0148-0227},
  Keywords                 = {magnetospheric physics},
  Url                      = {http://adsabs.harvard.edu/abs/2000JGR...10515729S}
}

@Article{Sartoretti1999,
  Title                    = {On the detection of satellites of extrasolar planets with the method of transits},
  Author                   = {Sartoretti, P. and Schneider, J.},
  Journal                  = {{\textbackslash}textbackslashaaps},
  Year                     = {1999},

  Month                    = feb,
  Pages                    = {553--560},
  Volume                   = {134},

  Doi                      = {10.1051/aas:1999148},
  Keywords                 = {PLANETS AND SA‚Ñ°LITES: GENERAL, Stars: Planetary Systems, TECHNIQUES: PHOTOMETRIC}
}

@Article{Sato2009,
  Title                    = {Effects of {Mutual} {Transits} by {Extrasolar} {Planet}-{Companion} {Systems} on {Light} {Curves}},
  Author                   = {Sato, M. and Asada, H.},
  Journal                  = {{\textbackslash}textbackslashpasj},
  Year                     = {2009},

  Month                    = aug,
  Pages                    = {L29},
  Volume                   = {61},

  Doi                      = {10.1093/pasj/61.4.L29},
  Keywords                 = {eclipses, occultations, planets and satellites: general, Stars: Planetary Systems, TECHNIQUES: PHOTOMETRIC}
}

@Article{Sauer2003,
  Title                    = {Oscillitons and gyrating ions in a beam-plasma system},
  Author                   = {Sauer, K. and Dubinin, E.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {2003},

  Month                    = dec,
  Pages                    = {2192},
  Volume                   = {30},

  Doi                      = {10.1029/2003GL018266},
  Keywords                 = {Interplanetary Physics: Energetic particles, Interplanetary Physics: MHD waves and turbulence, Magnetospheric Physics: MHD waves and instabilities, Magnetospheric Physics: Numerical modeling, planetary}
}

@Article{Sauvage2007,
  Title                    = {Remote sensed and in situ constraints on processes affecting tropical tropospheric ozone},
  Author                   = {Sauvage, B. and Martin, R. V. and Donkelaar, A. van and Liu, X. and Chance, K. and Jaegl‚Äö√†√∂¬¨¬©, L. and Palmer, P. I. and Wu, S. and Fu, T.-M.},
  Journal                  = {Atmos. Chem. Phys.},
  Year                     = {2007},
  Number                   = {3},
  Pages                    = {815--838},
  Volume                   = {7},

  Url                      = {http://www.atmos-chem-phys.net/7/815/2007/acp-7-815-2007.html?FrameEngine=false},
  Urldate                  = {2014-11-13}
}

@Article{Savoini2013,
  Title                    = {On the origin of the quasi-perpendicular ion foreshock: {Full}-particle simulations},
  Author                   = {Savoini, P. and Lembege, B. and Stienlet, J.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = mar,
  Pages                    = {1132--1145},
  Volume                   = {118},

  Doi                      = {10.1002/jgra.50158},
  Keywords                 = {acceleration, ion foreshock, shock wave}
}

@Article{Scarf1981,
  Title                    = {Plasma wave turbulence at planetary bow shocks},
  Author                   = {Scarf, FL and Gurnett, DA and Kurth, WS},
  Journal                  = {Nature},
  Year                     = {1981},
  Number                   = {5825},
  Pages                    = {747--750},
  Volume                   = {292}
}

@Article{Schaefer2004,
  Title                    = {A thermodynamic model of high temperature lava vaporization on {Io}},
  Author                   = {Schaefer, L. and Fegley, B.},
  Journal                  = {ƒ±carus},
  Year                     = {2004},

  Month                    = may,
  Pages                    = {216--241},
  Volume                   = {169},

  Doi                      = {10.1016/j.icarus.2003.08.023}
}

@Article{Schaefer2012,
  Title                    = {Vaporization of the {Earth}: {Application} to {Exoplanet} {Atmospheres}},
  Author                   = {Schaefer, L. and Lodders, K. and Fegley, B.},
  Journal                  = {{\textbackslash}textbackslashapj},
  Year                     = {2012},

  Month                    = aug,
  Pages                    = {41},
  Volume                   = {755},

  Doi                      = {10.1088/0004-637X/755/1/41},
  Keywords                 = {astrochemistry, atmospheric effects, planets and satellites: general}
}

@Book{Scherer2005,
  Title                    = {Space {Weather}: {The} physics behind a slogan},
  Author                   = {Scherer, Klaus},
  Publisher                = {Springer},
  Year                     = {2005},
  Volume                   = {656}
}

@Book{Schindler2006,
  Title                    = {Physics of space plasma activity},
  Author                   = {Schindler, Karl},
  Publisher                = {Cambridge University Press},
  Year                     = {2006}
}

@Article{Schindler1993,
  Title                    = {On the cause of thin current sheets in the near-{Earth} magnetotail and their possible significance for magnetospheric substorms},
  Author                   = {Schindler, K and Birn, J},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1993},
  Number                   = {A9},
  Pages                    = {15477--15485},
  Volume                   = {98}
}

@Article{Schmelz2012,
  Title                    = {Composition of the {Solar} {Corona}, {Solar} {Wind}, and {Solar} {Energetic} {Particles}},
  Author                   = {Schmelz, J. T. and Reames, D. V. and von Steiger, R. and Basu, S.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2012},

  Month                    = aug,
  Pages                    = {33},
  Volume                   = {755},

  Doi                      = {10.1088/0004-637X/755/1/33},
  Keywords                 = {Solar Wind, Sun: abundances, Sun: corona, Sun: helioseismology, Sun: Particle Emission, Sun: photosphere}
}

@Article{Schmelz2012a,
  Title                    = {Composition of the {Solar} {Corona}, {Solar} {Wind}, and {Solar} {Energetic} {Particles}},
  Author                   = {Schmelz, J. T. and Reames, D. V. and von Steiger, R. and Basu, S.},
  Journal                  = {{\textbackslash}textbackslashapj},
  Year                     = {2012},

  Month                    = aug,
  Pages                    = {33},
  Volume                   = {755},

  Doi                      = {10.1088/0004-637X/755/1/33},
  Keywords                 = {Solar Wind, Sun: abundances, Sun: corona, Sun: helioseismology, Sun: Particle Emission, Sun: photosphere}
}

@Article{Schoeffler2012,
  Title                    = {Scaling of the growth rate of magnetic islands in the heliosheath},
  Author                   = {Schoeffler, K. M. and Drake, J. F. and Swisdak, M.},
  Journal                  = {The Astrophysical Journal Letters},
  Year                     = {2012},
  Number                   = {2},
  Pages                    = {L30},
  Volume                   = {750},

  Url                      = {http://iopscience.iop.org/2041-8205/750/2/L30},
  Urldate                  = {2014-05-31}
}

@Article{Schoeffler2011,
  Title                    = {The effects of plasma beta and anisotropy instabilities on the dynamics of reconnecting magnetic fields in the heliosheath},
  Author                   = {Schoeffler, Kevin M. and Drake, J. F. and Swisdak, M.},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2011},
  Number                   = {1},
  Pages                    = {70},
  Volume                   = {743},

  Url                      = {http://iopscience.iop.org/0004-637X/743/1/70},
  Urldate                  = {2014-05-31}
}

@Article{Scholer1998,
  Title                    = {Injection and acceleration of energetic particles at collisionless shocks},
  Author                   = {Scholer, Manfred and Kucharek, Harald and Trattner, Karlheinz J},
  Journal                  = {Advances in Space Research},
  Year                     = {1998},
  Number                   = {4},
  Pages                    = {533--542},
  Volume                   = {21}
}

@Article{Scholer2004,
  Title                    = {Nonstationarity of quasi-perpendicular shocks: a comparison of full particle simulations with different ion to electron mass ratio},
  Author                   = {Scholer, M. and Matsukiyo, S.},
  Journal                  = {Ann. Geophys.},
  Year                     = {2004},

  Month                    = jul,
  Number                   = {7},
  Pages                    = {2345--2353},
  Volume                   = {22},

  Doi                      = {10.5194/angeo-22-2345-2004},
  ISSN                     = {1432-0576},
  Keywords                 = {kinetic and mhd the-, numerical simulation studies, ory, shock waves, Space Plasma Physics},
  Url                      = {http://www.ann-geophys.net/22/2345/2004/}
}

@InProceedings{Scholer2004a,
  Title                    = {Nonstationarity of quasi-perpendicular shocks: a comparison of full particle simulations with different ion to electron mass ratio},
  Author                   = {Scholer, M and Matsukiyo, S},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2004},
  Pages                    = {2345--2353},
  Volume                   = {22}
}

@Article{Schreiner2014,
  Title                    = {Wave-particle-interaction in kinetic plasmas},
  Author                   = {Schreiner, Cedric and Spanier, Felix},
  Journal                  = {Comput. Phys. Commun.},
  Year                     = {2014}
}

@Article{Schrijver2011,
  Title                    = {Long-range magnetic couplings between solar flares and coronal mass ejections observed by {SDO} and {STEREO}},
  Author                   = {Schrijver, C. J. and Title, A. M.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2011},

  Month                    = apr,
  Pages                    = {4108},
  Volume                   = {116},

  Doi                      = {10.1029/2010JA016224},
  Keywords                 = {and Astronomy: Coronal mass ejections (2101), and Astronomy: Flares, and Astronomy: Magnetic fields, ASTROPHYSICS, Solar Physics}
}

@Article{Schunk1977,
  Title                    = {Mathematical structure of transport equations for multispecies flows},
  Author                   = {Schunk, RW},
  Journal                  = {Rev. Geophys.},
  Year                     = {1977},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/RG015i004p00429/full}
}

@Article{Schunk2007,
  Title                    = {Time-dependent simulations of the global polar wind},
  Author                   = {Schunk, R. W.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2007},
  Number                   = {16},
  Pages                    = {2028--2047},
  Volume                   = {69},

  File                     = {Snapshot:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/QB9QKFXX/S136468260700243X.html:text/html},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S136468260700243X},
  Urldate                  = {2015-12-09}
}

@Article{Schwadron1999,
  Title                    = {Elemental {Fractionation} in the {Slow} {Solar} {Wind}},
  Author                   = {Schwadron, N. A. and Fisk, L. A. and Zurbuchen, T. H.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {1999},

  Month                    = aug,
  Pages                    = {859--867},
  Volume                   = {521},

  Doi                      = {10.1086/307575},
  Keywords                 = {Magnetohydrodynamics: MHD, Sun: activity, Sun: corona, Sun: magnetic fields, Sun: solar wind}
}

@Article{Schwartz1995,
  Title                    = {Hot flow anomalies near the {Earth}'s bow shock},
  Author                   = {Schwartz, SJ},
  Journal                  = {Advances in space research},
  Year                     = {1995},
  Number                   = {8},
  Pages                    = {107--116},
  Volume                   = {15}
}

@Article{Schwartz1998,
  Title                    = {Shock and discontinuity normals, {Mach} numbers, and related parameters},
  Author                   = {Schwartz, Steven J},
  Journal                  = {ISSI Scientific Reports Series},
  Year                     = {1998},
  Pages                    = {249--270},
  Volume                   = {1}
}

@Article{Schwartz2006,
  Title                    = {Kinetic aspects of foreshock cavities},
  Author                   = {Schwartz, Steven J. and Sibeck, David and Wilber, Mark and Meziane, Karim and Horbury, Timothy S.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2006},
  Pages                    = {12103},
  Volume                   = {33},

  Abstract                 = {We have investigated the kinetic signatures within, and at the edges of, a foreshock cavity. Such cavities are believed to be formed when an isolated collection of interplanetary magnetic field lines connect to quasi-parallel regions of the Earth's bow shock, allowing energetic ions to flow upstream and excavate a local cavity. Observations by the Cluster spacecraft show precisely this configuration. The suprathermal ions can be seen just outside the edges of the cavity within a restricted range of gyrophases, consistent with their gyromotion tangential to the layer containing the cavity. Foreshock cavities, if sufficiently common, may play significant roles in triggering magnetospheric events. Thus our confirmation of their relatively simple formation mechanism lends support to their inferred frequency.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Interplanetary Physics: Planetary bow shocks Space Plasma Physics: Shock waves (4455)},
  Url                      = {http://adsabs.harvard.edu/abs/2006GeoRL..3312103S}
}

@Article{Schwenn2006,
  Title                    = {Solar {Wind} {Sources} and {Their} {Variations} {Over} the {Solar} {Cycle}},
  Author                   = {Schwenn, R.},
  Journal                  = {ßr},
  Year                     = {2006},

  Month                    = jun,
  Pages                    = {51--76},
  Volume                   = {124},

  Doi                      = {10.1007/s11214-006-9099-5},
  Keywords                 = {corona, coronal mass ejections (CMEs), differential rotation, high-speed streams, solar activity cycle, Solar Wind, streamers}
}

@Article{Schwenn2006a,
  Title                    = {Space weather: {The} solar perspective},
  Author                   = {Schwenn, Rainer},
  Journal                  = {Living Reviews in Solar Physics},
  Year                     = {2006},
  Number                   = {2},
  Pages                    = {1--72},
  Volume                   = {3}
}

@Article{Schwenn1980,
  Title                    = {Singly-ionized helium in the driver gas of an interplanetary shock wave},
  Author                   = {Schwenn, R. and Rosenbauer, H. and Muehlhaeuser, K.-H.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {1980},

  Month                    = mar,
  Pages                    = {201--204},
  Volume                   = {7},

  Doi                      = {10.1029/GL007i003p00201},
  Keywords                 = {Cold Plasmas, Helios 1, Helium Plasma, INTERPLANETARY MEDIUM, Ionized Gases, Plasma diagnostics, Rarefied Plasmas, Shock Wave Propagation, Solar Protons}
}

@Article{Scudder1995,
  Title                    = {A review of the physics of electron heating at collisionless shocks},
  Author                   = {Scudder, Jack David},
  Journal                  = {Advances in Space Research},
  Year                     = {1995},
  Number                   = {8},
  Pages                    = {181--223},
  Volume                   = {15}
}

@Article{Sedykh2014,
  Title                    = {Bow shock: {Power} aspects},
  Author                   = {Sedykh, PA},
  Journal                  = {Advances in Space Research},
  Year                     = {2014}
}

@Article{Seki2001,
  Title                    = {On {Atmospheric} {Loss} of {Oxygen} {Ions} from {Earth} {Through} {Magnetospheric} {Processes}},
  Author                   = {Seki, K. and Elphic, R. C. and Hirahara, M. and Terasawa, T. and Mukai, T.},
  Journal                  = {Science},
  Year                     = {2001},

  Month                    = mar,
  Pages                    = {1939--1941},
  Volume                   = {291},

  Doi                      = {10.1126/science.1058913}
}

@Article{Seki2001a,
  Title                    = {On {Atmospheric} {Loss} of {Oxygen} {Ions} from {Earth} {Through} {Magnetospheric} {Processes}},
  Author                   = {Seki, K. and Elphic, R. C. and Hirahara, M. and Terasawa, T. and Mukai, T.},
  Journal                  = {Science},
  Year                     = {2001},

  Month                    = mar,
  Pages                    = {1939--1941},
  Volume                   = {291},

  Doi                      = {10.1126/science.1058913}
}

@Article{Seki2009,
  Title                    = {Observations of loss cone–shaped back streaming energetic protons upstream of the {Earth}'s bow shock},
  Author                   = {Seki, Y and Nishino, MN and Fujimoto, M and Miyashita, Y and Keika, K and Hasegawa, H and Okabe, K and Kasaba, Y and Terasawa, T and Yamamoto, TI and {others}},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2009},
  Number                   = {A11},
  Volume                   = {114}
}

@Article{Sembay2012,
  Title                    = {{AXIOM}: {Advanced} {X}-ray imaging of the magnetosheath},
  Author                   = {Sembay, S. and Branduardi-Raymont, G. and Eastwood, J. P. and Sibeck, D. G. and Abbey, A. and Brown, P. and Carter, J. A. and Carr, C. M. and Forsyth, C. and Kataria, D. and Kemble, S. and Milan, S. and Owen, C. J. and Read, A. M. and Peacocke, L. and Arridge, C. S. and Coates, A. J. and Collier, M. R. and Cowley, S. W. H. and Fazakerley, A. N. and Fraser, G. and Jones, G. H. and Lallement, R. and Lester, M. and Porter, F. S. and Yeoman, T.},
  Journal                  = {Astronomische Nachrichten},
  Year                     = {2012},
  Pages                    = {388--392},
  Volume                   = {333},

  Abstract                 = {AXIOM (Advanced X-ray Imaging Of the Magnetosphere) is a concept mission which aims to explain how the Earth's magnetosphere responds to the changing impact of the solar wind using a unique method never attempted before; performing wide-field soft X-ray imaging and spectroscopy of the magnetosheath, magnetopause and bow shock at high spatial and temporal resolution. Global imaging of these regions is possible because of the solar wind charge exchange (SWCX) process which produces elevated soft X-ray emission from the interaction of high charge-state solar wind ions with primarily neutral hydrogen in the Earth's exosphere and near-interplanetary space.},
  ISSN                     = {0004-6337},
  Keywords                 = {Earth interplanetary medium magnetic fields space vehicles: instruments X-rays: general},
  Url                      = {http://adsabs.harvard.edu/abs/2012AN....333..388S}
}

@Article{Semenov2002,
  Title                    = {A simple model of magnetopause erosion as a consequence of pile-up process and bursty reconnection},
  Author                   = {Semenov, VS and Alexandrova, OA and Erkaev, NV and Mühlbachler, S and Biernat, HK},
  Journal                  = {International Journal of Geomagnetism and Aeronomy},
  Year                     = {2002},
  Number                   = {2},
  Pages                    = {109--116},
  Volume                   = {3}
}

@Article{Sergeev1993,
  Title                    = {Structure of the tail plasma/current sheet at 11 {RE} and its changes in the course of a substorm},
  Author                   = {Sergeev, VA and Mitchell, DG and Russell, CT and Williams, DJ},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1993},
  Number                   = {A10},
  Pages                    = {17345--17365},
  Volume                   = {98}
}

@Article{Sergeev2003,
  Title                    = {Current sheet flapping motion and structure observed by {Cluster}},
  Author                   = {Sergeev, V and Runov, A and Baumjohann, W and Nakamura, R and Zhang, TL and Volwerk, M and Balogh, A and Reme, H and Sauvaud, JA and André, M and {others}},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2003},
  Number                   = {6},
  Volume                   = {30}
}

@Article{Shabat2007,
  Title                    = {Analysis of the sensitivity of self-focused nonlinear optical evanescent waveguide sensors},
  Author                   = {Shabat, Mohammed M and Khalil, Hala and Taya, Sofyan A and Abadla, Mazen M},
  Journal                  = {International Journal of Optomechatronics},
  Year                     = {2007},
  Number                   = {3},
  Pages                    = {284--296},
  Volume                   = {1}
}

@Article{Shaikhislamov2011,
  Title                    = {Small scale magnetosphere: {Laboratory} experiment, physical model and {Hall} {MHD} simulation},
  Author                   = {Shaikhislamov, IF and Antonov, VM and Zakharov, Yu P and Boyarintsev, EL and Melekhov, AV and Posukh, VG and Ponomarenko, AG},
  Journal                  = {arXiv preprint arXiv:1110.4461},
  Year                     = {2011}
}

@Article{Sharma2012,
  Title                    = {Presence of solar filament plasma detected in interplanetary coronal mass ejections by in situ spacecraft},
  Author                   = {Sharma, R. and Srivastava, N.},
  Journal                  = {Journal of Space Weather and Space Climate},
  Year                     = {2012},

  Month                    = jul,
  Number                   = {27},
  Pages                    = {A10},
  Volume                   = {2},

  Doi                      = {10.1051/swsc/2012010},
  Keywords                 = {filaments, interplanetary coronal mass ejection (ICME), plasma, Solar Wind}
}

@Article{Sharma2013,
  Title                    = {Interplanetary and geomagnetic consequences of 5 {January} 2005 {CMEs} associated with eruptive filaments},
  Author                   = {Sharma, R. and Srivastava, N. and Chakrabarty, D. and Möstl, C. and Hu, Q.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = jul,
  Pages                    = {3954--3967},
  Volume                   = {118},

  Doi                      = {10.1002/jgra.50362},
  Keywords                 = {CME, filament plasma, flux rope, ICME, magnetic cloud, sub-storm}
}

@Article{Shay2007,
  Title                    = {Two-{Scale} {Structure} of the {Electron} {Dissipation} {Region} during {Collisionless} {Magnetic} {Reconnection}},
  Author                   = {Shay, M. A. and Drake, J. F. and Swisdak, M.},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2007},

  Month                    = oct,
  Number                   = {15},
  Pages                    = {155002},
  Volume                   = {99},

  Doi                      = {10.1103/PhysRevLett.99.155002},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.99.155002}
}

@Article{Shay2007a,
  Title                    = {{Two-Scale Structure of the Electron Dissipation Region during Collisionless Magnetic Reconnection}},
  Author                   = {Shay, M A and Drake, J F and Swisdak, M},
  Journal                  = {Phys. Rev. Lett.},
  Year                     = {2007},

  Month                    = {oct},
  Number                   = {15},
  Pages                    = {155002},
  Volume                   = {99},

  __markedentry            = {[suleimanbaraka:6]},
  Doi                      = {10.1103/PhysRevLett.99.155002},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Shay, Drake, Swisdak/Phys. Rev. Lett/Shay - 2007 - Two-Scale Structure of the Electron Dissipation Region during Collisionless Magnetic Reconnection.pdf:pdf},
  Owner                    = {suleimanbaraka},
  Publisher                = {American Physical Society},
  Timestamp                = {2016.02.23},
  Url                      = {http://link.aps.org/doi/10.1103/PhysRevLett.99.155002}
}

@Article{Shen2011,
  Title                    = {The magnetic configuration of the high-latitude cusp and dayside magnetopause under strong magnetic shears},
  Author                   = {Shen, C. and Dunlop, M. and Ma, Y. H. and Chen, Z. Q. and Yan, G. Q. and Liu, Z. X. and Bogdanova, Y. V. and Sibeck, D. G. and Carr, C. M. and Zhang, Q. H. and Lucek, E.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2011},
  Pages                    = {9228},
  Volume                   = {116},

  Abstract                 = {This paper investigates the structure of the magnetic field near the magnetopause (MP) by analyzing the multiple-point magnetic measurements from the Cluster mission. In this paper, the spatial distribution of the curvature radius of the MP surface at the noon-midnight meridian and for situations with moderate dynamical pressure of solar wind is implied from direct measurements of magnetic field curvature for the first time. The investigation focused on conditions of strong magnetic shear and in which a clear boundary layer is present at the MP. It has been confirmed that the magnetic field lines surrounding the cusp bend sunward at the precusp region and tailward at the postcusp region, implying the existence of a cusp field indentation. The minimum curvature radius of the near-MP field at both precusp and postcusp regions is about 2 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}. As the latitude decreases, the curvature radius at the MP increases gradually, so that, as the subsolar point is approached, the curvature radius of the MP is nearly equal to the geocentric distance. These results compare well with existing MP models but reveal the limitations inherent in such statistical estimates of local MP curvature, particularly surrounding the cusp regions. The analysis of the magnetic measurements has also verified the existence of the magnetic bottles at both precusp and postcusp regions, which may play a role for the trapping of the charged particles of magnetosphere.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Cusp Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetospheric configuration and dynamics Space Plasma Physics: Discontinuities (2109)},
  Url                      = {http://adsabs.harvard.edu/abs/2011JGRA..116.9228S}
}

@Article{Shen2008,
  Title                    = {Stability of the {Distant} {Satellites} of the {Giant} {Planets} in the {Solar} {System}},
  Author                   = {Shen, Y. and Tremaine, S.},
  Journal                  = {{\textbackslash}textbackslashaj},
  Year                     = {2008},

  Month                    = dec,
  Pages                    = {2453--2467},
  Volume                   = {136},

  Doi                      = {10.1088/0004-6256/136/6/2453},
  Keywords                 = {asteroids, celestial mechanics, minor planets, planets and satellites: formation, planets and satellites: general}
}

@Article{Shue2011,
  Title                    = {Uneven compression levels of {Earth}'s magnetic fields by shocked solar wind},
  Author                   = {Shue, J.-H. and Chen, Y.-S. and Hsieh, W.-C. and Nowada, M. and Lee, B. S. and Song, P. and Russell, C. T. and Angelopoulos, V. and Glassmeier, K. H. and McFadden, J. P. and Larson, D.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2011},

  Month                    = feb,
  Pages                    = {2203},
  Volume                   = {116},

  Doi                      = {10.1029/2010JA016149},
  Keywords                 = {7835), Magnetospheric Physics: Magnetic reconnection (7526, Magnetospheric Physics: Magnetopause and boundary layers, Magnetospheric Physics: Magnetosphere: inner, Magnetospheric Physics: Solar wind/magnetosphere interactions}
}

@Article{Shue2001,
  Title                    = {Effects of solar wind density on auroral electrojets},
  Author                   = {Shue, J-H and Kamide, Y},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2001},
  Number                   = {11},
  Pages                    = {2181--2184},
  Volume                   = {28}
}

@Book{Shukla2001,
  Title                    = {Introduction to dusty plasma physics},
  Author                   = {Shukla, Padma K and Mamun, AA},
  Publisher                = {CRC Press},
  Year                     = {2001}
}

@Article{Sibeck1994,
  Title                    = {Signatures of flux erosion from the dayside magnetosphere},
  Author                   = {Sibeck, DG},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1994},
  Number                   = {A5},
  Pages                    = {8513--8529},
  Volume                   = {99}
}

@Article{Sibeck1999a,
  Title                    = {Comprehensive study of the magnetospheric response to a hot flow anomaly},
  Author                   = {Sibeck, DG and Borodkova, NL and Schwartz, SJ and Owen, CJ and Kessel, R and Kokubun, S and Lepping, RP and Lin, R and Liou, K and Lühr, H and {others}},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1999},
  Number                   = {A3},
  Pages                    = {4577--4593},
  Volume                   = {104}
}

@Article{Sibeck2004,
  Title                    = {Radial dependence of foreshock cavities: a case study},
  Author                   = {Sibeck, D. and Kudela, K. and Mukai, T. and Nemecek, Z. and Safrankova, J.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2004},
  Pages                    = {4143--4151},
  Volume                   = {22},

  Abstract                 = {We present a case study of Geotail, Interball-1, IMP-8, and Wind observations of density and magnetic field strength cavities excavated by the enhanced pressures associated with bursts of energetic ions in the foreshock. Consistent with theoretical predictions, the pressure of the energetic ions diminishes rapidly with upstream distance due to a decrease in the flux of energetic ions and a transition from near-isotropic to streaming pitch angle distributions. Consequently, the cavities can only be observed immediately upstream from the bow shock. A comparison of conditions upstream from the pre- and post-noon bow shock demonstrates that foreshock cavities introduce perturbations into the oncoming solar wind flow with dimensions smaller than those of the magnetosphere. Dayside geosynchronous magnetic field strength variations observed by GOES-8 do not track the density variations seen by any of the spacecraft upstream from the bow shock in a one-to-one manner, indicating that none of these spacecraft observed the precise sequence of density variations that actually struck the subsolar magnetopause.},
  ISSN                     = {0992-7689},
  Url                      = {http://adsabs.harvard.edu/abs/2004AnGeo..22.4143S}
}

@Article{Sibeck2008a,
  Title                    = {On the edge of the foreshock: model-data comparisons},
  Author                   = {Sibeck, DG and Omidi, N and Dandouras, I and Lucek, E},
  Journal                  = {Ann. Geophys},
  Year                     = {2008},
  Pages                    = {1539--1544},
  Volume                   = {26}
}

@Article{Sibeck2003,
  Title                    = {Preface},
  Author                   = {Sibeck, D. G.},
  Journal                  = {Advances in Space Research},
  Year                     = {2003},
  Pages                    = {1125--1125},
  Volume                   = {31},

  Abstract                 = {Not Available},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/2003AdSpR..31.1125S}
}

@Article{Sibeck1995,
  Title                    = {Coupling processes at the magnetopause},
  Author                   = {Sibeck, D. G.},
  Journal                  = {Surveys in Geophysics},
  Year                     = {1995},
  Pages                    = {267--298},
  Volume                   = {16},

  Abstract                 = {This review covers several aspects of magnetopause research during the two-year period from mid-1991 to mid-1993. It focusses upon three topics which received renewed attention: the structure of the steady-state magnetopause, the origin of the transient events which are superimposed upon it, and the cause of transient signatures observed by high-latitude dayside ground magnetometers. Case and statistical studies defined the relatively unknown characteristics of the magnetosheath plasma layers lying outside the magnetopause, while theoretical studies provided alternative explanations for the presence of magnetosheath plasma within the LLBL. Evidence was presented for a steady transition from magnetosheath to magnetospheric plasma parameters. Detailed studies described the plasma, energetic particle, and magnetic field characteristics of transient events in the outer dayside magnetosphere, and multipoint studies provided important new information concerning the ionospheric response to sudden changes in solar wind parameters. This review emphasizes the competing explanations which have been advanced to explain these phenomena.},
  ISSN                     = {0169-3298},
  Keywords                 = {Magnetopause solar wind-magnetosphere interaction reconnection boundary layers flux transfer events travelling ionospheric convection vortices},
  Url                      = {http://adsabs.harvard.edu/abs/1995SGeo...16..267S}
}

@Article{Sibeck1995a,
  Title                    = {The {Magnetospheric} {Response} to {Foreshock} {Pressure} {Pulses}},
  Author                   = {Sibeck, David G.},
  Journal                  = {Washington DC American Geophysical Union Geophysical Monograph Series},
  Year                     = {1995},
  Note                     = {ISBN: {\textless}ISBN{\textgreater}0-87590-047-X{\textless}/ISBN{\textgreater}},
  Pages                    = {293},
  Volume                   = {90},

  Abstract                 = {Not Available},
  ISSN                     = {0-87590-047-X},
  Url                      = {http://adsabs.harvard.edu/abs/1995GMS....90..293S}
}

@Article{Sibeck1994a,
  Title                    = {Signatures of flux erosion from the dayside magnetosphere},
  Author                   = {Sibeck, D. G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1994},
  Pages                    = {8513--8529},
  Volume                   = {99},

  Abstract                 = {The rate of merging and the strength of the region 1 Birkeland currents increase during periods of southward interplanetary magnetic field (IMF). Fringe fields of the Birkeland currents depress dayside magnetospheric magnetic field strengths and remove magnetic flux from the dayside magnetophere, thereby allowing the dayside magnetopause to move inward and the cusp equatorward. We use previously derived fits to the magnetospause location as a function of IMF B(sub z), the condition of pressure balance at the magnetopause, and an idealized model of region 1 Birkeland currents to estimate that strong southward IMF turnings will produce approximately 13- to 26-nT depressions in the geosynchronous magnetic field strength over periods of 30-60 min. We then present three case studies of geosynchronous magnetic field strength variations during periods of nearly constant solar wind dynamic pressure and southward IMF. The dayside magnetospheric magnetic field strength was depressed approximately 10 nT during a period of strongly southward IMF (B(sub z) = -6 nT), but only approximately 5 nT during two more typical periods of slightly southward IMF (B(sub z) = -2 to -3 nT). The depressions correspond to periods of enhanced AL index, which we interpret as evidence for directly driven solar wind-magnetosphere interaction rather than the unloading of energy stored within the magnetotail. Dayside geosynchronous magnetic field strengths are weakly correlated with IMF B(sub z).},
  ISSN                     = {0148-0227},
  Keywords                 = {Birkeland Currents Earth Magnetosphere Interplanetary Magnetic Fields Magnetic Field Reconnection Magnetic Flux Polar Cusps Solar Terrestrial Interactions Solar Wind Data Reduction Geosynchronous Orbits Magnetopause},
  Url                      = {http://adsabs.harvard.edu/abs/1994JGR....99.8513S}
}

@Article{Sibeck1994b,
  Title                    = {Magnethosheath magnetic field variability},
  Author                   = {Sibeck, D. G.},
  Journal                  = {Advances in Space Research},
  Year                     = {1994},
  Pages                    = {91--94},
  Volume                   = {14},

  Abstract                 = {A case study using simultaneous IRM and CCE observations demonstrates that transient magnetospheric events correspond to pressure pulses in the magnetosheath, inward bow shock motions and magnetopause compression. Statistical surveys indicate that the magnetosheath magnetic field orientation rarely remains constant during periods of magnetopause and bow shock motion (both characterized by periods of 1-10 min). There is no tendency for bow shock motion to occur for southward IMF orientations.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/1994AdSpR..14...91S}
}

@Article{Sibeck1990,
  Title                    = {{A Model for the Transient Magnetospheric Response to Sudden Solar Wind Dynamic Pressure Variations}},
  Author                   = {Sibeck, David G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1990},
  Number                   = {A4},
  Pages                    = {3755--3771},
  Volume                   = {95},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {The evidence for transient variations in the solar wind dynamic pressure, their effect on magnetopause boundary motion, and the signatures they produce within the magnetosphere and at high-latitude auroral ground stations, are examined. A qualitative model for the magnetospheric response to such variations explaining a wide variety of transient magnetopause, magnetospheric and ground signatures is proposed, and its applicability is shown. The model is presented as an alternative explanation for many of the signatures previously interpreted as direct on site evidence of patchy, sporadic, magnetic field merging, namely the flux transfer events (FTEs).},
  Doi                      = {10.1029/JA095iA04p03755},
  ISSN                     = {0148-0227},
  Keywords                 = {doi:10.,http://dx.doi.org/10.1029/JA095iA04p03755},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23},
  Url                      = {http://www.agu.org/pubs/crossref/1990/JA095iA04p03755.shtml}
}

@Article{Sibeck2008,
  Title                    = {{THEMIS science objectives and mission phases}},
  Author                   = {Sibeck, D. G. and Angelopoulos, V.},
  Journal                  = {Space Sci. Rev.},
  Year                     = {2008},
  Number                   = {1-4},
  Pages                    = {35--59},
  Volume                   = {141},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {Issue Title: The THEMIS Mission The five THEMIS spacecraft and a dedicated ground-based observatory array will pinpoint when and where substorms occur, thereby providing the observations needed to identify the processes that cause substorms to suddenly release solar wind energy stored within the Earth's magnetotail. The primary science which drove the mission design enables unprecedented observations relevant to magnetospheric research areas ranging from the foreshock to the Earth's radiation belts. This paper describes how THEMIS will reach closure on its baseline scientific objectives as a function of mission phase. [PUBLICATION ABSTRACT]},
  Doi                      = {10.1007/s11214-008-9393-5},
  ISSN                     = {00386308},
  Keywords                 = {Magnetopause,Magnetosphere,Radiation belts,Substorms,THEMIS},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Sibeck2008b,
  Title                    = {{THEMIS} {Science} {Objectives} and {Mission} {Phases}},
  Author                   = {Sibeck, D. G. and Angelopoulos, V.},
  Journal                  = {Space Science Reviews},
  Year                     = {2008},
  Pages                    = {35--59},
  Volume                   = {141},

  Abstract                 = {The five THEMIS spacecraft and a dedicated ground-based observatory array will pinpoint when and where substorms occur, thereby providing the observations needed to identify the processes that cause substorms to suddenly release solar wind energy stored within the Earth’s magnetotail. The primary science which drove the mission design enables unprecedented observations relevant to magnetospheric research areas ranging from the foreshock to the Earth’s radiation belts. This paper describes how THEMIS will reach closure on its baseline scientific objectives as a function of mission phase.},
  ISSN                     = {0038-6308},
  Keywords                 = {THEMIS Magnetosphere Substorms Radiation belts Magnetopause},
  Url                      = {http://adsabs.harvard.edu/abs/2008SSRv..141...35S}
}

@Article{Sibeck2011,
  Title                    = {{ARTEMIS} {Science} {Objectives}},
  Author                   = {Sibeck, D. G. and Angelopoulos, V. and Brain, D. A. and Delory, G. T. and Eastwood, J. P. and Farrell, W. M. and Grimm, R. E. and Halekas, J. S. and Hasegawa, H. and Hellinger, P. and Khurana, K. K. and Lillis, R. J. and Øieroset, M. and Phan, T.-D. and Raeder, J. and Russell, C. T. and Schriver, D. and Slavin, J. A. and Travnicek, P. M. and Weygand, J. M.},
  Journal                  = {Space Science Reviews},
  Year                     = {2011},
  Pages                    = {59--91},
  Volume                   = {165},

  Abstract                 = {NASA's two spacecraft ARTEMIS mission will address both heliospheric and planetary research questions, first while in orbit about the Earth with the Moon and subsequently while in orbit about the Moon. Heliospheric topics include the structure of the Earth's magnetotail; reconnection, particle acceleration, and turbulence in the Earth's magnetosphere, at the bow shock, and in the solar wind; and the formation and structure of the lunar wake. Planetary topics include the lunar exosphere and its relationship to the composition of the lunar surface, the effects of electric fields on dust in the exosphere, internal structure of the Moon, and the lunar crustal magnetic field. This paper describes the expected contributions of ARTEMIS to these baseline scientific objectives.},
  ISSN                     = {0038-6308},
  Keywords                 = {ARTEMIS Moon Reconnection Particle acceleration Turbulence Wake Lunar surface Lunar core Dust Electric fields Crustal anomalies},
  Url                      = {http://adsabs.harvard.edu/abs/2011SSRv..165...59S}
}

@Article{Sibeck1989,
  Title                    = {The magnetospheric response to 8-minute period strong-amplitude upstream pressure variations},
  Author                   = {Sibeck, David G and Baumjohann, W and Elphic, RC and Fairfield, DH and Fennell, JF and Gail, WB and Lanzerotti, LJ and Lopez, RE and Luehr, H and Lui, ATY and {others}},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1989},
  Number                   = {A3},
  Pages                    = {2505--2519},
  Volume                   = {94}
}

@Article{Sibeck1999b,
  Title                    = {Comprehensive study of the magnetospheric response to a hot flow anomaly},
  Author                   = {Sibeck, D. G. and Borodkova, N. L. and Schwartz, S. J. and Owen, C. J. and Kessel, R. and Kokubun, S. and Lepping, R. P. and Lin, R. and Liou, K. and Lühr, H. and McEntire, R. W. and Meng, C.-I. and Mukai, T. and Nemecek, Z. and Parks, G. and Phan, T. D. and Romanov, S. A. and Safrankova, J. and Sauvaud, J.-A. and Singer, H. J. and Solovyev, S. I. and Szabo, A. and Takahashi, K. and Williams, D. J. and Yumoto, K. and Zastenker, G. N.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1999},
  Pages                    = {4577--4594},
  Volume                   = {104},

  Abstract                 = {We present a comprehensive observational study of the magnetospheric response to an interplanetary magnetic field (IMF) tangential discontinuity, which first struck the postnoon bow shock and magnetopause and then swept past the prenoon bow shock and magnetopause on July 24, 1996. Although unaccompanied by any significant plasma variation, the discontinuity interacted with the bow shock to form a hot flow anomaly (HFA), which was observed by Interball-1 just upstream from the prenoon bow shock. Pressures within and Earthward of the HFA were depressed by an order of magnitude, which allowed the magnetopause to briefly ( 7 min) move outward some 5R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} beyond its nominal position and engulf Interball-1. A timing study employing nearby Interball-1 and Magion-4 observations demonstrates that this motion corresponded to an antisunward and northward moving wave on the magnetopause. The same wave then engulfed Geotail, which was nominally located downstream in the outer dawn magnetosheath. Despite its large amplitude, the wave produced only minor effects in GOES-8 geosynchronous observations near local dawn. Polar Untraviolet Imager (UVI) observed a sudden brightening of the afternoon aurora, followed by an even more intense transient brightening of the morning aurora. Consistent with this asymmetry, the discontinuity produced only weak near-simultaneous perturbations in high-latitude postnoon ground magnetometers but a transient convection vortex in the prenoon Greenland ground magnetograms. The results of this study indicate that the solar wind interaction with the bow shock is far more dynamic than previously imagined and far more significant to the solar wind-magnetosphere interaction.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/1999JGR...104.4577S}
}

@Article{Sibeck1996a,
  Title                    = {Solar wind variations as a source of short-term magnetic field perturbations in the dayside magnetosphere},
  Author                   = {Sibeck, D. G. and Borodkova, N. L. and Zastenker, G. N.},
  Journal                  = {Kosmicheskie Issledovaniia},
  Year                     = {1996},
  Pages                    = {248--263},
  Volume                   = {34},

  Abstract                 = {Short variations (about several minutes) in the dayside magnetospheric magnetic field measured by the GOES-5 and GOES-6 geosynchronous satellites were compared with simultaneous observations of the solar wind plasma and magnetic field aboard the Prognoz-10 and IMP-8 satellites. The results indicate that more than half of the events were caused by dynamic pressure variations in the solar wind. A considerable portion of the events can be associated with fluctuations in the orientation of the interplanetary magnetic field, influencing the foreshock plasma pressure.},
  Keywords                 = {Solar Wind: Geomagnetic Field Solar Wind: Variations Solar Wind: Interplanetary Magnetic Field},
  Url                      = {http://adsabs.harvard.edu/abs/1996KosIs..34..248S}
}

@Article{Sibeck1996b,
  Title                    = {Solar {Wind} {Variations} as a {Source} of {Short}-{Term} {Magnetic} {Field} {Disturbances} in the {Dayside} {Magnetosphere}},
  Author                   = {Sibeck, D. G. and Borodkova, N. L. and Zastenker, G. N.},
  Journal                  = {Cosmic Research},
  Year                     = {1996},
  Pages                    = {228},
  Volume                   = {34},

  Abstract                 = {Not Available},
  ISSN                     = {0023-4206},
  Url                      = {http://adsabs.harvard.edu/abs/1996CosRe..34..228S}
}

@Article{Sibeck1998,
  Title                    = {Gross deformation of the dayside magnetopause},
  Author                   = {Sibeck, D. G. and Borodkova, N. L. and Zastenker, G. N. and Romanov, S. A. and Sauvaud, J.-A.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1998},
  Pages                    = {453--456},
  Volume                   = {25},

  Abstract                 = {On July 24, 1996, the entire magnetosheath moved past the Interball-1 spacecraft twice within 7 min. Such rapid transits through the magnetosheath suggest the passage of an antisunward-moving boundary wave with an amplitude in excess of 5 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}. A wave of this amplitude requires an order of magnitude decrease in the pressure confining the magnetosphere. Such decreases have been reported only in conjunction with hot flow anomalies, features accompanying interplanetary magnetic field discontinuities, bounded by narrow shocks, and identified on the basis of heated deflected flows transverse to the Earth-Sun line. We identify all these features just outside the Interball-1 magnetopause crossings on July 24, 1996.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers},
  Url                      = {http://adsabs.harvard.edu/abs/1998GeoRL..25..453S}
}

@Article{Sibeck2001,
  Title                    = {Solar wind preconditioning in the flank foreshock: {IMP} 8 observations},
  Author                   = {Sibeck, D. G. and Decker, R. B. and Mitchell, D. G. and Lazarus, A. J. and Lepping, R. P. and Szabo, A.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2001},
  Pages                    = {21675--21688},
  Volume                   = {106},

  Abstract                 = {We use IMP 8 plasma, magnetic field, and energetic ion observations within the Earth's foreshock from January through August 1995 to determine the effects of energetic ion bursts on the ambient solar wind for comparison with model predictions. Owing to the spiral interplanetary magnetic field orientation, the events are far more common upstream from the prenoon than postnoon bow shock. Pressures associated with the energetic ions depress foreshock magnetic field strengths and plasma densities. The magnitude of the depression is proportional to the intensity of energetic ions. The excavated plasma and magnetic field sometimes pile up in narrow regions of enhanced plasma densities and magnetic field strengths, but depressed flow velocities, just outside the foreshock cavities. Typical amplitudes of the depressions and enhancements at IMP 8 far upstream from the bow shock are far less (20\% and 10\%, respectively) than those seen in past case studies of events observed just outside the bow shock. The cavities occur preferentially during high-speed solar wind streams but show no clear dependence upon other solar wind parameters. The distribution of burst durations resembles those for interarrival times for interplanetary magnetic field discontinuities, magnetopause motion, and flux transfer events, suggesting causal relationships between these phenomena.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Energetic particles planetary Interplanetary Physics: Planetary bow shocks Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2001JGR...10621675S}
}

@Article{Sibeck1996,
  Title                    = {{Magnetosheath density fluctuations and magnetopause motion}},
  Author                   = {Sibeck, D G and Gosling, J T},
  Journal                  = {J Geophys Res},
  Year                     = {1996},
  Pages                    = {31--40},
  Volume                   = {101},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {The interplanetary magnetic field (IMF) orientation controls foreshock densities and modulates the fraction of the solar wind dynamic pressure applied to the magnetosphere. Such pressure variations produce bow shock and magnetopause motion and cause the radial profiles for various magnetosheath parameters to sweep inward and outward past nearly stationary satellites. We report ISEE 2 observations of correlated density and speed fluctuations, and anticorrelated density and temperature fluctuations, on an outbound pass through the northern dawnside magnetosheath. Densities decreased when the magnetic field rotated southward and draped about the magnetopause. In the absence of any significant solar wind density or dynamic pressure variations, we interpret the magnetosheath fluctuations as evidence for radial magnetosheath motion induced by variations in the IMF orientation.},
  Doi                      = {10.1029/95JA03141},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Planetary bow shocks Magne},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23},
  Url                      = {http://adsabs.harvard.edu/abs/1996JGR...101...31S}
}

@Article{Sibeck1996c,
  Title                    = {Magnetosheath density fluctuations and magnetopause motion},
  Author                   = {Sibeck, D. G. and Gosling, J. T.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1996},
  Pages                    = {31--40},
  Volume                   = {101},

  Abstract                 = {The interplanetary magnetic field (IMF) orientation controls foreshock densities and modulates the fraction of the solar wind dynamic pressure applied to the magnetosphere. Such pressure variations produce bow shock and magnetopause motion and cause the radial profiles for various magnetosheath parameters to sweep inward and outward past nearly stationary satellites. We report ISEE 2 observations of correlated density and speed fluctuations, and anticorrelated density and temperature fluctuations, on an outbound pass through the northern dawnside magnetosheath. Densities decreased when the magnetic field rotated southward and draped about the magnetopause. In the absence of any significant solar wind density or dynamic pressure variations, we interpret the magnetosheath fluctuations as evidence for radial magnetosheath motion induced by variations in the IMF orientation.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Planetary bow shocks Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/1996JGR...101...31S}
}

@Article{Sibeck1996d,
  Title                    = {Concerning possible effects of ionospheric conductivity upon the occurrence patterns of impulsive events in high-latitude ground magnetograms},
  Author                   = {Sibeck, D. G. and Greenwald, R. A. and Bristow, W. A. and Korotova, G. I.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1996},
  Pages                    = {13407--13412},
  Volume                   = {101},

  Abstract                 = {Previous studies have interpreted the occurrence patterns of impulsive events in the high-latitude dayside ionosphere in terms of transient processes occurring near the dayside magnetopause. In particular, the fact that most impulsive ground magnetometer events occur prior to local noon has been interpreted as evidence for a dawn/dusk asymmetry in transient processes at the magnetopause. In this paper, we seek to raise the awareness of the community that the high-latitude distribution of the Hall conductivity also influences the signatures observed by ground magnetometers. In particular, we will show that impulsive event occurrence patterns bear a striking resemblance to reported statistical patterns for the Hall conductivity. We suggest that this similarity be taken into account when interpreting occurrence patterns for impulsive ground events.},
  ISSN                     = {0148-0227},
  Keywords                 = {Ionosphere: Auroral ionosphere Ionosphere: Current systems Ionosphere: Electric fields Ionosphere: Particle precipitation},
  Url                      = {http://adsabs.harvard.edu/abs/1996JGR...10113407S}
}

@Article{Sibeck2012a,
  Title                    = {Frequency doubling and field-aligned ion streaming in a long-period poloidal pulsation},
  Author                   = {Sibeck, D. G. and Korotova, G. and Turner, D. L. and Angelopoulos, V. and Glaßmeier, K.-H. and McFadden, J. P.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2012},
  Pages                    = {11215},
  Volume                   = {117},

  Abstract                 = {We reexamine a long-period (10-18 min) poloidal pulsation observed by THEMIS-A in the outer dawn magnetosphere from 10:00 to 12:30 UT on 7 November 2007. The interval was originally reported by Korotova et al. (2009). Although the nonlinear compressional plasma and magnetic field perturbations observed by THEMIS-A during this interval agree well with model predictions for the linear perturbations associated with antisymmetric waves generated by the ballooning-mirror mode instability, the phase relationships between these perturbations indicates a complex frequency rather than the purely imaginary frequency that theory predicts for the outer dawnside magnetosphere. Variations in the radial plasma velocity confirm that a phase-locked north/south oscillation in the equatorial line of nodes associated with the ballooning-mirror mode waves doubles the frequency of the compressional component of the magnetic field during these pulsations. The same velocity and magnetic field perturbations exclude explanations for the frequency doubling in terms of spatial gradients sweeping back and forth across the spacecraft or drift-bounce resonances. Azimuthal electric fields associated with the pulsations generate field-aligned anisotropies in the pitch angle distributions that become more prominent with increasing ion energy due to the presence of drift-shell splitting and radial flux gradients that steepen with increasing energy. Although there was no evidence for drift-bounce interactions during this event, the role of such events in ion energization in other events and at other locations remains to be evaluated.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Energetic particles: trapped Magnetospheric Physics: Plasma waves and instabilities (2471) Magnetospheric Physics: Ring current},
  Url                      = {http://adsabs.harvard.edu/abs/2012JGRA..11711215S}
}

@Article{Sibeck2000,
  Title                    = {Testing models for traveling convection vortices: {Two} case studies},
  Author                   = {Sibeck, D. G. and Korotova, G. I.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2000},
  Pages                    = {325--328},
  Volume                   = {27},

  Abstract                 = {We use geosynchronous magnetic field observations to discriminate between two models for traveling convection vortices (TCVs) generated by pressure variations applied to the magnetosphere. According to the model of Glassmeier [1992], an azimuthal gradient in the pressure generates a single field-aligned current into the high-latitude ionosphere and a single TCV. According to the model of Southwood and Kivelson [1990], an azimuthal gradient in the pressure generates a pair of oppositely directed currents and TCVs. We reexamine two well-documented examples of TCVs and show that their signatures correspond better to the predictions of the Southwood/Kivelson model than to the predictions of the Glassmeier model.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2000GeoRL..27..325S}
}

@Article{Sibeck1996e,
  Title                    = {Occurrence patterns for transient magnetic field signatures at high latitudes},
  Author                   = {Sibeck, D. G. and Korotova, G. I.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1996},
  Pages                    = {13413--13428},
  Volume                   = {101},

  Abstract                 = {Impulsive events marked by durations ranging from 5 to 15 min and peak-to-peak variations in the H component exceeding 40 nT are common in observations by high-latitude dayside ground magnetometers. We survey observations by a global network of high-latitude ground magnetometers to distinguish between their proposed causes. Peak event amplitudes and occurrence rates occur prior to local noon in the range of geomagnetic latitudes from 70° to 76°. Although most events can be associated with abrupt changes in the interplanetary magnetic field (IMF) orientation, few can be associated with abrupt changes in the solar wind dynamic pressure. Many events can be observed during intervals of steadily northward IMF orientation, but only a few can be observed during intervals of steadily southward IMF orientation. We suggest an interpretation of the events in terms of a model in which changes in the IMF orientation modulate the fraction of the solar wind pressure applied to the magnetosphere.},
  ISSN                     = {0148-0227},
  Keywords                 = {Ionosphere: Polar cap ionosphere Magnetospheric Physics: Magnetosphere/ionosphere interactions Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/1996JGR...10113413S}
}

@Article{Sibeck2000a,
  Title                    = {Magnetopause motion driven by interplanetary magnetic field variations},
  Author                   = {Sibeck, D. G. and Kudela, K. and Lepping, R. P. and Lin, R. and Nemecek, Z. and Nozdrachev, M. N. and Phan, T.-D. and Prech, L. and Safrankova, J. and Singer, H. and Yermolaev, Y.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2000},
  Pages                    = {25155--25170},
  Volume                   = {105},

  Abstract                 = {We use previously reported observations of hot flow anomalies (HFAs) and foreshock cavities to predict the characteristics of corresponding features in the dayside magnetosheath, at the magnetopause, and in the outer dayside magnetosphere. We compare these predictions with Interball 1, Magion 4, and GOES 8/GOES 9 observations of magnetopause motion on the dusk flank of the magnetosphere from 1800 UT on January 17 to 0200},
  ISSN                     = {0148-0227},
  Keywords                 = {magnetospheric physics},
  Url                      = {http://adsabs.harvard.edu/abs/2000JGR...10525155S}
}

@Article{Sibeck2008c,
  Title                    = {Crater {FTEs}: {Simulation} results and {THEMIS} observations},
  Author                   = {Sibeck, D. G. and Kuznetsova, M. and Angelopoulos, V. and Glaßmeier, K.-H. and McFadden, J. P.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2008},
  Volume                   = {35},

  Abstract                 = {The BATS-R-US magnetohydrodynamic (MHD) model predicts flux transfer events (FTEs) with strong core magnetic fields embedded within a broadened current layer of weak magnetic field strengths on the equatorial dayside magnetopause during intervals of southward and duskward interplanetary magnetic field (IMF) orientation. Multipoint THEMIS observations at 2202 UT on June 20, 2007 of a southward-moving FTE on the post-noon magnetopause confirm the predictions of the model. THEMIS-E and -A with large impact parameters simply observe enhanced magnetic field strengths in draped magnetosheath magnetic field lines, THEMIS-B and -C with moderate impact parameters pass through the broadened current layer to observe crater FTEs with deep troughs bounding a strong core field, while THEMIS-D with a very low impact parameter observes the core magnetic field strength enhancement embedded in the current layer.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Magnetosheath},
  Url                      = {http://adsabs.harvard.edu/abs/2008GeoRL..3517S06S}
}

@Article{Sibeck2014,
  Title                    = {Size and shape of the distant magnetotail},
  Author                   = {Sibeck, D. G. and Lin, R.-Q.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2014},
  Pages                    = {1028--1043},
  Volume                   = {119},

  Abstract                 = {We employ a global magnetohydrodynamic model to study the effects of the interplanetary magnetic field (IMF) strength and direction upon the cross section of the magnetotail at lunar distances. The anisotropic pressure of draped magnetosheath magnetic field lines and the inclusion of a reconnection-generated standing slow mode wave fan bounded by a rotational discontinuity within the definition of the magnetotail result in cross sections elongated in the direction parallel to the component of the IMF in the plane perpendicular to the Sun-Earth line. Tilted cross-tail plasma sheets separate the northern and southern lobes within these cross sections. Greater fast-mode speeds perpendicular than parallel to the draped magnetosheath magnetic field lines result in greater distances to the bow shock in the direction perpendicular than parallel to the component of the IMF in the plane transverse to the Sun-Earth line. The magnetotail cross section responds rapidly to variations in the IMF orientation. The rotational discontinuity associated with newly reconnected magnetic field lines requires no more than the magnetosheath convection time to appear at any distance downstream, and further adjustments of the cross section in response to the anisotropic pressures of the draped magnetic field lines require no more than 10-20 min. Consequently, for typical ecliptic IMF orientations and strengths, the magnetotail cross section is oblate, while the bow shock is prolate.},
  ISSN                     = {0148-0227},
  Keywords                 = {magnetotail magnetopause bow shock},
  Url                      = {http://adsabs.harvard.edu/abs/2014JGRA..119.1028S}
}

@Article{Sibeck2011a,
  Title                    = {Concerning the motion and orientation of flux transfer events produced by component and antiparallel reconnection},
  Author                   = {Sibeck, D. G. and Lin, R.-Q.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2011},
  Pages                    = {7206},
  Volume                   = {116},

  Abstract                 = {We employ the Cooling et al. (2001) model to predict the location, orientation, motion, and signatures of flux transfer events (FTEs) generated at the solstices and equinoxes along extended subsolar component and high-latitude antiparallel reconnection curves for typical solar wind plasma conditions and various interplanetary magnetic field (IMF) strengths and directions. In general, events generated by the two mechanisms maintain the strikingly different orientations they begin with as they move toward the terminator in opposite pairs of magnetopause quadrants. The curves along which events generated by component reconnection form bow toward the winter cusp. Events generated by antiparallel reconnection form on the equatorial magnetopause during intervals of strongly southward IMF orientation during the equinoxes, form in the winter hemisphere and only reach the dayside equatorial magnetopause during the solstices when the IMF strength is very large and the IMF points strongly southward, never reach the equatorial dayside magnetopause when the IMF has a substantial dawnward or duskward component, and never reach the equatorial flank magnetopause during intervals of northward and dawnward or duskward IMF orientation. Magnetosheath magnetic fields typically have strong components transverse to events generated by component reconnection but only weak components transverse to the axes of events generated by antiparallel reconnection. As a result, much stronger bipolar magnetic field signatures normal to the nominal magnetopause should accompany events generated by component reconnection. The results presented in this paper suggest that events generated by component reconnection predominate on the dayside equatorial and flank magnetopause for most solar wind conditions.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2011JGRA..116.7206S}
}

@Article{Sibeck2010,
  Title                    = {Concerning the motion of flux transfer events generated by component reconnection across the dayside magnetopause},
  Author                   = {Sibeck, D. G. and Lin, R.-Q.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2010},
  Pages                    = {4209},
  Volume                   = {115},

  Abstract                 = {We generate flux transfer events (FTEs) along subsolar component reconnection curves whose tilt depends upon the interplanetary magnetic field (IMF) orientation, track their motion in response to pressure gradient and magnetic curvature forces, and estimate the perturbations they produce in the ambient magnetosheath and magnetosphere. During periods of southward IMF orientation, FTEs move poleward rapidly without ever reaching the flanks of the magnetosphere, while during periods of northward and duskward IMF they slip slowly over the flanks. Speeds increase when a depletion layer is present. For southward IMF orientations, the greatest magnetic field perturbations occur near the equator and diminish with distance from the posited reconnection line. For northward and duskward IMF orientations, dayside perturbation amplitudes are lower but increase with downstream distance at off-equatorial locations. Consequently events occurring for southward IMF orientations should dominate statistical surveys of dayside events but not those of flank events. The events move through the ambient media, invariably generating outward/inward flow perturbations in the magnetosheath but inward/outward perturbations in the magnetosphere. Multipoint spacecraft timing studies can be used to determine event axes and the component of event motion perpendicular to these axes. Because FTEs retain their initial orientations, timing studies afford an opportunity to determine the orientation of the dayside reconnection curve from remote locations.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetic reconnection (7526 7835)},
  Url                      = {http://adsabs.harvard.edu/abs/2010JGRA..115.4209S}
}

@Article{Sibeck1991,
  Title                    = {Solar wind control of the magnetopause shape, location, and motion},
  Author                   = {Sibeck, David G and Lopez, RE and Roelof, EC},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1991},
  Number                   = {A4},
  Pages                    = {5489--5495},
  Volume                   = {96}
}

@Article{Sibeck1987,
  Title                    = {{Magnetic field drift shell splitting - Cause of unusual dayside particle pitch angle distributions during storms and substorms}},
  Author                   = {Sibeck, D G and Mcentire, R W and Lui, a T Y and Lopez, R E and Krimigis, S M},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1987},
  Number                   = {A12},
  Pages                    = {13485--13497},
  Volume                   = {92},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {This paper presents a magnetic field drift shell-splitting model for the unusual butterfly and head-and-shoulder energetic (E greater than 25 keV) particle pitch angle distributions (PADs) which appear deep within the dayside magnetosphere during the course of storms and substorms. Drift shell splitting separates the high and low pitch angle particles in nightside injections as they move to the dayside magnetosphere, so that the higher pitch angle particles move radially away from earth. Consequently, butterfly PADs with a surplus of low pitch angle particles form on the inner edge of the injection, but head-and-shoulder PADs with a surplus of high pitch angle particles form on the outer edge. A similar process removes high pitch angle particles from the inner dayside magnetosphere during storms, leaving the remaining lower pitch angle particles to form butterfly PADs on the inner edge of the ring current. A detailed case and statistical study of Charge Composition Explorer/Medium-energy Particle Analyzer observations, as well as a review of previous work, shows most examples of unusual PADs to be consistent with the model.},
  Doi                      = {10.1029/JA092iA12p13485},
  ISSN                     = {0148-0227},
  Keywords                 = {http://dx.doi.org/10.1029/JA092iA12p13485, doi:10.},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23},
  Url                      = {http://www.agu.org/pubs/crossref/1987/JA092iA12p13485.shtml}
}

@Article{Sibeck1996f,
  Title                    = {Reply},
  Author                   = {Sibeck, David G. and Newell, Patrick T.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1996},
  Pages                    = {13351--13352},
  Volume                   = {101},

  Abstract                 = {Not Available},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: MHD waves and instabilities Magnetospheric Physics: Solar wind/magnetosphere interactions Space Plasma Physics: Magnetic reconnection},
  Url                      = {http://adsabs.harvard.edu/abs/1996JGR...10113351S}
}

@Article{Sibeck1995b,
  Title                    = {Pressure-pulse driven surface waves at the magnetopause: {A} rebuttal},
  Author                   = {Sibeck, D. G. and Newell, P. T.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1995},
  Pages                    = {21773--21778},
  Volume                   = {100},

  Abstract                 = {A variety of mechanisms have been proposed to account for transient events observed in the vicinity of the dayside magnetopause. Discriminating among the various proposed mechanisms is a key objective of magnetospheric physics but requires careful consideration of their predictions. Song et al. (1994) recently reported the results of an effort to determine the characteristics of transient events produced by variations in the solar wind dynamic pressure. Noting that the observed characteristics did not coincide with those they predicted, they concluded that transient events in the vicinity of the dayside magnetopause could not be caused by solar wind dynamic pressure variations. In this rebuttal, we call attention to our previous work concerning the expected characteristics of transient events produced by variations in the solar wind and foreshock pressure; that work uses more realistic parameters to conclude that the transient events are consistent with a solar wind/foreshock pressure mechanism.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetosheath},
  Url                      = {http://adsabs.harvard.edu/abs/1995JGR...10021773S}
}

@Article{Sibeck1995c,
  Title                    = {Interplanetary magnetic field orientation for transient events in the outer magnetosphere},
  Author                   = {Sibeck, D. G. and Newell, P. T.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1995},
  Pages                    = {175--183},
  Volume                   = {100},

  Abstract                 = {It is generally believed that flux transfer events (FTEs) in the outer dayside magneosphere, usually identified by transient (approximately 1 min) bipolar magneitc field perturbations in the direction normal to the nominal magnetopause, occur when the magnetosheath magetic field has a southward component. We compare the results of three methods for determining the magnetosheath magnetic field orientationat the times of previously identified UKS/IRM events: (1) the average magnetosheath magnetic field orientation in the 30-min period adjacent to the nearest magnetopause crossing, (2) the magnetosheath magnetic field orientation observed just outside the magnetopause, and (3) the lagged interplanetary magnetic field (IMF) orientation at the time of the transient events. Whereas the results of method 2 indicate that the events tend to occur for a southward magnetosheath magnetic field, the results of methods 1 and 3 show no such tnedency. The fact that the three methods yield significantly diffeent results emphasizes the need for caution in future studies.},
  ISSN                     = {0148-0227},
  Keywords                 = {Flux Transfer Events Interplanetary Magnetic Fields Magnetic Fields Magnetic Flux Magnetosheath Daytime Directivity Statistical Analysis},
  Url                      = {http://adsabs.harvard.edu/abs/1995JGR...100..175S}
}

@Article{Sibeck2012,
  Title                    = {{Flux transfer events: Motion and signatures}},
  Author                   = {Sibeck, D. G. and Omidi, N.},
  Journal                  = {J. Atmos. Solar-Terrestrial Phys.},
  Year                     = {2012},
  Pages                    = {20--24},
  Volume                   = {87-88},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {We present results from a 2.5 dimensional hybrid code simulation for the evolution of flux transfer events (FTEs) during intervals of due southward interplanetary magnetic field (IMF) orientation. The structures invariably form between pairs of reconnection lines, often remaining nearly stationary on the subsolar magnetopause before their motion begins. Although a few structures move sunward, ultimately coalescing with others, most eventually accelerate antisunward, reaching velocities many times greater than the sound speed in the magnetosheath but only about one Alfv{\'{e}}n speed greater than the ambient magnetosheath flow. At these velocities, slow mode wakes (but not shocks) marked by density enhancements and magnetic field strength decreases extend outward from the structures into the magnetosheath. Upon encountering the cusps, the structures decelerate, undergo reconnection, and are destroyed. ¬© 2011.},
  Doi                      = {10.1016/j.jastp.2011.07.010},
  ISSN                     = {13646826},
  Keywords                 = {Flux transfer events,Magnetopause,Reconnection},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Sibeck2012b,
  Title                    = {Flux transfer events: {Motion} and signatures},
  Author                   = {Sibeck, D. G. and Omidi, N.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2012},

  Month                    = oct,
  Pages                    = {20--24},
  Volume                   = {87},

  Doi                      = {10.1016/j.jastp.2011.07.010}
}

@Article{Sibeck2012c,
  Title                    = {Flux transfer events: {Motion} and signatures},
  Author                   = {Sibeck, D. G. and Omidi, N.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2012},
  Pages                    = {20--24},
  Volume                   = {87},

  Abstract                 = {We present results from a 2.5 dimensional hybrid code simulation for the evolution of flux transfer events (FTEs) during intervals of due southward interplanetary magnetic field (IMF) orientation. The structures invariably form between pairs of reconnection lines, often remaining nearly stationary on the subsolar magnetopause before their motion begins. Although a few structures move sunward, ultimately coalescing with others, most eventually accelerate antisunward, reaching velocities many times greater than the sound speed in the magnetosheath but only about one Alfvén speed greater than the ambient magnetosheath flow. At these velocities, slow mode wakes (but not shocks) marked by density enhancements and magnetic field strength decreases extend outward from the structures into the magnetosheath. Upon encountering the cusps, the structures decelerate, undergo reconnection, and are destroyed.},
  ISSN                     = {1364-6826},
  Url                      = {http://adsabs.harvard.edu/abs/2012JASTP..87...20S}
}

@Article{Sibeck1999,
  Title                    = {{Plasma transfer processes at the magnetopause}},
  Author                   = {Sibeck, D.G. G and Paschmann, G. and Treumann, R. a. and Fuselier, S.a. a and Lennartson, W. and Lockwood, M and Lundin, R. and Ogilvie, K. W. and Onsager, T.G. G and Phan, T.-D. and Roth, M. and Scholer, M and Sckopke, N. and Stasiewicz, K. and Yamauchi, M.},
  Journal                  = {Magnetos. Plasma Sources Losses},
  Year                     = {1999},
  Pages                    = {207--283},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {Final Report of the ISSI Study Project on Source and Loss Processes Series: Space Sciences Series of ISSI, Vol. 6},
  Doi                      = {10.1023/a:1005255801425},
  ISBN                     = {0038-6308},
  ISSN                     = {0038-6308},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Sibeck1999c,
  Title                    = {Chapter 5-{Plasma} {Transfer} {Processes} at the {Magnetopause}},
  Author                   = {Sibeck, D. G. and Paschmann, G. and Treumann, R. A. and Fuselier, S. A. and Lennartsson, W. and Lockwood, M. and Lundin, R. and Ogilvie, K. W. and Onsager, T. G. and Phan, T.-D. and Roth, M. and Scholer, M. and Sckopke, N. and Stasiewicz, K. and Yamauchi, M.},
  Journal                  = {Space Science Reviews},
  Year                     = {1999},
  Pages                    = {207--283},
  Volume                   = {88},

  Abstract                 = {Not Available},
  ISSN                     = {0038-6308},
  Url                      = {http://adsabs.harvard.edu/abs/1999SSRv...88..207S}
}

@Article{Sibeck2002,
  Title                    = {Wind observations of foreshock cavities: {A} case study},
  Author                   = {Sibeck, D. G. and Phan, T.-D. and Lin, R. and Lepping, R. P. and Szabo, A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2002},
  Pages                    = {1271},
  Volume                   = {107},

  Abstract                 = {We present a case study of plasma, energetic particle, and magnetic field perturbations seen by Wind in the dawn foreshock on 19 April 1996. A comparison with the results of hybrid simulations confirms model predictions for a diamagnetic cavity flanked by regions of enhanced density and magnetic field strength but filled with a suprathermal ion population. In contrast to previously reported hot flow anomalies, flow velocities within the foreshock cavities are nearly identical to those in the ambient solar wind, ion temperatures do not rise greatly, thermal pressures are only slightly greater than those in the ambient solar wind, and the events do not lie centered upon interplanetary magnetic field (IMF) tangential discontinuities intersecting the bow shock. We attribute the cavities to the diamagnetic effects of ions Fermi accelerated within the foreshock. A review suggests that foreshock cavities are far more common than hot flow anomalies.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Planetary bow shocks Interplanetary Physics: Energetic particles planetary Magnetospheric Physics: Solar wind/magnetosphere interactions foreshock bow shock cavities pulses energetic ions},
  Url                      = {http://adsabs.harvard.edu/abs/2002JGRA..107.1271S}
}

@Article{Sibeck2000b,
  Title                    = {A survey of {MHD} waves in the magnetosheath: {International} {Solar} {Terrestial} {Program} observations},
  Author                   = {Sibeck, D. G. and Phan, T.-D. and Lin, R. P. and Lepping, R. P. and Mukai, T. and Kokubun, S.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2000},
  Pages                    = {129--138},
  Volume                   = {105},

  Abstract                 = {We present case and statistical studies of magnetohydrodynamic (MHD) fluctuations observed by the Wind and Geotail spacecraft in the Earth's dawn and dusk magnetosheath. A case study with simultaneous IMP 8 interplanetary magnetic field observations confirms theoretical predictions that most of the fluctuations originate in the solar wind rather than at the magnetopause and that the fluctuations can be almost absent from the outer magnetosheath. A second case study indicates that northward plasma velocity perturbations observed in the prenoon magnetosheath correspond to southward velocity perturbations in the postnoon magnetosheath, implying that the MHD perturbations apply a torque to the magnetosphere. A statistical survey reveals that the fluctuations almost invariably propagate antisunward in the magnetosheath, independent of their propagation direction relative to the interplanetary magnetic field.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Planetary bow shocks Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2000JGR...105..129S}
}

@Article{Sibeck2000c,
  Title                    = {Two-point measurements of the magnetopause: {Interball} observations},
  Author                   = {Sibeck, D. G. and Prech, L. and Safrankova, J. and Nemecek, Z.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2000},
  Pages                    = {237--244},
  Volume                   = {105},

  Abstract                 = {The impulsive penetration model predicts that blobs of solar wind plasma penetrate the magnetosphere by becoming detached from the magnetopause. If so, negative radial density gradients should be common near the magnetopause. We present the results of case and statistical studies of simultaneous Interball 1 and Magion 4 omnidirectional plasma sensors (VDP) plasma observations during magnetopause passes. The spacecraft observe very similar features when their interspacing is small. By contrast, the spacecraft located farther radially outward invariably observes densities greater than or equal to those seen at the spacecraft nearer Earth when the interspacing increases. The observations are consistent with the standard interpretation in which a boundary layer of plasma with intermediate densities often lies sandwiched between the magnetosheath and the magnetosphere proper. Blobs of magnetosheath or boundary layer plasma rarely, if ever, become detached from the magnetopause.},
  ISSN                     = {0148-0227},
  Keywords                 = {magnetospheric physics},
  Url                      = {http://adsabs.harvard.edu/abs/2000JGR...105..237S}
}

@Article{Sibeck1997,
  Title                    = {Toward forecasting space weather in the heliosphere},
  Author                   = {Sibeck, D. G. and Richardson, J. D.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1997},
  Pages                    = {14721--14734},
  Volume                   = {102},

  Abstract                 = {We cross correlate years of solar wind ion plasma speed and entropy observations at various sites throughout the heliosphere to determine the conditions under which one spacecraft can be successfully used as a monitor for other spacecraft. Peak correlation coefficients occur when two spacecraft lie radially aligned, although coefficients are generally enhanced during an 2- to 3-month period surrounding alignment. Within the inner heliosphere, the prevalence of corotating solar wind streams can enable useful predictions even when the monitoring spacecraft lies on the other side of the Sun. Similarly, observations at Earth can be useful in predicting conditions in the outer heliosphere to the orbit of Jupiter or even Saturn during periods of near-radial alignment. Observations at Earth cannot be used to successfully predict conditions beyond this distance without considering steepening on the leading edge of streams or stream interactions.},
  ISSN                     = {0148-0227},
  Keywords                 = {Interplanetary Physics: Ejecta driver gases and magnetic clouds Interplanetary Physics: Interplanetary magnetic fields Interplanetary Physics: Solar wind plasma Interplanetary Physics: Sources of the solar wind},
  Url                      = {http://adsabs.harvard.edu/abs/1997JGR...10214721S}
}

@Article{Sibeck1997a,
  Title                    = {A case study of oppositely propagating {Alfvénic} fluctuations in the solar wind and magnetosheath},
  Author                   = {Sibeck, D. G. and Takahashi, K. and Kokubun, S. and Mukai, T. and Ogilvie, K. W. and Szabo, A.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1997},
  Pages                    = {3133--3136},
  Volume                   = {24},

  Abstract                 = {MHD solutions indicate that solar wind Alfvénic fluctuations striking the bow shock should launch a variety of disturbances into the magnetosheath, including both forward (antisunward) and reverse (sunward) propagating Alfvénic fluctuations. We present the first observational evidence of this prediction. This case study presents observations of the Wind spacecraft of Alfvénic fluctuations propagating antisunward along the away sector Parker spiral interplanetary magnetic field (IMF) on April 26 to 27, 1995. Simultaneous Geotail solar wind observations confirm the presence of Alfvénic fluctuations propagating along the spiral IMF, but Geotail magnetosheath observations indicate Alfvénic fluctuations propagating in the opposite direction relative to the draped, prenoon, magnetic field. The reversal in wave propagation direction at the bow shock provides striking evidence for the MHD model of waveshock interaction.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetosheath Interplanetary Physics: Discontinuities Interplanetary Physics: Planetary bow shocks},
  Url                      = {http://adsabs.harvard.edu/abs/1997GeoRL..24.3133S}
}

@Article{Sibeck1998a,
  Title                    = {Concerning the origin of signatures in dayside equatorial ground magnetograms},
  Author                   = {Sibeck, D. G. and Takahashi, K. and Yumoto, K. and Reeves, G. D.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1998},
  Pages                    = {6763--6770},
  Volume                   = {103},

  Abstract                 = {Previous reports suggest that north/south interplanetary magnetic field (IMF) turnings are the predominant cause of north/south fluctuations in dayside equatorial ground magnetograms. We compare 210° Magnetic Meridian (MM) ground magnetograms with simultaneous IMP 8 solar wind and LANL geosynchronous energetic electron observations during 1993 and 1994 to search for this effect. About one third of the northward equatorial magnetic field enhancements can be associated with increases in the solar wind dynamic pressure, a second third with substorm onset as measured by energetic electron injections, and the final third with southward IMF turnings. An alternative explanation can be found for most enhancements associated with north/south IMF variations but not for enhancements associated with solar wind dynamic pressure variations or substorm onsets. Our results suggest that dayside equatorial ground magnetograms may be used to monitor both solar wind dynamic pressure variations and nightside substorm onsets.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: MHD waves and instabilities Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Storms and substorms},
  Url                      = {http://adsabs.harvard.edu/abs/1998JGR...103.6763S}
}

@Article{Sibeck2003a,
  Title                    = {Pressure-pulse interaction with the magnetosphere and ionosphere},
  Author                   = {Sibeck, D. G. and Trivedi, N. B. and Zesta, E. and Decker, R. B. and Singer, H. J. and Szabo, A. and Tachihara, H. and Watermann, J.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2003},
  Pages                    = {1095},
  Volume                   = {108},

  Abstract                 = {We reexamine traveling convection vortices (TCVs) seen by the Magnetometer Array for Cusp and Cleft Studies on 9 November 1993. IMP-8 energetic ion observations confirm that the solar wind pressure variations previously associated with these TCVs were generated by kinetic processes within the Earth's foreshock. As expected during this interval of spiral IMF orientation, fast mode waves launched by the pressure variations first arrived in the equatorial ionosphere near dusk and propagated dawnward. We derive a model for the field-aligned currents generated by transient compressions of the magnetopause and show that it accounts for the number of TCVs seen in the prenoon ionosphere, their sense of rotation, the latitude at which they occur, and their absence in the postnoon ionosphere.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Interplanetary Physics: Planetary bow shocks Magnetospheric Physics: Magnetopause cusp and boundary layers Ionosphere: Ionosphere/magnetosphere interactions (2736) traveling convection vortices pressure pulses},
  Url                      = {http://adsabs.harvard.edu/abs/2003JGRA..108.1095S}
}

@Article{Sigsbee2010,
  Title                    = {Characteristics of {Langmuir} electric field waveforms and power spectra exhibiting nonlinear behavior in {Earth}'s foreshock},
  Author                   = {Sigsbee, K and Kletzing, CA and Pickett, JS and Gurnett, DA and Schwartz, SJ and Lefebvre, B and Lucek, E and Fazakerley, AN and Kucharek, H},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2010},
  Number                   = {A10},
  Volume                   = {115}
}

@Article{Silin2011,
  Title                    = {Hybrid {Fourier}-{Vlasov} simulation in non-inertial reference frames},
  Author                   = {Silin, I. and Sydora, R.},
  Journal                  = {Comput. Phys. Commun.},
  Year                     = {2011},

  Month                    = dec,
  Pages                    = {2508--2518},
  Volume                   = {182},

  Doi                      = {10.1016/j.cpc.2011.07.008}
}

@Article{Simon2012,
  Title                    = {Signals of exomoons in averaged light curves of exoplanets},
  Author                   = {Simon, A. E. and Szab√≥, G. M. and Kiss, L. L. and Szatm√°ry, K.},
  Journal                  = {{\textbackslash}textbackslashmnras},
  Year                     = {2012},

  Month                    = jan,
  Pages                    = {164--171},
  Volume                   = {419},

  Doi                      = {10.1111/j.1365-2966.2011.19682.x},
  Keywords                 = {methods: numerical, planetary systems, planets and satellites: general, TECHNIQUES: PHOTOMETRIC}
}

@Book{Singer2011,
  Title                    = {Space {Weather} {Forcasting} and {Major} {Problems} in {Space} {Weather}.},
  Author                   = {Singer, Howard J},
  Year                     = {2011},
  Month                    = jul,
  Note                     = {Published: PPT in CISM summer school, Boulder , CO
CISM SUMMER SCHOOL 2011},

  Annote                   = {two weeks summer school about Space Weather.},
  Keywords                 = {space weather}
}

@InProceedings{Siscoe1997,
  Title                    = {On storm weakening during substorm expansion phase},
  Author                   = {Siscoe, GL and Petschek, HE},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {1997},
  Pages                    = {211--216},
  Publisher                = {Springer},
  Volume                   = {15}
}

@Article{Sitnov2000,
  Title                    = {Thin current sheet embedded within a thicker plasma sheet: {Self}-consistent kinetic theory},
  Author                   = {Sitnov, MI and Zelenyi, LM and Malova, HV and Sharma, AS},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2000},
  Number                   = {A6},
  Pages                    = {13029--13043},
  Volume                   = {105}
}

@Article{Skillman1971,
  Title                    = {Magnetopause crossing of the geostationary satellite {ATS} 5 at 6.6 {RE}},
  Author                   = {Skillman, Thomas L and Sugiura, Masahisa},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1971},
  Number                   = {1},
  Pages                    = {44--50},
  Volume                   = {76}
}

@Article{Skoug2004,
  Title                    = {Extremely high speed solar wind: 29–30 {October} 2003},
  Author                   = {Skoug, RM and Gosling, JT and Steinberg, JT and McComas, DJ and Smith, CW and Ness, NF and Hu, Q and Burlaga, LF},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2004},
  Number                   = {A9},
  Volume                   = {109}
}

@Article{Skoug1999,
  Title                    = {A prolonged {He}$^{\textrm{+\$}}$ enhancement within a coronal mass ejection in the solar wind},
  Author                   = {Skoug, R. M. and Bame, S. J. and Feldman, W. C. and Gosling, J. T. and McComas, D. J. and Steinberg, J. T. and Tokar, R. L. and Riley, P. and Burlaga, L. F. and Ness, N. F. and Smith, C. W.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {1999},
  Pages                    = {161--164},
  Volume                   = {26},

  Doi                      = {10.1029/1998GL900207},
  Keywords                 = {and Astronomy: Coronal mass ejections, and magnetic clouds, ASTROPHYSICS, driver gases, Interplanetary Physics: Ejecta, Interplanetary Physics: Solar wind plasma, Solar Physics}
}

@InProceedings{Slapak2011,
  Title                    = {O+ heating associated with strong wave activity in the high altitude cusp and mantle},
  Author                   = {Slapak, Rikard and Nilsson, H and Waara, Martin and André, Mats and Stenberg, G and Barghouthi, IA},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2011},
  Pages                    = {931--944},
  Publisher                = {Copernicus GmbH},
  Volume                   = {29}
}

@InProceedings{Slapak2013,
  Title                    = {A statistical study on {O}+ flux in the dayside magnetosheath},
  Author                   = {Slapak, R and Nilsson, H and Westerberg, LG},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2013},
  Pages                    = {1005--1010},
  Publisher                = {Citeseer},
  Volume                   = {31}
}

@Article{Slapak2012,
  Title                    = {Observations of oxygen ions in the dayside magnetosheath associated with southward {IMF}},
  Author                   = {Slapak, R and Nilsson, H and Westerberg, LG and Eriksson, Anders},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2012},
  Number                   = {A7},
  Volume                   = {117}
}

@Article{Slapak2013a,
  Title                    = {A statistical study on {O}+ flux in the dayside magnetosheath},
  Author                   = {Slapak, R. and Nilsson, H. and Westerberg, L. G.},
  Journal                  = {Ann. Geophys},
  Year                     = {2013},
  Pages                    = {1005--1010},
  Volume                   = {31},

  File                     = {[PDF] from psu.edu:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/3UGG397N/Slapak et al. - 2013 - A statistical study on O+ flux in the dayside magn.pdf:application/pdf},
  Url                      = {http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.307.622&rep=rep1&type=pdf},
  Urldate                  = {2015-12-09}
}

@Article{Slavin1981,
  Title                    = {Solar wind flow about the terrestrial planets 1. {Modeling} bow shock position and shape},
  Author                   = {Slavin, James A and Holzer, Robert E},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1981},
  Number                   = {A13},
  Pages                    = {11401--11418},
  Volume                   = {86}
}

@Article{Slavin2003,
  Title                    = {Cluster four spacecraft measurements of small traveling compression regions in the near-tail},
  Author                   = {Slavin, J. A. and Owen, C. J. and Dunlop, M. W. and Borälv, E. and Moldwin, M. B. and Sibeck, D. G. and Tanskanen, E. and Goldstein, M. L. and Fazakerley, A. and Balogh, A. and Lucek, E. and Richter, I. and Reme, H. and Bosqued, J. M.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2003},
  Pages                    = {2208},
  Volume                   = {30},

  Abstract                 = {Cluster observations taken during a substorm on September 19, 2001 have revealed the presence of small traveling compression regions (TCRs) in the near tail. These measurements are used to determine directly the speed and direction of TCR propagation and the amplitude of the underlying bulge in the plasma sheet. The time-of-flight speeds derived from the arrival times of the magnetic perturbations at the different Cluster s/c yielded a mean speed of 413 km/s. For 2 of the TCRs s/c 1, 2 and 4 were located sufficiently close to the plasma sheet that they were immersed in the central plasma sheet plasma as the TCR swept over s/c 3. In this manner the Cluster measurements directly demonstrated that these small TCRs are caused by moving bulges in the plasma sheet-lobe interface. In summary, our analysis of the Cluster measurements has directly demonstrated the existence of moving bulges in the north-south thickness of the plasma sheet, most probably due to the formation of flux ropes, and their role in producing traveling compression regions.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetotail Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Plasma sheet Magnetospheric Physics: Storms and substorms},
  Url                      = {http://adsabs.harvard.edu/abs/2003GeoRL..30.2208S}
}

@Article{Slavin1985,
  Title                    = {Solar wind flow about the outer planets: {Gas} dynamic modeling of the {Jupiter} and {Saturn} bow shocks},
  Author                   = {Slavin, JA and Smith, EJ and Spreiter, JR and Stahara, SS},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1985},
  Number                   = {A7},
  Pages                    = {6275--6286},
  Volume                   = {90}
}

@Article{Slinker2003,
  Title                    = {Simulation of magnetopause oscillations observed {January} 9, 1996},
  Author                   = {Slinker, S. P. and Fedder, J. A. and Sibeck, D. G. and Lyon, J. G. and Frank, L. A. and Mukai, T.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2003},
  Pages                    = {1569},
  Volume                   = {30},

  Abstract                 = {On January 9, 1996, the Geotail spacecraft was near the dusk flank of the magnetopause at 18 MLT. From 0100-0300 UT several short excursions out of the magnetosphere were observed. This time interval was simulated with a 3D MHD magnetosphere model using measured solar wind and IMF data. The simulation produced oscillations resembling those recorded in terms of amplitude and frequency. We describe the details and global nature of the oscillations from the simulation and discuss the most likely source: the Kelvin-Helmholtz instability.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Space Plasma Physics: Numerical simulation studies Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2003GeoRL..30.1569S}
}

@Article{Smith1967,
  Title                    = {Magnetic noise in the magnetosheath in the frequency range 3-300 hz},
  Author                   = {Smith, E. J. and Holzer, R. E. and McLeod, M. G. and Russell, C. T.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1967},

  Month                    = oct,
  Pages                    = {4803--4813},
  Volume                   = {72},

  Doi                      = {10.1029/JZ072i019p04803},
  Keywords                 = {Particles and Fields in the Earth's Magnetosphere: Interaction between solar wind and magnetosphere, Particles and Fields in the Earth's Magnetosphere: Magnetosheath, Particles and Fields in the Earth's Magnetosphere: Wave propagation}
}

@Article{Smith1976,
  Title                    = {Magnetosheath lion roars},
  Author                   = {Smith, E. J. and Tsurutani, B. T.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1976},

  Month                    = may,
  Pages                    = {2261--2266},
  Volume                   = {81},

  Doi                      = {10.1029/JA081i013p02261},
  Keywords                 = {Cyclotron Resonance, Earth Magnetosphere, Extremely Low Frequencies, Geomagnetism, magnetosheath, Ogo-5, Propagation Modes, Wave Generation, Wave Packets, Whistlers}
}

@Article{Smith1996,
  Title                    = {Earth's magnetospheric cusps},
  Author                   = {Smith, MF and Lockwood, M},
  Journal                  = {Rev. Geophys.},
  Year                     = {1996},
  Number                   = {2},
  Pages                    = {233--260},
  Volume                   = {34}
}

@Article{Sokolov2013,
  Title                    = {Magnetohydrodynamic {Waves} and {Coronal} {Heating}: {Unifying} {Empirical} and {MHD} {Turbulence} {Models}},
  Author                   = {Sokolov, I. V. and van der Holst, B. and Oran, R. and Downs, C. and Roussev, I. I. and Jin, M. and Manchester, IV, W. B. and Evans, R. M. and Gombosi, T. I.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2013},

  Month                    = feb,
  Pages                    = {23},
  Volume                   = {764},

  Doi                      = {10.1088/0004-637X/764/1/23},
  Keywords                 = {Solar Wind, Sun: corona, Sun: transition region, Sun: UV Radiation}
}

@Article{Sonett1959,
  Title                    = {Evidence {Concerning} {Instabilities} of the {Distant} {Geomagnetic} {Field} {Pioneer} {I}},
  Author                   = {Sonett, C. P. and Judge, D. L. and Kelso, J. M.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1959},

  Month                    = aug,
  Pages                    = {941--943},
  Volume                   = {64},

  Abstract                 = {Not Available},
  Doi                      = {10.1029/JZ064i008p00941}
}

@Article{Song2000,
  Title                    = {A model of solar wind–magnetosphere–ionosphere coupling for due northward {IMF}},
  Author                   = {Song, P and Gombosi, TI and DeZeeuw, DL and Powell, KG and Groth, CPT},
  Journal                  = {Planetary and space science},
  Year                     = {2000},
  Number                   = {1},
  Pages                    = {29--39},
  Volume                   = {48}
}

@Article{Song1992,
  Title                    = {Model of the formation of the low-latitude boundary layer for strongly northward interplanetary magnetic field},
  Author                   = {Song, P and Russell, CT},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1992},
  Number                   = {A2},
  Pages                    = {1411--1420},
  Volume                   = {97}
}

@Book{Song2001,
  Title                    = {Space weather},
  Author                   = {Song, Paul and Singer, Howard J and Siscoe, George L},
  Publisher                = {American Geophysical Union},
  Year                     = {2001},
  Volume                   = {125}
}

@Article{Sonnerup1981,
  Title                    = {Evidence for magnetic field reconnection at the {Earth}'s magnetopause},
  Author                   = {Sonnerup, BUÖ and Paschmann, G and Papamastorakis, I and Sckopke, N and Haerendel, G and Bame, SJ and Asbridge, JR and Gosling, JT and Russell, CT},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1981},
  Number                   = {A12},
  Pages                    = {10049--10067},
  Volume                   = {86}
}

@InProceedings{SouzaCosta2012,
  Title                    = {Simulation of the {Magnetopause} {Response} to the {April}, 2010 and {April}, 2012 {Events}: {Analysis} of {Possible} {Magnetic} {Reconnection} {Regions}},
  Author                   = {de Souza Costa, C. L. and Alves, M. V. and Jauer, P. R. and Gonzalez, W. D.},
  Booktitle                = {{AGU} {Fall} {Meeting} {Abstracts}},
  Year                     = {2012},
  Pages                    = {2254},
  Volume                   = {1},

  Shorttitle               = {Simulation of the {Magnetopause} {Response} to the {April}, 2010 and {April}, 2012 {Events}},
  Url                      = {http://adsabs.harvard.edu/abs/2012AGUFMSM21A2254D},
  Urldate                  = {2014-10-22}
}

@Article{Spangler1988,
  Title                    = {An observational study of {MHD} wave-induced density fluctuations upstream of the {Earth}'s bow shock},
  Author                   = {Spangler, Steven and Fuselier, Stephen and Fey, Alan and Anderson, Gregory},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1988},
  Number                   = {A2},
  Pages                    = {845--857},
  Volume                   = {93}
}

@Article{Speiser1967,
  Title                    = {Particle trajectories in model current sheets: 2. {Applications} to auroras using a geomagnetic tail model},
  Author                   = {Speiser, Theodore Wesley},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1967},
  Number                   = {15},
  Pages                    = {3919--3932},
  Volume                   = {72}
}

@Article{Spicer2006,
  Title                    = {A {Kopp}-{Pneuman}-like {Picture} of {Coronal} {Mass} {Ejections}},
  Author                   = {Spicer, D. S. and Sibeck, D. and Thompson, B. J. and Davila, J. M.},
  Journal                  = {The Astrophysical Journal},
  Year                     = {2006},
  Pages                    = {1304--1316},
  Volume                   = {643},

  Abstract                 = {A new coronal mass ejection (CME) picture is described that utilizes a number of attributes commonly found operating during magnetotail reconnection events. We first present key observational constraints any final model of CMEs must explain. We then describe how three-dimensional reconnection occurs in the magnetotail and how magnetotail reconnection helps explain a variety of observed CME attributes. We then argue why reconnection, as usually described in the literature, cannot explain the particle acceleration process that occurs during the CME/flare process. Instead we argue that it is the flow fields that are driven by the relaxation of the magnetic stresses due to reconnection that are ultimately the cause of particle acceleration. In particular, it is the electrons that make up the discharging field-aligned currents, which connect flow field-driven cross field inertial currents in the high corona with the chromosphere, that are in fact the high-energy electrons needed to explain flare ribbons and other high-energy emissions. We compute the expected electron fluxes from these current systems and find that they are of order those required. In addition, we discuss betatron acceleration during the dipolarization process that occurs when the flux rope/CME is ejected and how the hot particles generated during the dipolarization process can lead to traps in solar loops, thereby helping to explain long-duration events. Further, we examine whether particle acceleration by shocks can contribute to the mix. We also note that our new picture eliminates a number of paradoxes, specifically elimination of magnetic flux from the Sun and how the Aly conjecture is not of consequence in our picture. Finally, we examine what will be needed to numerically simulate our picture of a CME.},
  ISSN                     = {0004-637X},
  Keywords                 = {Acceleration of Particles Sun: Coronal Mass Ejections (CMEs) Sun: Flares Sun: Particle Emission},
  Url                      = {http://adsabs.harvard.edu/abs/2006ApJ...643.1304S}
}

@Article{Spreiter1995,
  Title                    = {The location of planetary bow shocks: a critical overview of theory and observations},
  Author                   = {Spreiter, John R and Stahara, SS},
  Journal                  = {Advances in Space Research},
  Year                     = {1995},
  Number                   = {8},
  Pages                    = {433--449},
  Volume                   = {15}
}

@Book{Spreiter1984,
  Title                    = {Magnetohydrodynamic and gasdynamic theories for planetary bow waves},
  Author                   = {Spreiter, John R and Stahara, Stephen S},
  Publisher                = {Wiley Online Library},
  Year                     = {1984}
}

@Article{Springel2005,
  Title                    = {Black holes in galaxy mergers: the formation of red elliptical galaxies},
  Author                   = {Springel, Volker and Di Matteo, Tiziana and Hernquist, Lars},
  Journal                  = {The Astrophysical Journal Letters},
  Year                     = {2005},
  Number                   = {2},
  Pages                    = {L79},
  Volume                   = {620}
}

@Article{Stammes2002,
  Title                    = {{OMI} algorithm theoretical basis document volume {III}: clouds, aerosols, and surface {UV} irradiance},
  Author                   = {Stammes, P and Noordhoek, R},
  Journal                  = {Accessed December},
  Year                     = {2002},
  Pages                    = {2012},
  Volume                   = {1}
}

@Article{Stasiewicz2000,
  Title                    = {Stochastic {Ion} {Heating} by {Orbit} {Chaotization} on {Electrostatic} {Waves} and {Nonlinear} {Structures}},
  Author                   = {Stasiewicz, K. and Lundin, R. and Marklund, G.},
  Journal                  = {Physica Scripta Volume T},
  Year                     = {2000},
  Pages                    = {60--63},
  Volume                   = {84},

  Doi                      = {10.1238/Physica.Topical.084a00060},
  Keywords                 = {52.35.Ra, 94.20.Rs}
}

@Article{Stasiewicz2000a,
  Title                    = {Stochastic {Ion} {Heating} by {Orbit} {Chaotization} on {Electrostatic} {Waves} and {Nonlinear} {Structures}},
  Author                   = {Stasiewicz, K. and Lundin, R. and Marklund, G.},
  Journal                  = {Physica Scripta Volume T},
  Year                     = {2000},
  Pages                    = {60--63},
  Volume                   = {84},

  Doi                      = {10.1238/Physica.Topical.084a00060},
  Keywords                 = {52.35.Ra, 94.20.Rs}
}

@Article{Steiger1993,
  Title                    = {Solar wind composition and expectations for high solar latitudes},
  Author                   = {von Steiger, Rudolf and Geiss, Johannes},
  Journal                  = {Advances in Space Research},
  Year                     = {1993},

  Month                    = jun,
  Pages                    = {63--74},
  Volume                   = {13},

  Doi                      = {10.1016/0273-1177(93)90392-O},
  Keywords                 = {EXTREME ULTRAVIOLET RADIATION, INTERPLANETARY MEDIUM, LATITUDE, Plasma Composition, Solar Wind, Ulysses Mission}
}

@Article{Steiger1995,
  Title                    = {Kinetic {Properties} of {Heavy} {Ions} in the {Solar} {Wind} {From} {SWICS}/{Ulysses}},
  Author                   = {von Steiger, R. and Geiss, Johannes and Gloeckler, George and Galvin, A. B.},
  Journal                  = {ßr},
  Year                     = {1995},

  Month                    = apr,
  Pages                    = {71--76},
  Volume                   = {72},

  Doi                      = {10.1007/BF00768756},
  Keywords                 = {Heavy Ions, Solar Wind, Ulysses}
}

@Article{Steiger2000,
  Title                    = {Composition of quasi-stationary solar wind flows from {Ulysses}/{Solar} {Wind} {Ion} {Composition} {Spectrometer}},
  Author                   = {von Steiger, R. and Schwadron, N. A. and Fisk, L. A. and Geiss, J. and Gloeckler, G. and Hefti, S. and Wilken, B. and Wimmer-Schweingruber, R. F. and Zurbuchen, T. H.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {2000},

  Month                    = dec,
  Pages                    = {27217--27238},
  Volume                   = {105},

  Doi                      = {10.1029/1999JA000358},
  Keywords                 = {Interplanetary Physics: Instruments and techniques, Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Sources of the solar wind}
}

@Article{Steiger1995a,
  Title                    = {Abundance variations in the solar wind},
  Author                   = {von Steiger, R. and Schweingruber, R. F. W. and Geiss, J. and Gloeckler, G.},
  Journal                  = {Advances in Space Research},
  Year                     = {1995},

  Month                    = jul,
  Pages                    = {3--},
  Volume                   = {15},

  Keywords                 = {Abundance, Coronal holes, Helium, Ionization Potentials, Magnesium, Mass Spectrometers, Oxygen, Photosphere, Solar Atmosphere, Solar Temperature, Solar Wind, Solar Wind Velocity, Stellar Mass Ejection, Stellar Models, Ulysses Mission, Variations}
}

@Article{Steiger2011,
  Title                    = {Polar coronal holes during the past solar cycle: {Ulysses} observations},
  Author                   = {von Steiger, R. and Zurbuchen, T. H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2011},

  Month                    = jan,
  Pages                    = {1105},
  Volume                   = {116},

  Doi                      = {10.1029/2010JA015835},
  Keywords                 = {and Astronomy: Coronal holes, ASTROPHYSICS, Interplanetary Physics: Solar cycle variations (7536), Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Solar wind sources, Solar Physics}
}

@InProceedings{Steiger2005,
  Title                    = {Latitude {Distribution} of {Interplanetary} {Coronal} {Mass} {Ejections} during {Solar} {Maximum}},
  Author                   = {von Steiger, R. and Zurbuchen, T. H. and Kilchenmann, A.},
  Booktitle                = {Solar {Wind} 11/{SOHO} 16, {Connecting} {Sun} and {Heliosphere}},
  Year                     = {2005},
  Editor                   = {Fleck, B. and Zurbuchen, T. H. and Lacoste, H.},
  Month                    = sep,
  Pages                    = {317},
  Series                   = {{ESA} {Special} {Publication}},
  Volume                   = {592}
}

@Article{Steiger2010,
  Title                    = {Oxygen flux in the solar wind: {Ulysses} observations},
  Author                   = {von Steiger, R. and Zurbuchen, T. H. and McComas, D. J.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {2010},

  Month                    = nov,
  Pages                    = {22101},
  Volume                   = {37},

  Doi                      = {10.1029/2010GL045389},
  Keywords                 = {Interplanetary Physics: Solar cycle variations (7536), Interplanetary Physics: Solar wind plasma, Interplanetary Physics: Solar wind sources}
}

@InCollection{Stone1998,
  Title                    = {The advanced composition explorer},
  Author                   = {Stone, EC and Frandsen, AM and Mewaldt, RA and Christian, ER and Margolies, D and Ormes, JF and Snow, F},
  Booktitle                = {The {Advanced} {Composition} {Explorer} {Mission}},
  Publisher                = {Springer},
  Year                     = {1998},
  Pages                    = {1--22},

  Url                      = {http://link.springer.com/chapter/10.1007/978-94-011-4762-0_1}
}

@Article{Strumik2011,
  Title                    = {Comparison of {Heliospheric} {Models} with {Observations} of the {Voyager} and {IBEX} {Spacecraft}},
  Author                   = {Strumik, M. and Ben-Jaffel, L. and Ratkiewicz, R. and Grygorczuk, J.},
  Journal                  = {{\textbackslash}apjl},
  Year                     = {2011},

  Month                    = nov,
  Pages                    = {L6},
  Volume                   = {741},

  Doi                      = {10.1088/2041-8205/741/1/L6},
  Keywords                 = {INTERPLANETARY MEDIUM, Magnetic Fields, Solar Wind, Sun: heliosphere}
}

@Article{Strumik2011a,
  Title                    = {Comparison of heliospheric models with observations of the {Voyager} and {IBEX} spacecraft},
  Author                   = {Strumik, M and Ben-Jaffel, L and Ratkiewicz, R and Grygorczuk, J},
  Journal                  = {The Astrophysical Journal Letters},
  Year                     = {2011},
  Number                   = {1},
  Pages                    = {L6},
  Volume                   = {741}
}

@Book{Sturrock1994,
  Title                    = {Plasma {Physics}: an introduction to the theory of astrophysical, geophysical and laboratory plasmas},
  Author                   = {Sturrock, Peter Andrew},
  Publisher                = {Cambridge University Press},
  Year                     = {1994}
}

@Article{Su1998,
  Title                    = {Polar wind survey with the thermal ion dynamics experiment/plasma source instrument suite aboard {POLAR}},
  Author                   = {Su, YJ and Horwitz, JL and Moore, TE},
  Journal                  = {{\textbackslash}ldots Sp. Phys. (1978 {\textbackslash}ldots},
  Year                     = {1998},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/98JA02662/full}
}

@Article{Suess1999,
  Title                    = {Ulysses-{UVCS} {Coordinated} {Observations}},
  Author                   = {Suess, S. T. and Poletto, G. and Corti, G. and Simnett, G. and Noci, G. and Romoli, M. and Kohl, J. and Goldstein, B.},
  Journal                  = {ßr},
  Year                     = {1999},

  Month                    = jan,
  Pages                    = {319--322},
  Volume                   = {87},

  Doi                      = {10.1023/A:1005197812354},
  Keywords                 = {SOHO, streamers, Ulysses}
}

@Article{Suess2000,
  Title                    = {The {May} 1997 {SOHO}-{Ulysses} quadrature},
  Author                   = {Suess, S. T. and Poletto, G. and Romoli, M. and Neugebauer, M. and Goldstein, B. E. and Simnett, G.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {2000},

  Month                    = nov,
  Pages                    = {25033--25052},
  Volume                   = {105},

  Doi                      = {10.1029/2000JA000044},
  Keywords                 = {and Astronomy: Corona, ASTROPHYSICS, Interplanetary Physics: Sources of the solar wind, Solar Physics}
}

@Article{Sun2014,
  Title                    = {The current system associated with the boundary of plasma bubbles},
  Author                   = {Sun, Wei-jie and Fu, Suiyan and Pu, Zuyin and Parks, George K and Slavin, James A and Yao, Zhonghua and Zong, Qiu-gang and Shi, Quanqi and Zhao, Duo and Cui, Yanbo},
  Year                     = {2014},
  Pages                    = {1--7},

  Doi                      = {10.1002/2014GL062171.Abstract},
  Keywords                 = {10.1002/2014GL062171 and current system, boundary, plasma bubble}
}

@Article{Suvorova1999,
  Title                    = {{Dayside magnetopause models}},
  Author                   = {Suvorova, A. V. and Dmitriev, A. V. and Kuznetsov, S. N.},
  Journal                  = {Radiat. Meas.},
  Year                     = {1999},
  Number                   = {5},
  Pages                    = {687--692},
  Volume                   = {30},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {A review of empirical data-based models of the magnetopause and a comparative analysis are given with special attention to the dynamics of the dayside boundary. Recently different research groups have presented new magnetopause models as an alternative to the model of Roelof and Sibeck (1993, J. Geophys. Res. 94, 15, 125). All models have a greater parametric extent than the model of Roelof and Sibeck and allow prediction of the magnetopause location during extreme solar wind and IMF conditions. The models of Shue et al. (1997, J. Geophys. Res. 102, 9497-9511) and Kuznetsov et al. (1998), developed using classic multi-factor regression analysis are two-dimensional and bivariate. The model of Dmitriev et al. (1999) created using artificial neural networks (ANNs) is three-dimensional and contains multiple parameters. A statistical study of Kuznetsov et al. confirmed by the ANN modeling of Dmitriev et al. has shown that the shape of dayside magnetopause has dawn-dusk asymmetry. The uncertainty in the determination of the dayside magnetopause position is practically the same for these models in spite of some discrepancies of the model results caused by different data sets, different assumptions and functional forms, different treatment methods of the models.},
  Doi                      = {10.1016/S1350-4487(99)00220-6},
  ISSN                     = {13504487},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Suvorova2010,
  Title                    = {Magnetopause expansions for quasi-radial interplanetary magnetic field: {THEMIS} and {Geotail} observations},
  Author                   = {Suvorova, A. V. and Shue, J.-H. and Dmitriev, A. V. and Sibeck, D. G. and McFadden, J. P. and Hasegawa, H. and Ackerson, K. and Jelínek, K. and Šafránková, J. and Němeček, Z.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2010},
  Pages                    = {10216},
  Volume                   = {115},

  Abstract                 = {We report Time History of Events and Macroscale Interactions during Substorms (THEMIS) and Geotail observations of prolonged magnetopause (MP) expansions during long-lasting intervals of quasi-radial interplanetary magnetic field (IMF) and nearly constant solar wind dynamic pressure. The expansions were global: The magnetopause was located more than 3 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} and ˜7 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} outside its nominal dayside and magnetotail locations, respectively. The expanded states persisted several hours, just as long as the quasi-radial IMF conditions, indicating steady state situations. For an observed solar wind pressure of ˜1.1-1.3 nPa, the new equilibrium subsolar MP position lay at ˜14.5 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater}, far beyond its expected location. The equilibrium position was affected by geomagnetic activity. The magnetopause expansions result from significant decreases in the total pressure of the high-β magnetosheath, which we term the low-pressure magnetosheath (LPM) mode. A prominent LPM mode was observed for upstream conditions characterized by IMF cone angles less than 20°-25°, high Mach numbers and proton plasma β ≤ 1.3. The minimum value for the total pressure observed by THEMIS in the magnetosheath adjacent to the magnetopause was 0.16 nPa and the fraction of the solar wind pressure applied to the magnetopause was therefore 0.2, extremely small. The equilibrium location of the magnetopause was modulated by a nearly continuous wavy motion over a wide range of time and space scales.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Magnetosphere: outer},
  Url                      = {http://adsabs.harvard.edu/abs/2010JGRA..11510216S}
}

@Article{Suzuki2006,
  Title                    = {Solar winds driven by nonlinear low-frequency {Alfvén} waves from the photosphere: {Parametric} study for fast/slow winds and disappearance of solar winds},
  Author                   = {Suzuki, T. K. and Inutsuka, S.-I.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2006},

  Month                    = jun,
  Pages                    = {6101},
  Volume                   = {111},

  Doi                      = {10.1029/2005JA011502},
  Keywords                 = {2752, 6050), 6944), and Astronomy: Corona, and Astronomy: Coronal holes, ASTROPHYSICS, corona, Solar Physics, Solar Wind, Space Plasma Physics: Kinetic waves and instabilities, Space Plasma Physics: MHD waves and instabilities (2149, Space Plasma Physics: Nonlinear phenomena (4400, waves}
}

@Article{Toth2005a,
  Title                    = {{Space Weather Modeling Framework: A new tool for the space science community}},
  Author                   = {T{\'{o}}th, G{\'{a}}bor and Sokolov, Igor V and Gombosi, Tamas I and Chesney, David R and Clauer, C Robert and {De Zeeuw}, Darren L and Hansen, Kenneth C and Kane, Kevin J and Manchester, Ward B and Oehmke, Robert C and Others},
  Journal                  = {J. Geophys. Res. Sp. Phys.},
  Year                     = {2005},
  Number                   = {A12},
  Volume                   = {110},

  __markedentry            = {[suleimanbaraka:6]},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/T{\'{o}}th et al/Journal of Geophysical Research Space Physics (1978--2012)/T{\'{o}}th et al. - 2005 - Space Weather Modeling Framework A new tool for the space science community.pdf:pdf},
  Owner                    = {suleimanbaraka},
  Publisher                = {Wiley Online Library},
  Timestamp                = {2016.02.23}
}

@Article{Takahashi1991,
  Title                    = {{ULF} waves in the low-latitude boundary layer and their relationship to magnetospheric pulsations: {A} multisatellite observation},
  Author                   = {Takahashi, Kazue and Sibeck, David G and Newell, Patrick T and Spence, Harlan E},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1991},
  Number                   = {A6},
  Pages                    = {9503--9519},
  Volume                   = {96}
}

@Article{Takizuka1977,
  Title                    = {A binary collision model for plasma simulation with a particle code},
  Author                   = {Takizuka, Tomonor and Abe, Hirotada},
  Journal                  = {J. Comput. Phys.},
  Year                     = {1977},
  Number                   = {3},
  Pages                    = {205--219},
  Volume                   = {25}
}

@Article{Talaat1999,
  Title                    = {Nonmigrating diurnal tides in mesospheric and lower-thermospheric winds and temperatures},
  Author                   = {Talaat, Elsayed R and Lieberman, Ruth S},
  Journal                  = {J. Atmos. Sci.},
  Year                     = {1999},
  Number                   = {24},
  Pages                    = {4073--4087},
  Volume                   = {56}
}

@Article{Tam2007,
  Title                    = {Kinetic modeling of the polar wind},
  Author                   = {Tam, Sunny WY and Chang, T. and Pierrard, V.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2007},
  Number                   = {16},
  Pages                    = {1984--2027},
  Volume                   = {69},

  File                     = {Snapshot:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/KKRD9R5G/S1364682607002428.html:text/html},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S1364682607002428},
  Urldate                  = {2015-12-09}
}

@Article{Tam1995,
  Title                    = {Self-consistent kinetic photoelectron effects on the polar wind},
  Author                   = {Tam, Sunny WY and Yasseen, Fareed and Chang, Tom and Ganguli, Supriya B},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1995},
  Number                   = {16},
  Pages                    = {2107--2110},
  Volume                   = {22},

  Annote                   = {Added to JabRef: 2015.04.18}
}

@Article{Tam2007a,
  Title                    = {Kinetic modeling of the polar wind},
  Author                   = {Tam, S. W Y and Chang, T. and Pierrard, V.},
  Journal                  = {J. Atmos. Solar-Terrestrial Phys.},
  Year                     = {2007},
  Pages                    = {1984--2027},
  Volume                   = {69},

  Abstract                 = {The polar wind, a plasma outflow along open geomagnetic field lines from the Earth's ionosphere, has been the subject of many theoretical studies. Since the proposal of its existence more than 30 years ago, the polar wind has been described by various theoretical modeling approaches. In this paper, we first describe the two traditional modeling approaches for the classical polar wind: moment-based models and collisionless kinetic calculations; and discuss how other models of the outflow were formed by combining these two traditional approaches. We then discuss how kinetic calculations have been improved to take into account the effects of Coulomb collisions, which may contribute to the formation of double-peaked H+ velocity distributions in the polar wind. As observations of escaping O+ fluxes have guided theoreticians to go beyond the classical polar wind description, we discuss how models were modified or constructed in order to take into account the various non-classical effects, including those due to photoelectrons, which may also provide an explanation for the satellite observations of day-night asymmetries in addition to the acceleration of the O+ ions. {\textbackslash}copyright 2007 Elsevier Ltd. All rights reserved.},
  Doi                      = {10.1016/j.jastp.2007.08.006},
  ISSN                     = {13646826},
  Keywords                 = {Coulomb collisions, Fluid models, Hybrid models, ion acceleration, kinetic models, Photoelectrons}
}

@Article{Tanaka1983,
  Title                    = {A source of the backstreaming ion beams in the foreshock region},
  Author                   = {Tanaka, Motohiko and Goodrich, CC and Winske, D and Papadopoulos, K},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1983},
  Number                   = {A4},
  Pages                    = {3046--3054},
  Volume                   = {88}
}

@Article{Tanaka1983a,
  Title                    = {{A Source of the Backstreaming Ion Beams in the Foreshock Region A i " Reflected " Quasi-Perpendicu Bow Shock Magnetic}},
  Author                   = {Tanaka, Motohiko and Goodrich, C C and Winske, D and Papadopoulos, K},
  Year                     = {1983},
  Number                   = {3},
  Pages                    = {3046--3054},
  Volume                   = {88},

  __markedentry            = {[suleimanbaraka:6]},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Tanaka et al/Unknown/Tanaka et al. - 1983 - A Source of the Backstreaming Ion Beams in the Foreshock Region A i Reflected Quasi-Perpendicu Bow Shock Magnet.pdf:pdf},
  Keywords                 = {http://dx.doi.org/10.1029/JA088iA04p03046, doi:10.},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Tanaka1999,
  Title                    = {Configuration of the magnetosphere-ionosphere convection system under northward {IMF} conditions with nonzero {IMF} {B} y},
  Author                   = {Tanaka, T},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1999},
  Number                   = {A7},
  Pages                    = {14683--14690},
  Volume                   = {104}
}

@Article{Tanaka1995,
  Title                    = {Generation mechanisms for magnetosphere-ionosphere current systems deduced from a three-dimensional {MHD} simulation of the solar wind-magnetosphere-ionosphere coupling processes},
  Author                   = {Tanaka, T},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1995},
  Number                   = {A7},
  Pages                    = {12057--12074},
  Volume                   = {100}
}

@Article{Tang2013,
  Title                    = {{THEMIS} observations of the magnetopause electron diffusion region: {Large} amplitude waves and heated electrons},
  Author                   = {Tang, Xiangwei and Cattell, Cynthia and Dombeck, John and Dai, Lei and Wilson, Lynn B. and Breneman, Aaron and Hupach, Adam},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2013},
  Number                   = {12},
  Pages                    = {2884--2890},
  Volume                   = {40},

  Shorttitle               = {{THEMIS} observations of the magnetopause electron diffusion region},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1002/grl.50565/full},
  Urldate                  = {2014-10-22}
}

@Article{Tanskanen2006,
  Title                    = {Surface ultraviolet irradiance from {OMI}},
  Author                   = {Tanskanen, Aapo and Krotkov, Nickolay A. and Herman, Jay R. and Arola, Antti},
  Journal                  = {Geoscience and Remote Sensing, IEEE Transactions on},
  Year                     = {2006},
  Number                   = {5},
  Pages                    = {1267--1271},
  Volume                   = {44},

  Url                      = {http://ieeexplore.ieee.org/xpls/abs_all.jsp?arnumber=1624605},
  Urldate                  = {2014-11-13}
}

@Article{Tanskanen2007,
  Title                    = {Validation of daily erythemal doses from {Ozone} {Monitoring} {Instrument} with ground-based {UV} measurement data},
  Author                   = {Tanskanen, Aapo and Lindfors, Anders and M‚Äö√†√∂¬¨√ü‚Äö√†√∂¬¨√ütt‚Äö√†√∂¬¨√ü, Anu and Krotkov, Nickolay and Herman, Jay and Kaurola, Jussi and Koskela, Tapani and Lakkala, Kaisa and Fioletov, Vitali and Bernhard, Germar and {others}},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2007},
  Number                   = {D24},
  Volume                   = {112},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2007JD008830/full},
  Urldate                  = {2014-11-13}
}

@Article{Tanskanen2005,
  Title                    = {Magnetotail response to prolonged southward {IMF} {Bz} intervals: {Loading}, unloading, and continuous magnetospheric dissipation},
  Author                   = {Tanskanen, E. I. and Slavin, J. A. and Fairfield, D. H. and Sibeck, D. G. and Gjerloev, J. and Mukai, T. and Ieda, A. and Nagai, T.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2005},
  Pages                    = {3216},
  Volume                   = {110},

  Abstract                 = {The response of the Earth's magnetotail to prolonged southward interplanetary magnetic field (IMF) has been determined for the three Geotail magnetotail seasons from November to April, 1999-2002. We examine the total magnetotail pressure P{\textless}SUB{\textgreater}T,tail{\textless}/SUB{\textgreater} = B{\textless}SUP{\textgreater}2{\textless}/SUP{\textgreater}/2μ{\textless}SUB{\textgreater}0{\textless}/SUB{\textgreater} + N{\textless}SUB{\textgreater}i{\textless}/SUB{\textgreater}kT{\textless}SUB{\textgreater}i{\textless}/SUB{\textgreater} because variations should be similar in this parameter in the lobes and in the plasma sheet. We found 13 events when IMF B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} remained southward for 8 hours or longer and Geotail was located within the magnetotail farther than 10 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} downstream. All 13 events were subdivided into separate intervals characterized as (1) loading, if the tail total pressure increased more than 100\%; (2) unloading, if the total pressure decreased by more than 50\%; and (3) what we term here continuous magnetospheric dissipation (CMD), if the tail total pressure increased by less than 100\% and/or decreased less than 50\% during the entire mode interval. In total, 37 loading, 37 unloading, and 28 CMD events were found. The plasma sheet magnetic flux transfer rate, ϕ{\textless}SUB{\textgreater}Earth{\textless}/SUB{\textgreater} ≈ v{\textless}SUB{\textgreater}x{\textless}/SUB{\textgreater} · B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater}, and plasma bulk velocity has been analyzed to determine the steadiness of the plasma sheet convection. Plasma sheet convection was found to be highly disturbed and intense plasma flows (BBFs and FBs) were observed during all convection states. However, the occurence rate and amplitude of plasma flows distinguish loading-unloading and continuous dissipation periods from each other. BBFs seem to be more numerous (135) but weaker (about 500 km/s) during continuous dissipation intervals compared with BBFs existing during unloading mode (61 and 660 km/s). Finally, it was found that CMD-type convection is more likely when the mean southward IMF B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} {\textgreater} -5 nT, while loading-unloading is more likely when IMF B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} {\textless} -5 nT.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Plasma convection (2463) Magnetospheric Physics: Magnetotail Magnetospheric Physics: Plasma sheet Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Solar wind/magnetosphere interactions magnetospheric convection plasma sheet loading unloading and continuous magnetospheric dissipation},
  Url                      = {http://adsabs.harvard.edu/abs/2005JGRA..110.3216T}
}

@Article{Tarduno2010,
  Title                    = {{Geodynamo, solar wind, and magnetopause 3.4 to 3.45 billion years ago}},
  Author                   = {Tarduno, J A and Cottrell, R D and Watkeys, M K and Hofmann, A and Doubrovine, P V and Mamajek, E E and Liu, D and Sibeck, D G and Neukirch, L P and Usui, Y},
  Journal                  = {Science (80-. ).},
  Year                     = {2010},
  Number                   = {5970},
  Pages                    = {1238--1240},
  Volume                   = {327},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {Stellar wind standoff by a planetary magnetic field prevents atmospheric erosion and water loss. Although the early Earth retained its water and atmosphere, and thus evolved as a habitable planet, little is known about Earth's magnetic field strength during that time. We report paleointensity results from single silicate crystals bearing magnetic inclusions that record a geodynamo 3.4 to 3.45 billion years ago. The measured field strength is approximately 50 to 70{\%} that of the present-day field. When combined with a greater Paleoarchean solar wind pressure, the paleofield strength data suggest steady-state magnetopause standoff distances of < or = 5 Earth radii, similar to values observed during recent coronal mass ejection events. The data also suggest lower-latitude aurora and increases in polar cap area, as well as heating, expansion, and volatile loss from the exosphere that would have affected long-term atmospheric composition.},
  Doi                      = {10.1126/science.1183445},
  ISBN                     = {1095-9203 (Electronic)$\backslash$r0036-8075 (Linking)},
  ISSN                     = {0036-8075},
  Owner                    = {suleimanbaraka},
  Pmid                     = {20203044},
  Timestamp                = {2016.02.23},
  Url                      = {http://www.ncbi.nlm.nih.gov/pubmed/20203044}
}

@Article{Tarduno2010a,
  Title                    = {Geodynamo, {Solar} {Wind}, and {Magnetopause} 3.4 to 3.45 {Billion} {Years} {Ago}},
  Author                   = {Tarduno, John A. and Cottrell, Rory D. and Watkeys, Michael K. and Hofmann, Axel and Doubrovine, Pavel V. and Mamajek, Eric E. and Liu, Dunji and Sibeck, David G. and Neukirch, Levi P. and Usui, Yoichi},
  Journal                  = {Science},
  Year                     = {2010},
  Pages                    = {1238--},
  Volume                   = {327},

  Abstract                 = {Stellar wind standoff by a planetary magnetic field prevents atmospheric erosion and water loss. Although the early Earth retained its water and atmosphere, and thus evolved as a habitable planet, little is known about Earth’s magnetic field strength during that time. We report paleointensity results from single silicate crystals bearing magnetic inclusions that record a geodynamo 3.4 to 3.45 billion years ago. The measured field strength is 50 to 70\% that of the present-day field. When combined with a greater Paleoarchean solar wind pressure, the paleofield strength data suggest steady-state magnetopause standoff distances of ≤5 Earth radii, similar to values observed during recent coronal mass ejection events. The data also suggest lower-latitude aurora and increases in polar cap area, as well as heating, expansion, and volatile loss from the exosphere that would have affected long-term atmospheric composition.},
  ISSN                     = {0036-8075},
  Url                      = {http://adsabs.harvard.edu/abs/2010Sci...327.1238T}
}

@Article{Taubenschuss2010,
  Title                    = {The role of magnetic handedness in magnetic cloud propagation},
  Author                   = {Taubenschuss, U. and Erkaev, N. V. and Biernat, H. K. and Farrugia, C. J. and Möstl, C. and Amerstorfer, U. V.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2010},

  Month                    = may,
  Pages                    = {1075--1100},
  Volume                   = {28},

  Doi                      = {10.5194/angeo-28-1075-2010}
}

@Article{TenBarge2013,
  Title                    = {Collisionless {Reconnection} in the {Large} {Guide} {Field} {Regime}: {Gyrokinetic} {Versus} {Particle}-in-{Cell} {Simulations}},
  Author                   = {TenBarge, J. M. and Daughton, W. and Karimabadi, H. and Howes, G. G. and Dorland, W.},
  Journal                  = {arXiv preprint arXiv:1312.5166},
  Year                     = {2013},

  Shorttitle               = {Collisionless {Reconnection} in the {Large} {Guide} {Field} {Regime}},
  Url                      = {http://arxiv.org/abs/1312.5166},
  Urldate                  = {2014-05-31}
}

@Article{Teraki2011,
  Title                    = {A {Novel} {Emission} {Spectrum} from a {Relativistic} {Electron} {Moving} in a {Random} {Magnetic} {Field}},
  Author                   = {Teraki, Y. and Takahara, F.},
  Journal                  = {{\textbackslash}apjl},
  Year                     = {2011},

  Month                    = jul,
  Pages                    = {L44},
  Volume                   = {735},

  Doi                      = {10.1088/2041-8205/735/2/L44},
  Keywords                 = {gamma-ray burst: general, Magnetic Fields, radiation mechanisms: general, turbulence}
}

@InCollection{Thomas2004,
  Title                    = {The {Io} neutral clouds and plasma torus},
  Author                   = {Thomas, N. and Bagenal, F. and Hill, T. W. and Wilson, J. K.},
  Booktitle                = {Jupiter. {The} {Planet}, {Satellites} and {Magnetosphere}},
  Year                     = {2004},
  Editor                   = {Bagenal, F. and Dowling, T. E. and McKinnon, W. B.},
  Pages                    = {561--591},

  Keywords                 = {Io: Plasmasphere, Jupiter Satellites: Io}
}

@Article{Thomsen1988,
  Title                    = {On the origin of hot diamagnetic cavities near the {Earth}'s bow shock},
  Author                   = {Thomsen, MF and Gosling, JT and Bame, SJ and Quest, KB and Russell, CT and Fuselier, SA},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1988},
  Number                   = {A10},
  Pages                    = {11311--11325},
  Volume                   = {93}
}

@Book{Tidman1971,
  Title                    = {Shock waves in collisionless plasmas},
  Author                   = {Tidman, Derek A and Krall, Nicholas A},
  Publisher                = {Wiley-Interscience New York},
  Year                     = {1971}
}

@Article{Topliss2001,
  Title                    = {Charge neutrality and ion conic distributions at the equatorward electron edge of the midaltitude cusp},
  Author                   = {Topliss, S. and Johnstone, A. and Coates, A. and Peterson, W. K. and Kletzing, C. A. and Russell, C. T.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {2001},

  Month                    = oct,
  Pages                    = {21095--21108},
  Volume                   = {106},

  Doi                      = {10.1029/2000JA003032},
  Keywords                 = {and boundary layers, cusp, magnetospheric physics, Magnetospheric Physics: Magnetopause, Space Plasma Physics, Space Plasma Physics: Wave/particle interactions}
}

@Article{Topliss2001a,
  Title                    = {Charge neutrality and ion conic distributions at the equatorward electron edge of the midaltitude cusp},
  Author                   = {Topliss, S. and Johnstone, A. and Coates, A. and Peterson, W. K. and Kletzing, C. A. and Russell, C. T.},
  Journal                  = {{\textbackslash}textbackslashjgr},
  Year                     = {2001},

  Month                    = oct,
  Pages                    = {21095--21108},
  Volume                   = {106},

  Doi                      = {10.1029/2000JA003032},
  Keywords                 = {and boundary layers, cusp, magnetospheric physics, Magnetospheric Physics: Magnetopause, Space Plasma Physics, Space Plasma Physics: Wave/particle interactions}
}

@Article{Torres2007,
  Title                    = {Aerosols and surface {UV} products from {Ozone} {Monitoring} {Instrument} observations: {An} overview},
  Author                   = {Torres, Omar and Tanskanen, Aapo and Veihelmann, Ben and Ahn, Changwoo and Braak, Remco and Bhartia, Pawan K. and Veefkind, Pepijn and Levelt, Pieternel},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2007},
  Number                   = {D24},
  Volume                   = {112},

  Shorttitle               = {Aerosols and surface {UV} products from {Ozone} {Monitoring} {Instrument} observations},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2007JD008809/full},
  Urldate                  = {2014-11-13}
}

@Article{Toth2007,
  Title                    = {Sun-to-thermosphere simulation of the 28–30 {October} 2003 storm with the {Space} {Weather} {Modeling} {Framework}},
  Author                   = {Toth, Gabor and De Zeeuw, Darren L and Gombosi, Tamas I and Manchester, Ward B and Ridley, Aaron J and Sokolov, Igor V and Roussev, Ilia I},
  Journal                  = {Space Weather},
  Year                     = {2007},
  Number                   = {6},
  Volume                   = {5}
}

@Article{Toth2005,
  Title                    = {Space {Weather} {Modeling} {Framework}: {A} new tool for the space science community},
  Author                   = {Tóth, Gábor and Sokolov, Igor V and Gombosi, Tamas I and Chesney, David R and Clauer, C Robert and De Zeeuw, Darren L and Hansen, Kenneth C and Kane, Kevin J and Manchester, Ward B and Oehmke, Robert C and {others}},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2005},
  Number                   = {A12},
  Volume                   = {110}
}

@Article{Treumann2009,
  Title                    = {Fundamentals of collisionless shocks for astrophysical application, 1. {Non}-relativistic shocks},
  Author                   = {Treumann, RA},
  Journal                  = {The Astronomy and Astrophysics Review},
  Year                     = {2009},
  Number                   = {4},
  Pages                    = {409--535},
  Volume                   = {17}
}

@Article{Treumann2014,
  Title                    = {The strongest magnetic fields in the universe: how strong can they become?},
  Author                   = {Treumann, Rudolf a. and Baumjohann, Wolfgang and Balogh, AndrÃ¬¨¬®¬¨¬©},
  Journal                  = {Front. Phys.},
  Year                     = {2014},
  Number                   = {October},
  Pages                    = {1--4},
  Volume                   = {2},

  Doi                      = {10.3389/fphy.2014.00059},
  ISSN                     = {2296-424X},
  Keywords                 = {aharonov-bohm-scaling, electron radius, flux quanta, magnetars, neutron stars, pulsars, quantum limit, strong magnetic fields},
  Url                      = {http://journal.frontiersin.org/article/10.3389/fphy.2014.00059/abstract}
}

@Article{Treumann2008,
  Title                    = {Planetary bow shocks},
  Author                   = {Treumann, RA and Jaroschek, CH},
  Journal                  = {arXiv preprint arXiv:0808.1701},
  Year                     = {2008}
}

@Article{Trivedi2002,
  Title                    = {Signatures of traveling convection vortices in ground magnetograms under the equatorial electrojet},
  Author                   = {Trivedi, N. B. and Sibeck, D. G. and Zesta, E. and Santos, J. C. and Yumoto, K. and Kitamura, T. and Shinohara, M. and Dutra, S. L. G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2002},
  Pages                    = {1087},
  Volume                   = {107},

  Abstract                 = {Traveling convection vortices (TCVs) are transient events in high-latitude ground magnetograms that can be interpreted as evidence for localized vortical flows in the high-latitude ionosphere. Their centers travel eastward or westward at geomagnetic latitudes near 72° to 74°. TCVs have been attributed to various transient interactions at the magnetopause but also to processes occurring deeper within the magnetosphere. Each interaction mechanism should launch shear Alfvén waves that produce high-latitude ground signatures but also compressional waves that should produce signatures at lower latitudes. Zesta et al. [1999], Moretto et al. [1997], Ridley et al. [1998], and Lühr et al. [1998] report detailed analyses for several high-latitude TCVs. In this paper, we present evidence for corresponding signatures at Belem, São Luis, and Teresina and other stations under or nearby the equatorial electrojet. The equatorial signatures are most pronounced when the high-latitude signatures are (1) longitudinally extended, (2) isolated, and (3) attain greatest amplitudes.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Magnetopause cusp and boundary layers Magnetospheric Physics: Magnetosphere/ionosphere interactions Magnetospheric Physics: Plasma convection Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2002JGRA..107.1087T}
}

@Article{Tsurutani2004,
  Title                    = {Global dayside ionospheric uplift and enhancement associated with interplanetary electric fields},
  Author                   = {Tsurutani, B. and Mannucci, A. and Iijima, B. and Abdu, M. A. and Sobral, J. H. A. and Gonzalez, W. and Guarnieri, F. and Tsuda, T. and Saito, A. and Yumoto, K. and Fejer, B. and Fuller-Rowell, T. J. and Kozyra, J. and Foster, J. C. and Coster, A. and Vasyliunas, V. M.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},

  Month                    = aug,
  Pages                    = {8302},
  Volume                   = {109},

  Doi                      = {10.1029/2003JA010342},
  Keywords                 = {Interplanetary Physics: Interplanetary magnetic fields, ionosphere, Ionosphere: Equatorial ionosphere, Ionosphere: Ionosphere/magnetosphere interactions (2736), Ionosphere: Ionospheric disturbances, Ionosphere: Midlatitude ionosphere, magnetic storms, magnetosphere ionosphere coupling, solar wind-ionosphere coupling}
}

@Article{Tsyganenko1994,
  Title                    = {Concerning flux erosion from the dayside magnetosphere},
  Author                   = {Tsyganenko, N. A. and Sibeck, D. G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1994},
  Pages                    = {13425},
  Volume                   = {99},

  Abstract                 = {The dayside magnetopause moves inward during periods of southward interplanetary magnetic field in response to decreases in the outer magnetospheric magnetic field strength. We consider possible causes for the magnetic field strength decreases and demonstrate that they are consistent with increases in the region 1 Birkeland and cross-tail currents. We reexamine the well-known series of magnetopause crossings by OGO 5 on March 27, 1968, to demonstrate that they provide evidence for two intervals of gradual inward magnetopause motion associated with magnetic flux erosion and also for two intervals of inward magnetopause motion associated with sharp increases in the solar wind dynamic pressure.},
  ISSN                     = {0148-0227},
  Keywords                 = {Birkeland Currents Geomagnetic Tail Geomagnetism Interplanetary Magnetic Fields Magnetic Field Reconnection Magnetopause Ogo-5 Plasma Pressure Solar Terrestrial Interactions Solar Wind},
  Url                      = {http://adsabs.harvard.edu/abs/1994JGR....9913425T}
}

@Article{Tsyganenko1994a,
  Title                    = {Concerning flux erosion from the dayside magnetosphere},
  Author                   = {Tsyganenko, NA and Sibeck, DG},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1994},
  Number                   = {A7},
  Pages                    = {13425--13436},
  Volume                   = {99}
}

@Article{Tu1997,
  Title                    = {Two-{Fluid} {Model} for {Heating} of the {Solar} {Corona} and {Acceleration} of the {Solar} {Wind} by {High}-{Frequency} {Alfven} {Waves}},
  Author                   = {Tu, C.-Y. and Marsch, E.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {1997},

  Month                    = apr,
  Pages                    = {363--391},
  Volume                   = {171},

  Doi                      = {10.1023/A:1004968327196}
}

@Book{Tukey1977,
  Title                    = {Exploratory data analysis},
  Author                   = {Tukey, J. W.},
  Year                     = {1977}
}

@Article{Tulunay2005,
  Title                    = {Forecasting magnetopause crossing locations by using {Neural} {Networks}},
  Author                   = {Tulunay, Y. and Sibeck, D. G. and Senalp, E. T. and Tulunay, E.},
  Journal                  = {Advances in Space Research},
  Year                     = {2005},
  Pages                    = {2378--2383},
  Volume                   = {36},

  Abstract                 = {Given the highly complex and nonlinear nature of Near Earth Space processes, mathematical modeling of these processes is usually difficult or impossible. In such cases, modeling methods involving Artificial Intelligence may be employed. We demonstrate that data driven models, such as the Neural Network based approach, shows promise in its ability to forecast or predict the behavior of these processes. In this paper, modeling studies for forecasting magnetopause crossing locations are summarized and a Neural Network algorithm is presented to describe the nonlinear time-dependent response of the subsolar region of the magnetopause to varying solar wind conditions. In our approach the past history of the solar wind has, for the first time to the best knowledge of the authors, been included in forecasting the subsolar region of the magnetopause. It is proposed that the data driven approach is a valid approach to understanding and modeling the physical phenomena of Near Earth Space. The only basic requirement for the data driven approach is the availability of representative data for the phenomena. The objective of this paper is to demonstrate that by using WIND and GEOTAIL satellite data a Neural Network based model can be adapted to the modeling of the Earth’s magnetopause.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/2005AdSpR..36.2378T}
}

@Article{Tuerk2003,
  Title                    = {Search for plasma and magnetic field cavities in magnetosheath},
  Author                   = {Türk, Filiz and Kaymaz, Zerefşan and Sibeck, David G.},
  Journal                  = {Advances in Space Research},
  Year                     = {2003},
  Pages                    = {1455--1462},
  Volume                   = {31},

  Abstract                 = {In the solar wind, foreshock cavities create depressed magnetic field and density regions associated with high energetic particles due bow shock related processes. In this study, we searched for the presence of foreshock-type transient events in the magnetosheath using Interball-1 spacecraft data. In our search of four years of magnetosheath magnetic field, density, temperature, velocity and proton flux data, we have not found signatures of these cavities. The relation between magnetosheath parameters and energetic particles is not clearly revelaed in Interball-1 data. While these events are very clear and commonly found in the solar wind, why they are not observed in the magnetosheath emposes an interesting and challenging question on the evolution of these solar wind structures and their relation to the magnetosheath dynamics.},
  ISSN                     = {0273-1177},
  Url                      = {http://adsabs.harvard.edu/abs/2003AdSpR..31.1455T}
}

@Article{Turner2011,
  Title                    = {First {Observations} of a {Foreshock} {Bubble} at {Earth}: {Implications} for {Magnetospheric} {Activity} and {Energetic} {Particle} {Acceleration}},
  Author                   = {Turner, DL and Omidi, N and Sibeck, DG and Angelopoulos, V},
  Year                     = {2011}
}

@Article{Turner2011a,
  Title                    = {Multispacecraft observations of a foreshock-induced magnetopause disturbance exhibiting distinct plasma flows and an intense density compression},
  Author                   = {Turner, D. L. and Eriksson, S. and Phan, T. D. and Angelopoulos, V. and Tu, W. and Liu, W. and Li, X. and Teh, W.-L. and McFadden, J. P. and Glassmeier, K.-H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2011},

  Month                    = apr,
  Pages                    = {4230},
  Volume                   = {116},

  Doi                      = {10.1029/2010JA015668},
  Keywords                 = {7526), Space Plasma Physics: Magnetic reconnection (2723, Space Plasma Physics: Plasma energization, Space Plasma Physics: Transport processes}
}

@Article{Turner2013,
  Title                    = {First observations of foreshock bubbles upstream of {Earth}'s bow shock: {Characteristics} and comparisons to {HFAs}},
  Author                   = {Turner, D. L. and Omidi, N. and Sibeck, D. G. and Angelopoulos, V.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},
  Pages                    = {1552--1570},
  Volume                   = {118},

  Abstract                 = {Using multipoint in situ observations upstream of Earth's bow shock from the THEMIS mission, we present the first observations of foreshock bubbles (FBs) and compare them to observations of hot flow anomalies (HFAs). FBs are recently conceptualized kinetic phenomena that can form under the commonplace condition of a rotational discontinuity in the interplanetary magnetic field interacting with backstreaming energetic ions in Earth's quasi-parallel foreshock. FBs may have remained elusive until now due to their many observational similarities to HFAs and the lack of coordinated multipoint measurements. Here we introduce identification criteria for distinguishing between HFAs and FBs using in situ observations, and use them to analyze five example events that occurred on Bastille Day (14 July) and 11-12 August 2008. Three of these events satisfy the criteria for FBs and are inconsistent with multiple criteria for HFAs. The remaining two events are consistent with the traditional picture of HFAs. Furthermore, FBs involve two converging shocks, and using these events, we demonstrate their effectiveness at particle acceleration. Considering that their formation conditions are not extraordinary, FBs may be ubiquitous at collisionless, quasi-parallel shocks in a variety of astrophysical settings.},
  ISSN                     = {0148-0227},
  Keywords                 = {Ion foreshock Particle acceleration Kinetic phenomena},
  Url                      = {http://adsabs.harvard.edu/abs/2013JGRA..118.1552T}
}

@Article{Ukhorskiy2011,
  Title                    = {{Radiation belt storm probes: Resolving fundamental physics with practical consequences}},
  Author                   = {Ukhorskiy, Aleksandr Y. and Mauk, Barry H. and Fox, Nicola J. and Sibeck, David G. and Grebowsky, Joseph M.},
  Journal                  = {J. Atmos. Solar-Terrestrial Phys.},
  Year                     = {2011},
  Number                   = {11-12},
  Pages                    = {1417--1424},
  Volume                   = {73},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {The fundamental processes that energize, transport, and cause the loss of charged particles operate throughout the universe at locations as diverse as magnetized planets, the solar wind, our Sun, and other stars. The same processes operate within our immediate environment, the Earth's radiation belts. The Radiation Belt Storm Probes (RBSP) mission will provide coordinated two-spacecraft observations to obtain understanding of these fundamental processes controlling the dynamic variability of the near-Earth radiation environment. In this paper we discuss some of the profound mysteries of the radiation belt physics that will be addressed by RBSP and briefly describe the mission and its goals. ¬© 2010 Elsevier Ltd.},
  Doi                      = {10.1016/j.jastp.2010.12.005},
  ISSN                     = {13646826},
  Keywords                 = {Radiation belts,Space weather},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Ukhorskiy2011a,
  Title                    = {Radiation belt storm probes: {Resolving} fundamental physics with practical consequences},
  Author                   = {Ukhorskiy, Aleksandr Y. and Mauk, Barry H. and Fox, Nicola J. and Sibeck, David G. and Grebowsky, Joseph M.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2011},
  Pages                    = {1417--1424},
  Volume                   = {73},

  Abstract                 = {The fundamental processes that energize, transport, and cause the loss of charged particles operate throughout the universe at locations as diverse as magnetized planets, the solar wind, our Sun, and other stars. The same processes operate within our immediate environment, the Earth's radiation belts. The Radiation Belt Storm Probes (RBSP) mission will provide coordinated two-spacecraft observations to obtain understanding of these fundamental processes controlling the dynamic variability of the near-Earth radiation environment. In this paper we discuss some of the profound mysteries of the radiation belt physics that will be addressed by RBSP and briefly describe the mission and its goals.},
  ISSN                     = {1364-6826},
  Url                      = {http://adsabs.harvard.edu/abs/2011JASTP..73.1417U}
}

@Article{Ukhorskiy2008,
  Title                    = {Preface},
  Author                   = {Ukhorskiy, A. Y. and O'Brien, T. P. and Sibeck, D. G.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2008},
  Pages                    = {5},
  Volume                   = {70},

  Abstract                 = {Not Available},
  ISSN                     = {1364-6826},
  Url                      = {http://adsabs.harvard.edu/abs/2008JASTP..70D...5U}
}

@Article{Umeda2012,
  Title                    = {Microinstabilities at perpendicular collisionless shocks: {A} comparison of full particle simulations with different ion to electron mass ratio},
  Author                   = {Umeda, T. and Kidani, Y. and Matsukiyo, S. and Yamazaki, R.},
  Journal                  = {Phys. Plasmas},
  Year                     = {2012},

  Month                    = apr,
  Number                   = {4},
  Pages                    = {042109},
  Volume                   = {19},

  Doi                      = {10.1063/1.3703319},
  Keywords                 = {drift instability, Electromagnetic waves, Mach number, Microinstabilities, Particle-in-cell method, plasma shock waves, plasma simulation, plasma transport processes, Shock waves and discontinuities, Transport Properties, Whistlers}
}

@Article{Umeda2010,
  Title                    = {On the reformation at quasi-and exactly perpendicular shocks: {Full} particle-in-cell simulations},
  Author                   = {Umeda, Takayuki and Kidani, Yoshitaka and Yamao, Masahiro and Matsukiyo, Shuichi and Yamazaki, Ryo},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2010},
  Number                   = {A10},
  Volume                   = {115}
}

@InProceedings{Urbar2015,
  Title                    = {Two-point observations of solar wind beam deceleration upstream the {Earth} bow shock},
  Author                   = {Urbar, Jaroslav and Nemecek, Zdenek and Safrankova, Jana and Prech, Lubomir and Jelinek, Karel},
  Booktitle                = {{EGU} {General} {Assembly} {Conference} {Abstracts}},
  Year                     = {2015},
  Pages                    = {9946},
  Volume                   = {17},

  File                     = {Snapshot:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/BXI7KU3Q/2015EGUGA..17.html:text/html},
  Url                      = {http://adsabs.harvard.edu/abs/2015EGUGA..17.9946U},
  Urldate                  = {2016-01-11}
}

@Article{Uritsky2014,
  Title                    = {Active current sheets and candidate hot flow anomalies upstream of {Mercury}'s bow shock},
  Author                   = {Uritsky, V. M. and Slavin, J. A. and Boardsen, S. A. and Sundberg, T. and Raines, J. M. and Gershman, D. J. and Collinson, G. and Sibeck, D. and Khazanov, G. V. and Anderson, B. J. and Korth, H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2014},
  Pages                    = {853--876},
  Volume                   = {119},

  Abstract                 = {Hot flow anomalies (HFAs) represent a subset of solar wind discontinuities interacting with collisionless bow shocks. They are typically formed when the normal component of the motional (convective) electric field points toward the embedded current sheet on at least one of its sides. The core region of an HFA contains hot and highly deflected ion flows and rather low and turbulent magnetic field. In this paper, we report observations of possible HFA-like events at Mercury identified over a course of two planetary years. Using data from the orbital phase of the MESSENGER mission, we identify a representative ensemble of active current sheets magnetically connected to Mercury's bow shock. We show that some of these events exhibit magnetic and particle signatures of HFAs similar to those observed at other planets, and present their key physical characteristics. Our analysis suggests that Mercury's bow shock does not only mediate the flow of supersonic solar wind plasma but also provides conditions for local particle acceleration and heating as predicted by previous numerical simulations. Together with earlier observations of HFA activity at Earth, Venus, Mars, and Saturn, our results confirm that hot flow anomalies could be a common property of planetary bow shocks and show that the characteristic size of these events is controlled by the bow shock standoff distance and/or local solar wind conditions.},
  ISSN                     = {0148-0227},
  Keywords                 = {solar wind MESSENGER mission bow shock hot flow anomaly Mercury's magnetosphere},
  Url                      = {http://adsabs.harvard.edu/abs/2014JGRA..119..853U}
}

@Article{Usami2013,
  Title                    = {Development of multi-hierarchy simulation model with non-uniform space grids for collisionless driven reconnection},
  Author                   = {Usami, Shunsuke and Horiuchi, Ritoku and Ohtani, Hiroaki and Den, Mitsue},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2013},
  Number                   = {6},
  Pages                    = {061208},
  Volume                   = {20},

  Url                      = {http://scitation.aip.org/content/aip/journal/pop/20/6/10.1063/1.4811121},
  Urldate                  = {2014-05-31}
}

@Article{Usmanov2003,
  Title                    = {A tilted-dipole {MHD} model of the solar corona and solar wind},
  Author                   = {Usmanov, A. V. and Goldstein, M. L.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2003},

  Month                    = sep,
  Pages                    = {1354},
  Volume                   = {108},

  Doi                      = {10.1029/2002JA009777},
  Keywords                 = {and Astronomy: Solar activity cycle (2162), ASTROPHYSICS, Coronal holes, Interplanetary Physics: Corotating streams, Interplanetary Physics: Interplanetary magnetic fields, Interplanetary Physics: Sources of the solar wind, MHD simulation, Solar Physics, solar wind sources, solar wind structure, Ulysses, Wang-Sheeley model}
}

@Article{Vaisberg1976,
  Title                    = {Solar wind and magnetosheath observations at earth during {August} 1972},
  Author                   = {Vaisberg, O. L. and Zastenker, G. N.},
  Journal                  = {ßr},
  Year                     = {1976},

  Month                    = nov,
  Pages                    = {687--702},
  Volume                   = {19},

  Doi                      = {10.1007/BF00210646},
  Keywords                 = {Heos B Satellite, INTERPLANETARY MEDIUM, Magnetopause, magnetosheath, Magnetospheric Instability, Magnetospheric Ion Density, Plasma Density, Satellite Observation, Shock Wave Propagation, Solar Flares, Solar Wind}
}

@Article{Valin2011,
  Title                    = {Effects of model spatial resolution on the interpretation of satellite {NO} 2 observations},
  Author                   = {Valin, L. C. and Russell, A. R. and Hudman, R. C. and Cohen, R. C.},
  Journal                  = {Atmospheric Chemistry and Physics Discussions},
  Year                     = {2011},
  Number                   = {7},
  Pages                    = {20245--20265},
  Volume                   = {11},

  Url                      = {http://www.atmos-chem-phys-discuss.net/11/20245/2011/acpd-11-20245-2011.html},
  Urldate                  = {2014-11-13}
}

@Article{Valks2011,
  Title                    = {Operational total and tropospheric {NO}2 column retrieval for {GOME}-2},
  Author                   = {Valks, P. and Pinardi, G. and Richter, A. and Lambert, J. C. and Hao, N. and Loyola, D. and Van Roozendael, M. and Emmadi, S.},
  Journal                  = {Atmos. Meas. Tech. Discuss},
  Year                     = {2011},
  Pages                    = {1617--1676},
  Volume                   = {4},

  Url                      = {http://www.researchgate.net/publication/225025272_Operational_total_and_tropospheric_NO2_column_retrieval_for_GOME-2/file/d912f50e087808d527.pdf},
  Urldate                  = {2014-11-13}
}

@Article{Vapirev2013,
  Title                    = {Formation of a transient front structure near reconnection point in 3-{D} {PIC} simulations},
  Author                   = {Vapirev, AE and Lapenta, G and Divin, A and Markidis, S and Henri, P and Goldman, M and Newman, D},
  Journal                  = {Journal of Geophysical Research: Space Physics},
  Year                     = {2013}
}

@Article{Vasilkov2008,
  Title                    = {Evaluation of the {OMI} cloud pressures derived from rotational {Raman} scattering by comparisons with other satellite data and radiative transfer simulations},
  Author                   = {Vasilkov, Alexander and Joiner, Joanna and Spurr, Robert and Bhartia, Pawan K. and Levelt, Pieternel and Stephens, Graeme},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2008},
  Number                   = {D15},
  Volume                   = {113},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2007JD008689/full},
  Urldate                  = {2014-11-13}
}

@Article{Verigin1999,
  Title                    = {Shape and location of planetary bow shocks.},
  Author                   = {Verigin, MI and Kotova, GA and Remizov, AP and Styazhkin, VA and Shutte, NM and Zhang, T-L and Riedler, W and Rosenbauer, H and Szegö, K and Tatrallyay, M and {others}},
  Journal                  = {Kosmicheskie Issledovaniia},
  Year                     = {1999},
  Pages                    = {38--43},
  Volume                   = {37}
}

@Article{Verigin2001,
  Title                    = {Analysis of the 3-{D} shape of the terrestrial bow shock by {Interball}/{Magion} 4 observations},
  Author                   = {Verigin, MI and Kotova, GA and Slavin, J and Szabo, A and Kessel, M and Safrankova, J and Nemecek, Z and Gombosi, TI and Kabin, K and Shugaev, F and {others}},
  Journal                  = {Advances in Space Research},
  Year                     = {2001},
  Number                   = {6},
  Pages                    = {857--862},
  Volume                   = {28}
}

@Article{Verigin2003,
  Title                    = {Planetary bow shocks: {Gasdynamic} analytic approach},
  Author                   = {Verigin, M and Slavin, J and Szabo, A and Gombosi, T and Kotova, G and Plochova, O and Szegö, K and Tátrallyay, M and Kabin, K and Shugaev, F},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2003},
  Number                   = {A8},
  Volume                   = {108}
}

@Article{Verigin2003a,
  Title                    = {Planetary bow shocks: {Asymptotic} {MHD} {Mach} cones},
  Author                   = {Verigin, M and Slavin, J and Szabo, A and Kotova, G and Gombosi, T},
  Journal                  = {Earth, planets and space},
  Year                     = {2003},
  Number                   = {1},
  Pages                    = {33--38},
  Volume                   = {55}
}

@Article{Vidotto2010,
  Title                    = {Early {UV} {Ingress} in {WASP}-12b: {Measuring} {Planetary} {Magnetic} {Fields}},
  Author                   = {Vidotto, A. A. and Jardine, M. and Helling, C.},
  Journal                  = {{\textbackslash}textbackslashapjl},
  Year                     = {2010},

  Month                    = oct,
  Pages                    = {L168--L172},
  Volume                   = {722},

  Doi                      = {10.1088/2041-8205/722/2/L168},
  Keywords                 = {outflows, planets and satellites: individual: WASP-12b, planets and satellites: magnetic fields, planet-star interactions, stars: coronae, stars: individual: WASP-12, stars: winds}
}

@Article{Vijayaraghavan2008,
  Title                    = {Practical aspects of using satellite data in air quality modeling},
  Author                   = {Vijayaraghavan, Krish and Snell, Hilary E. and Seigneur, Christian},
  Journal                  = {Environmental science \& technology},
  Year                     = {2008},
  Number                   = {22},
  Pages                    = {8187--8192},
  Volume                   = {42},

  Url                      = {http://pubs.acs.org/doi/full/10.1021/es7031339},
  Urldate                  = {2014-11-13}
}

@Article{Villasenor1992,
  Title                    = {Rigorous charge conservation for local electromagnetic field solvers},
  Author                   = {Villasenor, John and Buneman, Oscar},
  Journal                  = {Comput. Phys. Commun.},
  Year                     = {1992},
  Number                   = {2},
  Pages                    = {306--316},
  Volume                   = {69}
}

@Article{Vincent2011,
  Title                    = {Updated {Analysis} of the {Upwind} {Interplanetary} {Hydrogen} {Velocity} as {Observed} by the {Hubble} {Space} {Telescope} during {Solar} {Cycle} 23},
  Author                   = {Vincent, F. E. and Ben-Jaffel, L. and Harris, W. M.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2011},

  Month                    = sep,
  Pages                    = {135},
  Volume                   = {738},

  Doi                      = {10.1088/0004-637X/738/2/135},
  Keywords                 = {INTERPLANETARY MEDIUM, Sun: activity, ULTRAVIOLET: ISM}
}

@Article{Vincent2014,
  Title                    = {Observations of the {Interplanetary} {Hydrogen} during {Solar} {Cycles} 23 and 24. {What} can {We} {Deduce} about the {Local} {Interstellar} {Medium}?},
  Author                   = {Vincent, Frédéric E and Katushkina, Olga and Ben-Jaffel, Lotfi and Harris, Walter M and Izmodenov, Vladislav and Quémerais, Eric and Koutroumpa, Dimitra and Clarke, John},
  Journal                  = {The Astrophysical Journal Letters},
  Year                     = {2014},
  Number                   = {2},
  Pages                    = {L25},
  Volume                   = {788}
}

@Article{Vo1994,
  Title                    = {Multipoint observations of a dayside transient event},
  Author                   = {Vo, H. B. and Murphree, J. S. and Elphinstone, R. D. and Elphic, R. C. and Friis-Christensen, E. and Luhr, H. and Sibeck, D. G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1994},
  Pages                    = {13409},
  Volume                   = {99},

  Abstract                 = {Many different processes may take place at the magnetopause. To distinguish the various mechanisms requires simultaneous multipoint observations in the dayside magnetosphere. Such coincident observations were made by a number of spacecraft located in the solar wind, at the magnetopause, at geosynchronous orbit, and at polar orbit on September 23, 1986. Beginning at 1110 UT, the B(sub z) component of the Interplanetary Magnetic Field (IMF) underwent three periodic cycles, each with a duration of about 7 min, and there were 4 solar wind pressure pulses with a period of 10 min, as recorded by the Interplanetary Monitroing Platform (IMP) 8 satellite. The International Sun Earth Explorer (ISEE) satellite pair crossed the magnetopause near local noon at 1125 UT and recorded two bipolar events in the normal component of the magnetic field at 1115 and 1120 UT. In addition, ISEE 1 observed a bipolar event at 1118 UT that ISEE 2 did not. Periodic oscillations and compressions of the magnetic field were then subsequently seen at geosynchronous orbit in the dawn sector. Greenland magnetometer stations also located in the morning sector recorded transient responses to the solar wind pressure pulses. The East Coast stations (near local noon) apparently observed a different vortex at 1122 UT. Viking auroral images show an activation of a localized feature poleward of the dayside auroral distribution at 1122 UT. An auroral enhancement, seen at 1128 UT in the afternoon sector, moved eastward at a speed of 5 km/sec and decayed in intensity by 1141 UT. Clear Pc 5 pulsations were seen equatorward of this activation. Differences in both in situ measurements and ionospheric responses to the two bipolar events lead to the conclusion that the 1118 UT event can be interpreted as being associated with reconnection at the same time that the magnetopause was in motion.},
  ISSN                     = {0148-0227},
  Keywords                 = {Auroras Field Aligned Currents Geomagnetic Pulsations Geosynchronous Orbits Interplanetary Magnetic Fields Magnetic Field Reconnection Magnetopause Vortices Explorer 50 Satellite International Sun Earth Explorers Magnetosphere-Ionosphere Coupling Solar Terrestrial Interactions Solar Wind},
  Url                      = {http://adsabs.harvard.edu/abs/1994JGR....9913409V}
}

@Article{Vorobjev2001,
  Title                    = {Aurora conjugacy during substorms: {Coordinated} {Antarctic} ground and {Polar} {Ultraviolet} observations},
  Author                   = {Vorobjev, V. G. and Yagodkina, O. I. and Sibeck, D. and Liou, K. and Meng, C.-I.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2001},
  Pages                    = {24579--24592},
  Volume                   = {106},

  Abstract                 = {Simultaneous optical observations at the Antarctic station Mirny (Φ{\textless}SUP{\textgreater}'{\textless}/SUP{\textgreater}=-77.4° Corrected geomagnetic latitude (CGL)) and Ultraviolet Imager images of the northern auroral oval from the POLAR satellite were used to determine the displacement of nightside aurorae in the Northern Hemisphere relative to those in the Southern Hemisphere during 10 (1.5 to 3 hour long) time intervals including auroral substorms. Displacements of the poleward edge of the auroral bulge can be significant, up to 5{\textless}SUP{\textgreater}0{\textless}/SUP{\textgreater} in CGL. The sense and magnitude of displacements are not related to the dipole tilt angle or differing ionospheric conductivity in the two hemispheres but rather to interplanetary magnetic field (IMF) orientations in the ecliptic plane. Aurorae reach higher latitudes in the Northern Hemisphere when Bx{\textless}0 and By{\textgreater}0 but occur at higher latitudes in the Southern Hemisphere when Bx{\textgreater}0 and By{\textless}0. Perturbations in conjugate ground magnetometers display a similar asymmetry. By contrast, displacements of the aurora are small when the IMF strength is weak, the IMF orientation fluctuates, or the IMF has an orthospiral orientation. Even when the latitudes are similar, local bright auroral forms and transient intensifications often occur in only one hemisphere. Our results testify to the effective penetration of the equatorial component of the IMF into the magnetosphere.},
  ISSN                     = {0148-0227},
  Keywords                 = {Ionosphere: Auroral ionosphere Magnetospheric Physics: Auroral phenomena Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2001JGR...10624579V}
}

@Article{Vorobjev2001a,
  Title                    = {Polar {UVI} observations of dayside auroral transient events},
  Author                   = {Vorobjev, V. G. and Yagodkina, O. I. and Sibeck, D. G. and Liou, K. and Meng, C.-I.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2001},
  Pages                    = {28897--28912},
  Volume                   = {106},

  Abstract                 = {We analyze Polar Ultraviolet Imager (UVI) observations of auroral transient events (ATEs) in the dayside Northern Hemisphere. During 5 winter months in 1996 and 1997, we found 31 prenoon ATEs but only 13 afternoon events. Prenoon and afternoon event characteristics differ. Prenoon ATEs generally appear as bright spots of auroral luminosity in the area from 0800 to 1000 magnetic local time (MLT) and 74.5° and 76.5° corrected geomagnetic latitude (CGL). Bright aurorae then quickly expand westward and poleward, accompanied by high-latitude magnetic impulsive events (MIE) and traveling convection vortices (TCV). Afternoon ATEs usually appear as a sudden intensification of aurorae in the area from 1400 to 1600 MLT and 75.5° to 78.5° CGL. Within 15-20 min the bright band of luminosity extends eastward to reach 2000-2100 MLT at 70°-72° CGL. Although midlatitude and low-latitude ground magnetograms in the evening sector record increases in the horizontal component of the magnetic field, no corresponding features occur at stations in the morning sector. Afternoon ATEs correspond to abrupt changes in the interplanetary magnetic field (IMF) orientation, but not to significant variations of the solar wind dynamic pressure, indicating that the auroral transient events occur as part of the magnetospheric response to abrupt changes in the foreshock geometry.},
  ISSN                     = {0148-0227},
  Keywords                 = {Ionosphere: Auroral ionosphere Magnetospheric Physics: Auroral phenomena Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2001JGR...10628897V}
}

@Article{Vorobjev1999,
  Title                    = {Daytime high-latitude auroral pulsations: {Some} morphological features and the region of the magnetospheric source},
  Author                   = {Vorobjev, V. G. and Yagodkina, O. I. and Sibeck, D. G. and Newell, P.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1999},
  Pages                    = {10135--10144},
  Volume                   = {104},

  Abstract                 = {We present the results of a statistical study of auroral pulsations observed at cusp and cleft latitudes as a function of solar wind and geomagnetic conditions. Pulsation periods range from 10 to 40 s but are modulated by longer-period variations ranging from 3 to 5 min. The auroral pulsations are generally accompanied by geomagnetic pulsations, which occur almost every day, whereas the auroral pulsations can only be seen on 20 to 30\% of all days studied. The auroral pulsations show a distinct tendency to occur during geomagnetically quiet periods when the interplanetary magnetic field (IMF) has dawnward and northward or only slightly southward components. The auroral pulsations are most common from 0800 to 1100 MLT at 74°-75° geomagnetic latitude. The shorter-period pulsations have latitudinal extents ranging from several 10 s to 100 km, and longitudinal extents of several hundred kilometers. The auroral pulsations show no tendency to occur during intervals of enhanced solar wind velocities or densities, or during intervals of near-radial IMF orientation. Case and statistical studies comparing the latitude at which the pulsations occur with observations by low-altitude DMSP F7 and NOAA 7 spacecraft demonstrate that they occur deep within the magnetosphere on closed magnetic field lines immediately equatorward of the high-latitude trapping boundary for energetic particles. Consequently, we conclude that they do not result from magnetic merging on the dayside magnetopause, the Kelvin-Helmholtz instability, or the transmission of pulsations generated within the Earth's foreshock through the magnetosheath and into the magnetosphere. The origin of the auroral pulsations remains unknown, although it may ultimately be possible to explain them in terms of instabilities at the outer edge of the radiation belt.},
  ISSN                     = {0148-0227},
  Keywords                 = {Atmospheric Composition and Structure: Airglow and aurora Ionosphere: Auroral ionosphere Magnetospheric Physics: Magnetosphere/ionosphere interactions Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/1999JGR...10410135V}
}

@Article{Voss1991,
  Title                    = {Astrophysical {Plasmas}},
  Author                   = {Voss, D.},
  Journal                  = {Science},
  Year                     = {1991},

  Month                    = apr,
  Pages                    = {353},
  Volume                   = {252},

  Abstract                 = {Not Available},
  Doi                      = {10.1126/science.252.5004.353}
}

@Article{Waara2012,
  Title                    = {Oxygen ion energization by waves in the high altitude cusp and mantle},
  Author                   = {Waara, M and Nilsson, H and Slapak, R and André, Mats and Stenberg, G},
  Journal                  = {Annales Geophysicae-Atmospheres Hydrospheresand Space Sciences},
  Year                     = {2012},
  Number                   = {9},
  Pages                    = {1309},
  Volume                   = {30}
}

@InProceedings{Waara2012a,
  Title                    = {Oxygen ion energization by waves in the high altitude cusp and mantle},
  Author                   = {Waara, M and Nilsson, H and Slapak, R and André, Mats and Stenberg, G},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2012},
  Pages                    = {1309--1314},
  Publisher                = {Copernicus GmbH},
  Volume                   = {30}
}

@InProceedings{Waara2010,
  Title                    = {Oxygen ion energization observed at high altitudes},
  Author                   = {Waara, Martin and Nilsson, H and Stenberg, G and André, Mats and Gunell, H and Reme, H},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2010},
  Pages                    = {907--916},
  Publisher                = {Copernicus GmbH},
  Volume                   = {28}
}

@Article{Waara2010a,
  Title                    = {Oxygen ion energization observed at high altitudes},
  Author                   = {Waara, M. and Nilsson, H. and Stenberg, G. and André, M. and Gunell, H. and Rème, H.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2010},

  Month                    = apr,
  Pages                    = {907--916},
  Volume                   = {28},

  Doi                      = {10.5194/angeo-28-907-2010}
}

@Article{Waara2010b,
  Title                    = {Oxygen ion energization observed at high altitudes},
  Author                   = {Waara, M. and Nilsson, H. and Stenberg, G. and Andr√©, M. and Gunell, H. and R√®me, H.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2010},

  Month                    = apr,
  Pages                    = {907--916},
  Volume                   = {28},

  Doi                      = {10.5194/angeo-28-907-2010}
}

@Article{Walker1999,
  Title                    = {Chapter 6-{Source} and {Loss} {Processes} in the {Magnetotail}},
  Author                   = {Walker, R. and Terasawa, T. and Christon, S. P. and Angelopoulos, V. and Hoshino, M. and Lennartsson, W. and Maezawa, K. and Sibeck, D. G. and Treumann, R. A. and Williams, D. J. and Zelenyi, L.},
  Journal                  = {Space Science Reviews},
  Year                     = {1999},
  Pages                    = {285--353},
  Volume                   = {88},

  Abstract                 = {Not Available},
  ISSN                     = {0038-6308},
  Url                      = {http://adsabs.harvard.edu/abs/1999SSRv...88..285W}
}

@Article{Walsh2014,
  Title                    = {{Simultaneous Ground- and Space-Based Observations of the Plasmaspheric Plume and Reconnection}},
  Author                   = {Walsh, B M and Foster, J C and Erickson, P J and Sibeck, D G},
  Journal                  = {Science (80-. ).},
  Year                     = {2014},
  Number                   = {6175},
  Pages                    = {1122--1125},
  Volume                   = {343},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {Abstract Magnetic reconnection is the primary process through which energy couples from the solar wind into Earth's magnetosphere and ionosphere. Conditions both in the incident solar wind and in the magnetosphere are important in determining the efficiency of this ... $\backslash$n},
  Doi                      = {10.1126/science.1247212},
  ISBN                     = {1095-9203 (Electronic)$\backslash$r0036-8075 (Linking)},
  ISSN                     = {1095-9203},
  Owner                    = {suleimanbaraka},
  Pmid                     = {24604196},
  Timestamp                = {2016.02.23},
  Url                      = {http://www.sciencemag.org/cgi/doi/10.1126/science.1247212$\backslash$npapers3://publication/doi/10.1126/science.1247212}
}

@Article{Walsh2014a,
  Title                    = {The plasmaspheric plume and magnetopause reconnection},
  Author                   = {Walsh, B. M. and Phan, T. D. and Sibeck, D. G. and Souza, V. M.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2014},
  Pages                    = {223--228},
  Volume                   = {41},

  Abstract                 = {We present near-simultaneous measurements from two THEMIS spacecraft at the dayside magnetopause with a 1.5 h separation in local time. One spacecraft observes a high-density plasmaspheric plume while the other does not. Both spacecraft observe signatures of magnetic reconnection, providing a test for the changes to reconnection in local time along the magnetopause as well as the impact of high densities on the reconnection process. When the plume is present and the magnetospheric density exceeds that in the magnetosheath, the reconnection jet velocity decreases, the density within the jet increases, and the location of the faster jet is primarily on field lines with magnetosheath orientation. Slower jet velocities indicate that reconnection is occurring less efficiently. In the localized region where the plume contacts the magnetopause, the high-density plume may impede the solar wind-magnetosphere coupling by mass loading the reconnection site.},
  ISSN                     = {0094-8276},
  Keywords                 = {Reconnection Magnetosphere},
  Url                      = {http://adsabs.harvard.edu/abs/2014GeoRL..41..223W}
}

@Article{Walsh2013a,
  Title                    = {Energetic particle dynamics in {Mercury}'s magnetosphere},
  Author                   = {Walsh, B. M. and Ryou, A. S. and Sibeck, D. G. and Alexeev, I. I.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},
  Pages                    = {1992--1999},
  Volume                   = {118},

  Abstract                 = {We investigate the drift paths of energetic particles in Mercury's magnetosphere by tracing their motion through a model magnetic field. Test particle simulations solving the full Lorentz force show a quasi-trapped energetic particle population that gradient and curvature drift around the planet via "Shabansky" orbits, passing though high latitudes in the compressed dayside by equatorial latitudes on the nightside. Due to their large gyroradii, energetic H{\textless}SUP{\textgreater}+{\textless}/SUP{\textgreater} and Na{\textless}SUP{\textgreater}+{\textless}/SUP{\textgreater} ions will typically collide with the planet or the magnetopause and will not be able to complete a full drift orbit. These simulations provide direct comparison for recent spacecraft measurements from MESSENGER. Mercury's offset dipole results in an asymmetric loss cone and therefore an asymmetry in particle precipitation with more particles precipitating in the southern hemisphere. Since the planet lacks an atmosphere, precipitating particles will collide directly with the surface of the planet. The incident charged particles can kick up neutrals from the surface and have implications for the formation of the exosphere and weathering of the surface.},
  ISSN                     = {0148-0227},
  Keywords                 = {Mercury energetic particles},
  Url                      = {http://adsabs.harvard.edu/abs/2013JGRA..118.1992W}
}

@Article{Walsh2013,
  Title                    = {{Statistical analysis of the plasmaspheric plume at the magnetopause}},
  Author                   = {Walsh, B. M. and Sibeck, D. G. and Nishimura, Y. and Angelopoulos, V.},
  Journal                  = {J. Geophys. Res. Sp. Phys.},
  Year                     = {2013},
  Number                   = {8},
  Volume                   = {118},

  __markedentry            = {[suleimanbaraka:]},
  Doi                      = {10.1002/jgra.50458},
  ISSN                     = {21699402},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Walsh2013b,
  Title                    = {Statistical analysis of the plasmaspheric plume at the magnetopause},
  Author                   = {Walsh, B. M. and Sibeck, D. G. and Nishimura, Y. and Angelopoulos, V.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},
  Pages                    = {4844--4851},
  Volume                   = {118},

  Abstract                 = {During times of enhanced magnetospheric convection, cold dense plasma from the plasmasphere can form a plume extending sunward toward the dayside magnetopause. A statistical study is presented of cold high-density plasmaspheric plasma at the magnetopause. Observations from the Time History of Events and Macroscale Interactions (THEMIS) spacecraft show the plume to be present at the dayside magnetopause during 12.5\% (148 of 1184) of the crossings. Its most common location in magnetic local time when contacting the magnetopause is at 13.6 h. The magnetopause crossings show evidence for reconnection in 68\% of events with the plume while only 47\% of events without plume. Although the plume is more likely to be observed at the magnetopause when reconnection is occurring, the typical reconnection jet velocity is lower for plume events than nonplume events, indicating the presence of the plume may be slowing the efficiency of the reconnection process.},
  ISSN                     = {0148-0227},
  Keywords                 = {reconnection plume magnetopause},
  Url                      = {http://adsabs.harvard.edu/abs/2013JGRA..118.4844W}
}

@Article{Walsh2012,
  Title                    = {{Dawn-dusk asymmetries in the Earth's magnetosheath}},
  Author                   = {Walsh, B. M. and Sibeck, D. G. and Wang, Y. and Fairfield, D. H.},
  Journal                  = {J. Geophys. Res. Sp. Phys.},
  Year                     = {2012},
  Number                   = {12},
  Volume                   = {117},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {Statistical observations by the THEMIS spacecraft show a dawn-dusk asymmetry in plasma parameters within the Earth's magnetosheath. Proton density and temperature are greater on the dawnside while the magnetic field strength and bulk flow are greater on the duskside. The asymmetry has been measured just outside the magnetopause in the dayside magnetosheath through 1114 boundary crossings from 2008 through 2010. These results are compared with modeling from the BATS-R-US global MHD code and are consistent with the expected asymmetries that would result from the interactions of the Parker spiral interplanetary magnetic field with the Earth's bow shock. Solar cycle variations are analyzed for the current and past studies to predict the influence of upstream conditions during different time periods.},
  Doi                      = {10.1029/2012JA018240},
  ISBN                     = {2156-2202},
  ISSN                     = {21699402},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Walsh2012a,
  Title                    = {Dawn-dusk asymmetries in the {Earth}'s magnetosheath},
  Author                   = {Walsh, B. M. and Sibeck, D. G. and Wang, Y. and Fairfield, D. H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2012},
  Pages                    = {12211},
  Volume                   = {117},

  Abstract                 = {Statistical observations by the THEMIS spacecraft show a dawn-dusk asymmetry in plasma parameters within the Earth's magnetosheath. Proton density and temperature are greater on the dawnside while the magnetic field strength and bulk flow are greater on the duskside. The asymmetry has been measured just outside the magnetopause in the dayside magnetosheath through 1114 boundary crossings from 2008 through 2010. These results are compared with modeling from the BATS-R-US global MHD code and are consistent with the expected asymmetries that would result from the interactions of the Parker spiral interplanetary magnetic field with the Earth's bow shock. Solar cycle variations are analyzed for the current and past studies to predict the influence of upstream conditions during different time periods.},
  ISSN                     = {0148-0227},
  Keywords                 = {magnetopause magnetosheath Magnetospheric Physics: Magnetopause and boundary layers Magnetospheric Physics: Magnetosheath Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2012JGRA..11712211W}
}

@Article{Wang1995,
  Title                    = {3D electromagnetic plasma particle simulations on a {MIMD} parallel computer},
  Author                   = {Wang, J and Liewer, P and Decyk, V},
  Journal                  = {Comput. Phys. Commun.},
  Year                     = {1995},
  Number                   = {1},
  Pages                    = {35--53},
  Volume                   = {87}
}

@Article{Wang2004,
  Title                    = {{GOES} 8 aerosol optical thickness assimilation in a mesoscale model: {Online} integration of aerosol radiative effects},
  Author                   = {Wang, Jun and Nair, US and Christopher, Sundar A},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984–2012)},
  Year                     = {2004},
  Number                   = {D23},
  Volume                   = {109}
}

@Article{Wang2015,
  Title                    = {The dipole tilt angle dependence of the bow shock for southward {IMF}: {MHD} results},
  Author                   = {Wang, M. and Lu, J. Y. and Yuan, H. Z. and Kabin, K. and Liu, Z.-Q. and Zhao, M. X. and Li, G.},
  Journal                  = {Planetary and Space Science},
  Year                     = {2015},
  Pages                    = {99--107},
  Volume                   = {106},

  File                     = {[PDF] from researchgate.net:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/65Q33T9U/Wang et al. - 2015 - The dipole tilt angle dependence of the bow shock .pdf:application/pdf;Snapshot:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/R5MB4S96/S0032063314003948.html:text/html},
  Shorttitle               = {The dipole tilt angle dependence of the bow shock for southward {IMF}},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S0032063314003948},
  Urldate                  = {2016-01-11}
}

@Article{Wang2013,
  Title                    = {Hot flow anomaly formation and evolution: {Cluster} observations},
  Author                   = {Wang, S. and Zong, Q. and Zhang, H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = jul,
  Pages                    = {4360--4380},
  Volume                   = {118},

  Doi                      = {10.1002/jgra.50424},
  Keywords                 = {convective electric field, hot flow anomalies, interplanetary discontinuity, ion/electron velocity distribution, spectra fitting}
}

@Article{Wang2006,
  Title                    = {Generation of filamentary structures by beam-plasma interaction},
  Author                   = {Wang, X. Y. and Lin, Y.},
  Journal                  = {Phys. Plasmas},
  Year                     = {2006},

  Month                    = may,
  Number                   = {5},
  Pages                    = {052102},
  Volume                   = {13},

  Doi                      = {10.1063/1.2197797},
  Keywords                 = {Fluctuation and chaos phenomena, Hybrid methods, Macroinstabilities, Magnetohydrodynamic waves, Nonlinear phenomena: waves wave propagation and other interactions, Particle beam interactions in plasmas}
}

@Article{Wang2005,
  Title                    = {Simulation study of beam-plasma interaction and associated acceleration of background ions},
  Author                   = {Wang, X. Y. and Lin, Y.},
  Journal                  = {Washington DC American Geophysical Union Geophysical Monograph Series},
  Year                     = {2005},
  Pages                    = {117--123},
  Volume                   = {156},

  Doi                      = {10.1029/156GM15}
}

@Article{Wang2009,
  Title                    = {Hybrid simulation of foreshock waves and ion spectra and their linkage to cusp energetic ions},
  Author                   = {Wang, X. Y. and Lin, Y. and Chang, S.-W.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2009},

  Month                    = jun,
  Pages                    = {6203},
  Volume                   = {114},

  Doi                      = {10.1029/2008JA013745},
  Keywords                 = {6984), Interplanetary Physics: Interplanetary shocks, Magnetospheric Physics: Cusp, Magnetospheric Physics: Numerical modeling, Space Plasma Physics: Particle acceleration, Space Plasma Physics: Wave/particle interactions (2483}
}

@Article{Wang2013a,
  Title                    = {A new three-dimensional magnetopause model with a support vector regression machine and a large database of multiple spacecraft observations},
  Author                   = {Wang, Y. and Sibeck, D. G. and Merka, J. and Boardsen, S. A. and Karimabadi, H. and Sipes, T. B. and Šafránková, J. and Jelínek, K. and Lin, R.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},
  Pages                    = {2173--2184},
  Volume                   = {118},

  Abstract                 = {We present results from a new three-dimensional empirical magnetopause model based on 15,089 magnetopause crossings from 23 spacecraft. To construct the model, we introduce a Support Vector Regression Machine (SVRM) technique with a systematic approach that balances model smoothness with fitting accuracy to produce a model that reveals the manner in which the size and shape of the magnetopause depend upon various control parameters without any assumptions concerning the analytical shape of the magnetopause. The new model fits the data used in the modeling very accurately, and can guarantee a similar accuracy when predicting unseen observations within the applicable range of control parameters. We introduce a new error analysis technique based upon the SVRM that enables us to obtain model errors appropriate to different locations and control parameters. We find significant east-west elongations in the magnetopause shape for many combinations of control parameters. Variations in the Earth's dipole tilt can cause significant magnetopause north/south asymmetries and deviation of the magnetopause nose from the Sun-Earth line nonlinearly by as much as 5 Re. Subsolar magnetopause erosion effect under southward IMF is seen which is strongly affected by solar wind dynamic pressure. Further, we find significant shrinking of high-latitude magnetopause with decreased magnetopause flaring angle during northward IMF.},
  ISSN                     = {0148-0227},
  Keywords                 = {magnetopause empirical model support vector regression machine dipole tilt erosion},
  Url                      = {http://adsabs.harvard.edu/abs/2013JGRA..118.2173W}
}

@Article{Wang2012,
  Title                    = {On the {Nature} of the {Solar} {Wind} from {Coronal} {Pseudostreamers}},
  Author                   = {Wang, Y.-M. and Grappin, R. and Robbrecht, E. and Sheeley, Jr., N. R.},
  Journal                  = {{\textbackslash}apj},
  Year                     = {2012},

  Month                    = apr,
  Pages                    = {182},
  Volume                   = {749},

  Doi                      = {10.1088/0004-637X/749/2/182},
  Keywords                 = {INTERPLANETARY MEDIUM, Solar Wind, Sun: corona, Sun: heliosphere, Sun: magnetic topology}
}

@Article{Watanabe2004,
  Title                    = {Polar cap bifurcation during steady-state northward interplanetary magnetic field with‚Äö√†¬£ {BY}‚Äö√†¬£ {BZ}},
  Author                   = {Watanabe, Masakazu and Sofko, George J and André, Dieter A and Tanaka, Takashi and Hairston, Marc R},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2004},
  Number                   = {A1},
  Volume                   = {109}
}

@Article{Watari2009,
  Title                    = {Measurements of geomagnetically induced current in a power grid in {Hokkaido}, {Japan}},
  Author                   = {Watari, S and Kunitake, M and Kitamura, K and Hori, T and Kikuchi, T and Shiokawa, K and Nishitani, N and Kataoka, R and Kamide, Y and Aso, T and {others}},
  Journal                  = {Space Weather},
  Year                     = {2009},
  Number                   = {3},
  Volume                   = {7}
}

@Article{Watermann2009,
  Title                    = {The state of space weather scientific modeling‚àö‚â•an introduction},
  Author                   = {Watermann, J and Vainio, R and Lilensten, J and Belehaki, A and Messerotti, M},
  Journal                  = {Space science reviews},
  Year                     = {2009},
  Number                   = {3-4},
  Pages                    = {111--120},
  Volume                   = {147},

  Url                      = {http://link.springer.com/article/10.1007/s11214-009-9576-8}
}

@Article{Weidner2010,
  Title                    = {Limits on the orbits and masses of moons around currently-known transiting exoplanets},
  Author                   = {Weidner, C. and Horne, K.},
  Journal                  = {{\textbackslash}textbackslashaap},
  Year                     = {2010},

  Month                    = oct,
  Pages                    = {A76},
  Volume                   = {521},

  Doi                      = {10.1051/0004-6361/201014955},
  Keywords                 = {astrobiology, planets and satellites: detection, planets and satellites: dynamical evolution and stability, planets and satellites: formation}
}

@Article{Weimer1996,
  Title                    = {A flexible, {IMF} dependent model of high-latitude electric potentials having ‚àö√Æ‚àö‚àè≈í¬©space weather‚àö√Æ‚àö‚àè≈í¬© applications},
  Author                   = {Weimer, DR},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1996},
  Number                   = {18},
  Pages                    = {2549--2552},
  Volume                   = {23},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/96GL02255/full}
}

@InProceedings{Welling2013,
  Title                    = {Evaluating the {Importance} of {Outflow} {Velocity} at the {MHD} {Inner} {Boundary}},
  Author                   = {Welling, DT and Liemohn, MW and Toth, G and Glocer, A},
  Booktitle                = {{AGU} {Fall} {Meeting} {Abstracts}},
  Year                     = {2013},
  Pages                    = {2105},
  Volume                   = {1}
}

@Article{Werner2013,
  Title                    = {The {Effect} of {Mass} {Ratio} in {Relativistic}, {Collisionless} {Electron}-{Ion} {Reconnection}},
  Author                   = {Werner, Gregory and Begelman, Mitchell and Cerutti, Benoit and Nalewajko, Krzysztof and Uzdensky, Dmitri},
  Journal                  = {Bulletin of the American Physical Society},
  Year                     = {2013},
  Volume                   = {58},

  Url                      = {http://meetings.aps.org/Meeting/DPP13/Session/NO5.3},
  Urldate                  = {2014-05-31}
}

@Article{Wiehle2011,
  Title                    = {First lunar wake passage of {ARTEMIS}: {Discrimination} of wake effects and solar wind fluctuations by 3D hybrid simulations},
  Author                   = {Wiehle, S. and Plaschke, F. and Motschmann, U. and Glassmeier, K.-H. and Auster, H. U. and Angelopoulos, V. and Mueller, J. and Kriegel, H. and Georgescu, E. and Halekas, J. and Sibeck, D. G. and McFadden, J. P.},
  Journal                  = {Planetary and Space Science},
  Year                     = {2011},
  Pages                    = {661--671},
  Volume                   = {59},

  Abstract                 = {The spacecraft P1 of the new ARTEMIS (Acceleration, Reconnection, Turbulence, and Electrodynamics of the Moon's Interaction with the Sun) mission passed the lunar wake for the first time on February 13, 2010. We present magnetic field and plasma data of this event and results of 3D hybrid simulations. As the solar wind magnetic field was highly dynamic during the passage, a simulation with stationary solar wind input cannot distinguish whether distortions were caused by these solar wind variations or by the lunar wake; therefore, a dynamic real-time simulation of the flyby has been performed. The input values of this simulation are taken from NASA OMNI data and adapted to the P1 data, resulting in a good agreement between simulation and measurements. Combined with the stationary simulation showing non-transient lunar wake structures, a separation of solar wind and wake effects is achieved. An anisotropy in the magnitude of the plasma bulk flow velocity caused by a non-vanishing magnetic field component parallel to the solar wind flow and perturbations created by counterstreaming ions in the lunar wake are observed in data and simulations. The simulations help to interpret the data granting us the opportunity to examine the entire lunar plasma environment and, thus, extending the possibilities of measurements alone: A comparison of a simulation cross section to theoretical predictions of MHD wave propagation shows that all three basic MHD modes are present in the lunar wake and that their expansion governs the lunar wake refilling process.},
  ISSN                     = {0032-0633},
  Url                      = {http://adsabs.harvard.edu/abs/2011P%26SS...59..661W}
}

@Article{Wilber2008,
  Title                    = {Foreshock density holes in the context of known upstream plasma structures},
  Author                   = {Wilber, M. and Parks, G. K. and Meziane, K. and Lin, N. and Lee, E. and Mazelle, C. and Harris, A.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2008},

  Month                    = nov,
  Pages                    = {3741--3755},
  Volume                   = {26},

  Doi                      = {10.5194/angeo-26-3741-2008}
}

@Article{Wilhelm2011,
  Title                    = {Morphology, dynamics and plasma parameters of plumes and inter-plume regions in solar coronal holes},
  Author                   = {Wilhelm, K. and Abbo, L. and Auchère, F. and Barbey, N. and Feng, L. and Gabriel, A. H. and Giordano, S. and Imada, S. and Llebaria, A. and Matthaeus, W. H. and Poletto, G. and Raouafi, N.-E. and Suess, S. T. and Teriaca, L. and Wang, Y.-M.},
  Journal                  = {{\textbackslash}aapr},
  Year                     = {2011},

  Month                    = jun,
  Pages                    = {35},
  Volume                   = {19},

  Doi                      = {10.1007/s00159-011-0035-7},
  Keywords                 = {corona, Coronal holes, Coronal plumes, Inter-plume regions, Solar Wind, sun}
}

@Article{Wilhelm1995,
  Title                    = {{SUMER} - {Solar} {Ultraviolet} {Measurements} of {Emitted} {Radiation}},
  Author                   = {Wilhelm, K. and Curdt, W. and Marsch, E. and Schühle, U. and Lemaire, P. and Gabriel, A. and Vial, J.-C. and Grewing, M. and Huber, M. C. E. and Jordan, S. D. and Poland, A. I. and Thomas, R. J. and Kühne, M. and Timothy, J. G. and Hassler, D. M. and Siegmund, O. H. W.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {1995},

  Month                    = dec,
  Pages                    = {189--231},
  Volume                   = {162},

  Doi                      = {10.1007/BF00733430},
  Keywords                 = {Coronal heating, EUV Spectrometer, Solar EUV Emission Lines, Solar Wind Acceleration}
}

@Article{Wilson2013,
  Title                    = {Shocklets, {SLAMS}, and field-aligned ion beams in the terrestrial foreshock},
  Author                   = {Wilson, L. B. and Koval, A. and Sibeck, D. G. and Szabo, A. and Cattell, C. A. and Kasper, J. C. and Maruca, B. A. and Pulupa, M. and Salem, C. S. and Wilber, M.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},
  Pages                    = {957--966},
  Volume                   = {118},

  Abstract                 = {We present Wind spacecraft observations of ion distributions showing field-aligned beams (FABs) and large-amplitude magnetic fluctuations composed of a series of shocklets and short large-amplitude magnetic structures (SLAMS). The FABs are found to have T{\textless}SUB{\textgreater}b{\textless}/SUB{\textgreater} 80 - 850 eV, V{\textless}SUB{\textgreater}b{\textless}/SUB{\textgreater}/V{\textless}SUB{\textgreater}sw{\textless}/SUB{\textgreater} 1. 3 - 2. 4, T{\textless}SUB{\textgreater}⊥,b{\textless}/SUB{\textgreater}/T{\textless}SUB{\textgreater}∥,b{\textless}/SUB{\textgreater} 1-8, and n{\textless}SUB{\textgreater}b{\textless}/SUB{\textgreater}/n{\textless}SUB{\textgreater}o{\textless}/SUB{\textgreater} 0.2-11\%. Saturation amplitudes for ion/ion resonant and non-resonant instabilities are too small to explain the observed SLAMS amplitudes. We show two examples where groups of SLAMS can act like a local quasi-perpendicular shock reflecting ions to produce the FABs, a scenario distinct from the more common production at the quasi-perpendicular bow shock. The SLAMS exhibit a foot-like magnetic enhancement with a leading magnetosonic whistler train, consistent with previous observations. Strong ion and electron heating are observed within the series of shocklets and SLAMS with temperatures increasing by factors ≳ 5 and ≳ 3, respectively. Both the core and halo electron components show strong perpendicular heating inside the feature.},
  ISSN                     = {0148-0227},
  Keywords                 = {SLAMS field-aligned ion beams particle reflection particle acceleration whistler mode waves wave-particle interaction},
  Url                      = {http://adsabs.harvard.edu/abs/2013JGRA..118..957W}
}

@Article{Wilson2014,
  Title                    = {Quantified energy dissipation rates in the terrestrial bow shock: 1. {Analysis} techniques and methodology},
  Author                   = {Wilson, L. B. and Sibeck, D. G. and Breneman, A. W. and Contel, O. Le and Cully, C. and Turner, D. L. and Angelopoulos, V. and Malaspina, D. M.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2014},
  Pages                    = {6455--6474},
  Volume                   = {119},

  Abstract                 = {We present a detailed outline and discussion of the analysis techniques used to compare the relevance of different energy dissipation mechanisms at collisionless shock waves. We show that the low-frequency, quasi-static fields contribute less to ohmic energy dissipation, (-j·E), than their high-frequency counterparts. In fact, we found that high-frequency, large-amplitude ({\textgreater}100 mV/m and/or {\textgreater}1 nT) waves are ubiquitous in the transition region of collisionless shocks. We quantitatively show that their fields, through wave-particle interactions, cause enough energy dissipation to regulate the global structure of collisionless shocks. The purpose of this paper, part one of two, is to outline and describe in detail the background, analysis techniques, and theoretical motivation for our new results presented in the companion paper. The companion paper presents the results of our quantitative energy dissipation rate estimates and discusses the implications. Together, the two manuscripts present the first study quantifying the contribution that high-frequency waves provide, through wave-particle interactions, to the total energy dissipation budget of collisionless shock waves.},
  ISSN                     = {0148-0227},
  Keywords                 = {wave-particle interactions collisionless shock waves energy dissipation},
  Url                      = {http://adsabs.harvard.edu/abs/2014JGRA..119.6455W}
}

@Article{Wilson2014a,
  Title                    = {Quantified energy dissipation rates in the terrestrial bow shock: 2. {Waves} and dissipation},
  Author                   = {Wilson, L. B. and Sibeck, D. G. and Breneman, A. W. and Contel, O. Le and Cully, C. and Turner, D. L. and Angelopoulos, V. and Malaspina, D. M.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2014},
  Pages                    = {6475--6495},
  Volume                   = {119},

  Abstract                 = {We present the first quantified measure of the energy dissipation rates, due to wave-particle interactions, in the transition region of the Earth's collisionless bow shock using data from the Time History of Events and Macroscale Interactions during Substorms spacecraft. Our results show that wave-particle interactions can regulate the global structure and dominate the energy dissipation of collisionless shocks. In every bow shock crossing examined, we observed both low-frequency ({\textless}10 Hz) and high-frequency (≳10 Hz) electromagnetic waves throughout the entire transition region and into the magnetosheath. The low-frequency waves were consistent with magnetosonic-whistler waves. The high-frequency waves were combinations of ion-acoustic waves, electron cyclotron drift instability driven waves, electrostatic solitary waves, and whistler mode waves. The high-frequency waves had the following: (1) peak amplitudes exceeding δB˜ 10 nT and δE˜ 300 mV/m, though more typical values were δB˜ 0.1-1.0 nT and δE˜ 10-50 mV/m; (2) Poynting fluxes in excess of 2000 μW m{\textless}SUP{\textgreater}-2{\textless}/SUP{\textgreater} (typical values were ˜1-10 μW m{\textless}SUP{\textgreater}-2{\textless}/SUP{\textgreater}); (3) resistivities {\textgreater} 9000 Ω m; and (4) associated energy dissipation rates {\textgreater}10 μW m{\textless}SUP{\textgreater}-3{\textless}/SUP{\textgreater}. The dissipation rates due to wave-particle interactions exceeded rates necessary to explain the increase in entropy across the shock ramps for ˜90\% of the wave burst durations. For ˜22\% of these times, the wave-particle interactions needed to only be ≤ 0.1\% efficient to balance the nonlinear wave steepening that produced the shock waves. These results show that wave-particle interactions have the capacity to regulate the global structure and dominate the energy dissipation of collisionless shocks.},
  ISSN                     = {0148-0227},
  Keywords                 = {wave-particle interactions collisionless shock waves energy dissipation ion-acoustic waves electron cyclotron drift instability electrostatic solitary waves},
  Url                      = {http://adsabs.harvard.edu/abs/2014JGRA..119.6475W}
}

@InProceedings{Wimmer-Schweingruber2003,
  Title                    = {Solar {Wind} {Composition}},
  Author                   = {Wimmer-Schweingruber, Robert F.},
  Booktitle                = {Solar {Wind} {Ten}},
  Year                     = {2003},
  Editor                   = {Velli, M. and Bruno, R. and Malara, F. and Bucci, B.},
  Month                    = sep,
  Pages                    = {577--582},
  Series                   = {American {Institute} of {Physics} {Conference} {Series}},
  Volume                   = {679},

  Keywords                 = {Solar Atmosphere, solar composition, Solar Corona, solar evolution, Solar Wind}
}

@Article{Wing2005,
  Title                    = {Kp forecast models},
  Author                   = {Wing, S. and Johnson, J. R. and Jen, J. and Meng, C.-I. and Sibeck, D. G. and Bechtold, K. and Freeman, J. and Costello, K. and Balikhin, M. and Takahashi, K.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2005},
  Pages                    = {4203},
  Volume                   = {110},

  Abstract                 = {Magnetically active times, e.g., Kp {\textgreater} 5, are notoriously difficult to predict, precisely the times when such predictions are crucial to the space weather users. Taking advantage of the routinely available solar wind measurements at Langrangian point (L1) and nowcast Kps, Kp forecast models based on neural networks were developed with the focus on improving the forecast for active times. To satisfy different needs and operational constraints, three models were developed: (1) a model that inputs nowcast Kp and solar wind parameters and predicts Kp 1 hour ahead; (2) a model with the same input as model 1 and predicts Kp 4 hour ahead; and (3) a model that inputs only solar wind parameters and predicts Kp 1 hour ahead (the exact prediction lead time depends on the solar wind speed and the location of the solar wind monitor). Extensive evaluations of these models and other major operational Kp forecast models show that while the new models can predict Kps more accurately for all activities, the most dramatic improvements occur for moderate and active times. Information dynamics analysis of Kp suggests that geospace is more dominated by internal dynamics near solar minimum than near solar maximum, when it is more directly driven by external inputs, namely solar wind and interplanetary magnetic field (IMF).},
  ISSN                     = {0148-0227},
  Keywords                 = {Space Weather: Models Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: Forecasting (7924 7964) Space Weather: Forecasting (2722) Kp forecast APL Kp model Kp predictability solar cycle effect},
  Url                      = {http://adsabs.harvard.edu/abs/2005JGRA..110.4203W}
}

@Article{Wing1995,
  Title                    = {A large statistical study of the entry of interplanetary magnetic field {Y}-component into the magnetosphere},
  Author                   = {Wing, S. and Newell, P. T. and Sibeck, D. G. and Baker, K. B.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1995},
  Pages                    = {2083--2086},
  Volume                   = {22},

  Abstract                 = {We used 5 years of GOES-6 and 6 years of GOES-7 data to correlate the y-component of the geosynchronous magnetic field with the y-component of IMF. One motivation is that the subsolar merging model and the antiparallel model predict distinctly different patterns for B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater} in the magnetosphere as a function of IMF B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater}. Although both models predict that nightside magnetospheric magnetic field will tilt in the direction of the IMF B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater}, the antiparallel merging model predicts that magnetospheric magnetic field lines in the vicinity of local noon will tilt in the direction of the IMF, where as the subsolar model does not. The correlation coefficients between the geosynchronous data and the IMF B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater} peak at both noon (0.61) and midnight (0.50), favoring the antiparallel model. These results were obtained with 1789 (noon) and 1312 (midnight) data points. The slopes of the regression lines indicate 29\% IMF B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater} entry at noon and 79\% at midnight. The local-time distribution of the slopes varies smoothly from midnight peak to a broad minimum near noon.},
  ISSN                     = {0094-8276},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetospheric configuration and dynamics Interplanetary Physics: Interplanetary magnetic fields Magnetospheric Physics: General or miscellaneous},
  Url                      = {http://adsabs.harvard.edu/abs/1995GeoRL..22.2083W}
}

@Article{Wing1997,
  Title                    = {Effects of interplanetary magnetic field z component and the solar wind dynamic pressure on the geosynchronous magnetic field},
  Author                   = {Wing, Simon and Sibeck, David G},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1997},
  Number                   = {A4},
  Pages                    = {7207--7216},
  Volume                   = {102}
}

@Article{Wing1997a,
  Title                    = {Effects of interplanetary magnetic field {\textless}formula{\textgreater}z component and the solar wind dynamic pressure on the geosynchronous magnetic field},
  Author                   = {Wing, Simon and Sibeck, David G.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1997},
  Pages                    = {7207--7216},
  Volume                   = {102},

  Abstract                 = {A study of the correlation of the geosynchronous magnetic field with interplanetary magnetic field (IMF) B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} and the solar wind dynamic pressure (P{\textless}SUB{\textgreater}d{\textless}/SUB{\textgreater}) is presented. Hourly averages of 5 years of GOES 6 and 6 years of GOES 7 observations are correlated with IMF B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} and P{\textless}SUB{\textgreater}d{\textless}/SUB{\textgreater}. As previously reported, increases in P{\textless}SUB{\textgreater}d{\textless}/SUB{\textgreater} enhance geosynchronous B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} on the dayside, most strongly around noon, but depress it on the nightside, most strongly around midnight. This has been interpreted in terms of increases in the cross-tail and magnetopause currents. Our study shows that the dayside geosynchronous magnetic field decreases with IMF B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater}, particularly during periods of southward IMF. During periods of northward IMF, this trend continues but at much slower rate. The results of a multiple regression analysis of GOES B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} as a function of IMF B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} and P{\textless}SUB{\textgreater}d{\textless}/SUB{\textgreater} during periods of northward IMF show that roughly 30\% of the IMF B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} uniformly “penetrates” the geosynchronous B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater}. In contrast, during periods of southward IMF, the effect of IMF B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} on geosynchronous B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} is nonuniform and much larger at all local times, especially near dawn and dusk, apparently because of enhanced cross-tail current. During periods of southward IMF, geosynchronous B{\textless}SUB{\textgreater}x{\textless}/SUB{\textgreater} depends most strongly on IMF B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} near dawn, dusk, and midnight. The dawn and dusk correlations can be attributed to the enhanced region 1 Birkeland currents, and the midnight correlation can be attributed to enhanced cross-tail current. Geosynchronous B{\textless}SUB{\textgreater}y{\textless}/SUB{\textgreater} has the best correlations with IMF B{\textless}SUB{\textgreater}z{\textless}/SUB{\textgreater} near 2000},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetospheric configuration and dynamics},
  Url                      = {http://adsabs.harvard.edu/abs/1997JGR...102.7207W}
}

@Article{Wing2002,
  Title                    = {Geosynchronous magnetic field temporal response to solar wind and {IMF} variations},
  Author                   = {Wing, S. and Sibeck, D. G. and Wiltberger, M. and Singer, H.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2002},
  Pages                    = {1222},
  Volume                   = {107},

  Abstract                 = {We investigate the time-dependent response of the geosynchronous magnetic field to variations in the interplanetary magnetic field (IMF) orientation and sudden changes in the solar wind dynamic pressure. Because IMF discontinuities drape about the magnetopause, we expect the response to southward IMF turnings to occur nearly simultaneously over a wide range of local times. By contrast, the pressure variations launched by solar wind tangential discontinuities aligned with the spiral IMF into the magnetosheath should keep pace with the solar wind and generally strike the postnoon magnetopause first. Consistent with these predictions, we find that the magnetospheric magnetic field strength begins to diminish at all dayside local times within 4 to 5 min following the estimated arrival time of southward IMF turnings at the subsolar magnetopause, and that the nightside field begins to reconfigure within 12 min. By contrast, the response to pressure variations generally appears some 2.2 min after the arrival of the discontinuity in the noon-dusk sector, 4.4 min later in the noon-dawn sector, and 8.8 min later on the nightside.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Current systems (2409) Magnetospheric Physics: Magnetosphere-inner Magnetospheric Physics: Magnetospheric configuration and dynamics Magnetospheric Physics: MHD waves and instabilities Magnetospheric Physics: Solar wind/magnetosphere interactions},
  Url                      = {http://adsabs.harvard.edu/abs/2002JGRA..107.1222W}
}

@Article{Winglee2005,
  Title                    = {Mapping of the heavy ion outflows as seen by {IMAGE} and multifluid global modeling for the 17 {April} 2002 storm},
  Author                   = {Winglee, RM and Lewis, W and Lu, Gang},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2005},
  Number                   = {A12},
  Volume                   = {110}
}

@Article{Winglee2002,
  Title                    = {Global impact of ionospheric outflows on the dynamics of the magnetosphere and cross-polar cap potential},
  Author                   = {Winglee, R. M. and Chua, D. and Brittnacher, M. and Parks, G. K. and Lu, G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2002},

  Month                    = sep,
  Pages                    = {1237},
  Volume                   = {107},

  Doi                      = {10.1029/2001JA000214},
  Keywords                 = {Ionosphere: Ionosphere/magnetosphere interactions (2736), ionospheric outflows, Magnetospheric Physics: Magnetosphere/ionosphere interactions, Magnetospheric Physics: Magnetospheric configuration and dynamics, Magnetospheric Physics: Numerical modeling, polar cap potential, simulations}
}

@Article{Winglee2002a,
  Title                    = {Global impact of ionospheric outflows on the dynamics of the magnetosphere and cross-polar cap potential},
  Author                   = {Winglee, R. M. and Chua, D. and Brittnacher, M. and Parks, G. K. and Lu, G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2002},

  Month                    = sep,
  Pages                    = {1237},
  Volume                   = {107},

  Doi                      = {10.1029/2001JA000214},
  Keywords                 = {Ionosphere: Ionosphere/magnetosphere interactions (2736), ionospheric outflows, Magnetospheric Physics: Magnetosphere/ionosphere interactions, Magnetospheric Physics: Magnetospheric configuration and dynamics, Magnetospheric Physics: Numerical modeling, polar cap potential, simulations}
}

@Article{Winglee2002b,
  Title                    = {Global impact of ionospheric outflows on the dynamics of the magnetosphere and cross-polar cap potential},
  Author                   = {Winglee, R. M. and Chua, D. and Brittnacher, M. and Parks, G. K. and Lu, Gang},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2002},
  Number                   = {A9},
  Pages                    = {SMP--11},
  Volume                   = {107},

  File                     = {[HTML] from wiley.com:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/3D43ZSGE/full.html:text/html;Snapshot:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/5AVQXWJ3/pdf.html:text/html},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2001JA000214/pdf},
  Urldate                  = {2015-12-09}
}

@Article{Winkler1992,
  Title                    = {Results from improved {Monte} {Carlo} calculations of auroral ion velocity distributions},
  Author                   = {Winkler, E and St-Maurice, J-P and Barakat, AR},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1992},
  Number                   = {A6},
  Pages                    = {8399--8423},
  Volume                   = {97}
}

@Article{Winningham1984,
  Title                    = {Observations of large scale ion conic generation with {DE}-1},
  Author                   = {Winningham, JD and Burch, JL},
  Journal                  = {Phys. Sp. Plasmas},
  Year                     = {1984},

  Url                      = {http://adsabs.harvard.edu/abs/1984psp..conf..137W}
}

@Article{Winningham1981,
  Title                    = {The {Low} {Altitude} {Plasma} {Instrument}/{LAPI}},
  Author                   = {Winningham, JD and Burch, JL},
  Journal                  = {Sp. Sci. {\textbackslash}ldots},
  Year                     = {1981},

  Url                      = {http://adsabs.harvard.edu/abs/1981SSI.....5..465W}
}

@Article{Winske1996,
  Title                    = {A nonspecialist's guide to kinetic simulations of space plasmas},
  Author                   = {Winske, D. and Omidi, N.},
  Journal                  = {{\textbackslash}jgr},
  Year                     = {1996},

  Month                    = aug,
  Pages                    = {17287--17304},
  Volume                   = {101},

  Doi                      = {10.1029/96JA00982},
  Keywords                 = {Interplanetary Physics: Planetary bow shocks, Space Plasma Physics: Numerical simulation studies, Space Plasma Physics: Shock waves, Space Plasma Physics: Waves and instabilities}
}

@Article{Winske1988,
  Title                    = {Magnetic field and density fluctuations at perpendicular supercritical collisionless shocks},
  Author                   = {Winske, D and Quest, KB},
  Journal                  = {J. Geophys. Res.},
  Year                     = {1988},
  Number                   = {A9},
  Pages                    = {9681--9693},
  Volume                   = {93}
}

@InCollection{Winske2003,
  Title                    = {Hybrid simulation codes: past, present and future‚àö‚â•a tutorial},
  Author                   = {Winske, Dan and Yin, Lin and Omidi, Nick and Karimabadi, Homa and Quest, Kevin},
  Booktitle                = {Space {Plasma} {Simulation}},
  Publisher                = {Springer},
  Year                     = {2003},
  Pages                    = {136--165},

  Url                      = {http://link.springer.com/chapter/10.1007/3-540-36530-3_8}
}

@Article{Wittrock2006,
  Title                    = {Simultaneous global observations of glyoxal and formaldehyde from space},
  Author                   = {Wittrock, Folkard and Richter, Andreas and Oetjen, Hilke and Burrows, John P. and Kanakidou, Maria and Myriokefalitakis, Stelios and Volkamer, Rainer and Beirle, Steffen and Platt, Ulrich and Wagner, Thomas},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2006},
  Number                   = {16},
  Volume                   = {33},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2006GL026310/full},
  Urldate                  = {2014-11-13}
}

@InProceedings{Wodnicka2009,
  Title                    = {On a magnetosphere disturbed by solar wind; observations of macroelectrons},
  Author                   = {Wodnicka, EB},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2009},
  Pages                    = {2331--2339},
  Publisher                = {Copernicus GmbH},
  Volume                   = {27}
}

@Article{Wodnicka2001,
  Title                    = {Comparing two models of the {Earth}'s magnetosphere},
  Author                   = {Wodnicka, Elżbieta B},
  Journal                  = {Advances in Space Research},
  Year                     = {2001},
  Number                   = {12},
  Pages                    = {1727--1732},
  Volume                   = {28}
}

@Article{Wright2005,
  Title                    = {The physics of space security},
  Author                   = {Wright, David and Grego, Laura and Gronlund, Lisbeth},
  Journal                  = {A Reference Manual. Cambridge: American Academy of Arts and Sciences},
  Year                     = {2005}
}

@Article{Wu2006,
  Title                    = {Density {Depletion} in a {Coronal} {Flux} {Tube} {Associated} {With} {Solar} {Radio} {Emission}},
  Author                   = {Wu, C. S. and Wang, C. B. and Lu, Q. M.},
  Journal                  = {{\textbackslash}solphys},
  Year                     = {2006},

  Month                    = may,
  Pages                    = {317--329},
  Volume                   = {235},

  Doi                      = {10.1007/s11207-006-2068-z}
}

@Article{Wu2012,
  Title                    = {The impact of turbulence on electron heating and acceleration near the neutral point of externally driven reconnecting current sheets in solar flares},
  Author                   = {Wu, Gui-Ping and Ji, Hai-Sheng and Ning, Zong-Jun},
  Journal                  = {Research in Astronomy and Astrophysics},
  Year                     = {2012},
  Number                   = {12},
  Pages                    = {1701},
  Volume                   = {12},

  Url                      = {http://iopscience.iop.org/1674-4527/12/12/012},
  Urldate                  = {2014-05-31}
}

@Article{Wu2013,
  Title                    = {Intermittent heating in solar wind and kinetic simulations},
  Author                   = {Wu, P and Perri, S and Osman, K and Wan, M and Matthaeus, WH and Shay, MA and Goldstein, ML and Karimabadi, H and Chapman, S},
  Journal                  = {The Astrophysical Journal Letters},
  Year                     = {2013},
  Number                   = {2},
  Pages                    = {L30},
  Volume                   = {763}
}

@Article{Wu2002,
  Title                    = {Dynamic fluid kinetic ({DyFK}) simulation of auroral ion transport: {Synergistic} effects of parallel potentials, transverse ion heating, and soft electron precipitation},
  Author                   = {Wu, X.-Y. and Horwitz, J. L. and Tu, J.-N.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2002},

  Month                    = oct,
  Pages                    = {1283--1283},
  Volume                   = {107},

  Abstract                 = {Ion outflow processes along auroral field lines are simulated with a dynamic fluid kinetic (DyFK) model which couples a comprehensive fluid ionospheric (120-1100 km altitude) model to a semikinetic treatment for the topside through 3 RE region. Using a simplified electron description, large-scale extended parallel electrical fields driven by anisotropic hot plasma distributions have been incorporated in addition to the soft auroral electron precipitation and wave-driven ion-heating processes previously simulated [, 1999]. Simulations show that auroral ionospheric ion outflows involve initial evacuation, ion-heating, and replenishment phases. The ionospheric ion supply is effectively elevated by the soft electron precipitation to topside altitudes, where the wave-driven transverse ion heating pumps ions upward. The altitude distribution and duration of wave heating and potential drop largely affect the "pressure cooker" ion trap formation. With comparable and persistent downward potential drop and wave heating, the pressure cooker produces slow and dense suprathermal ion outflows. The ion velocity distribution evolves in an extended ion trap from bowl and counterstreaming suprathermal conic distributions at lower altitudes into mirrored conics and finally toroidal distributions at the top of the pressure cooker. The wave heating is less effective for H+ ions, owing partly to their fast transit through the wave-heating region. The H+ ion trap tends to be lower but more extended in altitudinal extent than the O+ ion trap. H+ flux and total flow are about a third to half of those of O+. Some of the toroidal distributions and ion species variations of beam and conic energies in these simulations qualitatively resemble satellite observations of such ion distributions.},
  Annote                   = {Added to JabRef: 2015.04.18},
  Doi                      = {10.1029/2000JA000190},
  Keywords                 = {auroral ionosphere, hybrid simulation, Ionosphere: Auroral ionosphere (2704), Ionosphere: Particle acceleration, ion transport, Outflow, Space Plasma Physics: Numerical simulation studies, Space Plasma Physics: Transport processes, upflow, wave heating}
}

@Article{Xiao2007,
  Title                    = {Satellite observations of separator-line geometry of three-dimensional magnetic reconnection},
  Author                   = {Xiao, CJ and Wang, XG and Pu, ZY and Ma, ZW and Zhao, H and Zhou, GP and Wang, JX and Kivelson, MG and Fu, SY and Liu, ZX and {others}},
  Journal                  = {Nature Physics},
  Year                     = {2007},
  Number                   = {9},
  Pages                    = {609--613},
  Volume                   = {3}
}

@Article{Yahnin1997,
  Title                    = {on the source region of traveling convection vortices},
  Author                   = {Yahnin, A. G. and Vorobjev, V. G. and Bösinger, T. and Rasinkangas, R. and Sibeck, D. G. and Newell, P. T.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {1997},
  Pages                    = {237--240},
  Volume                   = {24},

  Abstract                 = {We reexamined two well-documented traveling convection vortices (TCVs) which were observed in the pre-noon sector to investigate their position relative to particle precipitation boundaries obtained from low-altitude satellite measurements. DMSP observations of precipitating particles indicate that the TCVs' focii and trajectories lay inside of the plasma sheet near the CPS/BPS boundary. The TCVs occurred within the poleward part of the belt of trapped energetic (E {\textgreater} 30 keV) electrons. These findings and some auroral observations suggest that it is possible for TCVs to map to regions well within the magnetosphere, contrary to the general belief that TCV related currents originate at the magnetopause or LLBL.},
  ISSN                     = {0094-8276},
  Keywords                 = {Meteorology and Atmospheric Dynamics: Convective processes},
  Url                      = {http://adsabs.harvard.edu/abs/1997GeoRL..24..237Y}
}

@Article{Yamauchi1996,
  Title                    = {Dynamic response of the cusp morphology to the solar wind: {A} case study during passage of the solar wind plasma cloud on {February} 21, 1994},
  Author                   = {Yamauchi, M and Nilsson, H and Eliasson, L and Norberg, O and Boehm, M and Clemmons, JH and Lepping, RP and Blomberg, Lars and Ohtani, S-I and Yamamoto, T and {others}},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1996},
  Number                   = {A11},
  Pages                    = {24675--24687},
  Volume                   = {101}
}

@Article{Yan2014,
  Title                    = {Kelvin-{Helmholtz} vortices observed by {THEMIS} at the duskside of the magnetopause under southward interplanetary magnetic field},
  Author                   = {Yan, Guang Qing and Mozer, F. S. and Shen, C. and Chen, T. and Parks, G. K. and Cai, C. L. and McFadden, J. P.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2014},
  Number                   = {13},
  Pages                    = {4427--4434},
  Volume                   = {41},

  Url                      = {http://onlinelibrary.wiley.com/doi/10.1002/2014GL060589/full},
  Urldate                  = {2014-10-22}
}

@Article{Yang2010,
  Title                    = {Direct retrieval of sulfur dioxide amount and altitude from spaceborne hyperspectral {UV} measurements: {Theory} and application},
  Author                   = {Yang, Kai and Liu, Xiong and Bhartia, Pawan K. and Krotkov, Nickolay A. and Carn, Simon A. and Hughes, Eric J. and Krueger, Arlin J. and Spurr, Robert JD and Trahan, Samuel G.},
  Journal                  = {Journal of Geophysical Research: Atmospheres (1984‚Äö√Ñ√∂‚àö√ë‚àö¬®2012)},
  Year                     = {2010},
  Number                   = {D2},
  Volume                   = {115},

  Shorttitle               = {Direct retrieval of sulfur dioxide amount and altitude from spaceborne hyperspectral {UV} measurements},
  Url                      = {http://onlinelibrary.wiley.com/doi/10.1029/2010JD013982/full},
  Urldate                  = {2014-11-13}
}

@Article{Yao2010,
  Title                    = {Identification of prominence ejecta by the proton distribution function and magnetic fine structure in interplanetary coronal mass ejections in the inner heliosphere},
  Author                   = {Yao, S. and Marsch, E. and Tu, C.-Y. and Schwenn, R.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2010},

  Month                    = may,
  Pages                    = {5103},
  Volume                   = {115},

  Doi                      = {10.1029/2009JA014914},
  Keywords                 = {6050, 7836), and magnetic clouds, driver gases, Interplanetary Physics: Coronal mass ejections (7513), Interplanetary Physics: Ejecta, Interplanetary Physics: MHD waves and turbulence (2752, Interplanetary Physics: Solar wind plasma}
}

@Article{Yao2011,
  Title                    = {{Electromagnetic waves on ion gyro-radii scales across the magnetopause}},
  Author                   = {Yao, Y. and Chaston, C. C. and Glassmeier, K.-H. and Angelopoulos, V.},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2011},

  Month                    = {may},
  Number                   = {9},
  Pages                    = {n/a--n/a},
  Volume                   = {38},

  __markedentry            = {[suleimanbaraka:6]},
  Doi                      = {10.1029/2011GL047328},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Yao et al/Geophysical Research Letters/Yao et al. - 2011 - Electromagnetic waves on ion gyro-radii scales across the magnetopause.pdf:pdf},
  ISSN                     = {00948276},
  Keywords                 = {http://dx.doi.org/10.1029/2011GL047328, doi:10.102},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23},
  Url                      = {http://doi.wiley.com/10.1029/2011GL047328}
}

@Article{Yau1995,
  Title                    = {Akebono observations of electron temperature anisotropy in the polar wind},
  Author                   = {Yau, AW and Whalen, BA and Abe, T and Mukai, T and Oyama, KI and Chang, T},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1995},
  Number                   = {A9},
  Pages                    = {17451--17463},
  Volume                   = {100},

  Annote                   = {Added to JabRef: 2015.04.18}
}

@Article{Yau2007,
  Title                    = {The polar wind: {Recent} observations},
  Author                   = {Yau, Andrew W. and Abe, Takumi and Peterson, W. K.},
  Journal                  = {Journal of Atmospheric and Solar-Terrestrial Physics},
  Year                     = {2007},
  Number                   = {16},
  Pages                    = {1936--1983},
  Volume                   = {69},

  File                     = {[PDF] from colorado.edu:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/5IZX9N5C/Yau et al. - 2007 - The polar wind Recent observations.pdf:application/pdf;Snapshot:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/WQZA9KRD/S1364682607002416.html:text/html},
  Shorttitle               = {The polar wind},
  Url                      = {http://www.sciencedirect.com/science/article/pii/S1364682607002416},
  Urldate                  = {2015-12-09}
}

@Article{Yau2007a,
  Title                    = {The polar wind: {Recent} observations},
  Author                   = {Yau, Andrew W. and Abe, Takumi and Peterson, W. K.},
  Journal                  = {J. Atmos. Solar-Terrestrial Phys.},
  Year                     = {2007},
  Pages                    = {1936--1983},
  Volume                   = {69},

  Abstract                 = {The polar wind is an ambipolar outflow of thermal plasma from the high-latitude ionosphere to the magnetosphere, and it primarily consists of H+, He+ and O+ ions and electrons. Statistical and episodic studies based primarily on ion composition observations on the ISIS-2, DE-1, Akebono and Polar satellites over the past four decades have confirmed the existence of the polar wind. These observations spanned the altitude range from 1000 to ???50,500 km, and revealed several important features in the polar wind that are unexpected from "classical" polar wind theories. These include the day-night asymmetry in polar wind velocity, which is 1.5-2.0 times larger on the dayside; appreciable O+ flow at high altitudes, where the velocity at 5000-10,000 km is of 1-4 km/s; and significant electron temperature anisotropy in the sunlit polar wind, in which the upward-to-downward electron temperature ratio is 1.5-2. These features are attributable to a number of "non-classical" polar wind ion acceleration mechanisms resulting from strong ionospheric convection, enhanced electron and ion temperatures, and escaping atmospheric photoelectrons. The observed polar wind has an averaged ion temperature of ???0.2-0.3 eV, and a rate of ion velocity increase with altitude that correlates strongly with electron temperature and is greatest at low altitudes ({\textless}4000 km for H+). The rate of velocity increase below 4000 km is larger at solar minimum than at solar maximum. Above 4000 km, the reverse is the case. This suggests that the dominant polar wind ion acceleration process may be different at low and high altitudes, respectively. At a given altitude, the polar wind velocity is highly variable, and is on average largest for H+ and smallest for O+. Near solar maximum, H+, He+, and O+ ions typically reach a velocity of 1 km/s near 2000, 3000, and 6000 km, respectively, and velocities of 12, 7, and 4 km/s, respectively, at 10,000 km altitude. Near solar minimum, the velocity of all three species is smaller at high altitudes. Observationally it is not always possible to unambiguously separate an energized "non-polar-wind" ion such as a low-energy "cleft ion fountain" ion that has convected into a polar wind flux tube from an energized "polar-wind" ion that is accelerated locally by "non-classical" polar-wind ion acceleration mechanisms. Significant questions remain on the relative contribution between the cleft ion fountain, auroral bulk upflow, and the topside polar-cap ionosphere to the O+ polar wind population at high altitudes, the effect of positive spacecraft charging on the lowest-energy component of the H+ polar wind population, and the relative importance of the various classical and non-classical ion acceleration mechanisms. These questions pose several challenges in future polar wind observations: These include measurement of the lowest-energy component in the presence of positive spacecraft potential, definitive determination and if possible active control of the spacecraft potential, definitive discrimination between polar wind and other inter-mixed thermal ion populations, measurement of the three-dimensional ion drift velocity vector and the parallel and perpendicular ion temperatures or the detailed three-dimensional velocity distribution function, and resolution of He+ and other minor ion species in the polar wind population. ?? 2007 Elsevier Ltd. All rights reserved.},
  Doi                      = {10.1016/j.jastp.2007.08.010},
  ISSN                     = {13646826},
  Keywords                 = {ionosphere, Outflow, Polar wind}
}

@Article{Yee1966,
  Title                    = {Numerical solution of initial boundary value problems involving {Maxwell}‚àö√Æ‚àö‚àè≈í¬©s equations in isotropic media},
  Author                   = {Yee, Kane S and {others}},
  Journal                  = {IEEE Trans. Antennas Propag},
  Year                     = {1966},
  Number                   = {3},
  Pages                    = {302--307},
  Volume                   = {14}
}

@InProceedings{Yermolaev1997,
  Title                    = {Ion distribution dynamics near the {Earth}�s bow shock: first measurements with the 2D ion energy spectrometer {CORALL} on the {INTERBALL}/{Tail}-probe satellite},
  Author                   = {Yermolaev, Yu I and Fedorov, AO and Vaisberg, OL and Balebanov, VM and Obod, Yu A and Jimenez, R and Fleites, J and Llera, L and Omelchenko, AN},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {1997},
  Pages                    = {533--541},
  Publisher                = {Springer},
  Volume                   = {15}
}

@Article{Yin2007,
  Title                    = {Kinetic {Alfvén} waves and electron physics. {I}. {Generation} from ion-ion streaming},
  Author                   = {Yin, L. and Winske, D. and Daughton, W. and Bowers, K. J.},
  Journal                  = {Phys. Plasmas},
  Year                     = {2007},

  Month                    = jun,
  Number                   = {6},
  Pages                    = {062104},
  Volume                   = {14},

  Doi                      = {10.1063/1.2734950},
  Keywords                 = {Macroinstabilities, Magnetohydrodynamic waves, Particle-in-cell method, Plasma kinetic equations, Shock waves and discontinuities, Transport Properties}
}

@Article{Yin2001,
  Title                    = {Particle {Hall}-{MHD} simulation of collisionless reconnection: {Ion} gyro-radius correction},
  Author                   = {Yin, L. and Winske, D. and Gary, S. P. and Birn, J.},
  Journal                  = {{\textbackslash}grl},
  Year                     = {2001},
  Pages                    = {2173--2176},
  Volume                   = {28},

  Doi                      = {10.1029/2000GL012797},
  Keywords                 = {Magnetospheric Physics: Numerical modeling, Magnetospheric Physics: Plasma sheet, Space Plasma Physics: Magnetic reconnection, Space Plasma Physics: Numerical simulation studies}
}

@Article{Yin2001a,
  Title                    = {{Particle Hall{\&}{\#}8208;MHD simulation of collisionless reconnection: Ion gyro{\&}{\#}8208;radius correction}},
  Author                   = {Yin, L and Winske, D and Gary, S P and Birn, J},
  Year                     = {2001},
  Number                   = {11},
  Pages                    = {2173--2176},
  Volume                   = {28},

  __markedentry            = {[suleimanbaraka:6]},
  File                     = {:Users/suleimanbaraka/Documents/Mendeley Desktop/Yin et al/Unknown/Yin et al. - 2001 - Particle Hall{\&}{\#}8208MHD simulation of collisionless reconnection Ion gyro{\&}{\#}8208radius correction.pdf:pdf},
  Keywords                 = {http://dx.doi.org/10.1029/2000GL012797, doi:10.102},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Young2005,
  Title                    = {The {Ne}/{O} abundance ratio in the quiet {Sun}},
  Author                   = {Young, P. R.},
  Journal                  = {{\textbackslash}aap},
  Year                     = {2005},

  Month                    = dec,
  Pages                    = {L45--L48},
  Volume                   = {444},

  Doi                      = {10.1051/0004-6361:200500206}
}

@Article{Yuan2008,
  Title                    = {Numerical simulation of electron distributions upstream and downstream of high {Mach} number quasi-perpendicular collisionless shocks},
  Author                   = {Yuan, Xingqiu and Cairns, Iver H and Robinson, Peter A},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2008},
  Number                   = {A8},
  Volume                   = {113}
}

@Article{Yuan2007,
  Title                    = {Effects of overshoots on electron distributions upstream and downstream of quasi-perpendicular collisionless shocks},
  Author                   = {Yuan, Xingqiu and Cairns, Iver H and Robinson, PA and Kuncic, Z},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2007},
  Number                   = {A5},
  Volume                   = {112}
}

@Article{Yuan2008a,
  Title                    = {Effects of shock parameters on upstream energetic electron burst events},
  Author                   = {Yuan, Xingqiu and Cairns, Iver H and Trichtchenko, Larisa and Rankin, Robert},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {2008},
  Number                   = {A9},
  Volume                   = {113}
}

@Article{Zelenyi2013,
  Title                    = {Mechanisms of {Spontaneous} {Reconnection}: {From} {Magnetospheric} to {Fusion} {Plasma}},
  Author                   = {Zelenyi, Lev and Artemyev, Anton},
  Journal                  = {Space Sci. Rev.},
  Year                     = {2013},

  Month                    = mar,
  Number                   = {2-4},
  Pages                    = {441--457},
  Volume                   = {178},

  Doi                      = {10.1007/s11214-013-9959-8},
  ISSN                     = {0038-6308},
  Keywords                 = {Magnetic reconnection, tearing instability},
  Url                      = {http://link.springer.com/10.1007/s11214-013-9959-8}
}

@Article{Zelenyi1930,
  Title                    = {Thin and superthin ion current sheets. {Quasi}-adiabatic and nonadiabatic models},
  Author                   = {Zelenyi, LM and Sitnov, MI and Malova, HV and Sharma, AS},
  Journal                  = {Nonlinear processes in Geophysics},
  Year                     = {1930},
  Number                   = {3/4},
  Pages                    = {127--139},
  Volume                   = {7}
}

@Article{Zeng2006,
  Title                    = {Characteristic ion distributions in the dynamic auroral transition region},
  Author                   = {Zeng, W. and Horwitz, J. L. and Tu, J.-N.},
  Journal                  = {J. Geophys. Res.},
  Year                     = {2006},
  Number                   = {A4},
  Volume                   = {111},

  Doi                      = {10.1029/2005JA011417},
  ISSN                     = {0148-0227},
  Language                 = {en},
  Url                      = {http://doi.wiley.com/10.1029/2005JA011417},
  Urldate                  = {2015-04-18}
}

@Article{Zenitani2011,
  Title                    = {The inner structure of collisionless magnetic reconnection: {The} electron-frame dissipation measure and {Hall} fields},
  Author                   = {Zenitani, Seiji and Hesse, Michael and Klimas, Alex and Black, Carrie and Kuznetsova, Masha},
  Journal                  = {Physics of Plasmas (1994-present)},
  Year                     = {2011},
  Number                   = {12},
  Pages                    = {122108},
  Volume                   = {18},

  Shorttitle               = {The inner structure of collisionless magnetic reconnection},
  Url                      = {http://scitation.aip.org/content/aip/journal/pop/18/12/10.1063/1.3662430},
  Urldate                  = {2014-05-31}
}

@Article{Zesta2000,
  Title                    = {The auroral signature of earthward flow bursts observed in the magnetotail},
  Author                   = {Zesta, Eftyhia and Lyons, Lawrence R and Donovan, Eric},
  Journal                  = {Geophys. Res. Lett.},
  Year                     = {2000},
  Number                   = {20},
  Pages                    = {3241--3244},
  Volume                   = {27}
}

@Article{Zesta2004,
  Title                    = {A detailed description of the solar wind triggers of two dayside transients: {Events} of 25 {July} 1997},
  Author                   = {Zesta, Eftyhia and Sibeck, David G.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2004},
  Pages                    = {1201},
  Volume                   = {109},

  Abstract                 = {Traveling Convection Vortices (TCVs), a specific type of dayside transient event, offer a good opportunity to study the modes of interaction between the solar wind, bow shock and the magnetosphere/ionosphere system. We study here in detail the solar wind triggers of two TCV events that occurred at 1500 UT and 1835 UT on 25 July 1997. During these two events there was a fortuitous conjunction of four solar wind monitors near the Earth's magnetosphere. We were able to identify the exact solar wind discontinuity that triggered each ground TCV. We found that the 1500 UT TCV was triggered by the density (and thus dynamic pressure) enhancement accompanying a tangential discontinuity. We were able to determine the orientation of the discontinuity plane and thus predict, in good agreement with observations, the propagation of the discontinuity between the four spacecraft as well as the propagation of the transient in the magnetosphere (geosynchronous) and ionosphere. The ground transient was generated in the early afternoon local time and then propagated westward, first toward local noon and then away from noon toward dawn. The 1835 UT TCV, which was stronger, was triggered by a more complicated solar wind discontinuity that exhibited significant spatial structure and an unusual propagation pattern. A detailed analysis of the orientation of the discontinuity fronts explained the propagation of the discontinuity in the solar wind. Even though the discontinuity did not carry a significant dynamic pressure enhancement, it had the properties required to generate a hot flow anomaly (HFA) or a foreshock cavity at the bow shock. The corresponding pressure reduction in the magnetosheath interacted with the magnetosphere to generate the transient near local noon that propagates eastward toward dusk. Geosynchronous observations confirm these conclusions. To strengthen our conclusions, we compared the discontinuity that triggered the ground TCV event with four other discontinuities that occurred in the same 2-hour window. We found that none of the other four discontinuities carried significant dynamic pressure enhancements or had properties required to create a HFA at the bow shock. They did not trigger detectable transients on the ground. It thus seems that TCVs can be triggered by solar wind discontinuities that either carry dynamic pressure enhancements (or alternatively reductions) or by discontinuities that create HFAs or foreshock cavities at the bow shock.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetopause cusp and boundary layers Interplanetary Physics: Discontinuities Magnetospheric Physics: Magnetosphere/ionosphere interactions dayside transients traveling convection vortices hot flow anomaly foreshock cavities solar wind triggering},
  Url                      = {http://adsabs.harvard.edu/abs/2004JGRA..109.1201Z}
}

@Article{Zesta2013,
  Title                    = {The effect of the {January} 10, 1997, pressure pulse on the magnetosphere-ionosphere current system},
  Author                   = {Zesta, E and Singer, HJ and Lummerzheim, D and Russell, CT and Lyons, LR and Brittnacher, MJ},
  Journal                  = {Magnetospheric Current Systems},
  Year                     = {2013},
  Pages                    = {217--226}
}

@Article{Zhang2013,
  Title                    = {Predicting the location of polar cusp in the {Lyon}-{Fedder}-{Mobarry} global magnetosphere simulation},
  Author                   = {Zhang, B. and Brambles, O. and Lotko, W. and Dunlap-Shohl, W. and Smith, R. and Wiltberger, M. and Lyon, J.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = oct,
  Pages                    = {6327--6337},
  Volume                   = {118},

  Doi                      = {10.1002/jgra.50565},
  Keywords                 = {global simulations, polar cusp}
}

@Article{Zhang2010,
  Title                    = {Time {History} of {Events} and {Macroscale} {Interactions} during {Substorms} observations of a series of hot flow anomaly events},
  Author                   = {Zhang, H. and Sibeck, D. G. and Zong, Q.-G. and Gary, S. P. and McFadden, J. P. and Larson, D. and Glassmeier, K.-H. and Angelopoulos, V.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2010},
  Pages                    = {12235},
  Volume                   = {115},

  Abstract                 = {A series of seven hot flow anomaly (HFA) events has been observed by the Time History of Events and Macroscale Interactions during Substorms (THEMIS) C spacecraft just upstream from the subsolar bow shock from 0100 to 1300 UT on 19 August 2008. Both young (no shocks at edges, two distinct ion populations) and mature (strong shocks at edges, a single hot ion population) HFAs have been observed. Further upstream, THEMIS B observed four proto-HFAs (density and magnetic field strength depletions, plasma heating but no flow deflections) which later developed into HFAs observed by THEMIS C. We present evidence indicating that electromagnetic right-hand resonant ion beam instabilities heat ions inside HFAs. Observations of small-amplitude perturbations (ΔB/B {\textless} 50\%) consistent with the resonant ion beam instability in a proto-HFA, 30 s electromagnetic waves (ΔB/B ˜ 1) in a young HFA, and magnetic pulsations in a mature HFA (ΔB/B ˜ 4) indicate that they are at early, middle, and late (nonlinear) stages of the electromagnetic right-hand resonant ion beam instabilities. Both young and mature HFAs are associated with strong electromagnetic waves near the lower hybrid frequency (0.1-1 Hz). The lower hybrid waves are the likely source of the electron heating inside HFAs. THEMIS B observations of four proto-HFAs which later developed into HFAs observed by THEMIS C indicate that these four HFAs might extend beyond 14 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} upstream from the bow shock, while the other three HFAs may extend between 5 and 14 R{\textless}SUB{\textgreater}E{\textless}/SUB{\textgreater} upstream from the bow shock. We present an example of an HFA that lies displaced toward the side of the tangential discontinuity with a quasi-parallel bow shock configuration rather than lying centered on the driving interplanetary magnetic field discontinuity.},
  ISSN                     = {0148-0227},
  Keywords                 = {Space Plasma Physics: Wave/particle interactions (2483 6984) Space Plasma Physics: Plasma energization Ionosphere: Plasma waves and instabilities (2772) Space Plasma Physics: Shock waves (4455) Space Plasma Physics: Kinetic waves and instabilities hot flow anomaly particle heating wave particle interaction},
  Url                      = {http://adsabs.harvard.edu/abs/2010JGRA..11512235Z}
}

@Article{Zhang2012,
  Title                    = {Global magnetospheric response to an interplanetary shock: {THEMIS} observations},
  Author                   = {Zhang, H. and Sibeck, D. G. and Zong, Q.-G. and McFadden, J. P. and Larson, D. and Glassmeier, K.-H. and Angelopoulos, V.},
  Journal                  = {Annales Geophysicae},
  Year                     = {2012},
  Pages                    = {379--387},
  Volume                   = {30},

  Abstract                 = {We investigate the global response of the geospace plasma environment to an interplanetary (IP) shock at 02:24 UT on 28 May 2008 from multiple THEMIS spacecraft observations in the magnetosheath (THEMIS B and C), the mid-afternoon magnetosphere (THEMIS A), and the dusk magnetosphere (THEMIS D and E). The interaction of the transmitted IP shock with the magnetosphere has global effects. Consequently, it can affect geospace plasma significantly. After interacting with the bow shock, the IP shock transmitted a fast shock and a discontinuity which propagated through the magnetosheath toward the Earth at speeds of 301 km s{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater} and 137 km s{\textless}SUP{\textgreater}-1{\textless}/SUP{\textgreater}, respectively. THEMIS A observations indicate that the IP shock changed the properties of a plasmaspheric plume significantly. The plasmaspheric plume density increased rapidly from 10 to 100 cm{\textless}SUP{\textgreater}-3{\textless}/SUP{\textgreater} in 4 min and the ion distribution changed from an isotropic to a strongly anisotropic distribution. Electromagnetic ion cyclotron (EMIC) waves observed by THEMIS A are most likely excited by the anisotropic ion distributions caused by the IP shock impact. THEMIS A, but not D or E, observed a plasmaspheric plume in the dayside magnetosphere. Multiple spacecraft observations indicate that the dawn-side edge of the plasmaspheric plume was located between THEMIS A and D (or E).},
  ISSN                     = {0992-7689},
  Url                      = {http://adsabs.harvard.edu/abs/2012AnGeo..30..379Z}
}

@Article{Zhang2013a,
  Title                    = {Spontaneous hot flow anomalies at quasi-parallel shocks: 1. {Observations}},
  Author                   = {Zhang, H. and Sibeck, D. G. and Zong, Q.-G. and Omidi, N. and Turner, D. and Clausen, L. B. N.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},
  Pages                    = {3357--3363},
  Volume                   = {118},

  Abstract                 = {We present Time History of Events and Macroscale Interactions during Substorms (THEMIS) observations of a "Spontaneous Hot Flow Anomaly" (SHFA) upstream from the prenoon bow shock at 0431 UT on 12 August 2007. Although the SHFA exhibited the greatly heated and deflected solar wind plasmas used to identify hot flow anomalies (HFAs), it did not result from the standard mechanism invoked for the formation of HFAs, namely the interaction of an interplanetary magnetic field (IMF) discontinuity with the bow shock. We employ THEMIS A, B, C, and D observations to describe the evolution of the event from a proto-SHFA exhibiting regions of depressed magnetic field strength and density but little evidence for plasma heating or flow deflection, to a well-developed SHFA further downstream. These observations show that SHFA can be generated without the presence of an IMF discontinuity and are therefore a new category of HFAs.},
  ISSN                     = {0148-0227},
  Keywords                 = {hot flow anomaly quasi-parallel shocks foreshock},
  Url                      = {http://adsabs.harvard.edu/abs/2013JGRA..118.3357Z}
}

@Article{Zhang2009,
  Title                    = {{Dynamic motion of the bow shock and the magnetopause observed by THEMIS spacecraft}},
  Author                   = {Zhang, H. and Zong, Q. G. and Sibeck, D. G. and Fritz, T. A. and McFadden, J. P. and Glassmeier, K. H. and Larson, D.},
  Journal                  = {J. Geophys. Res. Sp. Phys.},
  Year                     = {2009},
  Number                   = {1},
  Volume                   = {114},

  __markedentry            = {[suleimanbaraka:]},
  Abstract                 = {We present an observational study of the of the and the and suggest that the of the is due to the interaction of an interplanetary with the Earth's . B crossed the , a },
  Doi                      = {10.1029/2008JA013488},
  ISSN                     = {21699402},
  Owner                    = {suleimanbaraka},
  Timestamp                = {2016.02.23}
}

@Article{Zhang2009a,
  Title                    = {Dynamic motion of the bow shock and the magnetopause observed by {THEMIS} spacecraft},
  Author                   = {Zhang, H. and Zong, Q.-G. and Sibeck, D. G. and Fritz, T. A. and McFadden, J. P. and Glassmeier, K.-H. and Larson, D.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2009},
  Volume                   = {114},

  Abstract                 = {We present an observational study of the dynamic motion of the bow shock and the magnetopause and suggest that the dynamic motion of the bow shock is due to the interaction of an interplanetary shock with the Earth's bow shock. THEMIS B spacecraft crossed the magnetopause, a discontinuity and the bow shock successively in 5 min during its outbound journey on 10 July 2007. Following THEMIS B, THEMIS C, D, E and A consecutively crossed the magnetopause and the discontinuity but not the bow shock. Timing analysis shows that the magnetopause and the discontinuity were moving earthward with speeds of 47 km/s and 90 km/s, respectively. There is a trend that the discontinuity decelerates as it propagates toward the magnetopause. We suggest that the dynamic motion and the discontinuity are results of the interaction of a weak (M {\textless}SUB{\textgreater} A {\textless}/SUB{\textgreater} = 1.4) interplanetary shock with the Earth's bow shock. After the interaction, the transmitted interplanetary shock took the form of a discontinuity where total magnetic field and density increase and the temperature decreases. The rotation of the magnetic field across this discontinuity was similar to that of the interplanetary shock. The expected fast shock ahead of the discontinuity for shock-shock interaction was not observed.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Solar wind/magnetosphere interactions Interplanetary Physics: Interplanetary shocks Interplanetary Physics: Pickup ions Interplanetary Physics: Discontinuities (7811) Magnetospheric Physics: Magnetopause and boundary layers},
  Url                      = {http://adsabs.harvard.edu/abs/2009JGRA..114.0C12Z}
}

@Article{Zhang2006,
  Title                    = {A statistical comparison of hot-ion properties at geosynchronous orbit during intense and moderate geomagnetic storms at solar maximum and minimum},
  Author                   = {Zhang, J. and Liemohn, M. W. and Thomsen, M. F. and Kozyra, J. U. and Denton, M. H. and Borovsky, J. E.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2006},

  Month                    = jul,
  Pages                    = {7206},
  Volume                   = {111},

  Doi                      = {10.1029/2005JA011559},
  Keywords                 = {geosynchronous orbit, Interplanetary Physics: Solar cycle variations (7536), magnetospheric physics, Magnetospheric Physics: Magnetic storms and substorms (7954), Magnetospheric Physics: Magnetosphere: inner, Magnetospheric Physics: Magnetospheric configuration and dynamics, Magnetospheric Physics: Plasma sheet, magnetospheric plasma sources}
}

@Article{Zhang2012a,
  Title                    = {Inner plasma structure of the low-latitude reconnection layer},
  Author                   = {Zhang, Q.-H. and Dunlop, M. W. and Lockwood, M. and Lavraud, B. and Bogdanova, Y. V. and Hasegawa, H. and Yang, H.-G. and Liu, R.-Y. and Hu, H.-Q. and Zhang, B.-C. and Pu, Z.-Y. and Yang, Z.-W. and Wang, J. and Taylor, M. G. G. T. and Berchem, J. and Constantinescu, D. and Volwerk, M. and Frey, H. and Fazakerley, A. N. and Shen, C. and Shi, J.-K. and Sibeck, D. and Escoubet, P. and Wild, J. A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2012},
  Pages                    = {8205},
  Volume                   = {117},

  Abstract                 = {We report a clear transition through a reconnection layer at the low-latitude magnetopause which shows a complete traversal across all reconnected field lines during northwestward interplanetary magnetic field (IMF) conditions. The associated plasma populations confirm details of the electron and ion mixing and the time history and acceleration through the current layer. This case has low magnetic shear with a strong guide field and the reconnection layer contains a single density depletion layer on the magnetosheath side which we suggest results from nearly field-aligned magnetosheath flows. Within the reconnection boundary layer, there are two plasma boundaries, close to the inferred separatrices on the magnetosphere and magnetosheath sides (S{\textless}SUB{\textgreater}sp{\textless}/SUB{\textgreater} and S{\textless}SUB{\textgreater}sh{\textless}/SUB{\textgreater}) and two boundaries associated with the Alfvén waves (or Rotational Discontinuities, RD{\textless}SUB{\textgreater}sp{\textless}/SUB{\textgreater} and RD{\textless}SUB{\textgreater}sh{\textless}/SUB{\textgreater}). The data are consistent with these being launched from the reconnection site and the plasma distributions are well ordered and suggestive of the time elapsed since reconnection of the field lines observed. In each sub-layer between the boundaries the plasma distribution is different and is centered around the current sheet, responsible for magnetosheath acceleration. We show evidence for a velocity dispersion effect in the electron anisotropy that is consistent with the time elapsed since reconnection. In addition, new evidence is presented for the occurrence of partial reflection of magnetosheath electrons at the magnetopause current layer.},
  ISSN                     = {0148-0227},
  Keywords                 = {density depletion layer magnetic reconnection reconnection layer Magnetospheric Physics: Magnetic reconnection (7526 7835) Magnetospheric Physics: Magnetopause and boundary layers Space Plasma Physics: Particle acceleration},
  Url                      = {http://adsabs.harvard.edu/abs/2012JGRA..117.8205Z}
}

@InProceedings{Zhang2005,
  Title                    = {Double {Star}/{Cluster} observation of neutral sheet oscillations on 5 {August} 2004},
  Author                   = {Zhang, TL and Nakamura, R and Volwerk, M and Runov, A and Baumjohann, W and Eichelberger, HU and Carr, C and Balogh, A and Sergeev, V and Shi, JK and {others}},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2005},
  Pages                    = {2909--2914},
  Publisher                = {Copernicus GmbH},
  Volume                   = {23}
}

@Article{Zhao2013,
  Title                    = {Association of solar wind proton flux extremes with pseudostreamers},
  Author                   = {Zhao, L. and Gibson, S. E. and Fisk, L. A.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2013},

  Month                    = jun,
  Pages                    = {2834--2841},
  Volume                   = {118},

  Doi                      = {10.1002/jgra.50335},
  Keywords                 = {Solar Corona, Solar cycle, Solar Wind, sun}
}

@InProceedings{Zheng2005,
  Title                    = {Cluster observation of continuous reconnection at dayside magnetopause in the vicinity of cusp},
  Author                   = {Zheng, Y and Le, G and Slavin, JA and Goldstein, ML and Cattell, C and Balogh, A and Lucek, EA and Reme, H and Eastwood, JP and Wilber, M and {others}},
  Booktitle                = {Annales {Geophysicae}},
  Year                     = {2005},
  Pages                    = {2199--2215},
  Volume                   = {23},

  Url                      = {http://hal.archives-ouvertes.fr/hal-00329427/}
}

@Article{Zhou2010,
  Title                    = {Interplanetary {Shock} {Generated} {Ionospheric} {Traveling} {Convection} {Vortex} {Near} {Local} {Noon}},
  Author                   = {Zhou, X.-Y. and Sibeck, D. G. and Amm, O. and Ruohoniemi, J. M.},
  Journal                  = {Advances in Geosciences, Volume 21: Solar Terrestrial (ST)},
  Year                     = {2010},
  Pages                    = {367},
  Volume                   = {21},

  Abstract                 = {Not Available},
  Url                      = {http://adsabs.harvard.edu/abs/2010aogs...21..367Z}
}

@Article{Zhou2003,
  Title                    = {Shock aurora: {FAST} and {DMSP} observations},
  Author                   = {Zhou, X.-Y. and Strangeway, R. J. and Anderson, P. C. and Sibeck, D. G. and Tsurutani, B. T. and Haerendel, G. and Frey, H. U. and Arballo, J. K.},
  Journal                  = {Journal of Geophysical Research (Space Physics)},
  Year                     = {2003},
  Pages                    = {8019},
  Volume                   = {108},

  Abstract                 = {Global signatures of the aurora caused by interplanetary shocks/pressure pulses have been studied in recent years using ultraviolet imager data from polar orbiting spacecraft. The signatures include the occurrence of the aurora first near local noon and then propagation antisunward along the auroral oval at very high speeds. To better understand the mechanisms of particle precipitation, in this paper we study shock auroras using near-Earth observations of the FAST and DMSP satellites. We have studied the events that occurred during 1996-2000 where FAST and/or DMSP crossed the dawnside or duskside auroral zone within 10 min after shocks/pressure pulses arrived at the nose of the magnetopause. It is found that the electron precipitation increased significantly above the dawnside and duskside auroral oval zone after the shock/pressure pulse arrivals. The precipitation structure is low-energy electrons ({\textless}˜1 keV) at higher latitudes (˜75°-83° ILAT within 0600-0900 MLT) and high-energy electrons (˜1-10 keV) at lower latitudes (˜65°-79° ILAT) of the auroral zone. There are a few degrees (1°-4° ILAT) of overlap between these two categories of precipitated electrons. The precipitation of low-energy electrons was along highly structured field-aligned currents. The precipitation of the high-energy electrons was highly isotropic filling the loss cone. Possible mechanisms of field-aligned current generation are some dynamic processes occurring on the dayside magnetopause, such as magnetic shearing, magnetopause perturbation, magnetic reconnection, and Alfvén wave generation. Adiabatic compression might have caused the high-energy electron precipitation. On the basis of observations of FAST and DMSP, shock auroras are speculated to be diffuse auroras at the lower latitudes of the dayside auroral oval and discrete auroras on the poleward boundary of the oval with a few latitude degree overlap of the two types of auroras.},
  ISSN                     = {0148-0227},
  Keywords                 = {Magnetospheric Physics: Auroral phenomena (2407) Magnetospheric Physics: Magnetopause cusp and boundary layers Ionosphere: Particle precipitation Magnetospheric Physics: Solar wind/magnetosphere interactions Magnetospheric Physics: Magnetosphere-outer solar wind-magnetosphere-ionosphere interaction auroras particle precipitation},
  Url                      = {http://adsabs.harvard.edu/abs/2003JGRA..108.8019Z}
}

@Article{Zhu1996,
  Title                    = {Tearing instability, flux ropes, and the kinetic current sheet kink instability in the {Earth}'s magnetotail: {A} three-dimensional perspective from particle simulations},
  Author                   = {Zhu, Zhongwei and Winglee, RM},
  Journal                  = {Journal of Geophysical Research: Space Physics (1978–2012)},
  Year                     = {1996},
  Number                   = {A3},
  Pages                    = {4885--4897},
  Volume                   = {101}
}

@Article{Zhuravlev1987,
  Title                    = {Sm-{Nd} age of relicts of the granite-greenstone terrain basement in the central {Dnieper} region},
  Author                   = {Zhuravlev, D. Z. and Pukhtel', I. S. and Samsonov, A. V. and Simon, A. K.},
  Journal                  = {Akademiia Nauk SSSR Doklady},
  Year                     = {1987},
  Pages                    = {1203--1208},
  Volume                   = {294},

  Keywords                 = {Earth (Planet), Geochronology, Granite, Igneous Rocks, Neodymium, Petrology, Planetary Composition, Rivers, Samarium, Terrain, U.S.S.R.}
}

@Article{Zoogman2011,
  Title                    = {Ozone air quality measurement requirements for a geostationary satellite mission},
  Author                   = {Zoogman, Peter and Jacob, Daniel J and Chance, Kelly and Zhang, Lin and Le Sager, Philippe and Fiore, Arlene M and Eldering, Annmarie and Liu, Xiong and Natraj, Vijay and Kulawik, Susan S},
  Journal                  = {Atmos. Environ.},
  Year                     = {2011},
  Number                   = {39},
  Pages                    = {7143--7150},
  Volume                   = {45}
}

@Article{Zurbuchen2007,
  Title                    = {A {New} {View} of the {Coupling} of the {Sun} and the {Heliosphere}},
  Author                   = {Zurbuchen, T. H.},
  Journal                  = {{\textbackslash}araa},
  Year                     = {2007},

  Month                    = sep,
  Pages                    = {297--338},
  Volume                   = {45},

  Doi                      = {10.1146/annurev.astro.45.010807.154030}
}

@Article{Zurbuchen2006,
  Title                    = {In-{Situ} {Solar} {Wind} and {Magnetic} {Field} {Signatures} of {Interplanetary} {Coronal} {Mass} {Ejections}},
  Author                   = {Zurbuchen, T. H. and Richardson, I. G.},
  Journal                  = {ßr},
  Year                     = {2006},

  Month                    = mar,
  Pages                    = {31--43},
  Volume                   = {123},

  Doi                      = {10.1007/s11214-006-9010-4},
  Keywords                 = {Interplanetary coronal mass ejections, interplanetary magnetic field, Solar wind plasma}
}

@Article{Zurbuchen2012,
  Title                    = {Sources of {Solar} {Wind} at {Solar} {Minimum}: {Constraints} from {Composition} {Data}},
  Author                   = {Zurbuchen, T. H. and von Steiger, R. and Gruesbeck, J. and Landi, E. and Lepri, S. T. and Zhao, L. and Hansteen, V.},
  Journal                  = {ßr},
  Year                     = {2012},

  Month                    = nov,
  Pages                    = {41--55},
  Volume                   = {172},

  Doi                      = {10.1007/s11214-012-9881-5},
  Keywords                 = {Solar corona composition, Solar Wind}
}

@Article{Oeieroset2001,
  Title                    = {In situ detection of collisionless reconnection in the {Earth}'s magnetotail},
  Author                   = {Øieroset, M and Phan, TD and Fujimoto, M and Lin, RP and Lepping, RP},
  Journal                  = {Nature},
  Year                     = {2001},
  Number                   = {6845},
  Pages                    = {414--417},
  Volume                   = {412}
}

@Book{Akasofu1979,
  Title                    = {Dynamics of the {Magnetosphere}},
  Editor                   = {Akasofu, S.-I.},
  Publisher                = {Springer Netherlands},
  Year                     = {1979},

  Address                  = {Dordrecht},
  Series                   = {Astrophysics and {Space} {Science} {Library}},
  Volume                   = {78},

  ISBN                     = {978-94-009-9521-5 978-94-009-9519-2},
  Url                      = {http://link.springer.com/10.1007/978-94-009-9519-2},
  Urldate                  = {2015-04-18}
}

@Book{Birn2007a,
  Title                    = {Reconnection of magnetic fields: magnetohydrodynamics and collisionless theory and observations},
  Editor                   = {Birn, J. and Priest, E. R.},
  Publisher                = {Cambridge University Press},
  Year                     = {2007},

  Address                  = {Cambridge},

  ISBN                     = {978-0-521-85420-7 0-521-85420-2},
  Keywords                 = {Magnetic reconnection, Magnetohydrodynamics},
  Shorttitle               = {Reconnection of magnetic fields}
}

@Book{Daglis2004,
  Title                    = {Effects of space weather on technology infrastructure},
  Editor                   = {Daglis, I. A.},
  Publisher                = {Kluwer Academic Publishers},
  Year                     = {2004},

  Address                  = {Dordrecht ; Boston ; London},
  Number                   = {v. 176},
  Series                   = {{NATO} science series},

  Annote                   = {Includes 1 CD ROM in pocket attached to inside back cover},
  ISBN                     = {1-4020-2747-8 1-4020-2748-6 1-4020-2754-0},
  Keywords                 = {Extraterrestrial radiation, magnetic storms, Space environment}
}

@Book{Kan1991,
  Title                    = {Magnetospheric substorms},
  Editor                   = {Kan, Joseph R.},
  Publisher                = {American Geophysical Union},
  Year                     = {1991},

  Address                  = {Washington, DC},
  Number                   = {64},
  Series                   = {Geophysical monograph},

  Annote                   = {Papers from the Chapman Conference on Magnetospheric Substorms, held Sept. 3-7, 1990, in Hakone, Japan},
  ISBN                     = {0-87590-030-5},
  Keywords                 = {Congresses, Magnetospheric substorms}
}

@Book{Kivelson1995a,
  Title                    = {Introduction to space physics},
  Editor                   = {Kivelson, M. G. and Russell, C. T.},
  Publisher                = {Cambridge University Press},
  Year                     = {1995},

  Address                  = {Cambridge ; New York},

  ISBN                     = {0-521-45104-3 0-521-45714-9},
  Keywords                 = {PLANETS, Space Plasmas, sun}
}

@Book{Rozelot2006,
  Title                    = {Solar and heliospheric origins of space weather phenomena},
  Editor                   = {Rozelot, J.-P.},
  Publisher                = {Springer},
  Year                     = {2006},

  Address                  = {Berlin ; New York},
  Number                   = {699},
  Series                   = {Lecture notes in physics},

  Annote                   = {Lectures given at the 7th in a series of CNRS Solar Astrophysics Schools, held in Saint-Pierre d'OleÃÅron, France},
  ISBN                     = {978-3-540-33758-4 3-540-33758-X},
  Keywords                 = {Congresses, Environmental aspects, Solar Wind, Space environment, sun}
}

@Book{Scherer2005a,
  Title                    = {Space weather: the physics behind a slogan},
  Editor                   = {Scherer, Klaus and {Arbeitsgemeinschaft Extraterrestrische Forschung}},
  Publisher                = {Springer},
  Year                     = {2005},

  Address                  = {Berlin ; New York},
  Number                   = {656},
  Series                   = {Lecture notes in physics},

  Annote                   = {Introduction to space weather / Daniel N. Baker – The sun and its restless magnetic field / Manfred SchuÃàssler – The application of radio diagnostics to the study of the solar drivers of space weather / Alexander Warmuth, Gottfried Mann – Interplanetary disturbances / Robert F. Wimmer-Schweingruber – The magnetosphere / Antonius Otto – Space weather effects in the upper atmosphere : low and middle latitudes / Gerd W. ProÃàlss – Space weather effects in the upper atmosphere : high latitudes / Kristian Schlegel – Space weather effects on technology / Eino Valtonen – Radiation risks from space / Juergen Kiefer},
  ISBN                     = {3-540-22907-8},
  Keywords                 = {Solar-terrestrial physics, Space environment},
  Shorttitle               = {Space weather}
}

@Article{,
  Title                    = {@{ARTICLE}\{2004AnGeo..22.2577D, author = \{\{{Darrouzet}\}, {F}. and \{{D}\{{\textbackslash}'e\}cr\{{\textbackslash}'e\}au\}, {P}. and \{de {Keyser}\}, {J}. and \{{Masson}\}, {A}. and \{{Gallagher}\}, {D}. and \{{Santolik}\}, {O}. and \{{Sandel}\}, {B}. and \{{Trotignon}\}, {J}. and \{{Rauch}\}, {J}. and \{{Le} {Guirriec}\}, {E}. and \{{Canu}\}, {P}. and \{{Sedgemore}\}, {F}. and \{{Andr}\{{\textbackslash}'e\}\}, {M}. and \{{Lemaire}\}, {J}.\}, title = "\{{Density} structures inside the plasmasphere: {Cluster} observations\}", journal = \{{Annales} {Geophysicae}\}, year = 2004, month = jul, volume = 22, pages = \{2577-2585\}, doi = \{10.5194/angeo-22-2577-2004\}, adsurl = \{http://adsabs.harvard.edu/abs/2004AnGeo..22.2577D\}, adsnote = \{{Provided} by the {SAO}/{NASA} {Astrophysics} {Data} {System}\} \}}
}

@Misc{,
  Title                    = {Resorting {Query} {Results}},

  File                     = {Resorting Query Results:/Users/suleimanbaraka/Library/Application Support/Zotero/Profiles/cywumnk8.default/zotero/storage/EACNI8GX/nph-abs_connect.html:text/html},
  Url                      = {http://adsabs.harvard.edu/cgi-bin/nph-abs_connect},
  Urldate                  = {2015-10-02}
}

@Article{2014,
  Title                    = {Journal of {Geophysical} {Research} : {Space} {Physics} {Plasma} and energetic particle behaviors during asymmetric magnetic reconnection at the magnetopause},
  Year                     = {2014},
  Pages                    = {1658--1672},

  Doi                      = {10.1002/2013JA019168.Received}
}

@Book{2013,
  Title                    = {Physics of magnetospheric substorms},
  Publisher                = {Springer},
  Year                     = {2013},

  Address                  = {[S.l.]},

  ISBN                     = {94-010-1166-4 978-94-010-1166-2},
  Language                 = {English}
}

@Article{2006,
  Title                    = {Electron cyclotron microinstability in the foot of a perpendicular shock: {A} self-consistent {PIC} simulation},
  Journal                  = {Advances in Space Research},
  Year                     = {2006},
  Volume                   = {37},

  Doi                      = {10.1016/j.asr.2005.03.077}
}

@Book{1995,
  Year                     = {1995},
  Month                    = sep,

  Keywords                 = {User Manual},
  Language                 = {English},
  Url                      = {https://earth.esa.int/web/guest/document-library/-/asset_publisher/2Xho/content/gome-users-manual-4711?p_r_p_1690003576_shoppingCartItemRef=GEN186&p_r_p_1690003576_shoppingCartItemDescription=ENVISAT%20and%20ERS%20Missions%20Data%20Access%20Guide&}
}



==> future.tex <==
	%%%%%%%%%%%%
     %	\section{Future and ongoing research}
     	\begin{enumerate}
     		\item Magnetosphere-Ionosphere coupling (Code validated and tested)
     		\item Simulation of plasmasphere (Paper under preparations)
     		\item Simulate day-night, summer winter asymmetry of the magnetosphere
     		\item Include chemical reaction of species and exchange of charges in magnetosphere ionosphere coupling. 
     		\item Ionospheric ions outflow as a function of altitude upward to magnetosphere
     	\end{enumerate}
